The Voice on the Line

A transcriber listening through one microphone also hears everyone near it. We train causal voice isolators that keep only the caller for a speech recogniser: masking transformers with 20 ms of latency that enroll the caller from the call itself. Short evaluation windows hide two failures that real calls expose: forgetting the caller when another voice talks alone for a while, and damaging a caller who is alone. Long calls with turns, memory beyond the attention window and real headset crosstalk address the first, at a cost to the second. WavLM-Large's own weights, made causal and trained inside the model, move that trade, and training windows cut from longer calls remove most of a lone caller's cold start. The release (555M parameters) makes 16.13% word errors on 60 s AMI windows, against 23.66% for VoxLock, the strongest open isolator, and 14.77% on average over nine test sets, against 18.04%; it is level on Krisp's benchmark, and a caller who is alone still loses more words than with VoxLock. Distilled without WavLM into 22.1M and 9.8M parameters, it runs live on one CPU thread inside a LiveKit agent, at 12.5% and 8.5% of a core per call, with 10.66% and 10.99% error on our development sets (the release 10.49%). In an agent that talks back, noise interrupts it 0.54 times a minute of its speech behind our agent model, which gates its output on a caller-presence head, against 1.18 for VoxLock. We open-source the models, with a LiveKit plugin, at https://huggingface.co/collections/Scicom-intl/voice-isolator.

==> numbers.tex <==
% generated by make_tables.py from results/; do not edit
\makeatletter
\newcommand{\val}[1]{\ifcsname v@#1\endcsname\csname v@#1\endcsname\else\textbf{??}\PackageWarning{val}{undefined value #1}\fi}
\expandafter\def\csname v@abl/arch/SB_abs_k010/ami_dev/leak\endcsname{12.10}
\expandafter\def\csname v@abl/arch/SB_abs_k010/ami_dev/miss\endcsname{11.18}
\expandafter\def\csname v@abl/arch/SB_abs_k010/ami_dev/wer\endcsname{15.77}
\expandafter\def\csname v@abl/arch/SB_abs_k010/keepdb\endcsname{-0.99}
\expandafter\def\csname v@abl/arch/SB_abs_k010/krisp/leak\endcsname{11.62}
\expandafter\def\csname v@abl/arch/SB_abs_k010/krisp/miss\endcsname{5.72}
\expandafter\def\csname v@abl/arch/SB_abs_k010/krisp/wer\endcsname{9.48}
\expandafter\def\csname v@abl/arch/SB_abs_k010/leakdb\endcsname{-25.1}
\expandafter\def\csname v@abl/arch/SB_abs_k010/nsf_dev/leak\endcsname{0.47}
\expandafter\def\csname v@abl/arch/SB_abs_k010/nsf_dev/miss\endcsname{6.63}
\expandafter\def\csname v@abl/arch/SB_abs_k010/nsf_dev/wer\endcsname{8.40}
\expandafter\def\csname v@abl/arch/SB_abs_k010/null-sisdri\endcsname{2.95}
\expandafter\def\csname v@abl/arch/SB_abs_k010/sisdri\endcsname{3.85}
\expandafter\def\csname v@abl/arch/S_abs_k010/ami_dev/leak\endcsname{10.63}
\expandafter\def\csname v@abl/arch/S_abs_k010/ami_dev/miss\endcsname{11.12}
\expandafter\def\csname v@abl/arch/S_abs_k010/ami_dev/wer\endcsname{15.74}
\expandafter\def\csname v@abl/arch/S_abs_k010/keepdb\endcsname{-1.05}
\expandafter\def\csname v@abl/arch/S_abs_k010/krisp/leak\endcsname{14.94}
\expandafter\def\csname v@abl/arch/S_abs_k010/krisp/miss\endcsname{6.07}
\expandafter\def\csname v@abl/arch/S_abs_k010/krisp/wer\endcsname{10.60}
\expandafter\def\csname v@abl/arch/S_abs_k010/leakdb\endcsname{-25.2}
\expandafter\def\csname v@abl/arch/S_abs_k010/nsf_dev/leak\endcsname{0.43}
\expandafter\def\csname v@abl/arch/S_abs_k010/nsf_dev/miss\endcsname{6.45}
\expandafter\def\csname v@abl/arch/S_abs_k010/nsf_dev/wer\endcsname{8.14}
\expandafter\def\csname v@abl/arch/S_abs_k010/null-sisdri\endcsname{2.87}
\expandafter\def\csname v@abl/arch/S_abs_k010/sisdri\endcsname{3.61}
\expandafter\def\csname v@abl/aug/SB_base/ami_dev/leak\endcsname{9.24}
\expandafter\def\csname v@abl/aug/SB_base/ami_dev/miss\endcsname{12.96}
\expandafter\def\csname v@abl/aug/SB_base/ami_dev/wer\endcsname{16.29}
\expandafter\def\csname v@abl/aug/SB_base/keepdb\endcsname{-1.05}
\expandafter\def\csname v@abl/aug/SB_base/krisp/leak\endcsname{5.88}
\expandafter\def\csname v@abl/aug/SB_base/krisp/miss\endcsname{5.38}
\expandafter\def\csname v@abl/aug/SB_base/krisp/wer\endcsname{7.51}
\expandafter\def\csname v@abl/aug/SB_base/leakdb\endcsname{-31.6}
\expandafter\def\csname v@abl/aug/SB_base/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/aug/SB_base/nsf_dev/miss\endcsname{7.20}
\expandafter\def\csname v@abl/aug/SB_base/nsf_dev/wer\endcsname{8.97}
\expandafter\def\csname v@abl/aug/SB_base/null-sisdri\endcsname{4.29}
\expandafter\def\csname v@abl/aug/SB_base/sisdri\endcsname{5.41}
\expandafter\def\csname v@abl/aug/SB_dry/ami_dev/leak\endcsname{10.00}
\expandafter\def\csname v@abl/aug/SB_dry/ami_dev/miss\endcsname{18.06}
\expandafter\def\csname v@abl/aug/SB_dry/ami_dev/wer\endcsname{21.83}
\expandafter\def\csname v@abl/aug/SB_dry/keepdb\endcsname{-0.81}
\expandafter\def\csname v@abl/aug/SB_dry/krisp/leak\endcsname{19.81}
\expandafter\def\csname v@abl/aug/SB_dry/krisp/miss\endcsname{6.14}
\expandafter\def\csname v@abl/aug/SB_dry/krisp/wer\endcsname{11.45}
\expandafter\def\csname v@abl/aug/SB_dry/leakdb\endcsname{-24.2}
\expandafter\def\csname v@abl/aug/SB_dry/nsf_dev/leak\endcsname{0.26}
\expandafter\def\csname v@abl/aug/SB_dry/nsf_dev/miss\endcsname{7.05}
\expandafter\def\csname v@abl/aug/SB_dry/nsf_dev/wer\endcsname{8.71}
\expandafter\def\csname v@abl/aug/SB_dry/null-sisdri\endcsname{3.64}
\expandafter\def\csname v@abl/aug/SB_dry/sisdri\endcsname{4.75}
\expandafter\def\csname v@abl/aug/SB_nobgonly/ami_dev/leak\endcsname{9.46}
\expandafter\def\csname v@abl/aug/SB_nobgonly/ami_dev/miss\endcsname{15.29}
\expandafter\def\csname v@abl/aug/SB_nobgonly/ami_dev/wer\endcsname{18.63}
\expandafter\def\csname v@abl/aug/SB_nobgonly/keepdb\endcsname{-0.94}
\expandafter\def\csname v@abl/aug/SB_nobgonly/krisp/leak\endcsname{9.36}
\expandafter\def\csname v@abl/aug/SB_nobgonly/krisp/miss\endcsname{5.25}
\expandafter\def\csname v@abl/aug/SB_nobgonly/krisp/wer\endcsname{8.33}
\expandafter\def\csname v@abl/aug/SB_nobgonly/leakdb\endcsname{-31.2}
\expandafter\def\csname v@abl/aug/SB_nobgonly/nsf_dev/leak\endcsname{0.30}
\expandafter\def\csname v@abl/aug/SB_nobgonly/nsf_dev/miss\endcsname{7.02}
\expandafter\def\csname v@abl/aug/SB_nobgonly/nsf_dev/wer\endcsname{8.68}
\expandafter\def\csname v@abl/aug/SB_nobgonly/null-sisdri\endcsname{3.99}
\expandafter\def\csname v@abl/aug/SB_nobgonly/sisdri\endcsname{5.46}
\expandafter\def\csname v@abl/aug/SB_nocross/ami_dev/leak\endcsname{58.62}
\expandafter\def\csname v@abl/aug/SB_nocross/ami_dev/miss\endcsname{9.11}
\expandafter\def\csname v@abl/aug/SB_nocross/ami_dev/wer\endcsname{29.84}
\expandafter\def\csname v@abl/aug/SB_nocross/keepdb\endcsname{0.18}
\expandafter\def\csname v@abl/aug/SB_nocross/krisp/leak\endcsname{27.04}
\expandafter\def\csname v@abl/aug/SB_nocross/krisp/miss\endcsname{5.02}
\expandafter\def\csname v@abl/aug/SB_nocross/krisp/wer\endcsname{12.75}
\expandafter\def\csname v@abl/aug/SB_nocross/leakdb\endcsname{-10.7}
\expandafter\def\csname v@abl/aug/SB_nocross/nsf_dev/leak\endcsname{0.47}
\expandafter\def\csname v@abl/aug/SB_nocross/nsf_dev/miss\endcsname{6.05}
\expandafter\def\csname v@abl/aug/SB_nocross/nsf_dev/wer\endcsname{7.85}
\expandafter\def\csname v@abl/aug/SB_nocross/null-sisdri\endcsname{3.15}
\expandafter\def\csname v@abl/aug/SB_nocross/sisdri\endcsname{3.29}
\expandafter\def\csname v@abl/aug/SB_noline/ami_dev/leak\endcsname{7.46}
\expandafter\def\csname v@abl/aug/SB_noline/ami_dev/miss\endcsname{12.68}
\expandafter\def\csname v@abl/aug/SB_noline/ami_dev/wer\endcsname{15.95}
\expandafter\def\csname v@abl/aug/SB_noline/keepdb\endcsname{-4.49}
\expandafter\def\csname v@abl/aug/SB_noline/krisp/leak\endcsname{7.59}
\expandafter\def\csname v@abl/aug/SB_noline/krisp/miss\endcsname{6.14}
\expandafter\def\csname v@abl/aug/SB_noline/krisp/wer\endcsname{8.81}
\expandafter\def\csname v@abl/aug/SB_noline/leakdb\endcsname{-34.6}
\expandafter\def\csname v@abl/aug/SB_noline/nsf_dev/leak\endcsname{0.26}
\expandafter\def\csname v@abl/aug/SB_noline/nsf_dev/miss\endcsname{7.00}
\expandafter\def\csname v@abl/aug/SB_noline/nsf_dev/wer\endcsname{8.73}
\expandafter\def\csname v@abl/aug/SB_noline/null-sisdri\endcsname{2.70}
\expandafter\def\csname v@abl/aug/SB_noline/sisdri\endcsname{3.13}
\expandafter\def\csname v@abl/aug/SB_nonoise/ami_dev/leak\endcsname{9.51}
\expandafter\def\csname v@abl/aug/SB_nonoise/ami_dev/miss\endcsname{29.28}
\expandafter\def\csname v@abl/aug/SB_nonoise/ami_dev/wer\endcsname{31.41}
\expandafter\def\csname v@abl/aug/SB_nonoise/keepdb\endcsname{-1.05}
\expandafter\def\csname v@abl/aug/SB_nonoise/krisp/leak\endcsname{8.51}
\expandafter\def\csname v@abl/aug/SB_nonoise/krisp/miss\endcsname{6.68}
\expandafter\def\csname v@abl/aug/SB_nonoise/krisp/wer\endcsname{9.51}
\expandafter\def\csname v@abl/aug/SB_nonoise/leakdb\endcsname{-26.5}
\expandafter\def\csname v@abl/aug/SB_nonoise/nsf_dev/leak\endcsname{0.64}
\expandafter\def\csname v@abl/aug/SB_nonoise/nsf_dev/miss\endcsname{17.74}
\expandafter\def\csname v@abl/aug/SB_nonoise/nsf_dev/wer\endcsname{19.34}
\expandafter\def\csname v@abl/aug/SB_nonoise/null-sisdri\endcsname{2.40}
\expandafter\def\csname v@abl/aug/SB_nonoise/sisdri\endcsname{4.09}
\expandafter\def\csname v@abl/data/SB_base/ami_dev/leak\endcsname{9.24}
\expandafter\def\csname v@abl/data/SB_base/ami_dev/miss\endcsname{12.96}
\expandafter\def\csname v@abl/data/SB_base/ami_dev/wer\endcsname{16.29}
\expandafter\def\csname v@abl/data/SB_base/keepdb\endcsname{-1.05}
\expandafter\def\csname v@abl/data/SB_base/krisp/leak\endcsname{5.88}
\expandafter\def\csname v@abl/data/SB_base/krisp/miss\endcsname{5.38}
\expandafter\def\csname v@abl/data/SB_base/krisp/wer\endcsname{7.51}
\expandafter\def\csname v@abl/data/SB_base/leakdb\endcsname{-31.6}
\expandafter\def\csname v@abl/data/SB_base/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/data/SB_base/nsf_dev/miss\endcsname{7.20}
\expandafter\def\csname v@abl/data/SB_base/nsf_dev/wer\endcsname{8.97}
\expandafter\def\csname v@abl/data/SB_base/null-sisdri\endcsname{4.29}
\expandafter\def\csname v@abl/data/SB_base/sisdri\endcsname{5.41}
\expandafter\def\csname v@abl/data/SB_english/ami_dev/leak\endcsname{8.79}
\expandafter\def\csname v@abl/data/SB_english/ami_dev/miss\endcsname{10.72}
\expandafter\def\csname v@abl/data/SB_english/ami_dev/wer\endcsname{14.57}
\expandafter\def\csname v@abl/data/SB_english/keepdb\endcsname{-1.18}
\expandafter\def\csname v@abl/data/SB_english/krisp/leak\endcsname{8.37}
\expandafter\def\csname v@abl/data/SB_english/krisp/miss\endcsname{5.60}
\expandafter\def\csname v@abl/data/SB_english/krisp/wer\endcsname{8.44}
\expandafter\def\csname v@abl/data/SB_english/leakdb\endcsname{-28.0}
\expandafter\def\csname v@abl/data/SB_english/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/data/SB_english/nsf_dev/miss\endcsname{6.49}
\expandafter\def\csname v@abl/data/SB_english/nsf_dev/wer\endcsname{8.18}
\expandafter\def\csname v@abl/data/SB_english/null-sisdri\endcsname{3.79}
\expandafter\def\csname v@abl/data/SB_english/sisdri\endcsname{4.68}
\expandafter\def\csname v@abl/data/SB_libri/ami_dev/leak\endcsname{7.81}
\expandafter\def\csname v@abl/data/SB_libri/ami_dev/miss\endcsname{12.97}
\expandafter\def\csname v@abl/data/SB_libri/ami_dev/wer\endcsname{16.26}
\expandafter\def\csname v@abl/data/SB_libri/keepdb\endcsname{-1.14}
\expandafter\def\csname v@abl/data/SB_libri/krisp/leak\endcsname{6.28}
\expandafter\def\csname v@abl/data/SB_libri/krisp/miss\endcsname{6.02}
\expandafter\def\csname v@abl/data/SB_libri/krisp/wer\endcsname{8.23}
\expandafter\def\csname v@abl/data/SB_libri/leakdb\endcsname{-28.6}
\expandafter\def\csname v@abl/data/SB_libri/nsf_dev/leak\endcsname{0.51}
\expandafter\def\csname v@abl/data/SB_libri/nsf_dev/miss\endcsname{6.66}
\expandafter\def\csname v@abl/data/SB_libri/nsf_dev/wer\endcsname{8.43}
\expandafter\def\csname v@abl/data/SB_libri/null-sisdri\endcsname{3.50}
\expandafter\def\csname v@abl/data/SB_libri/sisdri\endcsname{4.91}
\expandafter\def\csname v@abl/data/SB_norestored/ami_dev/leak\endcsname{7.68}
\expandafter\def\csname v@abl/data/SB_norestored/ami_dev/miss\endcsname{10.90}
\expandafter\def\csname v@abl/data/SB_norestored/ami_dev/wer\endcsname{14.52}
\expandafter\def\csname v@abl/data/SB_norestored/keepdb\endcsname{-1.06}
\expandafter\def\csname v@abl/data/SB_norestored/krisp/leak\endcsname{7.56}
\expandafter\def\csname v@abl/data/SB_norestored/krisp/miss\endcsname{5.63}
\expandafter\def\csname v@abl/data/SB_norestored/krisp/wer\endcsname{8.01}
\expandafter\def\csname v@abl/data/SB_norestored/leakdb\endcsname{-30.4}
\expandafter\def\csname v@abl/data/SB_norestored/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/data/SB_norestored/nsf_dev/miss\endcsname{6.20}
\expandafter\def\csname v@abl/data/SB_norestored/nsf_dev/wer\endcsname{7.99}
\expandafter\def\csname v@abl/data/SB_norestored/null-sisdri\endcsname{4.59}
\expandafter\def\csname v@abl/data/SB_norestored/sisdri\endcsname{5.50}
\expandafter\def\csname v@abl/enr/SB_base/ami_dev/leak\endcsname{9.24}
\expandafter\def\csname v@abl/enr/SB_base/ami_dev/miss\endcsname{12.96}
\expandafter\def\csname v@abl/enr/SB_base/ami_dev/wer\endcsname{16.29}
\expandafter\def\csname v@abl/enr/SB_base/keepdb\endcsname{-1.05}
\expandafter\def\csname v@abl/enr/SB_base/krisp/leak\endcsname{5.88}
\expandafter\def\csname v@abl/enr/SB_base/krisp/miss\endcsname{5.38}
\expandafter\def\csname v@abl/enr/SB_base/krisp/wer\endcsname{7.51}
\expandafter\def\csname v@abl/enr/SB_base/leakdb\endcsname{-31.6}
\expandafter\def\csname v@abl/enr/SB_base/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/enr/SB_base/nsf_dev/miss\endcsname{7.20}
\expandafter\def\csname v@abl/enr/SB_base/nsf_dev/wer\endcsname{8.97}
\expandafter\def\csname v@abl/enr/SB_base/null-sisdri\endcsname{4.29}
\expandafter\def\csname v@abl/enr/SB_base/sisdri\endcsname{5.41}
\expandafter\def\csname v@abl/enr/SB_noenroll/ami_dev/leak\endcsname{8.04}
\expandafter\def\csname v@abl/enr/SB_noenroll/ami_dev/miss\endcsname{10.85}
\expandafter\def\csname v@abl/enr/SB_noenroll/ami_dev/wer\endcsname{14.59}
\expandafter\def\csname v@abl/enr/SB_noenroll/keepdb\endcsname{-1.18}
\expandafter\def\csname v@abl/enr/SB_noenroll/krisp/leak\endcsname{19.03}
\expandafter\def\csname v@abl/enr/SB_noenroll/krisp/miss\endcsname{6.21}
\expandafter\def\csname v@abl/enr/SB_noenroll/krisp/wer\endcsname{11.93}
\expandafter\def\csname v@abl/enr/SB_noenroll/leakdb\endcsname{-26.2}
\expandafter\def\csname v@abl/enr/SB_noenroll/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/enr/SB_noenroll/nsf_dev/miss\endcsname{6.35}
\expandafter\def\csname v@abl/enr/SB_noenroll/nsf_dev/wer\endcsname{8.06}
\expandafter\def\csname v@abl/enr/SB_noenroll/null-sisdri\endcsname{4.28}
\expandafter\def\csname v@abl/enr/SB_noenroll/sisdri\endcsname{4.28}
\expandafter\def\csname v@abl/keep/SB_base/ami_dev/leak\endcsname{9.24}
\expandafter\def\csname v@abl/keep/SB_base/ami_dev/miss\endcsname{12.96}
\expandafter\def\csname v@abl/keep/SB_base/ami_dev/wer\endcsname{16.29}
\expandafter\def\csname v@abl/keep/SB_base/keepdb\endcsname{-1.05}
\expandafter\def\csname v@abl/keep/SB_base/krisp/leak\endcsname{5.88}
\expandafter\def\csname v@abl/keep/SB_base/krisp/miss\endcsname{5.38}
\expandafter\def\csname v@abl/keep/SB_base/krisp/wer\endcsname{7.51}
\expandafter\def\csname v@abl/keep/SB_base/leakdb\endcsname{-31.6}
\expandafter\def\csname v@abl/keep/SB_base/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/keep/SB_base/nsf_dev/miss\endcsname{7.20}
\expandafter\def\csname v@abl/keep/SB_base/nsf_dev/wer\endcsname{8.97}
\expandafter\def\csname v@abl/keep/SB_base/null-sisdri\endcsname{4.29}
\expandafter\def\csname v@abl/keep/SB_base/sisdri\endcsname{5.41}
\expandafter\def\csname v@abl/keep/SB_keep/ami_dev/leak\endcsname{13.08}
\expandafter\def\csname v@abl/keep/SB_keep/ami_dev/miss\endcsname{9.90}
\expandafter\def\csname v@abl/keep/SB_keep/ami_dev/wer\endcsname{15.47}
\expandafter\def\csname v@abl/keep/SB_keep/keepdb\endcsname{-0.24}
\expandafter\def\csname v@abl/keep/SB_keep/krisp/leak\endcsname{13.28}
\expandafter\def\csname v@abl/keep/SB_keep/krisp/miss\endcsname{4.53}
\expandafter\def\csname v@abl/keep/SB_keep/krisp/wer\endcsname{8.63}
\expandafter\def\csname v@abl/keep/SB_keep/leakdb\endcsname{-12.5}
\expandafter\def\csname v@abl/keep/SB_keep/nsf_dev/leak\endcsname{13.33}
\expandafter\def\csname v@abl/keep/SB_keep/nsf_dev/miss\endcsname{6.27}
\expandafter\def\csname v@abl/keep/SB_keep/nsf_dev/wer\endcsname{11.93}
\expandafter\def\csname v@abl/keep/SB_keep/null-sisdri\endcsname{4.59}
\expandafter\def\csname v@abl/keep/SB_keep/sisdri\endcsname{5.55}
\expandafter\def\csname v@abl/long/LC_seg24/ami_dev/leak\endcsname{10.36}
\expandafter\def\csname v@abl/long/LC_seg24/ami_dev/miss\endcsname{9.82}
\expandafter\def\csname v@abl/long/LC_seg24/ami_dev/wer\endcsname{14.68}
\expandafter\def\csname v@abl/long/LC_seg24/ami_dev_long/leak\endcsname{14.18}
\expandafter\def\csname v@abl/long/LC_seg24/ami_dev_long/miss\endcsname{21.37}
\expandafter\def\csname v@abl/long/LC_seg24/ami_dev_long/wer\endcsname{30.34}
\expandafter\def\csname v@abl/long/LC_seg24/keepdb\endcsname{-1.19}
\expandafter\def\csname v@abl/long/LC_seg24/krisp/leak\endcsname{1.89}
\expandafter\def\csname v@abl/long/LC_seg24/krisp/miss\endcsname{5.57}
\expandafter\def\csname v@abl/long/LC_seg24/krisp/wer\endcsname{6.73}
\expandafter\def\csname v@abl/long/LC_seg24/leakdb\endcsname{-19.4}
\expandafter\def\csname v@abl/long/LC_seg24/nsf_dev/leak\endcsname{0.55}
\expandafter\def\csname v@abl/long/LC_seg24/nsf_dev/miss\endcsname{5.91}
\expandafter\def\csname v@abl/long/LC_seg24/nsf_dev/wer\endcsname{7.75}
\expandafter\def\csname v@abl/long/LC_seg24/null-sisdri\endcsname{3.26}
\expandafter\def\csname v@abl/long/LC_seg24/sisdri\endcsname{3.86}
\expandafter\def\csname v@abl/long/LC_turns/ami_dev/leak\endcsname{8.53}
\expandafter\def\csname v@abl/long/LC_turns/ami_dev/miss\endcsname{11.44}
\expandafter\def\csname v@abl/long/LC_turns/ami_dev/wer\endcsname{15.22}
\expandafter\def\csname v@abl/long/LC_turns/ami_dev_long/leak\endcsname{16.33}
\expandafter\def\csname v@abl/long/LC_turns/ami_dev_long/miss\endcsname{16.97}
\expandafter\def\csname v@abl/long/LC_turns/ami_dev_long/wer\endcsname{27.28}
\expandafter\def\csname v@abl/long/LC_turns/keepdb\endcsname{-2.45}
\expandafter\def\csname v@abl/long/LC_turns/krisp/leak\endcsname{2.39}
\expandafter\def\csname v@abl/long/LC_turns/krisp/miss\endcsname{5.42}
\expandafter\def\csname v@abl/long/LC_turns/krisp/wer\endcsname{6.70}
\expandafter\def\csname v@abl/long/LC_turns/leakdb\endcsname{-26.0}
\expandafter\def\csname v@abl/long/LC_turns/nsf_dev/leak\endcsname{0.72}
\expandafter\def\csname v@abl/long/LC_turns/nsf_dev/miss\endcsname{6.27}
\expandafter\def\csname v@abl/long/LC_turns/nsf_dev/wer\endcsname{8.12}
\expandafter\def\csname v@abl/long/LC_turns/null-sisdri\endcsname{2.24}
\expandafter\def\csname v@abl/long/LC_turns/sisdri\endcsname{3.11}
\expandafter\def\csname v@abl/long/LC_turns_mem/ami_dev/leak\endcsname{7.86}
\expandafter\def\csname v@abl/long/LC_turns_mem/ami_dev/miss\endcsname{10.85}
\expandafter\def\csname v@abl/long/LC_turns_mem/ami_dev/wer\endcsname{14.52}
\expandafter\def\csname v@abl/long/LC_turns_mem/ami_dev_long/leak\endcsname{14.92}
\expandafter\def\csname v@abl/long/LC_turns_mem/ami_dev_long/miss\endcsname{16.51}
\expandafter\def\csname v@abl/long/LC_turns_mem/ami_dev_long/wer\endcsname{25.94}
\expandafter\def\csname v@abl/long/LC_turns_mem/keepdb\endcsname{-2.24}
\expandafter\def\csname v@abl/long/LC_turns_mem/krisp/leak\endcsname{0.68}
\expandafter\def\csname v@abl/long/LC_turns_mem/krisp/miss\endcsname{7.51}
\expandafter\def\csname v@abl/long/LC_turns_mem/krisp/wer\endcsname{8.36}
\expandafter\def\csname v@abl/long/LC_turns_mem/leakdb\endcsname{-25.7}
\expandafter\def\csname v@abl/long/LC_turns_mem/nsf_dev/leak\endcsname{0.51}
\expandafter\def\csname v@abl/long/LC_turns_mem/nsf_dev/miss\endcsname{5.98}
\expandafter\def\csname v@abl/long/LC_turns_mem/nsf_dev/wer\endcsname{7.76}
\expandafter\def\csname v@abl/long/LC_turns_mem/null-sisdri\endcsname{2.17}
\expandafter\def\csname v@abl/long/LC_turns_mem/sisdri\endcsname{3.18}
\expandafter\def\csname v@abl/long/LC_turns_mem4/ami_dev/leak\endcsname{8.39}
\expandafter\def\csname v@abl/long/LC_turns_mem4/ami_dev/miss\endcsname{10.75}
\expandafter\def\csname v@abl/long/LC_turns_mem4/ami_dev/wer\endcsname{14.84}
\expandafter\def\csname v@abl/long/LC_turns_mem4/ami_dev_long/leak\endcsname{14.94}
\expandafter\def\csname v@abl/long/LC_turns_mem4/ami_dev_long/miss\endcsname{17.31}
\expandafter\def\csname v@abl/long/LC_turns_mem4/ami_dev_long/wer\endcsname{26.73}
\expandafter\def\csname v@abl/long/LC_turns_mem4/keepdb\endcsname{-2.27}
\expandafter\def\csname v@abl/long/LC_turns_mem4/krisp/leak\endcsname{0.76}
\expandafter\def\csname v@abl/long/LC_turns_mem4/krisp/miss\endcsname{6.06}
\expandafter\def\csname v@abl/long/LC_turns_mem4/krisp/wer\endcsname{6.89}
\expandafter\def\csname v@abl/long/LC_turns_mem4/leakdb\endcsname{-25.8}
\expandafter\def\csname v@abl/long/LC_turns_mem4/nsf_dev/leak\endcsname{0.47}
\expandafter\def\csname v@abl/long/LC_turns_mem4/nsf_dev/miss\endcsname{6.06}
\expandafter\def\csname v@abl/long/LC_turns_mem4/nsf_dev/wer\endcsname{7.83}
\expandafter\def\csname v@abl/long/LC_turns_mem4/null-sisdri\endcsname{2.33}
\expandafter\def\csname v@abl/long/LC_turns_mem4/sisdri\endcsname{3.12}
\expandafter\def\csname v@abl/long/LC_turns_w1k/ami_dev/leak\endcsname{7.32}
\expandafter\def\csname v@abl/long/LC_turns_w1k/ami_dev/miss\endcsname{11.25}
\expandafter\def\csname v@abl/long/LC_turns_w1k/ami_dev/wer\endcsname{14.79}
\expandafter\def\csname v@abl/long/LC_turns_w1k/ami_dev_long/leak\endcsname{10.97}
\expandafter\def\csname v@abl/long/LC_turns_w1k/ami_dev_long/miss\endcsname{19.12}
\expandafter\def\csname v@abl/long/LC_turns_w1k/ami_dev_long/wer\endcsname{25.81}
\expandafter\def\csname v@abl/long/LC_turns_w1k/keepdb\endcsname{-1.91}
\expandafter\def\csname v@abl/long/LC_turns_w1k/krisp/leak\endcsname{0.25}
\expandafter\def\csname v@abl/long/LC_turns_w1k/krisp/miss\endcsname{7.88}
\expandafter\def\csname v@abl/long/LC_turns_w1k/krisp/wer\endcsname{8.63}
\expandafter\def\csname v@abl/long/LC_turns_w1k/leakdb\endcsname{-25.4}
\expandafter\def\csname v@abl/long/LC_turns_w1k/nsf_dev/leak\endcsname{0.43}
\expandafter\def\csname v@abl/long/LC_turns_w1k/nsf_dev/miss\endcsname{6.25}
\expandafter\def\csname v@abl/long/LC_turns_w1k/nsf_dev/wer\endcsname{7.96}
\expandafter\def\csname v@abl/long/LC_turns_w1k/null-sisdri\endcsname{2.68}
\expandafter\def\csname v@abl/long/LC_turns_w1k/sisdri\endcsname{3.51}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/ami_dev/leak\endcsname{7.14}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/ami_dev/miss\endcsname{10.89}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/ami_dev/wer\endcsname{14.45}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/ami_dev_long/leak\endcsname{9.89}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/ami_dev_long/miss\endcsname{18.10}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/ami_dev_long/wer\endcsname{23.91}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/keepdb\endcsname{-1.92}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/krisp/leak\endcsname{0.43}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/krisp/miss\endcsname{5.84}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/krisp/wer\endcsname{6.64}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/leakdb\endcsname{-25.7}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/nsf_dev/miss\endcsname{6.27}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/nsf_dev/wer\endcsname{7.93}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/null-sisdri\endcsname{2.44}
\expandafter\def\csname v@abl/long/LC_turns_w1k_mem/sisdri\endcsname{3.54}
\expandafter\def\csname v@abl/long/ftlb_off/ami_dev/leak\endcsname{9.78}
\expandafter\def\csname v@abl/long/ftlb_off/ami_dev/miss\endcsname{11.50}
\expandafter\def\csname v@abl/long/ftlb_off/ami_dev/wer\endcsname{15.47}
\expandafter\def\csname v@abl/long/ftlb_off/ami_dev_long/leak\endcsname{41.98}
\expandafter\def\csname v@abl/long/ftlb_off/ami_dev_long/miss\endcsname{14.73}
\expandafter\def\csname v@abl/long/ftlb_off/ami_dev_long/wer\endcsname{46.70}
\expandafter\def\csname v@abl/long/ftlb_off/keepdb\endcsname{-1.14}
\expandafter\def\csname v@abl/long/ftlb_off/krisp/leak\endcsname{11.81}
\expandafter\def\csname v@abl/long/ftlb_off/krisp/miss\endcsname{5.69}
\expandafter\def\csname v@abl/long/ftlb_off/krisp/wer\endcsname{9.41}
\expandafter\def\csname v@abl/long/ftlb_off/leakdb\endcsname{-27.0}
\expandafter\def\csname v@abl/long/ftlb_off/nsf_dev/leak\endcsname{0.47}
\expandafter\def\csname v@abl/long/ftlb_off/nsf_dev/miss\endcsname{6.70}
\expandafter\def\csname v@abl/long/ftlb_off/nsf_dev/wer\endcsname{8.39}
\expandafter\def\csname v@abl/long/ftlb_off/null-sisdri\endcsname{3.13}
\expandafter\def\csname v@abl/long/ftlb_off/sisdri\endcsname{4.26}
\expandafter\def\csname v@abl/long/ftlb_on/ami_dev/leak\endcsname{7.32}
\expandafter\def\csname v@abl/long/ftlb_on/ami_dev/miss\endcsname{12.60}
\expandafter\def\csname v@abl/long/ftlb_on/ami_dev/wer\endcsname{15.86}
\expandafter\def\csname v@abl/long/ftlb_on/ami_dev_long/leak\endcsname{33.59}
\expandafter\def\csname v@abl/long/ftlb_on/ami_dev_long/miss\endcsname{15.18}
\expandafter\def\csname v@abl/long/ftlb_on/ami_dev_long/wer\endcsname{40.08}
\expandafter\def\csname v@abl/long/ftlb_on/keepdb\endcsname{-1.36}
\expandafter\def\csname v@abl/long/ftlb_on/krisp/leak\endcsname{7.51}
\expandafter\def\csname v@abl/long/ftlb_on/krisp/miss\endcsname{9.05}
\expandafter\def\csname v@abl/long/ftlb_on/krisp/wer\endcsname{11.62}
\expandafter\def\csname v@abl/long/ftlb_on/leakdb\endcsname{-28.0}
\expandafter\def\csname v@abl/long/ftlb_on/nsf_dev/leak\endcsname{0.55}
\expandafter\def\csname v@abl/long/ftlb_on/nsf_dev/miss\endcsname{9.12}
\expandafter\def\csname v@abl/long/ftlb_on/nsf_dev/wer\endcsname{10.68}
\expandafter\def\csname v@abl/long/ftlb_on/null-sisdri\endcsname{2.60}
\expandafter\def\csname v@abl/long/ftlb_on/sisdri\endcsname{3.64}
\expandafter\def\csname v@abl/loss/SB_abs/ami_dev/leak\endcsname{8.53}
\expandafter\def\csname v@abl/loss/SB_abs/ami_dev/miss\endcsname{12.83}
\expandafter\def\csname v@abl/loss/SB_abs/ami_dev/wer\endcsname{16.51}
\expandafter\def\csname v@abl/loss/SB_abs/keepdb\endcsname{-1.14}
\expandafter\def\csname v@abl/loss/SB_abs/krisp/leak\endcsname{9.28}
\expandafter\def\csname v@abl/loss/SB_abs/krisp/miss\endcsname{5.57}
\expandafter\def\csname v@abl/loss/SB_abs/krisp/wer\endcsname{8.71}
\expandafter\def\csname v@abl/loss/SB_abs/leakdb\endcsname{-32.9}
\expandafter\def\csname v@abl/loss/SB_abs/nsf_dev/leak\endcsname{0.34}
\expandafter\def\csname v@abl/loss/SB_abs/nsf_dev/miss\endcsname{6.61}
\expandafter\def\csname v@abl/loss/SB_abs/nsf_dev/wer\endcsname{8.29}
\expandafter\def\csname v@abl/loss/SB_abs/null-sisdri\endcsname{4.19}
\expandafter\def\csname v@abl/loss/SB_abs/sisdri\endcsname{5.51}
\expandafter\def\csname v@abl/loss/SB_base/ami_dev/leak\endcsname{9.24}
\expandafter\def\csname v@abl/loss/SB_base/ami_dev/miss\endcsname{12.96}
\expandafter\def\csname v@abl/loss/SB_base/ami_dev/wer\endcsname{16.29}
\expandafter\def\csname v@abl/loss/SB_base/keepdb\endcsname{-1.05}
\expandafter\def\csname v@abl/loss/SB_base/krisp/leak\endcsname{5.88}
\expandafter\def\csname v@abl/loss/SB_base/krisp/miss\endcsname{5.38}
\expandafter\def\csname v@abl/loss/SB_base/krisp/wer\endcsname{7.51}
\expandafter\def\csname v@abl/loss/SB_base/leakdb\endcsname{-31.6}
\expandafter\def\csname v@abl/loss/SB_base/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/loss/SB_base/nsf_dev/miss\endcsname{7.20}
\expandafter\def\csname v@abl/loss/SB_base/nsf_dev/wer\endcsname{8.97}
\expandafter\def\csname v@abl/loss/SB_base/null-sisdri\endcsname{4.29}
\expandafter\def\csname v@abl/loss/SB_base/sisdri\endcsname{5.41}
\expandafter\def\csname v@abl/loss/SB_snr/ami_dev/leak\endcsname{32.37}
\expandafter\def\csname v@abl/loss/SB_snr/ami_dev/miss\endcsname{9.49}
\expandafter\def\csname v@abl/loss/SB_snr/ami_dev/wer\endcsname{21.10}
\expandafter\def\csname v@abl/loss/SB_snr/keepdb\endcsname{-0.79}
\expandafter\def\csname v@abl/loss/SB_snr/krisp/leak\endcsname{10.16}
\expandafter\def\csname v@abl/loss/SB_snr/krisp/miss\endcsname{4.14}
\expandafter\def\csname v@abl/loss/SB_snr/krisp/wer\endcsname{7.50}
\expandafter\def\csname v@abl/loss/SB_snr/leakdb\endcsname{-18.9}
\expandafter\def\csname v@abl/loss/SB_snr/nsf_dev/leak\endcsname{21.56}
\expandafter\def\csname v@abl/loss/SB_snr/nsf_dev/miss\endcsname{6.42}
\expandafter\def\csname v@abl/loss/SB_snr/nsf_dev/wer\endcsname{14.42}
\expandafter\def\csname v@abl/loss/SB_snr/null-sisdri\endcsname{4.99}
\expandafter\def\csname v@abl/loss/SB_snr/sisdri\endcsname{6.06}
\expandafter\def\csname v@abl/loss/SB_spec/ami_dev/leak\endcsname{12.77}
\expandafter\def\csname v@abl/loss/SB_spec/ami_dev/miss\endcsname{11.00}
\expandafter\def\csname v@abl/loss/SB_spec/ami_dev/wer\endcsname{16.33}
\expandafter\def\csname v@abl/loss/SB_spec/keepdb\endcsname{-0.85}
\expandafter\def\csname v@abl/loss/SB_spec/krisp/leak\endcsname{9.71}
\expandafter\def\csname v@abl/loss/SB_spec/krisp/miss\endcsname{4.34}
\expandafter\def\csname v@abl/loss/SB_spec/krisp/wer\endcsname{7.58}
\expandafter\def\csname v@abl/loss/SB_spec/leakdb\endcsname{-19.7}
\expandafter\def\csname v@abl/loss/SB_spec/nsf_dev/leak\endcsname{3.15}
\expandafter\def\csname v@abl/loss/SB_spec/nsf_dev/miss\endcsname{6.16}
\expandafter\def\csname v@abl/loss/SB_spec/nsf_dev/wer\endcsname{8.73}
\expandafter\def\csname v@abl/loss/SB_spec/null-sisdri\endcsname{4.81}
\expandafter\def\csname v@abl/loss/SB_spec/sisdri\endcsname{5.98}
\expandafter\def\csname v@abl/real/SB_base/ami_dev/leak\endcsname{9.24}
\expandafter\def\csname v@abl/real/SB_base/ami_dev/miss\endcsname{12.96}
\expandafter\def\csname v@abl/real/SB_base/ami_dev/wer\endcsname{16.29}
\expandafter\def\csname v@abl/real/SB_base/keepdb\endcsname{-1.05}
\expandafter\def\csname v@abl/real/SB_base/krisp/leak\endcsname{5.88}
\expandafter\def\csname v@abl/real/SB_base/krisp/miss\endcsname{5.38}
\expandafter\def\csname v@abl/real/SB_base/krisp/wer\endcsname{7.51}
\expandafter\def\csname v@abl/real/SB_base/leakdb\endcsname{-31.6}
\expandafter\def\csname v@abl/real/SB_base/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/real/SB_base/nsf_dev/miss\endcsname{7.20}
\expandafter\def\csname v@abl/real/SB_base/nsf_dev/wer\endcsname{8.97}
\expandafter\def\csname v@abl/real/SB_base/null-sisdri\endcsname{4.29}
\expandafter\def\csname v@abl/real/SB_base/sisdri\endcsname{5.41}
\expandafter\def\csname v@abl/real/SB_real/ami_dev/leak\endcsname{11.56}
\expandafter\def\csname v@abl/real/SB_real/ami_dev/miss\endcsname{9.95}
\expandafter\def\csname v@abl/real/SB_real/ami_dev/wer\endcsname{14.58}
\expandafter\def\csname v@abl/real/SB_real/keepdb\endcsname{-1.09}
\expandafter\def\csname v@abl/real/SB_real/krisp/leak\endcsname{10.78}
\expandafter\def\csname v@abl/real/SB_real/krisp/miss\endcsname{5.00}
\expandafter\def\csname v@abl/real/SB_real/krisp/wer\endcsname{8.48}
\expandafter\def\csname v@abl/real/SB_real/leakdb\endcsname{-29.5}
\expandafter\def\csname v@abl/real/SB_real/nsf_dev/leak\endcsname{0.85}
\expandafter\def\csname v@abl/real/SB_real/nsf_dev/miss\endcsname{6.04}
\expandafter\def\csname v@abl/real/SB_real/nsf_dev/wer\endcsname{8.05}
\expandafter\def\csname v@abl/real/SB_real/null-sisdri\endcsname{3.54}
\expandafter\def\csname v@abl/real/SB_real/sisdri\endcsname{4.60}
\expandafter\def\csname v@abl/scale/LB_main/ami_dev/leak\endcsname{8.13}
\expandafter\def\csname v@abl/scale/LB_main/ami_dev/miss\endcsname{11.86}
\expandafter\def\csname v@abl/scale/LB_main/ami_dev/wer\endcsname{15.31}
\expandafter\def\csname v@abl/scale/LB_main/keepdb\endcsname{-1.32}
\expandafter\def\csname v@abl/scale/LB_main/krisp/leak\endcsname{11.01}
\expandafter\def\csname v@abl/scale/LB_main/krisp/miss\endcsname{5.55}
\expandafter\def\csname v@abl/scale/LB_main/krisp/wer\endcsname{8.93}
\expandafter\def\csname v@abl/scale/LB_main/leakdb\endcsname{-30.4}
\expandafter\def\csname v@abl/scale/LB_main/nsf_dev/leak\endcsname{0.26}
\expandafter\def\csname v@abl/scale/LB_main/nsf_dev/miss\endcsname{6.73}
\expandafter\def\csname v@abl/scale/LB_main/nsf_dev/wer\endcsname{8.48}
\expandafter\def\csname v@abl/scale/LB_main/null-sisdri\endcsname{3.80}
\expandafter\def\csname v@abl/scale/LB_main/sisdri\endcsname{5.04}
\expandafter\def\csname v@abl/scale/MB_main/ami_dev/leak\endcsname{7.90}
\expandafter\def\csname v@abl/scale/MB_main/ami_dev/miss\endcsname{13.79}
\expandafter\def\csname v@abl/scale/MB_main/ami_dev/wer\endcsname{16.87}
\expandafter\def\csname v@abl/scale/MB_main/keepdb\endcsname{-1.19}
\expandafter\def\csname v@abl/scale/MB_main/krisp/leak\endcsname{5.65}
\expandafter\def\csname v@abl/scale/MB_main/krisp/miss\endcsname{5.27}
\expandafter\def\csname v@abl/scale/MB_main/krisp/wer\endcsname{7.38}
\expandafter\def\csname v@abl/scale/MB_main/leakdb\endcsname{-32.2}
\expandafter\def\csname v@abl/scale/MB_main/nsf_dev/leak\endcsname{0.30}
\expandafter\def\csname v@abl/scale/MB_main/nsf_dev/miss\endcsname{6.66}
\expandafter\def\csname v@abl/scale/MB_main/nsf_dev/wer\endcsname{8.36}
\expandafter\def\csname v@abl/scale/MB_main/null-sisdri\endcsname{3.90}
\expandafter\def\csname v@abl/scale/MB_main/sisdri\endcsname{5.30}
\expandafter\def\csname v@abl/scale/SB_base/ami_dev/leak\endcsname{9.24}
\expandafter\def\csname v@abl/scale/SB_base/ami_dev/miss\endcsname{12.96}
\expandafter\def\csname v@abl/scale/SB_base/ami_dev/wer\endcsname{16.29}
\expandafter\def\csname v@abl/scale/SB_base/keepdb\endcsname{-1.05}
\expandafter\def\csname v@abl/scale/SB_base/krisp/leak\endcsname{5.88}
\expandafter\def\csname v@abl/scale/SB_base/krisp/miss\endcsname{5.38}
\expandafter\def\csname v@abl/scale/SB_base/krisp/wer\endcsname{7.51}
\expandafter\def\csname v@abl/scale/SB_base/leakdb\endcsname{-31.6}
\expandafter\def\csname v@abl/scale/SB_base/nsf_dev/leak\endcsname{0.38}
\expandafter\def\csname v@abl/scale/SB_base/nsf_dev/miss\endcsname{7.20}
\expandafter\def\csname v@abl/scale/SB_base/nsf_dev/wer\endcsname{8.97}
\expandafter\def\csname v@abl/scale/SB_base/null-sisdri\endcsname{4.29}
\expandafter\def\csname v@abl/scale/SB_base/sisdri\endcsname{5.41}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_10ms/core\endcsname{28}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_10ms/max\endcsname{81.0}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_10ms/p50\endcsname{2.7}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_10ms/p99\endcsname{3.5}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_10ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_10ms/snr50\endcsname{101}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_20ms/core\endcsname{18}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_20ms/max\endcsname{11.1}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_20ms/p50\endcsname{3.6}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_20ms/p99\endcsname{4.4}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_20ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_20ms/snr50\endcsname{101}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_50ms/core\endcsname{10}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_50ms/max\endcsname{14.4}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_50ms/p50\endcsname{4.8}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_50ms/p99\endcsname{6.6}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_50ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/16k_50ms/snr50\endcsname{332}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/48k_50ms/core\endcsname{11}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/48k_50ms/max\endcsname{115.1}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/48k_50ms/p50\endcsname{5.2}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd/48k_50ms/p99\endcsname{8.7}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_10ms/core\endcsname{21}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_10ms/max\endcsname{13.7}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_10ms/p50\endcsname{2.0}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_10ms/p99\endcsname{2.5}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_10ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_10ms/snr50\endcsname{33}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_20ms/core\endcsname{14}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_20ms/max\endcsname{7.6}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_20ms/p50\endcsname{2.8}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_20ms/p99\endcsname{3.4}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_20ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_20ms/snr50\endcsname{37}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_50ms/core\endcsname{8}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_50ms/max\endcsname{8.9}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_50ms/p50\endcsname{3.9}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_50ms/p99\endcsname{5.3}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_50ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/16k_50ms/snr50\endcsname{332}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/48k_50ms/core\endcsname{9}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/48k_50ms/max\endcsname{21.5}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/48k_50ms/p50\endcsname{4.3}
\expandafter\def\csname v@agent/lk/C10_ftlong_kd_int8/48k_50ms/p99\endcsname{7.1}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_10ms/core\endcsname{53}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_10ms/max\endcsname{24.4}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_10ms/p50\endcsname{5.2}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_10ms/p99\endcsname{6.1}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_10ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_10ms/snr50\endcsname{101}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_20ms/core\endcsname{33}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_20ms/max\endcsname{13.8}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_20ms/p50\endcsname{6.5}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_20ms/p99\endcsname{7.5}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_20ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_20ms/snr50\endcsname{104}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_50ms/core\endcsname{17}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_50ms/max\endcsname{15.0}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_50ms/p50\endcsname{8.3}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_50ms/p99\endcsname{10.3}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_50ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/16k_50ms/snr50\endcsname{332}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/48k_50ms/core\endcsname{18}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/48k_50ms/max\endcsname{153.6}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/48k_50ms/p50\endcsname{8.7}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd/48k_50ms/p99\endcsname{15.3}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_10ms/core\endcsname{33}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_10ms/max\endcsname{19.5}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_10ms/p50\endcsname{3.2}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_10ms/p99\endcsname{4.0}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_10ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_10ms/snr50\endcsname{37}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_20ms/core\endcsname{22}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_20ms/max\endcsname{10.3}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_20ms/p50\endcsname{4.4}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_20ms/p99\endcsname{5.9}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_20ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_20ms/snr50\endcsname{40}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_50ms/core\endcsname{12}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_50ms/max\endcsname{12.9}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_50ms/p50\endcsname{5.8}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_50ms/p99\endcsname{8.8}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_50ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/16k_50ms/snr50\endcsname{332}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/48k_50ms/core\endcsname{13}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/48k_50ms/max\endcsname{21.9}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/48k_50ms/p50\endcsname{6.3}
\expandafter\def\csname v@agent/lk/C22_ftlong_kd_int8/48k_50ms/p99\endcsname{10.8}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_10ms/core\endcsname{52}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_10ms/max\endcsname{16.8}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_10ms/p50\endcsname{5.2}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_10ms/p99\endcsname{6.2}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_10ms/snr\endcsname{330}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_10ms/snr50\endcsname{100}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_20ms/core\endcsname{33}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_20ms/max\endcsname{12.8}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_20ms/p50\endcsname{6.6}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_20ms/p99\endcsname{7.4}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_20ms/snr\endcsname{330}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_20ms/snr50\endcsname{101}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_50ms/core\endcsname{17}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_50ms/max\endcsname{15.8}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_50ms/p50\endcsname{8.2}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_50ms/p99\endcsname{11.4}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_50ms/snr\endcsname{330}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/16k_50ms/snr50\endcsname{330}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/48k_50ms/core\endcsname{18}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/48k_50ms/max\endcsname{53.9}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/48k_50ms/p50\endcsname{8.6}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc/48k_50ms/p99\endcsname{15.3}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_10ms/core\endcsname{34}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_10ms/max\endcsname{17.5}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_10ms/p50\endcsname{3.3}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_10ms/p99\endcsname{4.9}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_10ms/snr\endcsname{330}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_10ms/snr50\endcsname{38}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_20ms/core\endcsname{22}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_20ms/max\endcsname{9.9}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_20ms/p50\endcsname{4.4}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_20ms/p99\endcsname{5.9}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_20ms/snr\endcsname{330}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_20ms/snr50\endcsname{35}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_50ms/core\endcsname{12}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_50ms/max\endcsname{11.3}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_50ms/p50\endcsname{5.8}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_50ms/p99\endcsname{8.6}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_50ms/snr\endcsname{330}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/16k_50ms/snr50\endcsname{330}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/48k_50ms/core\endcsname{13}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/48k_50ms/max\endcsname{21.6}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/48k_50ms/p50\endcsname{6.2}
\expandafter\def\csname v@agent/lk/C22_ftlong_sc_int8/48k_50ms/p99\endcsname{10.6}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_10ms/core\endcsname{108}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_10ms/max\endcsname{25.7}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_10ms/p50\endcsname{10.7}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_10ms/p99\endcsname{12.2}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_10ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_10ms/snr50\endcsname{102}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_20ms/core\endcsname{64}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_20ms/max\endcsname{20.0}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_20ms/p50\endcsname{12.7}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_20ms/p99\endcsname{14.2}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_20ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_20ms/snr50\endcsname{100}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_50ms/core\endcsname{31}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_50ms/max\endcsname{23.2}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_50ms/p50\endcsname{15.4}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_50ms/p99\endcsname{18.7}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_50ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/16k_50ms/snr50\endcsname{332}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/48k_50ms/core\endcsname{33}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/48k_50ms/max\endcsname{49.0}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/48k_50ms/p50\endcsname{16.0}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd/48k_50ms/p99\endcsname{28.7}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_10ms/core\endcsname{59}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_10ms/max\endcsname{23.6}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_10ms/p50\endcsname{5.7}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_10ms/p99\endcsname{7.9}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_10ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_10ms/snr50\endcsname{34}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_20ms/core\endcsname{39}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_20ms/max\endcsname{14.6}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_20ms/p50\endcsname{7.7}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_20ms/p99\endcsname{8.9}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_20ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_20ms/snr50\endcsname{34}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_50ms/core\endcsname{21}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_50ms/max\endcsname{16.2}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_50ms/p50\endcsname{10.1}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_50ms/p99\endcsname{12.9}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_50ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/16k_50ms/snr50\endcsname{332}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/48k_50ms/core\endcsname{22}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/48k_50ms/max\endcsname{26.4}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/48k_50ms/p50\endcsname{10.5}
\expandafter\def\csname v@agent/lk/C51_ftlong_kd_int8/48k_50ms/p99\endcsname{18.3}
\expandafter\def\csname v@agent/lk/S_functional/16k_10ms/core\endcsname{421}
\expandafter\def\csname v@agent/lk/S_functional/16k_10ms/max\endcsname{170.9}
\expandafter\def\csname v@agent/lk/S_functional/16k_10ms/p50\endcsname{41.6}
\expandafter\def\csname v@agent/lk/S_functional/16k_10ms/p99\endcsname{52.9}
\expandafter\def\csname v@agent/lk/S_functional/16k_10ms/snr\endcsname{104}
\expandafter\def\csname v@agent/lk/S_functional/16k_20ms/core\endcsname{247}
\expandafter\def\csname v@agent/lk/S_functional/16k_20ms/max\endcsname{65.7}
\expandafter\def\csname v@agent/lk/S_functional/16k_20ms/p50\endcsname{48.9}
\expandafter\def\csname v@agent/lk/S_functional/16k_20ms/p99\endcsname{59.4}
\expandafter\def\csname v@agent/lk/S_functional/16k_20ms/snr\endcsname{104}
\expandafter\def\csname v@agent/lk/S_functional/16k_50ms/core\endcsname{128}
\expandafter\def\csname v@agent/lk/S_functional/16k_50ms/max\endcsname{80.9}
\expandafter\def\csname v@agent/lk/S_functional/16k_50ms/p50\endcsname{63.4}
\expandafter\def\csname v@agent/lk/S_functional/16k_50ms/p99\endcsname{72.5}
\expandafter\def\csname v@agent/lk/S_functional/16k_50ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/S_functional/48k_50ms/core\endcsname{132}
\expandafter\def\csname v@agent/lk/S_functional/48k_50ms/max\endcsname{744.8}
\expandafter\def\csname v@agent/lk/S_functional/48k_50ms/p50\endcsname{64.4}
\expandafter\def\csname v@agent/lk/S_functional/48k_50ms/p99\endcsname{113.3}
\expandafter\def\csname v@agent/lk/student/16k_10ms/core\endcsname{53}
\expandafter\def\csname v@agent/lk/student/16k_10ms/max\endcsname{24.4}
\expandafter\def\csname v@agent/lk/student/16k_10ms/p50\endcsname{5.2}
\expandafter\def\csname v@agent/lk/student/16k_10ms/p99\endcsname{6.1}
\expandafter\def\csname v@agent/lk/student/16k_10ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/student/16k_10ms/snr50\endcsname{101}
\expandafter\def\csname v@agent/lk/student/16k_20ms/core\endcsname{33}
\expandafter\def\csname v@agent/lk/student/16k_20ms/max\endcsname{13.8}
\expandafter\def\csname v@agent/lk/student/16k_20ms/p50\endcsname{6.5}
\expandafter\def\csname v@agent/lk/student/16k_20ms/p99\endcsname{7.5}
\expandafter\def\csname v@agent/lk/student/16k_20ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/student/16k_20ms/snr50\endcsname{104}
\expandafter\def\csname v@agent/lk/student/16k_50ms/core\endcsname{17}
\expandafter\def\csname v@agent/lk/student/16k_50ms/max\endcsname{15.0}
\expandafter\def\csname v@agent/lk/student/16k_50ms/p50\endcsname{8.3}
\expandafter\def\csname v@agent/lk/student/16k_50ms/p99\endcsname{10.3}
\expandafter\def\csname v@agent/lk/student/16k_50ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/student/16k_50ms/snr50\endcsname{332}
\expandafter\def\csname v@agent/lk/student/48k_50ms/core\endcsname{18}
\expandafter\def\csname v@agent/lk/student/48k_50ms/max\endcsname{153.6}
\expandafter\def\csname v@agent/lk/student/48k_50ms/p50\endcsname{8.7}
\expandafter\def\csname v@agent/lk/student/48k_50ms/p99\endcsname{15.3}
\expandafter\def\csname v@agent/lk/student_int8/16k_10ms/core\endcsname{33}
\expandafter\def\csname v@agent/lk/student_int8/16k_10ms/max\endcsname{19.5}
\expandafter\def\csname v@agent/lk/student_int8/16k_10ms/p50\endcsname{3.2}
\expandafter\def\csname v@agent/lk/student_int8/16k_10ms/p99\endcsname{4.0}
\expandafter\def\csname v@agent/lk/student_int8/16k_10ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/student_int8/16k_10ms/snr50\endcsname{37}
\expandafter\def\csname v@agent/lk/student_int8/16k_20ms/core\endcsname{22}
\expandafter\def\csname v@agent/lk/student_int8/16k_20ms/max\endcsname{10.3}
\expandafter\def\csname v@agent/lk/student_int8/16k_20ms/p50\endcsname{4.4}
\expandafter\def\csname v@agent/lk/student_int8/16k_20ms/p99\endcsname{5.9}
\expandafter\def\csname v@agent/lk/student_int8/16k_20ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/student_int8/16k_20ms/snr50\endcsname{40}
\expandafter\def\csname v@agent/lk/student_int8/16k_50ms/core\endcsname{12}
\expandafter\def\csname v@agent/lk/student_int8/16k_50ms/max\endcsname{12.9}
\expandafter\def\csname v@agent/lk/student_int8/16k_50ms/p50\endcsname{5.8}
\expandafter\def\csname v@agent/lk/student_int8/16k_50ms/p99\endcsname{8.8}
\expandafter\def\csname v@agent/lk/student_int8/16k_50ms/snr\endcsname{332}
\expandafter\def\csname v@agent/lk/student_int8/16k_50ms/snr50\endcsname{332}
\expandafter\def\csname v@agent/lk/student_int8/48k_50ms/core\endcsname{13}
\expandafter\def\csname v@agent/lk/student_int8/48k_50ms/max\endcsname{21.9}
\expandafter\def\csname v@agent/lk/student_int8/48k_50ms/p50\endcsname{6.3}
\expandafter\def\csname v@agent/lk/student_int8/48k_50ms/p99\endcsname{10.8}
\expandafter\def\csname v@agent/lk/tiny/16k_10ms/core\endcsname{5}
\expandafter\def\csname v@agent/lk/tiny/16k_10ms/max\endcsname{75.0}
\expandafter\def\csname v@agent/lk/tiny/16k_10ms/p50\endcsname{0.5}
\expandafter\def\csname v@agent/lk/tiny/16k_10ms/p99\endcsname{0.8}
\expandafter\def\csname v@agent/lk/tiny/16k_10ms/snr\endcsname{108}
\expandafter\def\csname v@agent/lk/tiny/16k_20ms/core\endcsname{3}
\expandafter\def\csname v@agent/lk/tiny/16k_20ms/max\endcsname{2.3}
\expandafter\def\csname v@agent/lk/tiny/16k_20ms/p50\endcsname{0.6}
\expandafter\def\csname v@agent/lk/tiny/16k_20ms/p99\endcsname{1.1}
\expandafter\def\csname v@agent/lk/tiny/16k_20ms/snr\endcsname{108}
\expandafter\def\csname v@agent/lk/tiny/16k_50ms/core\endcsname{2}
\expandafter\def\csname v@agent/lk/tiny/16k_50ms/max\endcsname{2.4}
\expandafter\def\csname v@agent/lk/tiny/16k_50ms/p50\endcsname{1.0}
\expandafter\def\csname v@agent/lk/tiny/16k_50ms/p99\endcsname{1.2}
\expandafter\def\csname v@agent/lk/tiny/16k_50ms/snr\endcsname{333}
\expandafter\def\csname v@agent/lk/tiny/48k_50ms/core\endcsname{3}
\expandafter\def\csname v@agent/lk/tiny/48k_50ms/max\endcsname{83.4}
\expandafter\def\csname v@agent/lk/tiny/48k_50ms/p50\endcsname{1.2}
\expandafter\def\csname v@agent/lk/tiny/48k_50ms/p99\endcsname{2.2}
\expandafter\def\csname v@agent/onnx/C10_ftlong_kd/mb\endcsname{36}
\expandafter\def\csname v@agent/onnx/C10_ftlong_kd/rtf\endcsname{0.11}
\expandafter\def\csname v@agent/onnx/C10_ftlong_kd/snr-live\endcsname{133}
\expandafter\def\csname v@agent/onnx/C10_ftlong_kd/snr-null\endcsname{133}
\expandafter\def\csname v@agent/onnx/C10_ftlong_kd_int8/mb\endcsname{12}
\expandafter\def\csname v@agent/onnx/C10_ftlong_kd_int8/rtf\endcsname{0.09}
\expandafter\def\csname v@agent/onnx/C10_ftlong_kd_int8/snr-live\endcsname{58}
\expandafter\def\csname v@agent/onnx/C10_ftlong_kd_int8/snr-null\endcsname{58}
\expandafter\def\csname v@agent/onnx/C10n_agent/mb\endcsname{36}
\expandafter\def\csname v@agent/onnx/C10n_agent/rtf\endcsname{0.11}
\expandafter\def\csname v@agent/onnx/C10n_agent/snr-live\endcsname{96}
\expandafter\def\csname v@agent/onnx/C10n_agent/snr-null\endcsname{99}
\expandafter\def\csname v@agent/onnx/C10n_agent_int8/mb\endcsname{12}
\expandafter\def\csname v@agent/onnx/C10n_agent_int8/rtf\endcsname{0.09}
\expandafter\def\csname v@agent/onnx/C10n_agent_int8/snr-live\endcsname{31}
\expandafter\def\csname v@agent/onnx/C10n_agent_int8/snr-null\endcsname{26}
\expandafter\def\csname v@agent/onnx/C10n_ftlong_kd/mb\endcsname{36}
\expandafter\def\csname v@agent/onnx/C10n_ftlong_kd/rtf\endcsname{0.11}
\expandafter\def\csname v@agent/onnx/C10n_ftlong_kd/snr-live\endcsname{132}
\expandafter\def\csname v@agent/onnx/C10n_ftlong_kd/snr-null\endcsname{132}
\expandafter\def\csname v@agent/onnx/C10n_ftlong_kd_int8/mb\endcsname{12}
\expandafter\def\csname v@agent/onnx/C10n_ftlong_kd_int8/rtf\endcsname{0.09}
\expandafter\def\csname v@agent/onnx/C10n_ftlong_kd_int8/snr-live\endcsname{58}
\expandafter\def\csname v@agent/onnx/C10n_ftlong_kd_int8/snr-null\endcsname{57}
\expandafter\def\csname v@agent/onnx/C22_agent/mb\endcsname{86}
\expandafter\def\csname v@agent/onnx/C22_agent/rtf\endcsname{0.18}
\expandafter\def\csname v@agent/onnx/C22_agent/snr-live\endcsname{102}
\expandafter\def\csname v@agent/onnx/C22_agent/snr-null\endcsname{102}
\expandafter\def\csname v@agent/onnx/C22_agent_check/mb\endcsname{86}
\expandafter\def\csname v@agent/onnx/C22_agent_check/rtf\endcsname{0.18}
\expandafter\def\csname v@agent/onnx/C22_agent_check/snr-live\endcsname{102}
\expandafter\def\csname v@agent/onnx/C22_agent_check/snr-null\endcsname{102}
\expandafter\def\csname v@agent/onnx/C22_agent_int8/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/C22_agent_int8/rtf\endcsname{0.13}
\expandafter\def\csname v@agent/onnx/C22_agent_int8/snr-live\endcsname{35}
\expandafter\def\csname v@agent/onnx/C22_agent_int8/snr-null\endcsname{29}
\expandafter\def\csname v@agent/onnx/C22_agent_int8_check/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/C22_agent_int8_check/rtf\endcsname{0.13}
\expandafter\def\csname v@agent/onnx/C22_agent_int8_check/snr-live\endcsname{35}
\expandafter\def\csname v@agent/onnx/C22_agent_int8_check/snr-null\endcsname{29}
\expandafter\def\csname v@agent/onnx/C22_ftlong_kd/mb\endcsname{85}
\expandafter\def\csname v@agent/onnx/C22_ftlong_kd/rtf\endcsname{0.19}
\expandafter\def\csname v@agent/onnx/C22_ftlong_kd/snr-live\endcsname{133}
\expandafter\def\csname v@agent/onnx/C22_ftlong_kd/snr-null\endcsname{134}
\expandafter\def\csname v@agent/onnx/C22_ftlong_kd_int8/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/C22_ftlong_kd_int8/rtf\endcsname{0.14}
\expandafter\def\csname v@agent/onnx/C22_ftlong_kd_int8/snr-live\endcsname{49}
\expandafter\def\csname v@agent/onnx/C22_ftlong_kd_int8/snr-null\endcsname{56}
\expandafter\def\csname v@agent/onnx/C22_ftlong_sc/mb\endcsname{85}
\expandafter\def\csname v@agent/onnx/C22_ftlong_sc/rtf\endcsname{0.19}
\expandafter\def\csname v@agent/onnx/C22_ftlong_sc/snr-live\endcsname{129}
\expandafter\def\csname v@agent/onnx/C22_ftlong_sc/snr-null\endcsname{133}
\expandafter\def\csname v@agent/onnx/C22_ftlong_sc_int8/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/C22_ftlong_sc_int8/rtf\endcsname{0.14}
\expandafter\def\csname v@agent/onnx/C22_ftlong_sc_int8/snr-live\endcsname{46}
\expandafter\def\csname v@agent/onnx/C22_ftlong_sc_int8/snr-null\endcsname{54}
\expandafter\def\csname v@agent/onnx/C22_release/mb\endcsname{85}
\expandafter\def\csname v@agent/onnx/C22_release/rtf\endcsname{0.22}
\expandafter\def\csname v@agent/onnx/C22_release/snr-live\endcsname{96}
\expandafter\def\csname v@agent/onnx/C22_release/snr-null\endcsname{128}
\expandafter\def\csname v@agent/onnx/C22_release_int8/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/C22_release_int8/rtf\endcsname{0.14}
\expandafter\def\csname v@agent/onnx/C22_release_int8/snr-live\endcsname{32}
\expandafter\def\csname v@agent/onnx/C22_release_int8/snr-null\endcsname{53}
\expandafter\def\csname v@agent/onnx/C22_vb2/mb\endcsname{85}
\expandafter\def\csname v@agent/onnx/C22_vb2/rtf\endcsname{0.19}
\expandafter\def\csname v@agent/onnx/C22_vb2/snr-live\endcsname{90}
\expandafter\def\csname v@agent/onnx/C22_vb2/snr-null\endcsname{125}
\expandafter\def\csname v@agent/onnx/C22_vb2_int8/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/C22_vb2_int8/rtf\endcsname{0.13}
\expandafter\def\csname v@agent/onnx/C22_vb2_int8/snr-live\endcsname{24}
\expandafter\def\csname v@agent/onnx/C22_vb2_int8/snr-null\endcsname{47}
\expandafter\def\csname v@agent/onnx/C22_vbkd/mb\endcsname{85}
\expandafter\def\csname v@agent/onnx/C22_vbkd/rtf\endcsname{0.20}
\expandafter\def\csname v@agent/onnx/C22_vbkd/snr-live\endcsname{87}
\expandafter\def\csname v@agent/onnx/C22_vbkd/snr-null\endcsname{127}
\expandafter\def\csname v@agent/onnx/C22_vbkd_int8/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/C22_vbkd_int8/rtf\endcsname{0.13}
\expandafter\def\csname v@agent/onnx/C22_vbkd_int8/snr-live\endcsname{11}
\expandafter\def\csname v@agent/onnx/C22_vbkd_int8/snr-null\endcsname{51}
\expandafter\def\csname v@agent/onnx/C51_ftlong_kd/mb\endcsname{200}
\expandafter\def\csname v@agent/onnx/C51_ftlong_kd/rtf\endcsname{0.37}
\expandafter\def\csname v@agent/onnx/C51_ftlong_kd/snr-live\endcsname{134}
\expandafter\def\csname v@agent/onnx/C51_ftlong_kd/snr-null\endcsname{133}
\expandafter\def\csname v@agent/onnx/C51_ftlong_kd_int8/mb\endcsname{54}
\expandafter\def\csname v@agent/onnx/C51_ftlong_kd_int8/rtf\endcsname{0.22}
\expandafter\def\csname v@agent/onnx/C51_ftlong_kd_int8/snr-live\endcsname{54}
\expandafter\def\csname v@agent/onnx/C51_ftlong_kd_int8/snr-null\endcsname{54}
\expandafter\def\csname v@agent/onnx/SB_ftlong_ws/mb\endcsname{557}
\expandafter\def\csname v@agent/onnx/SB_ftlong_ws/rtf\endcsname{1.36}
\expandafter\def\csname v@agent/onnx/SB_ftlong_ws/snr-live\endcsname{124}
\expandafter\def\csname v@agent/onnx/SB_ftlong_ws/snr-null\endcsname{128}
\expandafter\def\csname v@agent/onnx/SB_ftlong_ws_int8/mb\endcsname{144}
\expandafter\def\csname v@agent/onnx/SB_ftlong_ws_int8/rtf\endcsname{0.50}
\expandafter\def\csname v@agent/onnx/SB_ftlong_ws_int8/snr-live\endcsname{40}
\expandafter\def\csname v@agent/onnx/SB_ftlong_ws_int8/snr-null\endcsname{40}
\expandafter\def\csname v@agent/onnx/speed_C10/mb\endcsname{36}
\expandafter\def\csname v@agent/onnx/speed_C10/rtf\endcsname{0.11}
\expandafter\def\csname v@agent/onnx/speed_C10/snr-live\endcsname{127}
\expandafter\def\csname v@agent/onnx/speed_C10/snr-null\endcsname{134}
\expandafter\def\csname v@agent/onnx/speed_C10_int8/mb\endcsname{12}
\expandafter\def\csname v@agent/onnx/speed_C10_int8/rtf\endcsname{0.09}
\expandafter\def\csname v@agent/onnx/speed_C10_int8/snr-live\endcsname{61}
\expandafter\def\csname v@agent/onnx/speed_C10_int8/snr-null\endcsname{65}
\expandafter\def\csname v@agent/onnx/speed_C10r64/mb\endcsname{35}
\expandafter\def\csname v@agent/onnx/speed_C10r64/rtf\endcsname{0.11}
\expandafter\def\csname v@agent/onnx/speed_C10r64/snr-live\endcsname{128}
\expandafter\def\csname v@agent/onnx/speed_C10r64/snr-null\endcsname{133}
\expandafter\def\csname v@agent/onnx/speed_C10r64_int8/mb\endcsname{12}
\expandafter\def\csname v@agent/onnx/speed_C10r64_int8/rtf\endcsname{0.09}
\expandafter\def\csname v@agent/onnx/speed_C10r64_int8/snr-live\endcsname{63}
\expandafter\def\csname v@agent/onnx/speed_C10r64_int8/snr-null\endcsname{64}
\expandafter\def\csname v@agent/onnx/speed_C10r96/mb\endcsname{36}
\expandafter\def\csname v@agent/onnx/speed_C10r96/rtf\endcsname{0.11}
\expandafter\def\csname v@agent/onnx/speed_C10r96/snr-live\endcsname{129}
\expandafter\def\csname v@agent/onnx/speed_C10r96/snr-null\endcsname{134}
\expandafter\def\csname v@agent/onnx/speed_C10r96_int8/mb\endcsname{12}
\expandafter\def\csname v@agent/onnx/speed_C10r96_int8/rtf\endcsname{0.09}
\expandafter\def\csname v@agent/onnx/speed_C10r96_int8/snr-live\endcsname{60}
\expandafter\def\csname v@agent/onnx/speed_C10r96_int8/snr-null\endcsname{66}
\expandafter\def\csname v@agent/onnx/speed_C11/mb\endcsname{44}
\expandafter\def\csname v@agent/onnx/speed_C11/rtf\endcsname{0.14}
\expandafter\def\csname v@agent/onnx/speed_C11/snr-live\endcsname{127}
\expandafter\def\csname v@agent/onnx/speed_C11/snr-null\endcsname{134}
\expandafter\def\csname v@agent/onnx/speed_C11_int8/mb\endcsname{14}
\expandafter\def\csname v@agent/onnx/speed_C11_int8/rtf\endcsname{0.12}
\expandafter\def\csname v@agent/onnx/speed_C11_int8/snr-live\endcsname{59}
\expandafter\def\csname v@agent/onnx/speed_C11_int8/snr-null\endcsname{64}
\expandafter\def\csname v@agent/onnx/speed_C22/mb\endcsname{85}
\expandafter\def\csname v@agent/onnx/speed_C22/rtf\endcsname{0.20}
\expandafter\def\csname v@agent/onnx/speed_C22/snr-live\endcsname{127}
\expandafter\def\csname v@agent/onnx/speed_C22/snr-null\endcsname{134}
\expandafter\def\csname v@agent/onnx/speed_C22_int8/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/speed_C22_int8/rtf\endcsname{0.14}
\expandafter\def\csname v@agent/onnx/speed_C22_int8/snr-live\endcsname{60}
\expandafter\def\csname v@agent/onnx/speed_C22_int8/snr-null\endcsname{65}
\expandafter\def\csname v@agent/onnx/speed_C7/mb\endcsname{24}
\expandafter\def\csname v@agent/onnx/speed_C7/rtf\endcsname{0.10}
\expandafter\def\csname v@agent/onnx/speed_C7/snr-live\endcsname{130}
\expandafter\def\csname v@agent/onnx/speed_C7/snr-null\endcsname{134}
\expandafter\def\csname v@agent/onnx/speed_C7_int8/mb\endcsname{9}
\expandafter\def\csname v@agent/onnx/speed_C7_int8/rtf\endcsname{0.08}
\expandafter\def\csname v@agent/onnx/speed_C7_int8/snr-live\endcsname{61}
\expandafter\def\csname v@agent/onnx/speed_C7_int8/snr-null\endcsname{65}
\expandafter\def\csname v@agent/onnx/student/mb\endcsname{85}
\expandafter\def\csname v@agent/onnx/student/rtf\endcsname{0.19}
\expandafter\def\csname v@agent/onnx/student/snr-live\endcsname{133}
\expandafter\def\csname v@agent/onnx/student/snr-null\endcsname{134}
\expandafter\def\csname v@agent/onnx/student_int8/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/student_int8/rtf\endcsname{0.14}
\expandafter\def\csname v@agent/onnx/student_int8/snr-live\endcsname{49}
\expandafter\def\csname v@agent/onnx/student_int8/snr-null\endcsname{56}
\expandafter\def\csname v@agent/onnx/test_C22_vbg/mb\endcsname{86}
\expandafter\def\csname v@agent/onnx/test_C22_vbg/rtf\endcsname{0.18}
\expandafter\def\csname v@agent/onnx/test_C22_vbg/snr-live\endcsname{101}
\expandafter\def\csname v@agent/onnx/test_C22_vbg/snr-null\endcsname{98}
\expandafter\def\csname v@agent/onnx/test_C22_vbg_int8/mb\endcsname{25}
\expandafter\def\csname v@agent/onnx/test_C22_vbg_int8/rtf\endcsname{0.15}
\expandafter\def\csname v@agent/onnx/test_C22_vbg_int8/snr-live\endcsname{37}
\expandafter\def\csname v@agent/onnx/test_C22_vbg_int8/snr-null\endcsname{30}
\expandafter\def\csname v@agent/onnx/tiny/mb\endcsname{1}
\expandafter\def\csname v@agent/onnx/tiny/rtf\endcsname{0.02}
\expandafter\def\csname v@agent/onnx/tiny/snr-live\endcsname{134}
\expandafter\def\csname v@agent/onnx/tiny/snr-null\endcsname{134}
\expandafter\def\csname v@agent/onnx/tiny_gate/mb\endcsname{1}
\expandafter\def\csname v@agent/onnx/tiny_gate/rtf\endcsname{0.03}
\expandafter\def\csname v@agent/onnx/tiny_gate/snr-live\endcsname{133}
\expandafter\def\csname v@agent/onnx/tiny_gate/snr-null\endcsname{131}
\expandafter\def\csname v@aic_calls/C22_ftlong_kd_selfl/dele\endcsname{3.35}
\expandafter\def\csname v@aic_calls/C22_ftlong_kd_selfl/dleak\endcsname{-4.98}
\expandafter\def\csname v@aic_calls/C22_ftlong_kd_selfl/dwer\endcsname{-2.46}
\expandafter\def\csname v@aic_calls/C22_ftlong_kd_selfl/dwer-hi\endcsname{+4.15}
\expandafter\def\csname v@aic_calls/C22_ftlong_kd_selfl/dwer-lo\endcsname{-31.73}
\expandafter\def\csname v@aic_calls/C22_ftlong_kd_selfl/ins\endcsname{11.40}
\expandafter\def\csname v@aic_calls/C22_ftlong_kd_selfl/leak_wpm\endcsname{13.25}
\expandafter\def\csname v@aic_calls/C22_ftlong_kd_selfl/miss\endcsname{6.63}
\expandafter\def\csname v@aic_calls/C22_ftlong_kd_selfl/wer\endcsname{18.03}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_loud/dele\endcsname{2.53}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_loud/dleak\endcsname{-12.93}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_loud/dwer\endcsname{-7.95}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_loud/dwer-hi\endcsname{+1.12}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_loud/dwer-lo\endcsname{-47.60}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_loud/ins\endcsname{7.06}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_loud/leak_wpm\endcsname{5.30}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_loud/miss\endcsname{5.49}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_loud/wer\endcsname{12.54}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_null/dele\endcsname{2.82}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{-9.78}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-6.02}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+2.88}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-44.26}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_null/ins\endcsname{8.27}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{8.45}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_null/miss\endcsname{6.20}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_null/wer\endcsname{14.47}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{2.57}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-9.84}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-6.24}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+2.39}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-42.80}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{8.52}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{8.39}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{5.74}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{14.26}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_loud/dele\endcsname{2.74}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_loud/dleak\endcsname{-9.40}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_loud/dwer\endcsname{-5.02}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_loud/dwer-hi\endcsname{+2.38}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_loud/dwer-lo\endcsname{-36.12}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_loud/ins\endcsname{9.16}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_loud/leak_wpm\endcsname{8.83}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_loud/miss\endcsname{6.31}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_loud/wer\endcsname{15.47}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_null/dele\endcsname{2.10}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_null/dleak\endcsname{-5.17}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_null/dwer\endcsname{-3.64}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_null/dwer-hi\endcsname{+2.94}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_null/dwer-lo\endcsname{-31.94}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_null/ins\endcsname{11.12}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_null/leak_wpm\endcsname{13.06}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_null/miss\endcsname{5.74}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_null/wer\endcsname{16.86}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_selfl/dele\endcsname{2.28}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_selfl/dleak\endcsname{-6.31}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_selfl/dwer\endcsname{-3.92}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_selfl/dwer-hi\endcsname{+3.26}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_selfl/dwer-lo\endcsname{-34.66}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_selfl/ins\endcsname{10.87}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_selfl/leak_wpm\endcsname{11.92}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_selfl/miss\endcsname{5.70}
\expandafter\def\csname v@aic_calls/MB_ftlong_ws_selfl/wer\endcsname{16.57}
\expandafter\def\csname v@aic_calls/SB_ftlong_ws_selfl/dele\endcsname{3.21}
\expandafter\def\csname v@aic_calls/SB_ftlong_ws_selfl/dleak\endcsname{-4.23}
\expandafter\def\csname v@aic_calls/SB_ftlong_ws_selfl/dwer\endcsname{-2.03}
\expandafter\def\csname v@aic_calls/SB_ftlong_ws_selfl/dwer-hi\endcsname{+4.30}
\expandafter\def\csname v@aic_calls/SB_ftlong_ws_selfl/dwer-lo\endcsname{-29.85}
\expandafter\def\csname v@aic_calls/SB_ftlong_ws_selfl/ins\endcsname{11.44}
\expandafter\def\csname v@aic_calls/SB_ftlong_ws_selfl/leak_wpm\endcsname{14.01}
\expandafter\def\csname v@aic_calls/SB_ftlong_ws_selfl/miss\endcsname{7.02}
\expandafter\def\csname v@aic_calls/SB_ftlong_ws_selfl/wer\endcsname{18.46}
\expandafter\def\csname v@aic_calls/dfn3/dele\endcsname{3.49}
\expandafter\def\csname v@aic_calls/dfn3/dleak\endcsname{+18.74}
\expandafter\def\csname v@aic_calls/dfn3/dwer\endcsname{+14.86}
\expandafter\def\csname v@aic_calls/dfn3/dwer-hi\endcsname{+25.26}
\expandafter\def\csname v@aic_calls/dfn3/dwer-lo\endcsname{+0.00}
\expandafter\def\csname v@aic_calls/dfn3/ins\endcsname{26.12}
\expandafter\def\csname v@aic_calls/dfn3/leak_wpm\endcsname{36.97}
\expandafter\def\csname v@aic_calls/dfn3/miss\endcsname{9.23}
\expandafter\def\csname v@aic_calls/dfn3/wer\endcsname{35.35}
\expandafter\def\csname v@aic_calls/raw/dele\endcsname{1.35}
\expandafter\def\csname v@aic_calls/raw/dleak\endcsname{+68.52}
\expandafter\def\csname v@aic_calls/raw/dwer\endcsname{+45.87}
\expandafter\def\csname v@aic_calls/raw/dwer-hi\endcsname{+182.05}
\expandafter\def\csname v@aic_calls/raw/dwer-lo\endcsname{+17.57}
\expandafter\def\csname v@aic_calls/raw/ins\endcsname{57.59}
\expandafter\def\csname v@aic_calls/raw/leak_wpm\endcsname{86.75}
\expandafter\def\csname v@aic_calls/raw/miss\endcsname{8.77}
\expandafter\def\csname v@aic_calls/raw/wer\endcsname{66.36}
\expandafter\def\csname v@aic_calls/voxlock/dele\endcsname{3.17}
\expandafter\def\csname v@aic_calls/voxlock/dleak\endcsname{-0.19}
\expandafter\def\csname v@aic_calls/voxlock/dwer\endcsname{-0.18}
\expandafter\def\csname v@aic_calls/voxlock/dwer-hi\endcsname{+0.07}
\expandafter\def\csname v@aic_calls/voxlock/dwer-lo\endcsname{-1.41}
\expandafter\def\csname v@aic_calls/voxlock/ins\endcsname{13.83}
\expandafter\def\csname v@aic_calls/voxlock/leak_wpm\endcsname{18.04}
\expandafter\def\csname v@aic_calls/voxlock/miss\endcsname{6.49}
\expandafter\def\csname v@aic_calls/voxlock/wer\endcsname{20.31}
\expandafter\def\csname v@aic_calls/voxlock_live/dele\endcsname{2.85}
\expandafter\def\csname v@aic_calls/voxlock_live/dleak\endcsname{+6.56}
\expandafter\def\csname v@aic_calls/voxlock_live/dwer\endcsname{+4.06}
\expandafter\def\csname v@aic_calls/voxlock_live/dwer-hi\endcsname{+9.80}
\expandafter\def\csname v@aic_calls/voxlock_live/dwer-lo\endcsname{-5.85}
\expandafter\def\csname v@aic_calls/voxlock_live/ins\endcsname{17.03}
\expandafter\def\csname v@aic_calls/voxlock_live/leak_wpm\endcsname{24.80}
\expandafter\def\csname v@aic_calls/voxlock_live/miss\endcsname{7.52}
\expandafter\def\csname v@aic_calls/voxlock_live/wer\endcsname{24.55}
\expandafter\def\csname v@aic_calls/voxlock_pt/dele\endcsname{3.17}
\expandafter\def\csname v@aic_calls/voxlock_pt/ins\endcsname{13.86}
\expandafter\def\csname v@aic_calls/voxlock_pt/leak_wpm\endcsname{18.23}
\expandafter\def\csname v@aic_calls/voxlock_pt/miss\endcsname{6.63}
\expandafter\def\csname v@aic_calls/voxlock_pt/wer\endcsname{20.49}
\expandafter\def\csname v@ali_test/C22_ftlong_kd_selfl/dele\endcsname{9.28}
\expandafter\def\csname v@ali_test/C22_ftlong_kd_selfl/dleak\endcsname{+0.95}
\expandafter\def\csname v@ali_test/C22_ftlong_kd_selfl/dwer\endcsname{+0.45}
\expandafter\def\csname v@ali_test/C22_ftlong_kd_selfl/dwer-hi\endcsname{+1.02}
\expandafter\def\csname v@ali_test/C22_ftlong_kd_selfl/dwer-lo\endcsname{-0.09}
\expandafter\def\csname v@ali_test/C22_ftlong_kd_selfl/ins\endcsname{1.17}
\expandafter\def\csname v@ali_test/C22_ftlong_kd_selfl/leak_wpm\endcsname{1.96}
\expandafter\def\csname v@ali_test/C22_ftlong_kd_selfl/miss\endcsname{14.66}
\expandafter\def\csname v@ali_test/C22_ftlong_kd_selfl/wer\endcsname{15.82}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_loud/dele\endcsname{8.90}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_loud/dleak\endcsname{+0.87}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_loud/dwer\endcsname{+0.02}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_loud/dwer-hi\endcsname{+0.53}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_loud/dwer-lo\endcsname{-0.47}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_loud/ins\endcsname{1.15}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_loud/leak_wpm\endcsname{1.88}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_loud/miss\endcsname{14.25}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_loud/wer\endcsname{15.40}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_null/dele\endcsname{9.18}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{+0.92}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{+0.36}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+0.93}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-0.17}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_null/ins\endcsname{1.25}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{1.93}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_null/miss\endcsname{14.49}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_null/wer\endcsname{15.74}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{9.11}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{+0.78}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{+0.31}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+0.80}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-0.16}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{1.21}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{1.79}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{14.47}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{15.69}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_loud/dele\endcsname{9.21}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_loud/dleak\endcsname{+12.02}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_loud/dwer\endcsname{+2.48}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_loud/dwer-hi\endcsname{+7.38}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_loud/dwer-lo\endcsname{-0.10}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_loud/ins\endcsname{3.29}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_loud/leak_wpm\endcsname{13.03}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_loud/miss\endcsname{14.56}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_loud/wer\endcsname{17.85}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_null/dele\endcsname{9.44}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_null/dleak\endcsname{+0.45}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_null/dwer\endcsname{+0.64}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_null/dwer-hi\endcsname{+1.18}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_null/dwer-lo\endcsname{+0.11}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_null/ins\endcsname{1.08}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_null/leak_wpm\endcsname{1.46}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_null/miss\endcsname{14.94}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_null/wer\endcsname{16.02}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_selfl/dele\endcsname{9.82}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_selfl/dleak\endcsname{+11.83}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_selfl/dwer\endcsname{+3.20}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_selfl/dwer-hi\endcsname{+7.98}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_selfl/dwer-lo\endcsname{+0.57}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_selfl/ins\endcsname{3.30}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_selfl/leak_wpm\endcsname{12.83}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_selfl/miss\endcsname{15.28}
\expandafter\def\csname v@ali_test/MB_ftlong_ws_selfl/wer\endcsname{18.57}
\expandafter\def\csname v@ali_test/SB_ftlong_ws_selfl/dele\endcsname{9.22}
\expandafter\def\csname v@ali_test/SB_ftlong_ws_selfl/dleak\endcsname{+11.97}
\expandafter\def\csname v@ali_test/SB_ftlong_ws_selfl/dwer\endcsname{+2.72}
\expandafter\def\csname v@ali_test/SB_ftlong_ws_selfl/dwer-hi\endcsname{+7.63}
\expandafter\def\csname v@ali_test/SB_ftlong_ws_selfl/dwer-lo\endcsname{+0.13}
\expandafter\def\csname v@ali_test/SB_ftlong_ws_selfl/ins\endcsname{3.39}
\expandafter\def\csname v@ali_test/SB_ftlong_ws_selfl/leak_wpm\endcsname{12.97}
\expandafter\def\csname v@ali_test/SB_ftlong_ws_selfl/miss\endcsname{14.70}
\expandafter\def\csname v@ali_test/SB_ftlong_ws_selfl/wer\endcsname{18.09}
\expandafter\def\csname v@ali_test/dfn3/dele\endcsname{10.86}
\expandafter\def\csname v@ali_test/dfn3/dleak\endcsname{+3.45}
\expandafter\def\csname v@ali_test/dfn3/dwer\endcsname{+3.10}
\expandafter\def\csname v@ali_test/dfn3/dwer-hi\endcsname{+4.58}
\expandafter\def\csname v@ali_test/dfn3/dwer-lo\endcsname{+1.90}
\expandafter\def\csname v@ali_test/dfn3/ins\endcsname{1.56}
\expandafter\def\csname v@ali_test/dfn3/leak_wpm\endcsname{4.46}
\expandafter\def\csname v@ali_test/dfn3/miss\endcsname{16.92}
\expandafter\def\csname v@ali_test/dfn3/wer\endcsname{18.48}
\expandafter\def\csname v@ali_test/raw/dele\endcsname{9.58}
\expandafter\def\csname v@ali_test/raw/dleak\endcsname{+60.11}
\expandafter\def\csname v@ali_test/raw/dwer\endcsname{+14.02}
\expandafter\def\csname v@ali_test/raw/dwer-hi\endcsname{+18.03}
\expandafter\def\csname v@ali_test/raw/dwer-lo\endcsname{+10.52}
\expandafter\def\csname v@ali_test/raw/ins\endcsname{14.28}
\expandafter\def\csname v@ali_test/raw/leak_wpm\endcsname{61.12}
\expandafter\def\csname v@ali_test/raw/miss\endcsname{15.12}
\expandafter\def\csname v@ali_test/raw/wer\endcsname{29.40}
\expandafter\def\csname v@ali_test/sidon_vi/dele\endcsname{8.51}
\expandafter\def\csname v@ali_test/sidon_vi/dleak\endcsname{+123.02}
\expandafter\def\csname v@ali_test/sidon_vi/dwer\endcsname{+27.57}
\expandafter\def\csname v@ali_test/sidon_vi/dwer-hi\endcsname{+31.48}
\expandafter\def\csname v@ali_test/sidon_vi/dwer-lo\endcsname{+24.18}
\expandafter\def\csname v@ali_test/sidon_vi/ins\endcsname{26.12}
\expandafter\def\csname v@ali_test/sidon_vi/leak_wpm\endcsname{124.03}
\expandafter\def\csname v@ali_test/sidon_vi/miss\endcsname{16.82}
\expandafter\def\csname v@ali_test/sidon_vi/wer\endcsname{42.94}
\expandafter\def\csname v@ali_test/sidon_vi_lite/dele\endcsname{9.69}
\expandafter\def\csname v@ali_test/sidon_vi_lite/dleak\endcsname{+8.24}
\expandafter\def\csname v@ali_test/sidon_vi_lite/dwer\endcsname{+3.93}
\expandafter\def\csname v@ali_test/sidon_vi_lite/dwer-hi\endcsname{+6.61}
\expandafter\def\csname v@ali_test/sidon_vi_lite/dwer-lo\endcsname{+1.87}
\expandafter\def\csname v@ali_test/sidon_vi_lite/ins\endcsname{3.56}
\expandafter\def\csname v@ali_test/sidon_vi_lite/leak_wpm\endcsname{9.25}
\expandafter\def\csname v@ali_test/sidon_vi_lite/miss\endcsname{15.75}
\expandafter\def\csname v@ali_test/sidon_vi_lite/wer\endcsname{19.31}
\expandafter\def\csname v@ali_test/voxlock/dele\endcsname{9.65}
\expandafter\def\csname v@ali_test/voxlock/dleak\endcsname{+0.20}
\expandafter\def\csname v@ali_test/voxlock/dwer\endcsname{+1.74}
\expandafter\def\csname v@ali_test/voxlock/dwer-hi\endcsname{+4.39}
\expandafter\def\csname v@ali_test/voxlock/dwer-lo\endcsname{+0.26}
\expandafter\def\csname v@ali_test/voxlock/ins\endcsname{1.97}
\expandafter\def\csname v@ali_test/voxlock/leak_wpm\endcsname{1.21}
\expandafter\def\csname v@ali_test/voxlock/miss\endcsname{15.15}
\expandafter\def\csname v@ali_test/voxlock/wer\endcsname{17.11}
\expandafter\def\csname v@ali_test/voxlock_live/dele\endcsname{10.27}
\expandafter\def\csname v@ali_test/voxlock_live/dleak\endcsname{+0.36}
\expandafter\def\csname v@ali_test/voxlock_live/dwer\endcsname{+0.90}
\expandafter\def\csname v@ali_test/voxlock_live/dwer-hi\endcsname{+1.45}
\expandafter\def\csname v@ali_test/voxlock_live/dwer-lo\endcsname{+0.41}
\expandafter\def\csname v@ali_test/voxlock_live/ins\endcsname{1.01}
\expandafter\def\csname v@ali_test/voxlock_live/leak_wpm\endcsname{1.37}
\expandafter\def\csname v@ali_test/voxlock_live/miss\endcsname{15.27}
\expandafter\def\csname v@ali_test/voxlock_live/wer\endcsname{16.28}
\expandafter\def\csname v@ali_test/voxlock_pt/dele\endcsname{9.05}
\expandafter\def\csname v@ali_test/voxlock_pt/ins\endcsname{1.00}
\expandafter\def\csname v@ali_test/voxlock_pt/leak_wpm\endcsname{1.01}
\expandafter\def\csname v@ali_test/voxlock_pt/miss\endcsname{14.38}
\expandafter\def\csname v@ali_test/voxlock_pt/wer\endcsname{15.38}
\expandafter\def\csname v@ami_dev/C22_ftlong_kd_selfl/dele\endcsname{3.25}
\expandafter\def\csname v@ami_dev/C22_ftlong_kd_selfl/dleak\endcsname{-1.07}
\expandafter\def\csname v@ami_dev/C22_ftlong_kd_selfl/dwer\endcsname{-0.72}
\expandafter\def\csname v@ami_dev/C22_ftlong_kd_selfl/dwer-hi\endcsname{+0.57}
\expandafter\def\csname v@ami_dev/C22_ftlong_kd_selfl/dwer-lo\endcsname{-2.10}
\expandafter\def\csname v@ami_dev/C22_ftlong_kd_selfl/ins\endcsname{4.38}
\expandafter\def\csname v@ami_dev/C22_ftlong_kd_selfl/leak_wpm\endcsname{8.84}
\expandafter\def\csname v@ami_dev/C22_ftlong_kd_selfl/miss\endcsname{9.24}
\expandafter\def\csname v@ami_dev/C22_ftlong_kd_selfl/wer\endcsname{13.62}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_null/dele\endcsname{3.26}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{-1.47}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-1.05}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+0.07}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-2.25}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_null/ins\endcsname{4.15}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{8.44}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_null/miss\endcsname{9.14}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_null/wer\endcsname{13.29}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{3.29}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-0.76}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-1.11}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+0.04}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-2.36}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{4.16}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{9.15}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{9.07}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{13.23}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_loud/dele\endcsname{3.58}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_loud/dleak\endcsname{-2.23}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_loud/dwer\endcsname{-0.98}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_loud/dwer-hi\endcsname{+0.28}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_loud/dwer-lo\endcsname{-2.30}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_loud/ins\endcsname{3.61}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_loud/leak_wpm\endcsname{7.68}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_loud/miss\endcsname{9.75}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_loud/wer\endcsname{13.36}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_null/dele\endcsname{3.11}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_null/dleak\endcsname{-0.27}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_null/dwer\endcsname{-0.44}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_null/dwer-hi\endcsname{+1.02}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_null/dwer-lo\endcsname{-1.89}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_null/ins\endcsname{4.88}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_null/leak_wpm\endcsname{9.64}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_null/miss\endcsname{9.02}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_null/wer\endcsname{13.90}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_selfl/dele\endcsname{2.95}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_selfl/dleak\endcsname{-1.61}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_selfl/dwer\endcsname{-1.17}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_selfl/dwer-hi\endcsname{+0.13}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_selfl/dwer-lo\endcsname{-2.48}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_selfl/ins\endcsname{4.40}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_selfl/leak_wpm\endcsname{8.30}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_selfl/miss\endcsname{8.78}
\expandafter\def\csname v@ami_dev/MB_ftlong_ws_selfl/wer\endcsname{13.18}
\expandafter\def\csname v@ami_dev/SB_ftlong_ws_selfl/dele\endcsname{3.11}
\expandafter\def\csname v@ami_dev/SB_ftlong_ws_selfl/dleak\endcsname{-1.70}
\expandafter\def\csname v@ami_dev/SB_ftlong_ws_selfl/dwer\endcsname{-1.11}
\expandafter\def\csname v@ami_dev/SB_ftlong_ws_selfl/dwer-hi\endcsname{+0.10}
\expandafter\def\csname v@ami_dev/SB_ftlong_ws_selfl/dwer-lo\endcsname{-2.36}
\expandafter\def\csname v@ami_dev/SB_ftlong_ws_selfl/ins\endcsname{4.05}
\expandafter\def\csname v@ami_dev/SB_ftlong_ws_selfl/leak_wpm\endcsname{8.21}
\expandafter\def\csname v@ami_dev/SB_ftlong_ws_selfl/miss\endcsname{9.18}
\expandafter\def\csname v@ami_dev/SB_ftlong_ws_selfl/wer\endcsname{13.23}
\expandafter\def\csname v@ami_dev/dfn3/dele\endcsname{4.88}
\expandafter\def\csname v@ami_dev/dfn3/dleak\endcsname{+74.87}
\expandafter\def\csname v@ami_dev/dfn3/dwer\endcsname{+27.37}
\expandafter\def\csname v@ami_dev/dfn3/dwer-hi\endcsname{+32.61}
\expandafter\def\csname v@ami_dev/dfn3/dwer-lo\endcsname{+22.14}
\expandafter\def\csname v@ami_dev/dfn3/ins\endcsname{30.32}
\expandafter\def\csname v@ami_dev/dfn3/leak_wpm\endcsname{84.78}
\expandafter\def\csname v@ami_dev/dfn3/miss\endcsname{11.39}
\expandafter\def\csname v@ami_dev/dfn3/wer\endcsname{41.71}
\expandafter\def\csname v@ami_dev/raw/dele\endcsname{3.25}
\expandafter\def\csname v@ami_dev/raw/dleak\endcsname{+112.86}
\expandafter\def\csname v@ami_dev/raw/dwer\endcsname{+38.58}
\expandafter\def\csname v@ami_dev/raw/dwer-hi\endcsname{+43.08}
\expandafter\def\csname v@ami_dev/raw/dwer-lo\endcsname{+34.32}
\expandafter\def\csname v@ami_dev/raw/ins\endcsname{41.75}
\expandafter\def\csname v@ami_dev/raw/leak_wpm\endcsname{122.77}
\expandafter\def\csname v@ami_dev/raw/miss\endcsname{11.17}
\expandafter\def\csname v@ami_dev/raw/wer\endcsname{52.92}
\expandafter\def\csname v@ami_dev/sidon_v2/dele\endcsname{3.83}
\expandafter\def\csname v@ami_dev/sidon_v2/dleak\endcsname{+126.65}
\expandafter\def\csname v@ami_dev/sidon_v2/dwer\endcsname{+43.33}
\expandafter\def\csname v@ami_dev/sidon_v2/dwer-hi\endcsname{+48.20}
\expandafter\def\csname v@ami_dev/sidon_v2/dwer-lo\endcsname{+38.51}
\expandafter\def\csname v@ami_dev/sidon_v2/ins\endcsname{46.84}
\expandafter\def\csname v@ami_dev/sidon_v2/leak_wpm\endcsname{136.56}
\expandafter\def\csname v@ami_dev/sidon_v2/miss\endcsname{10.83}
\expandafter\def\csname v@ami_dev/sidon_v2/wer\endcsname{57.68}
\expandafter\def\csname v@ami_dev/sidon_vi/dele\endcsname{3.45}
\expandafter\def\csname v@ami_dev/sidon_vi/dleak\endcsname{+97.63}
\expandafter\def\csname v@ami_dev/sidon_vi/dwer\endcsname{+31.32}
\expandafter\def\csname v@ami_dev/sidon_vi/dwer-hi\endcsname{+34.60}
\expandafter\def\csname v@ami_dev/sidon_vi/dwer-lo\endcsname{+27.85}
\expandafter\def\csname v@ami_dev/sidon_vi/ins\endcsname{35.80}
\expandafter\def\csname v@ami_dev/sidon_vi/leak_wpm\endcsname{107.55}
\expandafter\def\csname v@ami_dev/sidon_vi/miss\endcsname{9.86}
\expandafter\def\csname v@ami_dev/sidon_vi/wer\endcsname{45.67}
\expandafter\def\csname v@ami_dev/sidon_vi_lite/dele\endcsname{3.27}
\expandafter\def\csname v@ami_dev/sidon_vi_lite/dleak\endcsname{+67.32}
\expandafter\def\csname v@ami_dev/sidon_vi_lite/dwer\endcsname{+21.00}
\expandafter\def\csname v@ami_dev/sidon_vi_lite/dwer-hi\endcsname{+24.90}
\expandafter\def\csname v@ami_dev/sidon_vi_lite/dwer-lo\endcsname{+17.15}
\expandafter\def\csname v@ami_dev/sidon_vi_lite/ins\endcsname{25.59}
\expandafter\def\csname v@ami_dev/sidon_vi_lite/leak_wpm\endcsname{77.23}
\expandafter\def\csname v@ami_dev/sidon_vi_lite/miss\endcsname{9.75}
\expandafter\def\csname v@ami_dev/sidon_vi_lite/wer\endcsname{35.34}
\expandafter\def\csname v@ami_dev/voxlock/dele\endcsname{3.90}
\expandafter\def\csname v@ami_dev/voxlock/dleak\endcsname{-1.74}
\expandafter\def\csname v@ami_dev/voxlock/dwer\endcsname{-0.86}
\expandafter\def\csname v@ami_dev/voxlock/dwer-hi\endcsname{-0.22}
\expandafter\def\csname v@ami_dev/voxlock/dwer-lo\endcsname{-1.63}
\expandafter\def\csname v@ami_dev/voxlock/ins\endcsname{3.80}
\expandafter\def\csname v@ami_dev/voxlock/leak_wpm\endcsname{8.17}
\expandafter\def\csname v@ami_dev/voxlock/miss\endcsname{9.68}
\expandafter\def\csname v@ami_dev/voxlock/wer\endcsname{13.48}
\expandafter\def\csname v@ami_dev/voxlock_live/dele\endcsname{4.11}
\expandafter\def\csname v@ami_dev/voxlock_live/dleak\endcsname{+3.21}
\expandafter\def\csname v@ami_dev/voxlock_live/dwer\endcsname{+2.04}
\expandafter\def\csname v@ami_dev/voxlock_live/dwer-hi\endcsname{+3.65}
\expandafter\def\csname v@ami_dev/voxlock_live/dwer-lo\endcsname{+0.48}
\expandafter\def\csname v@ami_dev/voxlock_live/ins\endcsname{6.64}
\expandafter\def\csname v@ami_dev/voxlock_live/leak_wpm\endcsname{13.13}
\expandafter\def\csname v@ami_dev/voxlock_live/miss\endcsname{9.74}
\expandafter\def\csname v@ami_dev/voxlock_live/wer\endcsname{16.38}
\expandafter\def\csname v@ami_dev/voxlock_pt/dele\endcsname{4.20}
\expandafter\def\csname v@ami_dev/voxlock_pt/ins\endcsname{4.33}
\expandafter\def\csname v@ami_dev/voxlock_pt/leak_wpm\endcsname{9.91}
\expandafter\def\csname v@ami_dev/voxlock_pt/miss\endcsname{10.02}
\expandafter\def\csname v@ami_dev/voxlock_pt/wer\endcsname{14.34}
\expandafter\def\csname v@ami_dev_long/C22_ftlong_kd_selfl/dele\endcsname{7.17}
\expandafter\def\csname v@ami_dev_long/C22_ftlong_kd_selfl/dleak\endcsname{-2.79}
\expandafter\def\csname v@ami_dev_long/C22_ftlong_kd_selfl/dwer\endcsname{-8.51}
\expandafter\def\csname v@ami_dev_long/C22_ftlong_kd_selfl/dwer-hi\endcsname{-4.90}
\expandafter\def\csname v@ami_dev_long/C22_ftlong_kd_selfl/dwer-lo\endcsname{-12.09}
\expandafter\def\csname v@ami_dev_long/C22_ftlong_kd_selfl/ins\endcsname{3.54}
\expandafter\def\csname v@ami_dev_long/C22_ftlong_kd_selfl/leak_wpm\endcsname{6.65}
\expandafter\def\csname v@ami_dev_long/C22_ftlong_kd_selfl/miss\endcsname{14.92}
\expandafter\def\csname v@ami_dev_long/C22_ftlong_kd_selfl/wer\endcsname{18.45}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_null/dele\endcsname{6.34}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{+3.07}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-4.40}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{-0.56}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-8.17}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_null/ins\endcsname{8.41}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{12.50}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_null/miss\endcsname{14.15}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_null/wer\endcsname{22.57}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{7.76}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-3.81}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-8.97}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{-5.63}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-12.24}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{2.98}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{5.63}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{15.02}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{18.00}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_loud/dele\endcsname{7.85}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_loud/dleak\endcsname{-1.69}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_loud/dwer\endcsname{-7.36}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_loud/dwer-hi\endcsname{-3.32}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_loud/dwer-lo\endcsname{-11.44}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_loud/ins\endcsname{4.73}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_loud/leak_wpm\endcsname{7.74}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_loud/miss\endcsname{14.88}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_loud/wer\endcsname{19.61}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_null/dele\endcsname{7.08}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_null/dleak\endcsname{+6.58}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_null/dwer\endcsname{-0.73}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_null/dwer-hi\endcsname{+4.18}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_null/dwer-lo\endcsname{-5.45}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_null/ins\endcsname{11.76}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_null/leak_wpm\endcsname{16.02}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_null/miss\endcsname{14.48}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_null/wer\endcsname{26.24}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_selfl/dele\endcsname{7.04}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_selfl/dleak\endcsname{-1.50}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_selfl/dwer\endcsname{-7.51}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_selfl/dwer-hi\endcsname{-3.63}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_selfl/dwer-lo\endcsname{-11.62}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_selfl/ins\endcsname{5.27}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_selfl/leak_wpm\endcsname{7.94}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_selfl/miss\endcsname{14.19}
\expandafter\def\csname v@ami_dev_long/MB_ftlong_ws_selfl/wer\endcsname{19.46}
\expandafter\def\csname v@ami_dev_long/SB_ftlong_ws_selfl/dele\endcsname{8.29}
\expandafter\def\csname v@ami_dev_long/SB_ftlong_ws_selfl/dleak\endcsname{-1.92}
\expandafter\def\csname v@ami_dev_long/SB_ftlong_ws_selfl/dwer\endcsname{-6.95}
\expandafter\def\csname v@ami_dev_long/SB_ftlong_ws_selfl/dwer-hi\endcsname{-3.78}
\expandafter\def\csname v@ami_dev_long/SB_ftlong_ws_selfl/dwer-lo\endcsname{-10.10}
\expandafter\def\csname v@ami_dev_long/SB_ftlong_ws_selfl/ins\endcsname{4.17}
\expandafter\def\csname v@ami_dev_long/SB_ftlong_ws_selfl/leak_wpm\endcsname{7.52}
\expandafter\def\csname v@ami_dev_long/SB_ftlong_ws_selfl/miss\endcsname{15.85}
\expandafter\def\csname v@ami_dev_long/SB_ftlong_ws_selfl/wer\endcsname{20.02}
\expandafter\def\csname v@ami_dev_long/dfn3/dele\endcsname{6.08}
\expandafter\def\csname v@ami_dev_long/dfn3/dleak\endcsname{+82.54}
\expandafter\def\csname v@ami_dev_long/dfn3/dwer\endcsname{+62.86}
\expandafter\def\csname v@ami_dev_long/dfn3/dwer-hi\endcsname{+80.05}
\expandafter\def\csname v@ami_dev_long/dfn3/dwer-lo\endcsname{+47.44}
\expandafter\def\csname v@ami_dev_long/dfn3/ins\endcsname{75.17}
\expandafter\def\csname v@ami_dev_long/dfn3/leak_wpm\endcsname{91.98}
\expandafter\def\csname v@ami_dev_long/dfn3/miss\endcsname{14.66}
\expandafter\def\csname v@ami_dev_long/dfn3/wer\endcsname{89.83}
\expandafter\def\csname v@ami_dev_long/raw/dele\endcsname{1.69}
\expandafter\def\csname v@ami_dev_long/raw/dleak\endcsname{+146.05}
\expandafter\def\csname v@ami_dev_long/raw/dwer\endcsname{+114.59}
\expandafter\def\csname v@ami_dev_long/raw/dwer-hi\endcsname{+131.90}
\expandafter\def\csname v@ami_dev_long/raw/dwer-lo\endcsname{+99.27}
\expandafter\def\csname v@ami_dev_long/raw/ins\endcsname{129.22}
\expandafter\def\csname v@ami_dev_long/raw/leak_wpm\endcsname{155.49}
\expandafter\def\csname v@ami_dev_long/raw/miss\endcsname{12.33}
\expandafter\def\csname v@ami_dev_long/raw/wer\endcsname{141.56}
\expandafter\def\csname v@ami_dev_long/sidon_vi/dele\endcsname{2.18}
\expandafter\def\csname v@ami_dev_long/sidon_vi/dleak\endcsname{+117.93}
\expandafter\def\csname v@ami_dev_long/sidon_vi/dwer\endcsname{+85.39}
\expandafter\def\csname v@ami_dev_long/sidon_vi/dwer-hi\endcsname{+100.44}
\expandafter\def\csname v@ami_dev_long/sidon_vi/dwer-lo\endcsname{+72.14}
\expandafter\def\csname v@ami_dev_long/sidon_vi/ins\endcsname{100.66}
\expandafter\def\csname v@ami_dev_long/sidon_vi/leak_wpm\endcsname{127.37}
\expandafter\def\csname v@ami_dev_long/sidon_vi/miss\endcsname{11.70}
\expandafter\def\csname v@ami_dev_long/sidon_vi/wer\endcsname{112.36}
\expandafter\def\csname v@ami_dev_long/sidon_vi_lite/dele\endcsname{2.20}
\expandafter\def\csname v@ami_dev_long/sidon_vi_lite/dleak\endcsname{+90.06}
\expandafter\def\csname v@ami_dev_long/sidon_vi_lite/dwer\endcsname{+63.93}
\expandafter\def\csname v@ami_dev_long/sidon_vi_lite/dwer-hi\endcsname{+77.00}
\expandafter\def\csname v@ami_dev_long/sidon_vi_lite/dwer-lo\endcsname{+51.83}
\expandafter\def\csname v@ami_dev_long/sidon_vi_lite/ins\endcsname{78.75}
\expandafter\def\csname v@ami_dev_long/sidon_vi_lite/leak_wpm\endcsname{99.50}
\expandafter\def\csname v@ami_dev_long/sidon_vi_lite/miss\endcsname{12.15}
\expandafter\def\csname v@ami_dev_long/sidon_vi_lite/wer\endcsname{90.90}
\expandafter\def\csname v@ami_dev_long/voxlock/dele\endcsname{13.34}
\expandafter\def\csname v@ami_dev_long/voxlock/dleak\endcsname{-3.26}
\expandafter\def\csname v@ami_dev_long/voxlock/dwer\endcsname{-3.31}
\expandafter\def\csname v@ami_dev_long/voxlock/dwer-hi\endcsname{-0.96}
\expandafter\def\csname v@ami_dev_long/voxlock/dwer-lo\endcsname{-5.86}
\expandafter\def\csname v@ami_dev_long/voxlock/ins\endcsname{2.83}
\expandafter\def\csname v@ami_dev_long/voxlock/leak_wpm\endcsname{6.18}
\expandafter\def\csname v@ami_dev_long/voxlock/miss\endcsname{20.83}
\expandafter\def\csname v@ami_dev_long/voxlock/wer\endcsname{23.66}
\expandafter\def\csname v@ami_dev_long/voxlock_live/dele\endcsname{12.68}
\expandafter\def\csname v@ami_dev_long/voxlock_live/dleak\endcsname{+1.31}
\expandafter\def\csname v@ami_dev_long/voxlock_live/dwer\endcsname{+0.42}
\expandafter\def\csname v@ami_dev_long/voxlock_live/dwer-hi\endcsname{+4.09}
\expandafter\def\csname v@ami_dev_long/voxlock_live/dwer-lo\endcsname{-3.14}
\expandafter\def\csname v@ami_dev_long/voxlock_live/ins\endcsname{6.50}
\expandafter\def\csname v@ami_dev_long/voxlock_live/leak_wpm\endcsname{10.75}
\expandafter\def\csname v@ami_dev_long/voxlock_live/miss\endcsname{20.89}
\expandafter\def\csname v@ami_dev_long/voxlock_live/wer\endcsname{27.39}
\expandafter\def\csname v@ami_dev_long/voxlock_pt/dele\endcsname{14.23}
\expandafter\def\csname v@ami_dev_long/voxlock_pt/ins\endcsname{5.07}
\expandafter\def\csname v@ami_dev_long/voxlock_pt/leak_wpm\endcsname{9.44}
\expandafter\def\csname v@ami_dev_long/voxlock_pt/miss\endcsname{21.90}
\expandafter\def\csname v@ami_dev_long/voxlock_pt/wer\endcsname{26.97}
\expandafter\def\csname v@ami_headset2/C22_ftlong_kd_selfl/dele\endcsname{3.35}
\expandafter\def\csname v@ami_headset2/C22_ftlong_kd_selfl/dleak\endcsname{+0.40}
\expandafter\def\csname v@ami_headset2/C22_ftlong_kd_selfl/dwer\endcsname{+0.97}
\expandafter\def\csname v@ami_headset2/C22_ftlong_kd_selfl/dwer-hi\endcsname{+3.53}
\expandafter\def\csname v@ami_headset2/C22_ftlong_kd_selfl/dwer-lo\endcsname{-0.58}
\expandafter\def\csname v@ami_headset2/C22_ftlong_kd_selfl/ins\endcsname{3.32}
\expandafter\def\csname v@ami_headset2/C22_ftlong_kd_selfl/leak_wpm\endcsname{2.52}
\expandafter\def\csname v@ami_headset2/C22_ftlong_kd_selfl/miss\endcsname{7.91}
\expandafter\def\csname v@ami_headset2/C22_ftlong_kd_selfl/wer\endcsname{11.23}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_loud/dele\endcsname{3.25}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_loud/dleak\endcsname{+0.13}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_loud/dwer\endcsname{+1.11}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_loud/dwer-hi\endcsname{+3.90}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_loud/dwer-lo\endcsname{-0.45}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_loud/ins\endcsname{3.39}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_loud/leak_wpm\endcsname{2.25}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_loud/miss\endcsname{7.98}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_loud/wer\endcsname{11.37}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_null/dele\endcsname{2.04}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{+0.13}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-0.24}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+0.26}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-0.63}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_null/ins\endcsname{3.32}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{2.25}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_null/miss\endcsname{6.70}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_null/wer\endcsname{10.02}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{2.04}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{+0.27}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-0.07}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+0.40}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-0.41}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{3.46}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{2.39}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{6.74}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{10.19}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_loud/dele\endcsname{3.49}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_loud/dleak\endcsname{+0.13}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_loud/dwer\endcsname{+0.97}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_loud/dwer-hi\endcsname{+3.57}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_loud/dwer-lo\endcsname{-0.55}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_loud/ins\endcsname{3.14}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_loud/leak_wpm\endcsname{2.25}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_loud/miss\endcsname{8.09}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_loud/wer\endcsname{11.23}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_null/dele\endcsname{2.04}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_null/dleak\endcsname{+0.80}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_null/dwer\endcsname{+0.00}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_null/dwer-hi\endcsname{+0.74}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_null/dwer-lo\endcsname{-0.53}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_null/ins\endcsname{3.42}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_null/leak_wpm\endcsname{2.92}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_null/miss\endcsname{6.84}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_null/wer\endcsname{10.26}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_selfl/dele\endcsname{2.00}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_selfl/dleak\endcsname{+0.13}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_selfl/dwer\endcsname{-0.31}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_selfl/dwer-hi\endcsname{+0.10}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_selfl/dwer-lo\endcsname{-0.64}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_selfl/ins\endcsname{3.28}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_selfl/leak_wpm\endcsname{2.25}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_selfl/miss\endcsname{6.67}
\expandafter\def\csname v@ami_headset2/MB_ftlong_ws_selfl/wer\endcsname{9.95}
\expandafter\def\csname v@ami_headset2/SB_ftlong_ws_selfl/dele\endcsname{2.11}
\expandafter\def\csname v@ami_headset2/SB_ftlong_ws_selfl/dleak\endcsname{+0.00}
\expandafter\def\csname v@ami_headset2/SB_ftlong_ws_selfl/dwer\endcsname{-0.03}
\expandafter\def\csname v@ami_headset2/SB_ftlong_ws_selfl/dwer-hi\endcsname{+0.24}
\expandafter\def\csname v@ami_headset2/SB_ftlong_ws_selfl/dwer-lo\endcsname{-0.30}
\expandafter\def\csname v@ami_headset2/SB_ftlong_ws_selfl/ins\endcsname{3.35}
\expandafter\def\csname v@ami_headset2/SB_ftlong_ws_selfl/leak_wpm\endcsname{2.12}
\expandafter\def\csname v@ami_headset2/SB_ftlong_ws_selfl/miss\endcsname{6.88}
\expandafter\def\csname v@ami_headset2/SB_ftlong_ws_selfl/wer\endcsname{10.23}
\expandafter\def\csname v@ami_headset2/dfn3/dele\endcsname{7.95}
\expandafter\def\csname v@ami_headset2/dfn3/dleak\endcsname{+21.21}
\expandafter\def\csname v@ami_headset2/dfn3/dwer\endcsname{+11.30}
\expandafter\def\csname v@ami_headset2/dfn3/dwer-hi\endcsname{+19.20}
\expandafter\def\csname v@ami_headset2/dfn3/dwer-lo\endcsname{+5.57}
\expandafter\def\csname v@ami_headset2/dfn3/ins\endcsname{8.88}
\expandafter\def\csname v@ami_headset2/dfn3/leak_wpm\endcsname{23.33}
\expandafter\def\csname v@ami_headset2/dfn3/miss\endcsname{12.68}
\expandafter\def\csname v@ami_headset2/dfn3/wer\endcsname{21.56}
\expandafter\def\csname v@ami_headset2/raw/dele\endcsname{3.25}
\expandafter\def\csname v@ami_headset2/raw/dleak\endcsname{+76.08}
\expandafter\def\csname v@ami_headset2/raw/dwer\endcsname{+22.74}
\expandafter\def\csname v@ami_headset2/raw/dwer-hi\endcsname{+29.23}
\expandafter\def\csname v@ami_headset2/raw/dwer-lo\endcsname{+17.85}
\expandafter\def\csname v@ami_headset2/raw/ins\endcsname{24.95}
\expandafter\def\csname v@ami_headset2/raw/leak_wpm\endcsname{78.20}
\expandafter\def\csname v@ami_headset2/raw/miss\endcsname{8.05}
\expandafter\def\csname v@ami_headset2/raw/wer\endcsname{33.00}
\expandafter\def\csname v@ami_headset2/sidon_v2/dele\endcsname{3.52}
\expandafter\def\csname v@ami_headset2/sidon_v2/dleak\endcsname{+119.02}
\expandafter\def\csname v@ami_headset2/sidon_v2/dwer\endcsname{+34.28}
\expandafter\def\csname v@ami_headset2/sidon_v2/dwer-hi\endcsname{+38.66}
\expandafter\def\csname v@ami_headset2/sidon_v2/dwer-lo\endcsname{+31.14}
\expandafter\def\csname v@ami_headset2/sidon_v2/ins\endcsname{35.45}
\expandafter\def\csname v@ami_headset2/sidon_v2/leak_wpm\endcsname{121.14}
\expandafter\def\csname v@ami_headset2/sidon_v2/miss\endcsname{9.09}
\expandafter\def\csname v@ami_headset2/sidon_v2/wer\endcsname{44.54}
\expandafter\def\csname v@ami_headset2/sidon_vi/dele\endcsname{3.80}
\expandafter\def\csname v@ami_headset2/sidon_vi/dleak\endcsname{+77.27}
\expandafter\def\csname v@ami_headset2/sidon_vi/dwer\endcsname{+22.18}
\expandafter\def\csname v@ami_headset2/sidon_vi/dwer-hi\endcsname{+28.37}
\expandafter\def\csname v@ami_headset2/sidon_vi/dwer-lo\endcsname{+17.94}
\expandafter\def\csname v@ami_headset2/sidon_vi/ins\endcsname{23.43}
\expandafter\def\csname v@ami_headset2/sidon_vi/leak_wpm\endcsname{79.39}
\expandafter\def\csname v@ami_headset2/sidon_vi/miss\endcsname{9.02}
\expandafter\def\csname v@ami_headset2/sidon_vi/wer\endcsname{32.45}
\expandafter\def\csname v@ami_headset2/sidon_vi_lite/dele\endcsname{3.80}
\expandafter\def\csname v@ami_headset2/sidon_vi_lite/dleak\endcsname{+18.95}
\expandafter\def\csname v@ami_headset2/sidon_vi_lite/dwer\endcsname{+7.19}
\expandafter\def\csname v@ami_headset2/sidon_vi_lite/dwer-hi\endcsname{+12.35}
\expandafter\def\csname v@ami_headset2/sidon_vi_lite/dwer-lo\endcsname{+3.29}
\expandafter\def\csname v@ami_headset2/sidon_vi_lite/ins\endcsname{8.43}
\expandafter\def\csname v@ami_headset2/sidon_vi_lite/leak_wpm\endcsname{21.07}
\expandafter\def\csname v@ami_headset2/sidon_vi_lite/miss\endcsname{9.02}
\expandafter\def\csname v@ami_headset2/sidon_vi_lite/wer\endcsname{17.45}
\expandafter\def\csname v@ami_headset2/voxlock/dele\endcsname{3.42}
\expandafter\def\csname v@ami_headset2/voxlock/dleak\endcsname{+0.53}
\expandafter\def\csname v@ami_headset2/voxlock/dwer\endcsname{+1.00}
\expandafter\def\csname v@ami_headset2/voxlock/dwer-hi\endcsname{+3.71}
\expandafter\def\csname v@ami_headset2/voxlock/dwer-lo\endcsname{-0.49}
\expandafter\def\csname v@ami_headset2/voxlock/ins\endcsname{3.14}
\expandafter\def\csname v@ami_headset2/voxlock/leak_wpm\endcsname{2.65}
\expandafter\def\csname v@ami_headset2/voxlock/miss\endcsname{8.12}
\expandafter\def\csname v@ami_headset2/voxlock/wer\endcsname{11.26}
\expandafter\def\csname v@ami_headset2/voxlock_live/dele\endcsname{3.49}
\expandafter\def\csname v@ami_headset2/voxlock_live/dleak\endcsname{+0.93}
\expandafter\def\csname v@ami_headset2/voxlock_live/dwer\endcsname{+1.45}
\expandafter\def\csname v@ami_headset2/voxlock_live/dwer-hi\endcsname{+3.96}
\expandafter\def\csname v@ami_headset2/voxlock_live/dwer-lo\endcsname{-0.22}
\expandafter\def\csname v@ami_headset2/voxlock_live/ins\endcsname{3.73}
\expandafter\def\csname v@ami_headset2/voxlock_live/leak_wpm\endcsname{3.05}
\expandafter\def\csname v@ami_headset2/voxlock_live/miss\endcsname{7.98}
\expandafter\def\csname v@ami_headset2/voxlock_live/wer\endcsname{11.71}
\expandafter\def\csname v@ami_headset2/voxlock_pt/dele\endcsname{2.21}
\expandafter\def\csname v@ami_headset2/voxlock_pt/ins\endcsname{3.39}
\expandafter\def\csname v@ami_headset2/voxlock_pt/leak_wpm\endcsname{2.12}
\expandafter\def\csname v@ami_headset2/voxlock_pt/miss\endcsname{6.88}
\expandafter\def\csname v@ami_headset2/voxlock_pt/wer\endcsname{10.26}
\expandafter\def\csname v@ami_test/C22_ftlong_kd_selfl/dele\endcsname{2.94}
\expandafter\def\csname v@ami_test/C22_ftlong_kd_selfl/dleak\endcsname{-0.85}
\expandafter\def\csname v@ami_test/C22_ftlong_kd_selfl/dwer\endcsname{-0.02}
\expandafter\def\csname v@ami_test/C22_ftlong_kd_selfl/dwer-hi\endcsname{+0.65}
\expandafter\def\csname v@ami_test/C22_ftlong_kd_selfl/dwer-lo\endcsname{-0.85}
\expandafter\def\csname v@ami_test/C22_ftlong_kd_selfl/ins\endcsname{2.40}
\expandafter\def\csname v@ami_test/C22_ftlong_kd_selfl/leak_wpm\endcsname{1.29}
\expandafter\def\csname v@ami_test/C22_ftlong_kd_selfl/miss\endcsname{7.89}
\expandafter\def\csname v@ami_test/C22_ftlong_kd_selfl/wer\endcsname{10.29}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_loud/dele\endcsname{2.81}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_loud/dleak\endcsname{-0.23}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_loud/dwer\endcsname{+0.03}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_loud/dwer-hi\endcsname{+0.70}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_loud/dwer-lo\endcsname{-0.79}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_loud/ins\endcsname{2.51}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_loud/leak_wpm\endcsname{1.90}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_loud/miss\endcsname{7.83}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_loud/wer\endcsname{10.35}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_null/dele\endcsname{2.68}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{-0.23}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-0.22}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+0.30}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-0.94}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_null/ins\endcsname{2.55}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{1.90}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_null/miss\endcsname{7.54}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_null/wer\endcsname{10.09}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{2.62}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-0.23}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-0.13}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+0.52}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-0.97}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{2.67}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{1.90}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{7.51}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{10.18}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_loud/dele\endcsname{3.16}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_loud/dleak\endcsname{-0.26}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_loud/dwer\endcsname{+0.31}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_loud/dwer-hi\endcsname{+1.12}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_loud/dwer-lo\endcsname{-0.60}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_loud/ins\endcsname{2.49}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_loud/leak_wpm\endcsname{1.87}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_loud/miss\endcsname{8.13}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_loud/wer\endcsname{10.62}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_null/dele\endcsname{2.83}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_null/dleak\endcsname{-0.50}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_null/dwer\endcsname{-0.04}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_null/dwer-hi\endcsname{+0.61}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_null/dwer-lo\endcsname{-0.83}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_null/ins\endcsname{2.44}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_null/leak_wpm\endcsname{1.64}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_null/miss\endcsname{7.83}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_null/wer\endcsname{10.27}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_selfl/dele\endcsname{2.92}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_selfl/dleak\endcsname{-0.12}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_selfl/dwer\endcsname{+0.19}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_selfl/dwer-hi\endcsname{+1.17}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_selfl/dwer-lo\endcsname{-0.76}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_selfl/ins\endcsname{2.56}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_selfl/leak_wpm\endcsname{2.02}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_selfl/miss\endcsname{7.95}
\expandafter\def\csname v@ami_test/MB_ftlong_ws_selfl/wer\endcsname{10.51}
\expandafter\def\csname v@ami_test/SB_ftlong_ws_selfl/dele\endcsname{3.12}
\expandafter\def\csname v@ami_test/SB_ftlong_ws_selfl/dleak\endcsname{-0.59}
\expandafter\def\csname v@ami_test/SB_ftlong_ws_selfl/dwer\endcsname{+0.15}
\expandafter\def\csname v@ami_test/SB_ftlong_ws_selfl/dwer-hi\endcsname{+0.87}
\expandafter\def\csname v@ami_test/SB_ftlong_ws_selfl/dwer-lo\endcsname{-0.74}
\expandafter\def\csname v@ami_test/SB_ftlong_ws_selfl/ins\endcsname{2.41}
\expandafter\def\csname v@ami_test/SB_ftlong_ws_selfl/leak_wpm\endcsname{1.55}
\expandafter\def\csname v@ami_test/SB_ftlong_ws_selfl/miss\endcsname{8.05}
\expandafter\def\csname v@ami_test/SB_ftlong_ws_selfl/wer\endcsname{10.47}
\expandafter\def\csname v@ami_test/dfn3/dele\endcsname{8.90}
\expandafter\def\csname v@ami_test/dfn3/dleak\endcsname{+30.66}
\expandafter\def\csname v@ami_test/dfn3/dwer\endcsname{+15.69}
\expandafter\def\csname v@ami_test/dfn3/dwer-hi\endcsname{+19.51}
\expandafter\def\csname v@ami_test/dfn3/dwer-lo\endcsname{+12.53}
\expandafter\def\csname v@ami_test/dfn3/ins\endcsname{11.60}
\expandafter\def\csname v@ami_test/dfn3/leak_wpm\endcsname{32.79}
\expandafter\def\csname v@ami_test/dfn3/miss\endcsname{14.40}
\expandafter\def\csname v@ami_test/dfn3/wer\endcsname{26.00}
\expandafter\def\csname v@ami_test/raw/dele\endcsname{3.56}
\expandafter\def\csname v@ami_test/raw/dleak\endcsname{+99.26}
\expandafter\def\csname v@ami_test/raw/dwer\endcsname{+32.28}
\expandafter\def\csname v@ami_test/raw/dwer-hi\endcsname{+36.23}
\expandafter\def\csname v@ami_test/raw/dwer-lo\endcsname{+28.55}
\expandafter\def\csname v@ami_test/raw/ins\endcsname{32.84}
\expandafter\def\csname v@ami_test/raw/leak_wpm\endcsname{101.40}
\expandafter\def\csname v@ami_test/raw/miss\endcsname{9.75}
\expandafter\def\csname v@ami_test/raw/wer\endcsname{42.59}
\expandafter\def\csname v@ami_test/sidon_v2/dele\endcsname{2.72}
\expandafter\def\csname v@ami_test/sidon_v2/dleak\endcsname{+128.66}
\expandafter\def\csname v@ami_test/sidon_v2/dwer\endcsname{+39.61}
\expandafter\def\csname v@ami_test/sidon_v2/dwer-hi\endcsname{+43.48}
\expandafter\def\csname v@ami_test/sidon_v2/dwer-lo\endcsname{+35.51}
\expandafter\def\csname v@ami_test/sidon_v2/ins\endcsname{40.62}
\expandafter\def\csname v@ami_test/sidon_v2/leak_wpm\endcsname{130.80}
\expandafter\def\csname v@ami_test/sidon_v2/miss\endcsname{9.30}
\expandafter\def\csname v@ami_test/sidon_v2/wer\endcsname{49.92}
\expandafter\def\csname v@ami_test/sidon_vi/dele\endcsname{2.65}
\expandafter\def\csname v@ami_test/sidon_vi/dleak\endcsname{+95.90}
\expandafter\def\csname v@ami_test/sidon_vi/dwer\endcsname{+27.20}
\expandafter\def\csname v@ami_test/sidon_vi/dwer-hi\endcsname{+30.11}
\expandafter\def\csname v@ami_test/sidon_vi/dwer-lo\endcsname{+23.91}
\expandafter\def\csname v@ami_test/sidon_vi/ins\endcsname{29.04}
\expandafter\def\csname v@ami_test/sidon_vi/leak_wpm\endcsname{98.03}
\expandafter\def\csname v@ami_test/sidon_vi/miss\endcsname{8.47}
\expandafter\def\csname v@ami_test/sidon_vi/wer\endcsname{37.51}
\expandafter\def\csname v@ami_test/sidon_vi_lite/dele\endcsname{2.58}
\expandafter\def\csname v@ami_test/sidon_vi_lite/dleak\endcsname{+47.13}
\expandafter\def\csname v@ami_test/sidon_vi_lite/dwer\endcsname{+13.75}
\expandafter\def\csname v@ami_test/sidon_vi_lite/dwer-hi\endcsname{+16.67}
\expandafter\def\csname v@ami_test/sidon_vi_lite/dwer-lo\endcsname{+10.90}
\expandafter\def\csname v@ami_test/sidon_vi_lite/ins\endcsname{15.81}
\expandafter\def\csname v@ami_test/sidon_vi_lite/leak_wpm\endcsname{49.26}
\expandafter\def\csname v@ami_test/sidon_vi_lite/miss\endcsname{8.26}
\expandafter\def\csname v@ami_test/sidon_vi_lite/wer\endcsname{24.06}
\expandafter\def\csname v@ami_test/voxlock/dele\endcsname{2.84}
\expandafter\def\csname v@ami_test/voxlock/dleak\endcsname{-0.94}
\expandafter\def\csname v@ami_test/voxlock/dwer\endcsname{-0.62}
\expandafter\def\csname v@ami_test/voxlock/dwer-hi\endcsname{-0.12}
\expandafter\def\csname v@ami_test/voxlock/dwer-lo\endcsname{-1.34}
\expandafter\def\csname v@ami_test/voxlock/ins\endcsname{2.17}
\expandafter\def\csname v@ami_test/voxlock/leak_wpm\endcsname{1.20}
\expandafter\def\csname v@ami_test/voxlock/miss\endcsname{7.53}
\expandafter\def\csname v@ami_test/voxlock/wer\endcsname{9.70}
\expandafter\def\csname v@ami_test/voxlock_live/dele\endcsname{3.27}
\expandafter\def\csname v@ami_test/voxlock_live/dleak\endcsname{+1.67}
\expandafter\def\csname v@ami_test/voxlock_live/dwer\endcsname{+1.76}
\expandafter\def\csname v@ami_test/voxlock_live/dwer-hi\endcsname{+2.83}
\expandafter\def\csname v@ami_test/voxlock_live/dwer-lo\endcsname{+0.76}
\expandafter\def\csname v@ami_test/voxlock_live/ins\endcsname{3.69}
\expandafter\def\csname v@ami_test/voxlock_live/leak_wpm\endcsname{3.80}
\expandafter\def\csname v@ami_test/voxlock_live/miss\endcsname{8.39}
\expandafter\def\csname v@ami_test/voxlock_live/wer\endcsname{12.07}
\expandafter\def\csname v@ami_test/voxlock_pt/dele\endcsname{3.10}
\expandafter\def\csname v@ami_test/voxlock_pt/ins\endcsname{2.45}
\expandafter\def\csname v@ami_test/voxlock_pt/leak_wpm\endcsname{2.14}
\expandafter\def\csname v@ami_test/voxlock_pt/miss\endcsname{7.87}
\expandafter\def\csname v@ami_test/voxlock_pt/wer\endcsname{10.31}
\expandafter\def\csname v@ami_test_long/C22_ftlong_kd_selfl/dele\endcsname{6.89}
\expandafter\def\csname v@ami_test_long/C22_ftlong_kd_selfl/dleak\endcsname{-2.39}
\expandafter\def\csname v@ami_test_long/C22_ftlong_kd_selfl/dwer\endcsname{-4.64}
\expandafter\def\csname v@ami_test_long/C22_ftlong_kd_selfl/dwer-hi\endcsname{-2.23}
\expandafter\def\csname v@ami_test_long/C22_ftlong_kd_selfl/dwer-lo\endcsname{-7.62}
\expandafter\def\csname v@ami_test_long/C22_ftlong_kd_selfl/ins\endcsname{3.51}
\expandafter\def\csname v@ami_test_long/C22_ftlong_kd_selfl/leak_wpm\endcsname{3.08}
\expandafter\def\csname v@ami_test_long/C22_ftlong_kd_selfl/miss\endcsname{12.04}
\expandafter\def\csname v@ami_test_long/C22_ftlong_kd_selfl/wer\endcsname{15.55}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_loud/dele\endcsname{6.54}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_loud/dleak\endcsname{-1.57}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_loud/dwer\endcsname{-3.98}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_loud/dwer-hi\endcsname{-1.57}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_loud/dwer-lo\endcsname{-6.98}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_loud/ins\endcsname{4.39}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_loud/leak_wpm\endcsname{3.91}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_loud/miss\endcsname{11.82}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_loud/wer\endcsname{16.22}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_null/dele\endcsname{5.89}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{-0.13}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-4.01}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{-0.43}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-8.02}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_null/ins\endcsname{5.09}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{5.34}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_null/miss\endcsname{11.10}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_null/wer\endcsname{16.19}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{6.30}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-1.36}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-4.07}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{-1.68}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-7.02}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{4.58}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{4.11}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{11.55}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{16.13}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_loud/dele\endcsname{7.75}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_loud/dleak\endcsname{-2.39}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_loud/dwer\endcsname{-3.75}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_loud/dwer-hi\endcsname{-0.98}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_loud/dwer-lo\endcsname{-7.03}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_loud/ins\endcsname{3.46}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_loud/leak_wpm\endcsname{3.08}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_loud/miss\endcsname{12.98}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_loud/wer\endcsname{16.44}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_null/dele\endcsname{6.80}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_null/dleak\endcsname{+1.25}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_null/dwer\endcsname{-1.80}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_null/dwer-hi\endcsname{+2.53}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_null/dwer-lo\endcsname{-5.64}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_null/ins\endcsname{6.40}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_null/leak_wpm\endcsname{6.72}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_null/miss\endcsname{11.99}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_null/wer\endcsname{18.39}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_selfl/dele\endcsname{7.69}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_selfl/dleak\endcsname{-1.88}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_selfl/dwer\endcsname{-3.36}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_selfl/dwer-hi\endcsname{-0.63}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_selfl/dwer-lo\endcsname{-6.41}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_selfl/ins\endcsname{3.90}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_selfl/leak_wpm\endcsname{3.59}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_selfl/miss\endcsname{12.94}
\expandafter\def\csname v@ami_test_long/MB_ftlong_ws_selfl/wer\endcsname{16.84}
\expandafter\def\csname v@ami_test_long/SB_ftlong_ws_selfl/dele\endcsname{6.60}
\expandafter\def\csname v@ami_test_long/SB_ftlong_ws_selfl/dleak\endcsname{-2.37}
\expandafter\def\csname v@ami_test_long/SB_ftlong_ws_selfl/dwer\endcsname{-4.72}
\expandafter\def\csname v@ami_test_long/SB_ftlong_ws_selfl/dwer-hi\endcsname{-2.29}
\expandafter\def\csname v@ami_test_long/SB_ftlong_ws_selfl/dwer-lo\endcsname{-7.81}
\expandafter\def\csname v@ami_test_long/SB_ftlong_ws_selfl/ins\endcsname{3.74}
\expandafter\def\csname v@ami_test_long/SB_ftlong_ws_selfl/leak_wpm\endcsname{3.10}
\expandafter\def\csname v@ami_test_long/SB_ftlong_ws_selfl/miss\endcsname{11.74}
\expandafter\def\csname v@ami_test_long/SB_ftlong_ws_selfl/wer\endcsname{15.48}
\expandafter\def\csname v@ami_test_long/dfn3/dele\endcsname{15.08}
\expandafter\def\csname v@ami_test_long/dfn3/dleak\endcsname{+18.90}
\expandafter\def\csname v@ami_test_long/dfn3/dwer\endcsname{+21.57}
\expandafter\def\csname v@ami_test_long/dfn3/dwer-hi\endcsname{+31.79}
\expandafter\def\csname v@ami_test_long/dfn3/dwer-lo\endcsname{+14.69}
\expandafter\def\csname v@ami_test_long/dfn3/ins\endcsname{19.60}
\expandafter\def\csname v@ami_test_long/dfn3/leak_wpm\endcsname{24.37}
\expandafter\def\csname v@ami_test_long/dfn3/miss\endcsname{22.17}
\expandafter\def\csname v@ami_test_long/dfn3/wer\endcsname{41.77}
\expandafter\def\csname v@ami_test_long/raw/dele\endcsname{2.75}
\expandafter\def\csname v@ami_test_long/raw/dleak\endcsname{+131.70}
\expandafter\def\csname v@ami_test_long/raw/dwer\endcsname{+101.59}
\expandafter\def\csname v@ami_test_long/raw/dwer-hi\endcsname{+122.96}
\expandafter\def\csname v@ami_test_long/raw/dwer-lo\endcsname{+82.24}
\expandafter\def\csname v@ami_test_long/raw/ins\endcsname{108.71}
\expandafter\def\csname v@ami_test_long/raw/leak_wpm\endcsname{137.17}
\expandafter\def\csname v@ami_test_long/raw/miss\endcsname{13.08}
\expandafter\def\csname v@ami_test_long/raw/wer\endcsname{121.79}
\expandafter\def\csname v@ami_test_long/sidon_vi/dele\endcsname{2.63}
\expandafter\def\csname v@ami_test_long/sidon_vi/dleak\endcsname{+113.45}
\expandafter\def\csname v@ami_test_long/sidon_vi/dwer\endcsname{+81.61}
\expandafter\def\csname v@ami_test_long/sidon_vi/dwer-hi\endcsname{+98.84}
\expandafter\def\csname v@ami_test_long/sidon_vi/dwer-lo\endcsname{+65.07}
\expandafter\def\csname v@ami_test_long/sidon_vi/ins\endcsname{91.76}
\expandafter\def\csname v@ami_test_long/sidon_vi/leak_wpm\endcsname{118.92}
\expandafter\def\csname v@ami_test_long/sidon_vi/miss\endcsname{10.04}
\expandafter\def\csname v@ami_test_long/sidon_vi/wer\endcsname{101.80}
\expandafter\def\csname v@ami_test_long/sidon_vi_lite/dele\endcsname{4.03}
\expandafter\def\csname v@ami_test_long/sidon_vi_lite/dleak\endcsname{+65.41}
\expandafter\def\csname v@ami_test_long/sidon_vi_lite/dwer\endcsname{+45.95}
\expandafter\def\csname v@ami_test_long/sidon_vi_lite/dwer-hi\endcsname{+60.76}
\expandafter\def\csname v@ami_test_long/sidon_vi_lite/dwer-lo\endcsname{+34.42}
\expandafter\def\csname v@ami_test_long/sidon_vi_lite/ins\endcsname{53.46}
\expandafter\def\csname v@ami_test_long/sidon_vi_lite/leak_wpm\endcsname{70.88}
\expandafter\def\csname v@ami_test_long/sidon_vi_lite/miss\endcsname{12.69}
\expandafter\def\csname v@ami_test_long/sidon_vi_lite/wer\endcsname{66.15}
\expandafter\def\csname v@ami_test_long/voxlock/dele\endcsname{10.55}
\expandafter\def\csname v@ami_test_long/voxlock/dleak\endcsname{-1.74}
\expandafter\def\csname v@ami_test_long/voxlock/dwer\endcsname{-0.67}
\expandafter\def\csname v@ami_test_long/voxlock/dwer-hi\endcsname{+0.98}
\expandafter\def\csname v@ami_test_long/voxlock/dwer-lo\endcsname{-3.01}
\expandafter\def\csname v@ami_test_long/voxlock/ins\endcsname{3.57}
\expandafter\def\csname v@ami_test_long/voxlock/leak_wpm\endcsname{3.73}
\expandafter\def\csname v@ami_test_long/voxlock/miss\endcsname{15.95}
\expandafter\def\csname v@ami_test_long/voxlock/wer\endcsname{19.52}
\expandafter\def\csname v@ami_test_long/voxlock_live/dele\endcsname{10.15}
\expandafter\def\csname v@ami_test_long/voxlock_live/dleak\endcsname{+3.64}
\expandafter\def\csname v@ami_test_long/voxlock_live/dwer\endcsname{+3.46}
\expandafter\def\csname v@ami_test_long/voxlock_live/dwer-hi\endcsname{+6.01}
\expandafter\def\csname v@ami_test_long/voxlock_live/dwer-lo\endcsname{+1.10}
\expandafter\def\csname v@ami_test_long/voxlock_live/ins\endcsname{7.66}
\expandafter\def\csname v@ami_test_long/voxlock_live/leak_wpm\endcsname{9.11}
\expandafter\def\csname v@ami_test_long/voxlock_live/miss\endcsname{16.00}
\expandafter\def\csname v@ami_test_long/voxlock_live/wer\endcsname{23.66}
\expandafter\def\csname v@ami_test_long/voxlock_pt/dele\endcsname{9.39}
\expandafter\def\csname v@ami_test_long/voxlock_pt/ins\endcsname{5.41}
\expandafter\def\csname v@ami_test_long/voxlock_pt/leak_wpm\endcsname{5.47}
\expandafter\def\csname v@ami_test_long/voxlock_pt/miss\endcsname{14.78}
\expandafter\def\csname v@ami_test_long/voxlock_pt/wer\endcsname{20.20}
\expandafter\def\csname v@bge/ami_dev_long/C10_ftlong_kd_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C10_ftlong_kd_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C10_ftlong_kd_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C10_ftlong_kd_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C10_ftlong_kd_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_ini_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_ini_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_ini_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_ini_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_ini_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kd_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kd_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kd_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kd_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kd_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kdo_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kdo_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kdo_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kdo_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_kdo_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_sc_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_sc_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_sc_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_sc_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C22_ftlong_sc_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C51_ftlong_kd_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C51_ftlong_kd_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/C51_ftlong_kd_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C51_ftlong_kd_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/C51_ftlong_kd_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_selfl/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_sslp_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_cwlt2_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_ftlong_ws_slow_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_null/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_k004_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_lvl_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_null/b0\endcsname{-5}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_null/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_null/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_self/b0\endcsname{-5}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_self/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_self/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_self/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LB_long_self/b4\endcsname{-5}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_null/b3\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_null/b4\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LB_main_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_null/b4\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_self/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_self/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LC_seg24_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_null/b4\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem4_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_null/b4\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_mem_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_null/b4\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_null/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_self/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_self/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_mem_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_null/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_self/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/LC_turns_w1k_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_self/b0\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_self/b0\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_selfl/b0\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_sslp_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t2_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwl0t_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlf_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g5_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2g_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2gm_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2hm_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2m_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2mr_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2mr_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2mr_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2mr_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2mr_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2p_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2r_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2r_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2r_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2r_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt2r_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_cwlt_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbl0t_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_hbx0t_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_sslb_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b0t_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_w2b2_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs0t_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_whs2_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls0t_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_ws_xls2_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_ftlong_wsp_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_null/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_null/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_self/b0\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_self/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_k004_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_null/b0\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_null/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_null/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_self/b0\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_self/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_lvl_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_null/b0\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_null/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_null/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_self/b0\endcsname{-5}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_long_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_null/b1\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_null/b3\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_null/b4\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/MB_main_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_null/b0\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_null/b1\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_null/b3\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_null/b4\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_base_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_null/b0\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_null/b1\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_null/b3\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_null/b4\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_selfl/b1\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ft_selfl/b4\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_em_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_k2000_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_solo_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslb_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_sslp_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wob_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2c_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2g_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gc_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2gm_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2h_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_null/b0\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2m_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2mr_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2mr_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2mr_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2mr_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2mr_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2r_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2r_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2r_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2r_selfl/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_cwlt2r_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_ws_sslb_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_ftlong_wsp_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_null/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_far_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_self/b0\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_k03_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_keep_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lk_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_loud/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_loud/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_loud/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_loud/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_loud/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_null/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_selfl/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_lvl_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_null/b0\endcsname{-5}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_null/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_self/b0\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_null/b0\endcsname{-5}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_null/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_self/b0\endcsname{-5}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sir_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_self/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_self/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_spk_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_null/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_self/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_selfl/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_selfl/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_selfl/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_selfl/b3\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_ssl_selfl/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_loud/b0\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_loud/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_loud/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_loud/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_loud/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_null/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/SB_long_sslb_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/dfn3/b0\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/dfn3/b1\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/dfn3/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/dfn3/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/dfn3/b4\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_null/b0\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_null/b3\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_null/b4\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_self/b4\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_selfa/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_selfa/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_selfa/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_selfa/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_off_selfa/b4\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_null/b1\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_null/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_null/b4\endcsname{-1}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_self/b3\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/ftlb_on_self/b4\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/voxlock/b0\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/voxlock/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/voxlock/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/voxlock/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/voxlock/b4\endcsname{-8}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_live/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_live/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_live/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_live/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_live/b4\endcsname{-8}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_pt/b0\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_pt/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_pt/b2\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_pt/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/voxlock_pt/b4\endcsname{-8}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_null/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_null/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_null/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_null/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_self/b0\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_self/b1\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_self/b2\endcsname{-2}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_self/b3\endcsname{-3}
\expandafter\def\csname v@bge/ami_dev_long/w1_base_self/b4\endcsname{-3}
\expandafter\def\csname v@bge/krisp/C10_ftlong_kd_selfl/b0\endcsname{-22}
\expandafter\def\csname v@bge/krisp/C10_ftlong_kd_selfl/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/C10_ftlong_kd_selfl/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/C10_ftlong_kd_selfl/b3\endcsname{-27}
\expandafter\def\csname v@bge/krisp/C10_ftlong_kd_selfl/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/C22_ftlong_ini_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/C22_ftlong_ini_selfl/b1\endcsname{-23}
\expandafter\def\csname v@bge/krisp/C22_ftlong_ini_selfl/b2\endcsname{-25}
\expandafter\def\csname v@bge/krisp/C22_ftlong_ini_selfl/b3\endcsname{-27}
\expandafter\def\csname v@bge/krisp/C22_ftlong_ini_selfl/b4\endcsname{-28}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kd_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kd_selfl/b1\endcsname{-22}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kd_selfl/b2\endcsname{-31}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kd_selfl/b3\endcsname{-34}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kd_selfl/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kdo_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kdo_selfl/b1\endcsname{-24}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kdo_selfl/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kdo_selfl/b3\endcsname{-33}
\expandafter\def\csname v@bge/krisp/C22_ftlong_kdo_selfl/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/C22_ftlong_sc_selfl/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/C22_ftlong_sc_selfl/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/C22_ftlong_sc_selfl/b2\endcsname{-35}
\expandafter\def\csname v@bge/krisp/C22_ftlong_sc_selfl/b3\endcsname{-41}
\expandafter\def\csname v@bge/krisp/C22_ftlong_sc_selfl/b4\endcsname{-30}
\expandafter\def\csname v@bge/krisp/C51_ftlong_kd_selfl/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/C51_ftlong_kd_selfl/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/C51_ftlong_kd_selfl/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/C51_ftlong_kd_selfl/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/C51_ftlong_kd_selfl/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/LB_ftlong_null/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/LB_ftlong_null/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LB_ftlong_null/b2\endcsname{-24}
\expandafter\def\csname v@bge/krisp/LB_ftlong_null/b3\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LB_ftlong_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/LB_ftlong_self/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_ftlong_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LB_ftlong_self/b2\endcsname{-24}
\expandafter\def\csname v@bge/krisp/LB_ftlong_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/LB_ftlong_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_ftlong_selfl/b0\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LB_ftlong_selfl/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LB_ftlong_selfl/b2\endcsname{-33}
\expandafter\def\csname v@bge/krisp/LB_ftlong_selfl/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/LB_ftlong_selfl/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_null/b2\endcsname{-25}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_null/b3\endcsname{-18}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_null/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_self/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_self/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_self/b2\endcsname{-29}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_self/b3\endcsname{-28}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_selfl/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_selfl/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_selfl/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_selfl/b3\endcsname{-31}
\expandafter\def\csname v@bge/krisp/LB_ftlong_sslp_selfl/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_null/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_null/b2\endcsname{-41}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_null/b3\endcsname{-23}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_null/b4\endcsname{-8}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_self/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_self/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_self/b2\endcsname{-41}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_self/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_selfl/b0\endcsname{-28}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_selfl/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_selfl/b2\endcsname{-50}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_selfl/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_cwlt2_selfl/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_null/b0\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_null/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_null/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_null/b3\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_null/b4\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_self/b0\endcsname{-24}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_self/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_self/b2\endcsname{-32}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_self/b3\endcsname{-25}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_self/b4\endcsname{-20}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_selfl/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_selfl/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_selfl/b2\endcsname{-36}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_selfl/b3\endcsname{-28}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_selfl/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_null/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_null/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_null/b3\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_null/b4\endcsname{-15}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_self/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_self/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_self/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_self/b3\endcsname{-24}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_selfl/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_selfl/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_selfl/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_selfl/b3\endcsname{-26}
\expandafter\def\csname v@bge/krisp/LB_ftlong_ws_slow_selfl/b4\endcsname{-25}
\expandafter\def\csname v@bge/krisp/LB_long_k004_null/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LB_long_k004_null/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LB_long_k004_null/b2\endcsname{-29}
\expandafter\def\csname v@bge/krisp/LB_long_k004_null/b3\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_long_k004_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/LB_long_k004_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LB_long_k004_self/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LB_long_k004_self/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/LB_long_k004_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/LB_long_k004_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_null/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_null/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_null/b3\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_null/b4\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_self/b0\endcsname{-24}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_self/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_self/b2\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/LB_long_lvl_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LB_long_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LB_long_null/b1\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LB_long_null/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/LB_long_null/b3\endcsname{-23}
\expandafter\def\csname v@bge/krisp/LB_long_null/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/LB_long_self/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/LB_long_self/b1\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LB_long_self/b2\endcsname{-29}
\expandafter\def\csname v@bge/krisp/LB_long_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/LB_long_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LB_main_null/b0\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LB_main_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LB_main_null/b2\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LB_main_null/b3\endcsname{-5}
\expandafter\def\csname v@bge/krisp/LB_main_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/krisp/LB_main_self/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/LB_main_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/LB_main_self/b2\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LB_main_self/b3\endcsname{-8}
\expandafter\def\csname v@bge/krisp/LB_main_self/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/LC_seg24_null/b0\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LC_seg24_null/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LC_seg24_null/b2\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LC_seg24_null/b3\endcsname{-12}
\expandafter\def\csname v@bge/krisp/LC_seg24_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/LC_seg24_self/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/LC_seg24_self/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/LC_seg24_self/b2\endcsname{-23}
\expandafter\def\csname v@bge/krisp/LC_seg24_self/b3\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LC_seg24_self/b4\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_null/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_null/b2\endcsname{-23}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_null/b3\endcsname{-12}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_null/b4\endcsname{-15}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_self/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_self/b2\endcsname{-25}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_self/b3\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LC_turns_mem4_self/b4\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_null/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_null/b3\endcsname{-12}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_null/b4\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_self/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_self/b2\endcsname{-23}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_self/b3\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LC_turns_mem_self/b4\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LC_turns_null/b0\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LC_turns_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LC_turns_null/b2\endcsname{-23}
\expandafter\def\csname v@bge/krisp/LC_turns_null/b3\endcsname{-12}
\expandafter\def\csname v@bge/krisp/LC_turns_null/b4\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LC_turns_self/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LC_turns_self/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LC_turns_self/b2\endcsname{-22}
\expandafter\def\csname v@bge/krisp/LC_turns_self/b3\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LC_turns_self/b4\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_null/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_null/b2\endcsname{-20}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_null/b3\endcsname{-20}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_null/b4\endcsname{-14}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_self/b0\endcsname{-23}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_self/b1\endcsname{-27}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_self/b2\endcsname{-24}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_self/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_mem_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_null/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_null/b2\endcsname{-25}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_null/b3\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_null/b4\endcsname{-13}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_self/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_self/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_self/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_self/b3\endcsname{-31}
\expandafter\def\csname v@bge/krisp/LC_turns_w1k_self/b4\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_null/b0\endcsname{-10}
\expandafter\def\csname v@bge/krisp/MB_ftlong_null/b1\endcsname{-10}
\expandafter\def\csname v@bge/krisp/MB_ftlong_null/b2\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_null/b3\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_null/b4\endcsname{-13}
\expandafter\def\csname v@bge/krisp/MB_ftlong_self/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_self/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_self/b2\endcsname{-35}
\expandafter\def\csname v@bge/krisp/MB_ftlong_self/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_self/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_selfl/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_selfl/b1\endcsname{-31}
\expandafter\def\csname v@bge/krisp/MB_ftlong_selfl/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_selfl/b3\endcsname{-41}
\expandafter\def\csname v@bge/krisp/MB_ftlong_selfl/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_null/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_null/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_null/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_null/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_self/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_self/b2\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_self/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_selfl/b1\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_selfl/b2\endcsname{-36}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_selfl/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/MB_ftlong_sslp_selfl/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_null/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_null/b1\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_null/b2\endcsname{-37}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_null/b3\endcsname{-39}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_null/b4\endcsname{-8}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_self/b0\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_self/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_self/b2\endcsname{-36}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_self/b3\endcsname{-44}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_self/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_selfl/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_selfl/b1\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_selfl/b2\endcsname{-46}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_selfl/b3\endcsname{-45}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t2_selfl/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_null/b0\endcsname{-14}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_null/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_null/b3\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_self/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_self/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_selfl/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_selfl/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_selfl/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwl0t_selfl/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_null/b0\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_null/b1\endcsname{-8}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_null/b2\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_null/b3\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_null/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_self/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_self/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_self/b3\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_selfl/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_selfl/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_selfl/b3\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlf_selfl/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_null/b0\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_null/b1\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_null/b2\endcsname{-43}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_null/b3\endcsname{-32}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_self/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_self/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_self/b2\endcsname{-46}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_self/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_self/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_selfl/b0\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_selfl/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_selfl/b2\endcsname{-47}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_selfl/b3\endcsname{-46}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2_selfl/b4\endcsname{-25}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_null/b0\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_null/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_null/b2\endcsname{-40}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_null/b3\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_null/b4\endcsname{-8}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_selfl/b0\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_selfl/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_selfl/b2\endcsname{-46}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_selfl/b3\endcsname{-43}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g5_selfl/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_null/b0\endcsname{-25}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_null/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_null/b2\endcsname{-47}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_null/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_selfl/b0\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_selfl/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_selfl/b2\endcsname{-51}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_selfl/b3\endcsname{-45}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2g_selfl/b4\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_null/b0\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_null/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_null/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_null/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_selfl/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_selfl/b1\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_selfl/b2\endcsname{-36}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_selfl/b3\endcsname{-44}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2gm_selfl/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_null/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_null/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_null/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_null/b3\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_selfl/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_selfl/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_selfl/b2\endcsname{-39}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_selfl/b3\endcsname{-36}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2hm_selfl/b4\endcsname{-25}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_null/b0\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_null/b1\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_null/b2\endcsname{-46}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_null/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_null/b4\endcsname{-8}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_selfl/b0\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_selfl/b1\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_selfl/b2\endcsname{-47}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_selfl/b3\endcsname{-51}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2m_selfl/b4\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2mr_selfl/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2mr_selfl/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2mr_selfl/b2\endcsname{-52}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2mr_selfl/b3\endcsname{-52}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2mr_selfl/b4\endcsname{-25}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_null/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_null/b2\endcsname{-40}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_null/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_self/b0\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_self/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_self/b2\endcsname{-43}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_self/b3\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_self/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_selfl/b0\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_selfl/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_selfl/b2\endcsname{-45}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_selfl/b3\endcsname{-47}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2p_selfl/b4\endcsname{-25}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2r_selfl/b0\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2r_selfl/b1\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2r_selfl/b2\endcsname{-44}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2r_selfl/b3\endcsname{-45}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt2r_selfl/b4\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_null/b0\endcsname{-12}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_null/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_null/b2\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_null/b3\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_self/b0\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_self/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_self/b2\endcsname{-48}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_self/b3\endcsname{-38}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_self/b4\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_selfl/b0\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_selfl/b1\endcsname{-25}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_selfl/b2\endcsname{-50}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_selfl/b3\endcsname{-54}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_cwlt_selfl/b4\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_null/b0\endcsname{-10}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_null/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_null/b2\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_null/b3\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_self/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_self/b2\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_self/b3\endcsname{-33}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_self/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_selfl/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_selfl/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_selfl/b2\endcsname{-37}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_selfl/b3\endcsname{-36}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbl0t_selfl/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_null/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_null/b2\endcsname{-32}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_null/b3\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_null/b4\endcsname{-8}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_self/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_self/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_selfl/b1\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_selfl/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_selfl/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_hbx0t_selfl/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_null/b0\endcsname{-11}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_null/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_null/b2\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_null/b3\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_self/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_self/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_self/b3\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_self/b4\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_selfl/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_selfl/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_selfl/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_selfl/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_null/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_null/b2\endcsname{-31}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_null/b3\endcsname{-15}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_null/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_self/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_self/b2\endcsname{-33}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_selfl/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_selfl/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_selfl/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_sslb_selfl/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_null/b0\endcsname{-13}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_null/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_null/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_null/b3\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_self/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_self/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_self/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_selfl/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_selfl/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_selfl/b2\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_selfl/b3\endcsname{-31}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b0t_selfl/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_null/b0\endcsname{-31}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_null/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_null/b2\endcsname{-36}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_null/b3\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_self/b0\endcsname{-32}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_self/b1\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_self/b2\endcsname{-36}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_self/b3\endcsname{-32}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_selfl/b0\endcsname{-32}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_selfl/b1\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_selfl/b2\endcsname{-38}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_selfl/b3\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_w2b2_selfl/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_null/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_null/b2\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_null/b3\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_self/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_self/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_self/b3\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_self/b4\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_selfl/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_selfl/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_selfl/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs0t_selfl/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_null/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_null/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_null/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_null/b3\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_self/b0\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_self/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_self/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_self/b3\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_selfl/b0\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_selfl/b1\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_selfl/b2\endcsname{-37}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_selfl/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_whs2_selfl/b4\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_null/b0\endcsname{-8}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_null/b1\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_null/b2\endcsname{-8}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_null/b3\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_self/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_self/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_self/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_self/b3\endcsname{-32}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_self/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_selfl/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_selfl/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_selfl/b2\endcsname{-40}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_selfl/b3\endcsname{-34}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls0t_selfl/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_null/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_null/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_null/b2\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_null/b3\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_self/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_self/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_self/b2\endcsname{-38}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_self/b3\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_self/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_selfl/b0\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_selfl/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_selfl/b2\endcsname{-39}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_selfl/b3\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_ws_xls2_selfl/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_null/b0\endcsname{-13}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_null/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_null/b3\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_self/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_self/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_self/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_selfl/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_selfl/b2\endcsname{-31}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_selfl/b3\endcsname{-32}
\expandafter\def\csname v@bge/krisp/MB_ftlong_wsp_selfl/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_long_k004_null/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/MB_long_k004_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_long_k004_null/b2\endcsname{-32}
\expandafter\def\csname v@bge/krisp/MB_long_k004_null/b3\endcsname{-28}
\expandafter\def\csname v@bge/krisp/MB_long_k004_null/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/MB_long_k004_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_long_k004_self/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_long_k004_self/b2\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_long_k004_self/b3\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_long_k004_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_null/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_null/b2\endcsname{-42}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_null/b3\endcsname{-27}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_self/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_self/b2\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_self/b3\endcsname{-25}
\expandafter\def\csname v@bge/krisp/MB_long_lvl_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/MB_long_null/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/MB_long_null/b1\endcsname{-25}
\expandafter\def\csname v@bge/krisp/MB_long_null/b2\endcsname{-37}
\expandafter\def\csname v@bge/krisp/MB_long_null/b3\endcsname{-25}
\expandafter\def\csname v@bge/krisp/MB_long_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/MB_long_self/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_long_self/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/MB_long_self/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/MB_long_self/b3\endcsname{-26}
\expandafter\def\csname v@bge/krisp/MB_long_self/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/MB_main_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/MB_main_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/MB_main_null/b2\endcsname{-17}
\expandafter\def\csname v@bge/krisp/MB_main_null/b3\endcsname{-5}
\expandafter\def\csname v@bge/krisp/MB_main_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/krisp/MB_main_self/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/MB_main_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/MB_main_self/b2\endcsname{-15}
\expandafter\def\csname v@bge/krisp/MB_main_self/b3\endcsname{-10}
\expandafter\def\csname v@bge/krisp/MB_main_self/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_null/b0\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_null/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_null/b2\endcsname{-7}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_null/b3\endcsname{-4}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_self/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_self/b2\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_self/b3\endcsname{-7}
\expandafter\def\csname v@bge/krisp/SB_abs_k010_self/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_base_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_base_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_base_null/b2\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_base_null/b3\endcsname{-6}
\expandafter\def\csname v@bge/krisp/SB_base_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/krisp/SB_base_self/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_base_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_base_self/b2\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_base_self/b3\endcsname{-11}
\expandafter\def\csname v@bge/krisp/SB_base_self/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_base_selfl/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_base_selfl/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_base_selfl/b2\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_base_selfl/b3\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_base_selfl/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_ft_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_ft_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_ft_null/b2\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_ft_null/b3\endcsname{-6}
\expandafter\def\csname v@bge/krisp/SB_ft_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/krisp/SB_ft_selfl/b0\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ft_selfl/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_ft_selfl/b2\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ft_selfl/b3\endcsname{-8}
\expandafter\def\csname v@bge/krisp/SB_ft_selfl/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_null/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_null/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_null/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_null/b3\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_null/b4\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_self/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_self/b2\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_self/b3\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_self/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_selfl/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_selfl/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_selfl/b2\endcsname{-29}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_selfl/b3\endcsname{-28}
\expandafter\def\csname v@bge/krisp/SB_ftlong_em_selfl/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_null/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_null/b2\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_null/b3\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_selfl/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_selfl/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_selfl/b3\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_ftlong_k2000_selfl/b4\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_null/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_ftlong_null/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_null/b2\endcsname{-29}
\expandafter\def\csname v@bge/krisp/SB_ftlong_null/b3\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_ftlong_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_ftlong_self/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_self/b2\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_self/b3\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_selfl/b0\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_selfl/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_selfl/b2\endcsname{-33}
\expandafter\def\csname v@bge/krisp/SB_ftlong_selfl/b3\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_ftlong_selfl/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_null/b0\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_null/b2\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_null/b3\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_self/b2\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_self/b3\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_selfl/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_selfl/b2\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_selfl/b3\endcsname{-28}
\expandafter\def\csname v@bge/krisp/SB_ftlong_solo_selfl/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_null/b0\endcsname{-8}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_null/b1\endcsname{-9}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_null/b2\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_null/b3\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_null/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_self/b2\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_self/b3\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_selfl/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_selfl/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_selfl/b2\endcsname{-32}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_selfl/b3\endcsname{-28}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslb_selfl/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_null/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_null/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_null/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_null/b3\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_null/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_self/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_self/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_self/b2\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_self/b3\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_selfl/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_selfl/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_selfl/b3\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_ftlong_sslp_selfl/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_null/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_null/b2\endcsname{-38}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_null/b3\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_self/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_self/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_self/b2\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_self/b3\endcsname{-32}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_self/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_selfl/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_selfl/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_selfl/b2\endcsname{-40}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_selfl/b3\endcsname{-38}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wob_selfl/b4\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_null/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_null/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_null/b2\endcsname{-34}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_null/b3\endcsname{-39}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_self/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_self/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_self/b2\endcsname{-43}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_self/b3\endcsname{-33}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_self/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_selfl/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_selfl/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_selfl/b2\endcsname{-45}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_selfl/b3\endcsname{-37}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2_selfl/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_null/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_null/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_null/b2\endcsname{-40}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_null/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_selfl/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_selfl/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_selfl/b2\endcsname{-38}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_selfl/b3\endcsname{-35}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2c_selfl/b4\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_null/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_null/b2\endcsname{-41}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_null/b3\endcsname{-31}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_selfl/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_selfl/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_selfl/b2\endcsname{-40}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_selfl/b3\endcsname{-36}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2g_selfl/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_null/b0\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_null/b2\endcsname{-42}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_null/b3\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_selfl/b0\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_selfl/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_selfl/b2\endcsname{-48}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_selfl/b3\endcsname{-39}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gc_selfl/b4\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_null/b0\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_null/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_null/b2\endcsname{-36}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_null/b3\endcsname{-37}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_selfl/b0\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_selfl/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_selfl/b2\endcsname{-40}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_selfl/b3\endcsname{-38}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2gm_selfl/b4\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_null/b0\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_null/b2\endcsname{-37}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_null/b3\endcsname{-39}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_null/b4\endcsname{-8}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_selfl/b0\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_selfl/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_selfl/b2\endcsname{-40}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_selfl/b3\endcsname{-36}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2h_selfl/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_null/b0\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_null/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_null/b2\endcsname{-38}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_null/b3\endcsname{-43}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_selfl/b0\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_selfl/b1\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_selfl/b2\endcsname{-41}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_selfl/b3\endcsname{-46}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2m_selfl/b4\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2mr_selfl/b0\endcsname{-28}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2mr_selfl/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2mr_selfl/b2\endcsname{-48}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2mr_selfl/b3\endcsname{-39}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2mr_selfl/b4\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2r_selfl/b0\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2r_selfl/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2r_selfl/b2\endcsname{-43}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2r_selfl/b3\endcsname{-49}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_cwlt2r_selfl/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_null/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_null/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_null/b2\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_null/b3\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_self/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_self/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_self/b3\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_selfl/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_selfl/b2\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_selfl/b3\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_selfl/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_null/b0\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_null/b2\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_null/b3\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_self/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_self/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_self/b3\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_selfl/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_selfl/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_selfl/b3\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_ws_sslb_selfl/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_null/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_null/b2\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_null/b3\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_self/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_self/b2\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_self/b3\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_selfl/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_selfl/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_selfl/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_selfl/b3\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_ftlong_wsp_selfl/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_long_far_null/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_far_null/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_long_far_null/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/SB_long_far_null/b3\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_far_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/SB_long_far_self/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_far_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_long_far_self/b2\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_far_self/b3\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_long_far_self/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_long_k03_null/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_k03_null/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_long_k03_null/b2\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_long_k03_null/b3\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_k03_null/b4\endcsname{-8}
\expandafter\def\csname v@bge/krisp/SB_long_k03_self/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_long_k03_self/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_long_k03_self/b2\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_k03_self/b3\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_k03_self/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_long_keep_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_long_keep_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_long_keep_null/b2\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_long_keep_null/b3\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_keep_null/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/SB_long_keep_self/b0\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_long_keep_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_long_keep_self/b2\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_long_keep_self/b3\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_keep_self/b4\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_lk_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_long_lk_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_long_lk_null/b2\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_long_lk_null/b3\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_lk_null/b4\endcsname{-8}
\expandafter\def\csname v@bge/krisp/SB_long_lk_self/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_long_lk_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_long_lk_self/b2\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_long_lk_self/b3\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_lk_self/b4\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_loud/b0\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_loud/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_loud/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_loud/b3\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_loud/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_null/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_null/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_null/b2\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_null/b3\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_self/b2\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_self/b3\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_selfl/b0\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_selfl/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_selfl/b2\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_selfl/b3\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_long_lvl_selfl/b4\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_long_null/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_null/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_null/b2\endcsname{-32}
\expandafter\def\csname v@bge/krisp/SB_long_null/b3\endcsname{-22}
\expandafter\def\csname v@bge/krisp/SB_long_null/b4\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_long_self/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_long_self/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_long_self/b2\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_self/b3\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_long_self/b4\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_long_sir_null/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_sir_null/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_sir_null/b2\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_long_sir_null/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/SB_long_sir_null/b4\endcsname{-13}
\expandafter\def\csname v@bge/krisp/SB_long_sir_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_sir_self/b1\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_long_sir_self/b2\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_sir_self/b3\endcsname{-24}
\expandafter\def\csname v@bge/krisp/SB_long_sir_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_long_spk_null/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_spk_null/b1\endcsname{-15}
\expandafter\def\csname v@bge/krisp/SB_long_spk_null/b2\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_long_spk_null/b3\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_long_spk_null/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/SB_long_spk_self/b0\endcsname{-36}
\expandafter\def\csname v@bge/krisp/SB_long_spk_self/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_spk_self/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/SB_long_spk_self/b3\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_long_spk_self/b4\endcsname{-14}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_null/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_null/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_null/b2\endcsname{-29}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_null/b3\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_null/b4\endcsname{-10}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_self/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_self/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_self/b2\endcsname{-28}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_self/b3\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_self/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_selfl/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_selfl/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_selfl/b2\endcsname{-30}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_selfl/b3\endcsname{-21}
\expandafter\def\csname v@bge/krisp/SB_long_ssl_selfl/b4\endcsname{-23}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_loud/b0\endcsname{-29}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_loud/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_loud/b2\endcsname{-35}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_loud/b3\endcsname{-27}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_loud/b4\endcsname{-26}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_null/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_null/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_null/b2\endcsname{-25}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_null/b3\endcsname{-20}
\expandafter\def\csname v@bge/krisp/SB_long_sslb_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/S_abs_k010_null/b0\endcsname{-10}
\expandafter\def\csname v@bge/krisp/S_abs_k010_null/b1\endcsname{-9}
\expandafter\def\csname v@bge/krisp/S_abs_k010_null/b2\endcsname{-6}
\expandafter\def\csname v@bge/krisp/S_abs_k010_null/b3\endcsname{-5}
\expandafter\def\csname v@bge/krisp/S_abs_k010_null/b4\endcsname{-3}
\expandafter\def\csname v@bge/krisp/S_abs_k010_self/b0\endcsname{-14}
\expandafter\def\csname v@bge/krisp/S_abs_k010_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/S_abs_k010_self/b2\endcsname{-12}
\expandafter\def\csname v@bge/krisp/S_abs_k010_self/b3\endcsname{-6}
\expandafter\def\csname v@bge/krisp/S_abs_k010_self/b4\endcsname{-8}
\expandafter\def\csname v@bge/krisp/dfn3/b0\endcsname{-4}
\expandafter\def\csname v@bge/krisp/dfn3/b1\endcsname{-4}
\expandafter\def\csname v@bge/krisp/dfn3/b2\endcsname{-3}
\expandafter\def\csname v@bge/krisp/dfn3/b3\endcsname{-4}
\expandafter\def\csname v@bge/krisp/dfn3/b4\endcsname{-4}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_null/b0\endcsname{-14}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_null/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_null/b2\endcsname{-10}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_null/b3\endcsname{-6}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_self/b0\endcsname{-14}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_self/b1\endcsname{-11}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_self/b2\endcsname{-14}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_self/b3\endcsname{-7}
\expandafter\def\csname v@bge/krisp/ftlb_off_k004_self/b4\endcsname{-9}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_null/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_null/b2\endcsname{-20}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_null/b3\endcsname{-7}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_null/b4\endcsname{-11}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_self/b0\endcsname{-17}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_self/b2\endcsname{-22}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_self/b3\endcsname{-8}
\expandafter\def\csname v@bge/krisp/ftlb_on_k004_self/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/krisp_default/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/krisp_default/b1\endcsname{-17}
\expandafter\def\csname v@bge/krisp/krisp_default/b2\endcsname{-15}
\expandafter\def\csname v@bge/krisp/krisp_default/b3\endcsname{-23}
\expandafter\def\csname v@bge/krisp/krisp_default/b4\endcsname{-21}
\expandafter\def\csname v@bge/krisp/krisp_hd/b0\endcsname{-10}
\expandafter\def\csname v@bge/krisp/krisp_hd/b1\endcsname{-9}
\expandafter\def\csname v@bge/krisp/krisp_hd/b2\endcsname{-8}
\expandafter\def\csname v@bge/krisp/krisp_hd/b3\endcsname{-16}
\expandafter\def\csname v@bge/krisp/krisp_hd/b4\endcsname{-19}
\expandafter\def\csname v@bge/krisp/sidon_v2/b0\endcsname{7}
\expandafter\def\csname v@bge/krisp/sidon_v2/b1\endcsname{12}
\expandafter\def\csname v@bge/krisp/sidon_v2/b2\endcsname{12}
\expandafter\def\csname v@bge/krisp/sidon_v2/b3\endcsname{12}
\expandafter\def\csname v@bge/krisp/sidon_v2/b4\endcsname{11}
\expandafter\def\csname v@bge/krisp/tfM_abs_null/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/tfM_abs_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/tfM_abs_null/b2\endcsname{-18}
\expandafter\def\csname v@bge/krisp/tfM_abs_null/b3\endcsname{-6}
\expandafter\def\csname v@bge/krisp/tfM_abs_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/krisp/tfM_abs_self/b0\endcsname{-15}
\expandafter\def\csname v@bge/krisp/tfM_abs_self/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/tfM_abs_self/b2\endcsname{-16}
\expandafter\def\csname v@bge/krisp/tfM_abs_self/b3\endcsname{-10}
\expandafter\def\csname v@bge/krisp/tfM_abs_self/b4\endcsname{-12}
\expandafter\def\csname v@bge/krisp/tfM_base_null/b0\endcsname{-18}
\expandafter\def\csname v@bge/krisp/tfM_base_null/b1\endcsname{-13}
\expandafter\def\csname v@bge/krisp/tfM_base_null/b2\endcsname{-17}
\expandafter\def\csname v@bge/krisp/tfM_base_null/b3\endcsname{-5}
\expandafter\def\csname v@bge/krisp/tfM_base_null/b4\endcsname{-4}
\expandafter\def\csname v@bge/krisp/tfM_base_self/b0\endcsname{-14}
\expandafter\def\csname v@bge/krisp/tfM_base_self/b1\endcsname{-12}
\expandafter\def\csname v@bge/krisp/tfM_base_self/b2\endcsname{-16}
\expandafter\def\csname v@bge/krisp/tfM_base_self/b3\endcsname{-12}
\expandafter\def\csname v@bge/krisp/tfM_base_self/b4\endcsname{-14}
\expandafter\def\csname v@bge/krisp/voxlock/b0\endcsname{-23}
\expandafter\def\csname v@bge/krisp/voxlock/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/voxlock/b2\endcsname{-31}
\expandafter\def\csname v@bge/krisp/voxlock/b3\endcsname{-31}
\expandafter\def\csname v@bge/krisp/voxlock/b4\endcsname{-29}
\expandafter\def\csname v@bge/krisp/voxlock_live/b0\endcsname{-21}
\expandafter\def\csname v@bge/krisp/voxlock_live/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/voxlock_live/b2\endcsname{-27}
\expandafter\def\csname v@bge/krisp/voxlock_live/b3\endcsname{-29}
\expandafter\def\csname v@bge/krisp/voxlock_live/b4\endcsname{-30}
\expandafter\def\csname v@bge/krisp/voxlock_pt/b0\endcsname{-23}
\expandafter\def\csname v@bge/krisp/voxlock_pt/b1\endcsname{-19}
\expandafter\def\csname v@bge/krisp/voxlock_pt/b2\endcsname{-31}
\expandafter\def\csname v@bge/krisp/voxlock_pt/b3\endcsname{-31}
\expandafter\def\csname v@bge/krisp/voxlock_pt/b4\endcsname{-29}
\expandafter\def\csname v@bge/krisp/w1_base_loud/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/w1_base_loud/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/w1_base_loud/b2\endcsname{-21}
\expandafter\def\csname v@bge/krisp/w1_base_loud/b3\endcsname{-23}
\expandafter\def\csname v@bge/krisp/w1_base_loud/b4\endcsname{-27}
\expandafter\def\csname v@bge/krisp/w1_base_null/b0\endcsname{-20}
\expandafter\def\csname v@bge/krisp/w1_base_null/b1\endcsname{-18}
\expandafter\def\csname v@bge/krisp/w1_base_null/b2\endcsname{-31}
\expandafter\def\csname v@bge/krisp/w1_base_null/b3\endcsname{-24}
\expandafter\def\csname v@bge/krisp/w1_base_null/b4\endcsname{-28}
\expandafter\def\csname v@bge/krisp/w1_base_self/b0\endcsname{-19}
\expandafter\def\csname v@bge/krisp/w1_base_self/b1\endcsname{-16}
\expandafter\def\csname v@bge/krisp/w1_base_self/b2\endcsname{-18}
\expandafter\def\csname v@bge/krisp/w1_base_self/b3\endcsname{-23}
\expandafter\def\csname v@bge/krisp/w1_base_self/b4\endcsname{-26}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/ami_dev/diff\endcsname{+0.19}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/ami_dev/hi\endcsname{+0.76}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/ami_dev/lo\endcsname{-0.35}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/ami_dev_long/diff\endcsname{+1.23}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/ami_dev_long/hi\endcsname{+2.52}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/ami_dev_long/lo\endcsname{-0.05}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/call_dev_clean/diff\endcsname{-0.10}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/call_dev_clean/hi\endcsname{+0.52}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/call_dev_clean/lo\endcsname{-0.74}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/dev4/diff\endcsname{+0.33}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/dev4/hi\endcsname{+0.72}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/dev4/lo\endcsname{-0.06}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/nsf_dev/diff\endcsname{-0.01}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/nsf_dev/hi\endcsname{+0.12}
\expandafter\def\csname v@boot/C10n_ftlong_kd_selfl/C22_ftlong_kd_selfl/nsf_dev/lo\endcsname{-0.14}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/ami_dev/diff\endcsname{+0.31}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/ami_dev/hi\endcsname{+0.89}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/ami_dev/lo\endcsname{-0.26}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/ami_dev_long/diff\endcsname{+0.88}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/ami_dev_long/hi\endcsname{+1.93}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/ami_dev_long/lo\endcsname{-0.05}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/call_dev_clean/diff\endcsname{-0.26}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/call_dev_clean/hi\endcsname{+0.21}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/call_dev_clean/lo\endcsname{-0.71}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/dev4/diff\endcsname{+0.24}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/dev4/hi\endcsname{+0.55}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/dev4/lo\endcsname{-0.07}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/nsf_dev/diff\endcsname{+0.02}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/nsf_dev/hi\endcsname{+0.16}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2g5_selfl/pre_selfl/nsf_dev/lo\endcsname{-0.11}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/diff\endcsname{-0.07}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/hi\endcsname{+0.75}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/lo\endcsname{-0.83}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/diff\endcsname{-1.09}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/hi\endcsname{+1.17}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/lo\endcsname{-3.48}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/diff\endcsname{+1.52}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/hi\endcsname{+2.39}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/lo\endcsname{+0.74}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/dev4/diff\endcsname{+0.08}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/dev4/hi\endcsname{+0.74}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/dev4/lo\endcsname{-0.58}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/diff\endcsname{-0.05}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/hi\endcsname{+0.10}
\expandafter\def\csname v@boot/MB_ftlong_ws_cwlt2r_selfl/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/lo\endcsname{-0.19}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/diff\endcsname{-0.17}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/hi\endcsname{+0.33}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/lo\endcsname{-0.64}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/diff\endcsname{-0.83}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/hi\endcsname{+1.59}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/lo\endcsname{-3.17}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/diff\endcsname{+1.63}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/hi\endcsname{+2.35}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/lo\endcsname{+0.92}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/dev4/diff\endcsname{+0.15}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/dev4/hi\endcsname{+0.78}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/dev4/lo\endcsname{-0.48}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/diff\endcsname{-0.05}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/hi\endcsname{+0.05}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/lo\endcsname{-0.15}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/ami_dev/diff\endcsname{+0.28}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/ami_dev/hi\endcsname{+0.90}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/ami_dev/lo\endcsname{-0.26}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/ami_dev_long/diff\endcsname{-1.40}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/ami_dev_long/hi\endcsname{-0.23}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/ami_dev_long/lo\endcsname{-3.05}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/call_dev_clean/diff\endcsname{+1.42}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/call_dev_clean/hi\endcsname{+2.55}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/call_dev_clean/lo\endcsname{+0.48}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/dev4/diff\endcsname{+0.08}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/dev4/hi\endcsname{+0.52}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/dev4/lo\endcsname{-0.42}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/nsf_dev/diff\endcsname{+0.01}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/nsf_dev/hi\endcsname{+0.14}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2h_selfl/nsf_dev/lo\endcsname{-0.11}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/ami_dev/diff\endcsname{-0.10}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/ami_dev/hi\endcsname{+0.70}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/ami_dev/lo\endcsname{-0.85}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/ami_dev_long/diff\endcsname{-1.32}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/ami_dev_long/hi\endcsname{-0.41}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/ami_dev_long/lo\endcsname{-2.42}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/call_dev_clean/diff\endcsname{+2.04}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/call_dev_clean/hi\endcsname{+3.00}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/call_dev_clean/lo\endcsname{+1.15}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/dev4/diff\endcsname{+0.14}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/dev4/hi\endcsname{+0.54}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/dev4/lo\endcsname{-0.27}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/nsf_dev/diff\endcsname{-0.06}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/nsf_dev/hi\endcsname{+0.10}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2m_selfl/nsf_dev/lo\endcsname{-0.22}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/ami_dev/diff\endcsname{+0.19}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/ami_dev/hi\endcsname{+0.78}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/ami_dev/lo\endcsname{-0.39}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/ami_dev_long/diff\endcsname{-1.51}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/ami_dev_long/hi\endcsname{-0.07}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/ami_dev_long/lo\endcsname{-3.14}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/call_dev_clean/diff\endcsname{+0.75}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/call_dev_clean/hi\endcsname{+1.51}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/call_dev_clean/lo\endcsname{+0.01}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/dev4/diff\endcsname{-0.15}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/dev4/hi\endcsname{+0.29}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/dev4/lo\endcsname{-0.63}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/nsf_dev/diff\endcsname{-0.02}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/nsf_dev/hi\endcsname{+0.10}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2_selfl/SB_ftlong_ws_cwlt2r_selfl/nsf_dev/lo\endcsname{-0.15}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/ami_dev/diff\endcsname{+0.03}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/ami_dev/hi\endcsname{+0.43}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/ami_dev/lo\endcsname{-0.33}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/ami_dev_long/diff\endcsname{+1.15}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/ami_dev_long/hi\endcsname{+2.47}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/ami_dev_long/lo\endcsname{+0.05}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/call_dev_clean/diff\endcsname{-1.08}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/call_dev_clean/hi\endcsname{-0.02}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/call_dev_clean/lo\endcsname{-2.40}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/dev4/diff\endcsname{+0.02}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/dev4/hi\endcsname{+0.45}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/dev4/lo\endcsname{-0.42}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/nsf_dev/diff\endcsname{-0.03}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/nsf_dev/hi\endcsname{+0.07}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2gc_selfl/SB_ftlong_ws_cwlt2_selfl/nsf_dev/lo\endcsname{-0.14}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/diff\endcsname{-0.07}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/hi\endcsname{+0.51}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/lo\endcsname{-0.78}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/diff\endcsname{+0.50}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/hi\endcsname{+2.91}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/lo\endcsname{-1.41}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/diff\endcsname{-0.42}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/hi\endcsname{+0.27}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/lo\endcsname{-1.20}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/dev4/diff\endcsname{+0.01}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/dev4/hi\endcsname{+0.65}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/dev4/lo\endcsname{-0.54}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/diff\endcsname{+0.01}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/hi\endcsname{+0.14}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/lo\endcsname{-0.13}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/diff\endcsname{-0.14}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/hi\endcsname{+0.42}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/lo\endcsname{-0.88}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/diff\endcsname{-0.32}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/hi\endcsname{+1.34}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/lo\endcsname{-1.63}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/diff\endcsname{-0.42}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/hi\endcsname{+0.33}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/lo\endcsname{-1.22}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/dev4/diff\endcsname{-0.20}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/dev4/hi\endcsname{+0.30}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/dev4/lo\endcsname{-0.63}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/diff\endcsname{+0.07}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/hi\endcsname{+0.23}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2m_selfl/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/lo\endcsname{-0.10}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/diff\endcsname{-0.43}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/hi\endcsname{+0.16}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/lo\endcsname{-1.06}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/diff\endcsname{-0.13}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/hi\endcsname{+2.25}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/lo\endcsname{-2.45}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/diff\endcsname{+0.87}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/hi\endcsname{+1.85}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/lo\endcsname{-0.02}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/dev4/diff\endcsname{+0.09}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/dev4/hi\endcsname{+0.74}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/dev4/lo\endcsname{-0.54}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/diff\endcsname{+0.03}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/hi\endcsname{+0.19}
\expandafter\def\csname v@boot/SB_ftlong_ws_cwlt2r_selfl/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/lo\endcsname{-0.13}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/ami_dev/diff\endcsname{-0.01}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/ami_dev/hi\endcsname{+0.67}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/ami_dev/lo\endcsname{-0.79}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/ami_dev_long/diff\endcsname{+0.03}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/ami_dev_long/hi\endcsname{+2.29}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/ami_dev_long/lo\endcsname{-2.06}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/call_dev_clean/diff\endcsname{-0.27}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/call_dev_clean/hi\endcsname{+0.58}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/call_dev_clean/lo\endcsname{-1.11}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/dev4/diff\endcsname{-0.07}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/dev4/hi\endcsname{+0.56}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/dev4/lo\endcsname{-0.68}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/nsf_dev/diff\endcsname{+0.00}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/nsf_dev/hi\endcsname{+0.11}
\expandafter\def\csname v@boot/pre_selfl/MB_ftlong_ws_cwlt2r_selfl/nsf_dev/lo\endcsname{-0.11}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/ami_dev/diff\endcsname{-0.24}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/ami_dev/hi\endcsname{+0.28}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/ami_dev/lo\endcsname{-0.74}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/ami_dev_long/diff\endcsname{-0.41}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/ami_dev_long/hi\endcsname{+0.81}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/ami_dev_long/lo\endcsname{-1.70}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/call_dev_clean/diff\endcsname{+0.96}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/call_dev_clean/hi\endcsname{+1.91}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/call_dev_clean/lo\endcsname{+0.14}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/dev4/diff\endcsname{+0.06}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/dev4/hi\endcsname{+0.45}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/dev4/lo\endcsname{-0.36}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/nsf_dev/diff\endcsname{-0.08}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/nsf_dev/hi\endcsname{+0.06}
\expandafter\def\csname v@boot/pre_selfl/rel_selfl/nsf_dev/lo\endcsname{-0.23}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/ami_dev/diff\endcsname{-0.06}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/ami_dev/hi\endcsname{+0.17}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/ami_dev/lo\endcsname{-0.30}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/ami_dev_long/diff\endcsname{-0.29}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/ami_dev_long/hi\endcsname{+0.05}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/ami_dev_long/lo\endcsname{-0.77}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/call_dev_clean/diff\endcsname{-0.07}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/call_dev_clean/hi\endcsname{+0.15}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/call_dev_clean/lo\endcsname{-0.29}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/dev4/diff\endcsname{-0.12}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/dev4/hi\endcsname{+0.01}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/dev4/lo\endcsname{-0.26}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/nsf_dev/diff\endcsname{-0.05}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/nsf_dev/hi\endcsname{+0.06}
\expandafter\def\csname v@boot/pre_selfl1/pre_selfl/nsf_dev/lo\endcsname{-0.15}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/ami_dev/diff\endcsname{+0.49}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/ami_dev/hi\endcsname{+1.18}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/ami_dev/lo\endcsname{-0.18}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/ami_dev_long/diff\endcsname{+1.07}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/ami_dev_long/hi\endcsname{+3.20}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/ami_dev_long/lo\endcsname{-0.93}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/call_dev_clean/diff\endcsname{-1.18}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/call_dev_clean/hi\endcsname{-0.46}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/call_dev_clean/lo\endcsname{-2.11}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/dev4/diff\endcsname{+0.10}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/dev4/hi\endcsname{+0.71}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/dev4/lo\endcsname{-0.47}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/nsf_dev/diff\endcsname{+0.05}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/nsf_dev/hi\endcsname{+0.25}
\expandafter\def\csname v@boot/pre_selfl_pr1/pre_selfl/nsf_dev/lo\endcsname{-0.17}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/ami_dev/diff\endcsname{+0.47}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/ami_dev/hi\endcsname{+1.13}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/ami_dev/lo\endcsname{-0.17}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/ami_dev_long/diff\endcsname{+1.60}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/ami_dev_long/hi\endcsname{+3.89}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/ami_dev_long/lo\endcsname{-0.62}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/call_dev_clean/diff\endcsname{-1.23}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/call_dev_clean/hi\endcsname{-0.18}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/call_dev_clean/lo\endcsname{-2.32}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/dev4/diff\endcsname{+0.22}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/dev4/hi\endcsname{+0.90}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/dev4/lo\endcsname{-0.41}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/nsf_dev/diff\endcsname{+0.05}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/nsf_dev/hi\endcsname{+0.25}
\expandafter\def\csname v@boot/pre_selfls_pr1/pre_selfl/nsf_dev/lo\endcsname{-0.17}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/ami_dev/diff\endcsname{-0.25}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/ami_dev/hi\endcsname{+0.26}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/ami_dev/lo\endcsname{-0.77}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/diff\endcsname{-1.60}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/hi\endcsname{-0.18}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/lo\endcsname{-3.21}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/diff\endcsname{+0.65}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/hi\endcsname{+1.41}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/lo\endcsname{-0.07}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/dev4/diff\endcsname{-0.30}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/dev4/hi\endcsname{+0.14}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/dev4/lo\endcsname{-0.75}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/nsf_dev/diff\endcsname{+0.02}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/nsf_dev/hi\endcsname{+0.16}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2gm_selfl/nsf_dev/lo\endcsname{-0.12}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/ami_dev/diff\endcsname{+0.24}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/ami_dev/hi\endcsname{+0.95}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/ami_dev/lo\endcsname{-0.28}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/ami_dev_long/diff\endcsname{-1.87}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/ami_dev_long/hi\endcsname{-0.28}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/ami_dev_long/lo\endcsname{-3.76}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/call_dev_clean/diff\endcsname{+0.50}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/call_dev_clean/hi\endcsname{+0.94}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/call_dev_clean/lo\endcsname{+0.13}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/dev4/diff\endcsname{-0.30}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/dev4/hi\endcsname{+0.15}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/dev4/lo\endcsname{-0.80}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/nsf_dev/diff\endcsname{-0.08}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/nsf_dev/hi\endcsname{+0.08}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2hm_selfl/nsf_dev/lo\endcsname{-0.30}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/diff\endcsname{+0.15}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/hi\endcsname{+0.76}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/lo\endcsname{-0.44}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/diff\endcsname{-0.66}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/hi\endcsname{+0.53}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/lo\endcsname{-1.78}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/diff\endcsname{+0.29}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/hi\endcsname{+0.88}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/lo\endcsname{-0.33}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/dev4/diff\endcsname{-0.05}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/dev4/hi\endcsname{+0.32}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/dev4/lo\endcsname{-0.40}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/diff\endcsname{+0.03}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/hi\endcsname{+0.16}
\expandafter\def\csname v@boot/rel_selfl/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/lo\endcsname{-0.08}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/ami_dev/diff\endcsname{-0.17}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/ami_dev/hi\endcsname{+0.03}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/ami_dev/lo\endcsname{-0.42}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/ami_dev_long/diff\endcsname{+0.10}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/ami_dev_long/hi\endcsname{+0.53}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/ami_dev_long/lo\endcsname{-0.37}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/call_dev_clean/diff\endcsname{+0.14}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/call_dev_clean/hi\endcsname{+0.37}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/call_dev_clean/lo\endcsname{-0.03}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/dev4/diff\endcsname{+0.03}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/dev4/hi\endcsname{+0.15}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/dev4/lo\endcsname{-0.12}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/nsf_dev/diff\endcsname{+0.02}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/nsf_dev/hi\endcsname{+0.14}
\expandafter\def\csname v@boot/rel_selfl1/rel_selfl/nsf_dev/lo\endcsname{-0.09}
\expandafter\def\csname v@call_dev_clean/C22_ftlong_kd_selfl/dele\endcsname{1.80}
\expandafter\def\csname v@call_dev_clean/C22_ftlong_kd_selfl/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/C22_ftlong_kd_selfl/dwer\endcsname{+0.96}
\expandafter\def\csname v@call_dev_clean/C22_ftlong_kd_selfl/dwer-hi\endcsname{+2.15}
\expandafter\def\csname v@call_dev_clean/C22_ftlong_kd_selfl/dwer-lo\endcsname{-0.22}
\expandafter\def\csname v@call_dev_clean/C22_ftlong_kd_selfl/ins\endcsname{0.26}
\expandafter\def\csname v@call_dev_clean/C22_ftlong_kd_selfl/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/C22_ftlong_kd_selfl/miss\endcsname{2.58}
\expandafter\def\csname v@call_dev_clean/C22_ftlong_kd_selfl/wer\endcsname{2.84}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_null/dele\endcsname{1.76}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{+0.73}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+1.74}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-0.39}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_null/ins\endcsname{0.23}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_null/miss\endcsname{2.39}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_null/wer\endcsname{2.62}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{1.96}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{+1.08}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+2.22}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-0.12}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{0.25}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{2.71}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{2.96}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_null/dele\endcsname{2.90}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_null/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_null/dwer\endcsname{+2.02}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_null/dwer-hi\endcsname{+3.24}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_null/dwer-lo\endcsname{+0.81}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_null/ins\endcsname{0.22}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_null/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_null/miss\endcsname{3.69}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_null/wer\endcsname{3.91}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_selfl/dele\endcsname{4.30}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_selfl/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_selfl/dwer\endcsname{+3.68}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_selfl/dwer-hi\endcsname{+5.49}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_selfl/dwer-lo\endcsname{+1.97}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_selfl/ins\endcsname{0.26}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_selfl/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_selfl/miss\endcsname{5.31}
\expandafter\def\csname v@call_dev_clean/MB_ftlong_ws_selfl/wer\endcsname{5.57}
\expandafter\def\csname v@call_dev_clean/SB_ftlong_ws_selfl/dele\endcsname{4.56}
\expandafter\def\csname v@call_dev_clean/SB_ftlong_ws_selfl/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/SB_ftlong_ws_selfl/dwer\endcsname{+3.90}
\expandafter\def\csname v@call_dev_clean/SB_ftlong_ws_selfl/dwer-hi\endcsname{+5.51}
\expandafter\def\csname v@call_dev_clean/SB_ftlong_ws_selfl/dwer-lo\endcsname{+2.35}
\expandafter\def\csname v@call_dev_clean/SB_ftlong_ws_selfl/ins\endcsname{0.20}
\expandafter\def\csname v@call_dev_clean/SB_ftlong_ws_selfl/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/SB_ftlong_ws_selfl/miss\endcsname{5.58}
\expandafter\def\csname v@call_dev_clean/SB_ftlong_ws_selfl/wer\endcsname{5.78}
\expandafter\def\csname v@call_dev_clean/dfn3/dele\endcsname{1.79}
\expandafter\def\csname v@call_dev_clean/dfn3/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/dfn3/dwer\endcsname{+0.68}
\expandafter\def\csname v@call_dev_clean/dfn3/dwer-hi\endcsname{+1.55}
\expandafter\def\csname v@call_dev_clean/dfn3/dwer-lo\endcsname{-0.22}
\expandafter\def\csname v@call_dev_clean/dfn3/ins\endcsname{0.20}
\expandafter\def\csname v@call_dev_clean/dfn3/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/dfn3/miss\endcsname{2.37}
\expandafter\def\csname v@call_dev_clean/dfn3/wer\endcsname{2.57}
\expandafter\def\csname v@call_dev_clean/raw/dele\endcsname{0.00}
\expandafter\def\csname v@call_dev_clean/raw/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/raw/dwer\endcsname{-1.89}
\expandafter\def\csname v@call_dev_clean/raw/dwer-hi\endcsname{-1.03}
\expandafter\def\csname v@call_dev_clean/raw/dwer-lo\endcsname{-3.06}
\expandafter\def\csname v@call_dev_clean/raw/ins\endcsname{0.00}
\expandafter\def\csname v@call_dev_clean/raw/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/raw/miss\endcsname{0.00}
\expandafter\def\csname v@call_dev_clean/raw/wer\endcsname{0.00}
\expandafter\def\csname v@call_dev_clean/voxlock/dele\endcsname{1.59}
\expandafter\def\csname v@call_dev_clean/voxlock/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/voxlock/dwer\endcsname{+0.50}
\expandafter\def\csname v@call_dev_clean/voxlock/dwer-hi\endcsname{+1.09}
\expandafter\def\csname v@call_dev_clean/voxlock/dwer-lo\endcsname{-0.07}
\expandafter\def\csname v@call_dev_clean/voxlock/ins\endcsname{0.24}
\expandafter\def\csname v@call_dev_clean/voxlock/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/voxlock/miss\endcsname{2.15}
\expandafter\def\csname v@call_dev_clean/voxlock/wer\endcsname{2.39}
\expandafter\def\csname v@call_dev_clean/voxlock_live/dele\endcsname{1.53}
\expandafter\def\csname v@call_dev_clean/voxlock_live/dleak\endcsname{+nan}
\expandafter\def\csname v@call_dev_clean/voxlock_live/dwer\endcsname{+0.20}
\expandafter\def\csname v@call_dev_clean/voxlock_live/dwer-hi\endcsname{+0.82}
\expandafter\def\csname v@call_dev_clean/voxlock_live/dwer-lo\endcsname{-0.38}
\expandafter\def\csname v@call_dev_clean/voxlock_live/ins\endcsname{0.08}
\expandafter\def\csname v@call_dev_clean/voxlock_live/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/voxlock_live/miss\endcsname{2.01}
\expandafter\def\csname v@call_dev_clean/voxlock_live/wer\endcsname{2.09}
\expandafter\def\csname v@call_dev_clean/voxlock_pt/dele\endcsname{1.49}
\expandafter\def\csname v@call_dev_clean/voxlock_pt/ins\endcsname{0.04}
\expandafter\def\csname v@call_dev_clean/voxlock_pt/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_dev_clean/voxlock_pt/miss\endcsname{1.85}
\expandafter\def\csname v@call_dev_clean/voxlock_pt/wer\endcsname{1.89}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_null/dele\endcsname{2.81}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{-44.78}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-11.39}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{-6.47}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-16.89}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_null/ins\endcsname{33.17}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{91.41}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_null/miss\endcsname{15.58}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_null/wer\endcsname{48.75}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{3.54}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-26.09}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-8.82}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{-3.97}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-13.60}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{34.88}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{110.10}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{16.44}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{51.32}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_null/dele\endcsname{4.05}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_null/dleak\endcsname{-42.11}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_null/dwer\endcsname{-7.06}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_null/dwer-hi\endcsname{-1.26}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_null/dwer-lo\endcsname{-12.86}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_null/ins\endcsname{38.64}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_null/leak_wpm\endcsname{94.08}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_null/miss\endcsname{14.43}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_null/wer\endcsname{53.08}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_selfl/dele\endcsname{5.47}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_selfl/dleak\endcsname{-30.20}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_selfl/dwer\endcsname{-7.95}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_selfl/dwer-hi\endcsname{-2.66}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_selfl/dwer-lo\endcsname{-13.29}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_selfl/ins\endcsname{35.00}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_selfl/leak_wpm\endcsname{105.99}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_selfl/miss\endcsname{17.19}
\expandafter\def\csname v@call_dev_mix/MB_ftlong_ws_selfl/wer\endcsname{52.19}
\expandafter\def\csname v@call_dev_mix/SB_ftlong_ws_selfl/dele\endcsname{4.71}
\expandafter\def\csname v@call_dev_mix/SB_ftlong_ws_selfl/dleak\endcsname{-21.98}
\expandafter\def\csname v@call_dev_mix/SB_ftlong_ws_selfl/dwer\endcsname{-8.72}
\expandafter\def\csname v@call_dev_mix/SB_ftlong_ws_selfl/dwer-hi\endcsname{-3.77}
\expandafter\def\csname v@call_dev_mix/SB_ftlong_ws_selfl/dwer-lo\endcsname{-13.75}
\expandafter\def\csname v@call_dev_mix/SB_ftlong_ws_selfl/ins\endcsname{34.64}
\expandafter\def\csname v@call_dev_mix/SB_ftlong_ws_selfl/leak_wpm\endcsname{114.21}
\expandafter\def\csname v@call_dev_mix/SB_ftlong_ws_selfl/miss\endcsname{16.78}
\expandafter\def\csname v@call_dev_mix/SB_ftlong_ws_selfl/wer\endcsname{51.42}
\expandafter\def\csname v@call_dev_mix/dfn3/dele\endcsname{2.82}
\expandafter\def\csname v@call_dev_mix/dfn3/dleak\endcsname{+11.30}
\expandafter\def\csname v@call_dev_mix/dfn3/dwer\endcsname{+13.30}
\expandafter\def\csname v@call_dev_mix/dfn3/dwer-hi\endcsname{+18.96}
\expandafter\def\csname v@call_dev_mix/dfn3/dwer-lo\endcsname{+7.94}
\expandafter\def\csname v@call_dev_mix/dfn3/ins\endcsname{59.95}
\expandafter\def\csname v@call_dev_mix/dfn3/leak_wpm\endcsname{147.48}
\expandafter\def\csname v@call_dev_mix/dfn3/miss\endcsname{13.49}
\expandafter\def\csname v@call_dev_mix/dfn3/wer\endcsname{73.44}
\expandafter\def\csname v@call_dev_mix/raw/dele\endcsname{1.98}
\expandafter\def\csname v@call_dev_mix/raw/dleak\endcsname{+10.07}
\expandafter\def\csname v@call_dev_mix/raw/dwer\endcsname{+14.57}
\expandafter\def\csname v@call_dev_mix/raw/dwer-hi\endcsname{+20.38}
\expandafter\def\csname v@call_dev_mix/raw/dwer-lo\endcsname{+8.90}
\expandafter\def\csname v@call_dev_mix/raw/ins\endcsname{61.62}
\expandafter\def\csname v@call_dev_mix/raw/leak_wpm\endcsname{146.25}
\expandafter\def\csname v@call_dev_mix/raw/miss\endcsname{13.08}
\expandafter\def\csname v@call_dev_mix/raw/wer\endcsname{74.70}
\expandafter\def\csname v@call_dev_mix/voxlock/dele\endcsname{3.13}
\expandafter\def\csname v@call_dev_mix/voxlock/dleak\endcsname{-12.74}
\expandafter\def\csname v@call_dev_mix/voxlock/dwer\endcsname{-1.30}
\expandafter\def\csname v@call_dev_mix/voxlock/dwer-hi\endcsname{+1.10}
\expandafter\def\csname v@call_dev_mix/voxlock/dwer-lo\endcsname{-3.81}
\expandafter\def\csname v@call_dev_mix/voxlock/ins\endcsname{38.71}
\expandafter\def\csname v@call_dev_mix/voxlock/leak_wpm\endcsname{123.45}
\expandafter\def\csname v@call_dev_mix/voxlock/miss\endcsname{20.12}
\expandafter\def\csname v@call_dev_mix/voxlock/wer\endcsname{58.84}
\expandafter\def\csname v@call_dev_mix/voxlock_live/dele\endcsname{2.45}
\expandafter\def\csname v@call_dev_mix/voxlock_live/dleak\endcsname{-10.07}
\expandafter\def\csname v@call_dev_mix/voxlock_live/dwer\endcsname{+4.68}
\expandafter\def\csname v@call_dev_mix/voxlock_live/dwer-hi\endcsname{+10.10}
\expandafter\def\csname v@call_dev_mix/voxlock_live/dwer-lo\endcsname{-0.91}
\expandafter\def\csname v@call_dev_mix/voxlock_live/ins\endcsname{45.12}
\expandafter\def\csname v@call_dev_mix/voxlock_live/leak_wpm\endcsname{126.12}
\expandafter\def\csname v@call_dev_mix/voxlock_live/miss\endcsname{19.70}
\expandafter\def\csname v@call_dev_mix/voxlock_live/wer\endcsname{64.82}
\expandafter\def\csname v@call_dev_mix/voxlock_pt/dele\endcsname{2.58}
\expandafter\def\csname v@call_dev_mix/voxlock_pt/ins\endcsname{42.29}
\expandafter\def\csname v@call_dev_mix/voxlock_pt/leak_wpm\endcsname{136.19}
\expandafter\def\csname v@call_dev_mix/voxlock_pt/miss\endcsname{17.85}
\expandafter\def\csname v@call_dev_mix/voxlock_pt/wer\endcsname{60.14}
\expandafter\def\csname v@call_test_clean/C22_ftlong_kd_selfl/dele\endcsname{2.04}
\expandafter\def\csname v@call_test_clean/C22_ftlong_kd_selfl/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/C22_ftlong_kd_selfl/dwer\endcsname{+2.45}
\expandafter\def\csname v@call_test_clean/C22_ftlong_kd_selfl/dwer-hi\endcsname{+3.63}
\expandafter\def\csname v@call_test_clean/C22_ftlong_kd_selfl/dwer-lo\endcsname{+1.34}
\expandafter\def\csname v@call_test_clean/C22_ftlong_kd_selfl/ins\endcsname{1.09}
\expandafter\def\csname v@call_test_clean/C22_ftlong_kd_selfl/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/C22_ftlong_kd_selfl/miss\endcsname{4.23}
\expandafter\def\csname v@call_test_clean/C22_ftlong_kd_selfl/wer\endcsname{5.32}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_loud/dele\endcsname{2.47}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_loud/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_loud/dwer\endcsname{+2.79}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_loud/dwer-hi\endcsname{+4.18}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_loud/dwer-lo\endcsname{+1.53}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_loud/ins\endcsname{1.09}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_loud/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_loud/miss\endcsname{4.57}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_loud/wer\endcsname{5.66}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_null/dele\endcsname{2.74}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{+3.03}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+4.49}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{+1.73}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_null/ins\endcsname{1.08}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_null/miss\endcsname{4.82}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_null/wer\endcsname{5.90}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{2.58}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{+2.70}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+4.06}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{+1.53}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{0.99}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{4.58}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{5.58}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_loud/dele\endcsname{4.01}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_loud/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_loud/dwer\endcsname{+4.73}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_loud/dwer-hi\endcsname{+6.41}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_loud/dwer-lo\endcsname{+3.31}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_loud/ins\endcsname{1.15}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_loud/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_loud/miss\endcsname{6.45}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_loud/wer\endcsname{7.60}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_null/dele\endcsname{3.50}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_null/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_null/dwer\endcsname{+3.96}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_null/dwer-hi\endcsname{+5.19}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_null/dwer-lo\endcsname{+2.78}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_null/ins\endcsname{1.16}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_null/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_null/miss\endcsname{5.67}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_null/wer\endcsname{6.84}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_selfl/dele\endcsname{5.16}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_selfl/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_selfl/dwer\endcsname{+5.93}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_selfl/dwer-hi\endcsname{+7.57}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_selfl/dwer-lo\endcsname{+4.43}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_selfl/ins\endcsname{1.18}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_selfl/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_selfl/miss\endcsname{7.62}
\expandafter\def\csname v@call_test_clean/MB_ftlong_ws_selfl/wer\endcsname{8.80}
\expandafter\def\csname v@call_test_clean/SB_ftlong_ws_selfl/dele\endcsname{4.58}
\expandafter\def\csname v@call_test_clean/SB_ftlong_ws_selfl/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/SB_ftlong_ws_selfl/dwer\endcsname{+5.67}
\expandafter\def\csname v@call_test_clean/SB_ftlong_ws_selfl/dwer-hi\endcsname{+7.31}
\expandafter\def\csname v@call_test_clean/SB_ftlong_ws_selfl/dwer-lo\endcsname{+4.17}
\expandafter\def\csname v@call_test_clean/SB_ftlong_ws_selfl/ins\endcsname{1.19}
\expandafter\def\csname v@call_test_clean/SB_ftlong_ws_selfl/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/SB_ftlong_ws_selfl/miss\endcsname{7.36}
\expandafter\def\csname v@call_test_clean/SB_ftlong_ws_selfl/wer\endcsname{8.55}
\expandafter\def\csname v@call_test_clean/dfn3/dele\endcsname{0.78}
\expandafter\def\csname v@call_test_clean/dfn3/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/dfn3/dwer\endcsname{-0.24}
\expandafter\def\csname v@call_test_clean/dfn3/dwer-hi\endcsname{+0.61}
\expandafter\def\csname v@call_test_clean/dfn3/dwer-lo\endcsname{-1.08}
\expandafter\def\csname v@call_test_clean/dfn3/ins\endcsname{0.93}
\expandafter\def\csname v@call_test_clean/dfn3/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/dfn3/miss\endcsname{1.70}
\expandafter\def\csname v@call_test_clean/dfn3/wer\endcsname{2.63}
\expandafter\def\csname v@call_test_clean/raw/dele\endcsname{0.00}
\expandafter\def\csname v@call_test_clean/raw/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/raw/dwer\endcsname{-2.84}
\expandafter\def\csname v@call_test_clean/raw/dwer-hi\endcsname{-2.10}
\expandafter\def\csname v@call_test_clean/raw/dwer-lo\endcsname{-3.70}
\expandafter\def\csname v@call_test_clean/raw/ins\endcsname{0.00}
\expandafter\def\csname v@call_test_clean/raw/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/raw/miss\endcsname{0.04}
\expandafter\def\csname v@call_test_clean/raw/wer\endcsname{0.04}
\expandafter\def\csname v@call_test_clean/voxlock/dele\endcsname{1.32}
\expandafter\def\csname v@call_test_clean/voxlock/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/voxlock/dwer\endcsname{+0.50}
\expandafter\def\csname v@call_test_clean/voxlock/dwer-hi\endcsname{+0.95}
\expandafter\def\csname v@call_test_clean/voxlock/dwer-lo\endcsname{+0.08}
\expandafter\def\csname v@call_test_clean/voxlock/ins\endcsname{0.59}
\expandafter\def\csname v@call_test_clean/voxlock/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/voxlock/miss\endcsname{2.78}
\expandafter\def\csname v@call_test_clean/voxlock/wer\endcsname{3.37}
\expandafter\def\csname v@call_test_clean/voxlock_live/dele\endcsname{0.78}
\expandafter\def\csname v@call_test_clean/voxlock_live/dleak\endcsname{+nan}
\expandafter\def\csname v@call_test_clean/voxlock_live/dwer\endcsname{+0.05}
\expandafter\def\csname v@call_test_clean/voxlock_live/dwer-hi\endcsname{+0.74}
\expandafter\def\csname v@call_test_clean/voxlock_live/dwer-lo\endcsname{-0.68}
\expandafter\def\csname v@call_test_clean/voxlock_live/ins\endcsname{0.73}
\expandafter\def\csname v@call_test_clean/voxlock_live/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/voxlock_live/miss\endcsname{2.19}
\expandafter\def\csname v@call_test_clean/voxlock_live/wer\endcsname{2.92}
\expandafter\def\csname v@call_test_clean/voxlock_pt/dele\endcsname{0.85}
\expandafter\def\csname v@call_test_clean/voxlock_pt/ins\endcsname{0.56}
\expandafter\def\csname v@call_test_clean/voxlock_pt/leak_wpm\endcsname{nan}
\expandafter\def\csname v@call_test_clean/voxlock_pt/miss\endcsname{2.32}
\expandafter\def\csname v@call_test_clean/voxlock_pt/wer\endcsname{2.87}
\expandafter\def\csname v@call_test_mix/C22_ftlong_kd_selfl/dele\endcsname{4.67}
\expandafter\def\csname v@call_test_mix/C22_ftlong_kd_selfl/dleak\endcsname{-2.01}
\expandafter\def\csname v@call_test_mix/C22_ftlong_kd_selfl/dwer\endcsname{+1.31}
\expandafter\def\csname v@call_test_mix/C22_ftlong_kd_selfl/dwer-hi\endcsname{+6.74}
\expandafter\def\csname v@call_test_mix/C22_ftlong_kd_selfl/dwer-lo\endcsname{-3.97}
\expandafter\def\csname v@call_test_mix/C22_ftlong_kd_selfl/ins\endcsname{24.46}
\expandafter\def\csname v@call_test_mix/C22_ftlong_kd_selfl/leak_wpm\endcsname{63.32}
\expandafter\def\csname v@call_test_mix/C22_ftlong_kd_selfl/miss\endcsname{25.44}
\expandafter\def\csname v@call_test_mix/C22_ftlong_kd_selfl/wer\endcsname{49.90}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_loud/dele\endcsname{4.53}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_loud/dleak\endcsname{-6.49}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_loud/dwer\endcsname{-0.73}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_loud/dwer-hi\endcsname{+4.36}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_loud/dwer-lo\endcsname{-5.99}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_loud/ins\endcsname{21.49}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_loud/leak_wpm\endcsname{58.84}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_loud/miss\endcsname{26.38}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_loud/wer\endcsname{47.87}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_null/dele\endcsname{4.69}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{-7.32}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-1.16}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+4.82}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-7.29}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_null/ins\endcsname{22.28}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{58.02}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_null/miss\endcsname{25.15}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_null/wer\endcsname{47.43}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{4.70}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-8.45}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-1.08}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+4.23}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-6.71}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{20.12}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{56.88}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{27.39}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{47.52}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_loud/dele\endcsname{5.73}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_loud/dleak\endcsname{-7.26}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_loud/dwer\endcsname{-0.61}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_loud/dwer-hi\endcsname{+4.83}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_loud/dwer-lo\endcsname{-5.78}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_loud/ins\endcsname{20.86}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_loud/leak_wpm\endcsname{58.07}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_loud/miss\endcsname{27.13}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_loud/wer\endcsname{47.99}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_null/dele\endcsname{5.07}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_null/dleak\endcsname{-0.31}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_null/dwer\endcsname{+2.25}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_null/dwer-hi\endcsname{+8.24}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_null/dwer-lo\endcsname{-3.98}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_null/ins\endcsname{24.61}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_null/leak_wpm\endcsname{65.02}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_null/miss\endcsname{26.24}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_null/wer\endcsname{50.85}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_selfl/dele\endcsname{6.06}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_selfl/dleak\endcsname{-6.70}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_selfl/dwer\endcsname{-0.38}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_selfl/dwer-hi\endcsname{+5.06}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_selfl/dwer-lo\endcsname{-5.86}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_selfl/ins\endcsname{19.89}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_selfl/leak_wpm\endcsname{58.63}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_selfl/miss\endcsname{28.33}
\expandafter\def\csname v@call_test_mix/MB_ftlong_ws_selfl/wer\endcsname{48.22}
\expandafter\def\csname v@call_test_mix/SB_ftlong_ws_selfl/dele\endcsname{4.87}
\expandafter\def\csname v@call_test_mix/SB_ftlong_ws_selfl/dleak\endcsname{-4.74}
\expandafter\def\csname v@call_test_mix/SB_ftlong_ws_selfl/dwer\endcsname{+0.27}
\expandafter\def\csname v@call_test_mix/SB_ftlong_ws_selfl/dwer-hi\endcsname{+5.98}
\expandafter\def\csname v@call_test_mix/SB_ftlong_ws_selfl/dwer-lo\endcsname{-5.37}
\expandafter\def\csname v@call_test_mix/SB_ftlong_ws_selfl/ins\endcsname{22.18}
\expandafter\def\csname v@call_test_mix/SB_ftlong_ws_selfl/leak_wpm\endcsname{60.59}
\expandafter\def\csname v@call_test_mix/SB_ftlong_ws_selfl/miss\endcsname{26.68}
\expandafter\def\csname v@call_test_mix/SB_ftlong_ws_selfl/wer\endcsname{48.86}
\expandafter\def\csname v@call_test_mix/dfn3/dele\endcsname{2.95}
\expandafter\def\csname v@call_test_mix/dfn3/dleak\endcsname{+47.71}
\expandafter\def\csname v@call_test_mix/dfn3/dwer\endcsname{+21.05}
\expandafter\def\csname v@call_test_mix/dfn3/dwer-hi\endcsname{+28.13}
\expandafter\def\csname v@call_test_mix/dfn3/dwer-lo\endcsname{+14.22}
\expandafter\def\csname v@call_test_mix/dfn3/ins\endcsname{44.05}
\expandafter\def\csname v@call_test_mix/dfn3/leak_wpm\endcsname{113.04}
\expandafter\def\csname v@call_test_mix/dfn3/miss\endcsname{25.60}
\expandafter\def\csname v@call_test_mix/dfn3/wer\endcsname{69.65}
\expandafter\def\csname v@call_test_mix/raw/dele\endcsname{2.59}
\expandafter\def\csname v@call_test_mix/raw/dleak\endcsname{+48.28}
\expandafter\def\csname v@call_test_mix/raw/dwer\endcsname{+21.20}
\expandafter\def\csname v@call_test_mix/raw/dwer-hi\endcsname{+28.52}
\expandafter\def\csname v@call_test_mix/raw/dwer-lo\endcsname{+14.14}
\expandafter\def\csname v@call_test_mix/raw/ins\endcsname{47.27}
\expandafter\def\csname v@call_test_mix/raw/leak_wpm\endcsname{113.61}
\expandafter\def\csname v@call_test_mix/raw/miss\endcsname{22.52}
\expandafter\def\csname v@call_test_mix/raw/wer\endcsname{69.79}
\expandafter\def\csname v@call_test_mix/voxlock/dele\endcsname{3.52}
\expandafter\def\csname v@call_test_mix/voxlock/dleak\endcsname{-3.66}
\expandafter\def\csname v@call_test_mix/voxlock/dwer\endcsname{-1.54}
\expandafter\def\csname v@call_test_mix/voxlock/dwer-hi\endcsname{+0.14}
\expandafter\def\csname v@call_test_mix/voxlock/dwer-lo\endcsname{-3.43}
\expandafter\def\csname v@call_test_mix/voxlock/ins\endcsname{23.52}
\expandafter\def\csname v@call_test_mix/voxlock/leak_wpm\endcsname{61.67}
\expandafter\def\csname v@call_test_mix/voxlock/miss\endcsname{23.54}
\expandafter\def\csname v@call_test_mix/voxlock/wer\endcsname{47.05}
\expandafter\def\csname v@call_test_mix/voxlock_live/dele\endcsname{2.92}
\expandafter\def\csname v@call_test_mix/voxlock_live/dleak\endcsname{+9.69}
\expandafter\def\csname v@call_test_mix/voxlock_live/dwer\endcsname{+8.06}
\expandafter\def\csname v@call_test_mix/voxlock_live/dwer-hi\endcsname{+14.88}
\expandafter\def\csname v@call_test_mix/voxlock_live/dwer-lo\endcsname{+1.73}
\expandafter\def\csname v@call_test_mix/voxlock_live/ins\endcsname{27.24}
\expandafter\def\csname v@call_test_mix/voxlock_live/leak_wpm\endcsname{75.02}
\expandafter\def\csname v@call_test_mix/voxlock_live/miss\endcsname{29.42}
\expandafter\def\csname v@call_test_mix/voxlock_live/wer\endcsname{56.65}
\expandafter\def\csname v@call_test_mix/voxlock_pt/dele\endcsname{2.87}
\expandafter\def\csname v@call_test_mix/voxlock_pt/ins\endcsname{25.15}
\expandafter\def\csname v@call_test_mix/voxlock_pt/leak_wpm\endcsname{65.33}
\expandafter\def\csname v@call_test_mix/voxlock_pt/miss\endcsname{23.44}
\expandafter\def\csname v@call_test_mix/voxlock_pt/wer\endcsname{48.59}
\expandafter\def\csname v@calls/ami_dev/sil3pm\endcsname{0.0}
\expandafter\def\csname v@calls/ami_dev/silent\endcsname{6}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2gm_null/elsewhere\endcsname{41}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2gm_null/start\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2gm_null/start_t0\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2gm_selfl/elsewhere\endcsname{44}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2gm_selfl/start\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2gm_selfl/start_t0\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2hm_null/elsewhere\endcsname{42}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2hm_null/start\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2hm_null/start_t0\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2hm_selfl/elsewhere\endcsname{44}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2hm_selfl/start\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2hm_selfl/start_t0\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2mr_selfl/elsewhere\endcsname{45}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2mr_selfl/start\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2mr_selfl/start_t0\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2r_selfl/elsewhere\endcsname{44}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2r_selfl/start\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/MB_ftlong_ws_cwlt2r_selfl/start_t0\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2_selfl/elsewhere\endcsname{45}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2_selfl/start\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2_selfl/start_t0\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2g_selfl/elsewhere\endcsname{44}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2g_selfl/start\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2g_selfl/start_t0\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2gc_selfl/elsewhere\endcsname{45}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2gc_selfl/start\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2gc_selfl/start_t0\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2h_selfl/elsewhere\endcsname{44}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2h_selfl/start\endcsname{11}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2h_selfl/start_t0\endcsname{11}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2m_selfl/elsewhere\endcsname{44}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2m_selfl/start\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/SB_ftlong_ws_cwlt2m_selfl/start_t0\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/opens_mid\endcsname{120}
\expandafter\def\csname v@calls/ami_dev_long/pre_selfl/elsewhere\endcsname{45}
\expandafter\def\csname v@calls/ami_dev_long/pre_selfl/start\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/pre_selfl/start_t0\endcsname{12}
\expandafter\def\csname v@calls/ami_dev_long/recordings\endcsname{120}
\expandafter\def\csname v@calls/ami_dev_long/rel_null/elsewhere\endcsname{42}
\expandafter\def\csname v@calls/ami_dev_long/rel_null/start\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/rel_null/start_t0\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/rel_selfl/elsewhere\endcsname{45}
\expandafter\def\csname v@calls/ami_dev_long/rel_selfl/start\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/rel_selfl/start_t0\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/sil3pm\endcsname{0.0}
\expandafter\def\csname v@calls/ami_dev_long/silent\endcsname{9}
\expandafter\def\csname v@calls/ami_dev_long/starts_late\endcsname{0}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_null/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_null/return\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_null/start\endcsname{17}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_null/start_late\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_null/start_t0\endcsname{28}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_selfl/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_selfl/return\endcsname{10}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_selfl/start\endcsname{19}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_selfl/start_late\endcsname{10}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2g5_selfl/start_t0\endcsname{28}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_null/elsewhere\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_null/return\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_null/start\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_null/start_late\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_null/start_t0\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_selfl/elsewhere\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_selfl/return\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_selfl/start\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_selfl/start_late\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2gm_selfl/start_t0\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_null/elsewhere\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_null/return\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_null/start\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_null/start_late\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_null/start_t0\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_selfl/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_selfl/return\endcsname{9}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_selfl/start\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_selfl/start_late\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2hm_selfl/start_t0\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2mr_selfl/elsewhere\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2mr_selfl/return\endcsname{10}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2mr_selfl/start\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2mr_selfl/start_late\endcsname{9}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2mr_selfl/start_t0\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2r_selfl/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2r_selfl/return\endcsname{9}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2r_selfl/start\endcsname{27}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2r_selfl/start_late\endcsname{10}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_cwlt2r_selfl/start_t0\endcsname{41}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_selfl/elsewhere\endcsname{10}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_selfl/return\endcsname{15}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_selfl/start\endcsname{27}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_selfl/start_late\endcsname{25}
\expandafter\def\csname v@calls/call_dev_clean/MB_ftlong_ws_selfl/start_t0\endcsname{32}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_null/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_null/return\endcsname{8}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_null/start\endcsname{20}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_null/start_late\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_null/start_t0\endcsname{33}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_selfl/elsewhere\endcsname{8}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_selfl/return\endcsname{14}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_selfl/start\endcsname{26}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_selfl/start_late\endcsname{21}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2_selfl/start_t0\endcsname{33}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2g_selfl/elsewhere\endcsname{8}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2g_selfl/return\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2g_selfl/start\endcsname{26}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2g_selfl/start_late\endcsname{23}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2g_selfl/start_t0\endcsname{30}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_null/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_null/return\endcsname{9}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_null/start\endcsname{26}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_null/start_late\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_null/start_t0\endcsname{45}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_selfl/elsewhere\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_selfl/return\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_selfl/start\endcsname{28}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_selfl/start_late\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gc_selfl/start_t0\endcsname{44}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_null/elsewhere\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_null/return\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_null/start\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_null/start_late\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_null/start_t0\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_selfl/elsewhere\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_selfl/return\endcsname{10}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_selfl/start\endcsname{8}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_selfl/start_late\endcsname{14}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2gm_selfl/start_t0\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2h_selfl/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2h_selfl/return\endcsname{10}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2h_selfl/start\endcsname{20}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2h_selfl/start_late\endcsname{13}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2h_selfl/start_t0\endcsname{28}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2m_selfl/elsewhere\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2m_selfl/return\endcsname{14}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2m_selfl/start\endcsname{8}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2m_selfl/start_late\endcsname{13}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2m_selfl/start_t0\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2mr_selfl/elsewhere\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2mr_selfl/return\endcsname{12}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2mr_selfl/start\endcsname{9}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2mr_selfl/start_late\endcsname{16}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2mr_selfl/start_t0\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2r_selfl/elsewhere\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2r_selfl/return\endcsname{13}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2r_selfl/start\endcsname{20}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2r_selfl/start_late\endcsname{14}
\expandafter\def\csname v@calls/call_dev_clean/SB_ftlong_ws_cwlt2r_selfl/start_t0\endcsname{27}
\expandafter\def\csname v@calls/call_dev_clean/dfn3/elsewhere\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/dfn3/return\endcsname{2}
\expandafter\def\csname v@calls/call_dev_clean/dfn3/start\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/dfn3/start_late\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/dfn3/start_t0\endcsname{2}
\expandafter\def\csname v@calls/call_dev_clean/opens_mid\endcsname{55}
\expandafter\def\csname v@calls/call_dev_clean/pre_loud/elsewhere\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/pre_loud/return\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/pre_loud/start\endcsname{17}
\expandafter\def\csname v@calls/call_dev_clean/pre_loud/start_late\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/pre_loud/start_t0\endcsname{28}
\expandafter\def\csname v@calls/call_dev_clean/pre_null/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_null/return\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/pre_null/start\endcsname{22}
\expandafter\def\csname v@calls/call_dev_clean/pre_null/start_late\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/pre_null/start_t0\endcsname{38}
\expandafter\def\csname v@calls/call_dev_clean/pre_null_pr1/elsewhere\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/pre_null_pr1/return\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/pre_null_pr1/start\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/pre_null_pr1/start_late\endcsname{2}
\expandafter\def\csname v@calls/call_dev_clean/pre_null_pr1/start_t0\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl/return\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl/start\endcsname{23}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl/start_late\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl/start_t0\endcsname{38}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl1/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl1/return\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl1/start\endcsname{21}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl1/start_late\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl1/start_t0\endcsname{34}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl2/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl2/return\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl2/start\endcsname{23}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl2/start_late\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl2/start_t0\endcsname{37}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pr1/elsewhere\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pr1/return\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pr1/start\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pr1/start_late\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pr1/start_t0\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pt3/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pt3/return\endcsname{11}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pt3/start\endcsname{2}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pt3/start_late\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfl_pt3/start_t0\endcsname{0}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls/return\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls/start\endcsname{29}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls/start_late\endcsname{18}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls/start_t0\endcsname{39}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls_pr1/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls_pr1/return\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls_pr1/start\endcsname{4}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls_pr1/start_late\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/pre_selfls_pr1/start_t0\endcsname{2}
\expandafter\def\csname v@calls/call_dev_clean/recordings\endcsname{120}
\expandafter\def\csname v@calls/call_dev_clean/rel_null/elsewhere\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/rel_null/return\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/rel_null/start\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/rel_null/start_late\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/rel_null/start_t0\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/rel_selfl/elsewhere\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/rel_selfl/return\endcsname{13}
\expandafter\def\csname v@calls/call_dev_clean/rel_selfl/start\endcsname{7}
\expandafter\def\csname v@calls/call_dev_clean/rel_selfl/start_late\endcsname{9}
\expandafter\def\csname v@calls/call_dev_clean/rel_selfl/start_t0\endcsname{6}
\expandafter\def\csname v@calls/call_dev_clean/sil3pm\endcsname{1.8}
\expandafter\def\csname v@calls/call_dev_clean/silent\endcsname{51}
\expandafter\def\csname v@calls/call_dev_clean/starts_late\endcsname{53}
\expandafter\def\csname v@calls/call_dev_clean/voxlock/elsewhere\endcsname{10}
\expandafter\def\csname v@calls/call_dev_clean/voxlock/return\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/voxlock/start\endcsname{8}
\expandafter\def\csname v@calls/call_dev_clean/voxlock/start_late\endcsname{10}
\expandafter\def\csname v@calls/call_dev_clean/voxlock/start_t0\endcsname{8}
\expandafter\def\csname v@calls/call_dev_clean/voxlock_live/elsewhere\endcsname{5}
\expandafter\def\csname v@calls/call_dev_clean/voxlock_live/return\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/voxlock_live/start\endcsname{1}
\expandafter\def\csname v@calls/call_dev_clean/voxlock_live/start_late\endcsname{3}
\expandafter\def\csname v@calls/call_dev_clean/voxlock_live/start_t0\endcsname{0}
\expandafter\def\csname v@calls/call_dev_mix/sil3pm\endcsname{0.5}
\expandafter\def\csname v@calls/call_dev_mix/silent\endcsname{26}
\expandafter\def\csname v@calls/call_test_clean/MB_ftlong_ws_selfl/elsewhere\endcsname{13}
\expandafter\def\csname v@calls/call_test_clean/MB_ftlong_ws_selfl/return\endcsname{10}
\expandafter\def\csname v@calls/call_test_clean/MB_ftlong_ws_selfl/start\endcsname{25}
\expandafter\def\csname v@calls/call_test_clean/dfn3/elsewhere\endcsname{4}
\expandafter\def\csname v@calls/call_test_clean/dfn3/return\endcsname{1}
\expandafter\def\csname v@calls/call_test_clean/dfn3/start\endcsname{4}
\expandafter\def\csname v@calls/call_test_clean/dfn3/start_late\endcsname{4}
\expandafter\def\csname v@calls/call_test_clean/dfn3/start_t0\endcsname{4}
\expandafter\def\csname v@calls/call_test_clean/opens_mid\endcsname{60}
\expandafter\def\csname v@calls/call_test_clean/pre_loud/elsewhere\endcsname{11}
\expandafter\def\csname v@calls/call_test_clean/pre_loud/return\endcsname{10}
\expandafter\def\csname v@calls/call_test_clean/pre_loud/start\endcsname{16}
\expandafter\def\csname v@calls/call_test_clean/pre_null/elsewhere\endcsname{10}
\expandafter\def\csname v@calls/call_test_clean/pre_null/return\endcsname{8}
\expandafter\def\csname v@calls/call_test_clean/pre_null/start\endcsname{22}
\expandafter\def\csname v@calls/call_test_clean/pre_null/start_late\endcsname{2}
\expandafter\def\csname v@calls/call_test_clean/pre_null/start_t0\endcsname{40}
\expandafter\def\csname v@calls/call_test_clean/pre_selfl/elsewhere\endcsname{11}
\expandafter\def\csname v@calls/call_test_clean/pre_selfl/return\endcsname{10}
\expandafter\def\csname v@calls/call_test_clean/pre_selfl/start\endcsname{23}
\expandafter\def\csname v@calls/call_test_clean/pre_selfl/start_late\endcsname{7}
\expandafter\def\csname v@calls/call_test_clean/pre_selfl/start_t0\endcsname{40}
\expandafter\def\csname v@calls/call_test_clean/recordings\endcsname{120}
\expandafter\def\csname v@calls/call_test_clean/rel_loud/elsewhere\endcsname{11}
\expandafter\def\csname v@calls/call_test_clean/rel_loud/return\endcsname{8}
\expandafter\def\csname v@calls/call_test_clean/rel_loud/start\endcsname{5}
\expandafter\def\csname v@calls/call_test_clean/rel_loud/start_late\endcsname{3}
\expandafter\def\csname v@calls/call_test_clean/rel_loud/start_t0\endcsname{6}
\expandafter\def\csname v@calls/call_test_clean/rel_null/elsewhere\endcsname{11}
\expandafter\def\csname v@calls/call_test_clean/rel_null/return\endcsname{7}
\expandafter\def\csname v@calls/call_test_clean/rel_null/start\endcsname{5}
\expandafter\def\csname v@calls/call_test_clean/rel_null/start_late\endcsname{3}
\expandafter\def\csname v@calls/call_test_clean/rel_null/start_t0\endcsname{8}
\expandafter\def\csname v@calls/call_test_clean/rel_selfl/elsewhere\endcsname{12}
\expandafter\def\csname v@calls/call_test_clean/rel_selfl/return\endcsname{8}
\expandafter\def\csname v@calls/call_test_clean/rel_selfl/start\endcsname{7}
\expandafter\def\csname v@calls/call_test_clean/rel_selfl/start_late\endcsname{8}
\expandafter\def\csname v@calls/call_test_clean/rel_selfl/start_t0\endcsname{8}
\expandafter\def\csname v@calls/call_test_clean/sil3pm\endcsname{2.8}
\expandafter\def\csname v@calls/call_test_clean/silent\endcsname{53}
\expandafter\def\csname v@calls/call_test_clean/starts_late\endcsname{43}
\expandafter\def\csname v@calls/call_test_clean/voxlock/elsewhere\endcsname{10}
\expandafter\def\csname v@calls/call_test_clean/voxlock/return\endcsname{5}
\expandafter\def\csname v@calls/call_test_clean/voxlock/start\endcsname{7}
\expandafter\def\csname v@calls/call_test_clean/voxlock/start_late\endcsname{2}
\expandafter\def\csname v@calls/call_test_clean/voxlock/start_t0\endcsname{12}
\expandafter\def\csname v@calls/call_test_clean/voxlock_live/elsewhere\endcsname{9}
\expandafter\def\csname v@calls/call_test_clean/voxlock_live/return\endcsname{5}
\expandafter\def\csname v@calls/call_test_clean/voxlock_live/start\endcsname{0}
\expandafter\def\csname v@calls/call_test_clean/voxlock_live/start_late\endcsname{0}
\expandafter\def\csname v@calls/call_test_clean/voxlock_live/start_t0\endcsname{0}
\expandafter\def\csname v@calls/krisp/sil3pm\endcsname{0.1}
\expandafter\def\csname v@calls/krisp/silent\endcsname{8}
\expandafter\def\csname v@calls/nsf_dev/sil3pm\endcsname{0.0}
\expandafter\def\csname v@calls/nsf_dev/silent\endcsname{2}
\expandafter\def\csname v@cpu/C10/fp32_B1/core-per-call\endcsname{0.36}
\expandafter\def\csname v@cpu/C10/fp32_B1/p99\endcsname{10}
\expandafter\def\csname v@cpu/C10/fp32_B32/core-per-call\endcsname{0.17}
\expandafter\def\csname v@cpu/C10/fp32_B32/p99\endcsname{134}
\expandafter\def\csname v@cpu/C10/fp32_B8/core-per-call\endcsname{0.15}
\expandafter\def\csname v@cpu/C10/fp32_B8/p99\endcsname{31}
\expandafter\def\csname v@cpu/C10/int8_B1/core-per-call\endcsname{0.38}
\expandafter\def\csname v@cpu/C10/int8_B1/p99\endcsname{8}
\expandafter\def\csname v@cpu/C10/int8_B32/core-per-call\endcsname{0.16}
\expandafter\def\csname v@cpu/C10/int8_B32/p99\endcsname{122}
\expandafter\def\csname v@cpu/C10/int8_B8/core-per-call\endcsname{0.14}
\expandafter\def\csname v@cpu/C10/int8_B8/p99\endcsname{30}
\expandafter\def\csname v@cpu/C10/params-m\endcsname{9.8}
\expandafter\def\csname v@cpu/C22/fp32_B1/core-per-call\endcsname{0.56}
\expandafter\def\csname v@cpu/C22/fp32_B1/p99\endcsname{16}
\expandafter\def\csname v@cpu/C22/fp32_B32/core-per-call\endcsname{0.28}
\expandafter\def\csname v@cpu/C22/fp32_B32/p99\endcsname{197}
\expandafter\def\csname v@cpu/C22/fp32_B8/core-per-call\endcsname{0.28}
\expandafter\def\csname v@cpu/C22/fp32_B8/p99\endcsname{51}
\expandafter\def\csname v@cpu/C22/int8_B1/core-per-call\endcsname{0.52}
\expandafter\def\csname v@cpu/C22/int8_B1/p99\endcsname{15}
\expandafter\def\csname v@cpu/C22/int8_B32/core-per-call\endcsname{0.26}
\expandafter\def\csname v@cpu/C22/int8_B32/p99\endcsname{191}
\expandafter\def\csname v@cpu/C22/int8_B8/core-per-call\endcsname{0.23}
\expandafter\def\csname v@cpu/C22/int8_B8/p99\endcsname{47}
\expandafter\def\csname v@cpu/C22/params-m\endcsname{22.1}
\expandafter\def\csname v@cpu/C36/fp32_B1/core-per-call\endcsname{0.75}
\expandafter\def\csname v@cpu/C36/fp32_B1/p99\endcsname{18}
\expandafter\def\csname v@cpu/C36/fp32_B32/core-per-call\endcsname{0.39}
\expandafter\def\csname v@cpu/C36/fp32_B32/p99\endcsname{284}
\expandafter\def\csname v@cpu/C36/fp32_B8/core-per-call\endcsname{0.40}
\expandafter\def\csname v@cpu/C36/fp32_B8/p99\endcsname{75}
\expandafter\def\csname v@cpu/C36/int8_B1/core-per-call\endcsname{0.62}
\expandafter\def\csname v@cpu/C36/int8_B1/p99\endcsname{15}
\expandafter\def\csname v@cpu/C36/int8_B32/core-per-call\endcsname{0.35}
\expandafter\def\csname v@cpu/C36/int8_B32/p99\endcsname{255}
\expandafter\def\csname v@cpu/C36/int8_B8/core-per-call\endcsname{0.31}
\expandafter\def\csname v@cpu/C36/int8_B8/p99\endcsname{59}
\expandafter\def\csname v@cpu/C36/params-m\endcsname{36.2}
\expandafter\def\csname v@cpu/C51/fp32_B1/core-per-call\endcsname{1.14}
\expandafter\def\csname v@cpu/C51/fp32_B1/p99\endcsname{31}
\expandafter\def\csname v@cpu/C51/fp32_B32/core-per-call\endcsname{0.67}
\expandafter\def\csname v@cpu/C51/fp32_B32/p99\endcsname{623}
\expandafter\def\csname v@cpu/C51/fp32_B8/core-per-call\endcsname{0.59}
\expandafter\def\csname v@cpu/C51/fp32_B8/p99\endcsname{108}
\expandafter\def\csname v@cpu/C51/int8_B1/core-per-call\endcsname{0.81}
\expandafter\def\csname v@cpu/C51/int8_B1/p99\endcsname{19}
\expandafter\def\csname v@cpu/C51/int8_B32/core-per-call\endcsname{0.57}
\expandafter\def\csname v@cpu/C51/int8_B32/p99\endcsname{443}
\expandafter\def\csname v@cpu/C51/int8_B8/core-per-call\endcsname{0.46}
\expandafter\def\csname v@cpu/C51/int8_B8/p99\endcsname{83}
\expandafter\def\csname v@cpu/C51/params-m\endcsname{50.9}
\expandafter\def\csname v@cpu/M/fp32_B1/core-per-call\endcsname{5.05}
\expandafter\def\csname v@cpu/M/fp32_B1/p99\endcsname{117}
\expandafter\def\csname v@cpu/M/params-m\endcsname{242.9}
\expandafter\def\csname v@cpu/S/fp32_B1/core-per-call\endcsname{3.36}
\expandafter\def\csname v@cpu/S/fp32_B1/p99\endcsname{75}
\expandafter\def\csname v@cpu/S/params-m\endcsname{140.0}
\expandafter\def\csname v@cpu/cmp/gtcrn/10/core\endcsname{5}
\expandafter\def\csname v@cpu/cmp/gtcrn/10/p99\endcsname{0.9}
\expandafter\def\csname v@cpu/cmp/gtcrn/20/core\endcsname{5}
\expandafter\def\csname v@cpu/cmp/gtcrn/20/p99\endcsname{1.7}
\expandafter\def\csname v@cpu/cmp/gtcrn/50/core\endcsname{5}
\expandafter\def\csname v@cpu/cmp/gtcrn/50/p99\endcsname{4.2}
\expandafter\def\csname v@cpu/cmp/inworld/20/core\endcsname{927}
\expandafter\def\csname v@cpu/cmp/inworld/20/p99\endcsname{302.3}
\expandafter\def\csname v@cpu/cmp/inworld/50/core\endcsname{936}
\expandafter\def\csname v@cpu/cmp/inworld/50/p99\endcsname{782.9}
\expandafter\def\csname v@cpu/cmp/ours-int8/10/core\endcsname{34}
\expandafter\def\csname v@cpu/cmp/ours-int8/10/p99\endcsname{4.0}
\expandafter\def\csname v@cpu/cmp/ours-int8/20/core\endcsname{23}
\expandafter\def\csname v@cpu/cmp/ours-int8/20/p99\endcsname{5.2}
\expandafter\def\csname v@cpu/cmp/ours-int8/50/core\endcsname{12}
\expandafter\def\csname v@cpu/cmp/ours-int8/50/p99\endcsname{7.2}
\expandafter\def\csname v@cpu/cmp/ours/10/core\endcsname{54}
\expandafter\def\csname v@cpu/cmp/ours/10/p99\endcsname{5.9}
\expandafter\def\csname v@cpu/cmp/ours/20/core\endcsname{33}
\expandafter\def\csname v@cpu/cmp/ours/20/p99\endcsname{7.1}
\expandafter\def\csname v@cpu/cmp/ours/50/core\endcsname{17}
\expandafter\def\csname v@cpu/cmp/ours/50/p99\endcsname{10.2}
\expandafter\def\csname v@cpu/cmp/voxlock-fp32/10/core\endcsname{264}
\expandafter\def\csname v@cpu/cmp/voxlock-fp32/10/p99\endcsname{30.5}
\expandafter\def\csname v@cpu/cmp/voxlock-fp32/20/core\endcsname{158}
\expandafter\def\csname v@cpu/cmp/voxlock-fp32/20/p99\endcsname{35.8}
\expandafter\def\csname v@cpu/cmp/voxlock-fp32/50/core\endcsname{88}
\expandafter\def\csname v@cpu/cmp/voxlock-fp32/50/p99\endcsname{50.6}
\expandafter\def\csname v@cpu/cmp/voxlock-int8-full/10/core\endcsname{151}
\expandafter\def\csname v@cpu/cmp/voxlock-int8-full/10/p99\endcsname{20.1}
\expandafter\def\csname v@cpu/cmp/voxlock-int8-full/20/core\endcsname{92}
\expandafter\def\csname v@cpu/cmp/voxlock-int8-full/20/p99\endcsname{22.1}
\expandafter\def\csname v@cpu/cmp/voxlock-int8-full/50/core\endcsname{47}
\expandafter\def\csname v@cpu/cmp/voxlock-int8-full/50/p99\endcsname{25.6}
\expandafter\def\csname v@cpu/cmp/voxlock/10/core\endcsname{227}
\expandafter\def\csname v@cpu/cmp/voxlock/10/p99\endcsname{26.8}
\expandafter\def\csname v@cpu/cmp/voxlock/20/core\endcsname{132}
\expandafter\def\csname v@cpu/cmp/voxlock/20/p99\endcsname{29.4}
\expandafter\def\csname v@cpu/cmp/voxlock/50/core\endcsname{65}
\expandafter\def\csname v@cpu/cmp/voxlock/50/p99\endcsname{37.0}
\expandafter\def\csname v@cpu/student\endcsname{C22}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev/dele\endcsname{3.11}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev/ins\endcsname{4.40}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev/leak_wpm\endcsname{8.93}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev/miss\endcsname{9.22}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev/wer\endcsname{13.62}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev_long/dele\endcsname{6.90}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev_long/ins\endcsname{3.31}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev_long/leak_wpm\endcsname{6.53}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev_long/miss\endcsname{14.62}
\expandafter\def\csname v@cpu/student/int8_selfl/ami_dev_long/wer\endcsname{17.93}
\expandafter\def\csname v@cpu/student/int8_selfl/call_dev_clean/dele\endcsname{1.82}
\expandafter\def\csname v@cpu/student/int8_selfl/call_dev_clean/ins\endcsname{0.25}
\expandafter\def\csname v@cpu/student/int8_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@cpu/student/int8_selfl/call_dev_clean/miss\endcsname{2.59}
\expandafter\def\csname v@cpu/student/int8_selfl/call_dev_clean/wer\endcsname{2.84}
\expandafter\def\csname v@cpu/student/int8_selfl/dev4\endcsname{10.52}
\expandafter\def\csname v@cpu/student/int8_selfl/meet3\endcsname{13.08}
\expandafter\def\csname v@cpu/student/int8_selfl/nsf_dev/dele\endcsname{1.44}
\expandafter\def\csname v@cpu/student/int8_selfl/nsf_dev/ins\endcsname{1.97}
\expandafter\def\csname v@cpu/student/int8_selfl/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@cpu/student/int8_selfl/nsf_dev/miss\endcsname{5.71}
\expandafter\def\csname v@cpu/student/int8_selfl/nsf_dev/wer\endcsname{7.68}
\expandafter\def\csname v@cpu/student/selfl/aic_calls/dele\endcsname{3.35}
\expandafter\def\csname v@cpu/student/selfl/aic_calls/dleak\endcsname{-4.98}
\expandafter\def\csname v@cpu/student/selfl/aic_calls/dwer\endcsname{-2.46}
\expandafter\def\csname v@cpu/student/selfl/aic_calls/dwer-hi\endcsname{+4.15}
\expandafter\def\csname v@cpu/student/selfl/aic_calls/dwer-lo\endcsname{-31.73}
\expandafter\def\csname v@cpu/student/selfl/aic_calls/ins\endcsname{11.40}
\expandafter\def\csname v@cpu/student/selfl/aic_calls/leak_wpm\endcsname{13.25}
\expandafter\def\csname v@cpu/student/selfl/aic_calls/miss\endcsname{6.63}
\expandafter\def\csname v@cpu/student/selfl/aic_calls/wer\endcsname{18.03}
\expandafter\def\csname v@cpu/student/selfl/ali_test/dele\endcsname{9.28}
\expandafter\def\csname v@cpu/student/selfl/ali_test/dleak\endcsname{+0.95}
\expandafter\def\csname v@cpu/student/selfl/ali_test/dwer\endcsname{+0.45}
\expandafter\def\csname v@cpu/student/selfl/ali_test/dwer-hi\endcsname{+1.02}
\expandafter\def\csname v@cpu/student/selfl/ali_test/dwer-lo\endcsname{-0.09}
\expandafter\def\csname v@cpu/student/selfl/ali_test/ins\endcsname{1.17}
\expandafter\def\csname v@cpu/student/selfl/ali_test/leak_wpm\endcsname{1.96}
\expandafter\def\csname v@cpu/student/selfl/ali_test/miss\endcsname{14.66}
\expandafter\def\csname v@cpu/student/selfl/ali_test/wer\endcsname{15.82}
\expandafter\def\csname v@cpu/student/selfl/ami_dev/dele\endcsname{3.25}
\expandafter\def\csname v@cpu/student/selfl/ami_dev/dleak\endcsname{-1.07}
\expandafter\def\csname v@cpu/student/selfl/ami_dev/dwer\endcsname{-0.72}
\expandafter\def\csname v@cpu/student/selfl/ami_dev/dwer-hi\endcsname{+0.57}
\expandafter\def\csname v@cpu/student/selfl/ami_dev/dwer-lo\endcsname{-2.10}
\expandafter\def\csname v@cpu/student/selfl/ami_dev/ins\endcsname{4.38}
\expandafter\def\csname v@cpu/student/selfl/ami_dev/leak_wpm\endcsname{8.84}
\expandafter\def\csname v@cpu/student/selfl/ami_dev/miss\endcsname{9.24}
\expandafter\def\csname v@cpu/student/selfl/ami_dev/wer\endcsname{13.62}
\expandafter\def\csname v@cpu/student/selfl/ami_dev_long/dele\endcsname{7.17}
\expandafter\def\csname v@cpu/student/selfl/ami_dev_long/dleak\endcsname{-2.79}
\expandafter\def\csname v@cpu/student/selfl/ami_dev_long/dwer\endcsname{-8.51}
\expandafter\def\csname v@cpu/student/selfl/ami_dev_long/dwer-hi\endcsname{-4.90}
\expandafter\def\csname v@cpu/student/selfl/ami_dev_long/dwer-lo\endcsname{-12.09}
\expandafter\def\csname v@cpu/student/selfl/ami_dev_long/ins\endcsname{3.54}
\expandafter\def\csname v@cpu/student/selfl/ami_dev_long/leak_wpm\endcsname{6.65}
\expandafter\def\csname v@cpu/student/selfl/ami_dev_long/miss\endcsname{14.92}
\expandafter\def\csname v@cpu/student/selfl/ami_dev_long/wer\endcsname{18.45}
\expandafter\def\csname v@cpu/student/selfl/ami_headset2/dele\endcsname{3.35}
\expandafter\def\csname v@cpu/student/selfl/ami_headset2/dleak\endcsname{+0.40}
\expandafter\def\csname v@cpu/student/selfl/ami_headset2/dwer\endcsname{+0.97}
\expandafter\def\csname v@cpu/student/selfl/ami_headset2/dwer-hi\endcsname{+3.53}
\expandafter\def\csname v@cpu/student/selfl/ami_headset2/dwer-lo\endcsname{-0.58}
\expandafter\def\csname v@cpu/student/selfl/ami_headset2/ins\endcsname{3.32}
\expandafter\def\csname v@cpu/student/selfl/ami_headset2/leak_wpm\endcsname{2.52}
\expandafter\def\csname v@cpu/student/selfl/ami_headset2/miss\endcsname{7.91}
\expandafter\def\csname v@cpu/student/selfl/ami_headset2/wer\endcsname{11.23}
\expandafter\def\csname v@cpu/student/selfl/ami_test/dele\endcsname{2.94}
\expandafter\def\csname v@cpu/student/selfl/ami_test/dleak\endcsname{-0.85}
\expandafter\def\csname v@cpu/student/selfl/ami_test/dwer\endcsname{-0.02}
\expandafter\def\csname v@cpu/student/selfl/ami_test/dwer-hi\endcsname{+0.65}
\expandafter\def\csname v@cpu/student/selfl/ami_test/dwer-lo\endcsname{-0.85}
\expandafter\def\csname v@cpu/student/selfl/ami_test/ins\endcsname{2.40}
\expandafter\def\csname v@cpu/student/selfl/ami_test/leak_wpm\endcsname{1.29}
\expandafter\def\csname v@cpu/student/selfl/ami_test/miss\endcsname{7.89}
\expandafter\def\csname v@cpu/student/selfl/ami_test/wer\endcsname{10.29}
\expandafter\def\csname v@cpu/student/selfl/ami_test_long/dele\endcsname{6.89}
\expandafter\def\csname v@cpu/student/selfl/ami_test_long/dleak\endcsname{-2.39}
\expandafter\def\csname v@cpu/student/selfl/ami_test_long/dwer\endcsname{-4.64}
\expandafter\def\csname v@cpu/student/selfl/ami_test_long/dwer-hi\endcsname{-2.23}
\expandafter\def\csname v@cpu/student/selfl/ami_test_long/dwer-lo\endcsname{-7.62}
\expandafter\def\csname v@cpu/student/selfl/ami_test_long/ins\endcsname{3.51}
\expandafter\def\csname v@cpu/student/selfl/ami_test_long/leak_wpm\endcsname{3.08}
\expandafter\def\csname v@cpu/student/selfl/ami_test_long/miss\endcsname{12.04}
\expandafter\def\csname v@cpu/student/selfl/ami_test_long/wer\endcsname{15.55}
\expandafter\def\csname v@cpu/student/selfl/bge/ami_dev_long/b0\endcsname{-2}
\expandafter\def\csname v@cpu/student/selfl/bge/ami_dev_long/b1\endcsname{-3}
\expandafter\def\csname v@cpu/student/selfl/bge/ami_dev_long/b2\endcsname{-2}
\expandafter\def\csname v@cpu/student/selfl/bge/ami_dev_long/b3\endcsname{-2}
\expandafter\def\csname v@cpu/student/selfl/bge/ami_dev_long/b4\endcsname{-3}
\expandafter\def\csname v@cpu/student/selfl/bge/krisp/b0\endcsname{-19}
\expandafter\def\csname v@cpu/student/selfl/bge/krisp/b1\endcsname{-22}
\expandafter\def\csname v@cpu/student/selfl/bge/krisp/b2\endcsname{-31}
\expandafter\def\csname v@cpu/student/selfl/bge/krisp/b3\endcsname{-34}
\expandafter\def\csname v@cpu/student/selfl/bge/krisp/b4\endcsname{-26}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/ami_dev/diff\endcsname{+0.19}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/ami_dev/hi\endcsname{+0.76}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/ami_dev/lo\endcsname{-0.35}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/ami_dev_long/diff\endcsname{+1.23}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/ami_dev_long/hi\endcsname{+2.52}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/ami_dev_long/lo\endcsname{-0.05}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/call_dev_clean/diff\endcsname{-0.10}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/call_dev_clean/hi\endcsname{+0.52}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/call_dev_clean/lo\endcsname{-0.74}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/dev4/diff\endcsname{+0.33}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/dev4/hi\endcsname{+0.72}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/dev4/lo\endcsname{-0.06}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/nsf_dev/diff\endcsname{-0.01}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/nsf_dev/hi\endcsname{+0.12}
\expandafter\def\csname v@cpu/student/selfl/boot/C10n_ftlong_kd_selfl/nsf_dev/lo\endcsname{-0.14}
\expandafter\def\csname v@cpu/student/selfl/call_dev_clean/dele\endcsname{1.80}
\expandafter\def\csname v@cpu/student/selfl/call_dev_clean/dleak\endcsname{+nan}
\expandafter\def\csname v@cpu/student/selfl/call_dev_clean/dwer\endcsname{+0.96}
\expandafter\def\csname v@cpu/student/selfl/call_dev_clean/dwer-hi\endcsname{+2.15}
\expandafter\def\csname v@cpu/student/selfl/call_dev_clean/dwer-lo\endcsname{-0.22}
\expandafter\def\csname v@cpu/student/selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@cpu/student/selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@cpu/student/selfl/call_dev_clean/miss\endcsname{2.58}
\expandafter\def\csname v@cpu/student/selfl/call_dev_clean/wer\endcsname{2.84}
\expandafter\def\csname v@cpu/student/selfl/call_test_clean/dele\endcsname{2.04}
\expandafter\def\csname v@cpu/student/selfl/call_test_clean/dleak\endcsname{+nan}
\expandafter\def\csname v@cpu/student/selfl/call_test_clean/dwer\endcsname{+2.45}
\expandafter\def\csname v@cpu/student/selfl/call_test_clean/dwer-hi\endcsname{+3.63}
\expandafter\def\csname v@cpu/student/selfl/call_test_clean/dwer-lo\endcsname{+1.34}
\expandafter\def\csname v@cpu/student/selfl/call_test_clean/ins\endcsname{1.09}
\expandafter\def\csname v@cpu/student/selfl/call_test_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@cpu/student/selfl/call_test_clean/miss\endcsname{4.23}
\expandafter\def\csname v@cpu/student/selfl/call_test_clean/wer\endcsname{5.32}
\expandafter\def\csname v@cpu/student/selfl/call_test_mix/dele\endcsname{4.67}
\expandafter\def\csname v@cpu/student/selfl/call_test_mix/dleak\endcsname{-2.01}
\expandafter\def\csname v@cpu/student/selfl/call_test_mix/dwer\endcsname{+1.31}
\expandafter\def\csname v@cpu/student/selfl/call_test_mix/dwer-hi\endcsname{+6.74}
\expandafter\def\csname v@cpu/student/selfl/call_test_mix/dwer-lo\endcsname{-3.97}
\expandafter\def\csname v@cpu/student/selfl/call_test_mix/ins\endcsname{24.46}
\expandafter\def\csname v@cpu/student/selfl/call_test_mix/leak_wpm\endcsname{63.32}
\expandafter\def\csname v@cpu/student/selfl/call_test_mix/miss\endcsname{25.44}
\expandafter\def\csname v@cpu/student/selfl/call_test_mix/wer\endcsname{49.90}
\expandafter\def\csname v@cpu/student/selfl/dev4\endcsname{10.66}
\expandafter\def\csname v@cpu/student/selfl/krisp/dele\endcsname{1.37}
\expandafter\def\csname v@cpu/student/selfl/krisp/dleak\endcsname{-0.06}
\expandafter\def\csname v@cpu/student/selfl/krisp/dwer\endcsname{+0.67}
\expandafter\def\csname v@cpu/student/selfl/krisp/dwer-hi\endcsname{+1.27}
\expandafter\def\csname v@cpu/student/selfl/krisp/dwer-lo\endcsname{+0.12}
\expandafter\def\csname v@cpu/student/selfl/krisp/ins\endcsname{0.69}
\expandafter\def\csname v@cpu/student/selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@cpu/student/selfl/krisp/miss\endcsname{4.98}
\expandafter\def\csname v@cpu/student/selfl/krisp/wer\endcsname{5.66}
\expandafter\def\csname v@cpu/student/selfl/main/aic_calls/ins\endcsname{11.40}
\expandafter\def\csname v@cpu/student/selfl/main/aic_calls/leak\endcsname{13.25}
\expandafter\def\csname v@cpu/student/selfl/main/aic_calls/miss\endcsname{6.63}
\expandafter\def\csname v@cpu/student/selfl/main/aic_calls/wer\endcsname{18.03}
\expandafter\def\csname v@cpu/student/selfl/main/ali_test/ins\endcsname{1.17}
\expandafter\def\csname v@cpu/student/selfl/main/ali_test/leak\endcsname{1.96}
\expandafter\def\csname v@cpu/student/selfl/main/ali_test/miss\endcsname{14.66}
\expandafter\def\csname v@cpu/student/selfl/main/ali_test/wer\endcsname{15.82}
\expandafter\def\csname v@cpu/student/selfl/main/ami_headset2/ins\endcsname{3.32}
\expandafter\def\csname v@cpu/student/selfl/main/ami_headset2/leak\endcsname{2.52}
\expandafter\def\csname v@cpu/student/selfl/main/ami_headset2/miss\endcsname{7.91}
\expandafter\def\csname v@cpu/student/selfl/main/ami_headset2/wer\endcsname{11.23}
\expandafter\def\csname v@cpu/student/selfl/main/ami_test/ins\endcsname{2.40}
\expandafter\def\csname v@cpu/student/selfl/main/ami_test/leak\endcsname{1.29}
\expandafter\def\csname v@cpu/student/selfl/main/ami_test/miss\endcsname{7.89}
\expandafter\def\csname v@cpu/student/selfl/main/ami_test/wer\endcsname{10.29}
\expandafter\def\csname v@cpu/student/selfl/main/ami_test_long/ins\endcsname{3.51}
\expandafter\def\csname v@cpu/student/selfl/main/ami_test_long/leak\endcsname{3.08}
\expandafter\def\csname v@cpu/student/selfl/main/ami_test_long/miss\endcsname{12.04}
\expandafter\def\csname v@cpu/student/selfl/main/ami_test_long/wer\endcsname{15.55}
\expandafter\def\csname v@cpu/student/selfl/main/call_test_clean/ins\endcsname{1.09}
\expandafter\def\csname v@cpu/student/selfl/main/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@cpu/student/selfl/main/call_test_clean/miss\endcsname{4.23}
\expandafter\def\csname v@cpu/student/selfl/main/call_test_clean/wer\endcsname{5.32}
\expandafter\def\csname v@cpu/student/selfl/main/call_test_mix/ins\endcsname{24.46}
\expandafter\def\csname v@cpu/student/selfl/main/call_test_mix/leak\endcsname{63.32}
\expandafter\def\csname v@cpu/student/selfl/main/call_test_mix/miss\endcsname{25.44}
\expandafter\def\csname v@cpu/student/selfl/main/call_test_mix/wer\endcsname{49.90}
\expandafter\def\csname v@cpu/student/selfl/main/krisp/ins\endcsname{0.69}
\expandafter\def\csname v@cpu/student/selfl/main/krisp/leak\endcsname{0.04}
\expandafter\def\csname v@cpu/student/selfl/main/krisp/miss\endcsname{4.98}
\expandafter\def\csname v@cpu/student/selfl/main/krisp/wer\endcsname{5.66}
\expandafter\def\csname v@cpu/student/selfl/main/nsf_test/ins\endcsname{1.84}
\expandafter\def\csname v@cpu/student/selfl/main/nsf_test/leak\endcsname{0.55}
\expandafter\def\csname v@cpu/student/selfl/main/nsf_test/miss\endcsname{5.74}
\expandafter\def\csname v@cpu/student/selfl/main/nsf_test/wer\endcsname{7.58}
\expandafter\def\csname v@cpu/student/selfl/meet3\endcsname{13.26}
\expandafter\def\csname v@cpu/student/selfl/nsf_dev/dele\endcsname{1.47}
\expandafter\def\csname v@cpu/student/selfl/nsf_dev/dleak\endcsname{+0.00}
\expandafter\def\csname v@cpu/student/selfl/nsf_dev/dwer\endcsname{-0.58}
\expandafter\def\csname v@cpu/student/selfl/nsf_dev/dwer-hi\endcsname{+0.02}
\expandafter\def\csname v@cpu/student/selfl/nsf_dev/dwer-lo\endcsname{-1.50}
\expandafter\def\csname v@cpu/student/selfl/nsf_dev/ins\endcsname{1.97}
\expandafter\def\csname v@cpu/student/selfl/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@cpu/student/selfl/nsf_dev/miss\endcsname{5.73}
\expandafter\def\csname v@cpu/student/selfl/nsf_dev/wer\endcsname{7.70}
\expandafter\def\csname v@cpu/student/selfl/nsf_test/dele\endcsname{1.69}
\expandafter\def\csname v@cpu/student/selfl/nsf_test/dleak\endcsname{-0.47}
\expandafter\def\csname v@cpu/student/selfl/nsf_test/dwer\endcsname{-0.21}
\expandafter\def\csname v@cpu/student/selfl/nsf_test/dwer-hi\endcsname{+0.03}
\expandafter\def\csname v@cpu/student/selfl/nsf_test/dwer-lo\endcsname{-0.46}
\expandafter\def\csname v@cpu/student/selfl/nsf_test/ins\endcsname{1.84}
\expandafter\def\csname v@cpu/student/selfl/nsf_test/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@cpu/student/selfl/nsf_test/miss\endcsname{5.74}
\expandafter\def\csname v@cpu/student/selfl/nsf_test/wer\endcsname{7.58}
\expandafter\def\csname v@cpu/student/selfl/vad/aic_calls/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@cpu/student/selfl/vad/aic_calls/bg_speech\endcsname{18.1}
\expandafter\def\csname v@cpu/student/selfl/vad/aic_calls/bg_starts_per_min\endcsname{2.46}
\expandafter\def\csname v@cpu/student/selfl/vad/aic_calls/files\endcsname{83}
\expandafter\def\csname v@cpu/student/selfl/vad/aic_calls/starts_per_min\endcsname{12.83}
\expandafter\def\csname v@cpu/student/selfl/vad/ami_test/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@cpu/student/selfl/vad/ami_test/bg_speech\endcsname{11.4}
\expandafter\def\csname v@cpu/student/selfl/vad/ami_test/bg_starts_per_min\endcsname{1.50}
\expandafter\def\csname v@cpu/student/selfl/vad/ami_test/files\endcsname{599}
\expandafter\def\csname v@cpu/student/selfl/vad/ami_test/starts_per_min\endcsname{10.52}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/end_delay_p50\endcsname{-0.03}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/false\endcsname{0.1}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/false_starts_per_min\endcsname{0.03}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/files\endcsname{120}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/held\endcsname{61}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/held-pct\endcsname{8}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/minutes\endcsname{120.00}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/missed\endcsname{4.9}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_clean/turns\endcsname{805}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/end_delay_p90\endcsname{1.34}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/false\endcsname{26.2}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/false_starts_per_min\endcsname{2.27}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/files\endcsname{120}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/held\endcsname{162}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/held-pct\endcsname{20}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/minutes\endcsname{120.00}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/missed\endcsname{6.7}
\expandafter\def\csname v@cpu/student/selfl/vad/call_test_mix/turns\endcsname{805}
\expandafter\def\csname v@cpu/student/selfl/vad/krisp/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@cpu/student/selfl/vad/krisp/bg_speech\endcsname{0.4}
\expandafter\def\csname v@cpu/student/selfl/vad/krisp/bg_starts_per_min\endcsname{0.08}
\expandafter\def\csname v@cpu/student/selfl/vad/krisp/files\endcsname{265}
\expandafter\def\csname v@cpu/student/selfl/vad/krisp/starts_per_min\endcsname{4.20}
\expandafter\def\csname v@cpu/voxlock/fp32/core-pct\endcsname{160}
\expandafter\def\csname v@cpu/voxlock/fp32/core-per-call\endcsname{1.60}
\expandafter\def\csname v@cpu/voxlock/fp32/p99\endcsname{43}
\expandafter\def\csname v@cpu/voxlock/int8-full/core-pct\endcsname{91}
\expandafter\def\csname v@cpu/voxlock/int8-full/core-per-call\endcsname{0.91}
\expandafter\def\csname v@cpu/voxlock/int8-full/p99\endcsname{24}
\expandafter\def\csname v@cpu/voxlock/int8/core-pct\endcsname{138}
\expandafter\def\csname v@cpu/voxlock/int8/core-per-call\endcsname{1.38}
\expandafter\def\csname v@cpu/voxlock/int8/p99\endcsname{36}
\expandafter\def\csname v@data/bgdist-p10\endcsname{1.1}
\expandafter\def\csname v@data/bgdist-p90\endcsname{5.2}
\expandafter\def\csname v@data/bgonly-frac\endcsname{21}
\expandafter\def\csname v@data/bgonly-share\endcsname{71}
\expandafter\def\csname v@data/bible-hours\endcsname{363}
\expandafter\def\csname v@data/bible-langs\endcsname{6}
\expandafter\def\csname v@data/car-share\endcsname{3.3}
\expandafter\def\csname v@data/cv-hours\endcsname{1,025}
\expandafter\def\csname v@data/cv-langs\endcsname{131}
\expandafter\def\csname v@data/english-hours\endcsname{423}
\expandafter\def\csname v@data/enrolled-share\endcsname{70}
\expandafter\def\csname v@data/mls-hours\endcsname{704}
\expandafter\def\csname v@data/mls-langs\endcsname{7}
\expandafter\def\csname v@data/noise-clips\endcsname{20,946}
\expandafter\def\csname v@data/noise-hours\endcsname{51.3}
\expandafter\def\csname v@data/pool-hours\endcsname{2,761}
\expandafter\def\csname v@data/pool-utts\endcsname{1,218,365}
\expandafter\def\csname v@data/rooms\endcsname{20,000}
\expandafter\def\csname v@data/rt60-p10\endcsname{0.28}
\expandafter\def\csname v@data/rt60-p90\endcsname{0.97}
\expandafter\def\csname v@data/sir-p10\endcsname{-2.5}
\expandafter\def\csname v@data/sir-p50\endcsname{6.1}
\expandafter\def\csname v@data/snr-p50\endcsname{14.0}
\expandafter\def\csname v@data/train-hours\endcsname{2,746}
\expandafter\def\csname v@eval/aic_calls/bgmin\endcsname{15.8}
\expandafter\def\csname v@eval/aic_calls/callers\endcsname{4}
\expandafter\def\csname v@eval/aic_calls/minutes\endcsname{35}
\expandafter\def\csname v@eval/aic_calls/windows\endcsname{83}
\expandafter\def\csname v@eval/ami_dev/bgmin\endcsname{22.4}
\expandafter\def\csname v@eval/ami_dev/callers\endcsname{65}
\expandafter\def\csname v@eval/ami_dev/minutes\endcsname{67}
\expandafter\def\csname v@eval/ami_dev/windows\endcsname{400}
\expandafter\def\csname v@eval/ami_dev_long/bgmin\endcsname{62.0}
\expandafter\def\csname v@eval/ami_dev_long/callers\endcsname{50}
\expandafter\def\csname v@eval/ami_dev_long/minutes\endcsname{123}
\expandafter\def\csname v@eval/ami_dev_long/windows\endcsname{120}
\expandafter\def\csname v@eval/ami_headset2/bgmin\endcsname{7.5}
\expandafter\def\csname v@eval/ami_headset2/callers\endcsname{19}
\expandafter\def\csname v@eval/ami_headset2/minutes\endcsname{26}
\expandafter\def\csname v@eval/ami_headset2/windows\endcsname{134}
\expandafter\def\csname v@eval/ami_test/bgmin\endcsname{34.2}
\expandafter\def\csname v@eval/ami_test/callers\endcsname{61}
\expandafter\def\csname v@eval/ami_test/minutes\endcsname{109}
\expandafter\def\csname v@eval/ami_test/windows\endcsname{599}
\expandafter\def\csname v@eval/ami_test_long/bgmin\endcsname{63.2}
\expandafter\def\csname v@eval/ami_test_long/callers\endcsname{44}
\expandafter\def\csname v@eval/ami_test_long/minutes\endcsname{124}
\expandafter\def\csname v@eval/ami_test_long/windows\endcsname{120}
\expandafter\def\csname v@eval/call_dev_clean/bgmin\endcsname{0.0}
\expandafter\def\csname v@eval/call_dev_clean/callers\endcsname{120}
\expandafter\def\csname v@eval/call_dev_clean/minutes\endcsname{120}
\expandafter\def\csname v@eval/call_dev_clean/windows\endcsname{120}
\expandafter\def\csname v@eval/call_dev_mix/bgmin\endcsname{4.9}
\expandafter\def\csname v@eval/call_dev_mix/callers\endcsname{120}
\expandafter\def\csname v@eval/call_dev_mix/minutes\endcsname{120}
\expandafter\def\csname v@eval/call_dev_mix/windows\endcsname{120}
\expandafter\def\csname v@eval/call_test_clean/bgmin\endcsname{0.0}
\expandafter\def\csname v@eval/call_test_clean/callers\endcsname{120}
\expandafter\def\csname v@eval/call_test_clean/minutes\endcsname{120}
\expandafter\def\csname v@eval/call_test_clean/windows\endcsname{120}
\expandafter\def\csname v@eval/call_test_mix/bgmin\endcsname{19.4}
\expandafter\def\csname v@eval/call_test_mix/callers\endcsname{120}
\expandafter\def\csname v@eval/call_test_mix/minutes\endcsname{120}
\expandafter\def\csname v@eval/call_test_mix/windows\endcsname{120}
\expandafter\def\csname v@eval/krisp/bgmin\endcsname{85.3}
\expandafter\def\csname v@eval/krisp/callers\endcsname{47}
\expandafter\def\csname v@eval/krisp/minutes\endcsname{337}
\expandafter\def\csname v@eval/krisp/windows\endcsname{265}
\expandafter\def\csname v@eval/nsf_dev/bgmin\endcsname{23.5}
\expandafter\def\csname v@eval/nsf_dev/callers\endcsname{156}
\expandafter\def\csname v@eval/nsf_dev/minutes\endcsname{69}
\expandafter\def\csname v@eval/nsf_dev/windows\endcsname{400}
\expandafter\def\csname v@eval/nsf_test/bgmin\endcsname{47.2}
\expandafter\def\csname v@eval/nsf_test/callers\endcsname{413}
\expandafter\def\csname v@eval/nsf_test/minutes\endcsname{140}
\expandafter\def\csname v@eval/nsf_test/windows\endcsname{800}
\expandafter\def\csname v@eval/simcall60/bgmin\endcsname{10.6}
\expandafter\def\csname v@eval/simcall60/callers\endcsname{40}
\expandafter\def\csname v@eval/simcall60/minutes\endcsname{200}
\expandafter\def\csname v@eval/simcall60/windows\endcsname{200}
\expandafter\def\csname v@evalbg/aic_calls/maxlen\endcsname{22.1}
\expandafter\def\csname v@evalbg/aic_calls/median\endcsname{1.8}
\expandafter\def\csname v@evalbg/aic_calls/over4\endcsname{50}
\expandafter\def\csname v@evalbg/aic_calls/over8\endcsname{28}
\expandafter\def\csname v@evalbg/ali_test/maxlen\endcsname{3.8}
\expandafter\def\csname v@evalbg/ali_test/median\endcsname{3.8}
\expandafter\def\csname v@evalbg/ali_test/over4\endcsname{0}
\expandafter\def\csname v@evalbg/ali_test/over8\endcsname{0}
\expandafter\def\csname v@evalbg/ami_dev/maxlen\endcsname{3.8}
\expandafter\def\csname v@evalbg/ami_dev/median\endcsname{3.8}
\expandafter\def\csname v@evalbg/ami_dev/over4\endcsname{0}
\expandafter\def\csname v@evalbg/ami_dev/over8\endcsname{0}
\expandafter\def\csname v@evalbg/ami_dev_long/maxlen\endcsname{40.3}
\expandafter\def\csname v@evalbg/ami_dev_long/median\endcsname{3.2}
\expandafter\def\csname v@evalbg/ami_dev_long/over4\endcsname{85}
\expandafter\def\csname v@evalbg/ami_dev_long/over8\endcsname{68}
\expandafter\def\csname v@evalbg/ami_headset2/maxlen\endcsname{3.8}
\expandafter\def\csname v@evalbg/ami_headset2/median\endcsname{3.6}
\expandafter\def\csname v@evalbg/ami_headset2/over4\endcsname{0}
\expandafter\def\csname v@evalbg/ami_headset2/over8\endcsname{0}
\expandafter\def\csname v@evalbg/ami_test/maxlen\endcsname{3.8}
\expandafter\def\csname v@evalbg/ami_test/median\endcsname{3.8}
\expandafter\def\csname v@evalbg/ami_test/over4\endcsname{0}
\expandafter\def\csname v@evalbg/ami_test/over8\endcsname{0}
\expandafter\def\csname v@evalbg/ami_test_long/maxlen\endcsname{38.0}
\expandafter\def\csname v@evalbg/ami_test_long/median\endcsname{3.4}
\expandafter\def\csname v@evalbg/ami_test_long/over4\endcsname{86}
\expandafter\def\csname v@evalbg/ami_test_long/over8\endcsname{68}
\expandafter\def\csname v@evalbg/call_dev_mix/maxlen\endcsname{18.6}
\expandafter\def\csname v@evalbg/call_dev_mix/median\endcsname{1.2}
\expandafter\def\csname v@evalbg/call_dev_mix/over4\endcsname{52}
\expandafter\def\csname v@evalbg/call_dev_mix/over8\endcsname{24}
\expandafter\def\csname v@evalbg/call_test_mix/maxlen\endcsname{16.9}
\expandafter\def\csname v@evalbg/call_test_mix/median\endcsname{2.4}
\expandafter\def\csname v@evalbg/call_test_mix/over4\endcsname{63}
\expandafter\def\csname v@evalbg/call_test_mix/over8\endcsname{22}
\expandafter\def\csname v@evalbg/krisp/maxlen\endcsname{57.8}
\expandafter\def\csname v@evalbg/krisp/median\endcsname{16.9}
\expandafter\def\csname v@evalbg/krisp/over4\endcsname{98}
\expandafter\def\csname v@evalbg/krisp/over8\endcsname{94}
\expandafter\def\csname v@evalbg/nsf_dev/maxlen\endcsname{3.8}
\expandafter\def\csname v@evalbg/nsf_dev/median\endcsname{3.8}
\expandafter\def\csname v@evalbg/nsf_dev/over4\endcsname{0}
\expandafter\def\csname v@evalbg/nsf_dev/over8\endcsname{0}
\expandafter\def\csname v@evalbg/nsf_test/maxlen\endcsname{3.8}
\expandafter\def\csname v@evalbg/nsf_test/median\endcsname{3.8}
\expandafter\def\csname v@evalbg/nsf_test/over4\endcsname{0}
\expandafter\def\csname v@evalbg/nsf_test/over8\endcsname{0}
\expandafter\def\csname v@iw/inworld/aic_calls/leak\endcsname{77.6}
\expandafter\def\csname v@iw/inworld/aic_calls/wer\endcsname{60.94}
\expandafter\def\csname v@iw/inworld/ali_test/leak\endcsname{15.3}
\expandafter\def\csname v@iw/inworld/ali_test/wer\endcsname{18.03}
\expandafter\def\csname v@iw/inworld/ami_headset2/leak\endcsname{25.6}
\expandafter\def\csname v@iw/inworld/ami_headset2/wer\endcsname{17.80}
\expandafter\def\csname v@iw/inworld/ami_test/leak\endcsname{72.0}
\expandafter\def\csname v@iw/inworld/ami_test/wer\endcsname{30.28}
\expandafter\def\csname v@iw/inworld/ami_test_long/leak\endcsname{113.7}
\expandafter\def\csname v@iw/inworld/ami_test_long/wer\endcsname{99.21}
\expandafter\def\csname v@iw/inworld/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@iw/inworld/call_test_clean/wer\endcsname{2.63}
\expandafter\def\csname v@iw/inworld/call_test_mix/leak\endcsname{113.4}
\expandafter\def\csname v@iw/inworld/call_test_mix/wer\endcsname{68.28}
\expandafter\def\csname v@iw/inworld/krisp/leak\endcsname{63.8}
\expandafter\def\csname v@iw/inworld/krisp/wer\endcsname{22.31}
\expandafter\def\csname v@iw/inworld/nsf_test/leak\endcsname{43.2}
\expandafter\def\csname v@iw/inworld/nsf_test/wer\endcsname{19.90}
\expandafter\def\csname v@iw/inworld_rt/aic_calls/leak\endcsname{77.3}
\expandafter\def\csname v@iw/inworld_rt/aic_calls/wer\endcsname{60.69}
\expandafter\def\csname v@iw/inworld_rt/ali_test/leak\endcsname{18.5}
\expandafter\def\csname v@iw/inworld_rt/ali_test/wer\endcsname{18.94}
\expandafter\def\csname v@iw/inworld_rt/ami_headset2/leak\endcsname{35.4}
\expandafter\def\csname v@iw/inworld_rt/ami_headset2/wer\endcsname{21.39}
\expandafter\def\csname v@iw/inworld_rt/ami_test/leak\endcsname{71.2}
\expandafter\def\csname v@iw/inworld_rt/ami_test/wer\endcsname{30.06}
\expandafter\def\csname v@iw/inworld_rt/ami_test_long/leak\endcsname{118.5}
\expandafter\def\csname v@iw/inworld_rt/ami_test_long/wer\endcsname{102.51}
\expandafter\def\csname v@iw/inworld_rt/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@iw/inworld_rt/call_test_clean/wer\endcsname{2.07}
\expandafter\def\csname v@iw/inworld_rt/call_test_mix/leak\endcsname{114.7}
\expandafter\def\csname v@iw/inworld_rt/call_test_mix/wer\endcsname{69.02}
\expandafter\def\csname v@iw/inworld_rt/krisp/leak\endcsname{64.2}
\expandafter\def\csname v@iw/inworld_rt/krisp/wer\endcsname{22.24}
\expandafter\def\csname v@iw/inworld_rt/nsf_test/leak\endcsname{52.1}
\expandafter\def\csname v@iw/inworld_rt/nsf_test/wer\endcsname{22.41}
\expandafter\def\csname v@kern/agree-db\endcsname{69}
\expandafter\def\csname v@kern/attn/ff/2/new\endcsname{0.10}
\expandafter\def\csname v@kern/attn/ff/2/old\endcsname{0.39}
\expandafter\def\csname v@kern/attn/ff/2/x\endcsname{3.8}
\expandafter\def\csname v@kern/attn/ff/4/new\endcsname{0.10}
\expandafter\def\csname v@kern/attn/ff/4/old\endcsname{0.40}
\expandafter\def\csname v@kern/attn/ff/4/x\endcsname{3.9}
\expandafter\def\csname v@kern/attn/wl/1/new\endcsname{0.07}
\expandafter\def\csname v@kern/attn/wl/1/old\endcsname{0.15}
\expandafter\def\csname v@kern/attn/wl/1/x\endcsname{2.1}
\expandafter\def\csname v@kern/attn/wl/2/new\endcsname{0.08}
\expandafter\def\csname v@kern/attn/wl/2/old\endcsname{0.27}
\expandafter\def\csname v@kern/attn/wl/2/x\endcsname{3.4}
\expandafter\def\csname v@kern/lstm/2/new\endcsname{0.10}
\expandafter\def\csname v@kern/lstm/2/old\endcsname{1.06}
\expandafter\def\csname v@kern/lstm/2/x\endcsname{11}
\expandafter\def\csname v@kern/lstm/4/new\endcsname{0.15}
\expandafter\def\csname v@kern/lstm/4/old\endcsname{1.14}
\expandafter\def\csname v@kern/lstm/4/x\endcsname{7}
\expandafter\def\csname v@kern/step/2/cut\endcsname{38}
\expandafter\def\csname v@kern/step/2/new\endcsname{11.6}
\expandafter\def\csname v@kern/step/2/old\endcsname{18.8}
\expandafter\def\csname v@kern/step/4/cut\endcsname{42}
\expandafter\def\csname v@kern/step/4/new\endcsname{13.5}
\expandafter\def\csname v@kern/step/4/old\endcsname{23.4}
\expandafter\def\csname v@krisp/C22_ftlong_kd_selfl/dele\endcsname{1.37}
\expandafter\def\csname v@krisp/C22_ftlong_kd_selfl/dleak\endcsname{-0.06}
\expandafter\def\csname v@krisp/C22_ftlong_kd_selfl/dwer\endcsname{+0.67}
\expandafter\def\csname v@krisp/C22_ftlong_kd_selfl/dwer-hi\endcsname{+1.27}
\expandafter\def\csname v@krisp/C22_ftlong_kd_selfl/dwer-lo\endcsname{+0.12}
\expandafter\def\csname v@krisp/C22_ftlong_kd_selfl/ins\endcsname{0.69}
\expandafter\def\csname v@krisp/C22_ftlong_kd_selfl/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@krisp/C22_ftlong_kd_selfl/miss\endcsname{4.98}
\expandafter\def\csname v@krisp/C22_ftlong_kd_selfl/wer\endcsname{5.66}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/dele\endcsname{1.75}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/dleak\endcsname{-0.05}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/dnsmos\endcsname{3.75}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/dwer\endcsname{+0.93}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/dwer-hi\endcsname{+1.88}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/dwer-lo\endcsname{+0.27}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/ins\endcsname{0.67}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/leak_wpm\endcsname{0.05}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/miss\endcsname{5.26}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_loud/wer\endcsname{5.93}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_null/dele\endcsname{1.59}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{+1.71}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{+1.28}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+2.38}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{+0.41}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_null/ins\endcsname{1.14}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{1.80}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_null/miss\endcsname{5.14}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_null/wer\endcsname{6.28}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{1.57}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-0.06}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{+0.75}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+1.71}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{+0.12}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{0.67}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{5.08}
\expandafter\def\csname v@krisp/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{5.74}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/dele\endcsname{1.26}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/dleak\endcsname{+0.39}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/dnsmos\endcsname{3.77}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/dwer\endcsname{+0.77}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/dwer-hi\endcsname{+1.23}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/dwer-lo\endcsname{+0.36}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/ins\endcsname{0.84}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/leak_wpm\endcsname{0.48}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/miss\endcsname{4.92}
\expandafter\def\csname v@krisp/MB_ftlong_ws_loud/wer\endcsname{5.76}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/dele\endcsname{1.52}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/dleak\endcsname{+2.62}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/dnsmos\endcsname{3.73}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/dwer\endcsname{+1.56}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/dwer-hi\endcsname{+2.13}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/dwer-lo\endcsname{+0.95}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/ins\endcsname{1.43}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/leak_wpm\endcsname{2.72}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/miss\endcsname{5.12}
\expandafter\def\csname v@krisp/MB_ftlong_ws_null/wer\endcsname{6.55}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/dele\endcsname{1.39}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/dleak\endcsname{+0.12}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/dnsmos\endcsname{3.77}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/dwer\endcsname{+0.79}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/dwer-hi\endcsname{+1.37}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/dwer-lo\endcsname{+0.31}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/ins\endcsname{0.73}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/leak_wpm\endcsname{0.21}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/miss\endcsname{5.05}
\expandafter\def\csname v@krisp/MB_ftlong_ws_selfl/wer\endcsname{5.79}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/dele\endcsname{1.54}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/dleak\endcsname{+0.02}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/dnsmos\endcsname{3.72}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/dwer\endcsname{+1.13}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/dwer-hi\endcsname{+1.91}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/dwer-lo\endcsname{+0.57}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/ins\endcsname{0.73}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/leak_wpm\endcsname{0.12}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/miss\endcsname{5.40}
\expandafter\def\csname v@krisp/SB_ftlong_ws_selfl/wer\endcsname{6.12}
\expandafter\def\csname v@krisp/dfn3/dele\endcsname{3.26}
\expandafter\def\csname v@krisp/dfn3/dleak\endcsname{+20.25}
\expandafter\def\csname v@krisp/dfn3/dnsmos\endcsname{4.06}
\expandafter\def\csname v@krisp/dfn3/dwer\endcsname{+8.15}
\expandafter\def\csname v@krisp/dfn3/dwer-hi\endcsname{+10.23}
\expandafter\def\csname v@krisp/dfn3/dwer-lo\endcsname{+5.73}
\expandafter\def\csname v@krisp/dfn3/ins\endcsname{6.18}
\expandafter\def\csname v@krisp/dfn3/leak_wpm\endcsname{20.34}
\expandafter\def\csname v@krisp/dfn3/miss\endcsname{6.96}
\expandafter\def\csname v@krisp/dfn3/wer\endcsname{13.15}
\expandafter\def\csname v@krisp/krisp_balanced/dele\endcsname{0.91}
\expandafter\def\csname v@krisp/krisp_balanced/dleak\endcsname{+1.92}
\expandafter\def\csname v@krisp/krisp_balanced/dwer\endcsname{+0.32}
\expandafter\def\csname v@krisp/krisp_balanced/dwer-hi\endcsname{+0.90}
\expandafter\def\csname v@krisp/krisp_balanced/dwer-lo\endcsname{-0.31}
\expandafter\def\csname v@krisp/krisp_balanced/ins\endcsname{1.26}
\expandafter\def\csname v@krisp/krisp_balanced/leak_wpm\endcsname{2.02}
\expandafter\def\csname v@krisp/krisp_balanced/miss\endcsname{4.06}
\expandafter\def\csname v@krisp/krisp_balanced/wer\endcsname{5.32}
\expandafter\def\csname v@krisp/krisp_default/dele\endcsname{0.89}
\expandafter\def\csname v@krisp/krisp_default/dleak\endcsname{+1.43}
\expandafter\def\csname v@krisp/krisp_default/dnsmos\endcsname{3.92}
\expandafter\def\csname v@krisp/krisp_default/dwer\endcsname{+0.31}
\expandafter\def\csname v@krisp/krisp_default/dwer-hi\endcsname{+0.93}
\expandafter\def\csname v@krisp/krisp_default/dwer-lo\endcsname{-0.27}
\expandafter\def\csname v@krisp/krisp_default/ins\endcsname{1.09}
\expandafter\def\csname v@krisp/krisp_default/leak_wpm\endcsname{1.52}
\expandafter\def\csname v@krisp/krisp_default/miss\endcsname{4.21}
\expandafter\def\csname v@krisp/krisp_default/wer\endcsname{5.30}
\expandafter\def\csname v@krisp/krisp_hd/dele\endcsname{0.95}
\expandafter\def\csname v@krisp/krisp_hd/dleak\endcsname{+2.65}
\expandafter\def\csname v@krisp/krisp_hd/dnsmos\endcsname{4.00}
\expandafter\def\csname v@krisp/krisp_hd/dwer\endcsname{+0.79}
\expandafter\def\csname v@krisp/krisp_hd/dwer-hi\endcsname{+1.77}
\expandafter\def\csname v@krisp/krisp_hd/dwer-lo\endcsname{-0.09}
\expandafter\def\csname v@krisp/krisp_hd/ins\endcsname{1.42}
\expandafter\def\csname v@krisp/krisp_hd/leak_wpm\endcsname{2.74}
\expandafter\def\csname v@krisp/krisp_hd/miss\endcsname{4.36}
\expandafter\def\csname v@krisp/krisp_hd/wer\endcsname{5.79}
\expandafter\def\csname v@krisp/krisp_lite/dele\endcsname{0.95}
\expandafter\def\csname v@krisp/krisp_lite/dleak\endcsname{+4.43}
\expandafter\def\csname v@krisp/krisp_lite/dwer\endcsname{+1.21}
\expandafter\def\csname v@krisp/krisp_lite/dwer-hi\endcsname{+2.03}
\expandafter\def\csname v@krisp/krisp_lite/dwer-lo\endcsname{+0.23}
\expandafter\def\csname v@krisp/krisp_lite/ins\endcsname{1.94}
\expandafter\def\csname v@krisp/krisp_lite/leak_wpm\endcsname{4.52}
\expandafter\def\csname v@krisp/krisp_lite/miss\endcsname{4.26}
\expandafter\def\csname v@krisp/krisp_lite/wer\endcsname{6.21}
\expandafter\def\csname v@krisp/raw/dele\endcsname{1.01}
\expandafter\def\csname v@krisp/raw/dleak\endcsname{+66.34}
\expandafter\def\csname v@krisp/raw/dnsmos\endcsname{3.59}
\expandafter\def\csname v@krisp/raw/dwer\endcsname{+18.20}
\expandafter\def\csname v@krisp/raw/dwer-hi\endcsname{+20.70}
\expandafter\def\csname v@krisp/raw/dwer-lo\endcsname{+15.50}
\expandafter\def\csname v@krisp/raw/ins\endcsname{18.92}
\expandafter\def\csname v@krisp/raw/leak_wpm\endcsname{66.44}
\expandafter\def\csname v@krisp/raw/miss\endcsname{4.27}
\expandafter\def\csname v@krisp/raw/wer\endcsname{23.19}
\expandafter\def\csname v@krisp/sidon_v2/dele\endcsname{0.71}
\expandafter\def\csname v@krisp/sidon_v2/dleak\endcsname{+103.31}
\expandafter\def\csname v@krisp/sidon_v2/dnsmos\endcsname{4.00}
\expandafter\def\csname v@krisp/sidon_v2/dwer\endcsname{+28.51}
\expandafter\def\csname v@krisp/sidon_v2/dwer-hi\endcsname{+31.76}
\expandafter\def\csname v@krisp/sidon_v2/dwer-lo\endcsname{+24.24}
\expandafter\def\csname v@krisp/sidon_v2/ins\endcsname{29.41}
\expandafter\def\csname v@krisp/sidon_v2/leak_wpm\endcsname{103.40}
\expandafter\def\csname v@krisp/sidon_v2/miss\endcsname{4.09}
\expandafter\def\csname v@krisp/sidon_v2/wer\endcsname{33.50}
\expandafter\def\csname v@krisp/sidon_vi/dele\endcsname{0.76}
\expandafter\def\csname v@krisp/sidon_vi/dleak\endcsname{+90.92}
\expandafter\def\csname v@krisp/sidon_vi/dnsmos\endcsname{4.08}
\expandafter\def\csname v@krisp/sidon_vi/dwer\endcsname{+24.50}
\expandafter\def\csname v@krisp/sidon_vi/dwer-hi\endcsname{+27.17}
\expandafter\def\csname v@krisp/sidon_vi/dwer-lo\endcsname{+20.93}
\expandafter\def\csname v@krisp/sidon_vi/ins\endcsname{25.45}
\expandafter\def\csname v@krisp/sidon_vi/leak_wpm\endcsname{91.02}
\expandafter\def\csname v@krisp/sidon_vi/miss\endcsname{4.04}
\expandafter\def\csname v@krisp/sidon_vi/wer\endcsname{29.49}
\expandafter\def\csname v@krisp/sidon_vi_lite/dele\endcsname{1.42}
\expandafter\def\csname v@krisp/sidon_vi_lite/dleak\endcsname{+42.40}
\expandafter\def\csname v@krisp/sidon_vi_lite/dnsmos\endcsname{4.00}
\expandafter\def\csname v@krisp/sidon_vi_lite/dwer\endcsname{+13.28}
\expandafter\def\csname v@krisp/sidon_vi_lite/dwer-hi\endcsname{+15.36}
\expandafter\def\csname v@krisp/sidon_vi_lite/dwer-lo\endcsname{+10.77}
\expandafter\def\csname v@krisp/sidon_vi_lite/ins\endcsname{12.05}
\expandafter\def\csname v@krisp/sidon_vi_lite/leak_wpm\endcsname{42.50}
\expandafter\def\csname v@krisp/sidon_vi_lite/miss\endcsname{6.22}
\expandafter\def\csname v@krisp/sidon_vi_lite/wer\endcsname{18.27}
\expandafter\def\csname v@krisp/voxlock/dele\endcsname{1.07}
\expandafter\def\csname v@krisp/voxlock/dleak\endcsname{-0.02}
\expandafter\def\csname v@krisp/voxlock/dnsmos\endcsname{3.95}
\expandafter\def\csname v@krisp/voxlock/dwer\endcsname{+0.20}
\expandafter\def\csname v@krisp/voxlock/dwer-hi\endcsname{+0.39}
\expandafter\def\csname v@krisp/voxlock/dwer-lo\endcsname{+0.01}
\expandafter\def\csname v@krisp/voxlock/ins\endcsname{0.72}
\expandafter\def\csname v@krisp/voxlock/leak_wpm\endcsname{0.07}
\expandafter\def\csname v@krisp/voxlock/miss\endcsname{4.46}
\expandafter\def\csname v@krisp/voxlock/wer\endcsname{5.19}
\expandafter\def\csname v@krisp/voxlock_live/dele\endcsname{1.23}
\expandafter\def\csname v@krisp/voxlock_live/dleak\endcsname{+0.20}
\expandafter\def\csname v@krisp/voxlock_live/dnsmos\endcsname{3.91}
\expandafter\def\csname v@krisp/voxlock_live/dwer\endcsname{+0.63}
\expandafter\def\csname v@krisp/voxlock_live/dwer-hi\endcsname{+1.31}
\expandafter\def\csname v@krisp/voxlock_live/dwer-lo\endcsname{+0.21}
\expandafter\def\csname v@krisp/voxlock_live/ins\endcsname{0.84}
\expandafter\def\csname v@krisp/voxlock_live/leak_wpm\endcsname{0.29}
\expandafter\def\csname v@krisp/voxlock_live/miss\endcsname{4.78}
\expandafter\def\csname v@krisp/voxlock_live/wer\endcsname{5.63}
\expandafter\def\csname v@krisp/voxlock_pt/dele\endcsname{0.94}
\expandafter\def\csname v@krisp/voxlock_pt/dnsmos\endcsname{3.91}
\expandafter\def\csname v@krisp/voxlock_pt/ins\endcsname{0.74}
\expandafter\def\csname v@krisp/voxlock_pt/leak_wpm\endcsname{0.09}
\expandafter\def\csname v@krisp/voxlock_pt/miss\endcsname{4.25}
\expandafter\def\csname v@krisp/voxlock_pt/wer\endcsname{4.99}
\expandafter\def\csname v@lk/final/gtcrn/caller_missed_pct\endcsname{0.7}
\expandafter\def\csname v@lk/final/gtcrn/calls\endcsname{32}
\expandafter\def\csname v@lk/final/gtcrn/delay_ms_max\endcsname{0}
\expandafter\def\csname v@lk/final/gtcrn/delay_ms_p50\endcsname{0}
\expandafter\def\csname v@lk/final/gtcrn/delay_ms_p99\endcsname{0}
\expandafter\def\csname v@lk/final/gtcrn/drift_s_p99\endcsname{0.038}
\expandafter\def\csname v@lk/final/gtcrn/false_starts_per_min\endcsname{2.88}
\expandafter\def\csname v@lk/final/gtcrn/filter_core_pct\endcsname{7}
\expandafter\def\csname v@lk/final/gtcrn/filter_core_per_call\endcsname{0.066}
\expandafter\def\csname v@lk/final/gtcrn/frame_ms_max\endcsname{25.93}
\expandafter\def\csname v@lk/final/gtcrn/frame_ms_p50\endcsname{3.05}
\expandafter\def\csname v@lk/final/gtcrn/frame_ms_p99\endcsname{5.58}
\expandafter\def\csname v@lk/final/gtcrn/held_pct\endcsname{22}
\expandafter\def\csname v@lk/final/gtcrn/job_core_per_call\endcsname{0.092}
\expandafter\def\csname v@lk/final/gtcrn/join_s_max\endcsname{26}
\expandafter\def\csname v@lk/final/gtcrn/join_s_p50\endcsname{25}
\expandafter\def\csname v@lk/final/gtcrn/pauses_heard_pct\endcsname{46.8}
\expandafter\def\csname v@lk/final/gtcrn/turn_end_p90_s\endcsname{2.03}
\expandafter\def\csname v@lk/final/gtcrn/turns\endcsname{239}
\expandafter\def\csname v@lk/final/gtcrn/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/final/local-int8/caller_missed_pct\endcsname{2.9}
\expandafter\def\csname v@lk/final/local-int8/calls\endcsname{32}
\expandafter\def\csname v@lk/final/local-int8/delay_ms_max\endcsname{10}
\expandafter\def\csname v@lk/final/local-int8/delay_ms_p50\endcsname{10}
\expandafter\def\csname v@lk/final/local-int8/delay_ms_p99\endcsname{10}
\expandafter\def\csname v@lk/final/local-int8/drift_s_p99\endcsname{0.061}
\expandafter\def\csname v@lk/final/local-int8/false_starts_per_min\endcsname{2.25}
\expandafter\def\csname v@lk/final/local-int8/filter_core_pct\endcsname{20}
\expandafter\def\csname v@lk/final/local-int8/filter_core_per_call\endcsname{0.200}
\expandafter\def\csname v@lk/final/local-int8/frame_ms_max\endcsname{50.87}
\expandafter\def\csname v@lk/final/local-int8/frame_ms_p50\endcsname{9.49}
\expandafter\def\csname v@lk/final/local-int8/frame_ms_p99\endcsname{16.66}
\expandafter\def\csname v@lk/final/local-int8/held_pct\endcsname{16}
\expandafter\def\csname v@lk/final/local-int8/job_core_per_call\endcsname{0.160}
\expandafter\def\csname v@lk/final/local-int8/join_s_max\endcsname{41}
\expandafter\def\csname v@lk/final/local-int8/join_s_p50\endcsname{39}
\expandafter\def\csname v@lk/final/local-int8/pauses_heard_pct\endcsname{28.2}
\expandafter\def\csname v@lk/final/local-int8/turn_end_p90_s\endcsname{1.04}
\expandafter\def\csname v@lk/final/local-int8/turns\endcsname{239}
\expandafter\def\csname v@lk/final/local-int8/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/final/local/caller_missed_pct\endcsname{3.0}
\expandafter\def\csname v@lk/final/local/calls\endcsname{32}
\expandafter\def\csname v@lk/final/local/delay_ms_max\endcsname{10}
\expandafter\def\csname v@lk/final/local/delay_ms_p50\endcsname{10}
\expandafter\def\csname v@lk/final/local/delay_ms_p99\endcsname{10}
\expandafter\def\csname v@lk/final/local/drift_s_p99\endcsname{0.066}
\expandafter\def\csname v@lk/final/local/false_starts_per_min\endcsname{2.12}
\expandafter\def\csname v@lk/final/local/filter_core_pct\endcsname{32}
\expandafter\def\csname v@lk/final/local/filter_core_per_call\endcsname{0.323}
\expandafter\def\csname v@lk/final/local/frame_ms_max\endcsname{59.11}
\expandafter\def\csname v@lk/final/local/frame_ms_p50\endcsname{15.21}
\expandafter\def\csname v@lk/final/local/frame_ms_p99\endcsname{24.88}
\expandafter\def\csname v@lk/final/local/held_pct\endcsname{18}
\expandafter\def\csname v@lk/final/local/job_core_per_call\endcsname{0.209}
\expandafter\def\csname v@lk/final/local/join_s_max\endcsname{38}
\expandafter\def\csname v@lk/final/local/join_s_p50\endcsname{36}
\expandafter\def\csname v@lk/final/local/pauses_heard_pct\endcsname{27.7}
\expandafter\def\csname v@lk/final/local/turn_end_p90_s\endcsname{1.03}
\expandafter\def\csname v@lk/final/local/turns\endcsname{239}
\expandafter\def\csname v@lk/final/local/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/final/none/caller_missed_pct\endcsname{0.3}
\expandafter\def\csname v@lk/final/none/calls\endcsname{32}
\expandafter\def\csname v@lk/final/none/delay_ms_max\endcsname{0}
\expandafter\def\csname v@lk/final/none/delay_ms_p50\endcsname{0}
\expandafter\def\csname v@lk/final/none/delay_ms_p99\endcsname{0}
\expandafter\def\csname v@lk/final/none/drift_s_p99\endcsname{0.016}
\expandafter\def\csname v@lk/final/none/false_starts_per_min\endcsname{2.84}
\expandafter\def\csname v@lk/final/none/filter_core_pct\endcsname{0}
\expandafter\def\csname v@lk/final/none/filter_core_per_call\endcsname{0.000}
\expandafter\def\csname v@lk/final/none/frame_ms_max\endcsname{0.04}
\expandafter\def\csname v@lk/final/none/frame_ms_p50\endcsname{0.00}
\expandafter\def\csname v@lk/final/none/frame_ms_p99\endcsname{0.00}
\expandafter\def\csname v@lk/final/none/held_pct\endcsname{23}
\expandafter\def\csname v@lk/final/none/job_core_per_call\endcsname{0.065}
\expandafter\def\csname v@lk/final/none/join_s_max\endcsname{25}
\expandafter\def\csname v@lk/final/none/join_s_p50\endcsname{24}
\expandafter\def\csname v@lk/final/none/pauses_heard_pct\endcsname{47.5}
\expandafter\def\csname v@lk/final/none/turn_end_p90_s\endcsname{2.04}
\expandafter\def\csname v@lk/final/none/turns\endcsname{239}
\expandafter\def\csname v@lk/final/none/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/final/remote-f20/caller_missed_pct\endcsname{6.8}
\expandafter\def\csname v@lk/final/remote-f20/calls\endcsname{32}
\expandafter\def\csname v@lk/final/remote-f20/delay_ms_max\endcsname{50}
\expandafter\def\csname v@lk/final/remote-f20/delay_ms_p50\endcsname{30}
\expandafter\def\csname v@lk/final/remote-f20/delay_ms_p99\endcsname{50}
\expandafter\def\csname v@lk/final/remote-f20/drift_s_p99\endcsname{0.021}
\expandafter\def\csname v@lk/final/remote-f20/false_starts_per_min\endcsname{1.59}
\expandafter\def\csname v@lk/final/remote-f20/filter_core_pct\endcsname{10}
\expandafter\def\csname v@lk/final/remote-f20/filter_core_per_call\endcsname{0.095}
\expandafter\def\csname v@lk/final/remote-f20/frame_ms_max\endcsname{14.94}
\expandafter\def\csname v@lk/final/remote-f20/frame_ms_p50\endcsname{0.12}
\expandafter\def\csname v@lk/final/remote-f20/frame_ms_p99\endcsname{11.83}
\expandafter\def\csname v@lk/final/remote-f20/held_pct\endcsname{18}
\expandafter\def\csname v@lk/final/remote-f20/job_core_per_call\endcsname{0.079}
\expandafter\def\csname v@lk/final/remote-f20/join_s_max\endcsname{30}
\expandafter\def\csname v@lk/final/remote-f20/join_s_p50\endcsname{29}
\expandafter\def\csname v@lk/final/remote-f20/pauses_heard_pct\endcsname{24.1}
\expandafter\def\csname v@lk/final/remote-f20/turn_end_p90_s\endcsname{1.03}
\expandafter\def\csname v@lk/final/remote-f20/turns\endcsname{239}
\expandafter\def\csname v@lk/final/remote-f20/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/final/remote-nowait/caller_missed_pct\endcsname{7.0}
\expandafter\def\csname v@lk/final/remote-nowait/calls\endcsname{32}
\expandafter\def\csname v@lk/final/remote-nowait/delay_ms_max\endcsname{90}
\expandafter\def\csname v@lk/final/remote-nowait/delay_ms_p50\endcsname{90}
\expandafter\def\csname v@lk/final/remote-nowait/delay_ms_p99\endcsname{90}
\expandafter\def\csname v@lk/final/remote-nowait/drift_s_p99\endcsname{0.015}
\expandafter\def\csname v@lk/final/remote-nowait/false_starts_per_min\endcsname{1.59}
\expandafter\def\csname v@lk/final/remote-nowait/filter_core_pct\endcsname{0}
\expandafter\def\csname v@lk/final/remote-nowait/filter_core_per_call\endcsname{0.003}
\expandafter\def\csname v@lk/final/remote-nowait/frame_ms_max\endcsname{2.78}
\expandafter\def\csname v@lk/final/remote-nowait/frame_ms_p50\endcsname{0.11}
\expandafter\def\csname v@lk/final/remote-nowait/frame_ms_p99\endcsname{0.31}
\expandafter\def\csname v@lk/final/remote-nowait/held_pct\endcsname{19}
\expandafter\def\csname v@lk/final/remote-nowait/job_core_per_call\endcsname{0.066}
\expandafter\def\csname v@lk/final/remote-nowait/join_s_max\endcsname{25}
\expandafter\def\csname v@lk/final/remote-nowait/join_s_p50\endcsname{24}
\expandafter\def\csname v@lk/final/remote-nowait/pauses_heard_pct\endcsname{25.4}
\expandafter\def\csname v@lk/final/remote-nowait/turn_end_p90_s\endcsname{1.15}
\expandafter\def\csname v@lk/final/remote-nowait/turns\endcsname{239}
\expandafter\def\csname v@lk/final/remote-nowait/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/final/remote/caller_missed_pct\endcsname{6.9}
\expandafter\def\csname v@lk/final/remote/calls\endcsname{32}
\expandafter\def\csname v@lk/final/remote/delay_ms_max\endcsname{50}
\expandafter\def\csname v@lk/final/remote/delay_ms_p50\endcsname{40}
\expandafter\def\csname v@lk/final/remote/delay_ms_p99\endcsname{50}
\expandafter\def\csname v@lk/final/remote/drift_s_p99\endcsname{0.022}
\expandafter\def\csname v@lk/final/remote/false_starts_per_min\endcsname{1.75}
\expandafter\def\csname v@lk/final/remote/filter_core_pct\endcsname{32}
\expandafter\def\csname v@lk/final/remote/filter_core_per_call\endcsname{0.315}
\expandafter\def\csname v@lk/final/remote/frame_ms_max\endcsname{34.39}
\expandafter\def\csname v@lk/final/remote/frame_ms_p50\endcsname{14.46}
\expandafter\def\csname v@lk/final/remote/frame_ms_p99\endcsname{30.25}
\expandafter\def\csname v@lk/final/remote/held_pct\endcsname{18}
\expandafter\def\csname v@lk/final/remote/job_core_per_call\endcsname{0.070}
\expandafter\def\csname v@lk/final/remote/join_s_max\endcsname{30}
\expandafter\def\csname v@lk/final/remote/join_s_p50\endcsname{28}
\expandafter\def\csname v@lk/final/remote/pauses_heard_pct\endcsname{24.9}
\expandafter\def\csname v@lk/final/remote/turn_end_p90_s\endcsname{1.06}
\expandafter\def\csname v@lk/final/remote/turns\endcsname{239}
\expandafter\def\csname v@lk/final/remote/unfiltered_pct\endcsname{0.1}
\expandafter\def\csname v@lk/final64/remote-nowait/caller_missed_pct\endcsname{8.6}
\expandafter\def\csname v@lk/final64/remote-nowait/calls\endcsname{64}
\expandafter\def\csname v@lk/final64/remote-nowait/delay_ms_max\endcsname{180}
\expandafter\def\csname v@lk/final64/remote-nowait/delay_ms_p50\endcsname{100}
\expandafter\def\csname v@lk/final64/remote-nowait/delay_ms_p99\endcsname{110}
\expandafter\def\csname v@lk/final64/remote-nowait/drift_s_p99\endcsname{0.046}
\expandafter\def\csname v@lk/final64/remote-nowait/false_starts_per_min\endcsname{1.59}
\expandafter\def\csname v@lk/final64/remote-nowait/filter_core_pct\endcsname{0}
\expandafter\def\csname v@lk/final64/remote-nowait/filter_core_per_call\endcsname{0.003}
\expandafter\def\csname v@lk/final64/remote-nowait/frame_ms_max\endcsname{4.69}
\expandafter\def\csname v@lk/final64/remote-nowait/frame_ms_p50\endcsname{0.13}
\expandafter\def\csname v@lk/final64/remote-nowait/frame_ms_p99\endcsname{0.40}
\expandafter\def\csname v@lk/final64/remote-nowait/held_pct\endcsname{21}
\expandafter\def\csname v@lk/final64/remote-nowait/job_core_per_call\endcsname{0.062}
\expandafter\def\csname v@lk/final64/remote-nowait/join_s_max\endcsname{67}
\expandafter\def\csname v@lk/final64/remote-nowait/join_s_p50\endcsname{62}
\expandafter\def\csname v@lk/final64/remote-nowait/pauses_heard_pct\endcsname{22.8}
\expandafter\def\csname v@lk/final64/remote-nowait/turn_end_p90_s\endcsname{1.03}
\expandafter\def\csname v@lk/final64/remote-nowait/turns\endcsname{487}
\expandafter\def\csname v@lk/final64/remote-nowait/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/final64/remote/caller_missed_pct\endcsname{8.5}
\expandafter\def\csname v@lk/final64/remote/calls\endcsname{64}
\expandafter\def\csname v@lk/final64/remote/delay_ms_max\endcsname{50}
\expandafter\def\csname v@lk/final64/remote/delay_ms_p50\endcsname{50}
\expandafter\def\csname v@lk/final64/remote/delay_ms_p99\endcsname{50}
\expandafter\def\csname v@lk/final64/remote/drift_s_p99\endcsname{0.062}
\expandafter\def\csname v@lk/final64/remote/false_starts_per_min\endcsname{1.61}
\expandafter\def\csname v@lk/final64/remote/filter_core_pct\endcsname{38}
\expandafter\def\csname v@lk/final64/remote/filter_core_per_call\endcsname{0.380}
\expandafter\def\csname v@lk/final64/remote/frame_ms_max\endcsname{73.03}
\expandafter\def\csname v@lk/final64/remote/frame_ms_p50\endcsname{18.23}
\expandafter\def\csname v@lk/final64/remote/frame_ms_p99\endcsname{30.30}
\expandafter\def\csname v@lk/final64/remote/held_pct\endcsname{21}
\expandafter\def\csname v@lk/final64/remote/job_core_per_call\endcsname{0.065}
\expandafter\def\csname v@lk/final64/remote/join_s_max\endcsname{79}
\expandafter\def\csname v@lk/final64/remote/join_s_p50\endcsname{72}
\expandafter\def\csname v@lk/final64/remote/pauses_heard_pct\endcsname{22.8}
\expandafter\def\csname v@lk/final64/remote/server_busy_ms_p50\endcsname{33}
\expandafter\def\csname v@lk/final64/remote/server_calls\endcsname{64}
\expandafter\def\csname v@lk/final64/remote/server_step_ms_p50\endcsname{10}
\expandafter\def\csname v@lk/final64/remote/server_tick_ms\endcsname{40}
\expandafter\def\csname v@lk/final64/remote/turn_end_p90_s\endcsname{1.02}
\expandafter\def\csname v@lk/final64/remote/turns\endcsname{487}
\expandafter\def\csname v@lk/final64/remote/unfiltered_pct\endcsname{1.0}
\expandafter\def\csname v@lk/wait32/remote-b30/caller_missed_pct\endcsname{7.3}
\expandafter\def\csname v@lk/wait32/remote-b30/calls\endcsname{32}
\expandafter\def\csname v@lk/wait32/remote-b30/delay_ms_max\endcsname{90}
\expandafter\def\csname v@lk/wait32/remote-b30/delay_ms_p50\endcsname{40}
\expandafter\def\csname v@lk/wait32/remote-b30/delay_ms_p99\endcsname{80}
\expandafter\def\csname v@lk/wait32/remote-b30/drift_s_p99\endcsname{0.045}
\expandafter\def\csname v@lk/wait32/remote-b30/false_starts_per_min\endcsname{1.59}
\expandafter\def\csname v@lk/wait32/remote-b30/filter_core_pct\endcsname{32}
\expandafter\def\csname v@lk/wait32/remote-b30/filter_core_per_call\endcsname{0.316}
\expandafter\def\csname v@lk/wait32/remote-b30/frame_ms_max\endcsname{33.67}
\expandafter\def\csname v@lk/wait32/remote-b30/frame_ms_p50\endcsname{14.36}
\expandafter\def\csname v@lk/wait32/remote-b30/frame_ms_p99\endcsname{30.25}
\expandafter\def\csname v@lk/wait32/remote-b30/held_pct\endcsname{18}
\expandafter\def\csname v@lk/wait32/remote-b30/job_core_per_call\endcsname{0.069}
\expandafter\def\csname v@lk/wait32/remote-b30/join_s_max\endcsname{30}
\expandafter\def\csname v@lk/wait32/remote-b30/join_s_p50\endcsname{29}
\expandafter\def\csname v@lk/wait32/remote-b30/pauses_heard_pct\endcsname{24.7}
\expandafter\def\csname v@lk/wait32/remote-b30/turn_end_p90_s\endcsname{1.04}
\expandafter\def\csname v@lk/wait32/remote-b30/turns\endcsname{239}
\expandafter\def\csname v@lk/wait32/remote-b30/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/wait32/remote-c40/caller_missed_pct\endcsname{6.8}
\expandafter\def\csname v@lk/wait32/remote-c40/calls\endcsname{32}
\expandafter\def\csname v@lk/wait32/remote-c40/delay_ms_max\endcsname{50}
\expandafter\def\csname v@lk/wait32/remote-c40/delay_ms_p50\endcsname{40}
\expandafter\def\csname v@lk/wait32/remote-c40/delay_ms_p99\endcsname{50}
\expandafter\def\csname v@lk/wait32/remote-c40/drift_s_p99\endcsname{0.040}
\expandafter\def\csname v@lk/wait32/remote-c40/false_starts_per_min\endcsname{1.59}
\expandafter\def\csname v@lk/wait32/remote-c40/filter_core_pct\endcsname{32}
\expandafter\def\csname v@lk/wait32/remote-c40/filter_core_per_call\endcsname{0.316}
\expandafter\def\csname v@lk/wait32/remote-c40/frame_ms_max\endcsname{32.63}
\expandafter\def\csname v@lk/wait32/remote-c40/frame_ms_p50\endcsname{14.56}
\expandafter\def\csname v@lk/wait32/remote-c40/frame_ms_p99\endcsname{30.25}
\expandafter\def\csname v@lk/wait32/remote-c40/held_pct\endcsname{18}
\expandafter\def\csname v@lk/wait32/remote-c40/job_core_per_call\endcsname{0.069}
\expandafter\def\csname v@lk/wait32/remote-c40/join_s_max\endcsname{31}
\expandafter\def\csname v@lk/wait32/remote-c40/join_s_p50\endcsname{29}
\expandafter\def\csname v@lk/wait32/remote-c40/pauses_heard_pct\endcsname{24.5}
\expandafter\def\csname v@lk/wait32/remote-c40/turn_end_p90_s\endcsname{1.12}
\expandafter\def\csname v@lk/wait32/remote-c40/turns\endcsname{239}
\expandafter\def\csname v@lk/wait32/remote-c40/unfiltered_pct\endcsname{0.1}
\expandafter\def\csname v@lk/wait32/remote-p4x30/caller_missed_pct\endcsname{6.3}
\expandafter\def\csname v@lk/wait32/remote-p4x30/calls\endcsname{32}
\expandafter\def\csname v@lk/wait32/remote-p4x30/delay_ms_max\endcsname{90}
\expandafter\def\csname v@lk/wait32/remote-p4x30/delay_ms_p50\endcsname{40}
\expandafter\def\csname v@lk/wait32/remote-p4x30/delay_ms_p99\endcsname{60}
\expandafter\def\csname v@lk/wait32/remote-p4x30/drift_s_p99\endcsname{0.024}
\expandafter\def\csname v@lk/wait32/remote-p4x30/false_starts_per_min\endcsname{1.66}
\expandafter\def\csname v@lk/wait32/remote-p4x30/filter_core_pct\endcsname{33}
\expandafter\def\csname v@lk/wait32/remote-p4x30/filter_core_per_call\endcsname{0.329}
\expandafter\def\csname v@lk/wait32/remote-p4x30/frame_ms_max\endcsname{33.90}
\expandafter\def\csname v@lk/wait32/remote-p4x30/frame_ms_p50\endcsname{15.10}
\expandafter\def\csname v@lk/wait32/remote-p4x30/frame_ms_p99\endcsname{30.27}
\expandafter\def\csname v@lk/wait32/remote-p4x30/held_pct\endcsname{17}
\expandafter\def\csname v@lk/wait32/remote-p4x30/job_core_per_call\endcsname{0.068}
\expandafter\def\csname v@lk/wait32/remote-p4x30/join_s_max\endcsname{29}
\expandafter\def\csname v@lk/wait32/remote-p4x30/join_s_p50\endcsname{28}
\expandafter\def\csname v@lk/wait32/remote-p4x30/pauses_heard_pct\endcsname{25.2}
\expandafter\def\csname v@lk/wait32/remote-p4x30/turn_end_p90_s\endcsname{1.11}
\expandafter\def\csname v@lk/wait32/remote-p4x30/turns\endcsname{239}
\expandafter\def\csname v@lk/wait32/remote-p4x30/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/wait32/remote/caller_missed_pct\endcsname{7.0}
\expandafter\def\csname v@lk/wait32/remote/calls\endcsname{32}
\expandafter\def\csname v@lk/wait32/remote/delay_ms_max\endcsname{90}
\expandafter\def\csname v@lk/wait32/remote/delay_ms_p50\endcsname{90}
\expandafter\def\csname v@lk/wait32/remote/delay_ms_p99\endcsname{90}
\expandafter\def\csname v@lk/wait32/remote/drift_s_p99\endcsname{0.015}
\expandafter\def\csname v@lk/wait32/remote/false_starts_per_min\endcsname{1.59}
\expandafter\def\csname v@lk/wait32/remote/filter_core_pct\endcsname{0}
\expandafter\def\csname v@lk/wait32/remote/filter_core_per_call\endcsname{0.003}
\expandafter\def\csname v@lk/wait32/remote/frame_ms_max\endcsname{2.78}
\expandafter\def\csname v@lk/wait32/remote/frame_ms_p50\endcsname{0.11}
\expandafter\def\csname v@lk/wait32/remote/frame_ms_p99\endcsname{0.31}
\expandafter\def\csname v@lk/wait32/remote/held_pct\endcsname{19}
\expandafter\def\csname v@lk/wait32/remote/job_core_per_call\endcsname{0.066}
\expandafter\def\csname v@lk/wait32/remote/join_s_max\endcsname{25}
\expandafter\def\csname v@lk/wait32/remote/join_s_p50\endcsname{24}
\expandafter\def\csname v@lk/wait32/remote/pauses_heard_pct\endcsname{25.4}
\expandafter\def\csname v@lk/wait32/remote/turn_end_p90_s\endcsname{1.15}
\expandafter\def\csname v@lk/wait32/remote/turns\endcsname{239}
\expandafter\def\csname v@lk/wait32/remote/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/wait64/remote-b30/caller_missed_pct\endcsname{8.1}
\expandafter\def\csname v@lk/wait64/remote-b30/calls\endcsname{64}
\expandafter\def\csname v@lk/wait64/remote-b30/delay_ms_max\endcsname{90}
\expandafter\def\csname v@lk/wait64/remote-b30/delay_ms_p50\endcsname{60}
\expandafter\def\csname v@lk/wait64/remote-b30/delay_ms_p99\endcsname{90}
\expandafter\def\csname v@lk/wait64/remote-b30/drift_s_p99\endcsname{0.056}
\expandafter\def\csname v@lk/wait64/remote-b30/false_starts_per_min\endcsname{1.70}
\expandafter\def\csname v@lk/wait64/remote-b30/filter_core_pct\endcsname{23}
\expandafter\def\csname v@lk/wait64/remote-b30/filter_core_per_call\endcsname{0.235}
\expandafter\def\csname v@lk/wait64/remote-b30/frame_ms_max\endcsname{34.94}
\expandafter\def\csname v@lk/wait64/remote-b30/frame_ms_p50\endcsname{13.01}
\expandafter\def\csname v@lk/wait64/remote-b30/frame_ms_p99\endcsname{30.10}
\expandafter\def\csname v@lk/wait64/remote-b30/held_pct\endcsname{20}
\expandafter\def\csname v@lk/wait64/remote-b30/job_core_per_call\endcsname{0.064}
\expandafter\def\csname v@lk/wait64/remote-b30/join_s_max\endcsname{76}
\expandafter\def\csname v@lk/wait64/remote-b30/join_s_p50\endcsname{71}
\expandafter\def\csname v@lk/wait64/remote-b30/pauses_heard_pct\endcsname{23.0}
\expandafter\def\csname v@lk/wait64/remote-b30/turn_end_p90_s\endcsname{1.08}
\expandafter\def\csname v@lk/wait64/remote-b30/turns\endcsname{487}
\expandafter\def\csname v@lk/wait64/remote-b30/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lk/wait64/remote-c40/caller_missed_pct\endcsname{8.5}
\expandafter\def\csname v@lk/wait64/remote-c40/calls\endcsname{64}
\expandafter\def\csname v@lk/wait64/remote-c40/delay_ms_max\endcsname{50}
\expandafter\def\csname v@lk/wait64/remote-c40/delay_ms_p50\endcsname{50}
\expandafter\def\csname v@lk/wait64/remote-c40/delay_ms_p99\endcsname{50}
\expandafter\def\csname v@lk/wait64/remote-c40/drift_s_p99\endcsname{0.055}
\expandafter\def\csname v@lk/wait64/remote-c40/false_starts_per_min\endcsname{1.69}
\expandafter\def\csname v@lk/wait64/remote-c40/filter_core_pct\endcsname{37}
\expandafter\def\csname v@lk/wait64/remote-c40/filter_core_per_call\endcsname{0.370}
\expandafter\def\csname v@lk/wait64/remote-c40/frame_ms_max\endcsname{44.54}
\expandafter\def\csname v@lk/wait64/remote-c40/frame_ms_p50\endcsname{17.99}
\expandafter\def\csname v@lk/wait64/remote-c40/frame_ms_p99\endcsname{30.29}
\expandafter\def\csname v@lk/wait64/remote-c40/held_pct\endcsname{21}
\expandafter\def\csname v@lk/wait64/remote-c40/job_core_per_call\endcsname{0.065}
\expandafter\def\csname v@lk/wait64/remote-c40/join_s_max\endcsname{77}
\expandafter\def\csname v@lk/wait64/remote-c40/join_s_p50\endcsname{72}
\expandafter\def\csname v@lk/wait64/remote-c40/pauses_heard_pct\endcsname{22.9}
\expandafter\def\csname v@lk/wait64/remote-c40/turn_end_p90_s\endcsname{1.02}
\expandafter\def\csname v@lk/wait64/remote-c40/turns\endcsname{487}
\expandafter\def\csname v@lk/wait64/remote-c40/unfiltered_pct\endcsname{0.6}
\expandafter\def\csname v@lk/wait64/remote/caller_missed_pct\endcsname{8.6}
\expandafter\def\csname v@lk/wait64/remote/calls\endcsname{64}
\expandafter\def\csname v@lk/wait64/remote/delay_ms_max\endcsname{180}
\expandafter\def\csname v@lk/wait64/remote/delay_ms_p50\endcsname{100}
\expandafter\def\csname v@lk/wait64/remote/delay_ms_p99\endcsname{110}
\expandafter\def\csname v@lk/wait64/remote/drift_s_p99\endcsname{0.046}
\expandafter\def\csname v@lk/wait64/remote/false_starts_per_min\endcsname{1.59}
\expandafter\def\csname v@lk/wait64/remote/filter_core_pct\endcsname{0}
\expandafter\def\csname v@lk/wait64/remote/filter_core_per_call\endcsname{0.003}
\expandafter\def\csname v@lk/wait64/remote/frame_ms_max\endcsname{4.69}
\expandafter\def\csname v@lk/wait64/remote/frame_ms_p50\endcsname{0.13}
\expandafter\def\csname v@lk/wait64/remote/frame_ms_p99\endcsname{0.40}
\expandafter\def\csname v@lk/wait64/remote/held_pct\endcsname{21}
\expandafter\def\csname v@lk/wait64/remote/job_core_per_call\endcsname{0.062}
\expandafter\def\csname v@lk/wait64/remote/join_s_max\endcsname{67}
\expandafter\def\csname v@lk/wait64/remote/join_s_p50\endcsname{62}
\expandafter\def\csname v@lk/wait64/remote/pauses_heard_pct\endcsname{22.8}
\expandafter\def\csname v@lk/wait64/remote/turn_end_p90_s\endcsname{1.03}
\expandafter\def\csname v@lk/wait64/remote/turns\endcsname{487}
\expandafter\def\csname v@lk/wait64/remote/unfiltered_pct\endcsname{0.0}
\expandafter\def\csname v@lklone/before/others\endcsname{281}
\expandafter\def\csname v@lklone/calls\endcsname{16}
\expandafter\def\csname v@lklone/direct/cut-max\endcsname{72}
\expandafter\def\csname v@lklone/direct/cut-min\endcsname{35}
\expandafter\def\csname v@lklone/direct/others\endcsname{1}
\expandafter\def\csname v@lklone/livekit/cut-max\endcsname{10}
\expandafter\def\csname v@lklone/livekit/cut-min\endcsname{4}
\expandafter\def\csname v@lklone/livekit/others\endcsname{126}
\expandafter\def\csname v@lklone/livekit/unfiltered-pct\endcsname{33}
\expandafter\def\csname v@lklone/livekit/unfiltered-s\endcsname{147.9}
\expandafter\def\csname v@lklone/livekit_lag/cut-max\endcsname{78}
\expandafter\def\csname v@lklone/livekit_lag/cut-min\endcsname{32}
\expandafter\def\csname v@lklone/livekit_lag/delay-max\endcsname{260}
\expandafter\def\csname v@lklone/livekit_lag/delay-p50\endcsname{90}
\expandafter\def\csname v@lklone/livekit_lag/unfiltered-pct\endcsname{0}
\expandafter\def\csname v@lklone/livekit_lag/unfiltered-s\endcsname{0.3}
\expandafter\def\csname v@lklone/seconds\endcsname{453}
\expandafter\def\csname v@long/long_bg/over4\endcsname{0.7}
\expandafter\def\csname v@long/long_bg/over8\endcsname{0.0}
\expandafter\def\csname v@long/long_bg/primary\endcsname{45}
\expandafter\def\csname v@long/seg24/over4\endcsname{2.4}
\expandafter\def\csname v@long/seg24/over8\endcsname{1.6}
\expandafter\def\csname v@long/seg24/primary\endcsname{44}
\expandafter\def\csname v@long/stage1/over4\endcsname{0.1}
\expandafter\def\csname v@long/stage1/over8\endcsname{0.0}
\expandafter\def\csname v@long/stage1/primary\endcsname{55}
\expandafter\def\csname v@long/turns/over4\endcsname{7.5}
\expandafter\def\csname v@long/turns/over8\endcsname{4.5}
\expandafter\def\csname v@long/turns/primary\endcsname{33}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/aic_calls/ins\endcsname{10.16}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/aic_calls/leak\endcsname{11.86}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/aic_calls/miss\endcsname{5.95}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/aic_calls/wer\endcsname{16.11}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ali_test/ins\endcsname{1.15}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ali_test/leak\endcsname{1.46}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ali_test/miss\endcsname{14.58}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ali_test/wer\endcsname{15.73}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_headset2/ins\endcsname{3.18}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_headset2/leak\endcsname{2.52}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_headset2/miss\endcsname{7.88}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_headset2/wer\endcsname{11.06}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_test/ins\endcsname{2.66}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_test/leak\endcsname{1.90}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_test/miss\endcsname{8.07}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_test/wer\endcsname{10.73}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_test_long/ins\endcsname{4.23}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_test_long/leak\endcsname{3.76}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_test_long/miss\endcsname{11.70}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/ami_test_long/wer\endcsname{15.94}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/call_test_clean/ins\endcsname{0.85}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/call_test_clean/miss\endcsname{3.50}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/call_test_clean/wer\endcsname{4.35}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/call_test_mix/ins\endcsname{27.89}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/call_test_mix/leak\endcsname{68.68}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/call_test_mix/miss\endcsname{24.41}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/call_test_mix/wer\endcsname{52.30}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/krisp/ins\endcsname{0.72}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/krisp/leak\endcsname{0.02}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/krisp/miss\endcsname{4.72}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/krisp/wer\endcsname{5.44}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/nsf_test/ins\endcsname{1.83}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/nsf_test/leak\endcsname{0.32}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/nsf_test/miss\endcsname{5.69}
\expandafter\def\csname v@main/C10n_ftlong_kd_selfl/nsf_test/wer\endcsname{7.52}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/aic_calls/ins\endcsname{11.40}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/aic_calls/leak\endcsname{13.25}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/aic_calls/miss\endcsname{6.63}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/aic_calls/wer\endcsname{18.03}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ali_test/ins\endcsname{1.17}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ali_test/leak\endcsname{1.96}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ali_test/miss\endcsname{14.66}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ali_test/wer\endcsname{15.82}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_headset2/ins\endcsname{3.32}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_headset2/leak\endcsname{2.52}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_headset2/miss\endcsname{7.91}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_headset2/wer\endcsname{11.23}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_test/ins\endcsname{2.40}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_test/leak\endcsname{1.29}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_test/miss\endcsname{7.89}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_test/wer\endcsname{10.29}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_test_long/ins\endcsname{3.51}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_test_long/leak\endcsname{3.08}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_test_long/miss\endcsname{12.04}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/ami_test_long/wer\endcsname{15.55}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/call_test_clean/ins\endcsname{1.09}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/call_test_clean/miss\endcsname{4.23}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/call_test_clean/wer\endcsname{5.32}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/call_test_mix/ins\endcsname{24.46}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/call_test_mix/leak\endcsname{63.32}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/call_test_mix/miss\endcsname{25.44}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/call_test_mix/wer\endcsname{49.90}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/krisp/ins\endcsname{0.69}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/krisp/leak\endcsname{0.04}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/krisp/miss\endcsname{4.98}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/krisp/wer\endcsname{5.66}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/nsf_test/ins\endcsname{1.84}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/nsf_test/leak\endcsname{0.55}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/nsf_test/miss\endcsname{5.74}
\expandafter\def\csname v@main/C22_ftlong_kd_selfl/nsf_test/wer\endcsname{7.58}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/aic_calls/ins\endcsname{7.84}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/aic_calls/leak\endcsname{7.95}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/aic_calls/miss\endcsname{6.52}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/aic_calls/wer\endcsname{14.36}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ali_test/ins\endcsname{1.13}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ali_test/leak\endcsname{1.79}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ali_test/miss\endcsname{14.63}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ali_test/wer\endcsname{15.75}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_headset2/ins\endcsname{3.21}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_headset2/leak\endcsname{2.12}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_headset2/miss\endcsname{6.84}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_headset2/wer\endcsname{10.06}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_test/ins\endcsname{2.40}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_test/leak\endcsname{1.73}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_test/miss\endcsname{7.58}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_test/wer\endcsname{9.97}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_test_long/ins\endcsname{4.19}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_test_long/leak\endcsname{3.78}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_test_long/miss\endcsname{11.73}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/ami_test_long/wer\endcsname{15.91}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/call_test_clean/ins\endcsname{0.88}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/call_test_clean/miss\endcsname{6.39}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/call_test_clean/wer\endcsname{7.27}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/call_test_mix/ins\endcsname{21.52}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/call_test_mix/leak\endcsname{57.40}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/call_test_mix/miss\endcsname{26.85}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/call_test_mix/wer\endcsname{48.36}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/krisp/ins\endcsname{0.71}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/krisp/leak\endcsname{0.11}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/krisp/miss\endcsname{4.84}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/krisp/wer\endcsname{5.55}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/nsf_test/ins\endcsname{1.92}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/nsf_test/leak\endcsname{0.53}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/nsf_test/miss\endcsname{5.84}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2_selfl/nsf_test/wer\endcsname{7.76}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/aic_calls/ins\endcsname{7.06}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/aic_calls/leak\endcsname{5.30}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/aic_calls/miss\endcsname{5.49}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/aic_calls/wer\endcsname{12.54}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ali_test/ins\endcsname{1.15}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ali_test/leak\endcsname{1.88}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ali_test/miss\endcsname{14.25}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ali_test/wer\endcsname{15.40}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_headset2/ins\endcsname{3.39}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_headset2/leak\endcsname{2.25}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_headset2/miss\endcsname{7.98}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_headset2/wer\endcsname{11.37}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_test/ins\endcsname{2.51}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_test/leak\endcsname{1.90}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_test/miss\endcsname{7.83}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_test/wer\endcsname{10.35}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_test_long/ins\endcsname{4.39}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_test_long/leak\endcsname{3.91}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_test_long/miss\endcsname{11.82}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/ami_test_long/wer\endcsname{16.22}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/call_test_clean/ins\endcsname{1.09}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/call_test_clean/miss\endcsname{4.57}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/call_test_clean/wer\endcsname{5.66}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/call_test_mix/ins\endcsname{21.49}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/call_test_mix/leak\endcsname{58.84}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/call_test_mix/miss\endcsname{26.38}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/call_test_mix/wer\endcsname{47.87}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/krisp/ins\endcsname{0.67}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/krisp/leak\endcsname{0.05}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/krisp/miss\endcsname{5.26}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/krisp/wer\endcsname{5.93}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/nsf_test/ins\endcsname{1.89}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/nsf_test/leak\endcsname{0.47}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/nsf_test/miss\endcsname{5.79}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_loud/nsf_test/wer\endcsname{7.67}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/aic_calls/ins\endcsname{8.27}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/aic_calls/leak\endcsname{8.45}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/aic_calls/miss\endcsname{6.20}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/aic_calls/wer\endcsname{14.47}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ali_test/ins\endcsname{1.25}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ali_test/leak\endcsname{1.93}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ali_test/miss\endcsname{14.49}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ali_test/wer\endcsname{15.74}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_headset2/ins\endcsname{3.32}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_headset2/leak\endcsname{2.25}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_headset2/miss\endcsname{6.70}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_headset2/wer\endcsname{10.02}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_test/ins\endcsname{2.55}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_test/leak\endcsname{1.90}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_test/miss\endcsname{7.54}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_test/wer\endcsname{10.09}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_test_long/ins\endcsname{5.09}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_test_long/leak\endcsname{5.34}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_test_long/miss\endcsname{11.10}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/ami_test_long/wer\endcsname{16.19}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/call_test_clean/ins\endcsname{1.08}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/call_test_clean/miss\endcsname{4.82}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/call_test_clean/wer\endcsname{5.90}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/call_test_mix/ins\endcsname{22.28}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/call_test_mix/leak\endcsname{58.02}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/call_test_mix/miss\endcsname{25.15}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/call_test_mix/wer\endcsname{47.43}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/krisp/ins\endcsname{1.14}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/krisp/leak\endcsname{1.80}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/krisp/miss\endcsname{5.14}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/krisp/wer\endcsname{6.28}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/nsf_test/ins\endcsname{1.91}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/nsf_test/leak\endcsname{0.49}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/nsf_test/miss\endcsname{5.82}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_null/nsf_test/wer\endcsname{7.74}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/aic_calls/ins\endcsname{8.52}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/aic_calls/leak\endcsname{8.39}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/aic_calls/miss\endcsname{5.74}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/aic_calls/wer\endcsname{14.26}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ali_test/ins\endcsname{1.21}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ali_test/leak\endcsname{1.79}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ali_test/miss\endcsname{14.47}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ali_test/wer\endcsname{15.69}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_headset2/ins\endcsname{3.46}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_headset2/leak\endcsname{2.39}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_headset2/miss\endcsname{6.74}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_headset2/wer\endcsname{10.19}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_test/ins\endcsname{2.67}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_test/leak\endcsname{1.90}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_test/miss\endcsname{7.51}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_test/wer\endcsname{10.18}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_test_long/ins\endcsname{4.58}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_test_long/leak\endcsname{4.11}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_test_long/miss\endcsname{11.55}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/ami_test_long/wer\endcsname{16.13}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/call_test_clean/ins\endcsname{0.99}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/call_test_clean/miss\endcsname{4.58}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/call_test_clean/wer\endcsname{5.58}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/call_test_mix/ins\endcsname{20.12}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/call_test_mix/leak\endcsname{56.88}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/call_test_mix/miss\endcsname{27.39}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/call_test_mix/wer\endcsname{47.52}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/krisp/ins\endcsname{0.67}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/krisp/leak\endcsname{0.04}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/krisp/miss\endcsname{5.08}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/krisp/wer\endcsname{5.74}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/nsf_test/ins\endcsname{1.91}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/nsf_test/leak\endcsname{0.38}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/nsf_test/miss\endcsname{5.76}
\expandafter\def\csname v@main/MB_ftlong_ws_cwlt2m_selfl/nsf_test/wer\endcsname{7.67}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/aic_calls/ins\endcsname{9.16}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/aic_calls/leak\endcsname{8.83}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/aic_calls/miss\endcsname{6.31}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/aic_calls/wer\endcsname{15.47}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ali_test/ins\endcsname{3.29}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ali_test/leak\endcsname{13.03}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ali_test/miss\endcsname{14.56}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ali_test/wer\endcsname{17.85}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_headset2/ins\endcsname{3.14}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_headset2/leak\endcsname{2.25}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_headset2/miss\endcsname{8.09}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_headset2/wer\endcsname{11.23}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_test/ins\endcsname{2.49}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_test/leak\endcsname{1.87}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_test/miss\endcsname{8.13}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_test/wer\endcsname{10.62}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_test_long/ins\endcsname{3.46}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_test_long/leak\endcsname{3.08}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_test_long/miss\endcsname{12.98}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/ami_test_long/wer\endcsname{16.44}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/call_test_clean/ins\endcsname{1.15}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/call_test_clean/miss\endcsname{6.45}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/call_test_clean/wer\endcsname{7.60}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/call_test_mix/ins\endcsname{20.86}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/call_test_mix/leak\endcsname{58.07}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/call_test_mix/miss\endcsname{27.13}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/call_test_mix/wer\endcsname{47.99}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/krisp/ins\endcsname{0.84}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/krisp/leak\endcsname{0.48}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/krisp/miss\endcsname{4.92}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/krisp/wer\endcsname{5.76}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/nsf_test/ins\endcsname{1.87}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/nsf_test/leak\endcsname{0.38}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/nsf_test/miss\endcsname{5.83}
\expandafter\def\csname v@main/MB_ftlong_ws_loud/nsf_test/wer\endcsname{7.70}
\expandafter\def\csname v@main/MB_ftlong_ws_null/aic_calls/ins\endcsname{11.12}
\expandafter\def\csname v@main/MB_ftlong_ws_null/aic_calls/leak\endcsname{13.06}
\expandafter\def\csname v@main/MB_ftlong_ws_null/aic_calls/miss\endcsname{5.74}
\expandafter\def\csname v@main/MB_ftlong_ws_null/aic_calls/wer\endcsname{16.86}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ali_test/ins\endcsname{1.08}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ali_test/leak\endcsname{1.46}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ali_test/miss\endcsname{14.94}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ali_test/wer\endcsname{16.02}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_headset2/ins\endcsname{3.42}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_headset2/leak\endcsname{2.92}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_headset2/miss\endcsname{6.84}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_headset2/wer\endcsname{10.26}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_test/ins\endcsname{2.44}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_test/leak\endcsname{1.64}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_test/miss\endcsname{7.83}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_test/wer\endcsname{10.27}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_test_long/ins\endcsname{6.40}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_test_long/leak\endcsname{6.72}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_test_long/miss\endcsname{11.99}
\expandafter\def\csname v@main/MB_ftlong_ws_null/ami_test_long/wer\endcsname{18.39}
\expandafter\def\csname v@main/MB_ftlong_ws_null/call_test_clean/ins\endcsname{1.16}
\expandafter\def\csname v@main/MB_ftlong_ws_null/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/MB_ftlong_ws_null/call_test_clean/miss\endcsname{5.67}
\expandafter\def\csname v@main/MB_ftlong_ws_null/call_test_clean/wer\endcsname{6.84}
\expandafter\def\csname v@main/MB_ftlong_ws_null/call_test_mix/ins\endcsname{24.61}
\expandafter\def\csname v@main/MB_ftlong_ws_null/call_test_mix/leak\endcsname{65.02}
\expandafter\def\csname v@main/MB_ftlong_ws_null/call_test_mix/miss\endcsname{26.24}
\expandafter\def\csname v@main/MB_ftlong_ws_null/call_test_mix/wer\endcsname{50.85}
\expandafter\def\csname v@main/MB_ftlong_ws_null/krisp/ins\endcsname{1.43}
\expandafter\def\csname v@main/MB_ftlong_ws_null/krisp/leak\endcsname{2.72}
\expandafter\def\csname v@main/MB_ftlong_ws_null/krisp/miss\endcsname{5.12}
\expandafter\def\csname v@main/MB_ftlong_ws_null/krisp/wer\endcsname{6.55}
\expandafter\def\csname v@main/MB_ftlong_ws_null/nsf_test/ins\endcsname{1.83}
\expandafter\def\csname v@main/MB_ftlong_ws_null/nsf_test/leak\endcsname{0.47}
\expandafter\def\csname v@main/MB_ftlong_ws_null/nsf_test/miss\endcsname{5.81}
\expandafter\def\csname v@main/MB_ftlong_ws_null/nsf_test/wer\endcsname{7.64}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/aic_calls/ins\endcsname{10.87}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/aic_calls/leak\endcsname{11.92}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/aic_calls/miss\endcsname{5.70}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/aic_calls/wer\endcsname{16.57}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ali_test/ins\endcsname{3.30}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ali_test/leak\endcsname{12.83}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ali_test/miss\endcsname{15.28}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ali_test/wer\endcsname{18.57}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_headset2/ins\endcsname{3.28}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_headset2/leak\endcsname{2.25}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_headset2/miss\endcsname{6.67}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_headset2/wer\endcsname{9.95}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_test/ins\endcsname{2.56}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_test/leak\endcsname{2.02}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_test/miss\endcsname{7.95}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_test/wer\endcsname{10.51}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_test_long/ins\endcsname{3.90}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_test_long/leak\endcsname{3.59}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_test_long/miss\endcsname{12.94}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/ami_test_long/wer\endcsname{16.84}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/call_test_clean/ins\endcsname{1.18}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/call_test_clean/miss\endcsname{7.62}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/call_test_clean/wer\endcsname{8.80}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/call_test_mix/ins\endcsname{19.89}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/call_test_mix/leak\endcsname{58.63}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/call_test_mix/miss\endcsname{28.33}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/call_test_mix/wer\endcsname{48.22}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/krisp/leak\endcsname{0.21}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/krisp/miss\endcsname{5.05}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/krisp/wer\endcsname{5.79}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/nsf_test/ins\endcsname{1.84}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/nsf_test/leak\endcsname{0.42}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/nsf_test/miss\endcsname{5.74}
\expandafter\def\csname v@main/MB_ftlong_ws_selfl/nsf_test/wer\endcsname{7.58}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/aic_calls/ins\endcsname{11.44}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/aic_calls/leak\endcsname{14.01}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/aic_calls/miss\endcsname{7.02}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/aic_calls/wer\endcsname{18.46}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ali_test/ins\endcsname{3.39}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ali_test/leak\endcsname{12.97}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ali_test/miss\endcsname{14.70}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ali_test/wer\endcsname{18.09}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_headset2/ins\endcsname{3.35}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_headset2/leak\endcsname{2.12}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_headset2/miss\endcsname{6.88}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_headset2/wer\endcsname{10.23}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_test/ins\endcsname{2.41}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_test/leak\endcsname{1.55}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_test/miss\endcsname{8.05}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_test/wer\endcsname{10.47}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_test_long/ins\endcsname{3.74}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_test_long/leak\endcsname{3.10}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_test_long/miss\endcsname{11.74}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/ami_test_long/wer\endcsname{15.48}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/call_test_clean/ins\endcsname{1.19}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/call_test_clean/miss\endcsname{7.36}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/call_test_clean/wer\endcsname{8.55}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/call_test_mix/ins\endcsname{22.18}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/call_test_mix/leak\endcsname{60.59}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/call_test_mix/miss\endcsname{26.68}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/call_test_mix/wer\endcsname{48.86}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/krisp/leak\endcsname{0.12}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/krisp/miss\endcsname{5.40}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/krisp/wer\endcsname{6.12}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/nsf_test/ins\endcsname{1.90}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/nsf_test/leak\endcsname{0.53}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/nsf_test/miss\endcsname{5.89}
\expandafter\def\csname v@main/SB_ftlong_ws_selfl/nsf_test/wer\endcsname{7.78}
\expandafter\def\csname v@main/dfn3/aic_calls/ins\endcsname{26.12}
\expandafter\def\csname v@main/dfn3/aic_calls/leak\endcsname{36.97}
\expandafter\def\csname v@main/dfn3/aic_calls/miss\endcsname{9.23}
\expandafter\def\csname v@main/dfn3/aic_calls/wer\endcsname{35.35}
\expandafter\def\csname v@main/dfn3/ali_test/ins\endcsname{1.56}
\expandafter\def\csname v@main/dfn3/ali_test/leak\endcsname{4.46}
\expandafter\def\csname v@main/dfn3/ali_test/miss\endcsname{16.92}
\expandafter\def\csname v@main/dfn3/ali_test/wer\endcsname{18.48}
\expandafter\def\csname v@main/dfn3/ami_headset2/ins\endcsname{8.88}
\expandafter\def\csname v@main/dfn3/ami_headset2/leak\endcsname{23.33}
\expandafter\def\csname v@main/dfn3/ami_headset2/miss\endcsname{12.68}
\expandafter\def\csname v@main/dfn3/ami_headset2/wer\endcsname{21.56}
\expandafter\def\csname v@main/dfn3/ami_test/ins\endcsname{11.60}
\expandafter\def\csname v@main/dfn3/ami_test/leak\endcsname{32.79}
\expandafter\def\csname v@main/dfn3/ami_test/miss\endcsname{14.40}
\expandafter\def\csname v@main/dfn3/ami_test/wer\endcsname{26.00}
\expandafter\def\csname v@main/dfn3/ami_test_long/ins\endcsname{19.60}
\expandafter\def\csname v@main/dfn3/ami_test_long/leak\endcsname{24.37}
\expandafter\def\csname v@main/dfn3/ami_test_long/miss\endcsname{22.17}
\expandafter\def\csname v@main/dfn3/ami_test_long/wer\endcsname{41.77}
\expandafter\def\csname v@main/dfn3/call_test_clean/ins\endcsname{0.93}
\expandafter\def\csname v@main/dfn3/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/dfn3/call_test_clean/miss\endcsname{1.70}
\expandafter\def\csname v@main/dfn3/call_test_clean/wer\endcsname{2.63}
\expandafter\def\csname v@main/dfn3/call_test_mix/ins\endcsname{44.05}
\expandafter\def\csname v@main/dfn3/call_test_mix/leak\endcsname{113.04}
\expandafter\def\csname v@main/dfn3/call_test_mix/miss\endcsname{25.60}
\expandafter\def\csname v@main/dfn3/call_test_mix/wer\endcsname{69.65}
\expandafter\def\csname v@main/dfn3/krisp/ins\endcsname{6.18}
\expandafter\def\csname v@main/dfn3/krisp/leak\endcsname{20.34}
\expandafter\def\csname v@main/dfn3/krisp/miss\endcsname{6.96}
\expandafter\def\csname v@main/dfn3/krisp/wer\endcsname{13.15}
\expandafter\def\csname v@main/dfn3/nsf_test/ins\endcsname{9.14}
\expandafter\def\csname v@main/dfn3/nsf_test/leak\endcsname{26.09}
\expandafter\def\csname v@main/dfn3/nsf_test/miss\endcsname{6.23}
\expandafter\def\csname v@main/dfn3/nsf_test/wer\endcsname{15.38}
\expandafter\def\csname v@main/inworld/aic_calls/ins\endcsname{51.78}
\expandafter\def\csname v@main/inworld/aic_calls/leak\endcsname{77.60}
\expandafter\def\csname v@main/inworld/aic_calls/miss\endcsname{9.16}
\expandafter\def\csname v@main/inworld/aic_calls/wer\endcsname{60.94}
\expandafter\def\csname v@main/inworld/ali_test/ins\endcsname{3.72}
\expandafter\def\csname v@main/inworld/ali_test/leak\endcsname{15.33}
\expandafter\def\csname v@main/inworld/ali_test/miss\endcsname{14.32}
\expandafter\def\csname v@main/inworld/ali_test/wer\endcsname{18.03}
\expandafter\def\csname v@main/inworld/ami_headset2/ins\endcsname{9.57}
\expandafter\def\csname v@main/inworld/ami_headset2/leak\endcsname{25.58}
\expandafter\def\csname v@main/inworld/ami_headset2/miss\endcsname{8.22}
\expandafter\def\csname v@main/inworld/ami_headset2/wer\endcsname{17.80}
\expandafter\def\csname v@main/inworld/ami_test/ins\endcsname{22.51}
\expandafter\def\csname v@main/inworld/ami_test/leak\endcsname{72.02}
\expandafter\def\csname v@main/inworld/ami_test/miss\endcsname{7.77}
\expandafter\def\csname v@main/inworld/ami_test/wer\endcsname{30.28}
\expandafter\def\csname v@main/inworld/ami_test_long/ins\endcsname{88.39}
\expandafter\def\csname v@main/inworld/ami_test_long/leak\endcsname{113.69}
\expandafter\def\csname v@main/inworld/ami_test_long/miss\endcsname{10.81}
\expandafter\def\csname v@main/inworld/ami_test_long/wer\endcsname{99.21}
\expandafter\def\csname v@main/inworld/call_test_clean/ins\endcsname{1.01}
\expandafter\def\csname v@main/inworld/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/inworld/call_test_clean/miss\endcsname{1.62}
\expandafter\def\csname v@main/inworld/call_test_clean/wer\endcsname{2.63}
\expandafter\def\csname v@main/inworld/call_test_mix/ins\endcsname{49.13}
\expandafter\def\csname v@main/inworld/call_test_mix/leak\endcsname{113.35}
\expandafter\def\csname v@main/inworld/call_test_mix/miss\endcsname{19.15}
\expandafter\def\csname v@main/inworld/call_test_mix/wer\endcsname{68.28}
\expandafter\def\csname v@main/inworld/krisp/ins\endcsname{17.77}
\expandafter\def\csname v@main/inworld/krisp/leak\endcsname{63.82}
\expandafter\def\csname v@main/inworld/krisp/miss\endcsname{4.54}
\expandafter\def\csname v@main/inworld/krisp/wer\endcsname{22.31}
\expandafter\def\csname v@main/inworld/nsf_test/ins\endcsname{13.92}
\expandafter\def\csname v@main/inworld/nsf_test/leak\endcsname{43.23}
\expandafter\def\csname v@main/inworld/nsf_test/miss\endcsname{5.99}
\expandafter\def\csname v@main/inworld/nsf_test/wer\endcsname{19.90}
\expandafter\def\csname v@main/inworld_rt/aic_calls/ins\endcsname{51.53}
\expandafter\def\csname v@main/inworld_rt/aic_calls/leak\endcsname{77.29}
\expandafter\def\csname v@main/inworld_rt/aic_calls/miss\endcsname{9.16}
\expandafter\def\csname v@main/inworld_rt/aic_calls/wer\endcsname{60.69}
\expandafter\def\csname v@main/inworld_rt/ali_test/ins\endcsname{4.46}
\expandafter\def\csname v@main/inworld_rt/ali_test/leak\endcsname{18.47}
\expandafter\def\csname v@main/inworld_rt/ali_test/miss\endcsname{14.49}
\expandafter\def\csname v@main/inworld_rt/ali_test/wer\endcsname{18.94}
\expandafter\def\csname v@main/inworld_rt/ami_headset2/ins\endcsname{12.30}
\expandafter\def\csname v@main/inworld_rt/ami_headset2/leak\endcsname{35.39}
\expandafter\def\csname v@main/inworld_rt/ami_headset2/miss\endcsname{9.09}
\expandafter\def\csname v@main/inworld_rt/ami_headset2/wer\endcsname{21.39}
\expandafter\def\csname v@main/inworld_rt/ami_test/ins\endcsname{22.06}
\expandafter\def\csname v@main/inworld_rt/ami_test/leak\endcsname{71.21}
\expandafter\def\csname v@main/inworld_rt/ami_test/miss\endcsname{8.00}
\expandafter\def\csname v@main/inworld_rt/ami_test/wer\endcsname{30.06}
\expandafter\def\csname v@main/inworld_rt/ami_test_long/ins\endcsname{91.66}
\expandafter\def\csname v@main/inworld_rt/ami_test_long/leak\endcsname{118.49}
\expandafter\def\csname v@main/inworld_rt/ami_test_long/miss\endcsname{10.85}
\expandafter\def\csname v@main/inworld_rt/ami_test_long/wer\endcsname{102.51}
\expandafter\def\csname v@main/inworld_rt/call_test_clean/ins\endcsname{0.86}
\expandafter\def\csname v@main/inworld_rt/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/inworld_rt/call_test_clean/miss\endcsname{1.21}
\expandafter\def\csname v@main/inworld_rt/call_test_clean/wer\endcsname{2.07}
\expandafter\def\csname v@main/inworld_rt/call_test_mix/ins\endcsname{48.68}
\expandafter\def\csname v@main/inworld_rt/call_test_mix/leak\endcsname{114.74}
\expandafter\def\csname v@main/inworld_rt/call_test_mix/miss\endcsname{20.34}
\expandafter\def\csname v@main/inworld_rt/call_test_mix/wer\endcsname{69.02}
\expandafter\def\csname v@main/inworld_rt/krisp/ins\endcsname{18.09}
\expandafter\def\csname v@main/inworld_rt/krisp/leak\endcsname{64.19}
\expandafter\def\csname v@main/inworld_rt/krisp/miss\endcsname{4.15}
\expandafter\def\csname v@main/inworld_rt/krisp/wer\endcsname{22.24}
\expandafter\def\csname v@main/inworld_rt/nsf_test/ins\endcsname{16.08}
\expandafter\def\csname v@main/inworld_rt/nsf_test/leak\endcsname{52.06}
\expandafter\def\csname v@main/inworld_rt/nsf_test/miss\endcsname{6.32}
\expandafter\def\csname v@main/inworld_rt/nsf_test/wer\endcsname{22.41}
\expandafter\def\csname v@main/krisp_default/krisp/ins\endcsname{1.09}
\expandafter\def\csname v@main/krisp_default/krisp/leak\endcsname{1.52}
\expandafter\def\csname v@main/krisp_default/krisp/miss\endcsname{4.21}
\expandafter\def\csname v@main/krisp_default/krisp/wer\endcsname{5.30}
\expandafter\def\csname v@main/pre_selfl/aic_calls/ins\endcsname{7.84}
\expandafter\def\csname v@main/pre_selfl/aic_calls/leak\endcsname{7.95}
\expandafter\def\csname v@main/pre_selfl/aic_calls/miss\endcsname{6.52}
\expandafter\def\csname v@main/pre_selfl/aic_calls/wer\endcsname{14.36}
\expandafter\def\csname v@main/pre_selfl/ali_test/ins\endcsname{1.13}
\expandafter\def\csname v@main/pre_selfl/ali_test/leak\endcsname{1.79}
\expandafter\def\csname v@main/pre_selfl/ali_test/miss\endcsname{14.63}
\expandafter\def\csname v@main/pre_selfl/ali_test/wer\endcsname{15.75}
\expandafter\def\csname v@main/pre_selfl/ami_headset2/ins\endcsname{3.21}
\expandafter\def\csname v@main/pre_selfl/ami_headset2/leak\endcsname{2.12}
\expandafter\def\csname v@main/pre_selfl/ami_headset2/miss\endcsname{6.84}
\expandafter\def\csname v@main/pre_selfl/ami_headset2/wer\endcsname{10.06}
\expandafter\def\csname v@main/pre_selfl/ami_test/ins\endcsname{2.40}
\expandafter\def\csname v@main/pre_selfl/ami_test/leak\endcsname{1.73}
\expandafter\def\csname v@main/pre_selfl/ami_test/miss\endcsname{7.58}
\expandafter\def\csname v@main/pre_selfl/ami_test/wer\endcsname{9.97}
\expandafter\def\csname v@main/pre_selfl/ami_test_long/ins\endcsname{4.19}
\expandafter\def\csname v@main/pre_selfl/ami_test_long/leak\endcsname{3.78}
\expandafter\def\csname v@main/pre_selfl/ami_test_long/miss\endcsname{11.73}
\expandafter\def\csname v@main/pre_selfl/ami_test_long/wer\endcsname{15.91}
\expandafter\def\csname v@main/pre_selfl/call_test_clean/ins\endcsname{0.88}
\expandafter\def\csname v@main/pre_selfl/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/pre_selfl/call_test_clean/miss\endcsname{6.39}
\expandafter\def\csname v@main/pre_selfl/call_test_clean/wer\endcsname{7.27}
\expandafter\def\csname v@main/pre_selfl/call_test_mix/ins\endcsname{21.52}
\expandafter\def\csname v@main/pre_selfl/call_test_mix/leak\endcsname{57.40}
\expandafter\def\csname v@main/pre_selfl/call_test_mix/miss\endcsname{26.85}
\expandafter\def\csname v@main/pre_selfl/call_test_mix/wer\endcsname{48.36}
\expandafter\def\csname v@main/pre_selfl/krisp/ins\endcsname{0.71}
\expandafter\def\csname v@main/pre_selfl/krisp/leak\endcsname{0.11}
\expandafter\def\csname v@main/pre_selfl/krisp/miss\endcsname{4.84}
\expandafter\def\csname v@main/pre_selfl/krisp/wer\endcsname{5.55}
\expandafter\def\csname v@main/pre_selfl/nsf_test/ins\endcsname{1.92}
\expandafter\def\csname v@main/pre_selfl/nsf_test/leak\endcsname{0.53}
\expandafter\def\csname v@main/pre_selfl/nsf_test/miss\endcsname{5.84}
\expandafter\def\csname v@main/pre_selfl/nsf_test/wer\endcsname{7.76}
\expandafter\def\csname v@main/raw/aic_calls/ins\endcsname{57.59}
\expandafter\def\csname v@main/raw/aic_calls/leak\endcsname{86.75}
\expandafter\def\csname v@main/raw/aic_calls/miss\endcsname{8.77}
\expandafter\def\csname v@main/raw/aic_calls/wer\endcsname{66.36}
\expandafter\def\csname v@main/raw/ali_test/ins\endcsname{14.28}
\expandafter\def\csname v@main/raw/ali_test/leak\endcsname{61.12}
\expandafter\def\csname v@main/raw/ali_test/miss\endcsname{15.12}
\expandafter\def\csname v@main/raw/ali_test/wer\endcsname{29.40}
\expandafter\def\csname v@main/raw/ami_headset2/ins\endcsname{24.95}
\expandafter\def\csname v@main/raw/ami_headset2/leak\endcsname{78.20}
\expandafter\def\csname v@main/raw/ami_headset2/miss\endcsname{8.05}
\expandafter\def\csname v@main/raw/ami_headset2/wer\endcsname{33.00}
\expandafter\def\csname v@main/raw/ami_test/ins\endcsname{32.84}
\expandafter\def\csname v@main/raw/ami_test/leak\endcsname{101.40}
\expandafter\def\csname v@main/raw/ami_test/miss\endcsname{9.75}
\expandafter\def\csname v@main/raw/ami_test/wer\endcsname{42.59}
\expandafter\def\csname v@main/raw/ami_test_long/ins\endcsname{108.71}
\expandafter\def\csname v@main/raw/ami_test_long/leak\endcsname{137.17}
\expandafter\def\csname v@main/raw/ami_test_long/miss\endcsname{13.08}
\expandafter\def\csname v@main/raw/ami_test_long/wer\endcsname{121.79}
\expandafter\def\csname v@main/raw/call_test_clean/ins\endcsname{0.00}
\expandafter\def\csname v@main/raw/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/raw/call_test_clean/miss\endcsname{0.04}
\expandafter\def\csname v@main/raw/call_test_clean/wer\endcsname{0.04}
\expandafter\def\csname v@main/raw/call_test_mix/ins\endcsname{47.27}
\expandafter\def\csname v@main/raw/call_test_mix/leak\endcsname{113.61}
\expandafter\def\csname v@main/raw/call_test_mix/miss\endcsname{22.52}
\expandafter\def\csname v@main/raw/call_test_mix/wer\endcsname{69.79}
\expandafter\def\csname v@main/raw/krisp/ins\endcsname{18.92}
\expandafter\def\csname v@main/raw/krisp/leak\endcsname{66.44}
\expandafter\def\csname v@main/raw/krisp/miss\endcsname{4.27}
\expandafter\def\csname v@main/raw/krisp/wer\endcsname{23.19}
\expandafter\def\csname v@main/raw/nsf_test/ins\endcsname{27.86}
\expandafter\def\csname v@main/raw/nsf_test/leak\endcsname{90.90}
\expandafter\def\csname v@main/raw/nsf_test/miss\endcsname{6.84}
\expandafter\def\csname v@main/raw/nsf_test/wer\endcsname{34.70}
\expandafter\def\csname v@main/rel-pre/aic_calls/diff\endcsname{-0.11}
\expandafter\def\csname v@main/rel-pre/aic_calls/hi\endcsname{+2.30}
\expandafter\def\csname v@main/rel-pre/aic_calls/lo\endcsname{-14.89}
\expandafter\def\csname v@main/rel-pre/ali_test/diff\endcsname{-0.07}
\expandafter\def\csname v@main/rel-pre/ali_test/hi\endcsname{+0.32}
\expandafter\def\csname v@main/rel-pre/ali_test/lo\endcsname{-0.52}
\expandafter\def\csname v@main/rel-pre/ami_headset2/diff\endcsname{+0.14}
\expandafter\def\csname v@main/rel-pre/ami_headset2/hi\endcsname{+0.59}
\expandafter\def\csname v@main/rel-pre/ami_headset2/lo\endcsname{-0.32}
\expandafter\def\csname v@main/rel-pre/ami_test/diff\endcsname{+0.21}
\expandafter\def\csname v@main/rel-pre/ami_test/hi\endcsname{+0.54}
\expandafter\def\csname v@main/rel-pre/ami_test/lo\endcsname{-0.12}
\expandafter\def\csname v@main/rel-pre/ami_test_long/diff\endcsname{+0.22}
\expandafter\def\csname v@main/rel-pre/ami_test_long/hi\endcsname{+1.05}
\expandafter\def\csname v@main/rel-pre/ami_test_long/lo\endcsname{-0.61}
\expandafter\def\csname v@main/rel-pre/call_test_clean/diff\endcsname{-1.70}
\expandafter\def\csname v@main/rel-pre/call_test_clean/hi\endcsname{-0.59}
\expandafter\def\csname v@main/rel-pre/call_test_clean/lo\endcsname{-2.87}
\expandafter\def\csname v@main/rel-pre/call_test_mix/diff\endcsname{-0.85}
\expandafter\def\csname v@main/rel-pre/call_test_mix/hi\endcsname{+1.18}
\expandafter\def\csname v@main/rel-pre/call_test_mix/lo\endcsname{-3.04}
\expandafter\def\csname v@main/rel-pre/krisp/diff\endcsname{+0.19}
\expandafter\def\csname v@main/rel-pre/krisp/hi\endcsname{+0.71}
\expandafter\def\csname v@main/rel-pre/krisp/lo\endcsname{-0.22}
\expandafter\def\csname v@main/rel-pre/meet-max\endcsname{0.22}
\expandafter\def\csname v@main/rel-pre/nsf_test/diff\endcsname{-0.09}
\expandafter\def\csname v@main/rel-pre/nsf_test/hi\endcsname{+0.09}
\expandafter\def\csname v@main/rel-pre/nsf_test/lo\endcsname{-0.32}
\expandafter\def\csname v@main/rel_loud/aic_calls/ins\endcsname{7.06}
\expandafter\def\csname v@main/rel_loud/aic_calls/leak\endcsname{5.30}
\expandafter\def\csname v@main/rel_loud/aic_calls/miss\endcsname{5.49}
\expandafter\def\csname v@main/rel_loud/aic_calls/wer\endcsname{12.54}
\expandafter\def\csname v@main/rel_loud/ali_test/ins\endcsname{1.15}
\expandafter\def\csname v@main/rel_loud/ali_test/leak\endcsname{1.88}
\expandafter\def\csname v@main/rel_loud/ali_test/miss\endcsname{14.25}
\expandafter\def\csname v@main/rel_loud/ali_test/wer\endcsname{15.40}
\expandafter\def\csname v@main/rel_loud/ami_headset2/ins\endcsname{3.39}
\expandafter\def\csname v@main/rel_loud/ami_headset2/leak\endcsname{2.25}
\expandafter\def\csname v@main/rel_loud/ami_headset2/miss\endcsname{7.98}
\expandafter\def\csname v@main/rel_loud/ami_headset2/wer\endcsname{11.37}
\expandafter\def\csname v@main/rel_loud/ami_test/ins\endcsname{2.51}
\expandafter\def\csname v@main/rel_loud/ami_test/leak\endcsname{1.90}
\expandafter\def\csname v@main/rel_loud/ami_test/miss\endcsname{7.83}
\expandafter\def\csname v@main/rel_loud/ami_test/wer\endcsname{10.35}
\expandafter\def\csname v@main/rel_loud/ami_test_long/ins\endcsname{4.39}
\expandafter\def\csname v@main/rel_loud/ami_test_long/leak\endcsname{3.91}
\expandafter\def\csname v@main/rel_loud/ami_test_long/miss\endcsname{11.82}
\expandafter\def\csname v@main/rel_loud/ami_test_long/wer\endcsname{16.22}
\expandafter\def\csname v@main/rel_loud/call_test_clean/ins\endcsname{1.09}
\expandafter\def\csname v@main/rel_loud/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/rel_loud/call_test_clean/miss\endcsname{4.57}
\expandafter\def\csname v@main/rel_loud/call_test_clean/wer\endcsname{5.66}
\expandafter\def\csname v@main/rel_loud/call_test_mix/ins\endcsname{21.49}
\expandafter\def\csname v@main/rel_loud/call_test_mix/leak\endcsname{58.84}
\expandafter\def\csname v@main/rel_loud/call_test_mix/miss\endcsname{26.38}
\expandafter\def\csname v@main/rel_loud/call_test_mix/wer\endcsname{47.87}
\expandafter\def\csname v@main/rel_loud/krisp/ins\endcsname{0.67}
\expandafter\def\csname v@main/rel_loud/krisp/leak\endcsname{0.05}
\expandafter\def\csname v@main/rel_loud/krisp/miss\endcsname{5.26}
\expandafter\def\csname v@main/rel_loud/krisp/wer\endcsname{5.93}
\expandafter\def\csname v@main/rel_loud/nsf_test/ins\endcsname{1.89}
\expandafter\def\csname v@main/rel_loud/nsf_test/leak\endcsname{0.47}
\expandafter\def\csname v@main/rel_loud/nsf_test/miss\endcsname{5.79}
\expandafter\def\csname v@main/rel_loud/nsf_test/wer\endcsname{7.67}
\expandafter\def\csname v@main/rel_null/aic_calls/ins\endcsname{8.27}
\expandafter\def\csname v@main/rel_null/aic_calls/leak\endcsname{8.45}
\expandafter\def\csname v@main/rel_null/aic_calls/miss\endcsname{6.20}
\expandafter\def\csname v@main/rel_null/aic_calls/wer\endcsname{14.47}
\expandafter\def\csname v@main/rel_null/ali_test/ins\endcsname{1.25}
\expandafter\def\csname v@main/rel_null/ali_test/leak\endcsname{1.93}
\expandafter\def\csname v@main/rel_null/ali_test/miss\endcsname{14.49}
\expandafter\def\csname v@main/rel_null/ali_test/wer\endcsname{15.74}
\expandafter\def\csname v@main/rel_null/ami_headset2/ins\endcsname{3.32}
\expandafter\def\csname v@main/rel_null/ami_headset2/leak\endcsname{2.25}
\expandafter\def\csname v@main/rel_null/ami_headset2/miss\endcsname{6.70}
\expandafter\def\csname v@main/rel_null/ami_headset2/wer\endcsname{10.02}
\expandafter\def\csname v@main/rel_null/ami_test/ins\endcsname{2.55}
\expandafter\def\csname v@main/rel_null/ami_test/leak\endcsname{1.90}
\expandafter\def\csname v@main/rel_null/ami_test/miss\endcsname{7.54}
\expandafter\def\csname v@main/rel_null/ami_test/wer\endcsname{10.09}
\expandafter\def\csname v@main/rel_null/ami_test_long/ins\endcsname{5.09}
\expandafter\def\csname v@main/rel_null/ami_test_long/leak\endcsname{5.34}
\expandafter\def\csname v@main/rel_null/ami_test_long/miss\endcsname{11.10}
\expandafter\def\csname v@main/rel_null/ami_test_long/wer\endcsname{16.19}
\expandafter\def\csname v@main/rel_null/call_test_clean/ins\endcsname{1.08}
\expandafter\def\csname v@main/rel_null/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/rel_null/call_test_clean/miss\endcsname{4.82}
\expandafter\def\csname v@main/rel_null/call_test_clean/wer\endcsname{5.90}
\expandafter\def\csname v@main/rel_null/call_test_mix/ins\endcsname{22.28}
\expandafter\def\csname v@main/rel_null/call_test_mix/leak\endcsname{58.02}
\expandafter\def\csname v@main/rel_null/call_test_mix/miss\endcsname{25.15}
\expandafter\def\csname v@main/rel_null/call_test_mix/wer\endcsname{47.43}
\expandafter\def\csname v@main/rel_null/krisp/ins\endcsname{1.14}
\expandafter\def\csname v@main/rel_null/krisp/leak\endcsname{1.80}
\expandafter\def\csname v@main/rel_null/krisp/miss\endcsname{5.14}
\expandafter\def\csname v@main/rel_null/krisp/wer\endcsname{6.28}
\expandafter\def\csname v@main/rel_null/nsf_test/ins\endcsname{1.91}
\expandafter\def\csname v@main/rel_null/nsf_test/leak\endcsname{0.49}
\expandafter\def\csname v@main/rel_null/nsf_test/miss\endcsname{5.82}
\expandafter\def\csname v@main/rel_null/nsf_test/wer\endcsname{7.74}
\expandafter\def\csname v@main/rel_selfl/aic_calls/ins\endcsname{8.52}
\expandafter\def\csname v@main/rel_selfl/aic_calls/leak\endcsname{8.39}
\expandafter\def\csname v@main/rel_selfl/aic_calls/miss\endcsname{5.74}
\expandafter\def\csname v@main/rel_selfl/aic_calls/wer\endcsname{14.26}
\expandafter\def\csname v@main/rel_selfl/ali_test/ins\endcsname{1.21}
\expandafter\def\csname v@main/rel_selfl/ali_test/leak\endcsname{1.79}
\expandafter\def\csname v@main/rel_selfl/ali_test/miss\endcsname{14.47}
\expandafter\def\csname v@main/rel_selfl/ali_test/wer\endcsname{15.69}
\expandafter\def\csname v@main/rel_selfl/ami_headset2/ins\endcsname{3.46}
\expandafter\def\csname v@main/rel_selfl/ami_headset2/leak\endcsname{2.39}
\expandafter\def\csname v@main/rel_selfl/ami_headset2/miss\endcsname{6.74}
\expandafter\def\csname v@main/rel_selfl/ami_headset2/wer\endcsname{10.19}
\expandafter\def\csname v@main/rel_selfl/ami_test/ins\endcsname{2.67}
\expandafter\def\csname v@main/rel_selfl/ami_test/leak\endcsname{1.90}
\expandafter\def\csname v@main/rel_selfl/ami_test/miss\endcsname{7.51}
\expandafter\def\csname v@main/rel_selfl/ami_test/wer\endcsname{10.18}
\expandafter\def\csname v@main/rel_selfl/ami_test_long/ins\endcsname{4.58}
\expandafter\def\csname v@main/rel_selfl/ami_test_long/leak\endcsname{4.11}
\expandafter\def\csname v@main/rel_selfl/ami_test_long/miss\endcsname{11.55}
\expandafter\def\csname v@main/rel_selfl/ami_test_long/wer\endcsname{16.13}
\expandafter\def\csname v@main/rel_selfl/call_test_clean/ins\endcsname{0.99}
\expandafter\def\csname v@main/rel_selfl/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/rel_selfl/call_test_clean/miss\endcsname{4.58}
\expandafter\def\csname v@main/rel_selfl/call_test_clean/wer\endcsname{5.58}
\expandafter\def\csname v@main/rel_selfl/call_test_mix/ins\endcsname{20.12}
\expandafter\def\csname v@main/rel_selfl/call_test_mix/leak\endcsname{56.88}
\expandafter\def\csname v@main/rel_selfl/call_test_mix/miss\endcsname{27.39}
\expandafter\def\csname v@main/rel_selfl/call_test_mix/wer\endcsname{47.52}
\expandafter\def\csname v@main/rel_selfl/krisp/ins\endcsname{0.67}
\expandafter\def\csname v@main/rel_selfl/krisp/leak\endcsname{0.04}
\expandafter\def\csname v@main/rel_selfl/krisp/miss\endcsname{5.08}
\expandafter\def\csname v@main/rel_selfl/krisp/wer\endcsname{5.74}
\expandafter\def\csname v@main/rel_selfl/nsf_test/ins\endcsname{1.91}
\expandafter\def\csname v@main/rel_selfl/nsf_test/leak\endcsname{0.38}
\expandafter\def\csname v@main/rel_selfl/nsf_test/miss\endcsname{5.76}
\expandafter\def\csname v@main/rel_selfl/nsf_test/wer\endcsname{7.67}
\expandafter\def\csname v@main/sidon_vi/ali_test/ins\endcsname{26.12}
\expandafter\def\csname v@main/sidon_vi/ali_test/leak\endcsname{124.03}
\expandafter\def\csname v@main/sidon_vi/ali_test/miss\endcsname{16.82}
\expandafter\def\csname v@main/sidon_vi/ali_test/wer\endcsname{42.94}
\expandafter\def\csname v@main/sidon_vi/ami_headset2/ins\endcsname{23.43}
\expandafter\def\csname v@main/sidon_vi/ami_headset2/leak\endcsname{79.39}
\expandafter\def\csname v@main/sidon_vi/ami_headset2/miss\endcsname{9.02}
\expandafter\def\csname v@main/sidon_vi/ami_headset2/wer\endcsname{32.45}
\expandafter\def\csname v@main/sidon_vi/ami_test/ins\endcsname{29.04}
\expandafter\def\csname v@main/sidon_vi/ami_test/leak\endcsname{98.03}
\expandafter\def\csname v@main/sidon_vi/ami_test/miss\endcsname{8.47}
\expandafter\def\csname v@main/sidon_vi/ami_test/wer\endcsname{37.51}
\expandafter\def\csname v@main/sidon_vi/ami_test_long/ins\endcsname{91.76}
\expandafter\def\csname v@main/sidon_vi/ami_test_long/leak\endcsname{118.92}
\expandafter\def\csname v@main/sidon_vi/ami_test_long/miss\endcsname{10.04}
\expandafter\def\csname v@main/sidon_vi/ami_test_long/wer\endcsname{101.80}
\expandafter\def\csname v@main/sidon_vi/krisp/ins\endcsname{25.45}
\expandafter\def\csname v@main/sidon_vi/krisp/leak\endcsname{91.02}
\expandafter\def\csname v@main/sidon_vi/krisp/miss\endcsname{4.04}
\expandafter\def\csname v@main/sidon_vi/krisp/wer\endcsname{29.49}
\expandafter\def\csname v@main/sidon_vi/nsf_test/ins\endcsname{23.20}
\expandafter\def\csname v@main/sidon_vi/nsf_test/leak\endcsname{76.82}
\expandafter\def\csname v@main/sidon_vi/nsf_test/miss\endcsname{6.81}
\expandafter\def\csname v@main/sidon_vi/nsf_test/wer\endcsname{30.01}
\expandafter\def\csname v@main/sidon_vi_lite/ali_test/ins\endcsname{3.56}
\expandafter\def\csname v@main/sidon_vi_lite/ali_test/leak\endcsname{9.25}
\expandafter\def\csname v@main/sidon_vi_lite/ali_test/miss\endcsname{15.75}
\expandafter\def\csname v@main/sidon_vi_lite/ali_test/wer\endcsname{19.31}
\expandafter\def\csname v@main/sidon_vi_lite/ami_headset2/ins\endcsname{8.43}
\expandafter\def\csname v@main/sidon_vi_lite/ami_headset2/leak\endcsname{21.07}
\expandafter\def\csname v@main/sidon_vi_lite/ami_headset2/miss\endcsname{9.02}
\expandafter\def\csname v@main/sidon_vi_lite/ami_headset2/wer\endcsname{17.45}
\expandafter\def\csname v@main/sidon_vi_lite/ami_test/ins\endcsname{15.81}
\expandafter\def\csname v@main/sidon_vi_lite/ami_test/leak\endcsname{49.26}
\expandafter\def\csname v@main/sidon_vi_lite/ami_test/miss\endcsname{8.26}
\expandafter\def\csname v@main/sidon_vi_lite/ami_test/wer\endcsname{24.06}
\expandafter\def\csname v@main/sidon_vi_lite/ami_test_long/ins\endcsname{53.46}
\expandafter\def\csname v@main/sidon_vi_lite/ami_test_long/leak\endcsname{70.88}
\expandafter\def\csname v@main/sidon_vi_lite/ami_test_long/miss\endcsname{12.69}
\expandafter\def\csname v@main/sidon_vi_lite/ami_test_long/wer\endcsname{66.15}
\expandafter\def\csname v@main/sidon_vi_lite/krisp/ins\endcsname{12.05}
\expandafter\def\csname v@main/sidon_vi_lite/krisp/leak\endcsname{42.50}
\expandafter\def\csname v@main/sidon_vi_lite/krisp/miss\endcsname{6.22}
\expandafter\def\csname v@main/sidon_vi_lite/krisp/wer\endcsname{18.27}
\expandafter\def\csname v@main/sidon_vi_lite/nsf_test/ins\endcsname{7.36}
\expandafter\def\csname v@main/sidon_vi_lite/nsf_test/leak\endcsname{20.65}
\expandafter\def\csname v@main/sidon_vi_lite/nsf_test/miss\endcsname{6.04}
\expandafter\def\csname v@main/sidon_vi_lite/nsf_test/wer\endcsname{13.40}
\expandafter\def\csname v@main/voxlock/aic_calls/ins\endcsname{13.83}
\expandafter\def\csname v@main/voxlock/aic_calls/leak\endcsname{18.04}
\expandafter\def\csname v@main/voxlock/aic_calls/miss\endcsname{6.49}
\expandafter\def\csname v@main/voxlock/aic_calls/wer\endcsname{20.31}
\expandafter\def\csname v@main/voxlock/ali_test/ins\endcsname{1.97}
\expandafter\def\csname v@main/voxlock/ali_test/leak\endcsname{1.21}
\expandafter\def\csname v@main/voxlock/ali_test/miss\endcsname{15.15}
\expandafter\def\csname v@main/voxlock/ali_test/wer\endcsname{17.11}
\expandafter\def\csname v@main/voxlock/ami_headset2/ins\endcsname{3.14}
\expandafter\def\csname v@main/voxlock/ami_headset2/leak\endcsname{2.65}
\expandafter\def\csname v@main/voxlock/ami_headset2/miss\endcsname{8.12}
\expandafter\def\csname v@main/voxlock/ami_headset2/wer\endcsname{11.26}
\expandafter\def\csname v@main/voxlock/ami_test/ins\endcsname{2.17}
\expandafter\def\csname v@main/voxlock/ami_test/leak\endcsname{1.20}
\expandafter\def\csname v@main/voxlock/ami_test/miss\endcsname{7.53}
\expandafter\def\csname v@main/voxlock/ami_test/wer\endcsname{9.70}
\expandafter\def\csname v@main/voxlock/ami_test_long/ins\endcsname{3.57}
\expandafter\def\csname v@main/voxlock/ami_test_long/leak\endcsname{3.73}
\expandafter\def\csname v@main/voxlock/ami_test_long/miss\endcsname{15.95}
\expandafter\def\csname v@main/voxlock/ami_test_long/wer\endcsname{19.52}
\expandafter\def\csname v@main/voxlock/call_test_clean/ins\endcsname{0.59}
\expandafter\def\csname v@main/voxlock/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/voxlock/call_test_clean/miss\endcsname{2.78}
\expandafter\def\csname v@main/voxlock/call_test_clean/wer\endcsname{3.37}
\expandafter\def\csname v@main/voxlock/call_test_mix/ins\endcsname{23.52}
\expandafter\def\csname v@main/voxlock/call_test_mix/leak\endcsname{61.67}
\expandafter\def\csname v@main/voxlock/call_test_mix/miss\endcsname{23.54}
\expandafter\def\csname v@main/voxlock/call_test_mix/wer\endcsname{47.05}
\expandafter\def\csname v@main/voxlock/krisp/ins\endcsname{0.72}
\expandafter\def\csname v@main/voxlock/krisp/leak\endcsname{0.07}
\expandafter\def\csname v@main/voxlock/krisp/miss\endcsname{4.46}
\expandafter\def\csname v@main/voxlock/krisp/wer\endcsname{5.19}
\expandafter\def\csname v@main/voxlock/nsf_test/ins\endcsname{1.84}
\expandafter\def\csname v@main/voxlock/nsf_test/leak\endcsname{0.68}
\expandafter\def\csname v@main/voxlock/nsf_test/miss\endcsname{5.77}
\expandafter\def\csname v@main/voxlock/nsf_test/wer\endcsname{7.61}
\expandafter\def\csname v@main/voxlock_live/aic_calls/ins\endcsname{17.03}
\expandafter\def\csname v@main/voxlock_live/aic_calls/leak\endcsname{24.80}
\expandafter\def\csname v@main/voxlock_live/aic_calls/miss\endcsname{7.52}
\expandafter\def\csname v@main/voxlock_live/aic_calls/wer\endcsname{24.55}
\expandafter\def\csname v@main/voxlock_live/ali_test/ins\endcsname{1.01}
\expandafter\def\csname v@main/voxlock_live/ali_test/leak\endcsname{1.37}
\expandafter\def\csname v@main/voxlock_live/ali_test/miss\endcsname{15.27}
\expandafter\def\csname v@main/voxlock_live/ali_test/wer\endcsname{16.28}
\expandafter\def\csname v@main/voxlock_live/ami_headset2/ins\endcsname{3.73}
\expandafter\def\csname v@main/voxlock_live/ami_headset2/leak\endcsname{3.05}
\expandafter\def\csname v@main/voxlock_live/ami_headset2/miss\endcsname{7.98}
\expandafter\def\csname v@main/voxlock_live/ami_headset2/wer\endcsname{11.71}
\expandafter\def\csname v@main/voxlock_live/ami_test/ins\endcsname{3.69}
\expandafter\def\csname v@main/voxlock_live/ami_test/leak\endcsname{3.80}
\expandafter\def\csname v@main/voxlock_live/ami_test/miss\endcsname{8.39}
\expandafter\def\csname v@main/voxlock_live/ami_test/wer\endcsname{12.07}
\expandafter\def\csname v@main/voxlock_live/ami_test_long/ins\endcsname{7.66}
\expandafter\def\csname v@main/voxlock_live/ami_test_long/leak\endcsname{9.11}
\expandafter\def\csname v@main/voxlock_live/ami_test_long/miss\endcsname{16.00}
\expandafter\def\csname v@main/voxlock_live/ami_test_long/wer\endcsname{23.66}
\expandafter\def\csname v@main/voxlock_live/call_test_clean/ins\endcsname{0.73}
\expandafter\def\csname v@main/voxlock_live/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/voxlock_live/call_test_clean/miss\endcsname{2.19}
\expandafter\def\csname v@main/voxlock_live/call_test_clean/wer\endcsname{2.92}
\expandafter\def\csname v@main/voxlock_live/call_test_mix/ins\endcsname{27.24}
\expandafter\def\csname v@main/voxlock_live/call_test_mix/leak\endcsname{75.02}
\expandafter\def\csname v@main/voxlock_live/call_test_mix/miss\endcsname{29.42}
\expandafter\def\csname v@main/voxlock_live/call_test_mix/wer\endcsname{56.65}
\expandafter\def\csname v@main/voxlock_live/krisp/ins\endcsname{0.84}
\expandafter\def\csname v@main/voxlock_live/krisp/leak\endcsname{0.29}
\expandafter\def\csname v@main/voxlock_live/krisp/miss\endcsname{4.78}
\expandafter\def\csname v@main/voxlock_live/krisp/wer\endcsname{5.63}
\expandafter\def\csname v@main/voxlock_live/nsf_test/ins\endcsname{2.31}
\expandafter\def\csname v@main/voxlock_live/nsf_test/leak\endcsname{2.99}
\expandafter\def\csname v@main/voxlock_live/nsf_test/miss\endcsname{6.53}
\expandafter\def\csname v@main/voxlock_live/nsf_test/wer\endcsname{8.84}
\expandafter\def\csname v@main/voxlock_pt/aic_calls/ins\endcsname{13.86}
\expandafter\def\csname v@main/voxlock_pt/aic_calls/leak\endcsname{18.23}
\expandafter\def\csname v@main/voxlock_pt/aic_calls/miss\endcsname{6.63}
\expandafter\def\csname v@main/voxlock_pt/aic_calls/wer\endcsname{20.49}
\expandafter\def\csname v@main/voxlock_pt/ali_test/ins\endcsname{1.00}
\expandafter\def\csname v@main/voxlock_pt/ali_test/leak\endcsname{1.01}
\expandafter\def\csname v@main/voxlock_pt/ali_test/miss\endcsname{14.38}
\expandafter\def\csname v@main/voxlock_pt/ali_test/wer\endcsname{15.38}
\expandafter\def\csname v@main/voxlock_pt/ami_headset2/ins\endcsname{3.39}
\expandafter\def\csname v@main/voxlock_pt/ami_headset2/leak\endcsname{2.12}
\expandafter\def\csname v@main/voxlock_pt/ami_headset2/miss\endcsname{6.88}
\expandafter\def\csname v@main/voxlock_pt/ami_headset2/wer\endcsname{10.26}
\expandafter\def\csname v@main/voxlock_pt/ami_test/ins\endcsname{2.45}
\expandafter\def\csname v@main/voxlock_pt/ami_test/leak\endcsname{2.14}
\expandafter\def\csname v@main/voxlock_pt/ami_test/miss\endcsname{7.87}
\expandafter\def\csname v@main/voxlock_pt/ami_test/wer\endcsname{10.31}
\expandafter\def\csname v@main/voxlock_pt/ami_test_long/ins\endcsname{5.41}
\expandafter\def\csname v@main/voxlock_pt/ami_test_long/leak\endcsname{5.47}
\expandafter\def\csname v@main/voxlock_pt/ami_test_long/miss\endcsname{14.78}
\expandafter\def\csname v@main/voxlock_pt/ami_test_long/wer\endcsname{20.20}
\expandafter\def\csname v@main/voxlock_pt/call_test_clean/ins\endcsname{0.56}
\expandafter\def\csname v@main/voxlock_pt/call_test_clean/leak\endcsname{nan}
\expandafter\def\csname v@main/voxlock_pt/call_test_clean/miss\endcsname{2.32}
\expandafter\def\csname v@main/voxlock_pt/call_test_clean/wer\endcsname{2.87}
\expandafter\def\csname v@main/voxlock_pt/call_test_mix/ins\endcsname{25.15}
\expandafter\def\csname v@main/voxlock_pt/call_test_mix/leak\endcsname{65.33}
\expandafter\def\csname v@main/voxlock_pt/call_test_mix/miss\endcsname{23.44}
\expandafter\def\csname v@main/voxlock_pt/call_test_mix/wer\endcsname{48.59}
\expandafter\def\csname v@main/voxlock_pt/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@main/voxlock_pt/krisp/leak\endcsname{0.09}
\expandafter\def\csname v@main/voxlock_pt/krisp/miss\endcsname{4.25}
\expandafter\def\csname v@main/voxlock_pt/krisp/wer\endcsname{4.99}
\expandafter\def\csname v@main/voxlock_pt/nsf_test/ins\endcsname{1.94}
\expandafter\def\csname v@main/voxlock_pt/nsf_test/leak\endcsname{1.02}
\expandafter\def\csname v@main/voxlock_pt/nsf_test/miss\endcsname{5.84}
\expandafter\def\csname v@main/voxlock_pt/nsf_test/wer\endcsname{7.78}
\expandafter\def\csname v@model/L/gmac\endcsname{42.5}
\expandafter\def\csname v@model/L/gmacs\endcsname{42.5}
\expandafter\def\csname v@model/L/params\endcsname{374}
\expandafter\def\csname v@model/L/state-mb\endcsname{82}
\expandafter\def\csname v@model/LW/gmac\endcsname{61.6}
\expandafter\def\csname v@model/LW/params\endcsname{687}
\expandafter\def\csname v@model/LW/state-mb\endcsname{131}
\expandafter\def\csname v@model/M/gmac\endcsname{28.5}
\expandafter\def\csname v@model/M/gmacs\endcsname{28.5}
\expandafter\def\csname v@model/M/params\endcsname{243}
\expandafter\def\csname v@model/M/state-mb\endcsname{66}
\expandafter\def\csname v@model/MW/gmac\endcsname{47.7}
\expandafter\def\csname v@model/MW/params\endcsname{555}
\expandafter\def\csname v@model/MW/state-mb\endcsname{115}
\expandafter\def\csname v@model/S/gmac\endcsname{17.4}
\expandafter\def\csname v@model/S/gmacs\endcsname{17.4}
\expandafter\def\csname v@model/S/params\endcsname{140}
\expandafter\def\csname v@model/S/state-mb\endcsname{49}
\expandafter\def\csname v@model/SW/gmac\endcsname{36.5}
\expandafter\def\csname v@model/SW/params\endcsname{452}
\expandafter\def\csname v@model/SW/state-mb\endcsname{99}
\expandafter\def\csname v@model/enc/params\endcsname{0.87}
\expandafter\def\csname v@nine/C10n_ftlong_kd_selfl/wer\endcsname{15.46}
\expandafter\def\csname v@nine/C22_ftlong_kd_selfl/wer\endcsname{15.49}
\expandafter\def\csname v@nine/dfn3/wer\endcsname{27.11}
\expandafter\def\csname v@nine/inworld/wer\endcsname{37.71}
\expandafter\def\csname v@nine/inworld_rt/wer\endcsname{38.81}
\expandafter\def\csname v@nine/raw/wer\endcsname{46.76}
\expandafter\def\csname v@nine/rel_selfl/wer\endcsname{14.77}
\expandafter\def\csname v@nine/voxlock/wer\endcsname{15.68}
\expandafter\def\csname v@nine/voxlock_live/wer\endcsname{18.04}
\expandafter\def\csname v@nsf_dev/C22_ftlong_kd_selfl/dele\endcsname{1.47}
\expandafter\def\csname v@nsf_dev/C22_ftlong_kd_selfl/dleak\endcsname{+0.00}
\expandafter\def\csname v@nsf_dev/C22_ftlong_kd_selfl/dwer\endcsname{-0.58}
\expandafter\def\csname v@nsf_dev/C22_ftlong_kd_selfl/dwer-hi\endcsname{+0.02}
\expandafter\def\csname v@nsf_dev/C22_ftlong_kd_selfl/dwer-lo\endcsname{-1.50}
\expandafter\def\csname v@nsf_dev/C22_ftlong_kd_selfl/ins\endcsname{1.97}
\expandafter\def\csname v@nsf_dev/C22_ftlong_kd_selfl/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@nsf_dev/C22_ftlong_kd_selfl/miss\endcsname{5.73}
\expandafter\def\csname v@nsf_dev/C22_ftlong_kd_selfl/wer\endcsname{7.70}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_null/dele\endcsname{1.55}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{-0.13}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-0.51}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+0.07}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-1.40}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_null/ins\endcsname{1.93}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_null/miss\endcsname{5.84}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_null/wer\endcsname{7.77}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{1.56}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-0.21}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-0.51}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+0.07}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-1.41}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{1.90}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{5.87}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{7.77}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_loud/dele\endcsname{1.50}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_loud/dleak\endcsname{-0.13}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_loud/dwer\endcsname{-0.59}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_loud/dwer-hi\endcsname{-0.01}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_loud/dwer-lo\endcsname{-1.47}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_loud/ins\endcsname{1.85}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_loud/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_loud/miss\endcsname{5.84}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_loud/wer\endcsname{7.69}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_null/dele\endcsname{1.54}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_null/dleak\endcsname{-0.17}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_null/dwer\endcsname{-0.69}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_null/dwer-hi\endcsname{-0.09}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_null/dwer-lo\endcsname{-1.58}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_null/ins\endcsname{1.85}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_null/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_null/miss\endcsname{5.75}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_null/wer\endcsname{7.59}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_selfl/dele\endcsname{1.49}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_selfl/dleak\endcsname{-0.13}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_selfl/dwer\endcsname{-0.72}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_selfl/dwer-hi\endcsname{-0.14}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_selfl/dwer-lo\endcsname{-1.61}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_selfl/ins\endcsname{1.83}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_selfl/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_selfl/miss\endcsname{5.73}
\expandafter\def\csname v@nsf_dev/MB_ftlong_ws_selfl/wer\endcsname{7.56}
\expandafter\def\csname v@nsf_dev/SB_ftlong_ws_selfl/dele\endcsname{1.61}
\expandafter\def\csname v@nsf_dev/SB_ftlong_ws_selfl/dleak\endcsname{-0.21}
\expandafter\def\csname v@nsf_dev/SB_ftlong_ws_selfl/dwer\endcsname{-0.65}
\expandafter\def\csname v@nsf_dev/SB_ftlong_ws_selfl/dwer-hi\endcsname{-0.05}
\expandafter\def\csname v@nsf_dev/SB_ftlong_ws_selfl/dwer-lo\endcsname{-1.56}
\expandafter\def\csname v@nsf_dev/SB_ftlong_ws_selfl/ins\endcsname{1.87}
\expandafter\def\csname v@nsf_dev/SB_ftlong_ws_selfl/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@nsf_dev/SB_ftlong_ws_selfl/miss\endcsname{5.76}
\expandafter\def\csname v@nsf_dev/SB_ftlong_ws_selfl/wer\endcsname{7.63}
\expandafter\def\csname v@nsf_dev/dfn3/dele\endcsname{1.87}
\expandafter\def\csname v@nsf_dev/dfn3/dleak\endcsname{+27.86}
\expandafter\def\csname v@nsf_dev/dfn3/dwer\endcsname{+7.72}
\expandafter\def\csname v@nsf_dev/dfn3/dwer-hi\endcsname{+10.02}
\expandafter\def\csname v@nsf_dev/dfn3/dwer-lo\endcsname{+5.62}
\expandafter\def\csname v@nsf_dev/dfn3/ins\endcsname{9.90}
\expandafter\def\csname v@nsf_dev/dfn3/leak_wpm\endcsname{28.50}
\expandafter\def\csname v@nsf_dev/dfn3/miss\endcsname{6.11}
\expandafter\def\csname v@nsf_dev/dfn3/wer\endcsname{16.00}
\expandafter\def\csname v@nsf_dev/raw/dele\endcsname{1.73}
\expandafter\def\csname v@nsf_dev/raw/dleak\endcsname{+90.99}
\expandafter\def\csname v@nsf_dev/raw/dwer\endcsname{+26.42}
\expandafter\def\csname v@nsf_dev/raw/dwer-hi\endcsname{+29.64}
\expandafter\def\csname v@nsf_dev/raw/dwer-lo\endcsname{+23.45}
\expandafter\def\csname v@nsf_dev/raw/ins\endcsname{28.19}
\expandafter\def\csname v@nsf_dev/raw/leak_wpm\endcsname{91.63}
\expandafter\def\csname v@nsf_dev/raw/miss\endcsname{6.51}
\expandafter\def\csname v@nsf_dev/raw/wer\endcsname{34.71}
\expandafter\def\csname v@nsf_dev/sidon_v2/dele\endcsname{2.05}
\expandafter\def\csname v@nsf_dev/sidon_v2/dleak\endcsname{+138.19}
\expandafter\def\csname v@nsf_dev/sidon_v2/dwer\endcsname{+39.78}
\expandafter\def\csname v@nsf_dev/sidon_v2/dwer-hi\endcsname{+43.74}
\expandafter\def\csname v@nsf_dev/sidon_v2/dwer-lo\endcsname{+36.45}
\expandafter\def\csname v@nsf_dev/sidon_v2/ins\endcsname{41.16}
\expandafter\def\csname v@nsf_dev/sidon_v2/leak_wpm\endcsname{138.83}
\expandafter\def\csname v@nsf_dev/sidon_v2/miss\endcsname{6.90}
\expandafter\def\csname v@nsf_dev/sidon_v2/wer\endcsname{48.06}
\expandafter\def\csname v@nsf_dev/sidon_vi/dele\endcsname{1.71}
\expandafter\def\csname v@nsf_dev/sidon_vi/dleak\endcsname{+72.12}
\expandafter\def\csname v@nsf_dev/sidon_vi/dwer\endcsname{+19.63}
\expandafter\def\csname v@nsf_dev/sidon_vi/dwer-hi\endcsname{+22.78}
\expandafter\def\csname v@nsf_dev/sidon_vi/dwer-lo\endcsname{+16.89}
\expandafter\def\csname v@nsf_dev/sidon_vi/ins\endcsname{21.70}
\expandafter\def\csname v@nsf_dev/sidon_vi/leak_wpm\endcsname{72.76}
\expandafter\def\csname v@nsf_dev/sidon_vi/miss\endcsname{6.21}
\expandafter\def\csname v@nsf_dev/sidon_vi/wer\endcsname{27.91}
\expandafter\def\csname v@nsf_dev/sidon_vi_lite/dele\endcsname{1.50}
\expandafter\def\csname v@nsf_dev/sidon_vi_lite/dleak\endcsname{+16.44}
\expandafter\def\csname v@nsf_dev/sidon_vi_lite/dwer\endcsname{+3.85}
\expandafter\def\csname v@nsf_dev/sidon_vi_lite/dwer-hi\endcsname{+5.29}
\expandafter\def\csname v@nsf_dev/sidon_vi_lite/dwer-lo\endcsname{+2.45}
\expandafter\def\csname v@nsf_dev/sidon_vi_lite/ins\endcsname{6.34}
\expandafter\def\csname v@nsf_dev/sidon_vi_lite/leak_wpm\endcsname{17.08}
\expandafter\def\csname v@nsf_dev/sidon_vi_lite/miss\endcsname{5.79}
\expandafter\def\csname v@nsf_dev/sidon_vi_lite/wer\endcsname{12.13}
\expandafter\def\csname v@nsf_dev/voxlock/dele\endcsname{1.91}
\expandafter\def\csname v@nsf_dev/voxlock/dleak\endcsname{+0.00}
\expandafter\def\csname v@nsf_dev/voxlock/dwer\endcsname{-0.17}
\expandafter\def\csname v@nsf_dev/voxlock/dwer-hi\endcsname{+0.03}
\expandafter\def\csname v@nsf_dev/voxlock/dwer-lo\endcsname{-0.53}
\expandafter\def\csname v@nsf_dev/voxlock/ins\endcsname{1.90}
\expandafter\def\csname v@nsf_dev/voxlock/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@nsf_dev/voxlock/miss\endcsname{6.21}
\expandafter\def\csname v@nsf_dev/voxlock/wer\endcsname{8.11}
\expandafter\def\csname v@nsf_dev/voxlock_live/dele\endcsname{1.78}
\expandafter\def\csname v@nsf_dev/voxlock_live/dleak\endcsname{+1.06}
\expandafter\def\csname v@nsf_dev/voxlock_live/dwer\endcsname{-0.10}
\expandafter\def\csname v@nsf_dev/voxlock_live/dwer-hi\endcsname{+0.64}
\expandafter\def\csname v@nsf_dev/voxlock_live/dwer-lo\endcsname{-1.06}
\expandafter\def\csname v@nsf_dev/voxlock_live/ins\endcsname{2.12}
\expandafter\def\csname v@nsf_dev/voxlock_live/leak_wpm\endcsname{1.70}
\expandafter\def\csname v@nsf_dev/voxlock_live/miss\endcsname{6.06}
\expandafter\def\csname v@nsf_dev/voxlock_live/wer\endcsname{8.18}
\expandafter\def\csname v@nsf_dev/voxlock_pt/dele\endcsname{2.08}
\expandafter\def\csname v@nsf_dev/voxlock_pt/ins\endcsname{1.92}
\expandafter\def\csname v@nsf_dev/voxlock_pt/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@nsf_dev/voxlock_pt/miss\endcsname{6.36}
\expandafter\def\csname v@nsf_dev/voxlock_pt/wer\endcsname{8.28}
\expandafter\def\csname v@nsf_test/C22_ftlong_kd_selfl/dele\endcsname{1.69}
\expandafter\def\csname v@nsf_test/C22_ftlong_kd_selfl/dleak\endcsname{-0.47}
\expandafter\def\csname v@nsf_test/C22_ftlong_kd_selfl/dwer\endcsname{-0.21}
\expandafter\def\csname v@nsf_test/C22_ftlong_kd_selfl/dwer-hi\endcsname{+0.03}
\expandafter\def\csname v@nsf_test/C22_ftlong_kd_selfl/dwer-lo\endcsname{-0.46}
\expandafter\def\csname v@nsf_test/C22_ftlong_kd_selfl/ins\endcsname{1.84}
\expandafter\def\csname v@nsf_test/C22_ftlong_kd_selfl/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@nsf_test/C22_ftlong_kd_selfl/miss\endcsname{5.74}
\expandafter\def\csname v@nsf_test/C22_ftlong_kd_selfl/wer\endcsname{7.58}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_loud/dele\endcsname{1.69}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_loud/dleak\endcsname{-0.55}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_loud/dwer\endcsname{-0.11}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_loud/dwer-hi\endcsname{+0.11}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_loud/dwer-lo\endcsname{-0.36}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_loud/ins\endcsname{1.89}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_loud/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_loud/miss\endcsname{5.79}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_loud/wer\endcsname{7.67}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_null/dele\endcsname{1.73}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_null/dleak\endcsname{-0.53}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_null/dwer\endcsname{-0.05}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_null/dwer-hi\endcsname{+0.17}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_null/dwer-lo\endcsname{-0.30}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_null/ins\endcsname{1.91}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_null/leak_wpm\endcsname{0.49}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_null/miss\endcsname{5.82}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_null/wer\endcsname{7.74}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_selfl/dele\endcsname{1.73}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_selfl/dleak\endcsname{-0.64}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_selfl/dwer\endcsname{-0.11}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_selfl/dwer-hi\endcsname{+0.11}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_selfl/dwer-lo\endcsname{-0.35}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_selfl/ins\endcsname{1.91}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_selfl/leak_wpm\endcsname{0.38}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_selfl/miss\endcsname{5.76}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_cwlt2m_selfl/wer\endcsname{7.67}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_loud/dele\endcsname{1.73}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_loud/dleak\endcsname{-0.64}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_loud/dwer\endcsname{-0.08}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_loud/dwer-hi\endcsname{+0.20}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_loud/dwer-lo\endcsname{-0.36}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_loud/ins\endcsname{1.87}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_loud/leak_wpm\endcsname{0.38}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_loud/miss\endcsname{5.83}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_loud/wer\endcsname{7.70}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_null/dele\endcsname{1.72}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_null/dleak\endcsname{-0.55}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_null/dwer\endcsname{-0.14}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_null/dwer-hi\endcsname{+0.16}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_null/dwer-lo\endcsname{-0.42}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_null/ins\endcsname{1.83}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_null/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_null/miss\endcsname{5.81}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_null/wer\endcsname{7.64}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_selfl/dele\endcsname{1.61}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_selfl/dleak\endcsname{-0.59}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_selfl/dwer\endcsname{-0.21}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_selfl/dwer-hi\endcsname{+0.03}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_selfl/dwer-lo\endcsname{-0.46}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_selfl/ins\endcsname{1.84}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_selfl/leak_wpm\endcsname{0.42}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_selfl/miss\endcsname{5.74}
\expandafter\def\csname v@nsf_test/MB_ftlong_ws_selfl/wer\endcsname{7.58}
\expandafter\def\csname v@nsf_test/SB_ftlong_ws_selfl/dele\endcsname{1.81}
\expandafter\def\csname v@nsf_test/SB_ftlong_ws_selfl/dleak\endcsname{-0.49}
\expandafter\def\csname v@nsf_test/SB_ftlong_ws_selfl/dwer\endcsname{+0.00}
\expandafter\def\csname v@nsf_test/SB_ftlong_ws_selfl/dwer-hi\endcsname{+0.29}
\expandafter\def\csname v@nsf_test/SB_ftlong_ws_selfl/dwer-lo\endcsname{-0.28}
\expandafter\def\csname v@nsf_test/SB_ftlong_ws_selfl/ins\endcsname{1.90}
\expandafter\def\csname v@nsf_test/SB_ftlong_ws_selfl/leak_wpm\endcsname{0.53}
\expandafter\def\csname v@nsf_test/SB_ftlong_ws_selfl/miss\endcsname{5.89}
\expandafter\def\csname v@nsf_test/SB_ftlong_ws_selfl/wer\endcsname{7.78}
\expandafter\def\csname v@nsf_test/dfn3/dele\endcsname{1.97}
\expandafter\def\csname v@nsf_test/dfn3/dleak\endcsname{+25.08}
\expandafter\def\csname v@nsf_test/dfn3/dwer\endcsname{+7.59}
\expandafter\def\csname v@nsf_test/dfn3/dwer-hi\endcsname{+9.02}
\expandafter\def\csname v@nsf_test/dfn3/dwer-lo\endcsname{+6.32}
\expandafter\def\csname v@nsf_test/dfn3/ins\endcsname{9.14}
\expandafter\def\csname v@nsf_test/dfn3/leak_wpm\endcsname{26.09}
\expandafter\def\csname v@nsf_test/dfn3/miss\endcsname{6.23}
\expandafter\def\csname v@nsf_test/dfn3/wer\endcsname{15.38}
\expandafter\def\csname v@nsf_test/raw/dele\endcsname{2.22}
\expandafter\def\csname v@nsf_test/raw/dleak\endcsname{+89.89}
\expandafter\def\csname v@nsf_test/raw/dwer\endcsname{+26.92}
\expandafter\def\csname v@nsf_test/raw/dwer-hi\endcsname{+29.28}
\expandafter\def\csname v@nsf_test/raw/dwer-lo\endcsname{+24.75}
\expandafter\def\csname v@nsf_test/raw/ins\endcsname{27.86}
\expandafter\def\csname v@nsf_test/raw/leak_wpm\endcsname{90.90}
\expandafter\def\csname v@nsf_test/raw/miss\endcsname{6.84}
\expandafter\def\csname v@nsf_test/raw/wer\endcsname{34.70}
\expandafter\def\csname v@nsf_test/sidon_v2/dele\endcsname{3.45}
\expandafter\def\csname v@nsf_test/sidon_v2/dleak\endcsname{+130.17}
\expandafter\def\csname v@nsf_test/sidon_v2/dwer\endcsname{+39.57}
\expandafter\def\csname v@nsf_test/sidon_v2/dwer-hi\endcsname{+42.12}
\expandafter\def\csname v@nsf_test/sidon_v2/dwer-lo\endcsname{+37.17}
\expandafter\def\csname v@nsf_test/sidon_v2/ins\endcsname{38.89}
\expandafter\def\csname v@nsf_test/sidon_v2/leak_wpm\endcsname{131.19}
\expandafter\def\csname v@nsf_test/sidon_v2/miss\endcsname{8.47}
\expandafter\def\csname v@nsf_test/sidon_v2/wer\endcsname{47.35}
\expandafter\def\csname v@nsf_test/sidon_vi/dele\endcsname{2.29}
\expandafter\def\csname v@nsf_test/sidon_vi/dleak\endcsname{+75.80}
\expandafter\def\csname v@nsf_test/sidon_vi/dwer\endcsname{+22.23}
\expandafter\def\csname v@nsf_test/sidon_vi/dwer-hi\endcsname{+24.26}
\expandafter\def\csname v@nsf_test/sidon_vi/dwer-lo\endcsname{+20.25}
\expandafter\def\csname v@nsf_test/sidon_vi/ins\endcsname{23.20}
\expandafter\def\csname v@nsf_test/sidon_vi/leak_wpm\endcsname{76.82}
\expandafter\def\csname v@nsf_test/sidon_vi/miss\endcsname{6.81}
\expandafter\def\csname v@nsf_test/sidon_vi/wer\endcsname{30.01}
\expandafter\def\csname v@nsf_test/sidon_vi_lite/dele\endcsname{1.81}
\expandafter\def\csname v@nsf_test/sidon_vi_lite/dleak\endcsname{+19.63}
\expandafter\def\csname v@nsf_test/sidon_vi_lite/dwer\endcsname{+5.61}
\expandafter\def\csname v@nsf_test/sidon_vi_lite/dwer-hi\endcsname{+6.80}
\expandafter\def\csname v@nsf_test/sidon_vi_lite/dwer-lo\endcsname{+4.48}
\expandafter\def\csname v@nsf_test/sidon_vi_lite/ins\endcsname{7.36}
\expandafter\def\csname v@nsf_test/sidon_vi_lite/leak_wpm\endcsname{20.65}
\expandafter\def\csname v@nsf_test/sidon_vi_lite/miss\endcsname{6.04}
\expandafter\def\csname v@nsf_test/sidon_vi_lite/wer\endcsname{13.40}
\expandafter\def\csname v@nsf_test/voxlock/dele\endcsname{1.77}
\expandafter\def\csname v@nsf_test/voxlock/dleak\endcsname{-0.34}
\expandafter\def\csname v@nsf_test/voxlock/dwer\endcsname{-0.17}
\expandafter\def\csname v@nsf_test/voxlock/dwer-hi\endcsname{-0.02}
\expandafter\def\csname v@nsf_test/voxlock/dwer-lo\endcsname{-0.33}
\expandafter\def\csname v@nsf_test/voxlock/ins\endcsname{1.84}
\expandafter\def\csname v@nsf_test/voxlock/leak_wpm\endcsname{0.68}
\expandafter\def\csname v@nsf_test/voxlock/miss\endcsname{5.77}
\expandafter\def\csname v@nsf_test/voxlock/wer\endcsname{7.61}
\expandafter\def\csname v@nsf_test/voxlock_live/dele\endcsname{2.57}
\expandafter\def\csname v@nsf_test/voxlock_live/dleak\endcsname{+1.97}
\expandafter\def\csname v@nsf_test/voxlock_live/dwer\endcsname{+1.05}
\expandafter\def\csname v@nsf_test/voxlock_live/dwer-hi\endcsname{+1.66}
\expandafter\def\csname v@nsf_test/voxlock_live/dwer-lo\endcsname{+0.52}
\expandafter\def\csname v@nsf_test/voxlock_live/ins\endcsname{2.31}
\expandafter\def\csname v@nsf_test/voxlock_live/leak_wpm\endcsname{2.99}
\expandafter\def\csname v@nsf_test/voxlock_live/miss\endcsname{6.53}
\expandafter\def\csname v@nsf_test/voxlock_live/wer\endcsname{8.84}
\expandafter\def\csname v@nsf_test/voxlock_pt/dele\endcsname{1.80}
\expandafter\def\csname v@nsf_test/voxlock_pt/ins\endcsname{1.94}
\expandafter\def\csname v@nsf_test/voxlock_pt/leak_wpm\endcsname{1.02}
\expandafter\def\csname v@nsf_test/voxlock_pt/miss\endcsname{5.84}
\expandafter\def\csname v@nsf_test/voxlock_pt/wer\endcsname{7.78}
\expandafter\def\csname v@phone/dev/candidates\endcsname{63}
\expandafter\def\csname v@phone/dev/cpu/candidates\endcsname{35}
\expandafter\def\csname v@phone/dev/cpu_after-cpu_before/quiet_phone-pct\endcsname{+8.8}
\expandafter\def\csname v@phone/dev/cpu_after-cpu_before/score-pct\endcsname{+12.8}
\expandafter\def\csname v@phone/dev/cpu_after-cpu_before/wide-pct\endcsname{+1.5}
\expandafter\def\csname v@phone/dev/cpu_after/others\endcsname{22}
\expandafter\def\csname v@phone/dev/cpu_after/pause\endcsname{51.6}
\expandafter\def\csname v@phone/dev/cpu_after/quiet_phone\endcsname{1,224}
\expandafter\def\csname v@phone/dev/cpu_after/score\endcsname{2,510}
\expandafter\def\csname v@phone/dev/cpu_after/wide\endcsname{4,555}
\expandafter\def\csname v@phone/dev/cpu_before/others\endcsname{29}
\expandafter\def\csname v@phone/dev/cpu_before/pause\endcsname{55.4}
\expandafter\def\csname v@phone/dev/cpu_before/quiet_phone\endcsname{1,125}
\expandafter\def\csname v@phone/dev/cpu_before/score\endcsname{2,225}
\expandafter\def\csname v@phone/dev/cpu_before/wide\endcsname{4,486}
\expandafter\def\csname v@phone/dev/gpu/candidates\endcsname{28}
\expandafter\def\csname v@phone/dev/gpu/others\endcsname{58}
\expandafter\def\csname v@phone/dev/gpu/pause\endcsname{61.3}
\expandafter\def\csname v@phone/dev/gpu/quiet_phone\endcsname{1,264}
\expandafter\def\csname v@phone/dev/gpu/score\endcsname{2,767}
\expandafter\def\csname v@phone/dev/gpu/wide\endcsname{4,706}
\expandafter\def\csname v@phone/dev/gpu_ft-gpu/quiet_phone-pct\endcsname{+0.0}
\expandafter\def\csname v@phone/dev/gpu_ft-gpu/score-pct\endcsname{+1.5}
\expandafter\def\csname v@phone/dev/gpu_ft-gpu/wide-pct\endcsname{-0.6}
\expandafter\def\csname v@phone/dev/gpu_ft/others\endcsname{60}
\expandafter\def\csname v@phone/dev/gpu_ft/pause\endcsname{58.7}
\expandafter\def\csname v@phone/dev/gpu_ft/quiet_phone\endcsname{1,264}
\expandafter\def\csname v@phone/dev/gpu_ft/score\endcsname{2,809}
\expandafter\def\csname v@phone/dev/gpu_ft/wide\endcsname{4,677}
\expandafter\def\csname v@phone/dev/inworld-gpu/quiet_phone-pct\endcsname{-2.1}
\expandafter\def\csname v@phone/dev/inworld-gpu/score-pct\endcsname{+11.5}
\expandafter\def\csname v@phone/dev/inworld-gpu/wide-pct\endcsname{-0.8}
\expandafter\def\csname v@phone/dev/inworld/others\endcsname{123}
\expandafter\def\csname v@phone/dev/inworld/pause\endcsname{34.6}
\expandafter\def\csname v@phone/dev/inworld/quiet_phone\endcsname{1,237}
\expandafter\def\csname v@phone/dev/inworld/score\endcsname{3,086}
\expandafter\def\csname v@phone/dev/inworld/wide\endcsname{4,669}
\expandafter\def\csname v@phone/dev/none/others\endcsname{294}
\expandafter\def\csname v@phone/dev/none/pause\endcsname{0.0}
\expandafter\def\csname v@phone/dev/none/quiet_phone\endcsname{1,344}
\expandafter\def\csname v@phone/dev/none/score\endcsname{3,249}
\expandafter\def\csname v@phone/dev/none/wide\endcsname{4,848}
\expandafter\def\csname v@phone/heard/cpu_default/noisy/phone\endcsname{120}
\expandafter\def\csname v@phone/heard/cpu_default/noisy/phone_band\endcsname{164}
\expandafter\def\csname v@phone/heard/cpu_default/noisy/wide\endcsname{204}
\expandafter\def\csname v@phone/heard/cpu_default/noisy/wide_floor\endcsname{217}
\expandafter\def\csname v@phone/heard/cpu_default/quiet/phone\endcsname{226}
\expandafter\def\csname v@phone/heard/cpu_default/quiet/wide\endcsname{256}
\expandafter\def\csname v@phone/heard/cpu_voicebot/noisy/phone\endcsname{132}
\expandafter\def\csname v@phone/heard/cpu_voicebot/noisy/phone_band\endcsname{185}
\expandafter\def\csname v@phone/heard/cpu_voicebot/noisy/wide\endcsname{215}
\expandafter\def\csname v@phone/heard/cpu_voicebot/noisy/wide_floor\endcsname{232}
\expandafter\def\csname v@phone/heard/cpu_voicebot/quiet/phone\endcsname{218}
\expandafter\def\csname v@phone/heard/cpu_voicebot/quiet/wide\endcsname{256}
\expandafter\def\csname v@phone/heard/none/noisy/phone\endcsname{220}
\expandafter\def\csname v@phone/heard/none/noisy/phone_band\endcsname{221}
\expandafter\def\csname v@phone/heard/none/noisy/wide\endcsname{245}
\expandafter\def\csname v@phone/heard/none/noisy/wide_floor\endcsname{248}
\expandafter\def\csname v@phone/heard/none/quiet/phone\endcsname{230}
\expandafter\def\csname v@phone/heard/none/quiet/wide\endcsname{256}
\expandafter\def\csname v@phone/heard/prod_vb1/noisy/phone\endcsname{150}
\expandafter\def\csname v@phone/heard/prod_vb1/noisy/wide\endcsname{225}
\expandafter\def\csname v@phone/heard/prod_vb1/quiet/phone\endcsname{219}
\expandafter\def\csname v@phone/heard/prod_vb1/quiet/wide\endcsname{256}
\expandafter\def\csname v@phone/line/band-khz\endcsname{3.4}
\expandafter\def\csname v@phone/line/calls\endcsname{6}
\expandafter\def\csname v@phone/line/floor-db\endcsname{-24.7}
\expandafter\def\csname v@phone/line/ref-words\endcsname{258}
\expandafter\def\csname v@phone/lp/parakeet/cpu_dev/noisy\endcsname{120}
\expandafter\def\csname v@phone/lp/parakeet/cpu_dev/quiet\endcsname{226}
\expandafter\def\csname v@phone/lp/parakeet/cpu_lp/noisy\endcsname{170}
\expandafter\def\csname v@phone/lp/parakeet/cpu_lp/quiet\endcsname{205}
\expandafter\def\csname v@phone/lp/parakeet/gpu_dev/noisy\endcsname{165}
\expandafter\def\csname v@phone/lp/parakeet/gpu_dev/quiet\endcsname{220}
\expandafter\def\csname v@phone/lp/parakeet/gpu_lp/noisy\endcsname{180}
\expandafter\def\csname v@phone/lp/parakeet/gpu_lp/quiet\endcsname{195}
\expandafter\def\csname v@phone/lp/whisper/cpu_dev/noisy\endcsname{136}
\expandafter\def\csname v@phone/lp/whisper/cpu_dev/quiet\endcsname{223}
\expandafter\def\csname v@phone/lp/whisper/cpu_lp/noisy\endcsname{162}
\expandafter\def\csname v@phone/lp/whisper/cpu_lp/quiet\endcsname{220}
\expandafter\def\csname v@phone/lp/whisper/gpu_dev/noisy\endcsname{170}
\expandafter\def\csname v@phone/lp/whisper/gpu_dev/quiet\endcsname{218}
\expandafter\def\csname v@phone/lp/whisper/gpu_lp/noisy\endcsname{178}
\expandafter\def\csname v@phone/lp/whisper/gpu_lp/quiet\endcsname{233}
\expandafter\def\csname v@phone/test/cpu/cpu_cur/noisy\endcsname{333}
\expandafter\def\csname v@phone/test/cpu/cpu_cur/quiet\endcsname{428}
\expandafter\def\csname v@phone/test/cpu/cpu_pick/noisy\endcsname{331}
\expandafter\def\csname v@phone/test/cpu/cpu_pick/quiet\endcsname{466}
\expandafter\def\csname v@phone/test/cpu/none/noisy\endcsname{441}
\expandafter\def\csname v@phone/test/cpu/none/quiet\endcsname{484}
\expandafter\def\csname v@phone/test/gpu/tgbase_vb1/noisy\endcsname{404}
\expandafter\def\csname v@phone/test/gpu/tgbase_vb1/quiet\endcsname{492}
\expandafter\def\csname v@phone/test/gpu/tgpick_vb1/noisy\endcsname{399}
\expandafter\def\csname v@phone/test/gpu/tgpick_vb1/quiet\endcsname{507}
\expandafter\def\csname v@phone/vint/C22_vbjp_1750/all\endcsname{0.56}
\expandafter\def\csname v@phone/vint/calls\endcsname{160}
\expandafter\def\csname v@phone/vint/cbase/all\endcsname{0.56}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev/dele\endcsname{3.12}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev/ins\endcsname{4.65}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev/leak_wpm\endcsname{8.26}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev/miss\endcsname{9.14}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev/wer\endcsname{13.79}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev_long/dele\endcsname{7.90}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev_long/ins\endcsname{4.90}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev_long/leak_wpm\endcsname{7.70}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev_long/miss\endcsname{15.32}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/ami_dev_long/wer\endcsname{20.22}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/call_dev_clean/dele\endcsname{1.72}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/call_dev_clean/miss\endcsname{2.41}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/call_dev_clean/wer\endcsname{2.68}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/dev4\endcsname{11.10}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/meet3\endcsname{13.90}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/nsf_dev/ins\endcsname{1.91}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/nsf_dev/miss\endcsname{5.79}
\expandafter\def\csname v@r/C10_ftlong_kd_int8_selfl/nsf_dev/wer\endcsname{7.70}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/aic_calls/dele\endcsname{2.53}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/aic_calls/ins\endcsname{10.26}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/aic_calls/leak_wpm\endcsname{12.11}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/aic_calls/miss\endcsname{6.45}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/aic_calls/wer\endcsname{16.71}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev/dele\endcsname{3.11}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev/ins\endcsname{4.51}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev/leak_wpm\endcsname{8.21}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev/miss\endcsname{9.17}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev/wer\endcsname{13.68}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev_long/dele\endcsname{7.81}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev_long/ins\endcsname{4.87}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev_long/leak_wpm\endcsname{7.73}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev_long/miss\endcsname{15.21}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/ami_dev_long/wer\endcsname{20.08}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/call_dev_clean/dele\endcsname{1.74}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/call_dev_clean/ins\endcsname{0.29}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/call_dev_clean/miss\endcsname{2.49}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/call_dev_clean/wer\endcsname{2.77}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/dev4\endcsname{11.06}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/krisp/dele\endcsname{1.21}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/krisp/leak_wpm\endcsname{0.02}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/krisp/miss\endcsname{4.87}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/krisp/wer\endcsname{5.60}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/meet3\endcsname{13.82}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/nsf_dev/ins\endcsname{1.92}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/nsf_dev/miss\endcsname{5.79}
\expandafter\def\csname v@r/C10_ftlong_kd_selfl/nsf_dev/wer\endcsname{7.71}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev/dele\endcsname{2.95}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev/ins\endcsname{4.86}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev/leak_wpm\endcsname{8.84}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev/miss\endcsname{8.99}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev/wer\endcsname{13.84}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev_long/dele\endcsname{7.53}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev_long/ins\endcsname{4.61}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev_long/leak_wpm\endcsname{7.79}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev_long/miss\endcsname{15.31}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/ami_dev_long/wer\endcsname{19.92}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/call_dev_clean/dele\endcsname{1.72}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/call_dev_clean/ins\endcsname{0.22}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/call_dev_clean/miss\endcsname{2.45}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/call_dev_clean/wer\endcsname{2.66}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/dev4\endcsname{11.03}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/meet3\endcsname{13.82}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/nsf_dev/ins\endcsname{1.88}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/nsf_dev/miss\endcsname{5.82}
\expandafter\def\csname v@r/C10n_ftlong_kd_int8_selfl/nsf_dev/wer\endcsname{7.70}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/aic_calls/dele\endcsname{2.57}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/aic_calls/ins\endcsname{10.16}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/aic_calls/leak_wpm\endcsname{11.86}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/aic_calls/miss\endcsname{5.95}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/aic_calls/wer\endcsname{16.11}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev/dele\endcsname{2.93}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev/ins\endcsname{4.91}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev/leak_wpm\endcsname{8.84}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev/miss\endcsname{8.91}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev/wer\endcsname{13.82}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev_long/dele\endcsname{7.31}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev_long/ins\endcsname{4.72}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev_long/leak_wpm\endcsname{7.74}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev_long/miss\endcsname{14.97}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/ami_dev_long/wer\endcsname{19.69}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/call_dev_clean/dele\endcsname{1.77}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/call_dev_clean/miss\endcsname{2.52}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/call_dev_clean/wer\endcsname{2.75}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/dev4\endcsname{10.99}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/krisp/dele\endcsname{1.16}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/krisp/ins\endcsname{0.72}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/krisp/leak_wpm\endcsname{0.02}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/krisp/miss\endcsname{4.72}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/krisp/wer\endcsname{5.44}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/meet3\endcsname{13.73}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/nsf_dev/ins\endcsname{1.88}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/C10n_ftlong_kd_selfl/nsf_dev/wer\endcsname{7.69}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev/dele\endcsname{3.11}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev/ins\endcsname{4.12}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev/leak_wpm\endcsname{7.99}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev/miss\endcsname{9.20}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev/wer\endcsname{13.32}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev_long/dele\endcsname{7.17}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev_long/ins\endcsname{4.71}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev_long/leak_wpm\endcsname{7.97}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev_long/miss\endcsname{15.04}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/ami_dev_long/wer\endcsname{19.75}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/call_dev_clean/dele\endcsname{3.70}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/call_dev_clean/ins\endcsname{0.27}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/call_dev_clean/miss\endcsname{4.77}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/call_dev_clean/wer\endcsname{5.04}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/dev4\endcsname{11.47}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/krisp/dele\endcsname{2.04}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/krisp/ins\endcsname{0.72}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/krisp/leak_wpm\endcsname{0.02}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/krisp/miss\endcsname{5.86}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/krisp/wer\endcsname{6.58}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/meet3\endcsname{13.61}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/nsf_dev/miss\endcsname{5.84}
\expandafter\def\csname v@r/C22_ftlong_ini_selfl/nsf_dev/wer\endcsname{7.77}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev/dele\endcsname{3.11}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev/ins\endcsname{4.40}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev/leak_wpm\endcsname{8.93}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev/miss\endcsname{9.22}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev/wer\endcsname{13.62}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev_long/dele\endcsname{6.90}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev_long/ins\endcsname{3.31}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev_long/leak_wpm\endcsname{6.53}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev_long/miss\endcsname{14.62}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/ami_dev_long/wer\endcsname{17.93}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/call_dev_clean/dele\endcsname{1.82}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/call_dev_clean/ins\endcsname{0.25}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/call_dev_clean/miss\endcsname{2.59}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/call_dev_clean/wer\endcsname{2.84}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/dev4\endcsname{10.52}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/meet3\endcsname{13.08}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/nsf_dev/dele\endcsname{1.44}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/nsf_dev/ins\endcsname{1.97}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/nsf_dev/miss\endcsname{5.71}
\expandafter\def\csname v@r/C22_ftlong_kd_int8_selfl/nsf_dev/wer\endcsname{7.68}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/aic_calls/dele\endcsname{3.35}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/aic_calls/ins\endcsname{11.40}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/aic_calls/leak_wpm\endcsname{13.25}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/aic_calls/miss\endcsname{6.63}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/aic_calls/wer\endcsname{18.03}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev/dele\endcsname{3.25}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev/ins\endcsname{4.38}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev/leak_wpm\endcsname{8.84}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev/miss\endcsname{9.24}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev/wer\endcsname{13.62}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev_long/dele\endcsname{7.17}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev_long/ins\endcsname{3.54}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev_long/leak_wpm\endcsname{6.65}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev_long/miss\endcsname{14.92}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/ami_dev_long/wer\endcsname{18.45}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/call_dev_clean/dele\endcsname{1.80}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/call_dev_clean/miss\endcsname{2.58}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/call_dev_clean/wer\endcsname{2.84}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/dev4\endcsname{10.66}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/krisp/dele\endcsname{1.37}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/krisp/ins\endcsname{0.69}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/krisp/miss\endcsname{4.98}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/krisp/wer\endcsname{5.66}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/meet3\endcsname{13.26}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/nsf_dev/dele\endcsname{1.47}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/nsf_dev/ins\endcsname{1.97}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/nsf_dev/miss\endcsname{5.73}
\expandafter\def\csname v@r/C22_ftlong_kd_selfl/nsf_dev/wer\endcsname{7.70}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev/dele\endcsname{3.07}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev/ins\endcsname{4.48}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev/leak_wpm\endcsname{9.20}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev/miss\endcsname{9.14}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev/wer\endcsname{13.62}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev_long/dele\endcsname{7.94}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev_long/ins\endcsname{5.33}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev_long/leak_wpm\endcsname{8.52}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev_long/miss\endcsname{15.72}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/ami_dev_long/wer\endcsname{21.05}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/call_dev_clean/dele\endcsname{2.78}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/call_dev_clean/miss\endcsname{3.97}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/call_dev_clean/wer\endcsname{4.21}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/dev4\endcsname{11.64}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/krisp/dele\endcsname{1.68}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/krisp/leak_wpm\endcsname{0.11}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/krisp/miss\endcsname{5.59}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/krisp/wer\endcsname{6.33}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/meet3\endcsname{14.11}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/nsf_dev/dele\endcsname{1.43}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/nsf_dev/miss\endcsname{5.73}
\expandafter\def\csname v@r/C22_ftlong_kdo_selfl/nsf_dev/wer\endcsname{7.66}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/aic_calls/dele\endcsname{5.70}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/aic_calls/ins\endcsname{10.23}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/aic_calls/leak_wpm\endcsname{12.62}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/aic_calls/miss\endcsname{9.44}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/aic_calls/wer\endcsname{19.67}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev/dele\endcsname{3.15}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev/ins\endcsname{4.72}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev/leak_wpm\endcsname{9.24}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev/miss\endcsname{9.29}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev/wer\endcsname{14.01}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev_long/dele\endcsname{8.26}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev_long/ins\endcsname{4.26}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev_long/leak_wpm\endcsname{7.13}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev_long/miss\endcsname{15.67}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/ami_dev_long/wer\endcsname{19.93}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/call_dev_clean/dele\endcsname{5.37}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/call_dev_clean/ins\endcsname{0.36}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/call_dev_clean/miss\endcsname{6.64}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/call_dev_clean/wer\endcsname{7.00}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/dev4\endcsname{12.14}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/krisp/dele\endcsname{2.50}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/krisp/leak_wpm\endcsname{0.02}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/krisp/miss\endcsname{6.48}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/krisp/wer\endcsname{7.18}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/meet3\endcsname{13.85}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/nsf_dev/dele\endcsname{1.49}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/nsf_dev/ins\endcsname{1.84}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/nsf_dev/miss\endcsname{5.77}
\expandafter\def\csname v@r/C22_ftlong_sc_selfl/nsf_dev/wer\endcsname{7.61}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev/dele\endcsname{3.01}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev/ins\endcsname{4.88}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev/leak_wpm\endcsname{8.84}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev/miss\endcsname{8.85}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev/wer\endcsname{13.73}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev_long/dele\endcsname{7.87}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev_long/ins\endcsname{4.03}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev_long/leak_wpm\endcsname{6.44}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev_long/miss\endcsname{15.18}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/ami_dev_long/wer\endcsname{19.22}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/call_dev_clean/dele\endcsname{1.91}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/call_dev_clean/miss\endcsname{2.62}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/call_dev_clean/wer\endcsname{2.88}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/dev4\endcsname{10.87}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/meet3\endcsname{13.53}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/nsf_dev/ins\endcsname{1.87}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/nsf_dev/miss\endcsname{5.76}
\expandafter\def\csname v@r/C51_ftlong_kd_int8_selfl/nsf_dev/wer\endcsname{7.63}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/aic_calls/dele\endcsname{3.24}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/aic_calls/ins\endcsname{10.62}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/aic_calls/leak_wpm\endcsname{12.05}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/aic_calls/miss\endcsname{6.56}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/aic_calls/wer\endcsname{17.18}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev/dele\endcsname{2.98}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev/ins\endcsname{4.74}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev/leak_wpm\endcsname{8.66}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev/miss\endcsname{8.82}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev/wer\endcsname{13.57}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev_long/dele\endcsname{7.80}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev_long/ins\endcsname{4.20}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev_long/leak_wpm\endcsname{6.49}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev_long/miss\endcsname{14.87}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/ami_dev_long/wer\endcsname{19.07}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/call_dev_clean/dele\endcsname{1.94}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/call_dev_clean/miss\endcsname{2.60}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/call_dev_clean/wer\endcsname{2.87}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/dev4\endcsname{10.78}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/krisp/dele\endcsname{1.34}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/krisp/leak_wpm\endcsname{0.02}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/krisp/miss\endcsname{4.94}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/krisp/wer\endcsname{5.67}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/meet3\endcsname{13.42}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/nsf_dev/ins\endcsname{1.87}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/nsf_dev/miss\endcsname{5.76}
\expandafter\def\csname v@r/C51_ftlong_kd_selfl/nsf_dev/wer\endcsname{7.63}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev/dele\endcsname{2.90}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev/ins\endcsname{3.44}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev/leak_wpm\endcsname{7.37}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev/miss\endcsname{9.07}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev/wer\endcsname{12.51}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev_long/dele\endcsname{9.09}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev_long/ins\endcsname{5.35}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev_long/leak_wpm\endcsname{8.26}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev_long/miss\endcsname{16.41}
\expandafter\def\csname v@r/LB_ftlong_selfl/ami_dev_long/wer\endcsname{21.75}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_clean/dele\endcsname{7.44}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_clean/miss\endcsname{8.53}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_clean/wer\endcsname{8.79}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_mix/dele\endcsname{6.76}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_mix/ins\endcsname{32.06}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_mix/leak_wpm\endcsname{101.47}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_mix/miss\endcsname{20.24}
\expandafter\def\csname v@r/LB_ftlong_selfl/call_dev_mix/wer\endcsname{52.30}
\expandafter\def\csname v@r/LB_ftlong_selfl/dev4\endcsname{12.66}
\expandafter\def\csname v@r/LB_ftlong_selfl/krisp/dele\endcsname{2.62}
\expandafter\def\csname v@r/LB_ftlong_selfl/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/LB_ftlong_selfl/krisp/leak_wpm\endcsname{0.16}
\expandafter\def\csname v@r/LB_ftlong_selfl/krisp/miss\endcsname{6.58}
\expandafter\def\csname v@r/LB_ftlong_selfl/krisp/wer\endcsname{7.28}
\expandafter\def\csname v@r/LB_ftlong_selfl/meet3\endcsname{13.95}
\expandafter\def\csname v@r/LB_ftlong_selfl/nsf_dev/dele\endcsname{1.59}
\expandafter\def\csname v@r/LB_ftlong_selfl/nsf_dev/ins\endcsname{1.79}
\expandafter\def\csname v@r/LB_ftlong_selfl/nsf_dev/leak_wpm\endcsname{0.38}
\expandafter\def\csname v@r/LB_ftlong_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/LB_ftlong_selfl/nsf_dev/wer\endcsname{7.59}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev/dele\endcsname{2.83}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev/ins\endcsname{3.97}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev/leak_wpm\endcsname{8.93}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev/miss\endcsname{8.85}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev/wer\endcsname{12.82}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev_long/dele\endcsname{6.77}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev_long/ins\endcsname{3.91}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev_long/leak_wpm\endcsname{6.62}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev_long/miss\endcsname{13.99}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/ami_dev_long/wer\endcsname{17.89}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_clean/dele\endcsname{3.04}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_clean/miss\endcsname{3.86}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_clean/wer\endcsname{4.16}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_mix/dele\endcsname{4.12}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_mix/ins\endcsname{34.57}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_mix/leak_wpm\endcsname{113.18}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_mix/miss\endcsname{17.73}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/call_dev_mix/wer\endcsname{52.30}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/dev4\endcsname{10.66}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/krisp/dele\endcsname{1.30}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/krisp/leak_wpm\endcsname{0.19}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/krisp/miss\endcsname{4.73}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/krisp/wer\endcsname{5.47}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/meet3\endcsname{12.82}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/nsf_dev/miss\endcsname{5.82}
\expandafter\def\csname v@r/LB_ftlong_ws_cwlt2_selfl/nsf_dev/wer\endcsname{7.76}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev/dele\endcsname{2.65}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev/ins\endcsname{4.79}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev/leak_wpm\endcsname{10.09}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev/miss\endcsname{8.89}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev/wer\endcsname{13.68}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev_long/dele\endcsname{6.78}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev_long/ins\endcsname{12.89}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev_long/leak_wpm\endcsname{18.18}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev_long/miss\endcsname{14.89}
\expandafter\def\csname v@r/LB_ftlong_ws_null/ami_dev_long/wer\endcsname{27.78}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_clean/dele\endcsname{3.37}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_clean/ins\endcsname{0.27}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_clean/miss\endcsname{4.16}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_clean/wer\endcsname{4.43}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_mix/dele\endcsname{4.04}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_mix/ins\endcsname{37.22}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_mix/leak_wpm\endcsname{93.26}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_mix/miss\endcsname{16.47}
\expandafter\def\csname v@r/LB_ftlong_ws_null/call_dev_mix/wer\endcsname{53.69}
\expandafter\def\csname v@r/LB_ftlong_ws_null/dev4\endcsname{13.37}
\expandafter\def\csname v@r/LB_ftlong_ws_null/krisp/dele\endcsname{1.37}
\expandafter\def\csname v@r/LB_ftlong_ws_null/krisp/ins\endcsname{1.79}
\expandafter\def\csname v@r/LB_ftlong_ws_null/krisp/leak_wpm\endcsname{4.10}
\expandafter\def\csname v@r/LB_ftlong_ws_null/krisp/miss\endcsname{4.87}
\expandafter\def\csname v@r/LB_ftlong_ws_null/krisp/wer\endcsname{6.66}
\expandafter\def\csname v@r/LB_ftlong_ws_null/meet3\endcsname{16.34}
\expandafter\def\csname v@r/LB_ftlong_ws_null/nsf_dev/dele\endcsname{1.57}
\expandafter\def\csname v@r/LB_ftlong_ws_null/nsf_dev/ins\endcsname{1.81}
\expandafter\def\csname v@r/LB_ftlong_ws_null/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/LB_ftlong_ws_null/nsf_dev/miss\endcsname{5.76}
\expandafter\def\csname v@r/LB_ftlong_ws_null/nsf_dev/wer\endcsname{7.57}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev/dele\endcsname{2.64}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev/ins\endcsname{4.54}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev/leak_wpm\endcsname{9.46}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev/miss\endcsname{8.78}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev/wer\endcsname{13.32}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev_long/dele\endcsname{8.62}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev_long/ins\endcsname{5.55}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev_long/leak_wpm\endcsname{9.13}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev_long/miss\endcsname{16.10}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/ami_dev_long/wer\endcsname{21.65}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_clean/dele\endcsname{5.48}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_clean/ins\endcsname{0.36}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_clean/miss\endcsname{6.48}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_clean/wer\endcsname{6.83}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_mix/dele\endcsname{5.25}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_mix/ins\endcsname{38.19}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_mix/leak_wpm\endcsname{119.34}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_mix/miss\endcsname{18.09}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/call_dev_mix/wer\endcsname{56.28}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/dev4\endcsname{12.35}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/krisp/dele\endcsname{2.17}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/krisp/ins\endcsname{0.86}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/krisp/leak_wpm\endcsname{0.67}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/krisp/miss\endcsname{5.91}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/krisp/wer\endcsname{6.77}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/meet3\endcsname{14.18}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/nsf_dev/dele\endcsname{1.57}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/nsf_dev/ins\endcsname{1.83}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/nsf_dev/miss\endcsname{5.76}
\expandafter\def\csname v@r/LB_ftlong_ws_selfl/nsf_dev/wer\endcsname{7.58}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev/dele\endcsname{3.01}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev/ins\endcsname{4.61}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev/leak_wpm\endcsname{9.02}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev/miss\endcsname{8.75}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev/wer\endcsname{13.36}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev_long/dele\endcsname{7.14}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev_long/ins\endcsname{5.47}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev_long/leak_wpm\endcsname{8.79}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev_long/miss\endcsname{14.88}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/ami_dev_long/wer\endcsname{20.35}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_clean/dele\endcsname{5.27}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_clean/miss\endcsname{6.60}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_clean/wer\endcsname{6.83}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_mix/dele\endcsname{5.78}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_mix/ins\endcsname{35.05}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_mix/leak_wpm\endcsname{110.30}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_mix/miss\endcsname{17.59}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/call_dev_mix/wer\endcsname{52.63}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/dev4\endcsname{12.04}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/krisp/dele\endcsname{1.90}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/krisp/leak_wpm\endcsname{0.23}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/krisp/miss\endcsname{5.76}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/krisp/wer\endcsname{6.50}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/meet3\endcsname{13.77}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/nsf_dev/dele\endcsname{1.61}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/nsf_dev/ins\endcsname{1.80}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/LB_ftlong_ws_slow_selfl/nsf_dev/wer\endcsname{7.61}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev/dele\endcsname{3.45}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev/ins\endcsname{3.68}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev/leak_wpm\endcsname{7.41}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev/miss\endcsname{9.45}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev/wer\endcsname{13.12}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev_long/dele\endcsname{8.25}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev_long/ins\endcsname{4.39}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev_long/leak_wpm\endcsname{7.12}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev_long/miss\endcsname{15.46}
\expandafter\def\csname v@r/MB_ftlong_selfl/ami_dev_long/wer\endcsname{19.85}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_clean/dele\endcsname{6.02}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_clean/miss\endcsname{7.15}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_clean/wer\endcsname{7.38}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_mix/dele\endcsname{6.12}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_mix/ins\endcsname{29.70}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_mix/leak_wpm\endcsname{99.42}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_mix/miss\endcsname{19.12}
\expandafter\def\csname v@r/MB_ftlong_selfl/call_dev_mix/wer\endcsname{48.82}
\expandafter\def\csname v@r/MB_ftlong_selfl/dev4\endcsname{11.99}
\expandafter\def\csname v@r/MB_ftlong_selfl/krisp/dele\endcsname{2.08}
\expandafter\def\csname v@r/MB_ftlong_selfl/krisp/ins\endcsname{0.68}
\expandafter\def\csname v@r/MB_ftlong_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/MB_ftlong_selfl/krisp/miss\endcsname{6.05}
\expandafter\def\csname v@r/MB_ftlong_selfl/krisp/wer\endcsname{6.73}
\expandafter\def\csname v@r/MB_ftlong_selfl/meet3\endcsname{13.52}
\expandafter\def\csname v@r/MB_ftlong_selfl/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/MB_ftlong_selfl/nsf_dev/ins\endcsname{1.83}
\expandafter\def\csname v@r/MB_ftlong_selfl/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/MB_ftlong_selfl/nsf_dev/miss\endcsname{5.77}
\expandafter\def\csname v@r/MB_ftlong_selfl/nsf_dev/wer\endcsname{7.59}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev/dele\endcsname{2.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev/ins\endcsname{4.23}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev/leak_wpm\endcsname{8.08}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev/miss\endcsname{8.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev/wer\endcsname{12.97}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev_long/dele\endcsname{6.31}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev_long/ins\endcsname{4.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev_long/leak_wpm\endcsname{7.33}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev_long/miss\endcsname{13.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/ami_dev_long/wer\endcsname{18.25}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_clean/dele\endcsname{2.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_clean/ins\endcsname{0.18}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_clean/miss\endcsname{3.30}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_clean/wer\endcsname{3.48}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_mix/dele\endcsname{3.72}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_mix/ins\endcsname{36.65}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_mix/leak_wpm\endcsname{114.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_mix/miss\endcsname{16.01}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/call_dev_mix/wer\endcsname{52.66}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/dev4\endcsname{10.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/krisp/dele\endcsname{1.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/krisp/ins\endcsname{0.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/krisp/leak_wpm\endcsname{0.32}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/krisp/miss\endcsname{4.75}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/krisp/wer\endcsname{5.54}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/meet3\endcsname{12.97}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/nsf_dev/dele\endcsname{1.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/nsf_dev/ins\endcsname{1.88}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/nsf_dev/leak_wpm\endcsname{0.38}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t2_selfl/nsf_dev/wer\endcsname{7.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/aic_calls/dele\endcsname{2.92}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/aic_calls/ins\endcsname{9.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/aic_calls/leak_wpm\endcsname{10.22}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/aic_calls/miss\endcsname{6.49}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/aic_calls/wer\endcsname{16.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev/dele\endcsname{2.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev/ins\endcsname{4.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev/leak_wpm\endcsname{7.14}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev/miss\endcsname{8.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev/wer\endcsname{12.64}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev_long/dele\endcsname{6.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev_long/ins\endcsname{4.85}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev_long/leak_wpm\endcsname{7.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev_long/miss\endcsname{13.94}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/ami_dev_long/wer\endcsname{18.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_clean/dele\endcsname{2.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_clean/miss\endcsname{3.39}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_clean/wer\endcsname{3.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_mix/dele\endcsname{4.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_mix/ins\endcsname{36.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_mix/leak_wpm\endcsname{113.80}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_mix/miss\endcsname{18.31}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/call_dev_mix/wer\endcsname{54.71}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/dev4\endcsname{10.67}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/krisp/dele\endcsname{1.46}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/krisp/ins\endcsname{0.68}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/krisp/miss\endcsname{5.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/krisp/wer\endcsname{5.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/meet3\endcsname{13.01}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/nsf_dev/dele\endcsname{1.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/nsf_dev/ins\endcsname{1.81}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/MB_ftlong_ws_cwl0t_selfl/nsf_dev/wer\endcsname{7.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev/dele\endcsname{3.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev/ins\endcsname{3.91}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev/leak_wpm\endcsname{8.17}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev/miss\endcsname{9.09}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev/wer\endcsname{13.00}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev_long/dele\endcsname{6.72}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev_long/ins\endcsname{5.27}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev_long/leak_wpm\endcsname{8.68}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev_long/miss\endcsname{14.45}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/ami_dev_long/wer\endcsname{19.71}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_clean/dele\endcsname{3.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_clean/ins\endcsname{0.25}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_clean/miss\endcsname{4.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_clean/wer\endcsname{4.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_mix/dele\endcsname{4.92}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_mix/ins\endcsname{36.42}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_mix/leak_wpm\endcsname{116.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_mix/miss\endcsname{17.39}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/call_dev_mix/wer\endcsname{53.81}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/dev4\endcsname{11.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/krisp/dele\endcsname{1.34}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/krisp/leak_wpm\endcsname{0.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/krisp/miss\endcsname{4.95}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/krisp/wer\endcsname{5.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/meet3\endcsname{13.43}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/nsf_dev/dele\endcsname{1.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/nsf_dev/ins\endcsname{1.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/nsf_dev/miss\endcsname{5.75}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlf_selfl/nsf_dev/wer\endcsname{7.58}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/aic_calls/dele\endcsname{2.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/aic_calls/ins\endcsname{7.88}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/aic_calls/leak_wpm\endcsname{8.20}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/aic_calls/miss\endcsname{6.63}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/aic_calls/wer\endcsname{14.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev/dele\endcsname{3.08}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev/ins\endcsname{4.13}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev/leak_wpm\endcsname{9.15}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev/miss\endcsname{9.06}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev/wer\endcsname{13.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev_long/dele\endcsname{5.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev_long/ins\endcsname{7.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev_long/leak_wpm\endcsname{11.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev_long/miss\endcsname{13.29}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/ami_dev_long/wer\endcsname{21.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_clean/dele\endcsname{2.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_clean/miss\endcsname{3.37}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_clean/wer\endcsname{3.61}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_mix/dele\endcsname{3.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_mix/ins\endcsname{34.89}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_mix/leak_wpm\endcsname{99.42}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_mix/miss\endcsname{14.88}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/call_dev_mix/wer\endcsname{49.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/dev4\endcsname{11.43}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/krisp/dele\endcsname{1.36}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/krisp/ins\endcsname{1.09}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/krisp/leak_wpm\endcsname{1.39}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/krisp/miss\endcsname{4.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/krisp/wer\endcsname{5.85}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/meet3\endcsname{14.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/nsf_dev/miss\endcsname{5.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null/nsf_dev/wer\endcsname{7.72}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null_pr1/call_dev_clean/dele\endcsname{1.58}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null_pr1/call_dev_clean/ins\endcsname{0.22}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null_pr1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null_pr1/call_dev_clean/miss\endcsname{2.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_null_pr1/call_dev_clean/wer\endcsname{2.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/aic_calls/dele\endcsname{2.71}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/aic_calls/ins\endcsname{7.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/aic_calls/leak_wpm\endcsname{7.95}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/aic_calls/miss\endcsname{6.52}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/aic_calls/wer\endcsname{14.36}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev/dele\endcsname{3.25}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev/ins\endcsname{3.91}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev/leak_wpm\endcsname{8.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev/miss\endcsname{9.09}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev/wer\endcsname{13.00}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev_long/dele\endcsname{6.86}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev_long/ins\endcsname{3.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev_long/leak_wpm\endcsname{5.81}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev_long/miss\endcsname{14.39}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/ami_dev_long/wer\endcsname{17.59}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_clean/dele\endcsname{2.82}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_clean/ins\endcsname{0.29}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_clean/miss\endcsname{3.63}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_clean/wer\endcsname{3.92}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_mix/dele\endcsname{3.75}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_mix/ins\endcsname{34.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_mix/leak_wpm\endcsname{112.98}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_mix/miss\endcsname{16.54}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/call_dev_mix/wer\endcsname{51.05}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/dev4\endcsname{10.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/krisp/dele\endcsname{1.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/krisp/ins\endcsname{0.71}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/krisp/leak_wpm\endcsname{0.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/krisp/miss\endcsname{4.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/krisp/wer\endcsname{5.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/meet3\endcsname{12.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/nsf_dev/dele\endcsname{1.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/nsf_dev/miss\endcsname{5.75}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl/nsf_dev/wer\endcsname{7.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/aic_calls/dele\endcsname{2.96}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/aic_calls/ins\endcsname{8.09}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/aic_calls/leak_wpm\endcsname{7.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/aic_calls/miss\endcsname{6.52}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/aic_calls/wer\endcsname{14.61}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev/dele\endcsname{3.08}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev/ins\endcsname{3.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev/leak_wpm\endcsname{8.44}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev/miss\endcsname{9.18}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev/wer\endcsname{12.94}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev_long/dele\endcsname{6.54}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev_long/ins\endcsname{3.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev_long/leak_wpm\endcsname{5.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev_long/miss\endcsname{14.10}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/ami_dev_long/wer\endcsname{17.30}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_clean/dele\endcsname{2.68}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_clean/ins\endcsname{0.29}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_clean/miss\endcsname{3.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_clean/wer\endcsname{3.85}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_mix/dele\endcsname{3.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_mix/ins\endcsname{35.12}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_mix/leak_wpm\endcsname{111.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_mix/miss\endcsname{16.02}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/call_dev_mix/wer\endcsname{51.14}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/dev4\endcsname{10.43}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/krisp/dele\endcsname{1.49}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/krisp/leak_wpm\endcsname{0.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/krisp/miss\endcsname{4.91}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/krisp/wer\endcsname{5.63}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/meet3\endcsname{12.63}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/nsf_dev/miss\endcsname{5.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl1/nsf_dev/wer\endcsname{7.64}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev/dele\endcsname{3.20}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev/ins\endcsname{3.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev/leak_wpm\endcsname{8.30}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev/miss\endcsname{9.13}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev/wer\endcsname{13.03}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev_long/dele\endcsname{6.92}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev_long/ins\endcsname{3.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev_long/leak_wpm\endcsname{5.82}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev_long/miss\endcsname{14.39}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/ami_dev_long/wer\endcsname{17.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_clean/dele\endcsname{2.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_clean/miss\endcsname{3.58}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_clean/wer\endcsname{3.88}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_mix/dele\endcsname{3.75}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_mix/ins\endcsname{34.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_mix/leak_wpm\endcsname{112.98}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_mix/miss\endcsname{16.32}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/call_dev_mix/wer\endcsname{51.17}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/dev4\endcsname{10.52}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/krisp/dele\endcsname{1.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/krisp/leak_wpm\endcsname{0.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/krisp/miss\endcsname{4.88}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/krisp/wer\endcsname{5.58}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/meet3\endcsname{12.73}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/nsf_dev/miss\endcsname{5.72}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl2/nsf_dev/wer\endcsname{7.66}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev/dele\endcsname{2.82}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev/ins\endcsname{26.08}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev/leak_wpm\endcsname{75.27}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev/miss\endcsname{9.43}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev/wer\endcsname{35.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev_long/dele\endcsname{5.00}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev_long/ins\endcsname{88.28}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev_long/leak_wpm\endcsname{109.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev_long/miss\endcsname{14.94}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/ami_dev_long/wer\endcsname{103.22}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_clean/dele\endcsname{1.18}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_clean/miss\endcsname{1.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_clean/wer\endcsname{1.92}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_mix/dele\endcsname{2.17}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_mix/ins\endcsname{58.38}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_mix/leak_wpm\endcsname{146.66}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_mix/miss\endcsname{12.15}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/call_dev_mix/wer\endcsname{70.53}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/dev4\endcsname{39.95}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/krisp/dele\endcsname{0.72}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/krisp/ins\endcsname{8.75}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/krisp/leak_wpm\endcsname{29.97}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/krisp/miss\endcsname{4.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/krisp/wer\endcsname{12.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/meet3\endcsname{52.63}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/nsf_dev/dele\endcsname{1.94}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/nsf_dev/ins\endcsname{12.71}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/nsf_dev/leak_wpm\endcsname{38.89}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/nsf_dev/miss\endcsname{6.44}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa20/nsf_dev/wer\endcsname{19.16}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev/dele\endcsname{3.38}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev/ins\endcsname{21.27}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev/leak_wpm\endcsname{59.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev/miss\endcsname{9.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev/wer\endcsname{30.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev_long/dele\endcsname{4.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev_long/ins\endcsname{68.17}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev_long/leak_wpm\endcsname{85.37}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev_long/miss\endcsname{13.96}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/ami_dev_long/wer\endcsname{82.13}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_clean/dele\endcsname{1.27}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_clean/ins\endcsname{0.20}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_clean/miss\endcsname{1.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_clean/wer\endcsname{1.96}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_mix/dele\endcsname{2.71}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_mix/ins\endcsname{55.37}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_mix/leak_wpm\endcsname{142.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_mix/miss\endcsname{12.33}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/call_dev_mix/wer\endcsname{67.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/dev4\endcsname{31.14}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/krisp/dele\endcsname{0.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/krisp/ins\endcsname{3.67}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/krisp/leak_wpm\endcsname{11.18}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/krisp/miss\endcsname{4.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/krisp/wer\endcsname{7.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/meet3\endcsname{40.86}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/nsf_dev/ins\endcsname{3.85}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/nsf_dev/leak_wpm\endcsname{7.20}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/nsf_dev/miss\endcsname{5.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_oa30/nsf_dev/wer\endcsname{9.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev/dele\endcsname{3.33}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev/ins\endcsname{4.52}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev/leak_wpm\endcsname{9.06}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev/miss\endcsname{8.96}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev/wer\endcsname{13.48}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev_long/dele\endcsname{7.80}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev_long/ins\endcsname{3.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev_long/leak_wpm\endcsname{5.89}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev_long/miss\endcsname{15.25}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/ami_dev_long/wer\endcsname{18.66}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/call_dev_clean/dele\endcsname{1.82}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/call_dev_clean/miss\endcsname{2.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/call_dev_clean/wer\endcsname{2.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/dev4\endcsname{10.65}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/meet3\endcsname{13.29}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/nsf_dev/dele\endcsname{1.42}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/nsf_dev/ins\endcsname{1.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/nsf_dev/miss\endcsname{5.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pr1/nsf_dev/wer\endcsname{7.73}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev/dele\endcsname{3.91}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev/ins\endcsname{4.37}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev/leak_wpm\endcsname{7.95}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev/miss\endcsname{9.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev/wer\endcsname{14.14}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev_long/dele\endcsname{9.91}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev_long/ins\endcsname{3.98}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev_long/leak_wpm\endcsname{6.42}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev_long/miss\endcsname{17.87}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/ami_dev_long/wer\endcsname{21.85}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_clean/dele\endcsname{1.67}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_clean/miss\endcsname{2.33}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_clean/wer\endcsname{2.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_mix/dele\endcsname{3.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_mix/ins\endcsname{36.09}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_mix/leak_wpm\endcsname{112.15}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_mix/miss\endcsname{15.38}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/call_dev_mix/wer\endcsname{51.46}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/dev4\endcsname{11.64}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/krisp/dele\endcsname{1.40}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/krisp/ins\endcsname{0.71}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/krisp/leak_wpm\endcsname{0.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/krisp/miss\endcsname{4.80}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/krisp/wer\endcsname{5.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/meet3\endcsname{14.67}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/nsf_dev/dele\endcsname{1.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/nsf_dev/ins\endcsname{1.86}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/nsf_dev/miss\endcsname{6.16}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt3/nsf_dev/wer\endcsname{8.03}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev/dele\endcsname{3.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev/ins\endcsname{6.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev/leak_wpm\endcsname{13.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev/miss\endcsname{9.88}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev/wer\endcsname{16.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev_long/dele\endcsname{9.81}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev_long/ins\endcsname{6.24}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev_long/leak_wpm\endcsname{9.00}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev_long/miss\endcsname{17.61}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/ami_dev_long/wer\endcsname{23.85}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_clean/dele\endcsname{1.58}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_clean/miss\endcsname{2.21}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_clean/wer\endcsname{2.44}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_mix/dele\endcsname{3.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_mix/ins\endcsname{36.15}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_mix/leak_wpm\endcsname{112.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_mix/miss\endcsname{15.35}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/call_dev_mix/wer\endcsname{51.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/dev4\endcsname{13.07}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/krisp/dele\endcsname{1.36}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/krisp/miss\endcsname{4.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/krisp/wer\endcsname{5.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/meet3\endcsname{16.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/nsf_dev/dele\endcsname{1.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/nsf_dev/ins\endcsname{3.30}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/nsf_dev/leak_wpm\endcsname{4.73}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/nsf_dev/miss\endcsname{6.08}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfl_pt5/nsf_dev/wer\endcsname{9.39}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls/call_dev_clean/dele\endcsname{3.01}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls/call_dev_clean/ins\endcsname{0.32}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls/call_dev_clean/miss\endcsname{3.86}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls/call_dev_clean/wer\endcsname{4.18}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev/dele\endcsname{3.34}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev/ins\endcsname{4.43}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev/leak_wpm\endcsname{8.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev/miss\endcsname{9.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev/wer\endcsname{13.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev_long/dele\endcsname{8.43}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev_long/ins\endcsname{3.45}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev_long/leak_wpm\endcsname{5.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev_long/miss\endcsname{15.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/ami_dev_long/wer\endcsname{19.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/call_dev_clean/dele\endcsname{1.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/call_dev_clean/ins\endcsname{0.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/call_dev_clean/miss\endcsname{2.28}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/call_dev_clean/wer\endcsname{2.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/dev4\endcsname{10.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/meet3\endcsname{13.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/nsf_dev/dele\endcsname{1.42}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/nsf_dev/ins\endcsname{1.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/nsf_dev/miss\endcsname{5.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2_selfls_pr1/nsf_dev/wer\endcsname{7.73}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev/dele\endcsname{2.94}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev/ins\endcsname{4.52}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev/leak_wpm\endcsname{9.46}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev/miss\endcsname{8.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev/wer\endcsname{13.30}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev_long/dele\endcsname{7.28}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev_long/ins\endcsname{3.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev_long/leak_wpm\endcsname{6.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev_long/miss\endcsname{14.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/ami_dev_long/wer\endcsname{18.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_clean/dele\endcsname{2.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_clean/ins\endcsname{0.20}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_clean/miss\endcsname{3.45}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_clean/wer\endcsname{3.66}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_mix/dele\endcsname{3.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_mix/ins\endcsname{36.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_mix/leak_wpm\endcsname{115.03}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_mix/miss\endcsname{17.67}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/call_dev_mix/wer\endcsname{54.22}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/dev4\endcsname{10.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/krisp/dele\endcsname{1.16}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/krisp/ins\endcsname{0.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/krisp/leak_wpm\endcsname{0.33}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/krisp/miss\endcsname{4.73}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/krisp/wer\endcsname{5.49}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/meet3\endcsname{13.16}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/nsf_dev/dele\endcsname{1.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/nsf_dev/miss\endcsname{5.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g5_selfl/nsf_dev/wer\endcsname{7.71}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev/dele\endcsname{3.01}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev/ins\endcsname{4.09}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev/leak_wpm\endcsname{8.48}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev/miss\endcsname{8.97}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev/wer\endcsname{13.07}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev_long/dele\endcsname{7.28}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev_long/ins\endcsname{3.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev_long/leak_wpm\endcsname{5.86}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev_long/miss\endcsname{14.53}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/ami_dev_long/wer\endcsname{17.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_clean/dele\endcsname{3.80}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_clean/ins\endcsname{0.33}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_clean/miss\endcsname{4.54}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_clean/wer\endcsname{4.88}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_mix/dele\endcsname{4.05}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_mix/ins\endcsname{33.12}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_mix/leak_wpm\endcsname{115.03}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_mix/miss\endcsname{17.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/call_dev_mix/wer\endcsname{50.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/dev4\endcsname{10.89}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/krisp/dele\endcsname{1.38}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/krisp/miss\endcsname{4.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/krisp/wer\endcsname{5.54}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/meet3\endcsname{12.89}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/nsf_dev/ins\endcsname{1.95}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/nsf_dev/miss\endcsname{5.86}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2g_selfl/nsf_dev/wer\endcsname{7.82}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev/dele\endcsname{3.01}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev/ins\endcsname{4.91}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev/leak_wpm\endcsname{9.82}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev/miss\endcsname{8.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev/wer\endcsname{13.48}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/dele\endcsname{7.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/ins\endcsname{4.01}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/leak_wpm\endcsname{7.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/miss\endcsname{15.59}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/wer\endcsname{19.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/dele\endcsname{1.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/ins\endcsname{0.27}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/miss\endcsname{2.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/wer\endcsname{2.32}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/dele\endcsname{3.17}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/ins\endcsname{37.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/leak_wpm\endcsname{119.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/miss\endcsname{16.67}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/wer\endcsname{54.22}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/dev4\endcsname{10.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/krisp/dele\endcsname{1.00}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/krisp/leak_wpm\endcsname{0.29}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/krisp/miss\endcsname{4.54}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/krisp/wer\endcsname{5.27}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/meet3\endcsname{13.61}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/nsf_dev/dele\endcsname{1.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/nsf_dev/ins\endcsname{1.98}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/nsf_dev/miss\endcsname{5.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2gm_selfl/nsf_dev/wer\endcsname{7.75}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev/dele\endcsname{3.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev/ins\endcsname{4.23}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev/leak_wpm\endcsname{7.95}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev/miss\endcsname{8.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev/wer\endcsname{13.00}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev_long/dele\endcsname{6.73}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev_long/ins\endcsname{5.31}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev_long/leak_wpm\endcsname{8.83}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev_long/miss\endcsname{14.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/ami_dev_long/wer\endcsname{19.87}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_clean/dele\endcsname{1.64}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_clean/miss\endcsname{2.20}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_clean/wer\endcsname{2.46}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_mix/dele\endcsname{3.30}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_mix/ins\endcsname{34.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_mix/leak_wpm\endcsname{103.12}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_mix/miss\endcsname{15.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/call_dev_mix/wer\endcsname{50.13}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/dev4\endcsname{10.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/krisp/dele\endcsname{1.22}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/krisp/ins\endcsname{0.68}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/krisp/miss\endcsname{4.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/krisp/wer\endcsname{5.30}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/meet3\endcsname{13.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/nsf_dev/dele\endcsname{1.58}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/nsf_dev/ins\endcsname{1.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/nsf_dev/miss\endcsname{5.95}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2hm_selfl/nsf_dev/wer\endcsname{7.85}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/aic_calls/dele\endcsname{2.82}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/aic_calls/ins\endcsname{8.27}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/aic_calls/leak_wpm\endcsname{8.45}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/aic_calls/miss\endcsname{6.20}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/aic_calls/wer\endcsname{14.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev/dele\endcsname{3.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev/ins\endcsname{4.15}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev/leak_wpm\endcsname{8.44}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev/miss\endcsname{9.14}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev/wer\endcsname{13.29}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev_long/dele\endcsname{6.34}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev_long/ins\endcsname{8.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev_long/leak_wpm\endcsname{12.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev_long/miss\endcsname{14.15}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/ami_dev_long/wer\endcsname{22.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_clean/dele\endcsname{1.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_clean/miss\endcsname{2.39}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_clean/wer\endcsname{2.62}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_mix/dele\endcsname{2.81}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_mix/ins\endcsname{33.17}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_mix/leak_wpm\endcsname{91.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_mix/miss\endcsname{15.58}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/call_dev_mix/wer\endcsname{48.75}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/dev4\endcsname{11.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/krisp/dele\endcsname{1.59}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/krisp/ins\endcsname{1.14}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/krisp/leak_wpm\endcsname{1.80}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/krisp/miss\endcsname{5.14}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/krisp/wer\endcsname{6.28}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/meet3\endcsname{14.54}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/nsf_dev/dele\endcsname{1.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/nsf_dev/miss\endcsname{5.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_null/nsf_dev/wer\endcsname{7.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/aic_calls/dele\endcsname{2.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/aic_calls/ins\endcsname{8.52}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/aic_calls/leak_wpm\endcsname{8.39}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/aic_calls/miss\endcsname{5.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/aic_calls/wer\endcsname{14.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev/dele\endcsname{3.29}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev/ins\endcsname{4.16}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev/leak_wpm\endcsname{9.15}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev/miss\endcsname{9.07}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev/wer\endcsname{13.23}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev_long/dele\endcsname{7.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev_long/ins\endcsname{2.98}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev_long/leak_wpm\endcsname{5.63}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev_long/miss\endcsname{15.02}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/ami_dev_long/wer\endcsname{18.00}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_clean/dele\endcsname{1.96}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_clean/ins\endcsname{0.25}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_clean/miss\endcsname{2.71}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_clean/wer\endcsname{2.96}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_mix/dele\endcsname{3.54}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_mix/ins\endcsname{34.88}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_mix/leak_wpm\endcsname{110.10}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_mix/miss\endcsname{16.44}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/call_dev_mix/wer\endcsname{51.32}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/dev4\endcsname{10.49}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/krisp/dele\endcsname{1.57}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/krisp/ins\endcsname{0.67}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/krisp/miss\endcsname{5.08}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/krisp/wer\endcsname{5.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/meet3\endcsname{13.00}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/nsf_dev/ins\endcsname{1.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/nsf_dev/miss\endcsname{5.87}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl/nsf_dev/wer\endcsname{7.77}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev/dele\endcsname{3.16}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev/ins\endcsname{4.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev/leak_wpm\endcsname{8.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev/miss\endcsname{9.03}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev/wer\endcsname{13.07}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev_long/dele\endcsname{7.74}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev_long/ins\endcsname{3.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev_long/leak_wpm\endcsname{5.66}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev_long/miss\endcsname{14.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/ami_dev_long/wer\endcsname{18.10}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_clean/dele\endcsname{2.02}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_clean/miss\endcsname{2.84}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_clean/wer\endcsname{3.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_mix/dele\endcsname{3.81}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_mix/ins\endcsname{34.93}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_mix/leak_wpm\endcsname{114.00}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_mix/miss\endcsname{16.94}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/call_dev_mix/wer\endcsname{51.87}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/dev4\endcsname{10.52}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/krisp/dele\endcsname{1.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/krisp/ins\endcsname{0.67}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/krisp/miss\endcsname{5.12}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/krisp/wer\endcsname{5.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/meet3\endcsname{12.99}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/nsf_dev/ins\endcsname{1.92}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/nsf_dev/miss\endcsname{5.87}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2m_selfl1/nsf_dev/wer\endcsname{7.79}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/dele\endcsname{3.08}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/ins\endcsname{4.27}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/leak_wpm\endcsname{9.20}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/miss\endcsname{8.81}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev/wer\endcsname{13.08}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/dele\endcsname{8.16}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/ins\endcsname{2.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/leak_wpm\endcsname{5.65}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/miss\endcsname{15.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/wer\endcsname{18.66}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/dele\endcsname{1.83}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/ins\endcsname{0.22}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/miss\endcsname{2.46}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/wer\endcsname{2.68}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/dev4\endcsname{10.54}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/krisp/dele\endcsname{1.44}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/krisp/ins\endcsname{0.76}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/krisp/leak_wpm\endcsname{0.22}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/krisp/miss\endcsname{4.87}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/krisp/wer\endcsname{5.63}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/meet3\endcsname{13.16}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2mr_selfl/nsf_dev/wer\endcsname{7.73}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev/dele\endcsname{2.98}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev/ins\endcsname{3.98}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev/leak_wpm\endcsname{8.66}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev/miss\endcsname{9.03}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev/wer\endcsname{13.01}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev_long/dele\endcsname{7.01}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev_long/ins\endcsname{3.16}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev_long/leak_wpm\endcsname{5.87}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev_long/miss\endcsname{14.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/ami_dev_long/wer\endcsname{17.56}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/call_dev_clean/dele\endcsname{3.26}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/call_dev_clean/ins\endcsname{0.31}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/call_dev_clean/miss\endcsname{3.88}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/call_dev_clean/wer\endcsname{4.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/dev4\endcsname{10.61}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/krisp/dele\endcsname{1.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/krisp/miss\endcsname{4.90}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/krisp/wer\endcsname{5.60}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/meet3\endcsname{12.75}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/nsf_dev/dele\endcsname{1.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/nsf_dev/ins\endcsname{1.91}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/nsf_dev/miss\endcsname{5.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt2r_selfl/nsf_dev/wer\endcsname{7.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev/dele\endcsname{3.07}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev/ins\endcsname{3.44}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev/leak_wpm\endcsname{7.05}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev/miss\endcsname{9.34}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev/wer\endcsname{12.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev_long/dele\endcsname{7.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev_long/ins\endcsname{3.72}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev_long/leak_wpm\endcsname{6.50}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev_long/miss\endcsname{14.98}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/ami_dev_long/wer\endcsname{18.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_clean/dele\endcsname{4.22}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_clean/ins\endcsname{0.19}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_clean/miss\endcsname{5.11}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_clean/wer\endcsname{5.31}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_mix/dele\endcsname{5.01}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_mix/ins\endcsname{30.59}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_mix/leak_wpm\endcsname{114.41}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_mix/miss\endcsname{20.43}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/call_dev_mix/wer\endcsname{51.02}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/dev4\endcsname{11.12}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/krisp/dele\endcsname{1.48}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/krisp/leak_wpm\endcsname{0.02}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/krisp/miss\endcsname{4.98}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/krisp/wer\endcsname{5.69}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/meet3\endcsname{13.05}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/nsf_dev/ins\endcsname{1.91}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/nsf_dev/miss\endcsname{5.78}
\expandafter\def\csname v@r/MB_ftlong_ws_cwlt_selfl/nsf_dev/wer\endcsname{7.69}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev/dele\endcsname{3.00}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev/ins\endcsname{3.73}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev/leak_wpm\endcsname{7.63}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev/miss\endcsname{9.27}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev/wer\endcsname{13.00}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev_long/dele\endcsname{8.25}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev_long/ins\endcsname{4.86}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev_long/leak_wpm\endcsname{7.95}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev_long/miss\endcsname{15.34}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/ami_dev_long/wer\endcsname{20.20}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_clean/dele\endcsname{4.49}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_clean/miss\endcsname{5.66}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_clean/wer\endcsname{5.93}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_mix/dele\endcsname{5.65}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_mix/ins\endcsname{32.07}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_mix/leak_wpm\endcsname{108.05}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_mix/miss\endcsname{19.07}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/call_dev_mix/wer\endcsname{51.14}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/dev4\endcsname{11.69}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/krisp/dele\endcsname{1.57}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/krisp/leak_wpm\endcsname{0.08}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/krisp/miss\endcsname{5.33}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/krisp/wer\endcsname{6.03}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/meet3\endcsname{13.61}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/nsf_dev/dele\endcsname{1.51}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/nsf_dev/ins\endcsname{1.84}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/MB_ftlong_ws_hbl0t_selfl/nsf_dev/wer\endcsname{7.64}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev/dele\endcsname{2.87}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev/ins\endcsname{4.13}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev/leak_wpm\endcsname{8.17}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev/miss\endcsname{8.95}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev/wer\endcsname{13.08}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev_long/dele\endcsname{8.20}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev_long/ins\endcsname{5.71}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev_long/leak_wpm\endcsname{8.95}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev_long/miss\endcsname{15.50}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/ami_dev_long/wer\endcsname{21.22}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_clean/dele\endcsname{3.33}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_clean/miss\endcsname{4.28}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_clean/wer\endcsname{4.52}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_mix/dele\endcsname{4.29}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_mix/ins\endcsname{36.25}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_mix/leak_wpm\endcsname{118.73}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_mix/miss\endcsname{16.84}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/call_dev_mix/wer\endcsname{53.09}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/dev4\endcsname{11.62}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/krisp/dele\endcsname{1.44}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/krisp/leak_wpm\endcsname{0.21}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/krisp/miss\endcsname{5.21}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/krisp/wer\endcsname{5.95}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/meet3\endcsname{13.98}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/nsf_dev/ins\endcsname{1.85}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/MB_ftlong_ws_hbx0t_selfl/nsf_dev/wer\endcsname{7.65}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/aic_calls/dele\endcsname{2.74}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/aic_calls/ins\endcsname{9.16}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/aic_calls/leak_wpm\endcsname{8.83}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/aic_calls/miss\endcsname{6.31}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/aic_calls/wer\endcsname{15.47}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev/dele\endcsname{3.58}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev/ins\endcsname{3.61}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev/leak_wpm\endcsname{7.68}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev/miss\endcsname{9.75}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev/wer\endcsname{13.36}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev_long/dele\endcsname{7.85}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev_long/ins\endcsname{4.73}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev_long/leak_wpm\endcsname{7.74}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev_long/miss\endcsname{14.88}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/ami_dev_long/wer\endcsname{19.61}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/krisp/dele\endcsname{1.26}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/krisp/ins\endcsname{0.84}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/krisp/leak_wpm\endcsname{0.48}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/krisp/miss\endcsname{4.92}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/krisp/wer\endcsname{5.76}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/meet3\endcsname{13.55}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/nsf_dev/ins\endcsname{1.85}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/nsf_dev/miss\endcsname{5.84}
\expandafter\def\csname v@r/MB_ftlong_ws_loud/nsf_dev/wer\endcsname{7.69}
\expandafter\def\csname v@r/MB_ftlong_ws_null/aic_calls/dele\endcsname{2.10}
\expandafter\def\csname v@r/MB_ftlong_ws_null/aic_calls/ins\endcsname{11.12}
\expandafter\def\csname v@r/MB_ftlong_ws_null/aic_calls/leak_wpm\endcsname{13.06}
\expandafter\def\csname v@r/MB_ftlong_ws_null/aic_calls/miss\endcsname{5.74}
\expandafter\def\csname v@r/MB_ftlong_ws_null/aic_calls/wer\endcsname{16.86}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev/dele\endcsname{3.11}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev/ins\endcsname{4.88}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev/leak_wpm\endcsname{9.64}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev/miss\endcsname{9.02}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev/wer\endcsname{13.90}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev_long/dele\endcsname{7.08}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev_long/ins\endcsname{11.76}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev_long/leak_wpm\endcsname{16.02}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev_long/miss\endcsname{14.48}
\expandafter\def\csname v@r/MB_ftlong_ws_null/ami_dev_long/wer\endcsname{26.24}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_clean/dele\endcsname{2.90}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_clean/ins\endcsname{0.22}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_clean/miss\endcsname{3.69}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_clean/wer\endcsname{3.91}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_mix/dele\endcsname{4.05}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_mix/ins\endcsname{38.64}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_mix/leak_wpm\endcsname{94.08}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_mix/miss\endcsname{14.43}
\expandafter\def\csname v@r/MB_ftlong_ws_null/call_dev_mix/wer\endcsname{53.08}
\expandafter\def\csname v@r/MB_ftlong_ws_null/dev4\endcsname{12.91}
\expandafter\def\csname v@r/MB_ftlong_ws_null/krisp/dele\endcsname{1.52}
\expandafter\def\csname v@r/MB_ftlong_ws_null/krisp/ins\endcsname{1.43}
\expandafter\def\csname v@r/MB_ftlong_ws_null/krisp/leak_wpm\endcsname{2.72}
\expandafter\def\csname v@r/MB_ftlong_ws_null/krisp/miss\endcsname{5.12}
\expandafter\def\csname v@r/MB_ftlong_ws_null/krisp/wer\endcsname{6.55}
\expandafter\def\csname v@r/MB_ftlong_ws_null/meet3\endcsname{15.91}
\expandafter\def\csname v@r/MB_ftlong_ws_null/nsf_dev/dele\endcsname{1.54}
\expandafter\def\csname v@r/MB_ftlong_ws_null/nsf_dev/ins\endcsname{1.85}
\expandafter\def\csname v@r/MB_ftlong_ws_null/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/MB_ftlong_ws_null/nsf_dev/miss\endcsname{5.75}
\expandafter\def\csname v@r/MB_ftlong_ws_null/nsf_dev/wer\endcsname{7.59}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/aic_calls/dele\endcsname{2.28}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/aic_calls/ins\endcsname{10.87}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/aic_calls/leak_wpm\endcsname{11.92}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/aic_calls/miss\endcsname{5.70}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/aic_calls/wer\endcsname{16.57}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev/dele\endcsname{2.95}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev/ins\endcsname{4.40}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev/leak_wpm\endcsname{8.30}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev/miss\endcsname{8.78}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev/wer\endcsname{13.18}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev_long/dele\endcsname{7.04}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev_long/ins\endcsname{5.27}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev_long/leak_wpm\endcsname{7.94}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev_long/miss\endcsname{14.19}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/ami_dev_long/wer\endcsname{19.46}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_clean/dele\endcsname{4.30}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_clean/miss\endcsname{5.31}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_clean/wer\endcsname{5.57}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_mix/dele\endcsname{5.47}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_mix/ins\endcsname{35.00}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_mix/leak_wpm\endcsname{105.99}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_mix/miss\endcsname{17.19}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/call_dev_mix/wer\endcsname{52.19}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/dev4\endcsname{11.44}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/krisp/dele\endcsname{1.39}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/krisp/leak_wpm\endcsname{0.21}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/krisp/miss\endcsname{5.05}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/krisp/wer\endcsname{5.79}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/meet3\endcsname{13.40}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/nsf_dev/dele\endcsname{1.49}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/nsf_dev/ins\endcsname{1.83}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/nsf_dev/miss\endcsname{5.73}
\expandafter\def\csname v@r/MB_ftlong_ws_selfl/nsf_dev/wer\endcsname{7.56}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev/dele\endcsname{3.18}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev/ins\endcsname{3.90}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev/leak_wpm\endcsname{7.95}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev/miss\endcsname{9.18}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev/wer\endcsname{13.08}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev_long/dele\endcsname{7.39}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev_long/ins\endcsname{5.97}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev_long/leak_wpm\endcsname{8.91}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev_long/miss\endcsname{14.67}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/ami_dev_long/wer\endcsname{20.64}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_clean/dele\endcsname{5.14}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_clean/miss\endcsname{6.36}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_clean/wer\endcsname{6.66}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_mix/dele\endcsname{5.59}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_mix/ins\endcsname{32.48}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_mix/leak_wpm\endcsname{111.13}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_mix/miss\endcsname{18.58}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/call_dev_mix/wer\endcsname{51.06}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/dev4\endcsname{12.00}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/krisp/dele\endcsname{1.51}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/krisp/ins\endcsname{0.68}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/krisp/leak_wpm\endcsname{0.02}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/krisp/miss\endcsname{5.36}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/krisp/wer\endcsname{6.03}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/meet3\endcsname{13.78}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/nsf_dev/ins\endcsname{1.87}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/nsf_dev/miss\endcsname{5.76}
\expandafter\def\csname v@r/MB_ftlong_ws_sslb_selfl/nsf_dev/wer\endcsname{7.63}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev/dele\endcsname{2.98}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev/ins\endcsname{3.95}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev/leak_wpm\endcsname{8.17}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev/miss\endcsname{8.93}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev/wer\endcsname{12.89}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev_long/dele\endcsname{6.33}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev_long/ins\endcsname{5.73}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev_long/leak_wpm\endcsname{9.07}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev_long/miss\endcsname{13.78}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/ami_dev_long/wer\endcsname{19.51}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_clean/dele\endcsname{4.03}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_clean/miss\endcsname{5.19}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_clean/wer\endcsname{5.42}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_mix/dele\endcsname{4.92}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_mix/ins\endcsname{36.56}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_mix/leak_wpm\endcsname{113.18}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_mix/miss\endcsname{16.20}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/call_dev_mix/wer\endcsname{52.77}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/dev4\endcsname{11.35}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/krisp/dele\endcsname{1.47}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/krisp/leak_wpm\endcsname{0.15}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/krisp/miss\endcsname{5.13}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/krisp/wer\endcsname{5.87}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/meet3\endcsname{13.32}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/nsf_dev/dele\endcsname{1.49}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/nsf_dev/ins\endcsname{1.84}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/nsf_dev/miss\endcsname{5.73}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b0t_selfl/nsf_dev/wer\endcsname{7.57}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev/dele\endcsname{3.29}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev/ins\endcsname{3.86}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev/leak_wpm\endcsname{7.77}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev/miss\endcsname{9.13}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev/wer\endcsname{12.98}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev_long/dele\endcsname{6.49}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev_long/ins\endcsname{5.19}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev_long/leak_wpm\endcsname{8.07}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev_long/miss\endcsname{13.97}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/ami_dev_long/wer\endcsname{19.17}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_clean/dele\endcsname{4.70}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_clean/ins\endcsname{0.19}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_clean/miss\endcsname{5.56}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_clean/wer\endcsname{5.75}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_mix/dele\endcsname{4.31}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_mix/ins\endcsname{32.07}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_mix/leak_wpm\endcsname{114.21}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_mix/miss\endcsname{19.44}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/call_dev_mix/wer\endcsname{51.51}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/dev4\endcsname{11.40}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/krisp/dele\endcsname{1.37}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/krisp/ins\endcsname{0.92}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/krisp/leak_wpm\endcsname{0.81}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/krisp/miss\endcsname{4.87}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/krisp/wer\endcsname{5.79}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/meet3\endcsname{13.28}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/nsf_dev/dele\endcsname{1.43}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/nsf_dev/ins\endcsname{1.98}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/nsf_dev/miss\endcsname{5.72}
\expandafter\def\csname v@r/MB_ftlong_ws_w2b2_selfl/nsf_dev/wer\endcsname{7.70}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev/dele\endcsname{3.16}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev/ins\endcsname{3.87}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev/leak_wpm\endcsname{7.72}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev/miss\endcsname{9.16}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev/wer\endcsname{13.03}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev_long/dele\endcsname{7.43}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev_long/ins\endcsname{4.82}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev_long/leak_wpm\endcsname{7.47}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev_long/miss\endcsname{14.67}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/ami_dev_long/wer\endcsname{19.50}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_clean/dele\endcsname{4.97}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_clean/ins\endcsname{0.35}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_clean/miss\endcsname{6.40}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_clean/wer\endcsname{6.75}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_mix/dele\endcsname{5.72}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_mix/ins\endcsname{32.49}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_mix/leak_wpm\endcsname{113.59}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_mix/miss\endcsname{19.55}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/call_dev_mix/wer\endcsname{52.04}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/dev4\endcsname{11.74}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/krisp/dele\endcsname{1.85}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/krisp/leak_wpm\endcsname{0.07}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/krisp/miss\endcsname{5.72}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/krisp/wer\endcsname{6.45}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/meet3\endcsname{13.40}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/nsf_dev/dele\endcsname{1.61}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/nsf_dev/ins\endcsname{1.80}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/nsf_dev/miss\endcsname{5.87}
\expandafter\def\csname v@r/MB_ftlong_ws_whs0t_selfl/nsf_dev/wer\endcsname{7.68}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev/dele\endcsname{2.84}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev/ins\endcsname{3.95}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev/leak_wpm\endcsname{7.68}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev/miss\endcsname{9.09}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev/wer\endcsname{13.04}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev_long/dele\endcsname{8.04}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev_long/ins\endcsname{4.25}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev_long/leak_wpm\endcsname{7.07}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev_long/miss\endcsname{15.18}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/ami_dev_long/wer\endcsname{19.43}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_clean/dele\endcsname{3.49}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_clean/ins\endcsname{0.25}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_clean/miss\endcsname{4.54}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_clean/wer\endcsname{4.79}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_mix/dele\endcsname{4.30}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_mix/ins\endcsname{33.65}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_mix/leak_wpm\endcsname{109.28}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_mix/miss\endcsname{16.10}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/call_dev_mix/wer\endcsname{49.74}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/dev4\endcsname{11.24}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/krisp/dele\endcsname{1.22}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/krisp/ins\endcsname{0.81}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/krisp/leak_wpm\endcsname{0.36}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/krisp/miss\endcsname{4.83}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/krisp/wer\endcsname{5.64}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/meet3\endcsname{13.39}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/nsf_dev/ins\endcsname{1.88}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/nsf_dev/leak_wpm\endcsname{0.38}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/nsf_dev/miss\endcsname{5.82}
\expandafter\def\csname v@r/MB_ftlong_ws_whs2_selfl/nsf_dev/wer\endcsname{7.70}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev/dele\endcsname{2.93}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev/ins\endcsname{3.93}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev/leak_wpm\endcsname{7.23}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev/miss\endcsname{8.77}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev/wer\endcsname{12.69}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev_long/dele\endcsname{6.78}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev_long/ins\endcsname{4.61}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev_long/leak_wpm\endcsname{7.26}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev_long/miss\endcsname{14.14}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/ami_dev_long/wer\endcsname{18.75}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_clean/dele\endcsname{2.84}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_clean/ins\endcsname{0.29}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_clean/miss\endcsname{3.85}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_clean/wer\endcsname{4.13}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_mix/dele\endcsname{4.11}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_mix/ins\endcsname{34.59}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_mix/leak_wpm\endcsname{104.76}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_mix/miss\endcsname{15.89}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/call_dev_mix/wer\endcsname{50.48}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/dev4\endcsname{10.82}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/krisp/dele\endcsname{1.24}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/krisp/ins\endcsname{0.69}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/krisp/leak_wpm\endcsname{0.02}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/krisp/miss\endcsname{4.82}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/krisp/wer\endcsname{5.51}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/meet3\endcsname{13.05}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/nsf_dev/ins\endcsname{1.88}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/nsf_dev/miss\endcsname{5.82}
\expandafter\def\csname v@r/MB_ftlong_ws_xls0t_selfl/nsf_dev/wer\endcsname{7.70}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev/dele\endcsname{3.07}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev/ins\endcsname{5.60}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev/leak_wpm\endcsname{10.94}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev/miss\endcsname{9.02}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev/wer\endcsname{14.62}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev_long/dele\endcsname{7.71}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev_long/ins\endcsname{8.74}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev_long/leak_wpm\endcsname{11.97}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev_long/miss\endcsname{15.13}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/ami_dev_long/wer\endcsname{23.88}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_clean/dele\endcsname{2.52}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_clean/ins\endcsname{0.19}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_clean/miss\endcsname{3.24}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_clean/wer\endcsname{3.43}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_mix/dele\endcsname{3.51}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_mix/ins\endcsname{41.38}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_mix/leak_wpm\endcsname{122.42}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_mix/miss\endcsname{15.01}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/call_dev_mix/wer\endcsname{56.39}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/dev4\endcsname{12.48}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/krisp/dele\endcsname{0.97}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/krisp/ins\endcsname{0.75}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/krisp/leak_wpm\endcsname{0.21}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/krisp/miss\endcsname{4.35}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/krisp/wer\endcsname{5.10}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/meet3\endcsname{15.49}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/nsf_dev/ins\endcsname{2.17}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/nsf_dev/leak_wpm\endcsname{1.36}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/MB_ftlong_wsp_selfl/nsf_dev/wer\endcsname{7.98}
\expandafter\def\csname v@r/SB_base_null/ami_dev/dele\endcsname{6.03}
\expandafter\def\csname v@r/SB_base_null/ami_dev/ins\endcsname{3.32}
\expandafter\def\csname v@r/SB_base_null/ami_dev/leak_wpm\endcsname{8.57}
\expandafter\def\csname v@r/SB_base_null/ami_dev/miss\endcsname{12.87}
\expandafter\def\csname v@r/SB_base_null/ami_dev/wer\endcsname{16.19}
\expandafter\def\csname v@r/SB_base_null/ami_dev_long/dele\endcsname{6.62}
\expandafter\def\csname v@r/SB_base_null/ami_dev_long/ins\endcsname{40.91}
\expandafter\def\csname v@r/SB_base_null/ami_dev_long/leak_wpm\endcsname{53.26}
\expandafter\def\csname v@r/SB_base_null/ami_dev_long/miss\endcsname{14.94}
\expandafter\def\csname v@r/SB_base_null/ami_dev_long/wer\endcsname{55.85}
\expandafter\def\csname v@r/SB_base_null/call_dev_clean/dele\endcsname{4.78}
\expandafter\def\csname v@r/SB_base_null/call_dev_clean/ins\endcsname{0.22}
\expandafter\def\csname v@r/SB_base_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_base_null/call_dev_clean/miss\endcsname{5.75}
\expandafter\def\csname v@r/SB_base_null/call_dev_clean/wer\endcsname{5.96}
\expandafter\def\csname v@r/SB_base_null/call_dev_mix/dele\endcsname{4.29}
\expandafter\def\csname v@r/SB_base_null/call_dev_mix/ins\endcsname{45.31}
\expandafter\def\csname v@r/SB_base_null/call_dev_mix/leak_wpm\endcsname{129.20}
\expandafter\def\csname v@r/SB_base_null/call_dev_mix/miss\endcsname{15.59}
\expandafter\def\csname v@r/SB_base_null/call_dev_mix/wer\endcsname{60.90}
\expandafter\def\csname v@r/SB_base_null/dev4\endcsname{21.75}
\expandafter\def\csname v@r/SB_base_null/krisp/dele\endcsname{3.10}
\expandafter\def\csname v@r/SB_base_null/krisp/ins\endcsname{4.73}
\expandafter\def\csname v@r/SB_base_null/krisp/leak_wpm\endcsname{15.86}
\expandafter\def\csname v@r/SB_base_null/krisp/miss\endcsname{7.06}
\expandafter\def\csname v@r/SB_base_null/krisp/wer\endcsname{11.79}
\expandafter\def\csname v@r/SB_base_null/meet3\endcsname{27.01}
\expandafter\def\csname v@r/SB_base_null/nsf_dev/dele\endcsname{2.91}
\expandafter\def\csname v@r/SB_base_null/nsf_dev/ins\endcsname{1.70}
\expandafter\def\csname v@r/SB_base_null/nsf_dev/leak_wpm\endcsname{0.38}
\expandafter\def\csname v@r/SB_base_null/nsf_dev/miss\endcsname{7.29}
\expandafter\def\csname v@r/SB_base_null/nsf_dev/wer\endcsname{8.99}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev/dele\endcsname{5.49}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev/ins\endcsname{3.44}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev/leak_wpm\endcsname{8.66}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev/miss\endcsname{12.25}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev/wer\endcsname{15.69}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev_long/dele\endcsname{6.55}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev_long/ins\endcsname{19.01}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev_long/leak_wpm\endcsname{26.19}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev_long/miss\endcsname{14.85}
\expandafter\def\csname v@r/SB_base_selfl/ami_dev_long/wer\endcsname{33.87}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_clean/dele\endcsname{5.71}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_clean/ins\endcsname{0.29}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_clean/miss\endcsname{6.87}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_clean/wer\endcsname{7.16}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_mix/dele\endcsname{5.22}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_mix/ins\endcsname{44.39}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_mix/leak_wpm\endcsname{131.87}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_mix/miss\endcsname{17.24}
\expandafter\def\csname v@r/SB_base_selfl/call_dev_mix/wer\endcsname{61.63}
\expandafter\def\csname v@r/SB_base_selfl/dev4\endcsname{16.36}
\expandafter\def\csname v@r/SB_base_selfl/krisp/dele\endcsname{1.56}
\expandafter\def\csname v@r/SB_base_selfl/krisp/ins\endcsname{2.79}
\expandafter\def\csname v@r/SB_base_selfl/krisp/leak_wpm\endcsname{8.05}
\expandafter\def\csname v@r/SB_base_selfl/krisp/miss\endcsname{5.37}
\expandafter\def\csname v@r/SB_base_selfl/krisp/wer\endcsname{8.16}
\expandafter\def\csname v@r/SB_base_selfl/meet3\endcsname{19.42}
\expandafter\def\csname v@r/SB_base_selfl/nsf_dev/dele\endcsname{2.66}
\expandafter\def\csname v@r/SB_base_selfl/nsf_dev/ins\endcsname{1.77}
\expandafter\def\csname v@r/SB_base_selfl/nsf_dev/leak_wpm\endcsname{0.34}
\expandafter\def\csname v@r/SB_base_selfl/nsf_dev/miss\endcsname{6.94}
\expandafter\def\csname v@r/SB_base_selfl/nsf_dev/wer\endcsname{8.71}
\expandafter\def\csname v@r/SB_ft_null/ami_dev/dele\endcsname{3.61}
\expandafter\def\csname v@r/SB_ft_null/ami_dev/ins\endcsname{4.47}
\expandafter\def\csname v@r/SB_ft_null/ami_dev/leak_wpm\endcsname{9.96}
\expandafter\def\csname v@r/SB_ft_null/ami_dev/miss\endcsname{9.54}
\expandafter\def\csname v@r/SB_ft_null/ami_dev/wer\endcsname{14.01}
\expandafter\def\csname v@r/SB_ft_null/ami_dev_long/dele\endcsname{2.81}
\expandafter\def\csname v@r/SB_ft_null/ami_dev_long/ins\endcsname{57.21}
\expandafter\def\csname v@r/SB_ft_null/ami_dev_long/leak_wpm\endcsname{71.73}
\expandafter\def\csname v@r/SB_ft_null/ami_dev_long/miss\endcsname{10.74}
\expandafter\def\csname v@r/SB_ft_null/ami_dev_long/wer\endcsname{67.95}
\expandafter\def\csname v@r/SB_ft_null/call_dev_clean/dele\endcsname{1.59}
\expandafter\def\csname v@r/SB_ft_null/call_dev_clean/ins\endcsname{0.18}
\expandafter\def\csname v@r/SB_ft_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ft_null/call_dev_clean/miss\endcsname{2.37}
\expandafter\def\csname v@r/SB_ft_null/call_dev_clean/wer\endcsname{2.55}
\expandafter\def\csname v@r/SB_ft_null/call_dev_mix/dele\endcsname{2.65}
\expandafter\def\csname v@r/SB_ft_null/call_dev_mix/ins\endcsname{52.37}
\expandafter\def\csname v@r/SB_ft_null/call_dev_mix/leak_wpm\endcsname{137.83}
\expandafter\def\csname v@r/SB_ft_null/call_dev_mix/miss\endcsname{12.62}
\expandafter\def\csname v@r/SB_ft_null/call_dev_mix/wer\endcsname{64.99}
\expandafter\def\csname v@r/SB_ft_null/dev4\endcsname{23.04}
\expandafter\def\csname v@r/SB_ft_null/krisp/dele\endcsname{1.76}
\expandafter\def\csname v@r/SB_ft_null/krisp/ins\endcsname{9.46}
\expandafter\def\csname v@r/SB_ft_null/krisp/leak_wpm\endcsname{32.75}
\expandafter\def\csname v@r/SB_ft_null/krisp/miss\endcsname{5.43}
\expandafter\def\csname v@r/SB_ft_null/krisp/wer\endcsname{14.89}
\expandafter\def\csname v@r/SB_ft_null/meet3\endcsname{29.87}
\expandafter\def\csname v@r/SB_ft_null/nsf_dev/dele\endcsname{1.48}
\expandafter\def\csname v@r/SB_ft_null/nsf_dev/ins\endcsname{1.81}
\expandafter\def\csname v@r/SB_ft_null/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/SB_ft_null/nsf_dev/miss\endcsname{5.83}
\expandafter\def\csname v@r/SB_ft_null/nsf_dev/wer\endcsname{7.64}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev/dele\endcsname{3.45}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev/ins\endcsname{4.29}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev/leak_wpm\endcsname{9.24}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev/miss\endcsname{9.38}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev/wer\endcsname{13.66}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev_long/dele\endcsname{4.48}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev_long/ins\endcsname{30.70}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev_long/leak_wpm\endcsname{41.16}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev_long/miss\endcsname{13.59}
\expandafter\def\csname v@r/SB_ft_selfl/ami_dev_long/wer\endcsname{44.29}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_clean/dele\endcsname{2.70}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_clean/ins\endcsname{0.18}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_clean/miss\endcsname{3.67}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_clean/wer\endcsname{3.85}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_mix/dele\endcsname{3.27}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_mix/ins\endcsname{48.29}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_mix/leak_wpm\endcsname{133.31}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_mix/miss\endcsname{14.37}
\expandafter\def\csname v@r/SB_ft_selfl/call_dev_mix/wer\endcsname{62.66}
\expandafter\def\csname v@r/SB_ft_selfl/dev4\endcsname{17.42}
\expandafter\def\csname v@r/SB_ft_selfl/krisp/dele\endcsname{1.09}
\expandafter\def\csname v@r/SB_ft_selfl/krisp/ins\endcsname{3.48}
\expandafter\def\csname v@r/SB_ft_selfl/krisp/leak_wpm\endcsname{10.45}
\expandafter\def\csname v@r/SB_ft_selfl/krisp/miss\endcsname{4.77}
\expandafter\def\csname v@r/SB_ft_selfl/krisp/wer\endcsname{8.25}
\expandafter\def\csname v@r/SB_ft_selfl/meet3\endcsname{21.94}
\expandafter\def\csname v@r/SB_ft_selfl/nsf_dev/dele\endcsname{1.58}
\expandafter\def\csname v@r/SB_ft_selfl/nsf_dev/ins\endcsname{1.91}
\expandafter\def\csname v@r/SB_ft_selfl/nsf_dev/leak_wpm\endcsname{0.85}
\expandafter\def\csname v@r/SB_ft_selfl/nsf_dev/miss\endcsname{5.95}
\expandafter\def\csname v@r/SB_ft_selfl/nsf_dev/wer\endcsname{7.86}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev/dele\endcsname{3.18}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev/ins\endcsname{4.23}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev/leak_wpm\endcsname{7.72}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev/miss\endcsname{9.02}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev/wer\endcsname{13.25}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev_long/dele\endcsname{7.09}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev_long/ins\endcsname{3.70}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev_long/leak_wpm\endcsname{7.33}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev_long/miss\endcsname{14.70}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/ami_dev_long/wer\endcsname{18.40}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_clean/dele\endcsname{7.10}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_clean/miss\endcsname{8.52}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_clean/wer\endcsname{8.82}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_mix/dele\endcsname{6.14}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_mix/ins\endcsname{29.37}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_mix/leak_wpm\endcsname{92.85}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_mix/miss\endcsname{19.13}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/call_dev_mix/wer\endcsname{48.50}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/dev4\endcsname{12.08}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/krisp/dele\endcsname{3.26}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/krisp/leak_wpm\endcsname{0.07}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/krisp/miss\endcsname{7.38}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/krisp/wer\endcsname{8.11}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/meet3\endcsname{13.17}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/nsf_dev/dele\endcsname{1.70}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/nsf_dev/ins\endcsname{1.92}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/nsf_dev/miss\endcsname{5.93}
\expandafter\def\csname v@r/SB_ftlong_em_selfl/nsf_dev/wer\endcsname{7.85}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev/dele\endcsname{3.07}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev/ins\endcsname{4.27}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev/leak_wpm\endcsname{7.81}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev/miss\endcsname{9.02}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev/wer\endcsname{13.29}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev_long/dele\endcsname{6.95}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev_long/ins\endcsname{12.52}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev_long/leak_wpm\endcsname{17.17}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev_long/miss\endcsname{14.33}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/ami_dev_long/wer\endcsname{26.86}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/call_dev_clean/dele\endcsname{2.64}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/call_dev_clean/ins\endcsname{0.22}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/call_dev_clean/miss\endcsname{3.25}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/call_dev_clean/wer\endcsname{3.47}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/dev4\endcsname{12.80}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/krisp/dele\endcsname{1.19}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/krisp/ins\endcsname{1.81}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/krisp/leak_wpm\endcsname{4.08}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/krisp/miss\endcsname{4.77}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/krisp/wer\endcsname{6.57}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/meet3\endcsname{15.91}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/nsf_dev/dele\endcsname{1.49}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/nsf_dev/ins\endcsname{1.85}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/nsf_dev/miss\endcsname{5.75}
\expandafter\def\csname v@r/SB_ftlong_k2000_null/nsf_dev/wer\endcsname{7.59}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev/dele\endcsname{2.73}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev/ins\endcsname{4.18}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev/leak_wpm\endcsname{8.17}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev/miss\endcsname{8.73}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev/wer\endcsname{12.90}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev_long/dele\endcsname{8.63}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev_long/ins\endcsname{5.43}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev_long/leak_wpm\endcsname{8.47}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev_long/miss\endcsname{15.87}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/ami_dev_long/wer\endcsname{21.31}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/call_dev_clean/dele\endcsname{4.86}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/call_dev_clean/miss\endcsname{5.91}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/call_dev_clean/wer\endcsname{6.21}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/dev4\endcsname{12.01}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/krisp/dele\endcsname{1.16}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/krisp/ins\endcsname{0.82}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/krisp/leak_wpm\endcsname{0.53}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/krisp/miss\endcsname{4.71}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/krisp/wer\endcsname{5.52}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/meet3\endcsname{13.95}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/nsf_dev/ins\endcsname{1.92}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/nsf_dev/miss\endcsname{5.71}
\expandafter\def\csname v@r/SB_ftlong_k2000_selfl/nsf_dev/wer\endcsname{7.63}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev/dele\endcsname{3.12}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev/ins\endcsname{3.88}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev/leak_wpm\endcsname{7.68}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev/miss\endcsname{9.20}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev/wer\endcsname{13.08}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev_long/dele\endcsname{7.79}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev_long/ins\endcsname{9.60}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev_long/leak_wpm\endcsname{13.92}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev_long/miss\endcsname{15.40}
\expandafter\def\csname v@r/SB_ftlong_null/ami_dev_long/wer\endcsname{25.00}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_clean/dele\endcsname{3.97}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_clean/ins\endcsname{0.19}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_clean/miss\endcsname{4.77}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_clean/wer\endcsname{4.96}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_mix/dele\endcsname{3.90}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_mix/ins\endcsname{36.15}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_mix/leak_wpm\endcsname{95.10}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_mix/miss\endcsname{15.06}
\expandafter\def\csname v@r/SB_ftlong_null/call_dev_mix/wer\endcsname{51.20}
\expandafter\def\csname v@r/SB_ftlong_null/dev4\endcsname{12.69}
\expandafter\def\csname v@r/SB_ftlong_null/krisp/dele\endcsname{1.75}
\expandafter\def\csname v@r/SB_ftlong_null/krisp/ins\endcsname{1.48}
\expandafter\def\csname v@r/SB_ftlong_null/krisp/leak_wpm\endcsname{2.93}
\expandafter\def\csname v@r/SB_ftlong_null/krisp/miss\endcsname{5.53}
\expandafter\def\csname v@r/SB_ftlong_null/krisp/wer\endcsname{7.01}
\expandafter\def\csname v@r/SB_ftlong_null/meet3\endcsname{15.26}
\expandafter\def\csname v@r/SB_ftlong_null/nsf_dev/dele\endcsname{1.64}
\expandafter\def\csname v@r/SB_ftlong_null/nsf_dev/ins\endcsname{1.83}
\expandafter\def\csname v@r/SB_ftlong_null/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/SB_ftlong_null/nsf_dev/miss\endcsname{5.89}
\expandafter\def\csname v@r/SB_ftlong_null/nsf_dev/wer\endcsname{7.71}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev/dele\endcsname{3.27}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev/ins\endcsname{3.72}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev/leak_wpm\endcsname{7.28}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev/miss\endcsname{9.31}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev/wer\endcsname{13.03}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev_long/dele\endcsname{7.90}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev_long/ins\endcsname{4.68}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev_long/leak_wpm\endcsname{7.63}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev_long/miss\endcsname{14.97}
\expandafter\def\csname v@r/SB_ftlong_selfl/ami_dev_long/wer\endcsname{19.65}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_clean/dele\endcsname{5.90}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_clean/ins\endcsname{0.22}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_clean/miss\endcsname{7.31}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_clean/wer\endcsname{7.53}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_mix/dele\endcsname{5.07}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_mix/ins\endcsname{35.81}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_mix/leak_wpm\endcsname{109.69}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_mix/miss\endcsname{16.90}
\expandafter\def\csname v@r/SB_ftlong_selfl/call_dev_mix/wer\endcsname{52.71}
\expandafter\def\csname v@r/SB_ftlong_selfl/dev4\endcsname{11.98}
\expandafter\def\csname v@r/SB_ftlong_selfl/krisp/dele\endcsname{1.55}
\expandafter\def\csname v@r/SB_ftlong_selfl/krisp/ins\endcsname{0.77}
\expandafter\def\csname v@r/SB_ftlong_selfl/krisp/leak_wpm\endcsname{0.37}
\expandafter\def\csname v@r/SB_ftlong_selfl/krisp/miss\endcsname{5.29}
\expandafter\def\csname v@r/SB_ftlong_selfl/krisp/wer\endcsname{6.06}
\expandafter\def\csname v@r/SB_ftlong_selfl/meet3\endcsname{13.47}
\expandafter\def\csname v@r/SB_ftlong_selfl/nsf_dev/dele\endcsname{1.64}
\expandafter\def\csname v@r/SB_ftlong_selfl/nsf_dev/ins\endcsname{1.90}
\expandafter\def\csname v@r/SB_ftlong_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/SB_ftlong_selfl/nsf_dev/miss\endcsname{5.83}
\expandafter\def\csname v@r/SB_ftlong_selfl/nsf_dev/wer\endcsname{7.72}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev/dele\endcsname{3.36}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev/ins\endcsname{3.84}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev/leak_wpm\endcsname{7.50}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev/miss\endcsname{9.18}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev/wer\endcsname{13.03}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev_long/dele\endcsname{8.12}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev_long/ins\endcsname{4.12}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev_long/leak_wpm\endcsname{7.60}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev_long/miss\endcsname{15.78}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/ami_dev_long/wer\endcsname{19.91}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_clean/dele\endcsname{5.19}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_clean/ins\endcsname{0.29}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_clean/miss\endcsname{6.46}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_clean/wer\endcsname{6.75}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_mix/dele\endcsname{5.10}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_mix/ins\endcsname{32.18}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_mix/leak_wpm\endcsname{108.87}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_mix/miss\endcsname{19.06}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/call_dev_mix/wer\endcsname{51.24}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/dev4\endcsname{11.83}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/krisp/dele\endcsname{2.08}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/krisp/leak_wpm\endcsname{0.33}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/krisp/miss\endcsname{5.94}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/krisp/wer\endcsname{6.68}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/meet3\endcsname{13.52}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/nsf_dev/ins\endcsname{1.87}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/nsf_dev/miss\endcsname{5.75}
\expandafter\def\csname v@r/SB_ftlong_solo_selfl/nsf_dev/wer\endcsname{7.62}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev/dele\endcsname{3.00}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev/ins\endcsname{4.00}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev/leak_wpm\endcsname{7.54}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev/miss\endcsname{8.93}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev/wer\endcsname{12.93}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev_long/dele\endcsname{7.83}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev_long/ins\endcsname{4.15}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev_long/leak_wpm\endcsname{6.99}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev_long/miss\endcsname{15.22}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/ami_dev_long/wer\endcsname{19.37}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_clean/dele\endcsname{8.59}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_clean/ins\endcsname{0.27}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_clean/miss\endcsname{9.71}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_clean/wer\endcsname{9.99}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_mix/dele\endcsname{6.33}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_mix/ins\endcsname{29.36}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_mix/leak_wpm\endcsname{97.78}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_mix/miss\endcsname{20.03}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/call_dev_mix/wer\endcsname{49.38}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/dev4\endcsname{12.52}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/krisp/dele\endcsname{3.37}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/krisp/ins\endcsname{0.72}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/krisp/leak_wpm\endcsname{0.13}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/krisp/miss\endcsname{7.45}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/krisp/wer\endcsname{8.18}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/meet3\endcsname{13.37}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/nsf_dev/dele\endcsname{1.61}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/nsf_dev/miss\endcsname{5.87}
\expandafter\def\csname v@r/SB_ftlong_sslb_selfl/nsf_dev/wer\endcsname{7.80}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev/dele\endcsname{3.19}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev/ins\endcsname{4.59}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev/leak_wpm\endcsname{9.15}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev/miss\endcsname{9.02}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev/wer\endcsname{13.61}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev_long/dele\endcsname{7.55}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev_long/ins\endcsname{11.17}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev_long/leak_wpm\endcsname{15.39}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev_long/miss\endcsname{15.16}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/ami_dev_long/wer\endcsname{26.33}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_clean/dele\endcsname{3.24}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_clean/ins\endcsname{0.18}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_clean/miss\endcsname{3.86}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_clean/wer\endcsname{4.04}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_mix/dele\endcsname{3.70}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_mix/ins\endcsname{37.36}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_mix/leak_wpm\endcsname{89.76}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_mix/miss\endcsname{13.43}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/call_dev_mix/wer\endcsname{50.79}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/dev4\endcsname{12.95}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/krisp/dele\endcsname{1.27}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/krisp/ins\endcsname{1.48}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/krisp/leak_wpm\endcsname{2.75}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/krisp/miss\endcsname{4.81}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/krisp/wer\endcsname{6.29}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/meet3\endcsname{15.92}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/nsf_dev/dele\endcsname{1.59}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/nsf_dev/ins\endcsname{2.04}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/nsf_dev/leak_wpm\endcsname{0.89}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/nsf_dev/miss\endcsname{5.79}
\expandafter\def\csname v@r/SB_ftlong_sslp_null/nsf_dev/wer\endcsname{7.83}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev/dele\endcsname{3.20}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev/ins\endcsname{4.43}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev/leak_wpm\endcsname{9.87}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev/miss\endcsname{9.21}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev/wer\endcsname{13.64}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev_long/dele\endcsname{8.48}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev_long/ins\endcsname{5.63}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev_long/leak_wpm\endcsname{8.73}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev_long/miss\endcsname{15.72}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/ami_dev_long/wer\endcsname{21.34}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_clean/dele\endcsname{4.39}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_clean/ins\endcsname{0.31}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_clean/miss\endcsname{5.54}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_clean/wer\endcsname{5.85}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_mix/dele\endcsname{4.27}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_mix/ins\endcsname{34.26}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_mix/leak_wpm\endcsname{107.63}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_mix/miss\endcsname{15.99}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/call_dev_mix/wer\endcsname{50.24}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/dev4\endcsname{12.19}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/krisp/dele\endcsname{1.35}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/krisp/ins\endcsname{0.78}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/krisp/leak_wpm\endcsname{0.22}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/krisp/miss\endcsname{4.78}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/krisp/wer\endcsname{5.56}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/meet3\endcsname{14.31}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/nsf_dev/dele\endcsname{1.71}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/nsf_dev/ins\endcsname{2.05}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/nsf_dev/leak_wpm\endcsname{1.19}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/nsf_dev/miss\endcsname{5.90}
\expandafter\def\csname v@r/SB_ftlong_sslp_selfl/nsf_dev/wer\endcsname{7.94}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev/dele\endcsname{3.59}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev/ins\endcsname{3.48}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev/leak_wpm\endcsname{7.01}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev/miss\endcsname{9.70}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev/wer\endcsname{13.18}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev_long/dele\endcsname{6.81}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev_long/ins\endcsname{4.71}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev_long/leak_wpm\endcsname{7.55}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev_long/miss\endcsname{14.13}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/ami_dev_long/wer\endcsname{18.84}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_clean/dele\endcsname{7.00}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_clean/miss\endcsname{8.47}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_clean/wer\endcsname{8.77}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_mix/dele\endcsname{5.44}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_mix/ins\endcsname{32.92}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_mix/leak_wpm\endcsname{111.74}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_mix/miss\endcsname{19.38}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/call_dev_mix/wer\endcsname{52.30}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/dev4\endcsname{12.11}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/krisp/dele\endcsname{1.92}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/krisp/ins\endcsname{0.81}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/krisp/leak_wpm\endcsname{0.36}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/krisp/miss\endcsname{5.82}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/krisp/wer\endcsname{6.63}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/meet3\endcsname{13.23}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/nsf_dev/dele\endcsname{1.62}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/nsf_dev/ins\endcsname{1.83}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/nsf_dev/leak_wpm\endcsname{0.38}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/nsf_dev/miss\endcsname{5.84}
\expandafter\def\csname v@r/SB_ftlong_wob_selfl/nsf_dev/wer\endcsname{7.66}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/aic_calls/dele\endcsname{2.78}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/aic_calls/ins\endcsname{8.09}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/aic_calls/leak_wpm\endcsname{7.89}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/aic_calls/miss\endcsname{6.34}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/aic_calls/wer\endcsname{14.43}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev/dele\endcsname{2.79}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev/ins\endcsname{4.13}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev/leak_wpm\endcsname{8.21}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev/miss\endcsname{8.77}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev/wer\endcsname{12.90}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev_long/dele\endcsname{6.76}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev_long/ins\endcsname{3.36}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev_long/leak_wpm\endcsname{6.20}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev_long/miss\endcsname{14.04}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/ami_dev_long/wer\endcsname{17.40}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_clean/dele\endcsname{3.91}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_clean/ins\endcsname{0.43}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_clean/miss\endcsname{4.83}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_clean/wer\endcsname{5.26}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_mix/dele\endcsname{4.31}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_mix/ins\endcsname{33.44}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_mix/leak_wpm\endcsname{108.66}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_mix/miss\endcsname{18.19}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/call_dev_mix/wer\endcsname{51.63}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/dev4\endcsname{10.81}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/krisp/dele\endcsname{1.25}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/krisp/leak_wpm\endcsname{0.16}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/krisp/miss\endcsname{4.67}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/krisp/wer\endcsname{5.37}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/meet3\endcsname{12.67}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/nsf_dev/ins\endcsname{1.88}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/nsf_dev/miss\endcsname{5.82}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2_selfl/nsf_dev/wer\endcsname{7.70}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev/dele\endcsname{3.01}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev/ins\endcsname{4.19}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev/leak_wpm\endcsname{9.02}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev/miss\endcsname{9.00}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev/wer\endcsname{13.19}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev_long/dele\endcsname{7.27}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev_long/ins\endcsname{3.95}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev_long/leak_wpm\endcsname{6.76}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev_long/miss\endcsname{14.57}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/ami_dev_long/wer\endcsname{18.52}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_clean/dele\endcsname{3.02}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_clean/ins\endcsname{0.45}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_clean/miss\endcsname{3.76}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_clean/wer\endcsname{4.22}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_mix/dele\endcsname{3.80}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_mix/ins\endcsname{34.35}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_mix/leak_wpm\endcsname{107.22}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_mix/miss\endcsname{16.53}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/call_dev_mix/wer\endcsname{50.88}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/dev4\endcsname{10.90}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/krisp/dele\endcsname{1.63}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/krisp/ins\endcsname{0.69}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/krisp/miss\endcsname{5.09}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/krisp/wer\endcsname{5.79}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/meet3\endcsname{13.13}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/nsf_dev/dele\endcsname{1.54}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/nsf_dev/miss\endcsname{5.73}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2c_selfl/nsf_dev/wer\endcsname{7.68}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev/dele\endcsname{2.82}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev/ins\endcsname{4.30}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev/leak_wpm\endcsname{8.93}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev/miss\endcsname{8.86}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev/wer\endcsname{13.16}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev_long/dele\endcsname{6.45}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev_long/ins\endcsname{4.15}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev_long/leak_wpm\endcsname{6.94}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev_long/miss\endcsname{13.59}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/ami_dev_long/wer\endcsname{17.74}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_clean/dele\endcsname{3.27}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_clean/ins\endcsname{0.33}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_clean/miss\endcsname{4.59}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_clean/wer\endcsname{4.92}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_mix/dele\endcsname{4.33}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_mix/ins\endcsname{34.11}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_mix/leak_wpm\endcsname{108.87}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_mix/miss\endcsname{17.91}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/call_dev_mix/wer\endcsname{52.03}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/dev4\endcsname{10.89}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/krisp/dele\endcsname{1.34}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/krisp/leak_wpm\endcsname{0.16}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/krisp/miss\endcsname{4.80}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/krisp/wer\endcsname{5.50}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/meet3\endcsname{12.87}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/nsf_dev/dele\endcsname{1.48}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/nsf_dev/miss\endcsname{5.77}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2g_selfl/nsf_dev/wer\endcsname{7.71}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev/dele\endcsname{3.02}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev/ins\endcsname{4.06}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev/leak_wpm\endcsname{8.66}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev/miss\endcsname{8.86}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev/wer\endcsname{12.93}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev_long/dele\endcsname{7.13}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev_long/ins\endcsname{3.83}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev_long/leak_wpm\endcsname{7.02}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev_long/miss\endcsname{14.71}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/ami_dev_long/wer\endcsname{18.54}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_clean/dele\endcsname{2.96}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_clean/ins\endcsname{0.33}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_clean/miss\endcsname{3.85}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_clean/wer\endcsname{4.18}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_mix/dele\endcsname{3.19}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_mix/ins\endcsname{34.83}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_mix/leak_wpm\endcsname{110.72}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_mix/miss\endcsname{15.46}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/call_dev_mix/wer\endcsname{50.29}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/dev4\endcsname{10.83}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/krisp/dele\endcsname{1.05}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/krisp/ins\endcsname{0.71}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/krisp/leak_wpm\endcsname{0.02}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/krisp/miss\endcsname{4.53}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/krisp/wer\endcsname{5.24}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/meet3\endcsname{13.05}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/nsf_dev/dele\endcsname{1.58}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/nsf_dev/miss\endcsname{5.72}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gc_selfl/nsf_dev/wer\endcsname{7.66}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/dele\endcsname{2.79}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/ins\endcsname{4.48}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/leak_wpm\endcsname{9.06}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/miss\endcsname{8.59}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev/wer\endcsname{13.07}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/dele\endcsname{5.79}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/ins\endcsname{4.72}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/leak_wpm\endcsname{7.81}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/miss\endcsname{13.50}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/ami_dev_long/wer\endcsname{18.23}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/dele\endcsname{2.38}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/ins\endcsname{0.27}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/miss\endcsname{3.36}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_clean/wer\endcsname{3.63}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/dele\endcsname{2.84}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/ins\endcsname{37.28}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/leak_wpm\endcsname{118.93}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/miss\endcsname{15.47}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/call_dev_mix/wer\endcsname{52.75}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/dev4\endcsname{10.67}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/krisp/dele\endcsname{1.11}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/krisp/leak_wpm\endcsname{0.19}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/krisp/miss\endcsname{4.62}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/krisp/wer\endcsname{5.35}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/meet3\endcsname{13.01}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/dele\endcsname{1.45}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/ins\endcsname{1.95}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/miss\endcsname{5.79}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2gm_selfl/nsf_dev/wer\endcsname{7.75}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev/dele\endcsname{2.80}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev/ins\endcsname{4.09}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev/leak_wpm\endcsname{8.04}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev/miss\endcsname{8.53}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev/wer\endcsname{12.62}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev_long/dele\endcsname{7.17}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev_long/ins\endcsname{4.15}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev_long/leak_wpm\endcsname{7.12}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev_long/miss\endcsname{14.65}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/ami_dev_long/wer\endcsname{18.80}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_clean/dele\endcsname{2.59}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_clean/ins\endcsname{0.36}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_clean/miss\endcsname{3.48}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_clean/wer\endcsname{3.84}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_mix/dele\endcsname{3.74}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_mix/ins\endcsname{36.60}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_mix/leak_wpm\endcsname{118.93}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_mix/miss\endcsname{17.60}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/call_dev_mix/wer\endcsname{54.20}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/dev4\endcsname{10.74}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/krisp/dele\endcsname{1.00}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/krisp/ins\endcsname{0.69}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/krisp/leak_wpm\endcsname{0.12}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/krisp/miss\endcsname{4.46}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/krisp/wer\endcsname{5.15}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/meet3\endcsname{13.04}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/nsf_dev/ins\endcsname{1.88}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/nsf_dev/miss\endcsname{5.80}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2h_selfl/nsf_dev/wer\endcsname{7.69}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev/dele\endcsname{3.16}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev/ins\endcsname{3.97}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev/leak_wpm\endcsname{8.04}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev/miss\endcsname{9.03}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev/wer\endcsname{13.00}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev_long/dele\endcsname{7.29}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev_long/ins\endcsname{4.05}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev_long/leak_wpm\endcsname{7.29}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev_long/miss\endcsname{14.67}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/ami_dev_long/wer\endcsname{18.72}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_clean/dele\endcsname{2.10}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_clean/miss\endcsname{2.95}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_clean/wer\endcsname{3.21}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_mix/dele\endcsname{3.29}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_mix/ins\endcsname{36.96}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_mix/leak_wpm\endcsname{116.26}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_mix/miss\endcsname{15.77}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/call_dev_mix/wer\endcsname{52.73}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/dev4\endcsname{10.67}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/krisp/dele\endcsname{1.33}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/krisp/ins\endcsname{0.68}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/krisp/miss\endcsname{4.82}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/krisp/wer\endcsname{5.50}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/meet3\endcsname{13.16}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/nsf_dev/miss\endcsname{5.82}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2m_selfl/nsf_dev/wer\endcsname{7.76}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/dele\endcsname{2.91}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/ins\endcsname{4.22}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/leak_wpm\endcsname{8.75}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/miss\endcsname{8.92}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev/wer\endcsname{13.14}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/dele\endcsname{8.50}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/ins\endcsname{3.39}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/leak_wpm\endcsname{5.92}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/miss\endcsname{15.65}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/ami_dev_long/wer\endcsname{19.04}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/dele\endcsname{2.15}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/ins\endcsname{0.29}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/miss\endcsname{3.35}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/call_dev_clean/wer\endcsname{3.63}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/dev4\endcsname{10.87}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/krisp/dele\endcsname{1.32}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/krisp/ins\endcsname{0.69}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/krisp/miss\endcsname{4.89}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/krisp/wer\endcsname{5.58}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/meet3\endcsname{13.29}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/miss\endcsname{5.75}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2mr_selfl/nsf_dev/wer\endcsname{7.69}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev/dele\endcsname{2.69}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev/ins\endcsname{4.24}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev/leak_wpm\endcsname{8.08}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev/miss\endcsname{8.46}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev/wer\endcsname{12.71}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev_long/dele\endcsname{7.51}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev_long/ins\endcsname{3.98}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev_long/leak_wpm\endcsname{6.92}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev_long/miss\endcsname{14.93}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/ami_dev_long/wer\endcsname{18.91}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/call_dev_clean/dele\endcsname{3.21}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/call_dev_clean/miss\endcsname{4.21}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/call_dev_clean/wer\endcsname{4.50}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/dev4\endcsname{10.96}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/krisp/dele\endcsname{1.27}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/krisp/miss\endcsname{4.72}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/krisp/wer\endcsname{5.42}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/meet3\endcsname{13.11}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/nsf_dev/dele\endcsname{1.45}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/nsf_dev/miss\endcsname{5.79}
\expandafter\def\csname v@r/SB_ftlong_ws_cwlt2r_selfl/nsf_dev/wer\endcsname{7.72}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/aic_calls/dele\endcsname{3.28}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/aic_calls/ins\endcsname{8.48}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/aic_calls/leak_wpm\endcsname{7.82}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/aic_calls/miss\endcsname{6.81}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/aic_calls/wer\endcsname{15.29}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev/dele\endcsname{3.11}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev/ins\endcsname{3.81}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev/leak_wpm\endcsname{8.79}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev/miss\endcsname{9.61}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev/wer\endcsname{13.43}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev_long/dele\endcsname{7.87}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev_long/ins\endcsname{4.75}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev_long/leak_wpm\endcsname{8.00}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev_long/miss\endcsname{15.20}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/ami_dev_long/wer\endcsname{19.94}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/call_dev_clean/dele\endcsname{4.03}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/call_dev_clean/ins\endcsname{0.17}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/call_dev_clean/miss\endcsname{5.10}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/call_dev_clean/wer\endcsname{5.27}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/dev4\endcsname{11.56}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/krisp/dele\endcsname{1.44}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/krisp/ins\endcsname{0.77}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/krisp/leak_wpm\endcsname{0.19}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/krisp/miss\endcsname{5.30}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/krisp/wer\endcsname{6.08}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/meet3\endcsname{13.66}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/nsf_dev/ins\endcsname{1.85}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/nsf_dev/miss\endcsname{5.76}
\expandafter\def\csname v@r/SB_ftlong_ws_loud/nsf_dev/wer\endcsname{7.61}
\expandafter\def\csname v@r/SB_ftlong_ws_null/aic_calls/dele\endcsname{2.85}
\expandafter\def\csname v@r/SB_ftlong_ws_null/aic_calls/ins\endcsname{9.30}
\expandafter\def\csname v@r/SB_ftlong_ws_null/aic_calls/leak_wpm\endcsname{10.35}
\expandafter\def\csname v@r/SB_ftlong_ws_null/aic_calls/miss\endcsname{6.70}
\expandafter\def\csname v@r/SB_ftlong_ws_null/aic_calls/wer\endcsname{16.00}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev/dele\endcsname{3.23}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev/ins\endcsname{4.30}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev/leak_wpm\endcsname{8.79}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev/miss\endcsname{9.35}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev/wer\endcsname{13.65}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev_long/dele\endcsname{6.34}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev_long/ins\endcsname{12.61}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev_long/leak_wpm\endcsname{17.41}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev_long/miss\endcsname{13.97}
\expandafter\def\csname v@r/SB_ftlong_ws_null/ami_dev_long/wer\endcsname{26.59}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_clean/dele\endcsname{2.78}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_clean/ins\endcsname{0.20}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_clean/miss\endcsname{3.45}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_clean/wer\endcsname{3.66}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_mix/dele\endcsname{3.97}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_mix/ins\endcsname{39.72}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_mix/leak_wpm\endcsname{108.46}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_mix/miss\endcsname{14.54}
\expandafter\def\csname v@r/SB_ftlong_ws_null/call_dev_mix/wer\endcsname{54.26}
\expandafter\def\csname v@r/SB_ftlong_ws_null/dev4\endcsname{12.88}
\expandafter\def\csname v@r/SB_ftlong_ws_null/krisp/dele\endcsname{1.62}
\expandafter\def\csname v@r/SB_ftlong_ws_null/krisp/ins\endcsname{1.48}
\expandafter\def\csname v@r/SB_ftlong_ws_null/krisp/leak_wpm\endcsname{2.92}
\expandafter\def\csname v@r/SB_ftlong_ws_null/krisp/miss\endcsname{5.39}
\expandafter\def\csname v@r/SB_ftlong_ws_null/krisp/wer\endcsname{6.87}
\expandafter\def\csname v@r/SB_ftlong_ws_null/meet3\endcsname{15.96}
\expandafter\def\csname v@r/SB_ftlong_ws_null/nsf_dev/dele\endcsname{1.62}
\expandafter\def\csname v@r/SB_ftlong_ws_null/nsf_dev/ins\endcsname{1.86}
\expandafter\def\csname v@r/SB_ftlong_ws_null/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/SB_ftlong_ws_null/nsf_dev/miss\endcsname{5.77}
\expandafter\def\csname v@r/SB_ftlong_ws_null/nsf_dev/wer\endcsname{7.63}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev/dele\endcsname{2.84}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev/ins\endcsname{4.16}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev/leak_wpm\endcsname{8.17}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev/miss\endcsname{9.00}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev/wer\endcsname{13.16}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev_long/dele\endcsname{8.01}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev_long/ins\endcsname{3.74}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev_long/leak_wpm\endcsname{6.34}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev_long/miss\endcsname{14.90}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/ami_dev_long/wer\endcsname{18.65}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/meet3\endcsname{13.13}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/nsf_dev/dele\endcsname{1.53}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/nsf_dev/ins\endcsname{1.78}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/nsf_dev/miss\endcsname{5.81}
\expandafter\def\csname v@r/SB_ftlong_ws_oracle/nsf_dev/wer\endcsname{7.59}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev/dele\endcsname{3.20}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev/ins\endcsname{4.16}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev/leak_wpm\endcsname{8.71}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev/miss\endcsname{9.29}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev/wer\endcsname{13.46}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev_long/dele\endcsname{8.02}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev_long/ins\endcsname{6.11}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev_long/leak_wpm\endcsname{9.60}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev_long/miss\endcsname{15.41}
\expandafter\def\csname v@r/SB_ftlong_ws_self/ami_dev_long/wer\endcsname{21.52}
\expandafter\def\csname v@r/SB_ftlong_ws_self/call_dev_clean/dele\endcsname{4.21}
\expandafter\def\csname v@r/SB_ftlong_ws_self/call_dev_clean/ins\endcsname{0.27}
\expandafter\def\csname v@r/SB_ftlong_ws_self/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_self/call_dev_clean/miss\endcsname{5.05}
\expandafter\def\csname v@r/SB_ftlong_ws_self/call_dev_clean/wer\endcsname{5.33}
\expandafter\def\csname v@r/SB_ftlong_ws_self/dev4\endcsname{11.97}
\expandafter\def\csname v@r/SB_ftlong_ws_self/krisp/dele\endcsname{1.81}
\expandafter\def\csname v@r/SB_ftlong_ws_self/krisp/ins\endcsname{0.72}
\expandafter\def\csname v@r/SB_ftlong_ws_self/krisp/leak_wpm\endcsname{0.13}
\expandafter\def\csname v@r/SB_ftlong_ws_self/krisp/miss\endcsname{5.51}
\expandafter\def\csname v@r/SB_ftlong_ws_self/krisp/wer\endcsname{6.23}
\expandafter\def\csname v@r/SB_ftlong_ws_self/meet3\endcsname{14.18}
\expandafter\def\csname v@r/SB_ftlong_ws_self/nsf_dev/dele\endcsname{1.59}
\expandafter\def\csname v@r/SB_ftlong_ws_self/nsf_dev/ins\endcsname{1.85}
\expandafter\def\csname v@r/SB_ftlong_ws_self/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/SB_ftlong_ws_self/nsf_dev/miss\endcsname{5.72}
\expandafter\def\csname v@r/SB_ftlong_ws_self/nsf_dev/wer\endcsname{7.57}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/aic_calls/dele\endcsname{3.21}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/aic_calls/ins\endcsname{11.44}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/aic_calls/leak_wpm\endcsname{14.01}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/aic_calls/miss\endcsname{7.02}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/aic_calls/wer\endcsname{18.46}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev/dele\endcsname{3.11}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev/ins\endcsname{4.05}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev/leak_wpm\endcsname{8.21}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev/miss\endcsname{9.18}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev/wer\endcsname{13.23}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev_long/dele\endcsname{8.29}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev_long/ins\endcsname{4.17}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev_long/leak_wpm\endcsname{7.52}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev_long/miss\endcsname{15.85}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/ami_dev_long/wer\endcsname{20.02}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_clean/dele\endcsname{4.56}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_clean/ins\endcsname{0.20}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_clean/miss\endcsname{5.58}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_clean/wer\endcsname{5.78}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_mix/dele\endcsname{4.71}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_mix/ins\endcsname{34.64}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_mix/leak_wpm\endcsname{114.21}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_mix/miss\endcsname{16.78}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/call_dev_mix/wer\endcsname{51.42}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/dev4\endcsname{11.67}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/krisp/dele\endcsname{1.54}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/krisp/leak_wpm\endcsname{0.12}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/krisp/miss\endcsname{5.40}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/krisp/wer\endcsname{6.12}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/meet3\endcsname{13.63}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/nsf_dev/dele\endcsname{1.61}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/nsf_dev/ins\endcsname{1.87}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/nsf_dev/miss\endcsname{5.76}
\expandafter\def\csname v@r/SB_ftlong_ws_selfl/nsf_dev/wer\endcsname{7.63}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev/dele\endcsname{3.08}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev/ins\endcsname{4.31}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev/leak_wpm\endcsname{8.66}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev/miss\endcsname{9.29}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev/wer\endcsname{13.61}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev_long/dele\endcsname{7.88}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev_long/ins\endcsname{4.56}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev_long/leak_wpm\endcsname{7.62}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev_long/miss\endcsname{15.41}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/ami_dev_long/wer\endcsname{19.97}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_clean/dele\endcsname{4.49}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_clean/ins\endcsname{0.25}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_clean/miss\endcsname{6.11}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_clean/wer\endcsname{6.36}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_mix/dele\endcsname{4.23}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_mix/ins\endcsname{36.35}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_mix/leak_wpm\endcsname{120.16}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_mix/miss\endcsname{16.79}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/call_dev_mix/wer\endcsname{53.14}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/dev4\endcsname{11.92}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/krisp/dele\endcsname{1.28}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/krisp/ins\endcsname{0.78}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/krisp/leak_wpm\endcsname{0.45}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/krisp/miss\endcsname{4.96}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/krisp/wer\endcsname{5.74}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/meet3\endcsname{13.77}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/nsf_dev/dele\endcsname{1.55}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/nsf_dev/ins\endcsname{1.97}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/nsf_dev/miss\endcsname{5.77}
\expandafter\def\csname v@r/SB_ftlong_ws_sslb_selfl/nsf_dev/wer\endcsname{7.73}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev/dele\endcsname{2.89}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev/ins\endcsname{5.27}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev/leak_wpm\endcsname{9.73}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev/miss\endcsname{8.50}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev/wer\endcsname{13.77}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev_long/dele\endcsname{9.18}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev_long/ins\endcsname{6.20}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev_long/leak_wpm\endcsname{9.94}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev_long/miss\endcsname{16.89}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/ami_dev_long/wer\endcsname{23.09}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_clean/dele\endcsname{3.67}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_clean/miss\endcsname{4.67}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_clean/wer\endcsname{4.97}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_mix/dele\endcsname{3.06}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_mix/ins\endcsname{42.05}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_mix/leak_wpm\endcsname{128.18}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_mix/miss\endcsname{15.74}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/call_dev_mix/wer\endcsname{57.78}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/dev4\endcsname{12.40}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/krisp/dele\endcsname{0.92}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/krisp/ins\endcsname{0.75}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/krisp/leak_wpm\endcsname{0.12}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/krisp/miss\endcsname{4.32}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/krisp/wer\endcsname{5.07}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/meet3\endcsname{14.87}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/nsf_dev/ins\endcsname{1.98}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/nsf_dev/leak_wpm\endcsname{0.77}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/nsf_dev/miss\endcsname{5.78}
\expandafter\def\csname v@r/SB_ftlong_wsp_selfl/nsf_dev/wer\endcsname{7.76}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev/dele\endcsname{4.33}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev/ins\endcsname{4.00}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev/leak_wpm\endcsname{7.95}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev/miss\endcsname{10.45}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev/wer\endcsname{14.44}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev_long/dele\endcsname{8.63}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev_long/ins\endcsname{9.16}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev_long/leak_wpm\endcsname{13.88}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev_long/miss\endcsname{16.42}
\expandafter\def\csname v@r/SB_long_far_null/ami_dev_long/wer\endcsname{25.58}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_clean/dele\endcsname{5.48}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_clean/miss\endcsname{6.20}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_clean/wer\endcsname{6.43}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_mix/dele\endcsname{5.37}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_mix/ins\endcsname{29.26}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_mix/leak_wpm\endcsname{72.30}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_mix/miss\endcsname{17.15}
\expandafter\def\csname v@r/SB_long_far_null/call_dev_mix/wer\endcsname{46.41}
\expandafter\def\csname v@r/SB_long_far_null/dev4\endcsname{13.65}
\expandafter\def\csname v@r/SB_long_far_null/krisp/dele\endcsname{2.10}
\expandafter\def\csname v@r/SB_long_far_null/krisp/ins\endcsname{1.14}
\expandafter\def\csname v@r/SB_long_far_null/krisp/leak_wpm\endcsname{1.86}
\expandafter\def\csname v@r/SB_long_far_null/krisp/miss\endcsname{5.83}
\expandafter\def\csname v@r/SB_long_far_null/krisp/wer\endcsname{6.98}
\expandafter\def\csname v@r/SB_long_far_null/meet3\endcsname{16.05}
\expandafter\def\csname v@r/SB_long_far_null/nsf_dev/dele\endcsname{2.04}
\expandafter\def\csname v@r/SB_long_far_null/nsf_dev/ins\endcsname{1.79}
\expandafter\def\csname v@r/SB_long_far_null/nsf_dev/leak_wpm\endcsname{0.38}
\expandafter\def\csname v@r/SB_long_far_null/nsf_dev/miss\endcsname{6.34}
\expandafter\def\csname v@r/SB_long_far_null/nsf_dev/wer\endcsname{8.13}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev/dele\endcsname{3.45}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev/ins\endcsname{4.66}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev/leak_wpm\endcsname{9.82}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev/miss\endcsname{9.54}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev/wer\endcsname{14.20}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev_long/dele\endcsname{9.89}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev_long/ins\endcsname{10.92}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev_long/leak_wpm\endcsname{16.05}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev_long/miss\endcsname{17.59}
\expandafter\def\csname v@r/SB_long_k03_null/ami_dev_long/wer\endcsname{28.51}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_clean/dele\endcsname{3.25}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_clean/ins\endcsname{0.19}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_clean/miss\endcsname{3.87}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_clean/wer\endcsname{4.06}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_mix/dele\endcsname{3.41}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_mix/ins\endcsname{39.20}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_mix/leak_wpm\endcsname{95.52}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_mix/miss\endcsname{14.97}
\expandafter\def\csname v@r/SB_long_k03_null/call_dev_mix/wer\endcsname{54.18}
\expandafter\def\csname v@r/SB_long_k03_null/dev4\endcsname{13.92}
\expandafter\def\csname v@r/SB_long_k03_null/krisp/dele\endcsname{1.33}
\expandafter\def\csname v@r/SB_long_k03_null/krisp/ins\endcsname{1.92}
\expandafter\def\csname v@r/SB_long_k03_null/krisp/leak_wpm\endcsname{4.51}
\expandafter\def\csname v@r/SB_long_k03_null/krisp/miss\endcsname{4.74}
\expandafter\def\csname v@r/SB_long_k03_null/krisp/wer\endcsname{6.66}
\expandafter\def\csname v@r/SB_long_k03_null/meet3\endcsname{17.21}
\expandafter\def\csname v@r/SB_long_k03_null/nsf_dev/dele\endcsname{1.79}
\expandafter\def\csname v@r/SB_long_k03_null/nsf_dev/ins\endcsname{2.93}
\expandafter\def\csname v@r/SB_long_k03_null/nsf_dev/leak_wpm\endcsname{4.13}
\expandafter\def\csname v@r/SB_long_k03_null/nsf_dev/miss\endcsname{5.99}
\expandafter\def\csname v@r/SB_long_k03_null/nsf_dev/wer\endcsname{8.92}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_clean/dele\endcsname{6.72}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_clean/miss\endcsname{8.05}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_clean/wer\endcsname{8.35}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_mix/dele\endcsname{4.53}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_mix/ins\endcsname{40.18}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_mix/leak_wpm\endcsname{125.30}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_mix/miss\endcsname{18.71}
\expandafter\def\csname v@r/SB_long_k03_selfl/call_dev_mix/wer\endcsname{58.90}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev/dele\endcsname{4.05}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev/ins\endcsname{3.30}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev/leak_wpm\endcsname{6.61}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev/miss\endcsname{10.31}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev/wer\endcsname{13.61}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev_long/dele\endcsname{8.12}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev_long/ins\endcsname{9.34}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev_long/leak_wpm\endcsname{14.04}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev_long/miss\endcsname{15.78}
\expandafter\def\csname v@r/SB_long_lvl_null/ami_dev_long/wer\endcsname{25.12}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_clean/dele\endcsname{5.26}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_clean/ins\endcsname{0.36}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_clean/miss\endcsname{6.03}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_clean/wer\endcsname{6.39}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_mix/dele\endcsname{5.22}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_mix/ins\endcsname{30.58}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_mix/leak_wpm\endcsname{78.88}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_mix/miss\endcsname{17.67}
\expandafter\def\csname v@r/SB_long_lvl_null/call_dev_mix/wer\endcsname{48.25}
\expandafter\def\csname v@r/SB_long_lvl_null/dev4\endcsname{13.28}
\expandafter\def\csname v@r/SB_long_lvl_null/krisp/dele\endcsname{2.79}
\expandafter\def\csname v@r/SB_long_lvl_null/krisp/ins\endcsname{1.60}
\expandafter\def\csname v@r/SB_long_lvl_null/krisp/leak_wpm\endcsname{3.35}
\expandafter\def\csname v@r/SB_long_lvl_null/krisp/miss\endcsname{6.55}
\expandafter\def\csname v@r/SB_long_lvl_null/krisp/wer\endcsname{8.15}
\expandafter\def\csname v@r/SB_long_lvl_null/meet3\endcsname{15.57}
\expandafter\def\csname v@r/SB_long_lvl_null/nsf_dev/dele\endcsname{1.93}
\expandafter\def\csname v@r/SB_long_lvl_null/nsf_dev/ins\endcsname{1.80}
\expandafter\def\csname v@r/SB_long_lvl_null/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/SB_long_lvl_null/nsf_dev/miss\endcsname{6.18}
\expandafter\def\csname v@r/SB_long_lvl_null/nsf_dev/wer\endcsname{7.98}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev/dele\endcsname{4.09}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev/ins\endcsname{3.51}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev/leak_wpm\endcsname{7.01}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev/miss\endcsname{10.32}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev/wer\endcsname{13.83}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev_long/dele\endcsname{8.30}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev_long/ins\endcsname{4.00}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev_long/leak_wpm\endcsname{8.16}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev_long/miss\endcsname{16.65}
\expandafter\def\csname v@r/SB_long_lvl_self/ami_dev_long/wer\endcsname{20.64}
\expandafter\def\csname v@r/SB_long_lvl_self/krisp/dele\endcsname{1.76}
\expandafter\def\csname v@r/SB_long_lvl_self/krisp/ins\endcsname{0.85}
\expandafter\def\csname v@r/SB_long_lvl_self/krisp/leak_wpm\endcsname{0.69}
\expandafter\def\csname v@r/SB_long_lvl_self/krisp/miss\endcsname{5.49}
\expandafter\def\csname v@r/SB_long_lvl_self/krisp/wer\endcsname{6.34}
\expandafter\def\csname v@r/SB_long_lvl_self/meet3\endcsname{14.14}
\expandafter\def\csname v@r/SB_long_lvl_self/nsf_dev/dele\endcsname{1.87}
\expandafter\def\csname v@r/SB_long_lvl_self/nsf_dev/ins\endcsname{1.78}
\expandafter\def\csname v@r/SB_long_lvl_self/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/SB_long_lvl_self/nsf_dev/miss\endcsname{6.18}
\expandafter\def\csname v@r/SB_long_lvl_self/nsf_dev/wer\endcsname{7.96}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev/dele\endcsname{4.01}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev/ins\endcsname{2.95}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev/leak_wpm\endcsname{6.65}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev/miss\endcsname{10.35}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev/wer\endcsname{13.30}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev_long/dele\endcsname{9.04}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev_long/ins\endcsname{3.87}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev_long/leak_wpm\endcsname{6.84}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev_long/miss\endcsname{16.30}
\expandafter\def\csname v@r/SB_long_lvl_selfl/ami_dev_long/wer\endcsname{20.17}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_clean/dele\endcsname{8.48}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_clean/miss\endcsname{9.69}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_clean/wer\endcsname{9.99}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_mix/dele\endcsname{6.21}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_mix/ins\endcsname{30.84}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_mix/leak_wpm\endcsname{110.92}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_mix/miss\endcsname{20.98}
\expandafter\def\csname v@r/SB_long_lvl_selfl/call_dev_mix/wer\endcsname{51.82}
\expandafter\def\csname v@r/SB_long_lvl_selfl/dev4\endcsname{12.88}
\expandafter\def\csname v@r/SB_long_lvl_selfl/krisp/dele\endcsname{1.63}
\expandafter\def\csname v@r/SB_long_lvl_selfl/krisp/ins\endcsname{0.83}
\expandafter\def\csname v@r/SB_long_lvl_selfl/krisp/leak_wpm\endcsname{0.45}
\expandafter\def\csname v@r/SB_long_lvl_selfl/krisp/miss\endcsname{5.34}
\expandafter\def\csname v@r/SB_long_lvl_selfl/krisp/wer\endcsname{6.17}
\expandafter\def\csname v@r/SB_long_lvl_selfl/meet3\endcsname{13.85}
\expandafter\def\csname v@r/SB_long_lvl_selfl/nsf_dev/dele\endcsname{1.99}
\expandafter\def\csname v@r/SB_long_lvl_selfl/nsf_dev/ins\endcsname{1.79}
\expandafter\def\csname v@r/SB_long_lvl_selfl/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/SB_long_lvl_selfl/nsf_dev/miss\endcsname{6.27}
\expandafter\def\csname v@r/SB_long_lvl_selfl/nsf_dev/wer\endcsname{8.06}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev/dele\endcsname{4.33}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev/ins\endcsname{3.01}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev/leak_wpm\endcsname{6.34}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev/miss\endcsname{10.79}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev/wer\endcsname{13.80}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev_long/dele\endcsname{8.07}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev_long/ins\endcsname{8.95}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev_long/leak_wpm\endcsname{13.25}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev_long/miss\endcsname{15.76}
\expandafter\def\csname v@r/SB_long_spk_null/ami_dev_long/wer\endcsname{24.70}
\expandafter\def\csname v@r/SB_long_spk_null/krisp/dele\endcsname{2.07}
\expandafter\def\csname v@r/SB_long_spk_null/krisp/ins\endcsname{1.18}
\expandafter\def\csname v@r/SB_long_spk_null/krisp/leak_wpm\endcsname{1.80}
\expandafter\def\csname v@r/SB_long_spk_null/krisp/miss\endcsname{5.81}
\expandafter\def\csname v@r/SB_long_spk_null/krisp/wer\endcsname{6.99}
\expandafter\def\csname v@r/SB_long_spk_null/meet3\endcsname{15.59}
\expandafter\def\csname v@r/SB_long_spk_null/nsf_dev/dele\endcsname{2.38}
\expandafter\def\csname v@r/SB_long_spk_null/nsf_dev/ins\endcsname{1.66}
\expandafter\def\csname v@r/SB_long_spk_null/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/SB_long_spk_null/nsf_dev/miss\endcsname{6.61}
\expandafter\def\csname v@r/SB_long_spk_null/nsf_dev/wer\endcsname{8.27}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev/dele\endcsname{4.30}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev/ins\endcsname{3.45}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev/leak_wpm\endcsname{7.99}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev/miss\endcsname{10.56}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev/wer\endcsname{14.01}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev_long/dele\endcsname{10.37}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev_long/ins\endcsname{7.99}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev_long/leak_wpm\endcsname{12.75}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev_long/miss\endcsname{18.29}
\expandafter\def\csname v@r/SB_long_spk_self/ami_dev_long/wer\endcsname{26.28}
\expandafter\def\csname v@r/SB_long_spk_self/krisp/dele\endcsname{3.05}
\expandafter\def\csname v@r/SB_long_spk_self/krisp/ins\endcsname{1.39}
\expandafter\def\csname v@r/SB_long_spk_self/krisp/leak_wpm\endcsname{2.84}
\expandafter\def\csname v@r/SB_long_spk_self/krisp/miss\endcsname{7.57}
\expandafter\def\csname v@r/SB_long_spk_self/krisp/wer\endcsname{8.96}
\expandafter\def\csname v@r/SB_long_spk_self/meet3\endcsname{16.18}
\expandafter\def\csname v@r/SB_long_spk_self/nsf_dev/dele\endcsname{2.30}
\expandafter\def\csname v@r/SB_long_spk_self/nsf_dev/ins\endcsname{1.67}
\expandafter\def\csname v@r/SB_long_spk_self/nsf_dev/leak_wpm\endcsname{0.34}
\expandafter\def\csname v@r/SB_long_spk_self/nsf_dev/miss\endcsname{6.58}
\expandafter\def\csname v@r/SB_long_spk_self/nsf_dev/wer\endcsname{8.26}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev/dele\endcsname{4.63}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev/ins\endcsname{3.12}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev/leak_wpm\endcsname{6.52}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev/miss\endcsname{10.82}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev/wer\endcsname{13.94}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev_long/dele\endcsname{10.55}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev_long/ins\endcsname{2.97}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev_long/leak_wpm\endcsname{6.21}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev_long/miss\endcsname{17.98}
\expandafter\def\csname v@r/SB_long_ssl_selfl/ami_dev_long/wer\endcsname{20.95}
\expandafter\def\csname v@r/SB_long_ssl_selfl/krisp/dele\endcsname{3.50}
\expandafter\def\csname v@r/SB_long_ssl_selfl/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/SB_long_ssl_selfl/krisp/leak_wpm\endcsname{0.37}
\expandafter\def\csname v@r/SB_long_ssl_selfl/krisp/miss\endcsname{7.32}
\expandafter\def\csname v@r/SB_long_ssl_selfl/krisp/wer\endcsname{8.05}
\expandafter\def\csname v@r/SB_long_ssl_selfl/meet3\endcsname{14.42}
\expandafter\def\csname v@r/SB_long_ssl_selfl/nsf_dev/dele\endcsname{2.34}
\expandafter\def\csname v@r/SB_long_ssl_selfl/nsf_dev/ins\endcsname{1.76}
\expandafter\def\csname v@r/SB_long_ssl_selfl/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/SB_long_ssl_selfl/nsf_dev/miss\endcsname{6.61}
\expandafter\def\csname v@r/SB_long_ssl_selfl/nsf_dev/wer\endcsname{8.36}
\expandafter\def\csname v@r/dfn3/aic_calls/dele\endcsname{3.49}
\expandafter\def\csname v@r/dfn3/aic_calls/ins\endcsname{26.12}
\expandafter\def\csname v@r/dfn3/aic_calls/leak_wpm\endcsname{36.97}
\expandafter\def\csname v@r/dfn3/aic_calls/miss\endcsname{9.23}
\expandafter\def\csname v@r/dfn3/aic_calls/wer\endcsname{35.35}
\expandafter\def\csname v@r/dfn3/ami_dev/dele\endcsname{4.88}
\expandafter\def\csname v@r/dfn3/ami_dev/ins\endcsname{30.32}
\expandafter\def\csname v@r/dfn3/ami_dev/leak_wpm\endcsname{84.78}
\expandafter\def\csname v@r/dfn3/ami_dev/miss\endcsname{11.39}
\expandafter\def\csname v@r/dfn3/ami_dev/wer\endcsname{41.71}
\expandafter\def\csname v@r/dfn3/ami_dev_long/dele\endcsname{6.08}
\expandafter\def\csname v@r/dfn3/ami_dev_long/ins\endcsname{75.17}
\expandafter\def\csname v@r/dfn3/ami_dev_long/leak_wpm\endcsname{91.98}
\expandafter\def\csname v@r/dfn3/ami_dev_long/miss\endcsname{14.66}
\expandafter\def\csname v@r/dfn3/ami_dev_long/wer\endcsname{89.83}
\expandafter\def\csname v@r/dfn3/call_dev_clean/dele\endcsname{1.79}
\expandafter\def\csname v@r/dfn3/call_dev_clean/ins\endcsname{0.20}
\expandafter\def\csname v@r/dfn3/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/dfn3/call_dev_clean/miss\endcsname{2.37}
\expandafter\def\csname v@r/dfn3/call_dev_clean/wer\endcsname{2.57}
\expandafter\def\csname v@r/dfn3/call_dev_mix/dele\endcsname{2.82}
\expandafter\def\csname v@r/dfn3/call_dev_mix/ins\endcsname{59.95}
\expandafter\def\csname v@r/dfn3/call_dev_mix/leak_wpm\endcsname{147.48}
\expandafter\def\csname v@r/dfn3/call_dev_mix/miss\endcsname{13.49}
\expandafter\def\csname v@r/dfn3/call_dev_mix/wer\endcsname{73.44}
\expandafter\def\csname v@r/dfn3/dev4\endcsname{37.53}
\expandafter\def\csname v@r/dfn3/krisp/dele\endcsname{3.26}
\expandafter\def\csname v@r/dfn3/krisp/ins\endcsname{6.18}
\expandafter\def\csname v@r/dfn3/krisp/leak_wpm\endcsname{20.34}
\expandafter\def\csname v@r/dfn3/krisp/miss\endcsname{6.96}
\expandafter\def\csname v@r/dfn3/krisp/wer\endcsname{13.15}
\expandafter\def\csname v@r/dfn3/meet3\endcsname{49.18}
\expandafter\def\csname v@r/dfn3/nsf_dev/dele\endcsname{1.87}
\expandafter\def\csname v@r/dfn3/nsf_dev/ins\endcsname{9.90}
\expandafter\def\csname v@r/dfn3/nsf_dev/leak_wpm\endcsname{28.50}
\expandafter\def\csname v@r/dfn3/nsf_dev/miss\endcsname{6.11}
\expandafter\def\csname v@r/dfn3/nsf_dev/wer\endcsname{16.00}
\expandafter\def\csname v@r/pre_null/aic_calls/dele\endcsname{2.60}
\expandafter\def\csname v@r/pre_null/aic_calls/ins\endcsname{7.88}
\expandafter\def\csname v@r/pre_null/aic_calls/leak_wpm\endcsname{8.20}
\expandafter\def\csname v@r/pre_null/aic_calls/miss\endcsname{6.63}
\expandafter\def\csname v@r/pre_null/aic_calls/wer\endcsname{14.50}
\expandafter\def\csname v@r/pre_null/ami_dev/dele\endcsname{3.08}
\expandafter\def\csname v@r/pre_null/ami_dev/ins\endcsname{4.13}
\expandafter\def\csname v@r/pre_null/ami_dev/leak_wpm\endcsname{9.15}
\expandafter\def\csname v@r/pre_null/ami_dev/miss\endcsname{9.06}
\expandafter\def\csname v@r/pre_null/ami_dev/wer\endcsname{13.19}
\expandafter\def\csname v@r/pre_null/ami_dev_long/dele\endcsname{5.69}
\expandafter\def\csname v@r/pre_null/ami_dev_long/ins\endcsname{7.90}
\expandafter\def\csname v@r/pre_null/ami_dev_long/leak_wpm\endcsname{11.60}
\expandafter\def\csname v@r/pre_null/ami_dev_long/miss\endcsname{13.29}
\expandafter\def\csname v@r/pre_null/ami_dev_long/wer\endcsname{21.19}
\expandafter\def\csname v@r/pre_null/call_dev_clean/dele\endcsname{2.62}
\expandafter\def\csname v@r/pre_null/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/pre_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_null/call_dev_clean/miss\endcsname{3.37}
\expandafter\def\csname v@r/pre_null/call_dev_clean/wer\endcsname{3.61}
\expandafter\def\csname v@r/pre_null/call_dev_mix/dele\endcsname{3.26}
\expandafter\def\csname v@r/pre_null/call_dev_mix/ins\endcsname{34.89}
\expandafter\def\csname v@r/pre_null/call_dev_mix/leak_wpm\endcsname{99.42}
\expandafter\def\csname v@r/pre_null/call_dev_mix/miss\endcsname{14.88}
\expandafter\def\csname v@r/pre_null/call_dev_mix/wer\endcsname{49.77}
\expandafter\def\csname v@r/pre_null/dev4\endcsname{11.43}
\expandafter\def\csname v@r/pre_null/krisp/dele\endcsname{1.36}
\expandafter\def\csname v@r/pre_null/krisp/ins\endcsname{1.09}
\expandafter\def\csname v@r/pre_null/krisp/leak_wpm\endcsname{1.39}
\expandafter\def\csname v@r/pre_null/krisp/miss\endcsname{4.76}
\expandafter\def\csname v@r/pre_null/krisp/wer\endcsname{5.85}
\expandafter\def\csname v@r/pre_null/meet3\endcsname{14.04}
\expandafter\def\csname v@r/pre_null/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/pre_null/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/pre_null/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/pre_null/nsf_dev/miss\endcsname{5.79}
\expandafter\def\csname v@r/pre_null/nsf_dev/wer\endcsname{7.72}
\expandafter\def\csname v@r/pre_null_pr1/call_dev_clean/dele\endcsname{1.58}
\expandafter\def\csname v@r/pre_null_pr1/call_dev_clean/ins\endcsname{0.22}
\expandafter\def\csname v@r/pre_null_pr1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_null_pr1/call_dev_clean/miss\endcsname{2.26}
\expandafter\def\csname v@r/pre_null_pr1/call_dev_clean/wer\endcsname{2.47}
\expandafter\def\csname v@r/pre_selfl/aic_calls/dele\endcsname{2.71}
\expandafter\def\csname v@r/pre_selfl/aic_calls/ins\endcsname{7.84}
\expandafter\def\csname v@r/pre_selfl/aic_calls/leak_wpm\endcsname{7.95}
\expandafter\def\csname v@r/pre_selfl/aic_calls/miss\endcsname{6.52}
\expandafter\def\csname v@r/pre_selfl/aic_calls/wer\endcsname{14.36}
\expandafter\def\csname v@r/pre_selfl/ami_dev/dele\endcsname{3.25}
\expandafter\def\csname v@r/pre_selfl/ami_dev/ins\endcsname{3.91}
\expandafter\def\csname v@r/pre_selfl/ami_dev/leak_wpm\endcsname{8.57}
\expandafter\def\csname v@r/pre_selfl/ami_dev/miss\endcsname{9.09}
\expandafter\def\csname v@r/pre_selfl/ami_dev/wer\endcsname{13.00}
\expandafter\def\csname v@r/pre_selfl/ami_dev_long/dele\endcsname{6.86}
\expandafter\def\csname v@r/pre_selfl/ami_dev_long/ins\endcsname{3.19}
\expandafter\def\csname v@r/pre_selfl/ami_dev_long/leak_wpm\endcsname{5.81}
\expandafter\def\csname v@r/pre_selfl/ami_dev_long/miss\endcsname{14.39}
\expandafter\def\csname v@r/pre_selfl/ami_dev_long/wer\endcsname{17.59}
\expandafter\def\csname v@r/pre_selfl/call_dev_clean/dele\endcsname{2.82}
\expandafter\def\csname v@r/pre_selfl/call_dev_clean/ins\endcsname{0.29}
\expandafter\def\csname v@r/pre_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfl/call_dev_clean/miss\endcsname{3.63}
\expandafter\def\csname v@r/pre_selfl/call_dev_clean/wer\endcsname{3.92}
\expandafter\def\csname v@r/pre_selfl/call_dev_mix/dele\endcsname{3.75}
\expandafter\def\csname v@r/pre_selfl/call_dev_mix/ins\endcsname{34.51}
\expandafter\def\csname v@r/pre_selfl/call_dev_mix/leak_wpm\endcsname{112.98}
\expandafter\def\csname v@r/pre_selfl/call_dev_mix/miss\endcsname{16.54}
\expandafter\def\csname v@r/pre_selfl/call_dev_mix/wer\endcsname{51.05}
\expandafter\def\csname v@r/pre_selfl/dev4\endcsname{10.55}
\expandafter\def\csname v@r/pre_selfl/krisp/dele\endcsname{1.41}
\expandafter\def\csname v@r/pre_selfl/krisp/ins\endcsname{0.71}
\expandafter\def\csname v@r/pre_selfl/krisp/leak_wpm\endcsname{0.11}
\expandafter\def\csname v@r/pre_selfl/krisp/miss\endcsname{4.84}
\expandafter\def\csname v@r/pre_selfl/krisp/wer\endcsname{5.55}
\expandafter\def\csname v@r/pre_selfl/meet3\endcsname{12.76}
\expandafter\def\csname v@r/pre_selfl/nsf_dev/dele\endcsname{1.51}
\expandafter\def\csname v@r/pre_selfl/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/pre_selfl/nsf_dev/leak_wpm\endcsname{0.60}
\expandafter\def\csname v@r/pre_selfl/nsf_dev/miss\endcsname{5.75}
\expandafter\def\csname v@r/pre_selfl/nsf_dev/wer\endcsname{7.69}
\expandafter\def\csname v@r/pre_selfl1/aic_calls/dele\endcsname{2.96}
\expandafter\def\csname v@r/pre_selfl1/aic_calls/ins\endcsname{8.09}
\expandafter\def\csname v@r/pre_selfl1/aic_calls/leak_wpm\endcsname{7.70}
\expandafter\def\csname v@r/pre_selfl1/aic_calls/miss\endcsname{6.52}
\expandafter\def\csname v@r/pre_selfl1/aic_calls/wer\endcsname{14.61}
\expandafter\def\csname v@r/pre_selfl1/ami_dev/dele\endcsname{3.08}
\expandafter\def\csname v@r/pre_selfl1/ami_dev/ins\endcsname{3.76}
\expandafter\def\csname v@r/pre_selfl1/ami_dev/leak_wpm\endcsname{8.44}
\expandafter\def\csname v@r/pre_selfl1/ami_dev/miss\endcsname{9.18}
\expandafter\def\csname v@r/pre_selfl1/ami_dev/wer\endcsname{12.94}
\expandafter\def\csname v@r/pre_selfl1/ami_dev_long/dele\endcsname{6.54}
\expandafter\def\csname v@r/pre_selfl1/ami_dev_long/ins\endcsname{3.19}
\expandafter\def\csname v@r/pre_selfl1/ami_dev_long/leak_wpm\endcsname{5.84}
\expandafter\def\csname v@r/pre_selfl1/ami_dev_long/miss\endcsname{14.10}
\expandafter\def\csname v@r/pre_selfl1/ami_dev_long/wer\endcsname{17.30}
\expandafter\def\csname v@r/pre_selfl1/call_dev_clean/dele\endcsname{2.68}
\expandafter\def\csname v@r/pre_selfl1/call_dev_clean/ins\endcsname{0.29}
\expandafter\def\csname v@r/pre_selfl1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfl1/call_dev_clean/miss\endcsname{3.56}
\expandafter\def\csname v@r/pre_selfl1/call_dev_clean/wer\endcsname{3.85}
\expandafter\def\csname v@r/pre_selfl1/call_dev_mix/dele\endcsname{3.55}
\expandafter\def\csname v@r/pre_selfl1/call_dev_mix/ins\endcsname{35.12}
\expandafter\def\csname v@r/pre_selfl1/call_dev_mix/leak_wpm\endcsname{111.74}
\expandafter\def\csname v@r/pre_selfl1/call_dev_mix/miss\endcsname{16.02}
\expandafter\def\csname v@r/pre_selfl1/call_dev_mix/wer\endcsname{51.14}
\expandafter\def\csname v@r/pre_selfl1/dev4\endcsname{10.43}
\expandafter\def\csname v@r/pre_selfl1/krisp/dele\endcsname{1.49}
\expandafter\def\csname v@r/pre_selfl1/krisp/ins\endcsname{0.73}
\expandafter\def\csname v@r/pre_selfl1/krisp/leak_wpm\endcsname{0.11}
\expandafter\def\csname v@r/pre_selfl1/krisp/miss\endcsname{4.91}
\expandafter\def\csname v@r/pre_selfl1/krisp/wer\endcsname{5.63}
\expandafter\def\csname v@r/pre_selfl1/meet3\endcsname{12.63}
\expandafter\def\csname v@r/pre_selfl1/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/pre_selfl1/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/pre_selfl1/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@r/pre_selfl1/nsf_dev/miss\endcsname{5.70}
\expandafter\def\csname v@r/pre_selfl1/nsf_dev/wer\endcsname{7.64}
\expandafter\def\csname v@r/pre_selfl2/ami_dev/dele\endcsname{3.20}
\expandafter\def\csname v@r/pre_selfl2/ami_dev/ins\endcsname{3.90}
\expandafter\def\csname v@r/pre_selfl2/ami_dev/leak_wpm\endcsname{8.30}
\expandafter\def\csname v@r/pre_selfl2/ami_dev/miss\endcsname{9.13}
\expandafter\def\csname v@r/pre_selfl2/ami_dev/wer\endcsname{13.03}
\expandafter\def\csname v@r/pre_selfl2/ami_dev_long/dele\endcsname{6.92}
\expandafter\def\csname v@r/pre_selfl2/ami_dev_long/ins\endcsname{3.11}
\expandafter\def\csname v@r/pre_selfl2/ami_dev_long/leak_wpm\endcsname{5.82}
\expandafter\def\csname v@r/pre_selfl2/ami_dev_long/miss\endcsname{14.39}
\expandafter\def\csname v@r/pre_selfl2/ami_dev_long/wer\endcsname{17.50}
\expandafter\def\csname v@r/pre_selfl2/call_dev_clean/dele\endcsname{2.77}
\expandafter\def\csname v@r/pre_selfl2/call_dev_clean/ins\endcsname{0.30}
\expandafter\def\csname v@r/pre_selfl2/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfl2/call_dev_clean/miss\endcsname{3.58}
\expandafter\def\csname v@r/pre_selfl2/call_dev_clean/wer\endcsname{3.88}
\expandafter\def\csname v@r/pre_selfl2/call_dev_mix/dele\endcsname{3.75}
\expandafter\def\csname v@r/pre_selfl2/call_dev_mix/ins\endcsname{34.84}
\expandafter\def\csname v@r/pre_selfl2/call_dev_mix/leak_wpm\endcsname{112.98}
\expandafter\def\csname v@r/pre_selfl2/call_dev_mix/miss\endcsname{16.32}
\expandafter\def\csname v@r/pre_selfl2/call_dev_mix/wer\endcsname{51.17}
\expandafter\def\csname v@r/pre_selfl2/dev4\endcsname{10.52}
\expandafter\def\csname v@r/pre_selfl2/krisp/dele\endcsname{1.50}
\expandafter\def\csname v@r/pre_selfl2/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/pre_selfl2/krisp/leak_wpm\endcsname{0.11}
\expandafter\def\csname v@r/pre_selfl2/krisp/miss\endcsname{4.88}
\expandafter\def\csname v@r/pre_selfl2/krisp/wer\endcsname{5.58}
\expandafter\def\csname v@r/pre_selfl2/meet3\endcsname{12.73}
\expandafter\def\csname v@r/pre_selfl2/nsf_dev/dele\endcsname{1.52}
\expandafter\def\csname v@r/pre_selfl2/nsf_dev/ins\endcsname{1.94}
\expandafter\def\csname v@r/pre_selfl2/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@r/pre_selfl2/nsf_dev/miss\endcsname{5.72}
\expandafter\def\csname v@r/pre_selfl2/nsf_dev/wer\endcsname{7.66}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev/dele\endcsname{2.82}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev/ins\endcsname{26.08}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev/leak_wpm\endcsname{75.27}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev/miss\endcsname{9.43}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev/wer\endcsname{35.51}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev_long/dele\endcsname{5.00}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev_long/ins\endcsname{88.28}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev_long/leak_wpm\endcsname{109.79}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev_long/miss\endcsname{14.94}
\expandafter\def\csname v@r/pre_selfl_oa20/ami_dev_long/wer\endcsname{103.22}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_clean/dele\endcsname{1.18}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_clean/miss\endcsname{1.70}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_clean/wer\endcsname{1.92}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_mix/dele\endcsname{2.17}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_mix/ins\endcsname{58.38}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_mix/leak_wpm\endcsname{146.66}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_mix/miss\endcsname{12.15}
\expandafter\def\csname v@r/pre_selfl_oa20/call_dev_mix/wer\endcsname{70.53}
\expandafter\def\csname v@r/pre_selfl_oa20/dev4\endcsname{39.95}
\expandafter\def\csname v@r/pre_selfl_oa20/krisp/dele\endcsname{0.72}
\expandafter\def\csname v@r/pre_selfl_oa20/krisp/ins\endcsname{8.75}
\expandafter\def\csname v@r/pre_selfl_oa20/krisp/leak_wpm\endcsname{29.97}
\expandafter\def\csname v@r/pre_selfl_oa20/krisp/miss\endcsname{4.04}
\expandafter\def\csname v@r/pre_selfl_oa20/krisp/wer\endcsname{12.79}
\expandafter\def\csname v@r/pre_selfl_oa20/meet3\endcsname{52.63}
\expandafter\def\csname v@r/pre_selfl_oa20/nsf_dev/dele\endcsname{1.94}
\expandafter\def\csname v@r/pre_selfl_oa20/nsf_dev/ins\endcsname{12.71}
\expandafter\def\csname v@r/pre_selfl_oa20/nsf_dev/leak_wpm\endcsname{38.89}
\expandafter\def\csname v@r/pre_selfl_oa20/nsf_dev/miss\endcsname{6.44}
\expandafter\def\csname v@r/pre_selfl_oa20/nsf_dev/wer\endcsname{19.16}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev/dele\endcsname{3.38}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev/ins\endcsname{21.27}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev/leak_wpm\endcsname{59.11}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev/miss\endcsname{9.57}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev/wer\endcsname{30.84}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev_long/dele\endcsname{4.84}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev_long/ins\endcsname{68.17}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev_long/leak_wpm\endcsname{85.37}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev_long/miss\endcsname{13.96}
\expandafter\def\csname v@r/pre_selfl_oa30/ami_dev_long/wer\endcsname{82.13}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_clean/dele\endcsname{1.27}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_clean/ins\endcsname{0.20}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_clean/miss\endcsname{1.76}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_clean/wer\endcsname{1.96}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_mix/dele\endcsname{2.71}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_mix/ins\endcsname{55.37}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_mix/leak_wpm\endcsname{142.55}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_mix/miss\endcsname{12.33}
\expandafter\def\csname v@r/pre_selfl_oa30/call_dev_mix/wer\endcsname{67.70}
\expandafter\def\csname v@r/pre_selfl_oa30/dev4\endcsname{31.14}
\expandafter\def\csname v@r/pre_selfl_oa30/krisp/dele\endcsname{0.74}
\expandafter\def\csname v@r/pre_selfl_oa30/krisp/ins\endcsname{3.67}
\expandafter\def\csname v@r/pre_selfl_oa30/krisp/leak_wpm\endcsname{11.18}
\expandafter\def\csname v@r/pre_selfl_oa30/krisp/miss\endcsname{4.11}
\expandafter\def\csname v@r/pre_selfl_oa30/krisp/wer\endcsname{7.78}
\expandafter\def\csname v@r/pre_selfl_oa30/meet3\endcsname{40.86}
\expandafter\def\csname v@r/pre_selfl_oa30/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/pre_selfl_oa30/nsf_dev/ins\endcsname{3.85}
\expandafter\def\csname v@r/pre_selfl_oa30/nsf_dev/leak_wpm\endcsname{7.20}
\expandafter\def\csname v@r/pre_selfl_oa30/nsf_dev/miss\endcsname{5.77}
\expandafter\def\csname v@r/pre_selfl_oa30/nsf_dev/wer\endcsname{9.62}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev/dele\endcsname{3.33}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev/ins\endcsname{4.52}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev/leak_wpm\endcsname{9.06}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev/miss\endcsname{8.96}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev/wer\endcsname{13.48}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev_long/dele\endcsname{7.80}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev_long/ins\endcsname{3.41}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev_long/leak_wpm\endcsname{5.89}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev_long/miss\endcsname{15.25}
\expandafter\def\csname v@r/pre_selfl_pr1/ami_dev_long/wer\endcsname{18.66}
\expandafter\def\csname v@r/pre_selfl_pr1/call_dev_clean/dele\endcsname{1.82}
\expandafter\def\csname v@r/pre_selfl_pr1/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/pre_selfl_pr1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfl_pr1/call_dev_clean/miss\endcsname{2.50}
\expandafter\def\csname v@r/pre_selfl_pr1/call_dev_clean/wer\endcsname{2.74}
\expandafter\def\csname v@r/pre_selfl_pr1/dev4\endcsname{10.65}
\expandafter\def\csname v@r/pre_selfl_pr1/meet3\endcsname{13.29}
\expandafter\def\csname v@r/pre_selfl_pr1/nsf_dev/dele\endcsname{1.42}
\expandafter\def\csname v@r/pre_selfl_pr1/nsf_dev/ins\endcsname{1.84}
\expandafter\def\csname v@r/pre_selfl_pr1/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/pre_selfl_pr1/nsf_dev/miss\endcsname{5.90}
\expandafter\def\csname v@r/pre_selfl_pr1/nsf_dev/wer\endcsname{7.73}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev/dele\endcsname{3.91}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev/ins\endcsname{4.37}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev/leak_wpm\endcsname{7.95}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev/miss\endcsname{9.77}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev/wer\endcsname{14.14}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev_long/dele\endcsname{9.91}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev_long/ins\endcsname{3.98}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev_long/leak_wpm\endcsname{6.42}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev_long/miss\endcsname{17.87}
\expandafter\def\csname v@r/pre_selfl_pt3/ami_dev_long/wer\endcsname{21.85}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_clean/dele\endcsname{1.67}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_clean/miss\endcsname{2.33}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_clean/wer\endcsname{2.56}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_mix/dele\endcsname{3.11}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_mix/ins\endcsname{36.09}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_mix/leak_wpm\endcsname{112.15}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_mix/miss\endcsname{15.38}
\expandafter\def\csname v@r/pre_selfl_pt3/call_dev_mix/wer\endcsname{51.46}
\expandafter\def\csname v@r/pre_selfl_pt3/dev4\endcsname{11.64}
\expandafter\def\csname v@r/pre_selfl_pt3/krisp/dele\endcsname{1.40}
\expandafter\def\csname v@r/pre_selfl_pt3/krisp/ins\endcsname{0.71}
\expandafter\def\csname v@r/pre_selfl_pt3/krisp/leak_wpm\endcsname{0.11}
\expandafter\def\csname v@r/pre_selfl_pt3/krisp/miss\endcsname{4.80}
\expandafter\def\csname v@r/pre_selfl_pt3/krisp/wer\endcsname{5.51}
\expandafter\def\csname v@r/pre_selfl_pt3/meet3\endcsname{14.67}
\expandafter\def\csname v@r/pre_selfl_pt3/nsf_dev/dele\endcsname{1.84}
\expandafter\def\csname v@r/pre_selfl_pt3/nsf_dev/ins\endcsname{1.86}
\expandafter\def\csname v@r/pre_selfl_pt3/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/pre_selfl_pt3/nsf_dev/miss\endcsname{6.16}
\expandafter\def\csname v@r/pre_selfl_pt3/nsf_dev/wer\endcsname{8.03}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev/dele\endcsname{3.77}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev/ins\endcsname{6.74}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev/leak_wpm\endcsname{13.57}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev/miss\endcsname{9.88}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev/wer\endcsname{16.62}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev_long/dele\endcsname{9.81}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev_long/ins\endcsname{6.24}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev_long/leak_wpm\endcsname{9.00}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev_long/miss\endcsname{17.61}
\expandafter\def\csname v@r/pre_selfl_pt5/ami_dev_long/wer\endcsname{23.85}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_clean/dele\endcsname{1.58}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_clean/miss\endcsname{2.21}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_clean/wer\endcsname{2.44}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_mix/dele\endcsname{3.04}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_mix/ins\endcsname{36.15}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_mix/leak_wpm\endcsname{112.56}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_mix/miss\endcsname{15.35}
\expandafter\def\csname v@r/pre_selfl_pt5/call_dev_mix/wer\endcsname{51.50}
\expandafter\def\csname v@r/pre_selfl_pt5/dev4\endcsname{13.07}
\expandafter\def\csname v@r/pre_selfl_pt5/krisp/dele\endcsname{1.36}
\expandafter\def\csname v@r/pre_selfl_pt5/krisp/ins\endcsname{0.70}
\expandafter\def\csname v@r/pre_selfl_pt5/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/pre_selfl_pt5/krisp/miss\endcsname{4.77}
\expandafter\def\csname v@r/pre_selfl_pt5/krisp/wer\endcsname{5.47}
\expandafter\def\csname v@r/pre_selfl_pt5/meet3\endcsname{16.62}
\expandafter\def\csname v@r/pre_selfl_pt5/nsf_dev/dele\endcsname{1.70}
\expandafter\def\csname v@r/pre_selfl_pt5/nsf_dev/ins\endcsname{3.30}
\expandafter\def\csname v@r/pre_selfl_pt5/nsf_dev/leak_wpm\endcsname{4.73}
\expandafter\def\csname v@r/pre_selfl_pt5/nsf_dev/miss\endcsname{6.08}
\expandafter\def\csname v@r/pre_selfl_pt5/nsf_dev/wer\endcsname{9.39}
\expandafter\def\csname v@r/pre_selfls/call_dev_clean/dele\endcsname{3.01}
\expandafter\def\csname v@r/pre_selfls/call_dev_clean/ins\endcsname{0.32}
\expandafter\def\csname v@r/pre_selfls/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfls/call_dev_clean/miss\endcsname{3.86}
\expandafter\def\csname v@r/pre_selfls/call_dev_clean/wer\endcsname{4.18}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev/dele\endcsname{3.34}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev/ins\endcsname{4.43}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev/leak_wpm\endcsname{8.79}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev/miss\endcsname{9.04}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev/wer\endcsname{13.47}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev_long/dele\endcsname{8.43}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev_long/ins\endcsname{3.45}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev_long/leak_wpm\endcsname{5.78}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev_long/miss\endcsname{15.74}
\expandafter\def\csname v@r/pre_selfls_pr1/ami_dev_long/wer\endcsname{19.19}
\expandafter\def\csname v@r/pre_selfls_pr1/call_dev_clean/dele\endcsname{1.57}
\expandafter\def\csname v@r/pre_selfls_pr1/call_dev_clean/ins\endcsname{0.41}
\expandafter\def\csname v@r/pre_selfls_pr1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/pre_selfls_pr1/call_dev_clean/miss\endcsname{2.28}
\expandafter\def\csname v@r/pre_selfls_pr1/call_dev_clean/wer\endcsname{2.69}
\expandafter\def\csname v@r/pre_selfls_pr1/dev4\endcsname{10.77}
\expandafter\def\csname v@r/pre_selfls_pr1/meet3\endcsname{13.47}
\expandafter\def\csname v@r/pre_selfls_pr1/nsf_dev/dele\endcsname{1.42}
\expandafter\def\csname v@r/pre_selfls_pr1/nsf_dev/ins\endcsname{1.84}
\expandafter\def\csname v@r/pre_selfls_pr1/nsf_dev/leak_wpm\endcsname{0.55}
\expandafter\def\csname v@r/pre_selfls_pr1/nsf_dev/miss\endcsname{5.90}
\expandafter\def\csname v@r/pre_selfls_pr1/nsf_dev/wer\endcsname{7.73}
\expandafter\def\csname v@r/raw/aic_calls/dele\endcsname{1.35}
\expandafter\def\csname v@r/raw/aic_calls/ins\endcsname{57.59}
\expandafter\def\csname v@r/raw/aic_calls/leak_wpm\endcsname{86.75}
\expandafter\def\csname v@r/raw/aic_calls/miss\endcsname{8.77}
\expandafter\def\csname v@r/raw/aic_calls/wer\endcsname{66.36}
\expandafter\def\csname v@r/raw/ami_dev/dele\endcsname{3.25}
\expandafter\def\csname v@r/raw/ami_dev/ins\endcsname{41.75}
\expandafter\def\csname v@r/raw/ami_dev/leak_wpm\endcsname{122.77}
\expandafter\def\csname v@r/raw/ami_dev/miss\endcsname{11.17}
\expandafter\def\csname v@r/raw/ami_dev/wer\endcsname{52.92}
\expandafter\def\csname v@r/raw/ami_dev_long/dele\endcsname{1.69}
\expandafter\def\csname v@r/raw/ami_dev_long/ins\endcsname{129.22}
\expandafter\def\csname v@r/raw/ami_dev_long/leak_wpm\endcsname{155.49}
\expandafter\def\csname v@r/raw/ami_dev_long/miss\endcsname{12.33}
\expandafter\def\csname v@r/raw/ami_dev_long/wer\endcsname{141.56}
\expandafter\def\csname v@r/raw/call_dev_clean/dele\endcsname{0.00}
\expandafter\def\csname v@r/raw/call_dev_clean/ins\endcsname{0.00}
\expandafter\def\csname v@r/raw/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/raw/call_dev_clean/miss\endcsname{0.00}
\expandafter\def\csname v@r/raw/call_dev_clean/wer\endcsname{0.00}
\expandafter\def\csname v@r/raw/call_dev_mix/dele\endcsname{1.98}
\expandafter\def\csname v@r/raw/call_dev_mix/ins\endcsname{61.62}
\expandafter\def\csname v@r/raw/call_dev_mix/leak_wpm\endcsname{146.25}
\expandafter\def\csname v@r/raw/call_dev_mix/miss\endcsname{13.08}
\expandafter\def\csname v@r/raw/call_dev_mix/wer\endcsname{74.70}
\expandafter\def\csname v@r/raw/dev4\endcsname{57.30}
\expandafter\def\csname v@r/raw/krisp/dele\endcsname{1.01}
\expandafter\def\csname v@r/raw/krisp/ins\endcsname{18.92}
\expandafter\def\csname v@r/raw/krisp/leak_wpm\endcsname{66.44}
\expandafter\def\csname v@r/raw/krisp/miss\endcsname{4.27}
\expandafter\def\csname v@r/raw/krisp/wer\endcsname{23.19}
\expandafter\def\csname v@r/raw/meet3\endcsname{76.39}
\expandafter\def\csname v@r/raw/nsf_dev/dele\endcsname{1.73}
\expandafter\def\csname v@r/raw/nsf_dev/ins\endcsname{28.19}
\expandafter\def\csname v@r/raw/nsf_dev/leak_wpm\endcsname{91.63}
\expandafter\def\csname v@r/raw/nsf_dev/miss\endcsname{6.51}
\expandafter\def\csname v@r/raw/nsf_dev/wer\endcsname{34.71}
\expandafter\def\csname v@r/rel_null/aic_calls/dele\endcsname{2.82}
\expandafter\def\csname v@r/rel_null/aic_calls/ins\endcsname{8.27}
\expandafter\def\csname v@r/rel_null/aic_calls/leak_wpm\endcsname{8.45}
\expandafter\def\csname v@r/rel_null/aic_calls/miss\endcsname{6.20}
\expandafter\def\csname v@r/rel_null/aic_calls/wer\endcsname{14.47}
\expandafter\def\csname v@r/rel_null/ami_dev/dele\endcsname{3.26}
\expandafter\def\csname v@r/rel_null/ami_dev/ins\endcsname{4.15}
\expandafter\def\csname v@r/rel_null/ami_dev/leak_wpm\endcsname{8.44}
\expandafter\def\csname v@r/rel_null/ami_dev/miss\endcsname{9.14}
\expandafter\def\csname v@r/rel_null/ami_dev/wer\endcsname{13.29}
\expandafter\def\csname v@r/rel_null/ami_dev_long/dele\endcsname{6.34}
\expandafter\def\csname v@r/rel_null/ami_dev_long/ins\endcsname{8.41}
\expandafter\def\csname v@r/rel_null/ami_dev_long/leak_wpm\endcsname{12.50}
\expandafter\def\csname v@r/rel_null/ami_dev_long/miss\endcsname{14.15}
\expandafter\def\csname v@r/rel_null/ami_dev_long/wer\endcsname{22.57}
\expandafter\def\csname v@r/rel_null/call_dev_clean/dele\endcsname{1.76}
\expandafter\def\csname v@r/rel_null/call_dev_clean/ins\endcsname{0.23}
\expandafter\def\csname v@r/rel_null/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/rel_null/call_dev_clean/miss\endcsname{2.39}
\expandafter\def\csname v@r/rel_null/call_dev_clean/wer\endcsname{2.62}
\expandafter\def\csname v@r/rel_null/call_dev_mix/dele\endcsname{2.81}
\expandafter\def\csname v@r/rel_null/call_dev_mix/ins\endcsname{33.17}
\expandafter\def\csname v@r/rel_null/call_dev_mix/leak_wpm\endcsname{91.41}
\expandafter\def\csname v@r/rel_null/call_dev_mix/miss\endcsname{15.58}
\expandafter\def\csname v@r/rel_null/call_dev_mix/wer\endcsname{48.75}
\expandafter\def\csname v@r/rel_null/dev4\endcsname{11.56}
\expandafter\def\csname v@r/rel_null/krisp/dele\endcsname{1.59}
\expandafter\def\csname v@r/rel_null/krisp/ins\endcsname{1.14}
\expandafter\def\csname v@r/rel_null/krisp/leak_wpm\endcsname{1.80}
\expandafter\def\csname v@r/rel_null/krisp/miss\endcsname{5.14}
\expandafter\def\csname v@r/rel_null/krisp/wer\endcsname{6.28}
\expandafter\def\csname v@r/rel_null/meet3\endcsname{14.54}
\expandafter\def\csname v@r/rel_null/nsf_dev/dele\endcsname{1.55}
\expandafter\def\csname v@r/rel_null/nsf_dev/ins\endcsname{1.93}
\expandafter\def\csname v@r/rel_null/nsf_dev/leak_wpm\endcsname{0.51}
\expandafter\def\csname v@r/rel_null/nsf_dev/miss\endcsname{5.84}
\expandafter\def\csname v@r/rel_null/nsf_dev/wer\endcsname{7.77}
\expandafter\def\csname v@r/rel_selfl/aic_calls/dele\endcsname{2.57}
\expandafter\def\csname v@r/rel_selfl/aic_calls/ins\endcsname{8.52}
\expandafter\def\csname v@r/rel_selfl/aic_calls/leak_wpm\endcsname{8.39}
\expandafter\def\csname v@r/rel_selfl/aic_calls/miss\endcsname{5.74}
\expandafter\def\csname v@r/rel_selfl/aic_calls/wer\endcsname{14.26}
\expandafter\def\csname v@r/rel_selfl/ami_dev/dele\endcsname{3.29}
\expandafter\def\csname v@r/rel_selfl/ami_dev/ins\endcsname{4.16}
\expandafter\def\csname v@r/rel_selfl/ami_dev/leak_wpm\endcsname{9.15}
\expandafter\def\csname v@r/rel_selfl/ami_dev/miss\endcsname{9.07}
\expandafter\def\csname v@r/rel_selfl/ami_dev/wer\endcsname{13.23}
\expandafter\def\csname v@r/rel_selfl/ami_dev_long/dele\endcsname{7.76}
\expandafter\def\csname v@r/rel_selfl/ami_dev_long/ins\endcsname{2.98}
\expandafter\def\csname v@r/rel_selfl/ami_dev_long/leak_wpm\endcsname{5.63}
\expandafter\def\csname v@r/rel_selfl/ami_dev_long/miss\endcsname{15.02}
\expandafter\def\csname v@r/rel_selfl/ami_dev_long/wer\endcsname{18.00}
\expandafter\def\csname v@r/rel_selfl/call_dev_clean/dele\endcsname{1.96}
\expandafter\def\csname v@r/rel_selfl/call_dev_clean/ins\endcsname{0.25}
\expandafter\def\csname v@r/rel_selfl/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/rel_selfl/call_dev_clean/miss\endcsname{2.71}
\expandafter\def\csname v@r/rel_selfl/call_dev_clean/wer\endcsname{2.96}
\expandafter\def\csname v@r/rel_selfl/call_dev_mix/dele\endcsname{3.54}
\expandafter\def\csname v@r/rel_selfl/call_dev_mix/ins\endcsname{34.88}
\expandafter\def\csname v@r/rel_selfl/call_dev_mix/leak_wpm\endcsname{110.10}
\expandafter\def\csname v@r/rel_selfl/call_dev_mix/miss\endcsname{16.44}
\expandafter\def\csname v@r/rel_selfl/call_dev_mix/wer\endcsname{51.32}
\expandafter\def\csname v@r/rel_selfl/dev4\endcsname{10.49}
\expandafter\def\csname v@r/rel_selfl/krisp/dele\endcsname{1.57}
\expandafter\def\csname v@r/rel_selfl/krisp/ins\endcsname{0.67}
\expandafter\def\csname v@r/rel_selfl/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/rel_selfl/krisp/miss\endcsname{5.08}
\expandafter\def\csname v@r/rel_selfl/krisp/wer\endcsname{5.74}
\expandafter\def\csname v@r/rel_selfl/meet3\endcsname{13.00}
\expandafter\def\csname v@r/rel_selfl/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/rel_selfl/nsf_dev/ins\endcsname{1.90}
\expandafter\def\csname v@r/rel_selfl/nsf_dev/leak_wpm\endcsname{0.43}
\expandafter\def\csname v@r/rel_selfl/nsf_dev/miss\endcsname{5.87}
\expandafter\def\csname v@r/rel_selfl/nsf_dev/wer\endcsname{7.77}
\expandafter\def\csname v@r/rel_selfl1/ami_dev/dele\endcsname{3.16}
\expandafter\def\csname v@r/rel_selfl1/ami_dev/ins\endcsname{4.04}
\expandafter\def\csname v@r/rel_selfl1/ami_dev/leak_wpm\endcsname{8.84}
\expandafter\def\csname v@r/rel_selfl1/ami_dev/miss\endcsname{9.03}
\expandafter\def\csname v@r/rel_selfl1/ami_dev/wer\endcsname{13.07}
\expandafter\def\csname v@r/rel_selfl1/ami_dev_long/dele\endcsname{7.74}
\expandafter\def\csname v@r/rel_selfl1/ami_dev_long/ins\endcsname{3.19}
\expandafter\def\csname v@r/rel_selfl1/ami_dev_long/leak_wpm\endcsname{5.66}
\expandafter\def\csname v@r/rel_selfl1/ami_dev_long/miss\endcsname{14.90}
\expandafter\def\csname v@r/rel_selfl1/ami_dev_long/wer\endcsname{18.10}
\expandafter\def\csname v@r/rel_selfl1/call_dev_clean/dele\endcsname{2.02}
\expandafter\def\csname v@r/rel_selfl1/call_dev_clean/ins\endcsname{0.26}
\expandafter\def\csname v@r/rel_selfl1/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/rel_selfl1/call_dev_clean/miss\endcsname{2.84}
\expandafter\def\csname v@r/rel_selfl1/call_dev_clean/wer\endcsname{3.11}
\expandafter\def\csname v@r/rel_selfl1/call_dev_mix/dele\endcsname{3.81}
\expandafter\def\csname v@r/rel_selfl1/call_dev_mix/ins\endcsname{34.93}
\expandafter\def\csname v@r/rel_selfl1/call_dev_mix/leak_wpm\endcsname{114.00}
\expandafter\def\csname v@r/rel_selfl1/call_dev_mix/miss\endcsname{16.94}
\expandafter\def\csname v@r/rel_selfl1/call_dev_mix/wer\endcsname{51.87}
\expandafter\def\csname v@r/rel_selfl1/dev4\endcsname{10.52}
\expandafter\def\csname v@r/rel_selfl1/krisp/dele\endcsname{1.60}
\expandafter\def\csname v@r/rel_selfl1/krisp/ins\endcsname{0.67}
\expandafter\def\csname v@r/rel_selfl1/krisp/leak_wpm\endcsname{0.04}
\expandafter\def\csname v@r/rel_selfl1/krisp/miss\endcsname{5.12}
\expandafter\def\csname v@r/rel_selfl1/krisp/wer\endcsname{5.79}
\expandafter\def\csname v@r/rel_selfl1/meet3\endcsname{12.99}
\expandafter\def\csname v@r/rel_selfl1/nsf_dev/dele\endcsname{1.56}
\expandafter\def\csname v@r/rel_selfl1/nsf_dev/ins\endcsname{1.92}
\expandafter\def\csname v@r/rel_selfl1/nsf_dev/leak_wpm\endcsname{0.47}
\expandafter\def\csname v@r/rel_selfl1/nsf_dev/miss\endcsname{5.87}
\expandafter\def\csname v@r/rel_selfl1/nsf_dev/wer\endcsname{7.79}
\expandafter\def\csname v@r/sidon_vi/ami_dev/dele\endcsname{3.45}
\expandafter\def\csname v@r/sidon_vi/ami_dev/ins\endcsname{35.80}
\expandafter\def\csname v@r/sidon_vi/ami_dev/leak_wpm\endcsname{107.55}
\expandafter\def\csname v@r/sidon_vi/ami_dev/miss\endcsname{9.86}
\expandafter\def\csname v@r/sidon_vi/ami_dev/wer\endcsname{45.67}
\expandafter\def\csname v@r/sidon_vi/ami_dev_long/dele\endcsname{2.18}
\expandafter\def\csname v@r/sidon_vi/ami_dev_long/ins\endcsname{100.66}
\expandafter\def\csname v@r/sidon_vi/ami_dev_long/leak_wpm\endcsname{127.37}
\expandafter\def\csname v@r/sidon_vi/ami_dev_long/miss\endcsname{11.70}
\expandafter\def\csname v@r/sidon_vi/ami_dev_long/wer\endcsname{112.36}
\expandafter\def\csname v@r/sidon_vi/krisp/dele\endcsname{0.76}
\expandafter\def\csname v@r/sidon_vi/krisp/ins\endcsname{25.45}
\expandafter\def\csname v@r/sidon_vi/krisp/leak_wpm\endcsname{91.02}
\expandafter\def\csname v@r/sidon_vi/krisp/miss\endcsname{4.04}
\expandafter\def\csname v@r/sidon_vi/krisp/wer\endcsname{29.49}
\expandafter\def\csname v@r/sidon_vi/meet3\endcsname{61.98}
\expandafter\def\csname v@r/sidon_vi/nsf_dev/dele\endcsname{1.71}
\expandafter\def\csname v@r/sidon_vi/nsf_dev/ins\endcsname{21.70}
\expandafter\def\csname v@r/sidon_vi/nsf_dev/leak_wpm\endcsname{72.76}
\expandafter\def\csname v@r/sidon_vi/nsf_dev/miss\endcsname{6.21}
\expandafter\def\csname v@r/sidon_vi/nsf_dev/wer\endcsname{27.91}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev/dele\endcsname{3.27}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev/ins\endcsname{25.59}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev/leak_wpm\endcsname{77.23}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev/miss\endcsname{9.75}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev/wer\endcsname{35.34}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev_long/dele\endcsname{2.20}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev_long/ins\endcsname{78.75}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev_long/leak_wpm\endcsname{99.50}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev_long/miss\endcsname{12.15}
\expandafter\def\csname v@r/sidon_vi_lite/ami_dev_long/wer\endcsname{90.90}
\expandafter\def\csname v@r/sidon_vi_lite/krisp/dele\endcsname{1.42}
\expandafter\def\csname v@r/sidon_vi_lite/krisp/ins\endcsname{12.05}
\expandafter\def\csname v@r/sidon_vi_lite/krisp/leak_wpm\endcsname{42.50}
\expandafter\def\csname v@r/sidon_vi_lite/krisp/miss\endcsname{6.22}
\expandafter\def\csname v@r/sidon_vi_lite/krisp/wer\endcsname{18.27}
\expandafter\def\csname v@r/sidon_vi_lite/meet3\endcsname{46.13}
\expandafter\def\csname v@r/sidon_vi_lite/nsf_dev/dele\endcsname{1.50}
\expandafter\def\csname v@r/sidon_vi_lite/nsf_dev/ins\endcsname{6.34}
\expandafter\def\csname v@r/sidon_vi_lite/nsf_dev/leak_wpm\endcsname{17.08}
\expandafter\def\csname v@r/sidon_vi_lite/nsf_dev/miss\endcsname{5.79}
\expandafter\def\csname v@r/sidon_vi_lite/nsf_dev/wer\endcsname{12.13}
\expandafter\def\csname v@r/voxlock/aic_calls/dele\endcsname{3.17}
\expandafter\def\csname v@r/voxlock/aic_calls/ins\endcsname{13.83}
\expandafter\def\csname v@r/voxlock/aic_calls/leak_wpm\endcsname{18.04}
\expandafter\def\csname v@r/voxlock/aic_calls/miss\endcsname{6.49}
\expandafter\def\csname v@r/voxlock/aic_calls/wer\endcsname{20.31}
\expandafter\def\csname v@r/voxlock/ami_dev/dele\endcsname{3.90}
\expandafter\def\csname v@r/voxlock/ami_dev/ins\endcsname{3.80}
\expandafter\def\csname v@r/voxlock/ami_dev/leak_wpm\endcsname{8.17}
\expandafter\def\csname v@r/voxlock/ami_dev/miss\endcsname{9.68}
\expandafter\def\csname v@r/voxlock/ami_dev/wer\endcsname{13.48}
\expandafter\def\csname v@r/voxlock/ami_dev_long/dele\endcsname{13.34}
\expandafter\def\csname v@r/voxlock/ami_dev_long/ins\endcsname{2.83}
\expandafter\def\csname v@r/voxlock/ami_dev_long/leak_wpm\endcsname{6.18}
\expandafter\def\csname v@r/voxlock/ami_dev_long/miss\endcsname{20.83}
\expandafter\def\csname v@r/voxlock/ami_dev_long/wer\endcsname{23.66}
\expandafter\def\csname v@r/voxlock/call_dev_clean/dele\endcsname{1.59}
\expandafter\def\csname v@r/voxlock/call_dev_clean/ins\endcsname{0.24}
\expandafter\def\csname v@r/voxlock/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/voxlock/call_dev_clean/miss\endcsname{2.15}
\expandafter\def\csname v@r/voxlock/call_dev_clean/wer\endcsname{2.39}
\expandafter\def\csname v@r/voxlock/call_dev_mix/dele\endcsname{3.13}
\expandafter\def\csname v@r/voxlock/call_dev_mix/ins\endcsname{38.71}
\expandafter\def\csname v@r/voxlock/call_dev_mix/leak_wpm\endcsname{123.45}
\expandafter\def\csname v@r/voxlock/call_dev_mix/miss\endcsname{20.12}
\expandafter\def\csname v@r/voxlock/call_dev_mix/wer\endcsname{58.84}
\expandafter\def\csname v@r/voxlock/dev4\endcsname{11.91}
\expandafter\def\csname v@r/voxlock/krisp/dele\endcsname{1.07}
\expandafter\def\csname v@r/voxlock/krisp/ins\endcsname{0.72}
\expandafter\def\csname v@r/voxlock/krisp/leak_wpm\endcsname{0.07}
\expandafter\def\csname v@r/voxlock/krisp/miss\endcsname{4.46}
\expandafter\def\csname v@r/voxlock/krisp/wer\endcsname{5.19}
\expandafter\def\csname v@r/voxlock/meet3\endcsname{15.08}
\expandafter\def\csname v@r/voxlock/nsf_dev/dele\endcsname{1.91}
\expandafter\def\csname v@r/voxlock/nsf_dev/ins\endcsname{1.90}
\expandafter\def\csname v@r/voxlock/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@r/voxlock/nsf_dev/miss\endcsname{6.21}
\expandafter\def\csname v@r/voxlock/nsf_dev/wer\endcsname{8.11}
\expandafter\def\csname v@r/voxlock_live/aic_calls/dele\endcsname{2.85}
\expandafter\def\csname v@r/voxlock_live/aic_calls/ins\endcsname{17.03}
\expandafter\def\csname v@r/voxlock_live/aic_calls/leak_wpm\endcsname{24.80}
\expandafter\def\csname v@r/voxlock_live/aic_calls/miss\endcsname{7.52}
\expandafter\def\csname v@r/voxlock_live/aic_calls/wer\endcsname{24.55}
\expandafter\def\csname v@r/voxlock_live/ami_dev/dele\endcsname{4.11}
\expandafter\def\csname v@r/voxlock_live/ami_dev/ins\endcsname{6.64}
\expandafter\def\csname v@r/voxlock_live/ami_dev/leak_wpm\endcsname{13.13}
\expandafter\def\csname v@r/voxlock_live/ami_dev/miss\endcsname{9.74}
\expandafter\def\csname v@r/voxlock_live/ami_dev/wer\endcsname{16.38}
\expandafter\def\csname v@r/voxlock_live/ami_dev_long/dele\endcsname{12.68}
\expandafter\def\csname v@r/voxlock_live/ami_dev_long/ins\endcsname{6.50}
\expandafter\def\csname v@r/voxlock_live/ami_dev_long/leak_wpm\endcsname{10.75}
\expandafter\def\csname v@r/voxlock_live/ami_dev_long/miss\endcsname{20.89}
\expandafter\def\csname v@r/voxlock_live/ami_dev_long/wer\endcsname{27.39}
\expandafter\def\csname v@r/voxlock_live/call_dev_clean/dele\endcsname{1.53}
\expandafter\def\csname v@r/voxlock_live/call_dev_clean/ins\endcsname{0.08}
\expandafter\def\csname v@r/voxlock_live/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/voxlock_live/call_dev_clean/miss\endcsname{2.01}
\expandafter\def\csname v@r/voxlock_live/call_dev_clean/wer\endcsname{2.09}
\expandafter\def\csname v@r/voxlock_live/call_dev_mix/dele\endcsname{2.45}
\expandafter\def\csname v@r/voxlock_live/call_dev_mix/ins\endcsname{45.12}
\expandafter\def\csname v@r/voxlock_live/call_dev_mix/leak_wpm\endcsname{126.12}
\expandafter\def\csname v@r/voxlock_live/call_dev_mix/miss\endcsname{19.70}
\expandafter\def\csname v@r/voxlock_live/call_dev_mix/wer\endcsname{64.82}
\expandafter\def\csname v@r/voxlock_live/dev4\endcsname{13.51}
\expandafter\def\csname v@r/voxlock_live/krisp/dele\endcsname{1.23}
\expandafter\def\csname v@r/voxlock_live/krisp/ins\endcsname{0.84}
\expandafter\def\csname v@r/voxlock_live/krisp/leak_wpm\endcsname{0.29}
\expandafter\def\csname v@r/voxlock_live/krisp/miss\endcsname{4.78}
\expandafter\def\csname v@r/voxlock_live/krisp/wer\endcsname{5.63}
\expandafter\def\csname v@r/voxlock_live/meet3\endcsname{17.32}
\expandafter\def\csname v@r/voxlock_live/nsf_dev/dele\endcsname{1.78}
\expandafter\def\csname v@r/voxlock_live/nsf_dev/ins\endcsname{2.12}
\expandafter\def\csname v@r/voxlock_live/nsf_dev/leak_wpm\endcsname{1.70}
\expandafter\def\csname v@r/voxlock_live/nsf_dev/miss\endcsname{6.06}
\expandafter\def\csname v@r/voxlock_live/nsf_dev/wer\endcsname{8.18}
\expandafter\def\csname v@r/voxlock_pt/aic_calls/dele\endcsname{3.17}
\expandafter\def\csname v@r/voxlock_pt/aic_calls/ins\endcsname{13.86}
\expandafter\def\csname v@r/voxlock_pt/aic_calls/leak_wpm\endcsname{18.23}
\expandafter\def\csname v@r/voxlock_pt/aic_calls/miss\endcsname{6.63}
\expandafter\def\csname v@r/voxlock_pt/aic_calls/wer\endcsname{20.49}
\expandafter\def\csname v@r/voxlock_pt/ami_dev/dele\endcsname{4.20}
\expandafter\def\csname v@r/voxlock_pt/ami_dev/ins\endcsname{4.33}
\expandafter\def\csname v@r/voxlock_pt/ami_dev/leak_wpm\endcsname{9.91}
\expandafter\def\csname v@r/voxlock_pt/ami_dev/miss\endcsname{10.02}
\expandafter\def\csname v@r/voxlock_pt/ami_dev/wer\endcsname{14.34}
\expandafter\def\csname v@r/voxlock_pt/ami_dev_long/dele\endcsname{14.23}
\expandafter\def\csname v@r/voxlock_pt/ami_dev_long/ins\endcsname{5.07}
\expandafter\def\csname v@r/voxlock_pt/ami_dev_long/leak_wpm\endcsname{9.44}
\expandafter\def\csname v@r/voxlock_pt/ami_dev_long/miss\endcsname{21.90}
\expandafter\def\csname v@r/voxlock_pt/ami_dev_long/wer\endcsname{26.97}
\expandafter\def\csname v@r/voxlock_pt/call_dev_clean/dele\endcsname{1.49}
\expandafter\def\csname v@r/voxlock_pt/call_dev_clean/ins\endcsname{0.04}
\expandafter\def\csname v@r/voxlock_pt/call_dev_clean/leak_wpm\endcsname{nan}
\expandafter\def\csname v@r/voxlock_pt/call_dev_clean/miss\endcsname{1.85}
\expandafter\def\csname v@r/voxlock_pt/call_dev_clean/wer\endcsname{1.89}
\expandafter\def\csname v@r/voxlock_pt/call_dev_mix/dele\endcsname{2.58}
\expandafter\def\csname v@r/voxlock_pt/call_dev_mix/ins\endcsname{42.29}
\expandafter\def\csname v@r/voxlock_pt/call_dev_mix/leak_wpm\endcsname{136.19}
\expandafter\def\csname v@r/voxlock_pt/call_dev_mix/miss\endcsname{17.85}
\expandafter\def\csname v@r/voxlock_pt/call_dev_mix/wer\endcsname{60.14}
\expandafter\def\csname v@r/voxlock_pt/dev4\endcsname{12.87}
\expandafter\def\csname v@r/voxlock_pt/krisp/dele\endcsname{0.94}
\expandafter\def\csname v@r/voxlock_pt/krisp/ins\endcsname{0.74}
\expandafter\def\csname v@r/voxlock_pt/krisp/leak_wpm\endcsname{0.09}
\expandafter\def\csname v@r/voxlock_pt/krisp/miss\endcsname{4.25}
\expandafter\def\csname v@r/voxlock_pt/krisp/wer\endcsname{4.99}
\expandafter\def\csname v@r/voxlock_pt/meet3\endcsname{16.53}
\expandafter\def\csname v@r/voxlock_pt/nsf_dev/dele\endcsname{2.08}
\expandafter\def\csname v@r/voxlock_pt/nsf_dev/ins\endcsname{1.92}
\expandafter\def\csname v@r/voxlock_pt/nsf_dev/leak_wpm\endcsname{0.64}
\expandafter\def\csname v@r/voxlock_pt/nsf_dev/miss\endcsname{6.36}
\expandafter\def\csname v@r/voxlock_pt/nsf_dev/wer\endcsname{8.28}
\expandafter\def\csname v@realbank/ali/channels\endcsname{581}
\expandafter\def\csname v@realbank/ali/hours\endcsname{309}
\expandafter\def\csname v@realbank/ali/meetings\endcsname{179}
\expandafter\def\csname v@realbank/all/hours\endcsname{620}
\expandafter\def\csname v@realbank/all/meetings\endcsname{362}
\expandafter\def\csname v@realbank/ami/channels\endcsname{443}
\expandafter\def\csname v@realbank/ami/hours\endcsname{271}
\expandafter\def\csname v@realbank/ami/meetings\endcsname{111}
\expandafter\def\csname v@realbank/nsf/channels\endcsname{390}
\expandafter\def\csname v@realbank/nsf/hours\endcsname{40}
\expandafter\def\csname v@realbank/nsf/meetings\endcsname{72}
\expandafter\def\csname v@serve/L/cap\endcsname{320}
\expandafter\def\csname v@serve/L/p99-1\endcsname{3.2}
\expandafter\def\csname v@serve/M/cap\endcsname{384}
\expandafter\def\csname v@serve/M/cap-c1\endcsname{224}
\expandafter\def\csname v@serve/M/cap-c2\endcsname{384}
\expandafter\def\csname v@serve/M/cap-c4\endcsname{512}
\expandafter\def\csname v@serve/M/p99-1\endcsname{3.2}
\expandafter\def\csname v@serve/MW/112/dense\endcsname{15.2}
\expandafter\def\csname v@serve/MW/112/gather\endcsname{15.2}
\expandafter\def\csname v@serve/MW/112/late\endcsname{15.3}
\expandafter\def\csname v@serve/MW/128/dense\endcsname{16.3}
\expandafter\def\csname v@serve/MW/128/gather\endcsname{16.2}
\expandafter\def\csname v@serve/MW/128/late\endcsname{16.3}
\expandafter\def\csname v@serve/MW/16/dense\endcsname{7.8}
\expandafter\def\csname v@serve/MW/16/gather\endcsname{7.9}
\expandafter\def\csname v@serve/MW/16/late\endcsname{7.8}
\expandafter\def\csname v@serve/MW/160/dense\endcsname{19.1}
\expandafter\def\csname v@serve/MW/160/gather\endcsname{19.0}
\expandafter\def\csname v@serve/MW/160/late\endcsname{19.1}
\expandafter\def\csname v@serve/MW/192/dense\endcsname{21.3}
\expandafter\def\csname v@serve/MW/192/gather\endcsname{21.2}
\expandafter\def\csname v@serve/MW/192/late\endcsname{21.4}
\expandafter\def\csname v@serve/MW/2/dense\endcsname{6.8}
\expandafter\def\csname v@serve/MW/2/gather\endcsname{6.7}
\expandafter\def\csname v@serve/MW/2/late\endcsname{6.8}
\expandafter\def\csname v@serve/MW/224/dense\endcsname{24.1}
\expandafter\def\csname v@serve/MW/224/gather\endcsname{23.2}
\expandafter\def\csname v@serve/MW/224/late\endcsname{24.1}
\expandafter\def\csname v@serve/MW/256/dense\endcsname{26.5}
\expandafter\def\csname v@serve/MW/256/gather\endcsname{26.4}
\expandafter\def\csname v@serve/MW/256/late\endcsname{26.6}
\expandafter\def\csname v@serve/MW/32/dense\endcsname{9.0}
\expandafter\def\csname v@serve/MW/32/gather\endcsname{9.0}
\expandafter\def\csname v@serve/MW/32/late\endcsname{9.0}
\expandafter\def\csname v@serve/MW/320/dense\endcsname{31.8}
\expandafter\def\csname v@serve/MW/320/gather\endcsname{31.7}
\expandafter\def\csname v@serve/MW/320/late\endcsname{31.9}
\expandafter\def\csname v@serve/MW/384/dense\endcsname{36.6}
\expandafter\def\csname v@serve/MW/384/gather\endcsname{36.5}
\expandafter\def\csname v@serve/MW/384/late\endcsname{36.7}
\expandafter\def\csname v@serve/MW/4/dense\endcsname{7.0}
\expandafter\def\csname v@serve/MW/4/gather\endcsname{7.1}
\expandafter\def\csname v@serve/MW/4/late\endcsname{7.0}
\expandafter\def\csname v@serve/MW/448/dense\endcsname{41.5}
\expandafter\def\csname v@serve/MW/448/gather\endcsname{41.4}
\expandafter\def\csname v@serve/MW/448/late\endcsname{41.7}
\expandafter\def\csname v@serve/MW/48/dense\endcsname{10.3}
\expandafter\def\csname v@serve/MW/48/gather\endcsname{10.3}
\expandafter\def\csname v@serve/MW/48/late\endcsname{10.4}
\expandafter\def\csname v@serve/MW/512/dense\endcsname{47.0}
\expandafter\def\csname v@serve/MW/512/gather\endcsname{46.8}
\expandafter\def\csname v@serve/MW/512/late\endcsname{47.1}
\expandafter\def\csname v@serve/MW/64/dense\endcsname{11.5}
\expandafter\def\csname v@serve/MW/64/gather\endcsname{11.5}
\expandafter\def\csname v@serve/MW/64/late\endcsname{11.6}
\expandafter\def\csname v@serve/MW/768/dense\endcsname{67.2}
\expandafter\def\csname v@serve/MW/768/gather\endcsname{65.7}
\expandafter\def\csname v@serve/MW/768/late\endcsname{66.2}
\expandafter\def\csname v@serve/MW/8/dense\endcsname{7.3}
\expandafter\def\csname v@serve/MW/8/gather\endcsname{7.3}
\expandafter\def\csname v@serve/MW/8/late\endcsname{7.3}
\expandafter\def\csname v@serve/MW/80/dense\endcsname{13.1}
\expandafter\def\csname v@serve/MW/80/gather\endcsname{13.0}
\expandafter\def\csname v@serve/MW/80/late\endcsname{13.1}
\expandafter\def\csname v@serve/MW/96/dense\endcsname{14.0}
\expandafter\def\csname v@serve/MW/96/gather\endcsname{13.9}
\expandafter\def\csname v@serve/MW/96/late\endcsname{14.0}
\expandafter\def\csname v@serve/MW/cap-c2\endcsname{160}
\expandafter\def\csname v@serve/MW/cap-c4\endcsname{256}
\expandafter\def\csname v@serve/MW/equiv-snr\endcsname{69}
\expandafter\def\csname v@serve/MW/equiv-snr-prime\endcsname{70}
\expandafter\def\csname v@serve/S/cap\endcsname{512}
\expandafter\def\csname v@serve/S/p99-1\endcsname{3.0}
\expandafter\def\csname v@serve/drain/mpM/1/p50\endcsname{18}
\expandafter\def\csname v@serve/drain/mpM/1/p99\endcsname{19}
\expandafter\def\csname v@serve/drain/mpM/1/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpM/1/sp50\endcsname{18}
\expandafter\def\csname v@serve/drain/mpM/1/sp99\endcsname{19}
\expandafter\def\csname v@serve/drain/mpM/112/p50\endcsname{29}
\expandafter\def\csname v@serve/drain/mpM/112/p99\endcsname{40}
\expandafter\def\csname v@serve/drain/mpM/112/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpM/112/sp50\endcsname{29}
\expandafter\def\csname v@serve/drain/mpM/112/sp99\endcsname{39}
\expandafter\def\csname v@serve/drain/mpM/32/p50\endcsname{13}
\expandafter\def\csname v@serve/drain/mpM/32/p99\endcsname{20}
\expandafter\def\csname v@serve/drain/mpM/32/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpM/32/sp50\endcsname{13}
\expandafter\def\csname v@serve/drain/mpM/32/sp99\endcsname{20}
\expandafter\def\csname v@serve/drain/mpM/64/p50\endcsname{18}
\expandafter\def\csname v@serve/drain/mpM/64/p99\endcsname{27}
\expandafter\def\csname v@serve/drain/mpM/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpM/64/sp50\endcsname{18}
\expandafter\def\csname v@serve/drain/mpM/64/sp99\endcsname{26}
\expandafter\def\csname v@serve/drain/mpM/80/p50\endcsname{23}
\expandafter\def\csname v@serve/drain/mpM/80/p99\endcsname{32}
\expandafter\def\csname v@serve/drain/mpM/80/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpM/80/sp50\endcsname{23}
\expandafter\def\csname v@serve/drain/mpM/80/sp99\endcsname{32}
\expandafter\def\csname v@serve/drain/mpM/96/p50\endcsname{26}
\expandafter\def\csname v@serve/drain/mpM/96/p99\endcsname{37}
\expandafter\def\csname v@serve/drain/mpM/96/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpM/96/sp50\endcsname{26}
\expandafter\def\csname v@serve/drain/mpM/96/sp99\endcsname{37}
\expandafter\def\csname v@serve/drain/mpM/behind\endcsname{128}
\expandafter\def\csname v@serve/drain/mpM/hold\endcsname{112}
\expandafter\def\csname v@serve/drain/mpM/hold-sp50\endcsname{29}
\expandafter\def\csname v@serve/drain/mpM/hold-sp99\endcsname{39}
\expandafter\def\csname v@serve/drain/mpM/tested\endcsname{160}
\expandafter\def\csname v@serve/drain/mpMW/1/p50\endcsname{21}
\expandafter\def\csname v@serve/drain/mpMW/1/p99\endcsname{26}
\expandafter\def\csname v@serve/drain/mpMW/1/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMW/1/sp50\endcsname{21}
\expandafter\def\csname v@serve/drain/mpMW/1/sp99\endcsname{26}
\expandafter\def\csname v@serve/drain/mpMW/32/p50\endcsname{20}
\expandafter\def\csname v@serve/drain/mpMW/32/p99\endcsname{29}
\expandafter\def\csname v@serve/drain/mpMW/32/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMW/32/sp50\endcsname{20}
\expandafter\def\csname v@serve/drain/mpMW/32/sp99\endcsname{29}
\expandafter\def\csname v@serve/drain/mpMW/48/p50\endcsname{24}
\expandafter\def\csname v@serve/drain/mpMW/48/p99\endcsname{35}
\expandafter\def\csname v@serve/drain/mpMW/48/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMW/48/sp50\endcsname{24}
\expandafter\def\csname v@serve/drain/mpMW/48/sp99\endcsname{35}
\expandafter\def\csname v@serve/drain/mpMW/64/p50\endcsname{29}
\expandafter\def\csname v@serve/drain/mpMW/64/p99\endcsname{39}
\expandafter\def\csname v@serve/drain/mpMW/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMW/64/sp50\endcsname{29}
\expandafter\def\csname v@serve/drain/mpMW/64/sp99\endcsname{39}
\expandafter\def\csname v@serve/drain/mpMW/behind\endcsname{80}
\expandafter\def\csname v@serve/drain/mpMW/hold\endcsname{64}
\expandafter\def\csname v@serve/drain/mpMW/hold-sp50\endcsname{29}
\expandafter\def\csname v@serve/drain/mpMW/hold-sp99\endcsname{39}
\expandafter\def\csname v@serve/drain/mpMW/tested\endcsname{96}
\expandafter\def\csname v@serve/drain/mpMW40/112/p50\endcsname{56}
\expandafter\def\csname v@serve/drain/mpMW40/112/p99\endcsname{76}
\expandafter\def\csname v@serve/drain/mpMW40/112/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMW40/112/sp50\endcsname{56}
\expandafter\def\csname v@serve/drain/mpMW40/112/sp99\endcsname{76}
\expandafter\def\csname v@serve/drain/mpMW40/64/p50\endcsname{33}
\expandafter\def\csname v@serve/drain/mpMW40/64/p99\endcsname{48}
\expandafter\def\csname v@serve/drain/mpMW40/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMW40/64/sp50\endcsname{33}
\expandafter\def\csname v@serve/drain/mpMW40/64/sp99\endcsname{48}
\expandafter\def\csname v@serve/drain/mpMW40/96/p50\endcsname{50}
\expandafter\def\csname v@serve/drain/mpMW40/96/p99\endcsname{68}
\expandafter\def\csname v@serve/drain/mpMW40/96/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMW40/96/sp50\endcsname{50}
\expandafter\def\csname v@serve/drain/mpMW40/96/sp99\endcsname{68}
\expandafter\def\csname v@serve/drain/mpMW40/behind\endcsname{128}
\expandafter\def\csname v@serve/drain/mpMW40/hold\endcsname{112}
\expandafter\def\csname v@serve/drain/mpMW40/hold-sp50\endcsname{56}
\expandafter\def\csname v@serve/drain/mpMW40/hold-sp99\endcsname{76}
\expandafter\def\csname v@serve/drain/mpMW40/tested\endcsname{160}
\expandafter\def\csname v@serve/drain/mpMWg0/32/p50\endcsname{21}
\expandafter\def\csname v@serve/drain/mpMWg0/32/p99\endcsname{28}
\expandafter\def\csname v@serve/drain/mpMWg0/32/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMWg0/32/sp50\endcsname{21}
\expandafter\def\csname v@serve/drain/mpMWg0/32/sp99\endcsname{27}
\expandafter\def\csname v@serve/drain/mpMWg0/48/p50\endcsname{24}
\expandafter\def\csname v@serve/drain/mpMWg0/48/p99\endcsname{32}
\expandafter\def\csname v@serve/drain/mpMWg0/48/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMWg0/48/sp50\endcsname{24}
\expandafter\def\csname v@serve/drain/mpMWg0/48/sp99\endcsname{32}
\expandafter\def\csname v@serve/drain/mpMWg0/64/p50\endcsname{29}
\expandafter\def\csname v@serve/drain/mpMWg0/64/p99\endcsname{39}
\expandafter\def\csname v@serve/drain/mpMWg0/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/drain/mpMWg0/64/sp50\endcsname{29}
\expandafter\def\csname v@serve/drain/mpMWg0/64/sp99\endcsname{38}
\expandafter\def\csname v@serve/drain/mpMWg0/hold\endcsname{64}
\expandafter\def\csname v@serve/drain/mpMWg0/hold-sp50\endcsname{29}
\expandafter\def\csname v@serve/drain/mpMWg0/hold-sp99\endcsname{38}
\expandafter\def\csname v@serve/drain/mpMWg0/tested\endcsname{64}
\expandafter\def\csname v@serve/drain/start/final/p50-after30\endcsname{29}
\expandafter\def\csname v@serve/drain/start/final/p99-30s\endcsname{40}
\expandafter\def\csname v@serve/drain/start/final/runs\endcsname{3}
\expandafter\def\csname v@serve/drain/start/graph/p50-after30\endcsname{30}
\expandafter\def\csname v@serve/drain/start/graph/p99-30s\endcsname{297}
\expandafter\def\csname v@serve/drain/start/graph/runs\endcsname{3}
\expandafter\def\csname v@serve/drain/start/noenroll/p50-after30\endcsname{31}
\expandafter\def\csname v@serve/drain/start/noenroll/p99-30s\endcsname{41}
\expandafter\def\csname v@serve/drain/start/noenroll/runs\endcsname{2}
\expandafter\def\csname v@serve/drain/start/warmup/p50-after30\endcsname{261}
\expandafter\def\csname v@serve/drain/start/warmup/p99-30s\endcsname{712}
\expandafter\def\csname v@serve/drain/start/warmup/runs\endcsname{2}
\expandafter\def\csname v@serve/equiv-snr\endcsname{70}
\expandafter\def\csname v@serve/equiv-snr-fp32\endcsname{94}
\expandafter\def\csname v@serve/mpM/1/p50\endcsname{6}
\expandafter\def\csname v@serve/mpM/1/p99\endcsname{7}
\expandafter\def\csname v@serve/mpM/1/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/1/sp50\endcsname{6}
\expandafter\def\csname v@serve/mpM/1/sp99\endcsname{7}
\expandafter\def\csname v@serve/mpM/112/p50\endcsname{9}
\expandafter\def\csname v@serve/mpM/112/p99\endcsname{18}
\expandafter\def\csname v@serve/mpM/112/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/112/sp50\endcsname{9}
\expandafter\def\csname v@serve/mpM/112/sp99\endcsname{17}
\expandafter\def\csname v@serve/mpM/128/p50\endcsname{12}
\expandafter\def\csname v@serve/mpM/128/p99\endcsname{21}
\expandafter\def\csname v@serve/mpM/128/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/128/sp50\endcsname{12}
\expandafter\def\csname v@serve/mpM/128/sp99\endcsname{21}
\expandafter\def\csname v@serve/mpM/160/p50\endcsname{22}
\expandafter\def\csname v@serve/mpM/160/p99\endcsname{33}
\expandafter\def\csname v@serve/mpM/160/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/160/sp50\endcsname{23}
\expandafter\def\csname v@serve/mpM/160/sp99\endcsname{33}
\expandafter\def\csname v@serve/mpM/192/p50\endcsname{22}
\expandafter\def\csname v@serve/mpM/192/p99\endcsname{34}
\expandafter\def\csname v@serve/mpM/192/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/192/sp50\endcsname{22}
\expandafter\def\csname v@serve/mpM/192/sp99\endcsname{33}
\expandafter\def\csname v@serve/mpM/256/p50\endcsname{28}
\expandafter\def\csname v@serve/mpM/256/p99\endcsname{38}
\expandafter\def\csname v@serve/mpM/256/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/256/sp50\endcsname{28}
\expandafter\def\csname v@serve/mpM/256/sp99\endcsname{38}
\expandafter\def\csname v@serve/mpM/32/p50\endcsname{6}
\expandafter\def\csname v@serve/mpM/32/p99\endcsname{14}
\expandafter\def\csname v@serve/mpM/32/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/32/sp50\endcsname{6}
\expandafter\def\csname v@serve/mpM/32/sp99\endcsname{14}
\expandafter\def\csname v@serve/mpM/64/p50\endcsname{7}
\expandafter\def\csname v@serve/mpM/64/p99\endcsname{14}
\expandafter\def\csname v@serve/mpM/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/64/sp50\endcsname{7}
\expandafter\def\csname v@serve/mpM/64/sp99\endcsname{14}
\expandafter\def\csname v@serve/mpM/80/p50\endcsname{8}
\expandafter\def\csname v@serve/mpM/80/p99\endcsname{16}
\expandafter\def\csname v@serve/mpM/80/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/80/sp50\endcsname{8}
\expandafter\def\csname v@serve/mpM/80/sp99\endcsname{16}
\expandafter\def\csname v@serve/mpM/96/p50\endcsname{9}
\expandafter\def\csname v@serve/mpM/96/p99\endcsname{16}
\expandafter\def\csname v@serve/mpM/96/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpM/96/sp50\endcsname{8}
\expandafter\def\csname v@serve/mpM/96/sp99\endcsname{16}
\expandafter\def\csname v@serve/mpM/hold\endcsname{256}
\expandafter\def\csname v@serve/mpM/hold-sp50\endcsname{28}
\expandafter\def\csname v@serve/mpM/hold-sp99\endcsname{38}
\expandafter\def\csname v@serve/mpM/tested\endcsname{256}
\expandafter\def\csname v@serve/mpMW/1/p50\endcsname{18}
\expandafter\def\csname v@serve/mpMW/1/p99\endcsname{19}
\expandafter\def\csname v@serve/mpMW/1/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW/1/sp50\endcsname{17}
\expandafter\def\csname v@serve/mpMW/1/sp99\endcsname{19}
\expandafter\def\csname v@serve/mpMW/112/p50\endcsname{28}
\expandafter\def\csname v@serve/mpMW/112/p99\endcsname{37}
\expandafter\def\csname v@serve/mpMW/112/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW/112/sp50\endcsname{28}
\expandafter\def\csname v@serve/mpMW/112/sp99\endcsname{37}
\expandafter\def\csname v@serve/mpMW/128/p50\endcsname{27}
\expandafter\def\csname v@serve/mpMW/128/p99\endcsname{39}
\expandafter\def\csname v@serve/mpMW/128/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW/128/sp50\endcsname{27}
\expandafter\def\csname v@serve/mpMW/128/sp99\endcsname{38}
\expandafter\def\csname v@serve/mpMW/160/p50\endcsname{369}
\expandafter\def\csname v@serve/mpMW/160/p99\endcsname{457}
\expandafter\def\csname v@serve/mpMW/160/sover\endcsname{100.00}
\expandafter\def\csname v@serve/mpMW/160/sp50\endcsname{400}
\expandafter\def\csname v@serve/mpMW/160/sp99\endcsname{459}
\expandafter\def\csname v@serve/mpMW/32/p50\endcsname{16}
\expandafter\def\csname v@serve/mpMW/32/p99\endcsname{30}
\expandafter\def\csname v@serve/mpMW/32/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW/32/sp50\endcsname{16}
\expandafter\def\csname v@serve/mpMW/32/sp99\endcsname{29}
\expandafter\def\csname v@serve/mpMW/48/p50\endcsname{26}
\expandafter\def\csname v@serve/mpMW/48/p99\endcsname{36}
\expandafter\def\csname v@serve/mpMW/48/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW/48/sp50\endcsname{26}
\expandafter\def\csname v@serve/mpMW/48/sp99\endcsname{36}
\expandafter\def\csname v@serve/mpMW/64/p50\endcsname{24}
\expandafter\def\csname v@serve/mpMW/64/p99\endcsname{31}
\expandafter\def\csname v@serve/mpMW/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW/64/sp50\endcsname{24}
\expandafter\def\csname v@serve/mpMW/64/sp99\endcsname{31}
\expandafter\def\csname v@serve/mpMW/80/p50\endcsname{25}
\expandafter\def\csname v@serve/mpMW/80/p99\endcsname{35}
\expandafter\def\csname v@serve/mpMW/80/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW/80/sp50\endcsname{25}
\expandafter\def\csname v@serve/mpMW/80/sp99\endcsname{35}
\expandafter\def\csname v@serve/mpMW/96/p50\endcsname{25}
\expandafter\def\csname v@serve/mpMW/96/p99\endcsname{36}
\expandafter\def\csname v@serve/mpMW/96/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW/96/sp50\endcsname{25}
\expandafter\def\csname v@serve/mpMW/96/sp99\endcsname{36}
\expandafter\def\csname v@serve/mpMW/behind\endcsname{160}
\expandafter\def\csname v@serve/mpMW/hold\endcsname{128}
\expandafter\def\csname v@serve/mpMW/hold-sp50\endcsname{27}
\expandafter\def\csname v@serve/mpMW/hold-sp99\endcsname{38}
\expandafter\def\csname v@serve/mpMW/tested\endcsname{160}
\expandafter\def\csname v@serve/mpMW40/112/p50\endcsname{25}
\expandafter\def\csname v@serve/mpMW40/112/p99\endcsname{40}
\expandafter\def\csname v@serve/mpMW40/112/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW40/112/sp50\endcsname{25}
\expandafter\def\csname v@serve/mpMW40/112/sp99\endcsname{40}
\expandafter\def\csname v@serve/mpMW40/128/p50\endcsname{25}
\expandafter\def\csname v@serve/mpMW40/128/p99\endcsname{42}
\expandafter\def\csname v@serve/mpMW40/128/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW40/128/sp50\endcsname{24}
\expandafter\def\csname v@serve/mpMW40/128/sp99\endcsname{42}
\expandafter\def\csname v@serve/mpMW40/160/p50\endcsname{48}
\expandafter\def\csname v@serve/mpMW40/160/p99\endcsname{68}
\expandafter\def\csname v@serve/mpMW40/160/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW40/160/sp50\endcsname{49}
\expandafter\def\csname v@serve/mpMW40/160/sp99\endcsname{68}
\expandafter\def\csname v@serve/mpMW40/192/p50\endcsname{51}
\expandafter\def\csname v@serve/mpMW40/192/p99\endcsname{72}
\expandafter\def\csname v@serve/mpMW40/192/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW40/192/sp50\endcsname{51}
\expandafter\def\csname v@serve/mpMW40/192/sp99\endcsname{72}
\expandafter\def\csname v@serve/mpMW40/224/p50\endcsname{59}
\expandafter\def\csname v@serve/mpMW40/224/p99\endcsname{77}
\expandafter\def\csname v@serve/mpMW40/224/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW40/224/sp50\endcsname{59}
\expandafter\def\csname v@serve/mpMW40/224/sp99\endcsname{77}
\expandafter\def\csname v@serve/mpMW40/256/p50\endcsname{64}
\expandafter\def\csname v@serve/mpMW40/256/p99\endcsname{86}
\expandafter\def\csname v@serve/mpMW40/256/sover\endcsname{0.01}
\expandafter\def\csname v@serve/mpMW40/256/sp50\endcsname{63}
\expandafter\def\csname v@serve/mpMW40/256/sp99\endcsname{84}
\expandafter\def\csname v@serve/mpMW40/64/p50\endcsname{16}
\expandafter\def\csname v@serve/mpMW40/64/p99\endcsname{31}
\expandafter\def\csname v@serve/mpMW40/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW40/64/sp50\endcsname{16}
\expandafter\def\csname v@serve/mpMW40/64/sp99\endcsname{31}
\expandafter\def\csname v@serve/mpMW40/96/p50\endcsname{18}
\expandafter\def\csname v@serve/mpMW40/96/p99\endcsname{31}
\expandafter\def\csname v@serve/mpMW40/96/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMW40/96/sp50\endcsname{18}
\expandafter\def\csname v@serve/mpMW40/96/sp99\endcsname{31}
\expandafter\def\csname v@serve/mpMW40/behind\endcsname{256}
\expandafter\def\csname v@serve/mpMW40/hold\endcsname{224}
\expandafter\def\csname v@serve/mpMW40/hold-sp50\endcsname{59}
\expandafter\def\csname v@serve/mpMW40/hold-sp99\endcsname{77}
\expandafter\def\csname v@serve/mpMW40/tested\endcsname{256}
\expandafter\def\csname v@serve/mpMWg0/32/p50\endcsname{12}
\expandafter\def\csname v@serve/mpMWg0/32/p99\endcsname{25}
\expandafter\def\csname v@serve/mpMWg0/32/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMWg0/32/sp50\endcsname{12}
\expandafter\def\csname v@serve/mpMWg0/32/sp99\endcsname{26}
\expandafter\def\csname v@serve/mpMWg0/48/p50\endcsname{15}
\expandafter\def\csname v@serve/mpMWg0/48/p99\endcsname{21}
\expandafter\def\csname v@serve/mpMWg0/48/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMWg0/48/sp50\endcsname{15}
\expandafter\def\csname v@serve/mpMWg0/48/sp99\endcsname{21}
\expandafter\def\csname v@serve/mpMWg0/64/p50\endcsname{25}
\expandafter\def\csname v@serve/mpMWg0/64/p99\endcsname{33}
\expandafter\def\csname v@serve/mpMWg0/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/mpMWg0/64/sp50\endcsname{25}
\expandafter\def\csname v@serve/mpMWg0/64/sp99\endcsname{33}
\expandafter\def\csname v@serve/mpMWg0/hold\endcsname{64}
\expandafter\def\csname v@serve/mpMWg0/hold-sp50\endcsname{25}
\expandafter\def\csname v@serve/mpMWg0/hold-sp99\endcsname{33}
\expandafter\def\csname v@serve/mpMWg0/tested\endcsname{64}
\expandafter\def\csname v@serve/soakMW/calls\endcsname{64}
\expandafter\def\csname v@serve/soakMW/chunks-m\endcsname{5.76}
\expandafter\def\csname v@serve/soakMW/errors\endcsname{0}
\expandafter\def\csname v@serve/soakMW/gpu-pct\endcsname{44}
\expandafter\def\csname v@serve/soakMW/gpu_mb-first\endcsname{63,091}
\expandafter\def\csname v@serve/soakMW/gpu_mb-last\endcsname{63,091}
\expandafter\def\csname v@serve/soakMW/max\endcsname{74}
\expandafter\def\csname v@serve/soakMW/minutes\endcsname{30}
\expandafter\def\csname v@serve/soakMW/p50\endcsname{20}
\expandafter\def\csname v@serve/soakMW/p99\endcsname{32}
\expandafter\def\csname v@serve/soakMW/p99-first\endcsname{33}
\expandafter\def\csname v@serve/soakMW/p99-hi\endcsname{33}
\expandafter\def\csname v@serve/soakMW/p99-lo\endcsname{32}
\expandafter\def\csname v@serve/soakMW/rss-grow-pct\endcsname{1.7}
\expandafter\def\csname v@serve/soakMW/rss_mb-first\endcsname{2,957}
\expandafter\def\csname v@serve/soakMW/rss_mb-last\endcsname{3,008}
\expandafter\def\csname v@serve/soakMW/workers_rss_mb-first\endcsname{433}
\expandafter\def\csname v@serve/soakMW/workers_rss_mb-last\endcsname{446}
\expandafter\def\csname v@serve/soakMWcold/calls\endcsname{64}
\expandafter\def\csname v@serve/soakMWcold/chunks-m\endcsname{5.76}
\expandafter\def\csname v@serve/soakMWcold/errors\endcsname{0}
\expandafter\def\csname v@serve/soakMWcold/gpu-pct\endcsname{50}
\expandafter\def\csname v@serve/soakMWcold/gpu_mb-first\endcsname{71,591}
\expandafter\def\csname v@serve/soakMWcold/gpu_mb-last\endcsname{71,597}
\expandafter\def\csname v@serve/soakMWcold/max\endcsname{921}
\expandafter\def\csname v@serve/soakMWcold/minutes\endcsname{30}
\expandafter\def\csname v@serve/soakMWcold/p50\endcsname{29}
\expandafter\def\csname v@serve/soakMWcold/p99\endcsname{640}
\expandafter\def\csname v@serve/soakMWcold/p99-first\endcsname{900}
\expandafter\def\csname v@serve/soakMWcold/p99-hi\endcsname{40}
\expandafter\def\csname v@serve/soakMWcold/p99-lo\endcsname{39}
\expandafter\def\csname v@serve/soakMWcold/rss-grow-pct\endcsname{9.3}
\expandafter\def\csname v@serve/soakMWcold/rss_mb-first\endcsname{2,946}
\expandafter\def\csname v@serve/soakMWcold/rss_mb-last\endcsname{3,221}
\expandafter\def\csname v@serve/soakMWcold/workers_rss_mb-first\endcsname{417}
\expandafter\def\csname v@serve/soakMWcold/workers_rss_mb-last\endcsname{448}
\expandafter\def\csname v@serve/soakMWw/calls\endcsname{64}
\expandafter\def\csname v@serve/soakMWw/chunks-m\endcsname{0.38}
\expandafter\def\csname v@serve/soakMWw/errors\endcsname{0}
\expandafter\def\csname v@serve/soakMWw/gpu-pct\endcsname{52}
\expandafter\def\csname v@serve/soakMWw/gpu_mb-first\endcsname{74,973}
\expandafter\def\csname v@serve/soakMWw/gpu_mb-last\endcsname{74,973}
\expandafter\def\csname v@serve/soakMWw/max\endcsname{233}
\expandafter\def\csname v@serve/soakMWw/minutes\endcsname{2}
\expandafter\def\csname v@serve/soakMWw/p50\endcsname{31}
\expandafter\def\csname v@serve/soakMWw/p99\endcsname{221}
\expandafter\def\csname v@serve/soakMWw/p99-first\endcsname{225}
\expandafter\def\csname v@serve/soakMWw/p99-hi\endcsname{39}
\expandafter\def\csname v@serve/soakMWw/p99-lo\endcsname{39}
\expandafter\def\csname v@serve/soakMWw/rss-grow-pct\endcsname{4.0}
\expandafter\def\csname v@serve/soakMWw/rss_mb-first\endcsname{3,088}
\expandafter\def\csname v@serve/soakMWw/rss_mb-last\endcsname{3,210}
\expandafter\def\csname v@serve/soakMWw/workers_rss_mb-first\endcsname{417}
\expandafter\def\csname v@serve/soakMWw/workers_rss_mb-last\endcsname{446}
\expandafter\def\csname v@serve/soakMWwarm/calls\endcsname{64}
\expandafter\def\csname v@serve/soakMWwarm/chunks-m\endcsname{5.76}
\expandafter\def\csname v@serve/soakMWwarm/errors\endcsname{0}
\expandafter\def\csname v@serve/soakMWwarm/gpu-pct\endcsname{52}
\expandafter\def\csname v@serve/soakMWwarm/gpu_mb-first\endcsname{74,973}
\expandafter\def\csname v@serve/soakMWwarm/gpu_mb-last\endcsname{74,973}
\expandafter\def\csname v@serve/soakMWwarm/max\endcsname{674}
\expandafter\def\csname v@serve/soakMWwarm/minutes\endcsname{30}
\expandafter\def\csname v@serve/soakMWwarm/p50\endcsname{29}
\expandafter\def\csname v@serve/soakMWwarm/p99\endcsname{427}
\expandafter\def\csname v@serve/soakMWwarm/p99-first\endcsname{657}
\expandafter\def\csname v@serve/soakMWwarm/p99-hi\endcsname{39}
\expandafter\def\csname v@serve/soakMWwarm/p99-lo\endcsname{39}
\expandafter\def\csname v@serve/soakMWwarm/rss-grow-pct\endcsname{1.7}
\expandafter\def\csname v@serve/soakMWwarm/rss_mb-first\endcsname{3,171}
\expandafter\def\csname v@serve/soakMWwarm/rss_mb-last\endcsname{3,226}
\expandafter\def\csname v@serve/soakMWwarm/workers_rss_mb-first\endcsname{433}
\expandafter\def\csname v@serve/soakMWwarm/workers_rss_mb-last\endcsname{446}
\expandafter\def\csname v@serve/start/final/p50-after30\endcsname{26}
\expandafter\def\csname v@serve/start/final/p99-30s\endcsname{34}
\expandafter\def\csname v@serve/start/final/runs\endcsname{3}
\expandafter\def\csname v@serve/start/graph/p50-after30\endcsname{30}
\expandafter\def\csname v@serve/start/graph/p99-30s\endcsname{297}
\expandafter\def\csname v@serve/start/graph/runs\endcsname{3}
\expandafter\def\csname v@serve/start/noenroll/p50-after30\endcsname{31}
\expandafter\def\csname v@serve/start/noenroll/p99-30s\endcsname{41}
\expandafter\def\csname v@serve/start/noenroll/runs\endcsname{2}
\expandafter\def\csname v@serve/start/warmup/p50-after30\endcsname{261}
\expandafter\def\csname v@serve/start/warmup/p99-30s\endcsname{712}
\expandafter\def\csname v@serve/start/warmup/runs\endcsname{2}
\expandafter\def\csname v@serve/ws/1/p50\endcsname{20}
\expandafter\def\csname v@serve/ws/1/p99\endcsname{21}
\expandafter\def\csname v@serve/ws/1/sover\endcsname{0.00}
\expandafter\def\csname v@serve/ws/1/sp50\endcsname{20}
\expandafter\def\csname v@serve/ws/1/sp99\endcsname{21}
\expandafter\def\csname v@serve/ws/128/p50\endcsname{1028}
\expandafter\def\csname v@serve/ws/128/p99\endcsname{2477}
\expandafter\def\csname v@serve/ws/128/sover\endcsname{59.90}
\expandafter\def\csname v@serve/ws/128/sp50\endcsname{1202}
\expandafter\def\csname v@serve/ws/128/sp99\endcsname{2479}
\expandafter\def\csname v@serve/ws/16/p50\endcsname{18}
\expandafter\def\csname v@serve/ws/16/p99\endcsname{27}
\expandafter\def\csname v@serve/ws/16/sover\endcsname{0.00}
\expandafter\def\csname v@serve/ws/16/sp50\endcsname{18}
\expandafter\def\csname v@serve/ws/16/sp99\endcsname{27}
\expandafter\def\csname v@serve/ws/32/p50\endcsname{25}
\expandafter\def\csname v@serve/ws/32/p99\endcsname{38}
\expandafter\def\csname v@serve/ws/32/sover\endcsname{0.00}
\expandafter\def\csname v@serve/ws/32/sp50\endcsname{26}
\expandafter\def\csname v@serve/ws/32/sp99\endcsname{38}
\expandafter\def\csname v@serve/ws/64/p50\endcsname{18}
\expandafter\def\csname v@serve/ws/64/p99\endcsname{30}
\expandafter\def\csname v@serve/ws/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/ws/64/sp50\endcsname{18}
\expandafter\def\csname v@serve/ws/64/sp99\endcsname{29}
\expandafter\def\csname v@serve/ws/80/p50\endcsname{30}
\expandafter\def\csname v@serve/ws/80/p99\endcsname{43}
\expandafter\def\csname v@serve/ws/80/sover\endcsname{0.00}
\expandafter\def\csname v@serve/ws/80/sp50\endcsname{30}
\expandafter\def\csname v@serve/ws/80/sp99\endcsname{43}
\expandafter\def\csname v@serve/ws/96/p50\endcsname{21}
\expandafter\def\csname v@serve/ws/96/p99\endcsname{35}
\expandafter\def\csname v@serve/ws/96/sover\endcsname{0.00}
\expandafter\def\csname v@serve/ws/96/sp50\endcsname{20}
\expandafter\def\csname v@serve/ws/96/sp99\endcsname{35}
\expandafter\def\csname v@serve/ws/behind\endcsname{128}
\expandafter\def\csname v@serve/ws/hold\endcsname{96}
\expandafter\def\csname v@serve/ws/hold-sp50\endcsname{20}
\expandafter\def\csname v@serve/ws/hold-sp99\endcsname{35}
\expandafter\def\csname v@serve/ws/tested\endcsname{128}
\expandafter\def\csname v@serve/wsMW/1/p50\endcsname{18}
\expandafter\def\csname v@serve/wsMW/1/p99\endcsname{19}
\expandafter\def\csname v@serve/wsMW/1/sover\endcsname{0.00}
\expandafter\def\csname v@serve/wsMW/1/sp50\endcsname{18}
\expandafter\def\csname v@serve/wsMW/1/sp99\endcsname{19}
\expandafter\def\csname v@serve/wsMW/16/p50\endcsname{20}
\expandafter\def\csname v@serve/wsMW/16/p99\endcsname{30}
\expandafter\def\csname v@serve/wsMW/16/sover\endcsname{0.00}
\expandafter\def\csname v@serve/wsMW/16/sp50\endcsname{20}
\expandafter\def\csname v@serve/wsMW/16/sp99\endcsname{30}
\expandafter\def\csname v@serve/wsMW/32/p50\endcsname{21}
\expandafter\def\csname v@serve/wsMW/32/p99\endcsname{33}
\expandafter\def\csname v@serve/wsMW/32/sover\endcsname{0.00}
\expandafter\def\csname v@serve/wsMW/32/sp50\endcsname{21}
\expandafter\def\csname v@serve/wsMW/32/sp99\endcsname{33}
\expandafter\def\csname v@serve/wsMW/48/p50\endcsname{134}
\expandafter\def\csname v@serve/wsMW/48/p99\endcsname{558}
\expandafter\def\csname v@serve/wsMW/48/sover\endcsname{46.38}
\expandafter\def\csname v@serve/wsMW/48/sp50\endcsname{41}
\expandafter\def\csname v@serve/wsMW/48/sp99\endcsname{560}
\expandafter\def\csname v@serve/wsMW/64/p50\endcsname{30}
\expandafter\def\csname v@serve/wsMW/64/p99\endcsname{40}
\expandafter\def\csname v@serve/wsMW/64/sover\endcsname{0.00}
\expandafter\def\csname v@serve/wsMW/64/sp50\endcsname{31}
\expandafter\def\csname v@serve/wsMW/64/sp99\endcsname{40}
\expandafter\def\csname v@serve/wsMW/80/p50\endcsname{890}
\expandafter\def\csname v@serve/wsMW/80/p99\endcsname{1925}
\expandafter\def\csname v@serve/wsMW/80/sover\endcsname{71.99}
\expandafter\def\csname v@serve/wsMW/80/sp50\endcsname{1330}
\expandafter\def\csname v@serve/wsMW/80/sp99\endcsname{1926}
\expandafter\def\csname v@serve/wsMW/96/p50\endcsname{5142}
\expandafter\def\csname v@serve/wsMW/96/p99\endcsname{5766}
\expandafter\def\csname v@serve/wsMW/96/sover\endcsname{100.00}
\expandafter\def\csname v@serve/wsMW/96/sp50\endcsname{5189}
\expandafter\def\csname v@serve/wsMW/96/sp99\endcsname{5767}
\expandafter\def\csname v@serve/wsMW/behind\endcsname{48}
\expandafter\def\csname v@serve/wsMW/hold\endcsname{32}
\expandafter\def\csname v@serve/wsMW/hold-sp50\endcsname{21}
\expandafter\def\csname v@serve/wsMW/hold-sp99\endcsname{33}
\expandafter\def\csname v@serve/wsMW/tested\endcsname{96}
\expandafter\def\csname v@sidon/188m/dec_params\endcsname{187}
\expandafter\def\csname v@sidon/188m/fe_params\endcsname{580}
\expandafter\def\csname v@sidon/188m/params\endcsname{768}
\expandafter\def\csname v@sidon/lite/dec_params\endcsname{52}
\expandafter\def\csname v@sidon/lite/fe_params\endcsname{37}
\expandafter\def\csname v@sidon/lite/params\endcsname{89}
\expandafter\def\csname v@small/C10/cap-c2\endcsname{2,048}
\expandafter\def\csname v@small/C10/cap-c4\endcsname{3,072}
\expandafter\def\csname v@small/C10/params-m\endcsname{10}
\expandafter\def\csname v@small/C22/cap-c2\endcsname{1,536}
\expandafter\def\csname v@small/C22/cap-c4\endcsname{2,048}
\expandafter\def\csname v@small/C22/params-m\endcsname{22}
\expandafter\def\csname v@small/C36/cap-c2\endcsname{1,024}
\expandafter\def\csname v@small/C36/cap-c4\endcsname{1,536}
\expandafter\def\csname v@small/C36/params-m\endcsname{36}
\expandafter\def\csname v@small/C51/cap-c2\endcsname{1,024}
\expandafter\def\csname v@small/C51/cap-c4\endcsname{1,536}
\expandafter\def\csname v@small/C51/params-m\endcsname{51}
\expandafter\def\csname v@small/M/cap-c2\endcsname{384}
\expandafter\def\csname v@small/M/cap-c4\endcsname{512}
\expandafter\def\csname v@small/M/params-m\endcsname{243}
\expandafter\def\csname v@small/S/cap-c2\endcsname{512}
\expandafter\def\csname v@small/S/cap-c4\endcsname{768}
\expandafter\def\csname v@small/S/params-m\endcsname{140}
\expandafter\def\csname v@small/agent/gate\endcsname{0.9:30:0.2:1}
\expandafter\def\csname v@small/agent/server/default/differ\endcsname{0}
\expandafter\def\csname v@small/agent/server/default/snr-min\endcsname{50}
\expandafter\def\csname v@small/agent/server/voicebot/differ\endcsname{1}
\expandafter\def\csname v@small/agent/server/voicebot/snr-min\endcsname{45}
\expandafter\def\csname v@small/boot/ami_dev_long/diff\endcsname{+1.23}
\expandafter\def\csname v@small/boot/ami_dev_long/hi\endcsname{+2.52}
\expandafter\def\csname v@small/boot/ami_dev_long/lo\endcsname{-0.05}
\expandafter\def\csname v@small/boot/dev4/diff\endcsname{+0.33}
\expandafter\def\csname v@small/boot/dev4/hi\endcsname{+0.72}
\expandafter\def\csname v@small/boot/dev4/lo\endcsname{-0.06}
\expandafter\def\csname v@small/c10/fixed-pct\endcsname{5.8}
\expandafter\def\csname v@small/c10/hold-s\endcsname{0.5}
\expandafter\def\csname v@small/c10/params-m\endcsname{9.8}
\expandafter\def\csname v@small/c10/theta\endcsname{0.9}
\expandafter\def\csname v@small/c10/theta-off\endcsname{0.3}
\expandafter\def\csname v@small/d640x12/cap-c2\endcsname{768}
\expandafter\def\csname v@small/d640x12/cap-c4\endcsname{1,024}
\expandafter\def\csname v@small/d640x12/params-m\endcsname{77}
\expandafter\def\csname v@small/d768x12/cap-c2\endcsname{512}
\expandafter\def\csname v@small/d768x12/cap-c4\endcsname{1,024}
\expandafter\def\csname v@small/d768x12/params-m\endcsname{108}
\expandafter\def\csname v@small/plugin/C7/core\endcsname{8.8}
\expandafter\def\csname v@small/plugin/C7/params-m\endcsname{6.8}
\expandafter\def\csname v@small/plugin/C7_int8/core\endcsname{7.6}
\expandafter\def\csname v@small/ws/256/sp50\endcsname{6.6}
\expandafter\def\csname v@small/ws/256/sp99\endcsname{13.7}
\expandafter\def\csname v@small/ws/behind\endcsname{1024}
\expandafter\def\csname v@small/ws/hold\endcsname{768}
\expandafter\def\csname v@small/ws/hold-sp50\endcsname{29}
\expandafter\def\csname v@small/ws/hold-sp99\endcsname{40}
\expandafter\def\csname v@small/ws/tested\endcsname{1024}
\expandafter\def\csname v@ssl/cwl/cos12\endcsname{0.82}
\expandafter\def\csname v@ssl/cwl/cos12@0k\endcsname{0.61}
\expandafter\def\csname v@ssl/cwl/cos12@1k\endcsname{0.80}
\expandafter\def\csname v@ssl/cwl/cos16\endcsname{0.81}
\expandafter\def\csname v@ssl/cwl/cos16@0k\endcsname{0.59}
\expandafter\def\csname v@ssl/cwl/cos16@1k\endcsname{0.78}
\expandafter\def\csname v@ssl/cwl/cos20\endcsname{0.83}
\expandafter\def\csname v@ssl/cwl/cos20@0k\endcsname{0.63}
\expandafter\def\csname v@ssl/cwl/cos20@1k\endcsname{0.81}
\expandafter\def\csname v@ssl/cwl/cos24\endcsname{0.77}
\expandafter\def\csname v@ssl/cwl/cos24@0k\endcsname{0.45}
\expandafter\def\csname v@ssl/cwl/cos24@1k\endcsname{0.74}
\expandafter\def\csname v@ssl/cwl/cos4\endcsname{0.93}
\expandafter\def\csname v@ssl/cwl/cos4@0k\endcsname{0.73}
\expandafter\def\csname v@ssl/cwl/cos4@1k\endcsname{0.90}
\expandafter\def\csname v@ssl/cwl/cos8\endcsname{0.86}
\expandafter\def\csname v@ssl/cwl/cos8@0k\endcsname{0.67}
\expandafter\def\csname v@ssl/cwl/cos8@1k\endcsname{0.84}
\expandafter\def\csname v@ssl/cwl/params\endcsname{311}
\expandafter\def\csname v@ssl/cwl/steps\endcsname{20,000}
\expandafter\def\csname v@ssl/student/cos16\endcsname{0.79}
\expandafter\def\csname v@ssl/student/cos16@20k\endcsname{0.78}
\expandafter\def\csname v@ssl/student/cos24\endcsname{0.77}
\expandafter\def\csname v@ssl/student/cos24@20k\endcsname{0.75}
\expandafter\def\csname v@ssl/student/cos8\endcsname{0.84}
\expandafter\def\csname v@ssl/student/cos8@20k\endcsname{0.83}
\expandafter\def\csname v@ssl/student/params\endcsname{331}
\expandafter\def\csname v@ssl/student/steps\endcsname{60,000}
\expandafter\def\csname v@tp/check/tp2/agree\endcsname{70}
\expandafter\def\csname v@tp/check/tp2/allreduce-us\endcsname{11}
\expandafter\def\csname v@tp/check/tp2/offline\endcsname{66}
\expandafter\def\csname v@tp/check/tp2/offline-one\endcsname{66}
\expandafter\def\csname v@tp/check/tp4/agree\endcsname{71}
\expandafter\def\csname v@tp/check/tp4/allreduce-us\endcsname{77}
\expandafter\def\csname v@tp/check/tp4/offline\endcsname{65}
\expandafter\def\csname v@tp/check/tp4/offline-one\endcsname{66}
\expandafter\def\csname v@tp/tp1/c2/1/p50\endcsname{6.8}
\expandafter\def\csname v@tp/tp1/c2/1/p99\endcsname{7.0}
\expandafter\def\csname v@tp/tp1/c2/128/p50\endcsname{16.4}
\expandafter\def\csname v@tp/tp1/c2/128/p99\endcsname{16.5}
\expandafter\def\csname v@tp/tp1/c2/256/p50\endcsname{26.6}
\expandafter\def\csname v@tp/tp1/c2/256/p99\endcsname{26.8}
\expandafter\def\csname v@tp/tp1/c2/32/p50\endcsname{9.1}
\expandafter\def\csname v@tp/tp1/c2/32/p99\endcsname{9.2}
\expandafter\def\csname v@tp/tp1/c2/64/p50\endcsname{11.6}
\expandafter\def\csname v@tp/tp1/c2/64/p99\endcsname{11.8}
\expandafter\def\csname v@tp/tp1/c2/cap\endcsname{160}
\expandafter\def\csname v@tp/tp1/c2/par-gpu\endcsname{555}
\expandafter\def\csname v@tp/tp1/c2/state-mb\endcsname{110}
\expandafter\def\csname v@tp/tp1/c4/1/p50\endcsname{7.2}
\expandafter\def\csname v@tp/tp1/c4/1/p99\endcsname{7.4}
\expandafter\def\csname v@tp/tp1/c4/128/p50\endcsname{20.6}
\expandafter\def\csname v@tp/tp1/c4/128/p99\endcsname{20.9}
\expandafter\def\csname v@tp/tp1/c4/256/p50\endcsname{34.9}
\expandafter\def\csname v@tp/tp1/c4/256/p99\endcsname{35.3}
\expandafter\def\csname v@tp/tp1/c4/32/p50\endcsname{10.3}
\expandafter\def\csname v@tp/tp1/c4/32/p99\endcsname{10.4}
\expandafter\def\csname v@tp/tp1/c4/64/p50\endcsname{13.6}
\expandafter\def\csname v@tp/tp1/c4/64/p99\endcsname{13.7}
\expandafter\def\csname v@tp/tp1/c4/cap\endcsname{256}
\expandafter\def\csname v@tp/tp1/c4/par-gpu\endcsname{555}
\expandafter\def\csname v@tp/tp1/c4/state-mb\endcsname{110}
\expandafter\def\csname v@tp/tp2/c2/1/p50\endcsname{7.3}
\expandafter\def\csname v@tp/tp2/c2/1/p99\endcsname{7.7}
\expandafter\def\csname v@tp/tp2/c2/1/speedup\endcsname{0.93}
\expandafter\def\csname v@tp/tp2/c2/128/p50\endcsname{13.2}
\expandafter\def\csname v@tp/tp2/c2/128/p99\endcsname{13.6}
\expandafter\def\csname v@tp/tp2/c2/128/speedup\endcsname{1.24}
\expandafter\def\csname v@tp/tp2/c2/256/p50\endcsname{19.4}
\expandafter\def\csname v@tp/tp2/c2/256/p99\endcsname{19.9}
\expandafter\def\csname v@tp/tp2/c2/256/speedup\endcsname{1.37}
\expandafter\def\csname v@tp/tp2/c2/32/p50\endcsname{8.6}
\expandafter\def\csname v@tp/tp2/c2/32/p99\endcsname{9.0}
\expandafter\def\csname v@tp/tp2/c2/32/speedup\endcsname{1.05}
\expandafter\def\csname v@tp/tp2/c2/64/p50\endcsname{10.1}
\expandafter\def\csname v@tp/tp2/c2/64/p99\endcsname{10.5}
\expandafter\def\csname v@tp/tp2/c2/64/speedup\endcsname{1.15}
\expandafter\def\csname v@tp/tp2/c2/cap\endcsname{256}
\expandafter\def\csname v@tp/tp2/c2/cap-gain\endcsname{1.60}
\expandafter\def\csname v@tp/tp2/c2/cap-per-gpu\endcsname{128}
\expandafter\def\csname v@tp/tp2/c2/par-gpu\endcsname{295}
\expandafter\def\csname v@tp/tp2/c2/state-mb\endcsname{55}
\expandafter\def\csname v@tp/tp2/c4/1/p50\endcsname{7.7}
\expandafter\def\csname v@tp/tp2/c4/1/p99\endcsname{8.0}
\expandafter\def\csname v@tp/tp2/c4/1/speedup\endcsname{0.94}
\expandafter\def\csname v@tp/tp2/c4/128/p50\endcsname{16.5}
\expandafter\def\csname v@tp/tp2/c4/128/p99\endcsname{17.0}
\expandafter\def\csname v@tp/tp2/c4/128/speedup\endcsname{1.25}
\expandafter\def\csname v@tp/tp2/c4/256/p50\endcsname{25.8}
\expandafter\def\csname v@tp/tp2/c4/256/p99\endcsname{26.6}
\expandafter\def\csname v@tp/tp2/c4/256/speedup\endcsname{1.35}
\expandafter\def\csname v@tp/tp2/c4/32/p50\endcsname{9.7}
\expandafter\def\csname v@tp/tp2/c4/32/p99\endcsname{10.1}
\expandafter\def\csname v@tp/tp2/c4/32/speedup\endcsname{1.06}
\expandafter\def\csname v@tp/tp2/c4/64/p50\endcsname{11.8}
\expandafter\def\csname v@tp/tp2/c4/64/p99\endcsname{12.4}
\expandafter\def\csname v@tp/tp2/c4/64/speedup\endcsname{1.15}
\expandafter\def\csname v@tp/tp2/c4/cap\endcsname{384}
\expandafter\def\csname v@tp/tp2/c4/cap-gain\endcsname{1.50}
\expandafter\def\csname v@tp/tp2/c4/cap-per-gpu\endcsname{192}
\expandafter\def\csname v@tp/tp2/c4/par-gpu\endcsname{295}
\expandafter\def\csname v@tp/tp2/c4/state-mb\endcsname{55}
\expandafter\def\csname v@tp/ws/dp2/behind\endcsname{256}
\expandafter\def\csname v@tp/ws/dp2/hold\endcsname{192}
\expandafter\def\csname v@tp/ws/dp2/hold-p50\endcsname{25}
\expandafter\def\csname v@tp/ws/dp2/hold-p99\endcsname{37}
\expandafter\def\csname v@tp/ws/dp2/tested\endcsname{320}
\expandafter\def\csname v@tp/ws/tp1/behind\endcsname{160}
\expandafter\def\csname v@tp/ws/tp1/hold\endcsname{128}
\expandafter\def\csname v@tp/ws/tp1/hold-p50\endcsname{29}
\expandafter\def\csname v@tp/ws/tp1/hold-p99\endcsname{39}
\expandafter\def\csname v@tp/ws/tp1/tested\endcsname{160}
\expandafter\def\csname v@tp/ws/tp2/behind\endcsname{192}
\expandafter\def\csname v@tp/ws/tp2/hold\endcsname{128}
\expandafter\def\csname v@tp/ws/tp2/hold-p50\endcsname{26}
\expandafter\def\csname v@tp/ws/tp2/hold-p99\endcsname{36}
\expandafter\def\csname v@tp/ws/tp2/tested\endcsname{320}
\expandafter\def\csname v@vad/aic_calls/C10_ftlong_kd_selfl/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/C10_ftlong_kd_selfl/bg_speech\endcsname{18.5}
\expandafter\def\csname v@vad/aic_calls/C10_ftlong_kd_selfl/bg_starts_per_min\endcsname{2.84}
\expandafter\def\csname v@vad/aic_calls/C10_ftlong_kd_selfl/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/C10_ftlong_kd_selfl/starts_per_min\endcsname{13.02}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_kd_selfl/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_kd_selfl/bg_speech\endcsname{18.1}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_kd_selfl/bg_starts_per_min\endcsname{2.46}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_kd_selfl/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_kd_selfl/starts_per_min\endcsname{12.83}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_sc_selfl/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_sc_selfl/bg_speech\endcsname{18.4}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_sc_selfl/bg_starts_per_min\endcsname{2.65}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_sc_selfl/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/C22_ftlong_sc_selfl/starts_per_min\endcsname{12.66}
\expandafter\def\csname v@vad/aic_calls/C51_ftlong_kd_selfl/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/C51_ftlong_kd_selfl/bg_speech\endcsname{18.4}
\expandafter\def\csname v@vad/aic_calls/C51_ftlong_kd_selfl/bg_starts_per_min\endcsname{2.53}
\expandafter\def\csname v@vad/aic_calls/C51_ftlong_kd_selfl/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/C51_ftlong_kd_selfl/starts_per_min\endcsname{12.77}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_cwlt2m_selfl/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_cwlt2m_selfl/bg_speech\endcsname{15.9}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_cwlt2m_selfl/bg_starts_per_min\endcsname{1.77}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_cwlt2m_selfl/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_cwlt2m_selfl/starts_per_min\endcsname{12.83}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_selfl/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_selfl/bg_speech\endcsname{18.7}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_selfl/bg_starts_per_min\endcsname{2.84}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_selfl/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/MB_ftlong_ws_selfl/starts_per_min\endcsname{12.85}
\expandafter\def\csname v@vad/aic_calls/dfn3/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/dfn3/bg_speech\endcsname{41.8}
\expandafter\def\csname v@vad/aic_calls/dfn3/bg_starts_per_min\endcsname{8.46}
\expandafter\def\csname v@vad/aic_calls/dfn3/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/dfn3/starts_per_min\endcsname{12.35}
\expandafter\def\csname v@vad/aic_calls/gtcrn/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/gtcrn/bg_speech\endcsname{59.8}
\expandafter\def\csname v@vad/aic_calls/gtcrn/bg_starts_per_min\endcsname{10.54}
\expandafter\def\csname v@vad/aic_calls/gtcrn/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/gtcrn/starts_per_min\endcsname{10.94}
\expandafter\def\csname v@vad/aic_calls/raw/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/raw/bg_speech\endcsname{57.1}
\expandafter\def\csname v@vad/aic_calls/raw/bg_starts_per_min\endcsname{9.03}
\expandafter\def\csname v@vad/aic_calls/raw/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/raw/starts_per_min\endcsname{10.54}
\expandafter\def\csname v@vad/aic_calls/rel/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/rel/bg_speech\endcsname{15.9}
\expandafter\def\csname v@vad/aic_calls/rel/bg_starts_per_min\endcsname{1.77}
\expandafter\def\csname v@vad/aic_calls/rel/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/rel/starts_per_min\endcsname{12.83}
\expandafter\def\csname v@vad/aic_calls/voxlock_live/bg_minutes\endcsname{15.84}
\expandafter\def\csname v@vad/aic_calls/voxlock_live/bg_speech\endcsname{26.7}
\expandafter\def\csname v@vad/aic_calls/voxlock_live/bg_starts_per_min\endcsname{4.48}
\expandafter\def\csname v@vad/aic_calls/voxlock_live/files\endcsname{83}
\expandafter\def\csname v@vad/aic_calls/voxlock_live/starts_per_min\endcsname{12.43}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_cwlt2m_selfl/bg_minutes\endcsname{7.51}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_cwlt2m_selfl/bg_speech\endcsname{10.2}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_cwlt2m_selfl/bg_starts_per_min\endcsname{2.13}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_cwlt2m_selfl/files\endcsname{134}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_cwlt2m_selfl/starts_per_min\endcsname{10.53}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_selfl/bg_minutes\endcsname{7.51}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_selfl/bg_speech\endcsname{9.5}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_selfl/bg_starts_per_min\endcsname{1.73}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_selfl/files\endcsname{134}
\expandafter\def\csname v@vad/ami_headset2/MB_ftlong_ws_selfl/starts_per_min\endcsname{10.42}
\expandafter\def\csname v@vad/ami_headset2/dfn3/bg_minutes\endcsname{7.51}
\expandafter\def\csname v@vad/ami_headset2/dfn3/bg_speech\endcsname{18.8}
\expandafter\def\csname v@vad/ami_headset2/dfn3/bg_starts_per_min\endcsname{3.60}
\expandafter\def\csname v@vad/ami_headset2/dfn3/files\endcsname{134}
\expandafter\def\csname v@vad/ami_headset2/dfn3/starts_per_min\endcsname{10.61}
\expandafter\def\csname v@vad/ami_headset2/gtcrn/bg_minutes\endcsname{7.51}
\expandafter\def\csname v@vad/ami_headset2/gtcrn/bg_speech\endcsname{19.0}
\expandafter\def\csname v@vad/ami_headset2/gtcrn/bg_starts_per_min\endcsname{3.60}
\expandafter\def\csname v@vad/ami_headset2/gtcrn/files\endcsname{134}
\expandafter\def\csname v@vad/ami_headset2/gtcrn/starts_per_min\endcsname{11.71}
\expandafter\def\csname v@vad/ami_headset2/raw/bg_minutes\endcsname{7.51}
\expandafter\def\csname v@vad/ami_headset2/raw/bg_speech\endcsname{20.1}
\expandafter\def\csname v@vad/ami_headset2/raw/bg_starts_per_min\endcsname{3.06}
\expandafter\def\csname v@vad/ami_headset2/raw/files\endcsname{134}
\expandafter\def\csname v@vad/ami_headset2/raw/starts_per_min\endcsname{10.81}
\expandafter\def\csname v@vad/ami_headset2/rel/bg_minutes\endcsname{7.51}
\expandafter\def\csname v@vad/ami_headset2/rel/bg_speech\endcsname{10.2}
\expandafter\def\csname v@vad/ami_headset2/rel/bg_starts_per_min\endcsname{2.13}
\expandafter\def\csname v@vad/ami_headset2/rel/files\endcsname{134}
\expandafter\def\csname v@vad/ami_headset2/rel/starts_per_min\endcsname{10.53}
\expandafter\def\csname v@vad/ami_headset2/voxlock_live/bg_minutes\endcsname{7.51}
\expandafter\def\csname v@vad/ami_headset2/voxlock_live/bg_speech\endcsname{8.6}
\expandafter\def\csname v@vad/ami_headset2/voxlock_live/bg_starts_per_min\endcsname{1.60}
\expandafter\def\csname v@vad/ami_headset2/voxlock_live/files\endcsname{134}
\expandafter\def\csname v@vad/ami_headset2/voxlock_live/starts_per_min\endcsname{10.42}
\expandafter\def\csname v@vad/ami_test/C10_ftlong_kd_selfl/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/C10_ftlong_kd_selfl/bg_speech\endcsname{11.7}
\expandafter\def\csname v@vad/ami_test/C10_ftlong_kd_selfl/bg_starts_per_min\endcsname{1.41}
\expandafter\def\csname v@vad/ami_test/C10_ftlong_kd_selfl/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/C10_ftlong_kd_selfl/starts_per_min\endcsname{10.44}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_kd_selfl/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_kd_selfl/bg_speech\endcsname{11.4}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_kd_selfl/bg_starts_per_min\endcsname{1.50}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_kd_selfl/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_kd_selfl/starts_per_min\endcsname{10.52}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_sc_selfl/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_sc_selfl/bg_speech\endcsname{11.4}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_sc_selfl/bg_starts_per_min\endcsname{1.47}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_sc_selfl/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/C22_ftlong_sc_selfl/starts_per_min\endcsname{10.51}
\expandafter\def\csname v@vad/ami_test/C51_ftlong_kd_selfl/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/C51_ftlong_kd_selfl/bg_speech\endcsname{11.4}
\expandafter\def\csname v@vad/ami_test/C51_ftlong_kd_selfl/bg_starts_per_min\endcsname{1.32}
\expandafter\def\csname v@vad/ami_test/C51_ftlong_kd_selfl/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/C51_ftlong_kd_selfl/starts_per_min\endcsname{10.50}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_cwlt2m_selfl/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_cwlt2m_selfl/bg_speech\endcsname{12.1}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_cwlt2m_selfl/bg_starts_per_min\endcsname{1.71}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_cwlt2m_selfl/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_cwlt2m_selfl/starts_per_min\endcsname{10.51}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_selfl/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_selfl/bg_speech\endcsname{11.3}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_selfl/bg_starts_per_min\endcsname{1.32}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_selfl/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/MB_ftlong_ws_selfl/starts_per_min\endcsname{10.42}
\expandafter\def\csname v@vad/ami_test/dfn3/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/dfn3/bg_speech\endcsname{19.0}
\expandafter\def\csname v@vad/ami_test/dfn3/bg_starts_per_min\endcsname{2.62}
\expandafter\def\csname v@vad/ami_test/dfn3/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/dfn3/starts_per_min\endcsname{10.02}
\expandafter\def\csname v@vad/ami_test/gtcrn/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/gtcrn/bg_speech\endcsname{23.3}
\expandafter\def\csname v@vad/ami_test/gtcrn/bg_starts_per_min\endcsname{3.91}
\expandafter\def\csname v@vad/ami_test/gtcrn/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/gtcrn/starts_per_min\endcsname{11.24}
\expandafter\def\csname v@vad/ami_test/raw/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/raw/bg_speech\endcsname{21.1}
\expandafter\def\csname v@vad/ami_test/raw/bg_starts_per_min\endcsname{2.53}
\expandafter\def\csname v@vad/ami_test/raw/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/raw/starts_per_min\endcsname{10.55}
\expandafter\def\csname v@vad/ami_test/rel/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/rel/bg_speech\endcsname{12.1}
\expandafter\def\csname v@vad/ami_test/rel/bg_starts_per_min\endcsname{1.71}
\expandafter\def\csname v@vad/ami_test/rel/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/rel/starts_per_min\endcsname{10.51}
\expandafter\def\csname v@vad/ami_test/voxlock_live/bg_minutes\endcsname{34.00}
\expandafter\def\csname v@vad/ami_test/voxlock_live/bg_speech\endcsname{11.7}
\expandafter\def\csname v@vad/ami_test/voxlock_live/bg_starts_per_min\endcsname{1.18}
\expandafter\def\csname v@vad/ami_test/voxlock_live/files\endcsname{599}
\expandafter\def\csname v@vad/ami_test/voxlock_live/starts_per_min\endcsname{10.17}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/end_delay_p50\endcsname{-0.03}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/false\endcsname{0.2}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/false_starts_per_min\endcsname{0.03}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/held\endcsname{54}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/held-pct\endcsname{7}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/missed\endcsname{4.5}
\expandafter\def\csname v@vad/call_test_clean/C10_ftlong_kd_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/end_delay_p50\endcsname{-0.03}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/false\endcsname{0.1}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/false_starts_per_min\endcsname{0.03}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/held\endcsname{61}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/held-pct\endcsname{8}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/missed\endcsname{4.9}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_kd_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/end_delay_p50\endcsname{-0.03}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/false\endcsname{0.1}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/false_starts_per_min\endcsname{0.01}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/held\endcsname{79}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/held-pct\endcsname{10}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/missed\endcsname{7.6}
\expandafter\def\csname v@vad/call_test_clean/C22_ftlong_sc_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/end_delay_p50\endcsname{-0.03}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/false\endcsname{0.2}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/false_starts_per_min\endcsname{0.03}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/held\endcsname{64}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/held-pct\endcsname{8}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/missed\endcsname{4.8}
\expandafter\def\csname v@vad/call_test_clean/C51_ftlong_kd_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/end_delay_p50\endcsname{-0.03}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/false\endcsname{0.1}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/false_starts_per_min\endcsname{0.03}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/held\endcsname{63}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/held-pct\endcsname{8}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/missed\endcsname{5.2}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_cwlt2m_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/end_delay_p50\endcsname{-0.03}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/false\endcsname{0.2}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/false_starts_per_min\endcsname{0.03}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/held\endcsname{92}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/held-pct\endcsname{11}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/missed\endcsname{8.4}
\expandafter\def\csname v@vad/call_test_clean/MB_ftlong_ws_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/dfn3/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/dfn3/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/dfn3/false\endcsname{0.1}
\expandafter\def\csname v@vad/call_test_clean/dfn3/false_starts_per_min\endcsname{0.01}
\expandafter\def\csname v@vad/call_test_clean/dfn3/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/dfn3/held\endcsname{19}
\expandafter\def\csname v@vad/call_test_clean/dfn3/held-pct\endcsname{2}
\expandafter\def\csname v@vad/call_test_clean/dfn3/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/dfn3/missed\endcsname{0.9}
\expandafter\def\csname v@vad/call_test_clean/dfn3/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/false\endcsname{0.4}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/false_starts_per_min\endcsname{0.10}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/held\endcsname{11}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/held-pct\endcsname{1}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/missed\endcsname{0.6}
\expandafter\def\csname v@vad/call_test_clean/gtcrn/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/raw/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/raw/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/raw/false\endcsname{0.0}
\expandafter\def\csname v@vad/call_test_clean/raw/false_starts_per_min\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/raw/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/raw/held\endcsname{0}
\expandafter\def\csname v@vad/call_test_clean/raw/held-pct\endcsname{0}
\expandafter\def\csname v@vad/call_test_clean/raw/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/raw/missed\endcsname{0.0}
\expandafter\def\csname v@vad/call_test_clean/raw/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/rel/end_delay_p50\endcsname{-0.03}
\expandafter\def\csname v@vad/call_test_clean/rel/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/rel/false\endcsname{0.1}
\expandafter\def\csname v@vad/call_test_clean/rel/false_starts_per_min\endcsname{0.03}
\expandafter\def\csname v@vad/call_test_clean/rel/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/rel/held\endcsname{63}
\expandafter\def\csname v@vad/call_test_clean/rel/held-pct\endcsname{8}
\expandafter\def\csname v@vad/call_test_clean/rel/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/rel/missed\endcsname{5.2}
\expandafter\def\csname v@vad/call_test_clean/rel/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/end_delay_p90\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/false\endcsname{0.1}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/false_starts_per_min\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/held\endcsname{41}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/held-pct\endcsname{5}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/missed\endcsname{2.6}
\expandafter\def\csname v@vad/call_test_clean/voxlock_live/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/end_delay_p90\endcsname{1.47}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/false\endcsname{27.6}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/false_starts_per_min\endcsname{2.40}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/held\endcsname{167}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/held-pct\endcsname{21}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/missed\endcsname{6.6}
\expandafter\def\csname v@vad/call_test_mix/C10_ftlong_kd_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/end_delay_p90\endcsname{1.34}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/false\endcsname{26.2}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/false_starts_per_min\endcsname{2.27}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/held\endcsname{162}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/held-pct\endcsname{20}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/missed\endcsname{6.7}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_kd_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/end_delay_p90\endcsname{1.38}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/false\endcsname{22.9}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/false_starts_per_min\endcsname{2.08}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/held\endcsname{156}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/held-pct\endcsname{19}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/missed\endcsname{9.5}
\expandafter\def\csname v@vad/call_test_mix/C22_ftlong_sc_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/end_delay_p90\endcsname{1.38}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/false\endcsname{26.4}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/false_starts_per_min\endcsname{2.16}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/held\endcsname{167}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/held-pct\endcsname{21}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/missed\endcsname{5.9}
\expandafter\def\csname v@vad/call_test_mix/C51_ftlong_kd_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/end_delay_p90\endcsname{1.00}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/false\endcsname{22.8}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/false_starts_per_min\endcsname{1.94}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/held\endcsname{148}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/held-pct\endcsname{18}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/missed\endcsname{8.4}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_cwlt2m_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/end_delay_p90\endcsname{1.41}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/false\endcsname{24.2}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/false_starts_per_min\endcsname{2.27}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/held\endcsname{154}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/held-pct\endcsname{19}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/missed\endcsname{8.4}
\expandafter\def\csname v@vad/call_test_mix/MB_ftlong_ws_selfl/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/dfn3/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/dfn3/end_delay_p90\endcsname{2.28}
\expandafter\def\csname v@vad/call_test_mix/dfn3/false\endcsname{45.2}
\expandafter\def\csname v@vad/call_test_mix/dfn3/false_starts_per_min\endcsname{3.14}
\expandafter\def\csname v@vad/call_test_mix/dfn3/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/dfn3/held\endcsname{216}
\expandafter\def\csname v@vad/call_test_mix/dfn3/held-pct\endcsname{27}
\expandafter\def\csname v@vad/call_test_mix/dfn3/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/dfn3/missed\endcsname{0.6}
\expandafter\def\csname v@vad/call_test_mix/dfn3/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/end_delay_p90\endcsname{2.40}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/false\endcsname{48.3}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/false_starts_per_min\endcsname{3.58}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/held\endcsname{212}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/held-pct\endcsname{26}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/missed\endcsname{0.3}
\expandafter\def\csname v@vad/call_test_mix/gtcrn/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/raw/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/raw/end_delay_p90\endcsname{2.43}
\expandafter\def\csname v@vad/call_test_mix/raw/false\endcsname{47.9}
\expandafter\def\csname v@vad/call_test_mix/raw/false_starts_per_min\endcsname{3.33}
\expandafter\def\csname v@vad/call_test_mix/raw/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/raw/held\endcsname{223}
\expandafter\def\csname v@vad/call_test_mix/raw/held-pct\endcsname{28}
\expandafter\def\csname v@vad/call_test_mix/raw/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/raw/missed\endcsname{0.1}
\expandafter\def\csname v@vad/call_test_mix/raw/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/rel/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/rel/end_delay_p90\endcsname{1.00}
\expandafter\def\csname v@vad/call_test_mix/rel/false\endcsname{22.8}
\expandafter\def\csname v@vad/call_test_mix/rel/false_starts_per_min\endcsname{1.94}
\expandafter\def\csname v@vad/call_test_mix/rel/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/rel/held\endcsname{148}
\expandafter\def\csname v@vad/call_test_mix/rel/held-pct\endcsname{18}
\expandafter\def\csname v@vad/call_test_mix/rel/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/rel/missed\endcsname{8.4}
\expandafter\def\csname v@vad/call_test_mix/rel/turns\endcsname{805}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/end_delay_p50\endcsname{0.00}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/end_delay_p90\endcsname{1.51}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/false\endcsname{27.5}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/false_starts_per_min\endcsname{2.28}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/files\endcsname{120}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/held\endcsname{196}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/held-pct\endcsname{24}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/minutes\endcsname{120.00}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/missed\endcsname{11.0}
\expandafter\def\csname v@vad/call_test_mix/voxlock_live/turns\endcsname{805}
\expandafter\def\csname v@vad/krisp/C10_ftlong_kd_selfl/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/C10_ftlong_kd_selfl/bg_speech\endcsname{0.5}
\expandafter\def\csname v@vad/krisp/C10_ftlong_kd_selfl/bg_starts_per_min\endcsname{0.14}
\expandafter\def\csname v@vad/krisp/C10_ftlong_kd_selfl/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/C10_ftlong_kd_selfl/starts_per_min\endcsname{4.23}
\expandafter\def\csname v@vad/krisp/C22_ftlong_kd_selfl/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/C22_ftlong_kd_selfl/bg_speech\endcsname{0.4}
\expandafter\def\csname v@vad/krisp/C22_ftlong_kd_selfl/bg_starts_per_min\endcsname{0.08}
\expandafter\def\csname v@vad/krisp/C22_ftlong_kd_selfl/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/C22_ftlong_kd_selfl/starts_per_min\endcsname{4.20}
\expandafter\def\csname v@vad/krisp/C22_ftlong_sc_selfl/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/C22_ftlong_sc_selfl/bg_speech\endcsname{0.4}
\expandafter\def\csname v@vad/krisp/C22_ftlong_sc_selfl/bg_starts_per_min\endcsname{0.15}
\expandafter\def\csname v@vad/krisp/C22_ftlong_sc_selfl/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/C22_ftlong_sc_selfl/starts_per_min\endcsname{4.35}
\expandafter\def\csname v@vad/krisp/C51_ftlong_kd_selfl/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/C51_ftlong_kd_selfl/bg_speech\endcsname{0.5}
\expandafter\def\csname v@vad/krisp/C51_ftlong_kd_selfl/bg_starts_per_min\endcsname{0.14}
\expandafter\def\csname v@vad/krisp/C51_ftlong_kd_selfl/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/C51_ftlong_kd_selfl/starts_per_min\endcsname{4.23}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_cwlt2m_selfl/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_cwlt2m_selfl/bg_speech\endcsname{0.4}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_cwlt2m_selfl/bg_starts_per_min\endcsname{0.13}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_cwlt2m_selfl/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_cwlt2m_selfl/starts_per_min\endcsname{4.22}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_selfl/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_selfl/bg_speech\endcsname{0.9}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_selfl/bg_starts_per_min\endcsname{0.26}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_selfl/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/MB_ftlong_ws_selfl/starts_per_min\endcsname{4.35}
\expandafter\def\csname v@vad/krisp/dfn3/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/dfn3/bg_speech\endcsname{24.4}
\expandafter\def\csname v@vad/krisp/dfn3/bg_starts_per_min\endcsname{3.29}
\expandafter\def\csname v@vad/krisp/dfn3/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/dfn3/starts_per_min\endcsname{4.42}
\expandafter\def\csname v@vad/krisp/gtcrn/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/gtcrn/bg_speech\endcsname{53.1}
\expandafter\def\csname v@vad/krisp/gtcrn/bg_starts_per_min\endcsname{6.54}
\expandafter\def\csname v@vad/krisp/gtcrn/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/gtcrn/starts_per_min\endcsname{5.07}
\expandafter\def\csname v@vad/krisp/raw/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/raw/bg_speech\endcsname{43.2}
\expandafter\def\csname v@vad/krisp/raw/bg_starts_per_min\endcsname{5.09}
\expandafter\def\csname v@vad/krisp/raw/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/raw/starts_per_min\endcsname{4.52}
\expandafter\def\csname v@vad/krisp/rel/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/rel/bg_speech\endcsname{0.4}
\expandafter\def\csname v@vad/krisp/rel/bg_starts_per_min\endcsname{0.13}
\expandafter\def\csname v@vad/krisp/rel/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/rel/starts_per_min\endcsname{4.22}
\expandafter\def\csname v@vad/krisp/voxlock_live/bg_minutes\endcsname{85.34}
\expandafter\def\csname v@vad/krisp/voxlock_live/bg_speech\endcsname{0.6}
\expandafter\def\csname v@vad/krisp/voxlock_live/bg_starts_per_min\endcsname{0.16}
\expandafter\def\csname v@vad/krisp/voxlock_live/files\endcsname{265}
\expandafter\def\csname v@vad/krisp/voxlock_live/starts_per_min\endcsname{3.88}
\expandafter\def\csname v@vint/agent/head-p-enroll-mix\endcsname{30}
\expandafter\def\csname v@vint/agent/head-steps\endcsname{2,000}
\expandafter\def\csname v@vint/agent/head-width\endcsname{256}
\expandafter\def\csname v@vint/agent/hold-s\endcsname{1}
\expandafter\def\csname v@vint/agent/keep-db\endcsname{1}
\expandafter\def\csname v@vint/agent/p-tv\endcsname{40}
\expandafter\def\csname v@vint/agent/steps\endcsname{1,500}
\expandafter\def\csname v@vint/agent/theta\endcsname{0.9}
\expandafter\def\csname v@vint/agent/theta-off\endcsname{0.2}
\expandafter\def\csname v@vint/agent/tv-p\endcsname{80}
\expandafter\def\csname v@vint/agent/tv-sir-hi\endcsname{12}
\expandafter\def\csname v@vint/agent/tv-sir-lo\endcsname{-6}
\expandafter\def\csname v@vint/agent/w-gate\endcsname{5}
\expandafter\def\csname v@vint/c10/c10ag/after\endcsname{0.24}
\expandafter\def\csname v@vint/c10/c10ag/after-hi\endcsname{0.40}
\expandafter\def\csname v@vint/c10/c10ag/after-lo\endcsname{0.12}
\expandafter\def\csname v@vint/c10/c10ag/all\endcsname{0.60}
\expandafter\def\csname v@vint/c10/c10ag/all-hi\endcsname{0.86}
\expandafter\def\csname v@vint/c10/c10ag/all-lo\endcsname{0.37}
\expandafter\def\csname v@vint/c10/c10ag/greet\endcsname{3.41}
\expandafter\def\csname v@vint/c10/c10ag/greet-hi\endcsname{4.79}
\expandafter\def\csname v@vint/c10/c10ag/greet-lo\endcsname{2.13}
\expandafter\def\csname v@vint/c10/c10ag8/after\endcsname{0.25}
\expandafter\def\csname v@vint/c10/c10ag8/after-hi\endcsname{0.41}
\expandafter\def\csname v@vint/c10/c10ag8/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/c10/c10ag8/all\endcsname{0.60}
\expandafter\def\csname v@vint/c10/c10ag8/all-hi\endcsname{0.87}
\expandafter\def\csname v@vint/c10/c10ag8/all-lo\endcsname{0.38}
\expandafter\def\csname v@vint/c10/c10ag8/greet\endcsname{3.39}
\expandafter\def\csname v@vint/c10/c10ag8/greet-hi\endcsname{4.77}
\expandafter\def\csname v@vint/c10/c10ag8/greet-lo\endcsname{2.12}
\expandafter\def\csname v@vint/c10/c10agv/after\endcsname{0.25}
\expandafter\def\csname v@vint/c10/c10agv/after-hi\endcsname{0.40}
\expandafter\def\csname v@vint/c10/c10agv/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/c10/c10agv/all\endcsname{0.35}
\expandafter\def\csname v@vint/c10/c10agv/all-hi\endcsname{0.53}
\expandafter\def\csname v@vint/c10/c10agv/all-lo\endcsname{0.21}
\expandafter\def\csname v@vint/c10/c10agv/greet\endcsname{1.12}
\expandafter\def\csname v@vint/c10/c10agv/greet-hi\endcsname{1.64}
\expandafter\def\csname v@vint/c10/c10agv/greet-lo\endcsname{0.67}
\expandafter\def\csname v@vint/c10/c10agv8/after\endcsname{0.24}
\expandafter\def\csname v@vint/c10/c10agv8/after-hi\endcsname{0.39}
\expandafter\def\csname v@vint/c10/c10agv8/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/c10/c10agv8/all\endcsname{0.35}
\expandafter\def\csname v@vint/c10/c10agv8/all-hi\endcsname{0.52}
\expandafter\def\csname v@vint/c10/c10agv8/all-lo\endcsname{0.21}
\expandafter\def\csname v@vint/c10/c10agv8/greet\endcsname{1.14}
\expandafter\def\csname v@vint/c10/c10agv8/greet-hi\endcsname{1.67}
\expandafter\def\csname v@vint/c10/c10agv8/greet-lo\endcsname{0.67}
\expandafter\def\csname v@vint/c10/c10st8/after\endcsname{0.86}
\expandafter\def\csname v@vint/c10/c10st8/after-hi\endcsname{1.31}
\expandafter\def\csname v@vint/c10/c10st8/after-lo\endcsname{0.49}
\expandafter\def\csname v@vint/c10/c10st8/all\endcsname{1.43}
\expandafter\def\csname v@vint/c10/c10st8/all-hi\endcsname{1.97}
\expandafter\def\csname v@vint/c10/c10st8/all-lo\endcsname{0.97}
\expandafter\def\csname v@vint/c10/c10st8/greet\endcsname{5.87}
\expandafter\def\csname v@vint/c10/c10st8/greet-hi\endcsname{7.58}
\expandafter\def\csname v@vint/c10/c10st8/greet-lo\endcsname{4.26}
\expandafter\def\csname v@vint/c10/core/c10\endcsname{10.2}
\expandafter\def\csname v@vint/c10/core/c108\endcsname{8.5}
\expandafter\def\csname v@vint/c10/core/c10ag\endcsname{10.4}
\expandafter\def\csname v@vint/c10/core/c10ag8\endcsname{8.8}
\expandafter\def\csname v@vint/c10/core/c10agv\endcsname{10.5}
\expandafter\def\csname v@vint/c10/core/c10agv8\endcsname{8.8}
\expandafter\def\csname v@vint/c10/core/cpu\endcsname{16.9}
\expandafter\def\csname v@vint/c10/core/cpu8\endcsname{12.5}
\expandafter\def\csname v@vint/c10/core/cpuag\endcsname{16.9}
\expandafter\def\csname v@vint/c10/core/cpuag8\endcsname{12.6}
\expandafter\def\csname v@vint/c10/core/cpuagv\endcsname{17.0}
\expandafter\def\csname v@vint/c10/core/cpuagv8\endcsname{12.7}
\expandafter\def\csname v@vint/c10/cpu8/after\endcsname{0.80}
\expandafter\def\csname v@vint/c10/cpu8/after-hi\endcsname{1.24}
\expandafter\def\csname v@vint/c10/cpu8/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/c10/cpu8/all\endcsname{1.36}
\expandafter\def\csname v@vint/c10/cpu8/all-hi\endcsname{1.88}
\expandafter\def\csname v@vint/c10/cpu8/all-lo\endcsname{0.93}
\expandafter\def\csname v@vint/c10/cpu8/greet\endcsname{5.77}
\expandafter\def\csname v@vint/c10/cpu8/greet-hi\endcsname{7.41}
\expandafter\def\csname v@vint/c10/cpu8/greet-lo\endcsname{4.21}
\expandafter\def\csname v@vint/c10/cpuBv/after\endcsname{0.17}
\expandafter\def\csname v@vint/c10/cpuBv/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/c10/cpuBv/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/c10/cpuBv/all\endcsname{0.26}
\expandafter\def\csname v@vint/c10/cpuBv/all-hi\endcsname{0.44}
\expandafter\def\csname v@vint/c10/cpuBv/all-lo\endcsname{0.13}
\expandafter\def\csname v@vint/c10/cpuBv/greet\endcsname{0.97}
\expandafter\def\csname v@vint/c10/cpuBv/greet-hi\endcsname{1.47}
\expandafter\def\csname v@vint/c10/cpuBv/greet-lo\endcsname{0.55}
\expandafter\def\csname v@vint/c10/cpuBv8/after\endcsname{0.16}
\expandafter\def\csname v@vint/c10/cpuBv8/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/c10/cpuBv8/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/c10/cpuBv8/all\endcsname{0.26}
\expandafter\def\csname v@vint/c10/cpuBv8/all-hi\endcsname{0.42}
\expandafter\def\csname v@vint/c10/cpuBv8/all-lo\endcsname{0.13}
\expandafter\def\csname v@vint/c10/cpuBv8/greet\endcsname{0.97}
\expandafter\def\csname v@vint/c10/cpuBv8/greet-hi\endcsname{1.47}
\expandafter\def\csname v@vint/c10/cpuBv8/greet-lo\endcsname{0.55}
\expandafter\def\csname v@vint/c10/cpuag/after\endcsname{0.14}
\expandafter\def\csname v@vint/c10/cpuag/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/c10/cpuag/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/c10/cpuag/all\endcsname{0.48}
\expandafter\def\csname v@vint/c10/cpuag/all-hi\endcsname{0.71}
\expandafter\def\csname v@vint/c10/cpuag/all-lo\endcsname{0.29}
\expandafter\def\csname v@vint/c10/cpuag/greet\endcsname{3.14}
\expandafter\def\csname v@vint/c10/cpuag/greet-hi\endcsname{4.45}
\expandafter\def\csname v@vint/c10/cpuag/greet-lo\endcsname{1.94}
\expandafter\def\csname v@vint/c10/cpuag8/after\endcsname{0.14}
\expandafter\def\csname v@vint/c10/cpuag8/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/c10/cpuag8/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/c10/cpuag8/all\endcsname{0.48}
\expandafter\def\csname v@vint/c10/cpuag8/all-hi\endcsname{0.71}
\expandafter\def\csname v@vint/c10/cpuag8/all-lo\endcsname{0.29}
\expandafter\def\csname v@vint/c10/cpuag8/greet\endcsname{3.14}
\expandafter\def\csname v@vint/c10/cpuag8/greet-hi\endcsname{4.45}
\expandafter\def\csname v@vint/c10/cpuag8/greet-lo\endcsname{1.94}
\expandafter\def\csname v@vint/c10/diff/c10ag-c10ag8/all\endcsname{-0.00}
\expandafter\def\csname v@vint/c10/diff/c10ag-c10ag8/all-hi\endcsname{+0.00}
\expandafter\def\csname v@vint/c10/diff/c10ag-c10ag8/all-lo\endcsname{-0.01}
\expandafter\def\csname v@vint/c10/diff/c10ag8-cpuag8/all\endcsname{+0.12}
\expandafter\def\csname v@vint/c10/diff/c10ag8-cpuag8/all-hi\endcsname{+0.18}
\expandafter\def\csname v@vint/c10/diff/c10ag8-cpuag8/all-lo\endcsname{+0.07}
\expandafter\def\csname v@vint/c10/diff/c10ag8-reuse/all\endcsname{-0.35}
\expandafter\def\csname v@vint/c10/diff/c10ag8-reuse/all-hi\endcsname{-0.19}
\expandafter\def\csname v@vint/c10/diff/c10ag8-reuse/all-lo\endcsname{-0.52}
\expandafter\def\csname v@vint/c10/diff/c10agv-c10agv8/all\endcsname{+0.00}
\expandafter\def\csname v@vint/c10/diff/c10agv-c10agv8/all-hi\endcsname{+0.01}
\expandafter\def\csname v@vint/c10/diff/c10agv-c10agv8/all-lo\endcsname{-0.00}
\expandafter\def\csname v@vint/c10/diff/c10agv8-c10ag8/all\endcsname{-0.26}
\expandafter\def\csname v@vint/c10/diff/c10agv8-c10ag8/all-hi\endcsname{-0.14}
\expandafter\def\csname v@vint/c10/diff/c10agv8-c10ag8/all-lo\endcsname{-0.38}
\expandafter\def\csname v@vint/c10/diff/c10agv8-cpuBv8/all\endcsname{+0.09}
\expandafter\def\csname v@vint/c10/diff/c10agv8-cpuBv8/all-hi\endcsname{+0.15}
\expandafter\def\csname v@vint/c10/diff/c10agv8-cpuBv8/all-lo\endcsname{+0.04}
\expandafter\def\csname v@vint/c10/diff/c10agv8-reuse/all\endcsname{-0.60}
\expandafter\def\csname v@vint/c10/diff/c10agv8-reuse/all-hi\endcsname{-0.38}
\expandafter\def\csname v@vint/c10/diff/c10agv8-reuse/all-lo\endcsname{-0.84}
\expandafter\def\csname v@vint/c10/diff/c10st8-cpu8/all\endcsname{+0.06}
\expandafter\def\csname v@vint/c10/diff/c10st8-cpu8/all-hi\endcsname{+0.15}
\expandafter\def\csname v@vint/c10/diff/c10st8-cpu8/all-lo\endcsname{-0.01}
\expandafter\def\csname v@vint/c10/none/after\endcsname{2.42}
\expandafter\def\csname v@vint/c10/none/after-hi\endcsname{3.29}
\expandafter\def\csname v@vint/c10/none/after-lo\endcsname{1.64}
\expandafter\def\csname v@vint/c10/none/all\endcsname{2.77}
\expandafter\def\csname v@vint/c10/none/all-hi\endcsname{3.73}
\expandafter\def\csname v@vint/c10/none/all-lo\endcsname{1.91}
\expandafter\def\csname v@vint/c10/none/greet\endcsname{5.52}
\expandafter\def\csname v@vint/c10/none/greet-hi\endcsname{7.39}
\expandafter\def\csname v@vint/c10/none/greet-lo\endcsname{3.80}
\expandafter\def\csname v@vint/c10/reuse/after\endcsname{0.24}
\expandafter\def\csname v@vint/c10/reuse/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/c10/reuse/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/c10/reuse/all\endcsname{0.95}
\expandafter\def\csname v@vint/c10/reuse/all-hi\endcsname{1.30}
\expandafter\def\csname v@vint/c10/reuse/all-lo\endcsname{0.63}
\expandafter\def\csname v@vint/c10/reuse/greet\endcsname{6.54}
\expandafter\def\csname v@vint/c10/reuse/greet-hi\endcsname{8.46}
\expandafter\def\csname v@vint/c10/reuse/greet-lo\endcsname{4.71}
\expandafter\def\csname v@vint/c10/silence/c10ag/missed\endcsname{2.2}
\expandafter\def\csname v@vint/c10/silence/c10ag/wer\endcsname{14.8}
\expandafter\def\csname v@vint/c10/silence/c10ag8/missed\endcsname{2.2}
\expandafter\def\csname v@vint/c10/silence/c10ag8/wer\endcsname{14.8}
\expandafter\def\csname v@vint/c10/silence/c10agv/missed\endcsname{1.5}
\expandafter\def\csname v@vint/c10/silence/c10agv/wer\endcsname{15.9}
\expandafter\def\csname v@vint/c10/silence/c10agv8/missed\endcsname{1.5}
\expandafter\def\csname v@vint/c10/silence/c10agv8/wer\endcsname{15.8}
\expandafter\def\csname v@vint/c10/silence/c10st8/missed\endcsname{0.2}
\expandafter\def\csname v@vint/c10/silence/c10st8/wer\endcsname{11.4}
\expandafter\def\csname v@vint/c10/silence/cpu8/missed\endcsname{0.3}
\expandafter\def\csname v@vint/c10/silence/cpu8/wer\endcsname{11.8}
\expandafter\def\csname v@vint/c10/silence/cpuBv/missed\endcsname{1.6}
\expandafter\def\csname v@vint/c10/silence/cpuBv/wer\endcsname{16.8}
\expandafter\def\csname v@vint/c10/silence/cpuBv8/missed\endcsname{1.7}
\expandafter\def\csname v@vint/c10/silence/cpuBv8/wer\endcsname{16.8}
\expandafter\def\csname v@vint/c10/silence/cpuag/missed\endcsname{2.4}
\expandafter\def\csname v@vint/c10/silence/cpuag/wer\endcsname{16.0}
\expandafter\def\csname v@vint/c10/silence/cpuag8/missed\endcsname{2.4}
\expandafter\def\csname v@vint/c10/silence/cpuag8/wer\endcsname{16.2}
\expandafter\def\csname v@vint/c10/silence/none/missed\endcsname{0.4}
\expandafter\def\csname v@vint/c10/silence/none/wer\endcsname{7.4}
\expandafter\def\csname v@vint/c10/silence/reuse/missed\endcsname{2.6}
\expandafter\def\csname v@vint/c10/silence/reuse/wer\endcsname{16.9}
\expandafter\def\csname v@vint/calls\endcsname{816}
\expandafter\def\csname v@vint/check/arms\endcsname{5}
\expandafter\def\csname v@vint/check/pauses-pct\endcsname{94}
\expandafter\def\csname v@vint/check/starts-pct\endcsname{95}
\expandafter\def\csname v@vint/check/voxlock/starts-pct\endcsname{81}
\expandafter\def\csname v@vint/cpu/caught\endcsname{90.9}
\expandafter\def\csname v@vint/cpu/caught-d\endcsname{+1.0}
\expandafter\def\csname v@vint/cpu/caught-dabs\endcsname{1.0}
\expandafter\def\csname v@vint/cpu/caught-dhi\endcsname{+1.8}
\expandafter\def\csname v@vint/cpu/caught-dlo\endcsname{+0.2}
\expandafter\def\csname v@vint/cpu/caught-hi\endcsname{92.5}
\expandafter\def\csname v@vint/cpu/caught-lo\endcsname{89.1}
\expandafter\def\csname v@vint/cpu/core-pct\endcsname{18}
\expandafter\def\csname v@vint/cpu/cores\endcsname{0.18}
\expandafter\def\csname v@vint/cpu/fi\endcsname{1.36}
\expandafter\def\csname v@vint/cpu/fi-d\endcsname{+0.32}
\expandafter\def\csname v@vint/cpu/fi-dabs\endcsname{0.32}
\expandafter\def\csname v@vint/cpu/fi-dhi\endcsname{+0.47}
\expandafter\def\csname v@vint/cpu/fi-dlo\endcsname{+0.18}
\expandafter\def\csname v@vint/cpu/fi-hi\endcsname{1.88}
\expandafter\def\csname v@vint/cpu/fi-lo\endcsname{0.93}
\expandafter\def\csname v@vint/cpu/frame-p50\endcsname{8.3}
\expandafter\def\csname v@vint/cpu/frame-p99\endcsname{13.9}
\expandafter\def\csname v@vint/cpu/fs\endcsname{1.58}
\expandafter\def\csname v@vint/cpu/fs-d\endcsname{+0.35}
\expandafter\def\csname v@vint/cpu/fs-dabs\endcsname{0.35}
\expandafter\def\csname v@vint/cpu/fs-dhi\endcsname{+0.51}
\expandafter\def\csname v@vint/cpu/fs-dlo\endcsname{+0.20}
\expandafter\def\csname v@vint/cpu/fs-hi\endcsname{2.17}
\expandafter\def\csname v@vint/cpu/fs-lo\endcsname{1.05}
\expandafter\def\csname v@vint/cpu/held\endcsname{3.4}
\expandafter\def\csname v@vint/cpu/held-d\endcsname{-0.1}
\expandafter\def\csname v@vint/cpu/held-dabs\endcsname{0.1}
\expandafter\def\csname v@vint/cpu/held-dhi\endcsname{+0.5}
\expandafter\def\csname v@vint/cpu/held-dlo\endcsname{-0.7}
\expandafter\def\csname v@vint/cpu/held-hi\endcsname{5.4}
\expandafter\def\csname v@vint/cpu/held-lo\endcsname{1.7}
\expandafter\def\csname v@vint/cpu/kind/babble/fi\endcsname{1.52}
\expandafter\def\csname v@vint/cpu/kind/babble/fs\endcsname{1.72}
\expandafter\def\csname v@vint/cpu/kind/babble/missed\endcsname{0.0}
\expandafter\def\csname v@vint/cpu/kind/clean/fi\endcsname{0.00}
\expandafter\def\csname v@vint/cpu/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/cpu/kind/clean/missed\endcsname{0.0}
\expandafter\def\csname v@vint/cpu/kind/home/fi\endcsname{0.73}
\expandafter\def\csname v@vint/cpu/kind/home/fs\endcsname{0.81}
\expandafter\def\csname v@vint/cpu/kind/home/missed\endcsname{0.4}
\expandafter\def\csname v@vint/cpu/kind/music/fi\endcsname{0.50}
\expandafter\def\csname v@vint/cpu/kind/music/fs\endcsname{0.59}
\expandafter\def\csname v@vint/cpu/kind/music/missed\endcsname{0.0}
\expandafter\def\csname v@vint/cpu/kind/street/fi\endcsname{0.20}
\expandafter\def\csname v@vint/cpu/kind/street/fs\endcsname{0.19}
\expandafter\def\csname v@vint/cpu/kind/street/missed\endcsname{0.0}
\expandafter\def\csname v@vint/cpu/kind/talker/fi\endcsname{5.51}
\expandafter\def\csname v@vint/cpu/kind/talker/fs\endcsname{4.64}
\expandafter\def\csname v@vint/cpu/kind/talker/missed\endcsname{1.3}
\expandafter\def\csname v@vint/cpu/live/barge_p50\endcsname{0.67}
\expandafter\def\csname v@vint/cpu/live/caught\endcsname{90.3}
\expandafter\def\csname v@vint/cpu/live/eot_p50\endcsname{0.76}
\expandafter\def\csname v@vint/cpu/live/eot_p90\endcsname{1.55}
\expandafter\def\csname v@vint/cpu/live/fi_transcript\endcsname{4.22}
\expandafter\def\csname v@vint/cpu/live/fi_vad\endcsname{1.42}
\expandafter\def\csname v@vint/cpu/live/frame-p50\endcsname{10.9}
\expandafter\def\csname v@vint/cpu/live/frame-p99\endcsname{19.8}
\expandafter\def\csname v@vint/cpu/live/fs\endcsname{1.93}
\expandafter\def\csname v@vint/cpu/live/no_reply\endcsname{3.4}
\expandafter\def\csname v@vint/cpu/live/unfiltered_pct\endcsname{0.00}
\expandafter\def\csname v@vint/cpu/missed\endcsname{0.3}
\expandafter\def\csname v@vint/cpu/missed-d\endcsname{-0.3}
\expandafter\def\csname v@vint/cpu/missed-dabs\endcsname{0.3}
\expandafter\def\csname v@vint/cpu/missed-dhi\endcsname{-0.1}
\expandafter\def\csname v@vint/cpu/missed-dlo\endcsname{-0.6}
\expandafter\def\csname v@vint/cpu/missed-hi\endcsname{0.6}
\expandafter\def\csname v@vint/cpu/missed-lo\endcsname{0.1}
\expandafter\def\csname v@vint/cpu/recall\endcsname{93.4}
\expandafter\def\csname v@vint/cpu/snr/0.0/fi\endcsname{2.68}
\expandafter\def\csname v@vint/cpu/snr/10.0/fi\endcsname{1.22}
\expandafter\def\csname v@vint/cpu/snr/20.0/fi\endcsname{0.59}
\expandafter\def\csname v@vint/cpu/snr/None/fi\endcsname{0.00}
\expandafter\def\csname v@vint/cpu/wer\endcsname{11.8}
\expandafter\def\csname v@vint/cpu/wer/babble\endcsname{17.9}
\expandafter\def\csname v@vint/cpu/wer/clean\endcsname{1.1}
\expandafter\def\csname v@vint/cpu/wer/home\endcsname{12.4}
\expandafter\def\csname v@vint/cpu/wer/music\endcsname{9.1}
\expandafter\def\csname v@vint/cpu/wer/street\endcsname{8.4}
\expandafter\def\csname v@vint/cpu/wer/talker\endcsname{16.5}
\expandafter\def\csname v@vint/cpu_s1/live/barge_p50\endcsname{0.66}
\expandafter\def\csname v@vint/cpu_s1/live/caught\endcsname{90.0}
\expandafter\def\csname v@vint/cpu_s1/live/eot_p50\endcsname{0.79}
\expandafter\def\csname v@vint/cpu_s1/live/eot_p90\endcsname{1.55}
\expandafter\def\csname v@vint/cpu_s1/live/fi_transcript\endcsname{3.73}
\expandafter\def\csname v@vint/cpu_s1/live/fi_vad\endcsname{0.85}
\expandafter\def\csname v@vint/cpu_s1/live/frame-p50\endcsname{8.5}
\expandafter\def\csname v@vint/cpu_s1/live/frame-p99\endcsname{15.3}
\expandafter\def\csname v@vint/cpu_s1/live/fs\endcsname{1.63}
\expandafter\def\csname v@vint/cpu_s1/live/no_reply\endcsname{4.4}
\expandafter\def\csname v@vint/cpu_s1/live/unfiltered_pct\endcsname{0.00}
\expandafter\def\csname v@vint/cpu_s2/live/barge_p50\endcsname{0.66}
\expandafter\def\csname v@vint/cpu_s2/live/caught\endcsname{85.4}
\expandafter\def\csname v@vint/cpu_s2/live/eot_p50\endcsname{0.81}
\expandafter\def\csname v@vint/cpu_s2/live/eot_p90\endcsname{1.56}
\expandafter\def\csname v@vint/cpu_s2/live/fi_transcript\endcsname{3.57}
\expandafter\def\csname v@vint/cpu_s2/live/fi_vad\endcsname{1.53}
\expandafter\def\csname v@vint/cpu_s2/live/frame-p50\endcsname{8.5}
\expandafter\def\csname v@vint/cpu_s2/live/frame-p99\endcsname{15.7}
\expandafter\def\csname v@vint/cpu_s2/live/fs\endcsname{2.38}
\expandafter\def\csname v@vint/cpu_s2/live/no_reply\endcsname{4.9}
\expandafter\def\csname v@vint/cpu_s2/live/unfiltered_pct\endcsname{0.00}
\expandafter\def\csname v@vint/cpuagent/ckpt-step\endcsname{3,000}
\expandafter\def\csname v@vint/cpuagent/head-width\endcsname{256}
\expandafter\def\csname v@vint/cpuagent/hold-s\endcsname{0.3}
\expandafter\def\csname v@vint/cpuagent/rule/ckpt-step\endcsname{2,000}
\expandafter\def\csname v@vint/cpuagent/rule/hold-s\endcsname{0.5}
\expandafter\def\csname v@vint/cpuagent/rule/theta\endcsname{0.9}
\expandafter\def\csname v@vint/cpuagent/rule/theta-off\endcsname{0.3}
\expandafter\def\csname v@vint/cpuagent/steps\endcsname{3,000}
\expandafter\def\csname v@vint/cpuagent/theta\endcsname{0.9}
\expandafter\def\csname v@vint/cpuagent/theta-off\endcsname{0.2}
\expandafter\def\csname v@vint/cpuagent/w-gate\endcsname{5}
\expandafter\def\csname v@vint/cpugate/agent/after\endcsname{0.20}
\expandafter\def\csname v@vint/cpugate/agent/after-hi\endcsname{0.35}
\expandafter\def\csname v@vint/cpugate/agent/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/cpugate/agent/all\endcsname{0.54}
\expandafter\def\csname v@vint/cpugate/agent/all-hi\endcsname{0.79}
\expandafter\def\csname v@vint/cpugate/agent/all-lo\endcsname{0.33}
\expandafter\def\csname v@vint/cpugate/agent/greet\endcsname{3.22}
\expandafter\def\csname v@vint/cpugate/agent/greet-hi\endcsname{4.58}
\expandafter\def\csname v@vint/cpugate/agent/greet-lo\endcsname{1.98}
\expandafter\def\csname v@vint/cpugate/calls\endcsname{816}
\expandafter\def\csname v@vint/cpugate/core/cpu\endcsname{17}
\expandafter\def\csname v@vint/cpugate/core/cpu8\endcsname{12}
\expandafter\def\csname v@vint/cpugate/core/cpuag\endcsname{17}
\expandafter\def\csname v@vint/cpugate/core/cpuag8\endcsname{13}
\expandafter\def\csname v@vint/cpugate/core/cpuag_off\endcsname{17}
\expandafter\def\csname v@vint/cpugate/core/cpuag_off8\endcsname{12}
\expandafter\def\csname v@vint/cpugate/cpu/after\endcsname{0.80}
\expandafter\def\csname v@vint/cpugate/cpu/after-hi\endcsname{1.23}
\expandafter\def\csname v@vint/cpugate/cpu/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/cpugate/cpu/all\endcsname{1.36}
\expandafter\def\csname v@vint/cpugate/cpu/all-hi\endcsname{1.87}
\expandafter\def\csname v@vint/cpugate/cpu/all-lo\endcsname{0.92}
\expandafter\def\csname v@vint/cpugate/cpu/greet\endcsname{5.74}
\expandafter\def\csname v@vint/cpugate/cpu/greet-hi\endcsname{7.39}
\expandafter\def\csname v@vint/cpugate/cpu/greet-lo\endcsname{4.18}
\expandafter\def\csname v@vint/cpugate/cpu8/after\endcsname{0.80}
\expandafter\def\csname v@vint/cpugate/cpu8/after-hi\endcsname{1.24}
\expandafter\def\csname v@vint/cpugate/cpu8/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/cpugate/cpu8/all\endcsname{1.36}
\expandafter\def\csname v@vint/cpugate/cpu8/all-hi\endcsname{1.88}
\expandafter\def\csname v@vint/cpugate/cpu8/all-lo\endcsname{0.93}
\expandafter\def\csname v@vint/cpugate/cpu8/greet\endcsname{5.77}
\expandafter\def\csname v@vint/cpugate/cpu8/greet-hi\endcsname{7.41}
\expandafter\def\csname v@vint/cpugate/cpu8/greet-lo\endcsname{4.21}
\expandafter\def\csname v@vint/cpugate/cpuag/after\endcsname{0.14}
\expandafter\def\csname v@vint/cpugate/cpuag/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/cpugate/cpuag/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/cpugate/cpuag/all\endcsname{0.48}
\expandafter\def\csname v@vint/cpugate/cpuag/all-hi\endcsname{0.71}
\expandafter\def\csname v@vint/cpugate/cpuag/all-lo\endcsname{0.29}
\expandafter\def\csname v@vint/cpugate/cpuag/greet\endcsname{3.14}
\expandafter\def\csname v@vint/cpugate/cpuag/greet-hi\endcsname{4.45}
\expandafter\def\csname v@vint/cpugate/cpuag/greet-lo\endcsname{1.94}
\expandafter\def\csname v@vint/cpugate/cpuag8/after\endcsname{0.14}
\expandafter\def\csname v@vint/cpugate/cpuag8/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/cpugate/cpuag8/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/cpugate/cpuag8/all\endcsname{0.48}
\expandafter\def\csname v@vint/cpugate/cpuag8/all-hi\endcsname{0.71}
\expandafter\def\csname v@vint/cpugate/cpuag8/all-lo\endcsname{0.29}
\expandafter\def\csname v@vint/cpugate/cpuag8/greet\endcsname{3.14}
\expandafter\def\csname v@vint/cpugate/cpuag8/greet-hi\endcsname{4.45}
\expandafter\def\csname v@vint/cpugate/cpuag8/greet-lo\endcsname{1.94}
\expandafter\def\csname v@vint/cpugate/dev/c22j20/after\endcsname{0.64}
\expandafter\def\csname v@vint/cpugate/dev/c22j20/all\endcsname{1.22}
\expandafter\def\csname v@vint/cpugate/dev/c22j20/cut\endcsname{91.9}
\expandafter\def\csname v@vint/cpugate/dev/c22j20/missed\endcsname{0.16}
\expandafter\def\csname v@vint/cpugate/dev/c22j20/wer\endcsname{15.23}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h100_o20_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h100_o20_k1/all\endcsname{0.62}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h100_o20_k1/cut\endcsname{89.1}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h100_o20_k1/missed\endcsname{2.76}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h100_o20_k1/wer\endcsname{17.68}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h30_o20_k1/after\endcsname{0.11}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h30_o20_k1/all\endcsname{0.54}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h30_o20_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h30_o20_k1/missed\endcsname{3.00}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h30_o20_k1/wer\endcsname{19.82}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o20_k1/after\endcsname{0.13}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o20_k1/all\endcsname{0.56}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o20_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o20_k1/missed\endcsname{2.90}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o20_k1/wer\endcsname{19.18}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o30_k1/after\endcsname{0.12}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o30_k1/all\endcsname{0.55}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o30_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o30_k1/missed\endcsname{3.00}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t90_h50_o30_k1/wer\endcsname{19.49}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t95_h50_o20_k1/after\endcsname{0.13}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t95_h50_o20_k1/all\endcsname{0.52}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t95_h50_o20_k1/cut\endcsname{88.4}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t95_h50_o20_k1/missed\endcsname{4.20}
\expandafter\def\csname v@vint/cpugate/dev/c22j20g_t95_h50_o20_k1/wer\endcsname{19.63}
\expandafter\def\csname v@vint/cpugate/dev/c22j30/after\endcsname{0.67}
\expandafter\def\csname v@vint/cpugate/dev/c22j30/all\endcsname{1.23}
\expandafter\def\csname v@vint/cpugate/dev/c22j30/cut\endcsname{91.9}
\expandafter\def\csname v@vint/cpugate/dev/c22j30/missed\endcsname{0.16}
\expandafter\def\csname v@vint/cpugate/dev/c22j30/wer\endcsname{15.23}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h100_o20_k1/after\endcsname{0.20}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h100_o20_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h100_o20_k1/cut\endcsname{89.2}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h100_o20_k1/missed\endcsname{2.37}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h100_o20_k1/wer\endcsname{19.04}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h30_o20_k1/after\endcsname{0.11}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h30_o20_k1/all\endcsname{0.54}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h30_o20_k1/cut\endcsname{88.9}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h30_o20_k1/missed\endcsname{2.66}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h30_o20_k1/wer\endcsname{20.90}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o20_k1/after\endcsname{0.14}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o20_k1/all\endcsname{0.56}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o20_k1/cut\endcsname{88.9}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o20_k1/missed\endcsname{2.55}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o20_k1/wer\endcsname{20.27}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o30_k1/after\endcsname{0.13}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o30_k1/all\endcsname{0.54}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o30_k1/cut\endcsname{88.9}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o30_k1/missed\endcsname{2.64}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t90_h50_o30_k1/wer\endcsname{20.57}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t95_h50_o20_k1/after\endcsname{0.13}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t95_h50_o20_k1/all\endcsname{0.53}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t95_h50_o20_k1/cut\endcsname{87.9}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t95_h50_o20_k1/missed\endcsname{4.26}
\expandafter\def\csname v@vint/cpugate/dev/c22j30g_t95_h50_o20_k1/wer\endcsname{20.32}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10/after\endcsname{0.68}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10/all\endcsname{1.26}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10/cut\endcsname{91.8}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10/missed\endcsname{0.18}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10/wer\endcsname{15.04}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h100_o20_k1/after\endcsname{0.25}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h100_o20_k1/all\endcsname{0.67}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h100_o20_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h100_o20_k1/missed\endcsname{2.19}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h100_o20_k1/wer\endcsname{17.47}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h30_o20_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h30_o20_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h30_o20_k1/cut\endcsname{89.4}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h30_o20_k1/missed\endcsname{2.51}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h30_o20_k1/wer\endcsname{18.64}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o20_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o20_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o20_k1/cut\endcsname{89.4}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o20_k1/missed\endcsname{2.39}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o20_k1/wer\endcsname{18.16}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o30_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o30_k1/all\endcsname{0.59}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o30_k1/cut\endcsname{89.4}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o30_k1/missed\endcsname{2.41}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t90_h50_o30_k1/wer\endcsname{18.47}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t95_h50_o20_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t95_h50_o20_k1/all\endcsname{0.55}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t95_h50_o20_k1/cut\endcsname{88.9}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t95_h50_o20_k1/missed\endcsname{3.22}
\expandafter\def\csname v@vint/cpugate/dev/c22jh10g_t95_h50_o20_k1/wer\endcsname{19.08}
\expandafter\def\csname v@vint/cpugate/dev/c22kd/after\endcsname{0.61}
\expandafter\def\csname v@vint/cpugate/dev/c22kd/all\endcsname{1.22}
\expandafter\def\csname v@vint/cpugate/dev/c22kd/cut\endcsname{91.2}
\expandafter\def\csname v@vint/cpugate/dev/c22kd/missed\endcsname{0.61}
\expandafter\def\csname v@vint/cpugate/dev/c22kd/wer\endcsname{15.44}
\expandafter\def\csname v@vint/cpugate/dev/calls\endcsname{480}
\expandafter\def\csname v@vint/cpugate/dev/none/after\endcsname{2.02}
\expandafter\def\csname v@vint/cpugate/dev/none/all\endcsname{2.39}
\expandafter\def\csname v@vint/cpugate/dev/none/cut\endcsname{86.6}
\expandafter\def\csname v@vint/cpugate/dev/none/missed\endcsname{0.36}
\expandafter\def\csname v@vint/cpugate/dev/reuse8/after\endcsname{0.19}
\expandafter\def\csname v@vint/cpugate/dev/reuse8/all\endcsname{0.89}
\expandafter\def\csname v@vint/cpugate/dev/reuse8/cut\endcsname{88.5}
\expandafter\def\csname v@vint/cpugate/dev/reuse8/missed\endcsname{3.02}
\expandafter\def\csname v@vint/cpugate/dev/reuse8/wer\endcsname{20.52}
\expandafter\def\csname v@vint/cpugate/dev/vbj15g_t90_h100_o20_k1/after\endcsname{0.14}
\expandafter\def\csname v@vint/cpugate/dev/vbj15g_t90_h100_o20_k1/all\endcsname{0.54}
\expandafter\def\csname v@vint/cpugate/dev/vbj15g_t90_h100_o20_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/cpugate/dev/vbj15g_t90_h100_o20_k1/missed\endcsname{2.05}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-agent/after\endcsname{-0.06}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-agent/after-hi\endcsname{-0.02}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-agent/after-lo\endcsname{-0.11}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-agent/all\endcsname{-0.06}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-agent/all-hi\endcsname{-0.01}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-agent/all-lo\endcsname{-0.12}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-agent/greet\endcsname{-0.08}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-agent/greet-hi\endcsname{+0.17}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-agent/greet-lo\endcsname{-0.37}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-cpu/after\endcsname{-0.66}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-cpu/after-hi\endcsname{-0.37}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-cpu/after-lo\endcsname{-1.00}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-cpu/all\endcsname{-0.88}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-cpu/all-hi\endcsname{-0.58}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-cpu/all-lo\endcsname{-1.23}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-cpu/greet\endcsname{-2.60}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-cpu/greet-hi\endcsname{-1.86}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-cpu/greet-lo\endcsname{-3.38}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-reuse/after\endcsname{-0.10}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-reuse/after-hi\endcsname{+0.01}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-reuse/after-lo\endcsname{-0.23}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-reuse/all\endcsname{-0.47}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-reuse/all-hi\endcsname{-0.30}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-reuse/all-lo\endcsname{-0.66}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-reuse/greet\endcsname{-3.41}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-reuse/greet-hi\endcsname{-2.38}
\expandafter\def\csname v@vint/cpugate/diff/cpuag-reuse/greet-lo\endcsname{-4.51}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-agent/after\endcsname{-0.06}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-agent/after-hi\endcsname{-0.02}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-agent/after-lo\endcsname{-0.10}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-agent/all\endcsname{-0.06}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-agent/all-hi\endcsname{-0.01}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-agent/all-lo\endcsname{-0.12}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-agent/greet\endcsname{-0.08}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-agent/greet-hi\endcsname{+0.17}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-agent/greet-lo\endcsname{-0.37}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpu8/after\endcsname{-0.66}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpu8/after-hi\endcsname{-0.38}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpu8/after-lo\endcsname{-1.01}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpu8/all\endcsname{-0.89}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpu8/all-hi\endcsname{-0.58}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpu8/all-lo\endcsname{-1.24}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpu8/greet\endcsname{-2.63}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpu8/greet-hi\endcsname{-1.90}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpu8/greet-lo\endcsname{-3.41}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpuag/after\endcsname{+0.00}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpuag/after-hi\endcsname{+0.01}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpuag/after-lo\endcsname{-0.01}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpuag/all\endcsname{+0.00}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpuag/all-hi\endcsname{+0.01}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpuag/all-lo\endcsname{-0.01}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpuag/greet\endcsname{+0.00}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpuag/greet-hi\endcsname{+0.03}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-cpuag/greet-lo\endcsname{-0.03}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-reuse/after\endcsname{-0.10}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-reuse/after-hi\endcsname{+0.01}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-reuse/after-lo\endcsname{-0.22}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-reuse/all\endcsname{-0.47}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-reuse/all-hi\endcsname{-0.30}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-reuse/all-lo\endcsname{-0.67}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-reuse/greet\endcsname{-3.41}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-reuse/greet-hi\endcsname{-2.38}
\expandafter\def\csname v@vint/cpugate/diff/cpuag8-reuse/greet-lo\endcsname{-4.50}
\expandafter\def\csname v@vint/cpugate/export/fp32-calls\endcsname{4}
\expandafter\def\csname v@vint/cpugate/export/fp32-differ\endcsname{0.00}
\expandafter\def\csname v@vint/cpugate/export/fp32-snr-min\endcsname{105}
\expandafter\def\csname v@vint/cpugate/export/int8-calls\endcsname{4}
\expandafter\def\csname v@vint/cpugate/export/int8-differ\endcsname{0.00}
\expandafter\def\csname v@vint/cpugate/export/int8-snr-min\endcsname{35}
\expandafter\def\csname v@vint/cpugate/none/after\endcsname{2.42}
\expandafter\def\csname v@vint/cpugate/none/after-hi\endcsname{3.29}
\expandafter\def\csname v@vint/cpugate/none/after-lo\endcsname{1.64}
\expandafter\def\csname v@vint/cpugate/none/all\endcsname{2.77}
\expandafter\def\csname v@vint/cpugate/none/all-hi\endcsname{3.73}
\expandafter\def\csname v@vint/cpugate/none/all-lo\endcsname{1.91}
\expandafter\def\csname v@vint/cpugate/none/greet\endcsname{5.52}
\expandafter\def\csname v@vint/cpugate/none/greet-hi\endcsname{7.39}
\expandafter\def\csname v@vint/cpugate/none/greet-lo\endcsname{3.80}
\expandafter\def\csname v@vint/cpugate/reuse/after\endcsname{0.24}
\expandafter\def\csname v@vint/cpugate/reuse/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/cpugate/reuse/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/cpugate/reuse/all\endcsname{0.95}
\expandafter\def\csname v@vint/cpugate/reuse/all-hi\endcsname{1.30}
\expandafter\def\csname v@vint/cpugate/reuse/all-lo\endcsname{0.63}
\expandafter\def\csname v@vint/cpugate/reuse/greet\endcsname{6.54}
\expandafter\def\csname v@vint/cpugate/reuse/greet-hi\endcsname{8.46}
\expandafter\def\csname v@vint/cpugate/reuse/greet-lo\endcsname{4.71}
\expandafter\def\csname v@vint/cpugate/silence/agent/missed\endcsname{2.7}
\expandafter\def\csname v@vint/cpugate/silence/agent/recall\endcsname{88.4}
\expandafter\def\csname v@vint/cpugate/silence/agent/wer\endcsname{15.6}
\expandafter\def\csname v@vint/cpugate/silence/cpu/missed\endcsname{0.3}
\expandafter\def\csname v@vint/cpugate/silence/cpu/recall\endcsname{93.4}
\expandafter\def\csname v@vint/cpugate/silence/cpu/wer\endcsname{11.9}
\expandafter\def\csname v@vint/cpugate/silence/cpu8/missed\endcsname{0.3}
\expandafter\def\csname v@vint/cpugate/silence/cpu8/recall\endcsname{93.4}
\expandafter\def\csname v@vint/cpugate/silence/cpu8/wer\endcsname{11.8}
\expandafter\def\csname v@vint/cpugate/silence/cpuag/missed\endcsname{2.4}
\expandafter\def\csname v@vint/cpugate/silence/cpuag/recall\endcsname{88.7}
\expandafter\def\csname v@vint/cpugate/silence/cpuag/wer\endcsname{16.0}
\expandafter\def\csname v@vint/cpugate/silence/cpuag8/missed\endcsname{2.4}
\expandafter\def\csname v@vint/cpugate/silence/cpuag8/recall\endcsname{88.7}
\expandafter\def\csname v@vint/cpugate/silence/cpuag8/wer\endcsname{16.2}
\expandafter\def\csname v@vint/cpugate/silence/none/missed\endcsname{0.4}
\expandafter\def\csname v@vint/cpugate/silence/none/recall\endcsname{94.4}
\expandafter\def\csname v@vint/cpugate/silence/none/wer\endcsname{7.4}
\expandafter\def\csname v@vint/cpugate/silence/reuse/missed\endcsname{2.6}
\expandafter\def\csname v@vint/cpugate/silence/reuse/recall\endcsname{87.2}
\expandafter\def\csname v@vint/cpugate/silence/reuse/wer\endcsname{16.9}
\expandafter\def\csname v@vint/cpugate/test/agent/cut\endcsname{84.8}
\expandafter\def\csname v@vint/cpugate/test/cpu/cut\endcsname{91.2}
\expandafter\def\csname v@vint/cpugate/test/cpu8/cut\endcsname{91.0}
\expandafter\def\csname v@vint/cpugate/test/cpuag/cut\endcsname{87.9}
\expandafter\def\csname v@vint/cpugate/test/cpuag8/cut\endcsname{87.9}
\expandafter\def\csname v@vint/cpugate/test/none/cut\endcsname{84.8}
\expandafter\def\csname v@vint/cpugate/test/reuse/cut\endcsname{87.4}
\expandafter\def\csname v@vint/dev/arm_absent/fi\endcsname{0.74}
\expandafter\def\csname v@vint/dev/arm_absent/fs\endcsname{0.76}
\expandafter\def\csname v@vint/dev/arm_absent/kind/babble/fs\endcsname{0.15}
\expandafter\def\csname v@vint/dev/arm_absent/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/arm_absent/kind/home/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/arm_absent/kind/music/fs\endcsname{0.30}
\expandafter\def\csname v@vint/dev/arm_absent/kind/street/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/arm_absent/kind/talker/fs\endcsname{2.69}
\expandafter\def\csname v@vint/dev/arm_absent/missed\endcsname{0.6}
\expandafter\def\csname v@vint/dev/arm_absent/wer\endcsname{18.4}
\expandafter\def\csname v@vint/dev/arm_all/fi\endcsname{0.63}
\expandafter\def\csname v@vint/dev/arm_all/fs\endcsname{0.67}
\expandafter\def\csname v@vint/dev/arm_all/kind/babble/fs\endcsname{0.15}
\expandafter\def\csname v@vint/dev/arm_all/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/arm_all/kind/home/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/arm_all/kind/music/fs\endcsname{0.75}
\expandafter\def\csname v@vint/dev/arm_all/kind/street/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/arm_all/kind/talker/fs\endcsname{2.05}
\expandafter\def\csname v@vint/dev/arm_all/missed\endcsname{0.6}
\expandafter\def\csname v@vint/dev/arm_all/wer\endcsname{20.6}
\expandafter\def\csname v@vint/dev/arm_music/fi\endcsname{1.00}
\expandafter\def\csname v@vint/dev/arm_music/fs\endcsname{1.17}
\expandafter\def\csname v@vint/dev/arm_music/kind/babble/fs\endcsname{0.61}
\expandafter\def\csname v@vint/dev/arm_music/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/arm_music/kind/home/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/arm_music/kind/music/fs\endcsname{0.75}
\expandafter\def\csname v@vint/dev/arm_music/kind/street/fs\endcsname{0.34}
\expandafter\def\csname v@vint/dev/arm_music/kind/talker/fs\endcsname{3.59}
\expandafter\def\csname v@vint/dev/arm_music/missed\endcsname{0.3}
\expandafter\def\csname v@vint/dev/arm_music/wer\endcsname{16.2}
\expandafter\def\csname v@vint/dev/arm_silence/fi\endcsname{1.00}
\expandafter\def\csname v@vint/dev/arm_silence/fs\endcsname{1.08}
\expandafter\def\csname v@vint/dev/arm_silence/kind/babble/fs\endcsname{0.46}
\expandafter\def\csname v@vint/dev/arm_silence/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/arm_silence/kind/home/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/arm_silence/kind/music/fs\endcsname{0.75}
\expandafter\def\csname v@vint/dev/arm_silence/kind/street/fs\endcsname{0.34}
\expandafter\def\csname v@vint/dev/arm_silence/kind/talker/fs\endcsname{3.33}
\expandafter\def\csname v@vint/dev/arm_silence/missed\endcsname{0.3}
\expandafter\def\csname v@vint/dev/arm_silence/wer\endcsname{16.6}
\expandafter\def\csname v@vint/dev/calls\endcsname{32}
\expandafter\def\csname v@vint/dev/cpu/fi\endcsname{0.95}
\expandafter\def\csname v@vint/dev/cpu/fs\endcsname{1.43}
\expandafter\def\csname v@vint/dev/cpu/kind/babble/fs\endcsname{1.23}
\expandafter\def\csname v@vint/dev/cpu/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/cpu/kind/home/fs\endcsname{1.04}
\expandafter\def\csname v@vint/dev/cpu/kind/music/fs\endcsname{0.60}
\expandafter\def\csname v@vint/dev/cpu/kind/street/fs\endcsname{0.69}
\expandafter\def\csname v@vint/dev/cpu/kind/talker/fs\endcsname{3.46}
\expandafter\def\csname v@vint/dev/cpu/missed\endcsname{0.0}
\expandafter\def\csname v@vint/dev/cpu/wer\endcsname{15.2}
\expandafter\def\csname v@vint/dev/ft/fi\endcsname{0.84}
\expandafter\def\csname v@vint/dev/ft/fs\endcsname{0.88}
\expandafter\def\csname v@vint/dev/ft/kind/babble/fs\endcsname{0.46}
\expandafter\def\csname v@vint/dev/ft/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/ft/kind/home/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/ft/kind/music/fs\endcsname{0.45}
\expandafter\def\csname v@vint/dev/ft/kind/street/fs\endcsname{0.34}
\expandafter\def\csname v@vint/dev/ft/kind/talker/fs\endcsname{2.69}
\expandafter\def\csname v@vint/dev/ft/missed\endcsname{0.0}
\expandafter\def\csname v@vint/dev/ft/wer\endcsname{15.3}
\expandafter\def\csname v@vint/dev/ft2500/fi\endcsname{0.89}
\expandafter\def\csname v@vint/dev/ft2500/fs\endcsname{0.94}
\expandafter\def\csname v@vint/dev/ft2500/kind/babble/fs\endcsname{0.46}
\expandafter\def\csname v@vint/dev/ft2500/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/ft2500/kind/home/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/ft2500/kind/music/fs\endcsname{0.60}
\expandafter\def\csname v@vint/dev/ft2500/kind/street/fs\endcsname{0.34}
\expandafter\def\csname v@vint/dev/ft2500/kind/talker/fs\endcsname{2.82}
\expandafter\def\csname v@vint/dev/ft2500/missed\endcsname{0.0}
\expandafter\def\csname v@vint/dev/ft2500/wer\endcsname{15.3}
\expandafter\def\csname v@vint/dev/ft_oracle/fi\endcsname{0.37}
\expandafter\def\csname v@vint/dev/ft_oracle/fs\endcsname{0.61}
\expandafter\def\csname v@vint/dev/ft_oracle/kind/babble/fs\endcsname{0.15}
\expandafter\def\csname v@vint/dev/ft_oracle/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/ft_oracle/kind/home/fs\endcsname{0.35}
\expandafter\def\csname v@vint/dev/ft_oracle/kind/music/fs\endcsname{0.30}
\expandafter\def\csname v@vint/dev/ft_oracle/kind/street/fs\endcsname{0.34}
\expandafter\def\csname v@vint/dev/ft_oracle/kind/talker/fs\endcsname{1.79}
\expandafter\def\csname v@vint/dev/ft_oracle/missed\endcsname{0.3}
\expandafter\def\csname v@vint/dev/ft_skip/fi\endcsname{0.84}
\expandafter\def\csname v@vint/dev/ft_skip/fs\endcsname{0.94}
\expandafter\def\csname v@vint/dev/ft_skip/kind/babble/fs\endcsname{0.46}
\expandafter\def\csname v@vint/dev/ft_skip/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/ft_skip/kind/home/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/ft_skip/kind/music/fs\endcsname{0.45}
\expandafter\def\csname v@vint/dev/ft_skip/kind/street/fs\endcsname{0.34}
\expandafter\def\csname v@vint/dev/ft_skip/kind/talker/fs\endcsname{2.95}
\expandafter\def\csname v@vint/dev/ft_skip/missed\endcsname{0.0}
\expandafter\def\csname v@vint/dev/ft_skip/wer\endcsname{15.3}
\expandafter\def\csname v@vint/dev/none/fi\endcsname{2.47}
\expandafter\def\csname v@vint/dev/none/fs\endcsname{2.96}
\expandafter\def\csname v@vint/dev/none/kind/babble/fs\endcsname{2.15}
\expandafter\def\csname v@vint/dev/none/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/none/kind/home/fs\endcsname{0.87}
\expandafter\def\csname v@vint/dev/none/kind/music/fs\endcsname{1.49}
\expandafter\def\csname v@vint/dev/none/kind/street/fs\endcsname{1.72}
\expandafter\def\csname v@vint/dev/none/kind/talker/fs\endcsname{7.94}
\expandafter\def\csname v@vint/dev/none/missed\endcsname{0.0}
\expandafter\def\csname v@vint/dev/none/wer\endcsname{11.2}
\expandafter\def\csname v@vint/dev/rel/fi\endcsname{1.10}
\expandafter\def\csname v@vint/dev/rel/fs\endcsname{1.32}
\expandafter\def\csname v@vint/dev/rel/kind/babble/fs\endcsname{0.61}
\expandafter\def\csname v@vint/dev/rel/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/rel/kind/home/fs\endcsname{0.35}
\expandafter\def\csname v@vint/dev/rel/kind/music/fs\endcsname{0.60}
\expandafter\def\csname v@vint/dev/rel/kind/street/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/rel/kind/talker/fs\endcsname{4.36}
\expandafter\def\csname v@vint/dev/rel/missed\endcsname{0.3}
\expandafter\def\csname v@vint/dev/rel/wer\endcsname{16.8}
\expandafter\def\csname v@vint/dev/rel_oracle/fi\endcsname{0.37}
\expandafter\def\csname v@vint/dev/rel_oracle/fs\endcsname{0.61}
\expandafter\def\csname v@vint/dev/rel_oracle/kind/babble/fs\endcsname{0.15}
\expandafter\def\csname v@vint/dev/rel_oracle/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/rel_oracle/kind/home/fs\endcsname{0.35}
\expandafter\def\csname v@vint/dev/rel_oracle/kind/music/fs\endcsname{0.30}
\expandafter\def\csname v@vint/dev/rel_oracle/kind/street/fs\endcsname{0.17}
\expandafter\def\csname v@vint/dev/rel_oracle/kind/talker/fs\endcsname{1.92}
\expandafter\def\csname v@vint/dev/rel_oracle/missed\endcsname{0.0}
\expandafter\def\csname v@vint/dev/rel_oracle/wer\endcsname{15.8}
\expandafter\def\csname v@vint/dev/reuse/fi\endcsname{1.00}
\expandafter\def\csname v@vint/dev/reuse/fs\endcsname{1.05}
\expandafter\def\csname v@vint/dev/reuse/kind/babble/fs\endcsname{0.77}
\expandafter\def\csname v@vint/dev/reuse/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/reuse/kind/home/fs\endcsname{0.52}
\expandafter\def\csname v@vint/dev/reuse/kind/music/fs\endcsname{0.00}
\expandafter\def\csname v@vint/dev/reuse/kind/street/fs\endcsname{0.86}
\expandafter\def\csname v@vint/dev/reuse/kind/talker/fs\endcsname{2.95}
\expandafter\def\csname v@vint/dev/reuse/missed\endcsname{3.9}
\expandafter\def\csname v@vint/dev/reuse/wer\endcsname{20.1}
\expandafter\def\csname v@vint/ft/caught\endcsname{89.7}
\expandafter\def\csname v@vint/ft/caught-d\endcsname{-0.2}
\expandafter\def\csname v@vint/ft/caught-dabs\endcsname{0.2}
\expandafter\def\csname v@vint/ft/caught-dhi\endcsname{+0.2}
\expandafter\def\csname v@vint/ft/caught-dlo\endcsname{-0.5}
\expandafter\def\csname v@vint/ft/caught-hi\endcsname{91.3}
\expandafter\def\csname v@vint/ft/caught-lo\endcsname{88.0}
\expandafter\def\csname v@vint/ft/fi\endcsname{0.86}
\expandafter\def\csname v@vint/ft/fi-d\endcsname{-0.19}
\expandafter\def\csname v@vint/ft/fi-dabs\endcsname{0.19}
\expandafter\def\csname v@vint/ft/fi-dhi\endcsname{-0.10}
\expandafter\def\csname v@vint/ft/fi-dlo\endcsname{-0.30}
\expandafter\def\csname v@vint/ft/fi-hi\endcsname{1.21}
\expandafter\def\csname v@vint/ft/fi-lo\endcsname{0.56}
\expandafter\def\csname v@vint/ft/fs\endcsname{1.03}
\expandafter\def\csname v@vint/ft/fs-d\endcsname{-0.20}
\expandafter\def\csname v@vint/ft/fs-dabs\endcsname{0.20}
\expandafter\def\csname v@vint/ft/fs-dhi\endcsname{-0.08}
\expandafter\def\csname v@vint/ft/fs-dlo\endcsname{-0.35}
\expandafter\def\csname v@vint/ft/fs-hi\endcsname{1.47}
\expandafter\def\csname v@vint/ft/fs-lo\endcsname{0.65}
\expandafter\def\csname v@vint/ft/held\endcsname{3.3}
\expandafter\def\csname v@vint/ft/held-d\endcsname{-0.2}
\expandafter\def\csname v@vint/ft/held-dabs\endcsname{0.2}
\expandafter\def\csname v@vint/ft/held-dhi\endcsname{+0.4}
\expandafter\def\csname v@vint/ft/held-dlo\endcsname{-0.7}
\expandafter\def\csname v@vint/ft/held-hi\endcsname{5.0}
\expandafter\def\csname v@vint/ft/held-lo\endcsname{1.9}
\expandafter\def\csname v@vint/ft/kind/babble/fi\endcsname{0.76}
\expandafter\def\csname v@vint/ft/kind/babble/fs\endcsname{0.84}
\expandafter\def\csname v@vint/ft/kind/babble/missed\endcsname{0.3}
\expandafter\def\csname v@vint/ft/kind/clean/fi\endcsname{0.00}
\expandafter\def\csname v@vint/ft/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/ft/kind/clean/missed\endcsname{0.4}
\expandafter\def\csname v@vint/ft/kind/home/fi\endcsname{0.45}
\expandafter\def\csname v@vint/ft/kind/home/fs\endcsname{0.54}
\expandafter\def\csname v@vint/ft/kind/home/missed\endcsname{0.5}
\expandafter\def\csname v@vint/ft/kind/music/fi\endcsname{0.27}
\expandafter\def\csname v@vint/ft/kind/music/fs\endcsname{0.28}
\expandafter\def\csname v@vint/ft/kind/music/missed\endcsname{0.1}
\expandafter\def\csname v@vint/ft/kind/street/fi\endcsname{0.07}
\expandafter\def\csname v@vint/ft/kind/street/fs\endcsname{0.09}
\expandafter\def\csname v@vint/ft/kind/street/missed\endcsname{0.3}
\expandafter\def\csname v@vint/ft/kind/talker/fi\endcsname{3.88}
\expandafter\def\csname v@vint/ft/kind/talker/fs\endcsname{3.39}
\expandafter\def\csname v@vint/ft/kind/talker/missed\endcsname{1.7}
\expandafter\def\csname v@vint/ft/live/barge_p50\endcsname{0.75}
\expandafter\def\csname v@vint/ft/live/caught\endcsname{85.6}
\expandafter\def\csname v@vint/ft/live/eot_p50\endcsname{0.82}
\expandafter\def\csname v@vint/ft/live/eot_p90\endcsname{1.62}
\expandafter\def\csname v@vint/ft/live/fi_transcript\endcsname{3.85}
\expandafter\def\csname v@vint/ft/live/fi_vad\endcsname{0.92}
\expandafter\def\csname v@vint/ft/live/frame-p50\endcsname{0.2}
\expandafter\def\csname v@vint/ft/live/frame-p99\endcsname{25.6}
\expandafter\def\csname v@vint/ft/live/fs\endcsname{1.17}
\expandafter\def\csname v@vint/ft/live/no_reply\endcsname{2.9}
\expandafter\def\csname v@vint/ft/live/unfiltered_pct\endcsname{0.11}
\expandafter\def\csname v@vint/ft/missed\endcsname{0.6}
\expandafter\def\csname v@vint/ft/missed-d\endcsname{-0.1}
\expandafter\def\csname v@vint/ft/missed-dabs\endcsname{0.1}
\expandafter\def\csname v@vint/ft/missed-dhi\endcsname{+0.1}
\expandafter\def\csname v@vint/ft/missed-dlo\endcsname{-0.3}
\expandafter\def\csname v@vint/ft/missed-hi\endcsname{0.9}
\expandafter\def\csname v@vint/ft/missed-lo\endcsname{0.3}
\expandafter\def\csname v@vint/ft/recall\endcsname{91.1}
\expandafter\def\csname v@vint/ft/snr/0.0/fi\endcsname{1.65}
\expandafter\def\csname v@vint/ft/snr/10.0/fi\endcsname{0.65}
\expandafter\def\csname v@vint/ft/snr/20.0/fi\endcsname{0.52}
\expandafter\def\csname v@vint/ft/snr/None/fi\endcsname{0.00}
\expandafter\def\csname v@vint/ft/wer\endcsname{13.0}
\expandafter\def\csname v@vint/ft/wer/babble\endcsname{18.2}
\expandafter\def\csname v@vint/ft/wer/clean\endcsname{4.2}
\expandafter\def\csname v@vint/ft/wer/home\endcsname{13.5}
\expandafter\def\csname v@vint/ft/wer/music\endcsname{10.4}
\expandafter\def\csname v@vint/ft/wer/street\endcsname{10.2}
\expandafter\def\csname v@vint/ft/wer/talker\endcsname{16.9}
\expandafter\def\csname v@vint/ft_s2/live/barge_p50\endcsname{0.76}
\expandafter\def\csname v@vint/ft_s2/live/caught\endcsname{91.3}
\expandafter\def\csname v@vint/ft_s2/live/eot_p50\endcsname{0.86}
\expandafter\def\csname v@vint/ft_s2/live/eot_p90\endcsname{1.64}
\expandafter\def\csname v@vint/ft_s2/live/fi_transcript\endcsname{3.41}
\expandafter\def\csname v@vint/ft_s2/live/fi_vad\endcsname{1.14}
\expandafter\def\csname v@vint/ft_s2/live/frame-p50\endcsname{0.2}
\expandafter\def\csname v@vint/ft_s2/live/frame-p99\endcsname{30.3}
\expandafter\def\csname v@vint/ft_s2/live/fs\endcsname{1.53}
\expandafter\def\csname v@vint/ft_s2/live/no_reply\endcsname{2.9}
\expandafter\def\csname v@vint/ft_s2/live/unfiltered_pct\endcsname{5.83}
\expandafter\def\csname v@vint/gate/agent/after\endcsname{0.20}
\expandafter\def\csname v@vint/gate/agent/after-hi\endcsname{0.35}
\expandafter\def\csname v@vint/gate/agent/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/agent/all\endcsname{0.54}
\expandafter\def\csname v@vint/gate/agent/all-hi\endcsname{0.79}
\expandafter\def\csname v@vint/gate/agent/all-lo\endcsname{0.33}
\expandafter\def\csname v@vint/gate/agent/greet\endcsname{3.22}
\expandafter\def\csname v@vint/gate/agent/greet-hi\endcsname{4.58}
\expandafter\def\csname v@vint/gate/agent/greet-lo\endcsname{1.98}
\expandafter\def\csname v@vint/gate/calls\endcsname{816}
\expandafter\def\csname v@vint/gate/dev/round3/calls\endcsname{608}
\expandafter\def\csname v@vint/gate/dev/round3/none/after\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/round3/none/after-hi\endcsname{2.56}
\expandafter\def\csname v@vint/gate/dev/round3/none/after-lo\endcsname{1.57}
\expandafter\def\csname v@vint/gate/dev/round3/none/all\endcsname{2.38}
\expandafter\def\csname v@vint/gate/dev/round3/none/cut\endcsname{88.1}
\expandafter\def\csname v@vint/gate/dev/round3/none/cut-p50\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/round3/none/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/round3/none/greet\endcsname{5.10}
\expandafter\def\csname v@vint/gate/dev/round3/none/held\endcsname{10.2}
\expandafter\def\csname v@vint/gate/dev/round3/none/kind/babble\endcsname{1.93}
\expandafter\def\csname v@vint/gate/dev/round3/none/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/none/kind/home\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/round3/none/kind/music\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/round3/none/kind/street\endcsname{0.76}
\expandafter\def\csname v@vint/gate/dev/round3/none/kind/talker\endcsname{9.94}
\expandafter\def\csname v@vint/gate/dev/round3/none/missed\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/round3/none/recall\endcsname{94.5}
\expandafter\def\csname v@vint/gate/dev/round3/plans\endcsname{288}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/after-hi\endcsname{0.34}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/all\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/cut\endcsname{89.2}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/cut-p50\endcsname{0.65}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/greet\endcsname{6.04}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/held\endcsname{7.0}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/kind/home\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/kind/street\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/kind/talker\endcsname{1.39}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/missed\endcsname{3.19}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/recall\endcsname{87.6}
\expandafter\def\csname v@vint/gate/dev/round3/reuse8/wer\endcsname{19.88}
\expandafter\def\csname v@vint/gate/dev/round3/sessions\endcsname{13}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/after\endcsname{0.38}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/after-hi\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/after-lo\endcsname{0.20}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/all\endcsname{0.86}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/cut\endcsname{91.6}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/greet\endcsname{4.40}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/held\endcsname{2.8}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/kind/babble\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/kind/home\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/kind/music\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/kind/street\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/kind/talker\endcsname{2.57}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/missed\endcsname{0.48}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/recall\endcsname{91.9}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15/wer\endcsname{16.38}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/all\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/greet\endcsname{3.56}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/held\endcsname{4.0}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/kind/babble\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/kind/home\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/kind/talker\endcsname{1.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/missed\endcsname{2.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/recall\endcsname{89.7}
\expandafter\def\csname v@vint/gate/dev/round3/vbj15g_t90_h100_o20_k1/wer\endcsname{18.31}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/after\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/after-hi\endcsname{0.60}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/after-lo\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/all\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/cut\endcsname{91.4}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/greet\endcsname{4.64}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/held\endcsname{3.1}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/kind/babble\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/kind/home\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/kind/music\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/kind/street\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/kind/talker\endcsname{2.40}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/missed\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15/recall\endcsname{91.8}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/after-hi\endcsname{0.34}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/after-lo\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/all\endcsname{0.65}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/cut\endcsname{90.3}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/greet\endcsname{3.95}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/held\endcsname{3.6}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/kind/home\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/kind/music\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/kind/street\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/kind/talker\endcsname{1.41}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/missed\endcsname{1.20}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t80_h100_o20_k1/recall\endcsname{90.6}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/cut\endcsname{89.9}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/greet\endcsname{3.81}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/held\endcsname{4.0}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/kind/babble\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/kind/music\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/kind/street\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/kind/talker\endcsname{1.29}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/missed\endcsname{1.57}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t85_h100_o20_k1/recall\endcsname{90.2}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/cut\endcsname{89.5}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/greet\endcsname{3.70}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/held\endcsname{4.1}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/kind/babble\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/kind/home\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/kind/street\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/kind/talker\endcsname{1.19}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/missed\endcsname{1.84}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o10_k1/recall\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/after-hi\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/cut\endcsname{89.2}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/greet\endcsname{3.70}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/held\endcsname{4.4}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/kind/babble\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/kind/home\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/kind/music\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/kind/street\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/kind/talker\endcsname{1.19}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/missed\endcsname{2.13}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t90_h100_o20_k1/recall\endcsname{89.7}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/after-hi\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/cut\endcsname{89.1}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/greet\endcsname{3.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/held\endcsname{4.4}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/kind/babble\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/kind/music\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/kind/street\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/kind/talker\endcsname{1.14}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/missed\endcsname{2.21}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o10_k1/recall\endcsname{89.5}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/all\endcsname{0.57}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/greet\endcsname{3.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/held\endcsname{4.7}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/kind/babble\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/kind/home\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/kind/street\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/kind/talker\endcsname{1.14}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/missed\endcsname{2.50}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o20_k1/recall\endcsname{89.2}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/all\endcsname{0.56}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/cut\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/greet\endcsname{3.65}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/held\endcsname{5.1}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/kind/babble\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/kind/home\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/kind/talker\endcsname{1.11}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/missed\endcsname{2.68}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t95_h100_o30_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/all\endcsname{0.56}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/cut\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/greet\endcsname{3.63}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/held\endcsname{4.8}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/kind/home\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/kind/street\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/kind/talker\endcsname{1.14}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/missed\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/round3/vbjc15g_t97_h100_o20_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/after\endcsname{0.35}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/after-hi\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/after-lo\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/all\endcsname{0.86}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/cut\endcsname{91.5}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/greet\endcsname{4.62}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/held\endcsname{3.3}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/kind/home\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/kind/music\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/kind/talker\endcsname{2.37}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/missed\endcsname{0.53}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26/recall\endcsname{91.4}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/after\endcsname{0.20}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/after-lo\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/all\endcsname{0.64}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/cut\endcsname{90.4}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/greet\endcsname{3.97}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/held\endcsname{3.8}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/kind/babble\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/kind/home\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/kind/talker\endcsname{1.44}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/missed\endcsname{1.19}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t80_h100_o20_k1/recall\endcsname{90.2}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/all\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/greet\endcsname{3.90}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/held\endcsname{4.1}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/kind/babble\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/kind/home\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/kind/talker\endcsname{1.26}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/missed\endcsname{1.62}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t85_h100_o20_k1/recall\endcsname{89.8}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/after-hi\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/all\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/cut\endcsname{89.4}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/greet\endcsname{3.90}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/held\endcsname{4.4}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/kind/babble\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/kind/home\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/kind/music\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/kind/talker\endcsname{1.19}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/missed\endcsname{2.12}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o10_k1/recall\endcsname{89.4}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/after-hi\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/greet\endcsname{3.88}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/held\endcsname{4.7}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/kind/talker\endcsname{1.19}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/missed\endcsname{2.29}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t90_h100_o20_k1/recall\endcsname{89.2}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/all\endcsname{0.60}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/cut\endcsname{88.9}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/greet\endcsname{3.88}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/held\endcsname{4.8}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/kind/babble\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/kind/music\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/kind/talker\endcsname{1.14}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/missed\endcsname{2.57}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o10_k1/recall\endcsname{88.9}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/greet\endcsname{3.86}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/held\endcsname{5.0}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/kind/babble\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/kind/home\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/kind/talker\endcsname{1.14}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/missed\endcsname{2.76}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o20_k1/recall\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/after\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/after-hi\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/greet\endcsname{3.83}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/held\endcsname{5.5}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/kind/babble\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/kind/home\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/kind/talker\endcsname{1.06}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/missed\endcsname{2.97}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t95_h100_o30_k1/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/cut\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/greet\endcsname{3.81}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/held\endcsname{5.0}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/kind/home\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/kind/talker\endcsname{1.11}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/missed\endcsname{2.92}
\expandafter\def\csname v@vint/gate/dev/round3/vbjs26g_t97_h100_o20_k1/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/dev/screen/calls\endcsname{160}
\expandafter\def\csname v@vint/gate/dev/screen/none/after\endcsname{2.01}
\expandafter\def\csname v@vint/gate/dev/screen/none/after-hi\endcsname{2.48}
\expandafter\def\csname v@vint/gate/dev/screen/none/after-lo\endcsname{1.58}
\expandafter\def\csname v@vint/gate/dev/screen/none/all\endcsname{2.44}
\expandafter\def\csname v@vint/gate/dev/screen/none/cut\endcsname{91.0}
\expandafter\def\csname v@vint/gate/dev/screen/none/cut-p50\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/screen/none/cut-p90\endcsname{0.76}
\expandafter\def\csname v@vint/gate/dev/screen/none/greet\endcsname{5.48}
\expandafter\def\csname v@vint/gate/dev/screen/none/held\endcsname{10.5}
\expandafter\def\csname v@vint/gate/dev/screen/none/kind/babble\endcsname{1.96}
\expandafter\def\csname v@vint/gate/dev/screen/none/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/none/kind/home\endcsname{0.43}
\expandafter\def\csname v@vint/gate/dev/screen/none/kind/music\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/screen/none/kind/street\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/screen/none/kind/talker\endcsname{14.45}
\expandafter\def\csname v@vint/gate/dev/screen/none/missed\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/none/recall\endcsname{94.4}
\expandafter\def\csname v@vint/gate/dev/screen/plans\endcsname{160}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/after\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/after-hi\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/after-lo\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/all\endcsname{1.02}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/cut\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/greet\endcsname{6.68}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/held\endcsname{7.4}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/kind/babble\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/missed\endcsname{4.07}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/recall\endcsname{86.9}
\expandafter\def\csname v@vint/gate/dev/screen/reuse8/wer\endcsname{19.88}
\expandafter\def\csname v@vint/gate/dev/screen/sessions\endcsname{2}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/after\endcsname{0.49}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/after-hi\endcsname{0.69}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/after-lo\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/all\endcsname{1.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/cut\endcsname{91.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/cut-p90\endcsname{0.75}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/greet\endcsname{4.62}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/held\endcsname{3.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/kind/babble\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/kind/talker\endcsname{4.48}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/missed\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2k/recall\endcsname{91.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/after\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/after-hi\endcsname{0.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/after-lo\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/all\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/cut\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/held\endcsname{6.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/missed\endcsname{2.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t85_h15_o30/recall\endcsname{86.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/after\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/after-hi\endcsname{0.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/after-lo\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/all\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/held\endcsname{4.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/missed\endcsname{2.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/recall\endcsname{89.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1/wer\endcsname{17.53}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/all\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/cut\endcsname{87.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/cut-p50\endcsname{0.69}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/cut-p90\endcsname{1.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/greet\endcsname{3.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/held\endcsname{4.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/missed\endcsname{2.91}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a970/recall\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/after-hi\endcsname{0.23}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/all\endcsname{0.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/cut\endcsname{87.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/cut-p50\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/cut-p90\endcsname{1.29}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/greet\endcsname{3.08}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/held\endcsname{4.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/kind/talker\endcsname{1.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/missed\endcsname{2.91}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a990/recall\endcsname{87.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/after-hi\endcsname{0.23}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/all\endcsname{0.50}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/cut\endcsname{87.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/cut-p50\endcsname{0.98}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/cut-p90\endcsname{1.41}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/greet\endcsname{3.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/held\endcsname{4.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/kind/talker\endcsname{1.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/missed\endcsname{2.97}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a995/recall\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/after-hi\endcsname{0.23}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/all\endcsname{0.50}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/cut\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/cut-p50\endcsname{1.24}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/cut-p90\endcsname{1.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/greet\endcsname{3.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/held\endcsname{4.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/kind/talker\endcsname{1.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/missed\endcsname{3.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o10_k1_a999/recall\endcsname{85.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/after-lo\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/all\endcsname{0.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/greet\endcsname{3.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/held\endcsname{4.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/kind/talker\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/missed\endcsname{2.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h100_o30_k1/recall\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/after-lo\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/all\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/greet\endcsname{3.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/missed\endcsname{2.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t90_h50_o20_k1/recall\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/after-lo\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/all\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/greet\endcsname{3.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/held\endcsname{4.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/missed\endcsname{2.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/recall\endcsname{89.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o10_k1/wer\endcsname{17.95}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/after-lo\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/greet\endcsname{3.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/held\endcsname{4.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/missed\endcsname{2.97}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/recall\endcsname{88.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1/wer\endcsname{18.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/after\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/after-hi\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/all\endcsname{0.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/cut\endcsname{87.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/cut-p50\endcsname{0.69}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/cut-p90\endcsname{1.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/greet\endcsname{3.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/held\endcsname{5.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/kind/talker\endcsname{1.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/missed\endcsname{3.52}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a970/recall\endcsname{87.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/after\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/after-hi\endcsname{0.20}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/all\endcsname{0.47}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/cut\endcsname{87.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/cut-p50\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/cut-p90\endcsname{1.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/greet\endcsname{2.91}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/held\endcsname{5.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/kind/talker\endcsname{1.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/missed\endcsname{3.52}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o20_k1_a990/recall\endcsname{86.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/after-lo\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/all\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/greet\endcsname{3.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/kind/talker\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/missed\endcsname{2.97}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h100_o30_k1/recall\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/after-lo\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/all\endcsname{0.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/greet\endcsname{3.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/held\endcsname{5.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/missed\endcsname{3.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t95_h50_o20_k1/recall\endcsname{88.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/after-lo\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/cut\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/greet\endcsname{3.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/missed\endcsname{3.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbg2kg_t97_h100_o20_k1/recall\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/after\endcsname{0.45}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/after-hi\endcsname{0.65}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/after-lo\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/all\endcsname{0.96}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/cut\endcsname{92.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/greet\endcsname{4.54}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/held\endcsname{2.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/kind/babble\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/kind/talker\endcsname{4.33}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/missed\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/recall\endcsname{91.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15/wer\endcsname{16.38}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/after\endcsname{0.35}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/after-hi\endcsname{0.53}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/after-lo\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/all\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/cut\endcsname{91.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/greet\endcsname{4.28}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/held\endcsname{2.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/kind/music\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/kind/talker\endcsname{3.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/missed\endcsname{1.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o10/recall\endcsname{90.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/after\endcsname{0.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/after-hi\endcsname{0.52}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/after-lo\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/all\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/cut\endcsname{91.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/greet\endcsname{4.28}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/held\endcsname{2.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/kind/talker\endcsname{3.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/missed\endcsname{1.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t70_h100_o20/recall\endcsname{90.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/after\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/after-hi\endcsname{0.39}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/after-lo\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/all\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/greet\endcsname{3.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/held\endcsname{3.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/kind/music\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/kind/talker\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/missed\endcsname{1.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10/recall\endcsname{89.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/after\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/after-hi\endcsname{0.40}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/after-lo\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/all\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/cut\endcsname{90.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/greet\endcsname{3.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/held\endcsname{3.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/kind/music\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/kind/talker\endcsname{2.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/missed\endcsname{1.33}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o10_k1/recall\endcsname{90.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/after\endcsname{0.23}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/after-hi\endcsname{0.37}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/after-lo\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/all\endcsname{0.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/greet\endcsname{3.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/held\endcsname{3.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/kind/talker\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/missed\endcsname{2.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t80_h100_o20/recall\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/all\endcsname{0.57}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/greet\endcsname{3.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/held\endcsname{4.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/kind/talker\endcsname{1.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/missed\endcsname{3.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t85_h100_o20/recall\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/all\endcsname{0.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/cut\endcsname{90.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/greet\endcsname{3.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/held\endcsname{3.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/kind/talker\endcsname{1.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/missed\endcsname{1.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/recall\endcsname{89.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o05_k1/wer\endcsname{18.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/all\endcsname{0.52}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/cut\endcsname{88.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/cut-p90\endcsname{0.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/greet\endcsname{3.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/held\endcsname{5.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/kind/talker\endcsname{1.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/missed\endcsname{4.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10/recall\endcsname{87.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/cut\endcsname{90.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/greet\endcsname{3.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/held\endcsname{3.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/kind/talker\endcsname{1.73}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/missed\endcsname{2.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/recall\endcsname{89.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o10_k1/wer\endcsname{18.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/after\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/all\endcsname{0.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/cut\endcsname{88.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/cut-p90\endcsname{0.86}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/greet\endcsname{3.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/held\endcsname{6.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/kind/talker\endcsname{1.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/missed\endcsname{4.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20/recall\endcsname{86.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/all\endcsname{0.57}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/cut\endcsname{90.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/greet\endcsname{3.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/held\endcsname{3.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/kind/talker\endcsname{1.73}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/missed\endcsname{2.37}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/recall\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t90_h100_o20_k1/wer\endcsname{18.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/all\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/cut-p90\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/greet\endcsname{3.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/held\endcsname{4.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/missed\endcsname{2.61}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/recall\endcsname{88.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o10_k1/wer\endcsname{18.56}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/all\endcsname{0.54}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/greet\endcsname{3.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/held\endcsname{4.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/missed\endcsname{2.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/recall\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o20_k1/wer\endcsname{18.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/all\endcsname{0.54}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/greet\endcsname{3.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/held\endcsname{4.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/missed\endcsname{2.91}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/recall\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h100_o30_k1/wer\endcsname{18.89}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/all\endcsname{0.53}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/greet\endcsname{3.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/missed\endcsname{2.91}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/recall\endcsname{87.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t95_h50_o20_k1/wer\endcsname{19.78}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/all\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/greet\endcsname{3.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/held\endcsname{4.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/missed\endcsname{3.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/recall\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15g_t97_h100_o20_k1/wer\endcsname{18.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/after\endcsname{0.38}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/after-hi\endcsname{0.56}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/after-lo\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/all\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/cut\endcsname{91.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/greet\endcsname{4.37}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/held\endcsname{3.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/kind/babble\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/kind/talker\endcsname{3.76}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/missed\endcsname{1.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05/recall\endcsname{90.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/after-hi\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/all\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/greet\endcsname{3.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/held\endcsname{5.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/kind/talker\endcsname{1.73}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/missed\endcsname{3.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbj15s05g_t90_h100_o20_k1/recall\endcsname{88.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/after\endcsname{0.45}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/after-hi\endcsname{0.65}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/after-lo\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/all\endcsname{0.99}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/cut\endcsname{91.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/cut-p90\endcsname{0.75}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/greet\endcsname{4.80}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/held\endcsname{3.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/kind/babble\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/kind/home\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/kind/music\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/kind/talker\endcsname{4.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/missed\endcsname{1.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2k/recall\endcsname{90.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/after\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/after-hi\endcsname{0.40}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/all\endcsname{0.71}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/cut\endcsname{88.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/held\endcsname{4.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/kind/talker\endcsname{2.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/missed\endcsname{2.79}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o05_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/all\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/cut\endcsname{87.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/held\endcsname{5.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/missed\endcsname{3.28}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o10_k1/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/all\endcsname{0.65}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/cut\endcsname{87.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/held\endcsname{5.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/missed\endcsname{3.46}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t90_h100_o20_k1/recall\endcsname{88.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/all\endcsname{0.65}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/cut\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/greet\endcsname{3.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/held\endcsname{5.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/missed\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o10_k1/recall\endcsname{87.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/all\endcsname{0.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/cut\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/greet\endcsname{3.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/held\endcsname{5.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/missed\endcsname{4.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o20_k1/recall\endcsname{87.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/all\endcsname{0.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/cut\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/greet\endcsname{3.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/held\endcsname{6.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/missed\endcsname{4.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h100_o30_k1/recall\endcsname{87.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/all\endcsname{0.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/cut\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/greet\endcsname{3.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/held\endcsname{6.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/missed\endcsname{4.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t95_h50_o20_k1/recall\endcsname{86.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/all\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/cut\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/held\endcsname{5.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/missed\endcsname{4.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbjb2kg_t97_h100_o20_k1/recall\endcsname{87.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/after\endcsname{0.41}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/after-hi\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/after-lo\endcsname{0.23}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/all\endcsname{0.95}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/cut\endcsname{92.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/greet\endcsname{4.71}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/held\endcsname{2.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/kind/babble\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/kind/talker\endcsname{3.90}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/missed\endcsname{0.73}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15/recall\endcsname{91.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/after\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/after-hi\endcsname{0.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/after-lo\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/all\endcsname{0.72}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/cut\endcsname{90.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/held\endcsname{3.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/kind/talker\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/missed\endcsname{1.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t80_h100_o20_k1/recall\endcsname{90.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/after-hi\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/all\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/cut\endcsname{90.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/greet\endcsname{3.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/held\endcsname{3.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/missed\endcsname{2.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t85_h100_o20_k1/recall\endcsname{89.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/all\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/held\endcsname{3.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/kind/talker\endcsname{1.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/missed\endcsname{2.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o10_k1/recall\endcsname{89.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/all\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/held\endcsname{4.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/kind/talker\endcsname{1.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/missed\endcsname{2.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t90_h100_o20_k1/recall\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/all\endcsname{0.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/held\endcsname{4.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/missed\endcsname{2.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o10_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/all\endcsname{0.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/held\endcsname{4.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/missed\endcsname{3.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o20_k1/recall\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/greet\endcsname{3.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/held\endcsname{4.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/missed\endcsname{3.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t95_h100_o30_k1/recall\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/cut\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/greet\endcsname{3.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/held\endcsname{4.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/missed\endcsname{3.28}
\expandafter\def\csname v@vint/gate/dev/screen/vbjc15g_t97_h100_o20_k1/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/after\endcsname{0.39}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/after-hi\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/after-lo\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/all\endcsname{0.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/cut\endcsname{92.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/greet\endcsname{4.80}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/held\endcsname{3.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/kind/talker\endcsname{3.76}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/missed\endcsname{0.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26/recall\endcsname{90.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/after\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/after-hi\endcsname{0.38}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/all\endcsname{0.71}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/cut\endcsname{90.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/greet\endcsname{4.20}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/held\endcsname{4.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/kind/talker\endcsname{2.46}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/missed\endcsname{1.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t80_h100_o20_k1/recall\endcsname{89.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/after-hi\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/all\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/cut\endcsname{90.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/greet\endcsname{4.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/held\endcsname{4.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/kind/talker\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/missed\endcsname{2.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t85_h100_o20_k1/recall\endcsname{89.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/after-hi\endcsname{0.37}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/all\endcsname{0.69}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/greet\endcsname{4.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/held\endcsname{4.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/kind/talker\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/missed\endcsname{2.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o10_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/after-hi\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/all\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/greet\endcsname{4.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/held\endcsname{5.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/kind/talker\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/missed\endcsname{2.91}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t90_h100_o20_k1/recall\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/after-hi\endcsname{0.35}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/all\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/greet\endcsname{4.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/held\endcsname{5.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/missed\endcsname{3.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o10_k1/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/all\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/greet\endcsname{4.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/held\endcsname{5.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/missed\endcsname{3.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o20_k1/recall\endcsname{88.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/all\endcsname{0.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/cut-p90\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/held\endcsname{5.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/kind/talker\endcsname{1.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/missed\endcsname{3.46}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t95_h100_o30_k1/recall\endcsname{87.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/all\endcsname{0.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/cut\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/held\endcsname{5.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/kind/talker\endcsname{1.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/missed\endcsname{3.64}
\expandafter\def\csname v@vint/gate/dev/screen/vbjs26g_t97_h100_o20_k1/recall\endcsname{87.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/after\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/after-hi\endcsname{0.42}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/all\endcsname{0.72}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/held\endcsname{7.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/kind/talker\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/missed\endcsname{2.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1k/recall\endcsname{87.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/after\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/after-hi\endcsname{0.42}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/all\endcsname{0.71}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/greet\endcsname{3.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/held\endcsname{7.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/kind/talker\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/missed\endcsname{2.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h100_o05_k1/recall\endcsname{86.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/after\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/after-hi\endcsname{0.42}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/all\endcsname{0.71}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/greet\endcsname{3.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/held\endcsname{7.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/kind/talker\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/missed\endcsname{2.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t30_h150_o02_k2/recall\endcsname{87.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/after\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/after-hi\endcsname{0.40}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/after-lo\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/all\endcsname{0.71}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/cut\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/cut-p90\endcsname{0.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/held\endcsname{7.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/kind/talker\endcsname{2.46}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/missed\endcsname{3.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o05_k1/recall\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/after\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/after-hi\endcsname{0.38}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/after-lo\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/all\endcsname{0.70}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/cut\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/cut-p90\endcsname{0.86}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/held\endcsname{7.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/kind/talker\endcsname{2.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/missed\endcsname{3.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h100_o10_k1/recall\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/after\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/after-hi\endcsname{0.42}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/all\endcsname{0.72}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/cut\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/held\endcsname{7.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/kind/talker\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/missed\endcsname{2.91}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t50_h150_o05_k1/recall\endcsname{86.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/after\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/after-hi\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/all\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/cut\endcsname{87.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/greet\endcsname{3.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/held\endcsname{8.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/kind/talker\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/missed\endcsname{3.70}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t60_h100_o10_k1/recall\endcsname{85.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/all\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/cut\endcsname{85.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/cut-p90\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/greet\endcsname{3.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/held\endcsname{8.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/kind/talker\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/missed\endcsname{4.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t70_h100_o10_k1/recall\endcsname{85.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/all\endcsname{0.56}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/cut\endcsname{83.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/cut-p90\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/greet\endcsname{3.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/held\endcsname{9.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/kind/talker\endcsname{1.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/missed\endcsname{5.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t80_h100_o10_k1/recall\endcsname{83.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/after\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/after-hi\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/all\endcsname{0.33}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/cut\endcsname{76.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/cut-p50\endcsname{0.69}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/cut-p90\endcsname{1.10}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/greet\endcsname{2.23}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/held\endcsname{15.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/kind/talker\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/missed\endcsname{12.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10/recall\endcsname{76.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/after\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/after-hi\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/after-lo\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/all\endcsname{0.47}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/cut\endcsname{81.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/cut-p90\endcsname{0.90}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/greet\endcsname{3.08}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/held\endcsname{11.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/kind/talker\endcsname{1.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/missed\endcsname{7.58}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t90_h100_o10_k1/recall\endcsname{81.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/after\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/after-hi\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/after-lo\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/all\endcsname{0.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/cut\endcsname{81.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/cut-p90\endcsname{0.91}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/greet\endcsname{2.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/held\endcsname{12.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/kind/talker\endcsname{1.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/missed\endcsname{8.86}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o10_k1/recall\endcsname{81.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/after\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/after-hi\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/all\endcsname{0.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/cut\endcsname{80.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/cut-p90\endcsname{0.92}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/greet\endcsname{2.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/held\endcsname{12.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/kind/talker\endcsname{1.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/missed\endcsname{9.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbt1kg_t95_h100_o20_k1/recall\endcsname{80.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/after\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/after-lo\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/all\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/cut\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/greet\endcsname{4.28}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/held\endcsname{7.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/kind/talker\endcsname{2.74}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/missed\endcsname{2.61}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1k/recall\endcsname{87.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/after\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/after-hi\endcsname{0.23}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/all\endcsname{0.57}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/cut\endcsname{83.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/cut-p90\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/greet\endcsname{3.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/held\endcsname{8.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/kind/talker\endcsname{1.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/missed\endcsname{5.40}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t80_h100_o10_k1/recall\endcsname{84.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/after\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/after-hi\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/all\endcsname{0.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/cut\endcsname{76.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/cut-p90\endcsname{1.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/greet\endcsname{3.08}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/held\endcsname{14.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/kind/talker\endcsname{0.72}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/missed\endcsname{11.95}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10/recall\endcsname{77.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/after\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/after-hi\endcsname{0.20}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/all\endcsname{0.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/cut\endcsname{81.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/cut-p90\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/greet\endcsname{3.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/held\endcsname{10.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/kind/talker\endcsname{1.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/missed\endcsname{7.28}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t90_h100_o10_k1/recall\endcsname{82.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/after\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/after-hi\endcsname{0.20}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/all\endcsname{0.50}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/cut\endcsname{81.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/cut-p90\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/greet\endcsname{3.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/held\endcsname{11.2}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/kind/talker\endcsname{1.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/missed\endcsname{8.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o10_k1/recall\endcsname{81.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/after\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/after-hi\endcsname{0.20}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/all\endcsname{0.50}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/cut\endcsname{81.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/cut-p90\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/greet\endcsname{3.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/held\endcsname{11.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/kind/talker\endcsname{1.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/missed\endcsname{8.56}
\expandafter\def\csname v@vint/gate/dev/screen/vbtb1kg_t95_h100_o20_k1/recall\endcsname{81.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/after\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/after-lo\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/all\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/greet\endcsname{4.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/held\endcsname{4.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/kind/talker\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/missed\endcsname{1.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26/recall\endcsname{89.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/after\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/after-hi\endcsname{0.42}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/after-lo\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/all\endcsname{0.71}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/kind/talker\endcsname{2.46}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/missed\endcsname{1.58}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t50_h100_o10_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/after\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/after-hi\endcsname{0.35}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/after-lo\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/all\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/cut\endcsname{88.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/cut-p90\endcsname{0.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/held\endcsname{5.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/kind/talker\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/missed\endcsname{2.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t60_h100_o10_k1/recall\endcsname{88.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/after-hi\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/all\endcsname{0.57}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/cut\endcsname{86.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/cut-p90\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/greet\endcsname{3.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/held\endcsname{6.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/kind/talker\endcsname{1.73}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/missed\endcsname{2.97}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o10_k1/recall\endcsname{87.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/after-hi\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/all\endcsname{0.56}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/cut\endcsname{86.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/cut-p90\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/greet\endcsname{3.34}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/held\endcsname{6.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/kind/talker\endcsname{1.73}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/missed\endcsname{2.97}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t70_h100_o20_k1/recall\endcsname{87.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/after\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/after-hi\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/all\endcsname{0.50}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/cut\endcsname{84.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/cut-p90\endcsname{0.86}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/greet\endcsname{3.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/held\endcsname{6.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/kind/talker\endcsname{1.16}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/missed\endcsname{3.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t80_h100_o10_k1/recall\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/after\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/after-hi\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/all\endcsname{0.23}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/cut\endcsname{75.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/cut-p90\endcsname{1.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/greet\endcsname{1.80}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/held\endcsname{13.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/kind/talker\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/missed\endcsname{11.35}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10/recall\endcsname{77.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/after\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/after-hi\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/all\endcsname{0.41}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/cut\endcsname{83.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/cut-p90\endcsname{0.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/greet\endcsname{2.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/held\endcsname{7.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/kind/talker\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/missed\endcsname{5.58}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t90_h100_o10_k1/recall\endcsname{84.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/after\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/after-hi\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/all\endcsname{0.45}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/cut\endcsname{82.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/cut-p90\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/greet\endcsname{2.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/held\endcsname{8.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/kind/talker\endcsname{1.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/missed\endcsname{6.37}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o10_k1/recall\endcsname{84.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/after\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/after-hi\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/all\endcsname{0.45}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/cut\endcsname{82.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/cut-p90\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/greet\endcsname{2.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/held\endcsname{8.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/kind/babble\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/kind/talker\endcsname{1.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/missed\endcsname{6.55}
\expandafter\def\csname v@vint/gate/dev/screen/vbts26g_t95_h100_o20_k1/recall\endcsname{83.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/after\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/after-lo\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/all\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/cut\endcsname{84.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/greet\endcsname{4.88}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/held\endcsname{8.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/kind/babble\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/kind/talker\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/missed\endcsname{3.58}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26/recall\endcsname{86.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/all\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/cut\endcsname{81.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/greet\endcsname{4.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/held\endcsname{10.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/kind/music\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/kind/talker\endcsname{1.30}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/missed\endcsname{5.95}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t80_h100_o10_k1/recall\endcsname{83.7}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/after\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/after-hi\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/all\endcsname{0.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/cut\endcsname{74.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/cut-p90\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/greet\endcsname{3.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/held\endcsname{16.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/kind/talker\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/missed\endcsname{14.26}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10/recall\endcsname{76.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/after\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/after-hi\endcsname{0.20}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/all\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/cut\endcsname{81.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/greet\endcsname{3.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/held\endcsname{11.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/kind/talker\endcsname{1.01}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/missed\endcsname{7.95}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t90_h100_o10_k1/recall\endcsname{82.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/after\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/after-hi\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/after-lo\endcsname{0.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/all\endcsname{0.52}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/cut\endcsname{81.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/cut-p90\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/greet\endcsname{3.51}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/held\endcsname{12.1}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/kind/talker\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/missed\endcsname{8.74}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o10_k1/recall\endcsname{81.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/after\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/after-hi\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/after-lo\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/all\endcsname{0.50}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/cut\endcsname{80.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/cut-p90\endcsname{0.85}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/greet\endcsname{3.43}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/held\endcsname{12.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/kind/talker\endcsname{0.87}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/missed\endcsname{9.47}
\expandafter\def\csname v@vint/gate/dev/screen/vbtsb26g_t95_h100_o20_k1/recall\endcsname{80.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/after\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/after-hi\endcsname{0.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/all\endcsname{1.17}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/cut\endcsname{91.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/cut-p90\endcsname{0.73}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/greet\endcsname{4.62}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/held\endcsname{1.5}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/kind/babble\endcsname{0.42}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/kind/home\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/kind/music\endcsname{0.49}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/kind/street\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/kind/talker\endcsname{4.91}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/missed\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1k/recall\endcsname{93.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/after\endcsname{0.39}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/after-hi\endcsname{0.56}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/after-lo\endcsname{0.23}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/all\endcsname{0.86}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/cut\endcsname{90.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/cut-p90\endcsname{0.75}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/greet\endcsname{4.20}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/held\endcsname{1.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/kind/babble\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/kind/home\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/kind/music\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/kind/talker\endcsname{2.89}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/missed\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t80_h100_o10_k1/recall\endcsname{92.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/after\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/after-hi\endcsname{0.38}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/after-lo\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/all\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/cut\endcsname{88.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/greet\endcsname{3.60}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/held\endcsname{3.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/kind/babble\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/kind/music\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/kind/talker\endcsname{1.59}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/missed\endcsname{2.49}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10/recall\endcsname{90.4}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/after\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/after-hi\endcsname{0.46}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/after-lo\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/all\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/held\endcsname{2.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/kind/babble\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/kind/music\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/kind/talker\endcsname{2.31}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/missed\endcsname{1.33}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t90_h100_o10_k1/recall\endcsname{91.8}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/after\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/after-hi\endcsname{0.47}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/after-lo\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/all\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/cut\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/greet\endcsname{4.03}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/held\endcsname{2.6}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/kind/babble\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/kind/music\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/kind/talker\endcsname{2.46}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/missed\endcsname{1.70}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o10_k1/recall\endcsname{91.3}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/after\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/after-hi\endcsname{0.41}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/after-lo\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/all\endcsname{0.72}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/held\endcsname{2.9}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/kind/babble\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/kind/talker\endcsname{2.46}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/missed\endcsname{1.76}
\expandafter\def\csname v@vint/gate/dev/screen/vbz1kg_t95_h100_o20_k1/recall\endcsname{90.9}
\expandafter\def\csname v@vint/gate/dev/select/calls\endcsname{480}
\expandafter\def\csname v@vint/gate/dev/select/none/after\endcsname{2.02}
\expandafter\def\csname v@vint/gate/dev/select/none/after-hi\endcsname{2.61}
\expandafter\def\csname v@vint/gate/dev/select/none/after-lo\endcsname{1.45}
\expandafter\def\csname v@vint/gate/dev/select/none/all\endcsname{2.39}
\expandafter\def\csname v@vint/gate/dev/select/none/cut\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/select/none/cut-p50\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/select/none/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/select/none/greet\endcsname{5.20}
\expandafter\def\csname v@vint/gate/dev/select/none/held\endcsname{10.3}
\expandafter\def\csname v@vint/gate/dev/select/none/kind/babble\endcsname{1.94}
\expandafter\def\csname v@vint/gate/dev/select/none/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/none/kind/home\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/select/none/kind/music\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/select/none/kind/street\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/select/none/kind/talker\endcsname{9.15}
\expandafter\def\csname v@vint/gate/dev/select/none/missed\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/select/none/recall\endcsname{94.6}
\expandafter\def\csname v@vint/gate/dev/select/plans\endcsname{160}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/after-hi\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/all\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/cut\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/cut-p50\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/greet\endcsname{6.17}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/held\endcsname{7.0}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/kind/talker\endcsname{1.28}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/missed\endcsname{3.02}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/recall\endcsname{87.8}
\expandafter\def\csname v@vint/gate/dev/select/reuse8/wer\endcsname{19.88}
\expandafter\def\csname v@vint/gate/dev/select/sessions\endcsname{12}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/after\endcsname{0.43}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/after-hi\endcsname{0.70}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/after-lo\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/all\endcsname{0.95}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/cut\endcsname{90.5}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/greet\endcsname{4.94}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/held\endcsname{3.6}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/kind/babble\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/kind/home\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/kind/music\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/kind/street\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/kind/talker\endcsname{2.70}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/missed\endcsname{0.53}
\expandafter\def\csname v@vint/gate/dev/select/vbg2k/recall\endcsname{91.4}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/after-hi\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/all\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/cut\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/greet\endcsname{3.54}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/held\endcsname{7.1}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/kind/talker\endcsname{1.05}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/missed\endcsname{2.96}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t85_h15_o30/recall\endcsname{86.5}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/after\endcsname{0.20}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/after-hi\endcsname{0.34}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/all\endcsname{0.64}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/cut\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/greet\endcsname{3.97}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/held\endcsname{4.5}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/kind/babble\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/kind/street\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/kind/talker\endcsname{1.25}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/missed\endcsname{2.05}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/recall\endcsname{89.9}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1/wer\endcsname{17.53}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/after\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/all\endcsname{0.51}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/cut\endcsname{87.5}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/cut-p50\endcsname{0.69}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/cut-p90\endcsname{1.12}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/greet\endcsname{3.29}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/held\endcsname{4.8}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/kind/talker\endcsname{0.96}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/missed\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a970/recall\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/after\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/after-hi\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/all\endcsname{0.49}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/cut\endcsname{87.2}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/cut-p50\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/cut-p90\endcsname{1.41}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/greet\endcsname{3.14}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/kind/talker\endcsname{0.93}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/missed\endcsname{2.70}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a990/recall\endcsname{87.6}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/after\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/after-hi\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/all\endcsname{0.48}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/cut\endcsname{87.0}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/cut-p50\endcsname{0.97}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/cut-p90\endcsname{1.50}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/greet\endcsname{3.11}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/kind/talker\endcsname{0.93}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/missed\endcsname{2.76}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a995/recall\endcsname{86.7}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/after\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/after-hi\endcsname{0.24}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/all\endcsname{0.48}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/cut\endcsname{86.4}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/cut-p50\endcsname{1.30}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/cut-p90\endcsname{1.63}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/greet\endcsname{3.09}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/kind/talker\endcsname{0.90}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/missed\endcsname{2.78}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o10_k1_a999/recall\endcsname{85.1}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/held\endcsname{5.1}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/kind/talker\endcsname{1.22}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/missed\endcsname{2.25}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h100_o30_k1/recall\endcsname{89.4}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/cut\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/greet\endcsname{3.89}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/held\endcsname{5.6}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/kind/talker\endcsname{1.19}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/missed\endcsname{2.37}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t90_h50_o20_k1/recall\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/greet\endcsname{3.86}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/held\endcsname{4.7}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/kind/talker\endcsname{1.22}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/missed\endcsname{2.33}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/recall\endcsname{89.5}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o10_k1/wer\endcsname{17.95}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/cut\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/greet\endcsname{3.83}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/held\endcsname{5.0}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/kind/talker\endcsname{1.19}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/missed\endcsname{2.47}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/recall\endcsname{89.2}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o20_k1/wer\endcsname{18.17}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/cut\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/greet\endcsname{3.83}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/held\endcsname{5.3}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/kind/talker\endcsname{1.22}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/missed\endcsname{2.58}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h100_o30_k1/recall\endcsname{88.9}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/all\endcsname{0.57}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/cut\endcsname{88.4}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/greet\endcsname{3.71}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/held\endcsname{5.8}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/kind/talker\endcsname{1.19}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/missed\endcsname{2.68}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t95_h50_o20_k1/recall\endcsname{88.1}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/cut\endcsname{88.3}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/greet\endcsname{3.80}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/held\endcsname{5.1}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/kind/talker\endcsname{1.19}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/missed\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/select/vbg2kg_t97_h100_o20_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/after\endcsname{0.40}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/after-hi\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/after-lo\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/all\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/cut\endcsname{91.1}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/greet\endcsname{4.60}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/held\endcsname{3.0}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/kind/babble\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/kind/home\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/kind/music\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/kind/talker\endcsname{2.56}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/missed\endcsname{0.51}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/recall\endcsname{91.8}
\expandafter\def\csname v@vint/gate/dev/select/vbj15/wer\endcsname{16.38}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/after\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/all\endcsname{0.70}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/cut\endcsname{90.4}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/cut-p90\endcsname{0.76}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/held\endcsname{3.2}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/kind/home\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/kind/music\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/kind/street\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/kind/talker\endcsname{1.66}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/missed\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o10/recall\endcsname{91.2}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/after\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/after-hi\endcsname{0.43}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/after-lo\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/all\endcsname{0.69}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/cut\endcsname{90.2}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/cut-p90\endcsname{0.76}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/held\endcsname{3.2}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/kind/home\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/kind/music\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/kind/street\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/kind/talker\endcsname{1.63}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/missed\endcsname{0.91}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t70_h100_o20/recall\endcsname{91.1}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/after-hi\endcsname{0.35}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/cut\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/greet\endcsname{3.66}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/held\endcsname{3.9}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/kind/home\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/kind/music\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/kind/talker\endcsname{1.25}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/missed\endcsname{1.56}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o10/recall\endcsname{90.2}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/cut\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/greet\endcsname{3.63}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/held\endcsname{4.1}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/kind/home\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/kind/talker\endcsname{1.16}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/missed\endcsname{1.78}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t80_h100_o20/recall\endcsname{89.9}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/after-hi\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/all\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/cut\endcsname{88.3}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/greet\endcsname{3.46}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/kind/home\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/kind/talker\endcsname{1.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/missed\endcsname{2.66}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t85_h100_o20/recall\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/all\endcsname{0.57}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/cut\endcsname{89.5}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/greet\endcsname{3.57}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/held\endcsname{3.7}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/kind/home\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/kind/music\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/kind/talker\endcsname{1.08}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/missed\endcsname{1.60}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/recall\endcsname{90.2}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o05_k1/wer\endcsname{18.09}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/after-hi\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/all\endcsname{0.56}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/cut\endcsname{89.1}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/greet\endcsname{3.57}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/held\endcsname{4.0}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/kind/music\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/kind/talker\endcsname{1.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/missed\endcsname{1.80}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/recall\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o10_k1/wer\endcsname{18.26}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/after\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/after-hi\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/all\endcsname{0.45}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/cut\endcsname{86.6}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/cut-p90\endcsname{0.85}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/greet\endcsname{3.09}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/held\endcsname{6.3}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/kind/talker\endcsname{0.70}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/missed\endcsname{4.38}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20/recall\endcsname{86.9}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/after\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/all\endcsname{0.54}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/greet\endcsname{3.57}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/held\endcsname{4.2}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/kind/talker\endcsname{0.99}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/missed\endcsname{2.05}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/recall\endcsname{89.7}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t90_h100_o20_k1/wer\endcsname{18.31}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/after-hi\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/all\endcsname{0.54}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/cut\endcsname{88.9}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/greet\endcsname{3.51}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/held\endcsname{4.1}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/kind/talker\endcsname{0.99}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/missed\endcsname{2.07}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/recall\endcsname{89.6}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o10_k1/wer\endcsname{18.56}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/after\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/all\endcsname{0.52}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/cut\endcsname{88.6}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/greet\endcsname{3.51}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/held\endcsname{4.4}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/kind/talker\endcsname{0.96}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/missed\endcsname{2.31}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/recall\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o20_k1/wer\endcsname{18.68}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/after\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/all\endcsname{0.52}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/cut\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/greet\endcsname{3.51}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/held\endcsname{4.7}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/kind/talker\endcsname{0.96}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/missed\endcsname{2.47}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h100_o30_k1/wer\endcsname{18.89}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/after\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/all\endcsname{0.51}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/cut\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/greet\endcsname{3.43}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/held\endcsname{5.3}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/kind/talker\endcsname{0.96}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/missed\endcsname{2.58}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/recall\endcsname{88.3}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t95_h50_o20_k1/wer\endcsname{19.78}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/after\endcsname{0.13}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/all\endcsname{0.52}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/cut\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/cut-p90\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/greet\endcsname{3.49}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/held\endcsname{4.5}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/kind/talker\endcsname{0.96}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/missed\endcsname{2.43}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/recall\endcsname{89.1}
\expandafter\def\csname v@vint/gate/dev/select/vbj15g_t97_h100_o20_k1/wer\endcsname{18.77}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/after\endcsname{0.39}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/after-hi\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/after-lo\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/all\endcsname{0.90}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/cut\endcsname{90.6}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/greet\endcsname{4.86}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/held\endcsname{4.1}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/kind/home\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/kind/music\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/kind/talker\endcsname{2.41}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/missed\endcsname{0.95}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2k/recall\endcsname{91.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/after\endcsname{0.21}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/after-hi\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/all\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/cut\endcsname{87.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/greet\endcsname{4.14}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/held\endcsname{5.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/kind/babble\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/kind/home\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/kind/talker\endcsname{1.25}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/missed\endcsname{2.60}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o05_k1/recall\endcsname{88.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/all\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/cut\endcsname{87.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/greet\endcsname{4.14}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/held\endcsname{5.6}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/kind/babble\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/kind/talker\endcsname{1.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/missed\endcsname{2.92}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o10_k1/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/all\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/cut\endcsname{86.8}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/greet\endcsname{4.14}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/held\endcsname{6.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/kind/talker\endcsname{1.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/missed\endcsname{3.28}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t90_h100_o20_k1/recall\endcsname{88.1}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/cut\endcsname{86.7}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/greet\endcsname{4.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/held\endcsname{5.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/kind/talker\endcsname{1.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/missed\endcsname{3.43}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o10_k1/recall\endcsname{88.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/cut\endcsname{86.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/cut-p90\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/greet\endcsname{4.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/held\endcsname{6.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/kind/talker\endcsname{1.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/missed\endcsname{3.79}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o20_k1/recall\endcsname{87.6}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/after\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/after-hi\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/cut\endcsname{86.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/cut-p90\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/greet\endcsname{4.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/held\endcsname{6.8}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/kind/talker\endcsname{1.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/missed\endcsname{4.01}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h100_o30_k1/recall\endcsname{87.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/after\endcsname{0.14}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/after-hi\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/cut\endcsname{86.1}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/cut-p90\endcsname{0.83}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/greet\endcsname{4.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/held\endcsname{7.7}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/kind/talker\endcsname{1.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/missed\endcsname{4.14}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t95_h50_o20_k1/recall\endcsname{86.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/all\endcsname{0.60}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/cut\endcsname{86.1}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/cut-p90\endcsname{0.84}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/greet\endcsname{4.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/held\endcsname{6.4}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/kind/talker\endcsname{1.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/missed\endcsname{3.91}
\expandafter\def\csname v@vint/gate/dev/select/vbjb2kg_t97_h100_o20_k1/recall\endcsname{87.4}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/after\endcsname{0.37}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/after-hi\endcsname{0.65}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/after-lo\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/all\endcsname{0.88}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/cut\endcsname{90.8}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/greet\endcsname{4.74}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/held\endcsname{3.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/kind/babble\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/kind/home\endcsname{0.11}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/kind/music\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/kind/street\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/kind/talker\endcsname{2.38}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/missed\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15/recall\endcsname{91.7}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/after\endcsname{0.22}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/after-hi\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/after-lo\endcsname{0.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/all\endcsname{0.66}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/cut\endcsname{89.8}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/cut-p90\endcsname{0.76}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/greet\endcsname{4.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/held\endcsname{3.8}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/kind/home\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/kind/music\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/kind/street\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/kind/talker\endcsname{1.37}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/missed\endcsname{1.24}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t80_h100_o20_k1/recall\endcsname{90.6}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/all\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/cut\endcsname{89.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/cut-p90\endcsname{0.76}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/greet\endcsname{3.89}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/held\endcsname{4.1}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/kind/street\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/kind/talker\endcsname{1.25}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/missed\endcsname{1.56}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t85_h100_o20_k1/recall\endcsname{90.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/all\endcsname{0.60}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/held\endcsname{4.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/kind/talker\endcsname{1.16}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/missed\endcsname{1.82}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o10_k1/recall\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/cut\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/cut-p90\endcsname{0.77}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/greet\endcsname{3.77}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/held\endcsname{4.6}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/kind/talker\endcsname{1.16}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/missed\endcsname{2.17}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t90_h100_o20_k1/recall\endcsname{89.7}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/cut\endcsname{88.5}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/greet\endcsname{3.74}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/held\endcsname{4.6}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/kind/talker\endcsname{1.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/missed\endcsname{2.21}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o10_k1/recall\endcsname{89.5}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/after-hi\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/all\endcsname{0.57}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/cut\endcsname{88.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/cut-p90\endcsname{0.79}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/greet\endcsname{3.74}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/kind/talker\endcsname{1.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/missed\endcsname{2.55}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o20_k1/recall\endcsname{89.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/after-hi\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/all\endcsname{0.56}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/cut\endcsname{88.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/greet\endcsname{3.71}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/held\endcsname{5.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/kind/talker\endcsname{1.08}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/missed\endcsname{2.76}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t95_h100_o30_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/after-hi\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/all\endcsname{0.56}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/cut\endcsname{87.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/greet\endcsname{3.69}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/held\endcsname{5.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/kind/street\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/kind/talker\endcsname{1.10}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/missed\endcsname{2.66}
\expandafter\def\csname v@vint/gate/dev/select/vbjc15g_t97_h100_o20_k1/recall\endcsname{89.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/after\endcsname{0.37}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/after-hi\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/after-lo\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/all\endcsname{0.89}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/cut\endcsname{91.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/cut-p90\endcsname{0.74}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/greet\endcsname{4.80}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/held\endcsname{3.5}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/kind/babble\endcsname{0.12}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/kind/home\endcsname{0.09}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/kind/music\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/kind/street\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/kind/talker\endcsname{2.35}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/missed\endcsname{0.55}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26/recall\endcsname{91.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/after\endcsname{0.20}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/after-hi\endcsname{0.36}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/all\endcsname{0.65}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/cut\endcsname{90.0}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/greet\endcsname{4.03}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/held\endcsname{4.1}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/kind/talker\endcsname{1.42}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/missed\endcsname{1.20}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t80_h100_o20_k1/recall\endcsname{90.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/all\endcsname{0.62}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/cut\endcsname{89.4}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/held\endcsname{4.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/kind/talker\endcsname{1.31}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/missed\endcsname{1.62}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t85_h100_o20_k1/recall\endcsname{89.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/all\endcsname{0.63}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/cut\endcsname{88.8}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/greet\endcsname{3.97}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/held\endcsname{4.6}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/kind/babble\endcsname{0.08}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/kind/home\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/kind/talker\endcsname{1.22}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/missed\endcsname{2.11}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o10_k1/recall\endcsname{89.4}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/after-hi\endcsname{0.31}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/cut\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/cut-p90\endcsname{0.78}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/kind/talker\endcsname{1.22}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/missed\endcsname{2.31}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t90_h100_o20_k1/recall\endcsname{89.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/after\endcsname{0.17}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/all\endcsname{0.61}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/cut\endcsname{88.3}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/cut-p90\endcsname{0.80}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/greet\endcsname{3.94}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/held\endcsname{4.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/kind/babble\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/kind/home\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/kind/music\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/kind/talker\endcsname{1.16}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/missed\endcsname{2.58}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o10_k1/recall\endcsname{88.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/after\endcsname{0.16}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/after-hi\endcsname{0.29}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/all\endcsname{0.60}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/cut\endcsname{88.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/greet\endcsname{3.91}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/held\endcsname{5.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/kind/talker\endcsname{1.16}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/missed\endcsname{2.76}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o20_k1/recall\endcsname{88.7}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/cut\endcsname{88.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/cut-p90\endcsname{0.81}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/greet\endcsname{3.89}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/held\endcsname{5.7}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/kind/babble\endcsname{0.04}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/kind/home\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/kind/talker\endcsname{1.08}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/missed\endcsname{3.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t95_h100_o30_k1/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/after\endcsname{0.15}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/after-hi\endcsname{0.28}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/all\endcsname{0.58}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/cut\endcsname{87.9}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/cut-p90\endcsname{0.82}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/greet\endcsname{3.86}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/held\endcsname{5.2}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/kind/babble\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/kind/clean\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/kind/home\endcsname{0.02}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/kind/music\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/kind/street\endcsname{0.00}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/kind/talker\endcsname{1.13}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/missed\endcsname{2.94}
\expandafter\def\csname v@vint/gate/dev/select/vbjs26g_t97_h100_o20_k1/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/diff/agent-ft/after\endcsname{-0.20}
\expandafter\def\csname v@vint/gate/diff/agent-ft/after-hi\endcsname{-0.10}
\expandafter\def\csname v@vint/gate/diff/agent-ft/after-lo\endcsname{-0.31}
\expandafter\def\csname v@vint/gate/diff/agent-ft/all\endcsname{-0.32}
\expandafter\def\csname v@vint/gate/diff/agent-ft/all-hi\endcsname{-0.21}
\expandafter\def\csname v@vint/gate/diff/agent-ft/all-lo\endcsname{-0.46}
\expandafter\def\csname v@vint/gate/diff/agent-ft/greet\endcsname{-1.29}
\expandafter\def\csname v@vint/gate/diff/agent-ft/greet-hi\endcsname{-0.85}
\expandafter\def\csname v@vint/gate/diff/agent-ft/greet-lo\endcsname{-1.78}
\expandafter\def\csname v@vint/gate/diff/agent-gate0/after\endcsname{-0.06}
\expandafter\def\csname v@vint/gate/diff/agent-gate0/after-hi\endcsname{-0.02}
\expandafter\def\csname v@vint/gate/diff/agent-gate0/after-lo\endcsname{-0.10}
\expandafter\def\csname v@vint/gate/diff/agent-gate0/all\endcsname{-0.05}
\expandafter\def\csname v@vint/gate/diff/agent-gate0/all-hi\endcsname{-0.02}
\expandafter\def\csname v@vint/gate/diff/agent-gate0/all-lo\endcsname{-0.09}
\expandafter\def\csname v@vint/gate/diff/agent-gate0/greet\endcsname{+0.02}
\expandafter\def\csname v@vint/gate/diff/agent-gate0/greet-hi\endcsname{+0.14}
\expandafter\def\csname v@vint/gate/diff/agent-gate0/greet-lo\endcsname{-0.10}
\expandafter\def\csname v@vint/gate/diff/agent-pick/after\endcsname{+0.00}
\expandafter\def\csname v@vint/gate/diff/agent-pick/after-hi\endcsname{+0.00}
\expandafter\def\csname v@vint/gate/diff/agent-pick/after-lo\endcsname{+0.00}
\expandafter\def\csname v@vint/gate/diff/agent-pick/all\endcsname{-0.00}
\expandafter\def\csname v@vint/gate/diff/agent-pick/all-hi\endcsname{+0.00}
\expandafter\def\csname v@vint/gate/diff/agent-pick/all-lo\endcsname{-0.01}
\expandafter\def\csname v@vint/gate/diff/agent-pick/greet\endcsname{-0.02}
\expandafter\def\csname v@vint/gate/diff/agent-pick/greet-hi\endcsname{+0.00}
\expandafter\def\csname v@vint/gate/diff/agent-pick/greet-lo\endcsname{-0.05}
\expandafter\def\csname v@vint/gate/diff/agent-reuse/after\endcsname{-0.04}
\expandafter\def\csname v@vint/gate/diff/agent-reuse/after-hi\endcsname{+0.06}
\expandafter\def\csname v@vint/gate/diff/agent-reuse/after-lo\endcsname{-0.15}
\expandafter\def\csname v@vint/gate/diff/agent-reuse/all\endcsname{-0.41}
\expandafter\def\csname v@vint/gate/diff/agent-reuse/all-hi\endcsname{-0.26}
\expandafter\def\csname v@vint/gate/diff/agent-reuse/all-lo\endcsname{-0.57}
\expandafter\def\csname v@vint/gate/diff/agent-reuse/greet\endcsname{-3.32}
\expandafter\def\csname v@vint/gate/diff/agent-reuse/greet-hi\endcsname{-2.31}
\expandafter\def\csname v@vint/gate/diff/agent-reuse/greet-lo\endcsname{-4.40}
\expandafter\def\csname v@vint/gate/diff/ft-reuse/after\endcsname{+0.16}
\expandafter\def\csname v@vint/gate/diff/ft-reuse/after-hi\endcsname{+0.26}
\expandafter\def\csname v@vint/gate/diff/ft-reuse/after-lo\endcsname{+0.07}
\expandafter\def\csname v@vint/gate/diff/ft-reuse/all\endcsname{-0.09}
\expandafter\def\csname v@vint/gate/diff/ft-reuse/all-hi\endcsname{+0.02}
\expandafter\def\csname v@vint/gate/diff/ft-reuse/all-lo\endcsname{-0.20}
\expandafter\def\csname v@vint/gate/diff/ft-reuse/greet\endcsname{-2.03}
\expandafter\def\csname v@vint/gate/diff/ft-reuse/greet-hi\endcsname{-1.13}
\expandafter\def\csname v@vint/gate/diff/ft-reuse/greet-lo\endcsname{-3.02}
\expandafter\def\csname v@vint/gate/diff/gate0-reuse/after\endcsname{+0.02}
\expandafter\def\csname v@vint/gate/diff/gate0-reuse/after-hi\endcsname{+0.12}
\expandafter\def\csname v@vint/gate/diff/gate0-reuse/after-lo\endcsname{-0.09}
\expandafter\def\csname v@vint/gate/diff/gate0-reuse/all\endcsname{-0.36}
\expandafter\def\csname v@vint/gate/diff/gate0-reuse/all-hi\endcsname{-0.22}
\expandafter\def\csname v@vint/gate/diff/gate0-reuse/all-lo\endcsname{-0.52}
\expandafter\def\csname v@vint/gate/diff/gate0-reuse/greet\endcsname{-3.34}
\expandafter\def\csname v@vint/gate/diff/gate0-reuse/greet-hi\endcsname{-2.33}
\expandafter\def\csname v@vint/gate/diff/gate0-reuse/greet-lo\endcsname{-4.45}
\expandafter\def\csname v@vint/gate/diff/pick-reuse/after\endcsname{-0.04}
\expandafter\def\csname v@vint/gate/diff/pick-reuse/after-hi\endcsname{+0.06}
\expandafter\def\csname v@vint/gate/diff/pick-reuse/after-lo\endcsname{-0.15}
\expandafter\def\csname v@vint/gate/diff/pick-reuse/all\endcsname{-0.41}
\expandafter\def\csname v@vint/gate/diff/pick-reuse/all-hi\endcsname{-0.26}
\expandafter\def\csname v@vint/gate/diff/pick-reuse/all-lo\endcsname{-0.57}
\expandafter\def\csname v@vint/gate/diff/pick-reuse/greet\endcsname{-3.31}
\expandafter\def\csname v@vint/gate/diff/pick-reuse/greet-hi\endcsname{-2.29}
\expandafter\def\csname v@vint/gate/diff/pick-reuse/greet-lo\endcsname{-4.39}
\expandafter\def\csname v@vint/gate/engine/calls\endcsname{8}
\expandafter\def\csname v@vint/gate/engine/fp16-differ\endcsname{0.00}
\expandafter\def\csname v@vint/gate/engine/fp16-differ-n\endcsname{0}
\expandafter\def\csname v@vint/gate/engine/fp16-snr-min\endcsname{55}
\expandafter\def\csname v@vint/gate/engine/fp32-differ\endcsname{0.00}
\expandafter\def\csname v@vint/gate/engine/fp32-differ-n\endcsname{0}
\expandafter\def\csname v@vint/gate/engine/fp32-snr-min\endcsname{82}
\expandafter\def\csname v@vint/gate/engine/seconds\endcsname{60}
\expandafter\def\csname v@vint/gate/ft/after\endcsname{0.39}
\expandafter\def\csname v@vint/gate/ft/after-hi\endcsname{0.63}
\expandafter\def\csname v@vint/gate/ft/after-lo\endcsname{0.21}
\expandafter\def\csname v@vint/gate/ft/all\endcsname{0.86}
\expandafter\def\csname v@vint/gate/ft/all-hi\endcsname{1.21}
\expandafter\def\csname v@vint/gate/ft/all-lo\endcsname{0.56}
\expandafter\def\csname v@vint/gate/ft/greet\endcsname{4.51}
\expandafter\def\csname v@vint/gate/ft/greet-hi\endcsname{6.11}
\expandafter\def\csname v@vint/gate/ft/greet-lo\endcsname{3.08}
\expandafter\def\csname v@vint/gate/gate0/after\endcsname{0.25}
\expandafter\def\csname v@vint/gate/gate0/after-hi\endcsname{0.44}
\expandafter\def\csname v@vint/gate/gate0/after-lo\endcsname{0.12}
\expandafter\def\csname v@vint/gate/gate0/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/gate0/all-hi\endcsname{0.87}
\expandafter\def\csname v@vint/gate/gate0/all-lo\endcsname{0.36}
\expandafter\def\csname v@vint/gate/gate0/greet\endcsname{3.20}
\expandafter\def\csname v@vint/gate/gate0/greet-hi\endcsname{4.54}
\expandafter\def\csname v@vint/gate/gate0/greet-lo\endcsname{1.98}
\expandafter\def\csname v@vint/gate/none/after\endcsname{2.42}
\expandafter\def\csname v@vint/gate/none/after-hi\endcsname{3.29}
\expandafter\def\csname v@vint/gate/none/after-lo\endcsname{1.64}
\expandafter\def\csname v@vint/gate/none/all\endcsname{2.77}
\expandafter\def\csname v@vint/gate/none/all-hi\endcsname{3.73}
\expandafter\def\csname v@vint/gate/none/all-lo\endcsname{1.91}
\expandafter\def\csname v@vint/gate/none/greet\endcsname{5.52}
\expandafter\def\csname v@vint/gate/none/greet-hi\endcsname{7.39}
\expandafter\def\csname v@vint/gate/none/greet-lo\endcsname{3.80}
\expandafter\def\csname v@vint/gate/pick/after\endcsname{0.20}
\expandafter\def\csname v@vint/gate/pick/after-hi\endcsname{0.35}
\expandafter\def\csname v@vint/gate/pick/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/pick/all\endcsname{0.54}
\expandafter\def\csname v@vint/gate/pick/all-hi\endcsname{0.79}
\expandafter\def\csname v@vint/gate/pick/all-lo\endcsname{0.33}
\expandafter\def\csname v@vint/gate/pick/greet\endcsname{3.24}
\expandafter\def\csname v@vint/gate/pick/greet-hi\endcsname{4.60}
\expandafter\def\csname v@vint/gate/pick/greet-lo\endcsname{1.99}
\expandafter\def\csname v@vint/gate/reuse/after\endcsname{0.24}
\expandafter\def\csname v@vint/gate/reuse/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/gate/reuse/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/reuse/all\endcsname{0.95}
\expandafter\def\csname v@vint/gate/reuse/all-hi\endcsname{1.30}
\expandafter\def\csname v@vint/gate/reuse/all-lo\endcsname{0.63}
\expandafter\def\csname v@vint/gate/reuse/greet\endcsname{6.54}
\expandafter\def\csname v@vint/gate/reuse/greet-hi\endcsname{8.46}
\expandafter\def\csname v@vint/gate/reuse/greet-lo\endcsname{4.71}
\expandafter\def\csname v@vint/gate/sessions\endcsname{17}
\expandafter\def\csname v@vint/gate/silence/agent/after\endcsname{0.20}
\expandafter\def\csname v@vint/gate/silence/agent/after/silence\endcsname{98.6}
\expandafter\def\csname v@vint/gate/silence/agent/after/vad\endcsname{0.3}
\expandafter\def\csname v@vint/gate/silence/agent/all\endcsname{0.54}
\expandafter\def\csname v@vint/gate/silence/agent/before/silence\endcsname{87.3}
\expandafter\def\csname v@vint/gate/silence/agent/before/vad\endcsname{9.5}
\expandafter\def\csname v@vint/gate/silence/agent/greet\endcsname{3.22}
\expandafter\def\csname v@vint/gate/silence/agent/kind/babble/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/silence/agent/kind/babble/after-hi\endcsname{0.41}
\expandafter\def\csname v@vint/gate/silence/agent/kind/babble/after-lo\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/agent/kind/babble/after/silence\endcsname{98.7}
\expandafter\def\csname v@vint/gate/silence/agent/kind/babble/before/silence\endcsname{93.5}
\expandafter\def\csname v@vint/gate/silence/agent/kind/babble/greet\endcsname{2.11}
\expandafter\def\csname v@vint/gate/silence/agent/kind/babble/greet-hi\endcsname{3.52}
\expandafter\def\csname v@vint/gate/silence/agent/kind/babble/greet-lo\endcsname{0.95}
\expandafter\def\csname v@vint/gate/silence/agent/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/home/after\endcsname{0.12}
\expandafter\def\csname v@vint/gate/silence/agent/kind/home/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/silence/agent/kind/home/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/home/after/silence\endcsname{99.0}
\expandafter\def\csname v@vint/gate/silence/agent/kind/home/before/silence\endcsname{93.6}
\expandafter\def\csname v@vint/gate/silence/agent/kind/home/greet\endcsname{1.22}
\expandafter\def\csname v@vint/gate/silence/agent/kind/home/greet-hi\endcsname{2.24}
\expandafter\def\csname v@vint/gate/silence/agent/kind/home/greet-lo\endcsname{0.39}
\expandafter\def\csname v@vint/gate/silence/agent/kind/music/after\endcsname{0.10}
\expandafter\def\csname v@vint/gate/silence/agent/kind/music/after-hi\endcsname{0.21}
\expandafter\def\csname v@vint/gate/silence/agent/kind/music/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/music/after/silence\endcsname{99.4}
\expandafter\def\csname v@vint/gate/silence/agent/kind/music/before/silence\endcsname{99.6}
\expandafter\def\csname v@vint/gate/silence/agent/kind/music/greet\endcsname{0.09}
\expandafter\def\csname v@vint/gate/silence/agent/kind/music/greet-hi\endcsname{0.27}
\expandafter\def\csname v@vint/gate/silence/agent/kind/music/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/street/after\endcsname{0.01}
\expandafter\def\csname v@vint/gate/silence/agent/kind/street/after-hi\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/agent/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/street/after/silence\endcsname{99.8}
\expandafter\def\csname v@vint/gate/silence/agent/kind/street/before/silence\endcsname{99.0}
\expandafter\def\csname v@vint/gate/silence/agent/kind/street/greet\endcsname{0.17}
\expandafter\def\csname v@vint/gate/silence/agent/kind/street/greet-hi\endcsname{0.52}
\expandafter\def\csname v@vint/gate/silence/agent/kind/street/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/talker/after\endcsname{0.85}
\expandafter\def\csname v@vint/gate/silence/agent/kind/talker/after-hi\endcsname{1.88}
\expandafter\def\csname v@vint/gate/silence/agent/kind/talker/after-lo\endcsname{0.21}
\expandafter\def\csname v@vint/gate/silence/agent/kind/talker/after/silence\endcsname{95.5}
\expandafter\def\csname v@vint/gate/silence/agent/kind/talker/before/silence\endcsname{57.2}
\expandafter\def\csname v@vint/gate/silence/agent/kind/talker/greet\endcsname{14.90}
\expandafter\def\csname v@vint/gate/silence/agent/kind/talker/greet-hi\endcsname{18.00}
\expandafter\def\csname v@vint/gate/silence/agent/kind/talker/greet-lo\endcsname{12.18}
\expandafter\def\csname v@vint/gate/silence/agent/missed\endcsname{2.7}
\expandafter\def\csname v@vint/gate/silence/agent/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/silence/agent/trig/down-p50\endcsname{7}
\expandafter\def\csname v@vint/gate/silence/agent/trig/n\endcsname{93}
\expandafter\def\csname v@vint/gate/silence/agent/trig/over20\endcsname{16}
\expandafter\def\csname v@vint/gate/silence/agent/wer\endcsname{15.6}
\expandafter\def\csname v@vint/gate/silence/bed-calls\endcsname{765}
\expandafter\def\csname v@vint/gate/silence/calls\endcsname{816}
\expandafter\def\csname v@vint/gate/silence/ft/after\endcsname{0.39}
\expandafter\def\csname v@vint/gate/silence/ft/after/silence\endcsname{65.5}
\expandafter\def\csname v@vint/gate/silence/ft/after/vad\endcsname{0.7}
\expandafter\def\csname v@vint/gate/silence/ft/all\endcsname{0.86}
\expandafter\def\csname v@vint/gate/silence/ft/before/silence\endcsname{50.0}
\expandafter\def\csname v@vint/gate/silence/ft/before/vad\endcsname{12.2}
\expandafter\def\csname v@vint/gate/silence/ft/greet\endcsname{4.51}
\expandafter\def\csname v@vint/gate/silence/ft/kind/babble/after\endcsname{0.34}
\expandafter\def\csname v@vint/gate/silence/ft/kind/babble/after-hi\endcsname{0.69}
\expandafter\def\csname v@vint/gate/silence/ft/kind/babble/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/gate/silence/ft/kind/babble/after/silence\endcsname{56.9}
\expandafter\def\csname v@vint/gate/silence/ft/kind/babble/before/silence\endcsname{40.6}
\expandafter\def\csname v@vint/gate/silence/ft/kind/babble/greet\endcsname{3.96}
\expandafter\def\csname v@vint/gate/silence/ft/kind/babble/greet-hi\endcsname{5.42}
\expandafter\def\csname v@vint/gate/silence/ft/kind/babble/greet-lo\endcsname{2.46}
\expandafter\def\csname v@vint/gate/silence/ft/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/ft/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/ft/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/ft/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/ft/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/ft/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/ft/kind/home/after\endcsname{0.25}
\expandafter\def\csname v@vint/gate/silence/ft/kind/home/after-hi\endcsname{0.52}
\expandafter\def\csname v@vint/gate/silence/ft/kind/home/after-lo\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/ft/kind/home/after/silence\endcsname{71.8}
\expandafter\def\csname v@vint/gate/silence/ft/kind/home/before/silence\endcsname{59.6}
\expandafter\def\csname v@vint/gate/silence/ft/kind/home/greet\endcsname{2.10}
\expandafter\def\csname v@vint/gate/silence/ft/kind/home/greet-hi\endcsname{3.30}
\expandafter\def\csname v@vint/gate/silence/ft/kind/home/greet-lo\endcsname{1.10}
\expandafter\def\csname v@vint/gate/silence/ft/kind/music/after\endcsname{0.19}
\expandafter\def\csname v@vint/gate/silence/ft/kind/music/after-hi\endcsname{0.39}
\expandafter\def\csname v@vint/gate/silence/ft/kind/music/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/gate/silence/ft/kind/music/after/silence\endcsname{70.7}
\expandafter\def\csname v@vint/gate/silence/ft/kind/music/before/silence\endcsname{60.9}
\expandafter\def\csname v@vint/gate/silence/ft/kind/music/greet\endcsname{0.88}
\expandafter\def\csname v@vint/gate/silence/ft/kind/music/greet-hi\endcsname{1.83}
\expandafter\def\csname v@vint/gate/silence/ft/kind/music/greet-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/silence/ft/kind/street/after\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/ft/kind/street/after-hi\endcsname{0.09}
\expandafter\def\csname v@vint/gate/silence/ft/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/ft/kind/street/after/silence\endcsname{66.8}
\expandafter\def\csname v@vint/gate/silence/ft/kind/street/before/silence\endcsname{63.2}
\expandafter\def\csname v@vint/gate/silence/ft/kind/street/greet\endcsname{0.43}
\expandafter\def\csname v@vint/gate/silence/ft/kind/street/greet-hi\endcsname{0.78}
\expandafter\def\csname v@vint/gate/silence/ft/kind/street/greet-lo\endcsname{0.09}
\expandafter\def\csname v@vint/gate/silence/ft/kind/talker/after\endcsname{1.68}
\expandafter\def\csname v@vint/gate/silence/ft/kind/talker/after-hi\endcsname{3.17}
\expandafter\def\csname v@vint/gate/silence/ft/kind/talker/after-lo\endcsname{0.58}
\expandafter\def\csname v@vint/gate/silence/ft/kind/talker/after/silence\endcsname{59.9}
\expandafter\def\csname v@vint/gate/silence/ft/kind/talker/before/silence\endcsname{30.9}
\expandafter\def\csname v@vint/gate/silence/ft/kind/talker/greet\endcsname{18.25}
\expandafter\def\csname v@vint/gate/silence/ft/kind/talker/greet-hi\endcsname{20.83}
\expandafter\def\csname v@vint/gate/silence/ft/kind/talker/greet-lo\endcsname{15.83}
\expandafter\def\csname v@vint/gate/silence/ft/missed\endcsname{0.6}
\expandafter\def\csname v@vint/gate/silence/ft/recall\endcsname{91.1}
\expandafter\def\csname v@vint/gate/silence/ft/trig/down-p50\endcsname{11}
\expandafter\def\csname v@vint/gate/silence/ft/trig/n\endcsname{185}
\expandafter\def\csname v@vint/gate/silence/ft/trig/over20\endcsname{18}
\expandafter\def\csname v@vint/gate/silence/ft/wer\endcsname{13.0}
\expandafter\def\csname v@vint/gate/silence/gate0/after\endcsname{0.25}
\expandafter\def\csname v@vint/gate/silence/gate0/after/silence\endcsname{96.2}
\expandafter\def\csname v@vint/gate/silence/gate0/after/vad\endcsname{0.5}
\expandafter\def\csname v@vint/gate/silence/gate0/all\endcsname{0.59}
\expandafter\def\csname v@vint/gate/silence/gate0/before/silence\endcsname{86.6}
\expandafter\def\csname v@vint/gate/silence/gate0/before/vad\endcsname{10.0}
\expandafter\def\csname v@vint/gate/silence/gate0/greet\endcsname{3.20}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/babble/after\endcsname{0.24}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/babble/after-hi\endcsname{0.49}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/babble/after-lo\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/babble/after/silence\endcsname{95.8}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/babble/before/silence\endcsname{94.0}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/babble/greet\endcsname{1.94}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/babble/greet-hi\endcsname{3.40}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/babble/greet-lo\endcsname{0.79}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/home/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/home/after-hi\endcsname{0.37}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/home/after-lo\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/home/after/silence\endcsname{97.6}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/home/before/silence\endcsname{92.3}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/home/greet\endcsname{1.40}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/home/greet-hi\endcsname{2.37}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/home/greet-lo\endcsname{0.59}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/music/after\endcsname{0.11}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/music/after-hi\endcsname{0.23}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/music/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/music/after/silence\endcsname{97.3}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/music/before/silence\endcsname{99.6}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/music/greet\endcsname{0.09}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/music/greet-hi\endcsname{0.27}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/music/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/street/after\endcsname{0.01}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/street/after-hi\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/street/after/silence\endcsname{98.8}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/street/before/silence\endcsname{99.1}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/street/greet\endcsname{0.17}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/street/greet-hi\endcsname{0.52}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/street/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/talker/after\endcsname{1.06}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/talker/after-hi\endcsname{2.39}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/talker/after-lo\endcsname{0.26}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/talker/after/silence\endcsname{90.0}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/talker/before/silence\endcsname{54.9}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/talker/greet\endcsname{14.80}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/talker/greet-hi\endcsname{17.95}
\expandafter\def\csname v@vint/gate/silence/gate0/kind/talker/greet-lo\endcsname{12.03}
\expandafter\def\csname v@vint/gate/silence/gate0/missed\endcsname{2.5}
\expandafter\def\csname v@vint/gate/silence/gate0/recall\endcsname{89.1}
\expandafter\def\csname v@vint/gate/silence/gate0/trig/down-p50\endcsname{7}
\expandafter\def\csname v@vint/gate/silence/gate0/trig/n\endcsname{119}
\expandafter\def\csname v@vint/gate/silence/gate0/trig/over20\endcsname{16}
\expandafter\def\csname v@vint/gate/silence/gate0/wer\endcsname{15.4}
\expandafter\def\csname v@vint/gate/silence/none/after\endcsname{2.42}
\expandafter\def\csname v@vint/gate/silence/none/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/after/vad\endcsname{11.8}
\expandafter\def\csname v@vint/gate/silence/none/all\endcsname{2.77}
\expandafter\def\csname v@vint/gate/silence/none/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/before/vad\endcsname{18.3}
\expandafter\def\csname v@vint/gate/silence/none/greet\endcsname{5.52}
\expandafter\def\csname v@vint/gate/silence/none/kind/babble/after\endcsname{3.82}
\expandafter\def\csname v@vint/gate/silence/none/kind/babble/after-hi\endcsname{6.33}
\expandafter\def\csname v@vint/gate/silence/none/kind/babble/after-lo\endcsname{1.69}
\expandafter\def\csname v@vint/gate/silence/none/kind/babble/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/babble/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/babble/greet\endcsname{5.63}
\expandafter\def\csname v@vint/gate/silence/none/kind/babble/greet-hi\endcsname{7.27}
\expandafter\def\csname v@vint/gate/silence/none/kind/babble/greet-lo\endcsname{4.02}
\expandafter\def\csname v@vint/gate/silence/none/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/none/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/none/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/none/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/none/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/none/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/none/kind/home/after\endcsname{1.17}
\expandafter\def\csname v@vint/gate/silence/none/kind/home/after-hi\endcsname{1.95}
\expandafter\def\csname v@vint/gate/silence/none/kind/home/after-lo\endcsname{0.45}
\expandafter\def\csname v@vint/gate/silence/none/kind/home/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/home/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/home/greet\endcsname{2.54}
\expandafter\def\csname v@vint/gate/silence/none/kind/home/greet-hi\endcsname{4.14}
\expandafter\def\csname v@vint/gate/silence/none/kind/home/greet-lo\endcsname{1.10}
\expandafter\def\csname v@vint/gate/silence/none/kind/music/after\endcsname{0.07}
\expandafter\def\csname v@vint/gate/silence/none/kind/music/after-hi\endcsname{0.13}
\expandafter\def\csname v@vint/gate/silence/none/kind/music/after-lo\endcsname{0.02}
\expandafter\def\csname v@vint/gate/silence/none/kind/music/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/music/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/music/greet\endcsname{0.80}
\expandafter\def\csname v@vint/gate/silence/none/kind/music/greet-hi\endcsname{2.11}
\expandafter\def\csname v@vint/gate/silence/none/kind/music/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/none/kind/street/after\endcsname{0.69}
\expandafter\def\csname v@vint/gate/silence/none/kind/street/after-hi\endcsname{1.24}
\expandafter\def\csname v@vint/gate/silence/none/kind/street/after-lo\endcsname{0.30}
\expandafter\def\csname v@vint/gate/silence/none/kind/street/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/street/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/street/greet\endcsname{0.87}
\expandafter\def\csname v@vint/gate/silence/none/kind/street/greet-hi\endcsname{1.53}
\expandafter\def\csname v@vint/gate/silence/none/kind/street/greet-lo\endcsname{0.26}
\expandafter\def\csname v@vint/gate/silence/none/kind/talker/after\endcsname{9.35}
\expandafter\def\csname v@vint/gate/silence/none/kind/talker/after-hi\endcsname{10.38}
\expandafter\def\csname v@vint/gate/silence/none/kind/talker/after-lo\endcsname{8.28}
\expandafter\def\csname v@vint/gate/silence/none/kind/talker/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/talker/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/gate/silence/none/kind/talker/greet\endcsname{21.41}
\expandafter\def\csname v@vint/gate/silence/none/kind/talker/greet-hi\endcsname{23.43}
\expandafter\def\csname v@vint/gate/silence/none/kind/talker/greet-lo\endcsname{18.95}
\expandafter\def\csname v@vint/gate/silence/none/missed\endcsname{0.4}
\expandafter\def\csname v@vint/gate/silence/none/recall\endcsname{94.4}
\expandafter\def\csname v@vint/gate/silence/none/trig/down-p50\endcsname{0}
\expandafter\def\csname v@vint/gate/silence/none/trig/n\endcsname{1136}
\expandafter\def\csname v@vint/gate/silence/none/trig/over20\endcsname{0}
\expandafter\def\csname v@vint/gate/silence/none/wer\endcsname{7.4}
\expandafter\def\csname v@vint/gate/silence/pick/after\endcsname{0.20}
\expandafter\def\csname v@vint/gate/silence/pick/after/silence\endcsname{98.6}
\expandafter\def\csname v@vint/gate/silence/pick/after/vad\endcsname{0.3}
\expandafter\def\csname v@vint/gate/silence/pick/all\endcsname{0.54}
\expandafter\def\csname v@vint/gate/silence/pick/before/silence\endcsname{87.3}
\expandafter\def\csname v@vint/gate/silence/pick/before/vad\endcsname{9.6}
\expandafter\def\csname v@vint/gate/silence/pick/greet\endcsname{3.24}
\expandafter\def\csname v@vint/gate/silence/pick/kind/babble/after\endcsname{0.18}
\expandafter\def\csname v@vint/gate/silence/pick/kind/babble/after-hi\endcsname{0.41}
\expandafter\def\csname v@vint/gate/silence/pick/kind/babble/after-lo\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/pick/kind/babble/after/silence\endcsname{98.7}
\expandafter\def\csname v@vint/gate/silence/pick/kind/babble/before/silence\endcsname{93.5}
\expandafter\def\csname v@vint/gate/silence/pick/kind/babble/greet\endcsname{2.11}
\expandafter\def\csname v@vint/gate/silence/pick/kind/babble/greet-hi\endcsname{3.52}
\expandafter\def\csname v@vint/gate/silence/pick/kind/babble/greet-lo\endcsname{0.95}
\expandafter\def\csname v@vint/gate/silence/pick/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/home/after\endcsname{0.12}
\expandafter\def\csname v@vint/gate/silence/pick/kind/home/after-hi\endcsname{0.26}
\expandafter\def\csname v@vint/gate/silence/pick/kind/home/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/home/after/silence\endcsname{99.0}
\expandafter\def\csname v@vint/gate/silence/pick/kind/home/before/silence\endcsname{93.7}
\expandafter\def\csname v@vint/gate/silence/pick/kind/home/greet\endcsname{1.22}
\expandafter\def\csname v@vint/gate/silence/pick/kind/home/greet-hi\endcsname{2.24}
\expandafter\def\csname v@vint/gate/silence/pick/kind/home/greet-lo\endcsname{0.39}
\expandafter\def\csname v@vint/gate/silence/pick/kind/music/after\endcsname{0.10}
\expandafter\def\csname v@vint/gate/silence/pick/kind/music/after-hi\endcsname{0.21}
\expandafter\def\csname v@vint/gate/silence/pick/kind/music/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/music/after/silence\endcsname{99.4}
\expandafter\def\csname v@vint/gate/silence/pick/kind/music/before/silence\endcsname{99.6}
\expandafter\def\csname v@vint/gate/silence/pick/kind/music/greet\endcsname{0.09}
\expandafter\def\csname v@vint/gate/silence/pick/kind/music/greet-hi\endcsname{0.27}
\expandafter\def\csname v@vint/gate/silence/pick/kind/music/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/street/after\endcsname{0.01}
\expandafter\def\csname v@vint/gate/silence/pick/kind/street/after-hi\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/pick/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/street/after/silence\endcsname{99.8}
\expandafter\def\csname v@vint/gate/silence/pick/kind/street/before/silence\endcsname{99.0}
\expandafter\def\csname v@vint/gate/silence/pick/kind/street/greet\endcsname{0.17}
\expandafter\def\csname v@vint/gate/silence/pick/kind/street/greet-hi\endcsname{0.52}
\expandafter\def\csname v@vint/gate/silence/pick/kind/street/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/talker/after\endcsname{0.85}
\expandafter\def\csname v@vint/gate/silence/pick/kind/talker/after-hi\endcsname{1.88}
\expandafter\def\csname v@vint/gate/silence/pick/kind/talker/after-lo\endcsname{0.21}
\expandafter\def\csname v@vint/gate/silence/pick/kind/talker/after/silence\endcsname{95.5}
\expandafter\def\csname v@vint/gate/silence/pick/kind/talker/before/silence\endcsname{57.0}
\expandafter\def\csname v@vint/gate/silence/pick/kind/talker/greet\endcsname{15.00}
\expandafter\def\csname v@vint/gate/silence/pick/kind/talker/greet-hi\endcsname{18.10}
\expandafter\def\csname v@vint/gate/silence/pick/kind/talker/greet-lo\endcsname{12.26}
\expandafter\def\csname v@vint/gate/silence/pick/missed\endcsname{2.7}
\expandafter\def\csname v@vint/gate/silence/pick/recall\endcsname{88.4}
\expandafter\def\csname v@vint/gate/silence/pick/trig/down-p50\endcsname{7}
\expandafter\def\csname v@vint/gate/silence/pick/trig/n\endcsname{93}
\expandafter\def\csname v@vint/gate/silence/pick/trig/over20\endcsname{16}
\expandafter\def\csname v@vint/gate/silence/pick/wer\endcsname{15.6}
\expandafter\def\csname v@vint/gate/silence/reuse/after\endcsname{0.24}
\expandafter\def\csname v@vint/gate/silence/reuse/after/silence\endcsname{98.3}
\expandafter\def\csname v@vint/gate/silence/reuse/after/vad\endcsname{1.1}
\expandafter\def\csname v@vint/gate/silence/reuse/all\endcsname{0.95}
\expandafter\def\csname v@vint/gate/silence/reuse/before/silence\endcsname{49.1}
\expandafter\def\csname v@vint/gate/silence/reuse/before/vad\endcsname{17.7}
\expandafter\def\csname v@vint/gate/silence/reuse/greet\endcsname{6.54}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/babble/after\endcsname{0.06}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/babble/after-hi\endcsname{0.14}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/babble/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/babble/after/silence\endcsname{99.9}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/babble/before/silence\endcsname{47.3}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/babble/greet\endcsname{8.45}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/babble/greet-hi\endcsname{11.99}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/babble/greet-lo\endcsname{5.13}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/home/after\endcsname{0.04}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/home/after-hi\endcsname{0.10}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/home/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/home/after/silence\endcsname{99.9}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/home/before/silence\endcsname{51.3}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/home/greet\endcsname{4.37}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/home/greet-hi\endcsname{6.67}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/home/greet-lo\endcsname{2.16}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/music/after\endcsname{0.03}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/music/after-hi\endcsname{0.08}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/music/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/music/after/silence\endcsname{100.0}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/music/before/silence\endcsname{72.6}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/music/greet\endcsname{0.80}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/music/greet-hi\endcsname{1.66}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/music/greet-lo\endcsname{0.08}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/street/after\endcsname{0.02}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/street/after-hi\endcsname{0.05}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/street/after/silence\endcsname{100.0}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/street/before/silence\endcsname{59.5}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/street/greet\endcsname{1.30}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/street/greet-hi\endcsname{2.00}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/street/greet-lo\endcsname{0.65}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/talker/after\endcsname{1.47}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/talker/after-hi\endcsname{2.89}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/talker/after-lo\endcsname{0.41}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/talker/after/silence\endcsname{89.0}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/talker/before/silence\endcsname{21.5}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/talker/greet\endcsname{21.70}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/talker/greet-hi\endcsname{23.80}
\expandafter\def\csname v@vint/gate/silence/reuse/kind/talker/greet-lo\endcsname{19.67}
\expandafter\def\csname v@vint/gate/silence/reuse/missed\endcsname{2.6}
\expandafter\def\csname v@vint/gate/silence/reuse/recall\endcsname{87.2}
\expandafter\def\csname v@vint/gate/silence/reuse/trig/down-p50\endcsname{5}
\expandafter\def\csname v@vint/gate/silence/reuse/trig/n\endcsname{111}
\expandafter\def\csname v@vint/gate/silence/reuse/trig/over20\endcsname{5}
\expandafter\def\csname v@vint/gate/silence/reuse/wer\endcsname{16.9}
\expandafter\def\csname v@vint/gate/test/agent/cut\endcsname{84.8}
\expandafter\def\csname v@vint/gate/test/agent/cut-miss\endcsname{15.2}
\expandafter\def\csname v@vint/gate/test/agent/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/test/agent/cut-p90\endcsname{0.87}
\expandafter\def\csname v@vint/gate/test/ft/cut\endcsname{89.7}
\expandafter\def\csname v@vint/gate/test/ft/cut-miss\endcsname{10.3}
\expandafter\def\csname v@vint/gate/test/ft/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/test/ft/cut-p90\endcsname{0.76}
\expandafter\def\csname v@vint/gate/test/gate0/cut\endcsname{85.2}
\expandafter\def\csname v@vint/gate/test/gate0/cut-miss\endcsname{14.8}
\expandafter\def\csname v@vint/gate/test/gate0/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/test/gate0/cut-p90\endcsname{0.83}
\expandafter\def\csname v@vint/gate/test/none/cut\endcsname{84.8}
\expandafter\def\csname v@vint/gate/test/none/cut-miss\endcsname{15.2}
\expandafter\def\csname v@vint/gate/test/none/cut-p50\endcsname{0.61}
\expandafter\def\csname v@vint/gate/test/none/cut-p90\endcsname{0.76}
\expandafter\def\csname v@vint/gate/test/pick/cut\endcsname{84.8}
\expandafter\def\csname v@vint/gate/test/pick/cut-miss\endcsname{15.2}
\expandafter\def\csname v@vint/gate/test/pick/cut-p50\endcsname{0.67}
\expandafter\def\csname v@vint/gate/test/pick/cut-p90\endcsname{0.87}
\expandafter\def\csname v@vint/gate/test/reuse/cut\endcsname{87.4}
\expandafter\def\csname v@vint/gate/test/reuse/cut-miss\endcsname{12.6}
\expandafter\def\csname v@vint/gate/test/reuse/cut-p50\endcsname{0.68}
\expandafter\def\csname v@vint/gate/test/reuse/cut-p90\endcsname{0.86}
\expandafter\def\csname v@vint/greet/cpu/after\endcsname{0.80}
\expandafter\def\csname v@vint/greet/cpu/after-hi\endcsname{1.24}
\expandafter\def\csname v@vint/greet/cpu/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/greet/cpu/all\endcsname{1.36}
\expandafter\def\csname v@vint/greet/cpu/all-hi\endcsname{1.88}
\expandafter\def\csname v@vint/greet/cpu/all-lo\endcsname{0.93}
\expandafter\def\csname v@vint/greet/cpu/greet\endcsname{5.77}
\expandafter\def\csname v@vint/greet/cpu/greet-hi\endcsname{7.41}
\expandafter\def\csname v@vint/greet/cpu/greet-lo\endcsname{4.21}
\expandafter\def\csname v@vint/greet/cpu/n-after\endcsname{378}
\expandafter\def\csname v@vint/greet/cpu/n-greet\endcsname{344}
\expandafter\def\csname v@vint/greet/cpu/share\endcsname{48}
\expandafter\def\csname v@vint/greet/cpu/share-hi\endcsname{60}
\expandafter\def\csname v@vint/greet/cpu/share-lo\endcsname{39}
\expandafter\def\csname v@vint/greet/cpu8_ship/after\endcsname{0.80}
\expandafter\def\csname v@vint/greet/cpu8_ship/after-hi\endcsname{1.24}
\expandafter\def\csname v@vint/greet/cpu8_ship/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/greet/cpu8_ship/all\endcsname{1.36}
\expandafter\def\csname v@vint/greet/cpu8_ship/all-hi\endcsname{1.88}
\expandafter\def\csname v@vint/greet/cpu8_ship/all-lo\endcsname{0.93}
\expandafter\def\csname v@vint/greet/cpu8_ship/greet\endcsname{5.77}
\expandafter\def\csname v@vint/greet/cpu8_ship/greet-hi\endcsname{7.41}
\expandafter\def\csname v@vint/greet/cpu8_ship/greet-lo\endcsname{4.21}
\expandafter\def\csname v@vint/greet/cpu8_ship/n-after\endcsname{378}
\expandafter\def\csname v@vint/greet/cpu8_ship/n-greet\endcsname{344}
\expandafter\def\csname v@vint/greet/cpu8_ship/share\endcsname{48}
\expandafter\def\csname v@vint/greet/cpu8_ship/share-hi\endcsname{60}
\expandafter\def\csname v@vint/greet/cpu8_ship/share-lo\endcsname{39}
\expandafter\def\csname v@vint/greet/cpu8_vb/after\endcsname{0.82}
\expandafter\def\csname v@vint/greet/cpu8_vb/after-hi\endcsname{1.25}
\expandafter\def\csname v@vint/greet/cpu8_vb/after-lo\endcsname{0.45}
\expandafter\def\csname v@vint/greet/cpu8_vb/all\endcsname{1.13}
\expandafter\def\csname v@vint/greet/cpu8_vb/all-hi\endcsname{1.59}
\expandafter\def\csname v@vint/greet/cpu8_vb/all-lo\endcsname{0.75}
\expandafter\def\csname v@vint/greet/cpu8_vb/greet\endcsname{3.61}
\expandafter\def\csname v@vint/greet/cpu8_vb/greet-hi\endcsname{4.66}
\expandafter\def\csname v@vint/greet/cpu8_vb/greet-lo\endcsname{2.64}
\expandafter\def\csname v@vint/greet/cpu8_vb/n-after\endcsname{384}
\expandafter\def\csname v@vint/greet/cpu8_vb/n-greet\endcsname{215}
\expandafter\def\csname v@vint/greet/cpu8_vb/share\endcsname{36}
\expandafter\def\csname v@vint/greet/cpu8_vb/share-hi\endcsname{48}
\expandafter\def\csname v@vint/greet/cpu8_vb/share-lo\endcsname{28}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/after\endcsname{+0.01}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/after-hi\endcsname{+0.03}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/after-lo\endcsname{-0.00}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/all\endcsname{-0.23}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/all-hi\endcsname{-0.14}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/all-lo\endcsname{-0.34}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/greet\endcsname{-2.16}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/greet-hi\endcsname{-1.27}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/greet-lo\endcsname{-3.12}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/share\endcsname{-12}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/share-hi\endcsname{-7}
\expandafter\def\csname v@vint/greet/cpu8_vb/vs-cpu8_ship/share-lo\endcsname{-16}
\expandafter\def\csname v@vint/greet/cpu_ship/after\endcsname{0.80}
\expandafter\def\csname v@vint/greet/cpu_ship/after-hi\endcsname{1.23}
\expandafter\def\csname v@vint/greet/cpu_ship/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/greet/cpu_ship/all\endcsname{1.36}
\expandafter\def\csname v@vint/greet/cpu_ship/all-hi\endcsname{1.87}
\expandafter\def\csname v@vint/greet/cpu_ship/all-lo\endcsname{0.92}
\expandafter\def\csname v@vint/greet/cpu_ship/greet\endcsname{5.74}
\expandafter\def\csname v@vint/greet/cpu_ship/greet-hi\endcsname{7.39}
\expandafter\def\csname v@vint/greet/cpu_ship/greet-lo\endcsname{4.18}
\expandafter\def\csname v@vint/greet/cpu_ship/n-after\endcsname{376}
\expandafter\def\csname v@vint/greet/cpu_ship/n-greet\endcsname{342}
\expandafter\def\csname v@vint/greet/cpu_ship/share\endcsname{48}
\expandafter\def\csname v@vint/greet/cpu_ship/share-hi\endcsname{60}
\expandafter\def\csname v@vint/greet/cpu_ship/share-lo\endcsname{39}
\expandafter\def\csname v@vint/greet/cpu_vb/after\endcsname{0.80}
\expandafter\def\csname v@vint/greet/cpu_vb/after-hi\endcsname{1.23}
\expandafter\def\csname v@vint/greet/cpu_vb/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/greet/cpu_vb/all\endcsname{1.13}
\expandafter\def\csname v@vint/greet/cpu_vb/all-hi\endcsname{1.58}
\expandafter\def\csname v@vint/greet/cpu_vb/all-lo\endcsname{0.75}
\expandafter\def\csname v@vint/greet/cpu_vb/greet\endcsname{3.69}
\expandafter\def\csname v@vint/greet/cpu_vb/greet-hi\endcsname{4.77}
\expandafter\def\csname v@vint/greet/cpu_vb/greet-lo\endcsname{2.70}
\expandafter\def\csname v@vint/greet/cpu_vb/n-after\endcsname{378}
\expandafter\def\csname v@vint/greet/cpu_vb/n-greet\endcsname{220}
\expandafter\def\csname v@vint/greet/cpu_vb/share\endcsname{37}
\expandafter\def\csname v@vint/greet/cpu_vb/share-hi\endcsname{49}
\expandafter\def\csname v@vint/greet/cpu_vb/share-lo\endcsname{28}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/after\endcsname{+0.00}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/after-hi\endcsname{+0.03}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/after-lo\endcsname{-0.02}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/all\endcsname{-0.23}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/all-hi\endcsname{-0.13}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/all-lo\endcsname{-0.34}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/greet\endcsname{-2.05}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/greet-hi\endcsname{-1.16}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/greet-lo\endcsname{-3.01}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/share\endcsname{-11}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/share-hi\endcsname{-6}
\expandafter\def\csname v@vint/greet/cpu_vb/vs-cpu_ship/share-lo\endcsname{-15}
\expandafter\def\csname v@vint/greet/ft/after\endcsname{0.39}
\expandafter\def\csname v@vint/greet/ft/after-hi\endcsname{0.63}
\expandafter\def\csname v@vint/greet/ft/after-lo\endcsname{0.21}
\expandafter\def\csname v@vint/greet/ft/all\endcsname{0.86}
\expandafter\def\csname v@vint/greet/ft/all-hi\endcsname{1.21}
\expandafter\def\csname v@vint/greet/ft/all-lo\endcsname{0.56}
\expandafter\def\csname v@vint/greet/ft/greet\endcsname{4.51}
\expandafter\def\csname v@vint/greet/ft/greet-hi\endcsname{6.11}
\expandafter\def\csname v@vint/greet/ft/greet-lo\endcsname{3.08}
\expandafter\def\csname v@vint/greet/ft/n-after\endcsname{185}
\expandafter\def\csname v@vint/greet/ft/n-greet\endcsname{269}
\expandafter\def\csname v@vint/greet/ft/share\endcsname{59}
\expandafter\def\csname v@vint/greet/ft/share-hi\endcsname{71}
\expandafter\def\csname v@vint/greet/ft/share-lo\endcsname{49}
\expandafter\def\csname v@vint/greet/gtcrn/after\endcsname{5.07}
\expandafter\def\csname v@vint/greet/gtcrn/after-hi\endcsname{6.09}
\expandafter\def\csname v@vint/greet/gtcrn/after-lo\endcsname{4.10}
\expandafter\def\csname v@vint/greet/gtcrn/all\endcsname{5.33}
\expandafter\def\csname v@vint/greet/gtcrn/all-hi\endcsname{6.39}
\expandafter\def\csname v@vint/greet/gtcrn/all-lo\endcsname{4.31}
\expandafter\def\csname v@vint/greet/gtcrn/greet\endcsname{7.33}
\expandafter\def\csname v@vint/greet/gtcrn/greet-hi\endcsname{9.23}
\expandafter\def\csname v@vint/greet/gtcrn/greet-lo\endcsname{5.53}
\expandafter\def\csname v@vint/greet/gtcrn/n-after\endcsname{2382}
\expandafter\def\csname v@vint/greet/gtcrn/n-greet\endcsname{437}
\expandafter\def\csname v@vint/greet/gtcrn/share\endcsname{16}
\expandafter\def\csname v@vint/greet/gtcrn/share-hi\endcsname{18}
\expandafter\def\csname v@vint/greet/gtcrn/share-lo\endcsname{13}
\expandafter\def\csname v@vint/greet/iso/share-max\endcsname{78}
\expandafter\def\csname v@vint/greet/iso/share-min\endcsname{48}
\expandafter\def\csname v@vint/greet/lead-pct\endcsname{11}
\expandafter\def\csname v@vint/greet/none/after\endcsname{2.42}
\expandafter\def\csname v@vint/greet/none/after-hi\endcsname{3.29}
\expandafter\def\csname v@vint/greet/none/after-lo\endcsname{1.64}
\expandafter\def\csname v@vint/greet/none/all\endcsname{2.77}
\expandafter\def\csname v@vint/greet/none/all-hi\endcsname{3.73}
\expandafter\def\csname v@vint/greet/none/all-lo\endcsname{1.91}
\expandafter\def\csname v@vint/greet/none/greet\endcsname{5.52}
\expandafter\def\csname v@vint/greet/none/greet-hi\endcsname{7.39}
\expandafter\def\csname v@vint/greet/none/greet-lo\endcsname{3.80}
\expandafter\def\csname v@vint/greet/none/n-after\endcsname{1136}
\expandafter\def\csname v@vint/greet/none/n-greet\endcsname{329}
\expandafter\def\csname v@vint/greet/none/share\endcsname{22}
\expandafter\def\csname v@vint/greet/none/share-hi\endcsname{27}
\expandafter\def\csname v@vint/greet/none/share-lo\endcsname{19}
\expandafter\def\csname v@vint/greet/rel/after\endcsname{0.50}
\expandafter\def\csname v@vint/greet/rel/after-hi\endcsname{0.82}
\expandafter\def\csname v@vint/greet/rel/after-lo\endcsname{0.26}
\expandafter\def\csname v@vint/greet/rel/all\endcsname{1.05}
\expandafter\def\csname v@vint/greet/rel/all-hi\endcsname{1.48}
\expandafter\def\csname v@vint/greet/rel/all-lo\endcsname{0.69}
\expandafter\def\csname v@vint/greet/rel/greet\endcsname{5.32}
\expandafter\def\csname v@vint/greet/rel/greet-hi\endcsname{7.06}
\expandafter\def\csname v@vint/greet/rel/greet-lo\endcsname{3.73}
\expandafter\def\csname v@vint/greet/rel/n-after\endcsname{237}
\expandafter\def\csname v@vint/greet/rel/n-greet\endcsname{317}
\expandafter\def\csname v@vint/greet/rel/share\endcsname{57}
\expandafter\def\csname v@vint/greet/rel/share-hi\endcsname{70}
\expandafter\def\csname v@vint/greet/rel/share-lo\endcsname{48}
\expandafter\def\csname v@vint/greet/rel_ship/after\endcsname{0.50}
\expandafter\def\csname v@vint/greet/rel_ship/after-hi\endcsname{0.81}
\expandafter\def\csname v@vint/greet/rel_ship/after-lo\endcsname{0.25}
\expandafter\def\csname v@vint/greet/rel_ship/all\endcsname{1.02}
\expandafter\def\csname v@vint/greet/rel_ship/all-hi\endcsname{1.45}
\expandafter\def\csname v@vint/greet/rel_ship/all-lo\endcsname{0.66}
\expandafter\def\csname v@vint/greet/rel_ship/greet\endcsname{5.17}
\expandafter\def\csname v@vint/greet/rel_ship/greet-hi\endcsname{6.88}
\expandafter\def\csname v@vint/greet/rel_ship/greet-lo\endcsname{3.60}
\expandafter\def\csname v@vint/greet/rel_ship/n-after\endcsname{233}
\expandafter\def\csname v@vint/greet/rel_ship/n-greet\endcsname{308}
\expandafter\def\csname v@vint/greet/rel_ship/share\endcsname{57}
\expandafter\def\csname v@vint/greet/rel_ship/share-hi\endcsname{70}
\expandafter\def\csname v@vint/greet/rel_ship/share-lo\endcsname{47}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/after\endcsname{+0.26}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/after-hi\endcsname{+0.40}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/after-lo\endcsname{+0.14}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/all\endcsname{+0.08}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/all-hi\endcsname{+0.21}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/all-lo\endcsname{-0.05}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/greet\endcsname{-1.38}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/greet-hi\endcsname{-0.51}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/greet-lo\endcsname{-2.37}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/share\endcsname{-21}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/share-hi\endcsname{-14}
\expandafter\def\csname v@vint/greet/rel_ship/vs-reuse/share-lo\endcsname{-29}
\expandafter\def\csname v@vint/greet/rel_vb/after\endcsname{0.50}
\expandafter\def\csname v@vint/greet/rel_vb/after-hi\endcsname{0.81}
\expandafter\def\csname v@vint/greet/rel_vb/after-lo\endcsname{0.25}
\expandafter\def\csname v@vint/greet/rel_vb/all\endcsname{0.78}
\expandafter\def\csname v@vint/greet/rel_vb/all-hi\endcsname{1.13}
\expandafter\def\csname v@vint/greet/rel_vb/all-lo\endcsname{0.49}
\expandafter\def\csname v@vint/greet/rel_vb/greet\endcsname{3.02}
\expandafter\def\csname v@vint/greet/rel_vb/greet-hi\endcsname{3.97}
\expandafter\def\csname v@vint/greet/rel_vb/greet-lo\endcsname{2.12}
\expandafter\def\csname v@vint/greet/rel_vb/n-after\endcsname{233}
\expandafter\def\csname v@vint/greet/rel_vb/n-greet\endcsname{180}
\expandafter\def\csname v@vint/greet/rel_vb/share\endcsname{44}
\expandafter\def\csname v@vint/greet/rel_vb/share-hi\endcsname{59}
\expandafter\def\csname v@vint/greet/rel_vb/share-lo\endcsname{33}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/after\endcsname{+0.00}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/after-hi\endcsname{+0.01}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/after-lo\endcsname{-0.01}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/all\endcsname{-0.24}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/all-hi\endcsname{-0.13}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/all-lo\endcsname{-0.37}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/greet\endcsname{-2.15}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/greet-hi\endcsname{-1.20}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/greet-lo\endcsname{-3.22}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/share\endcsname{-13}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/share-hi\endcsname{-8}
\expandafter\def\csname v@vint/greet/rel_vb/vs-rel_ship/share-lo\endcsname{-18}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/after\endcsname{+0.26}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/after-hi\endcsname{+0.40}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/after-lo\endcsname{+0.14}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/all\endcsname{-0.17}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/all-hi\endcsname{-0.03}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/all-lo\endcsname{-0.31}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/greet\endcsname{-3.52}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/greet-hi\endcsname{-2.21}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/greet-lo\endcsname{-4.92}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/share\endcsname{-34}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/share-hi\endcsname{-26}
\expandafter\def\csname v@vint/greet/rel_vb/vs-reuse/share-lo\endcsname{-42}
\expandafter\def\csname v@vint/greet/reuse/after\endcsname{0.24}
\expandafter\def\csname v@vint/greet/reuse/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/greet/reuse/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/greet/reuse/all\endcsname{0.95}
\expandafter\def\csname v@vint/greet/reuse/all-hi\endcsname{1.30}
\expandafter\def\csname v@vint/greet/reuse/all-lo\endcsname{0.63}
\expandafter\def\csname v@vint/greet/reuse/greet\endcsname{6.54}
\expandafter\def\csname v@vint/greet/reuse/greet-hi\endcsname{8.46}
\expandafter\def\csname v@vint/greet/reuse/greet-lo\endcsname{4.71}
\expandafter\def\csname v@vint/greet/reuse/n-after\endcsname{111}
\expandafter\def\csname v@vint/greet/reuse/n-greet\endcsname{390}
\expandafter\def\csname v@vint/greet/reuse/share\endcsname{78}
\expandafter\def\csname v@vint/greet/reuse/share-hi\endcsname{91}
\expandafter\def\csname v@vint/greet/reuse/share-lo\endcsname{67}
\expandafter\def\csname v@vint/greet/voxlock/after\endcsname{0.65}
\expandafter\def\csname v@vint/greet/voxlock/after-hi\endcsname{1.00}
\expandafter\def\csname v@vint/greet/voxlock/after-lo\endcsname{0.36}
\expandafter\def\csname v@vint/greet/voxlock/all\endcsname{1.18}
\expandafter\def\csname v@vint/greet/voxlock/all-hi\endcsname{1.65}
\expandafter\def\csname v@vint/greet/voxlock/all-lo\endcsname{0.78}
\expandafter\def\csname v@vint/greet/voxlock/greet\endcsname{5.35}
\expandafter\def\csname v@vint/greet/voxlock/greet-hi\endcsname{7.13}
\expandafter\def\csname v@vint/greet/voxlock/greet-lo\endcsname{3.71}
\expandafter\def\csname v@vint/greet/voxlock/n-after\endcsname{305}
\expandafter\def\csname v@vint/greet/voxlock/n-greet\endcsname{319}
\expandafter\def\csname v@vint/greet/voxlock/share\endcsname{51}
\expandafter\def\csname v@vint/greet/voxlock/share-hi\endcsname{62}
\expandafter\def\csname v@vint/greet/voxlock/share-lo\endcsname{43}
\expandafter\def\csname v@vint/gtcrn/caught\endcsname{81.8}
\expandafter\def\csname v@vint/gtcrn/caught-d\endcsname{-8.0}
\expandafter\def\csname v@vint/gtcrn/caught-dabs\endcsname{8.0}
\expandafter\def\csname v@vint/gtcrn/caught-dhi\endcsname{-4.1}
\expandafter\def\csname v@vint/gtcrn/caught-dlo\endcsname{-12.4}
\expandafter\def\csname v@vint/gtcrn/caught-hi\endcsname{86.2}
\expandafter\def\csname v@vint/gtcrn/caught-lo\endcsname{76.9}
\expandafter\def\csname v@vint/gtcrn/core-pct\endcsname{6}
\expandafter\def\csname v@vint/gtcrn/cores\endcsname{0.06}
\expandafter\def\csname v@vint/gtcrn/fi\endcsname{5.33}
\expandafter\def\csname v@vint/gtcrn/fi-d\endcsname{+4.28}
\expandafter\def\csname v@vint/gtcrn/fi-dabs\endcsname{4.28}
\expandafter\def\csname v@vint/gtcrn/fi-dhi\endcsname{+5.17}
\expandafter\def\csname v@vint/gtcrn/fi-dlo\endcsname{+3.43}
\expandafter\def\csname v@vint/gtcrn/fi-hi\endcsname{6.39}
\expandafter\def\csname v@vint/gtcrn/fi-lo\endcsname{4.31}
\expandafter\def\csname v@vint/gtcrn/frame-p50\endcsname{2.5}
\expandafter\def\csname v@vint/gtcrn/frame-p99\endcsname{4.1}
\expandafter\def\csname v@vint/gtcrn/fs\endcsname{5.37}
\expandafter\def\csname v@vint/gtcrn/fs-d\endcsname{+4.14}
\expandafter\def\csname v@vint/gtcrn/fs-dabs\endcsname{4.14}
\expandafter\def\csname v@vint/gtcrn/fs-dhi\endcsname{+4.95}
\expandafter\def\csname v@vint/gtcrn/fs-dlo\endcsname{+3.35}
\expandafter\def\csname v@vint/gtcrn/fs-hi\endcsname{6.28}
\expandafter\def\csname v@vint/gtcrn/fs-lo\endcsname{4.44}
\expandafter\def\csname v@vint/gtcrn/held\endcsname{8.6}
\expandafter\def\csname v@vint/gtcrn/held-d\endcsname{+5.0}
\expandafter\def\csname v@vint/gtcrn/held-dabs\endcsname{5.0}
\expandafter\def\csname v@vint/gtcrn/held-dhi\endcsname{+8.1}
\expandafter\def\csname v@vint/gtcrn/held-dlo\endcsname{+2.4}
\expandafter\def\csname v@vint/gtcrn/held-hi\endcsname{12.6}
\expandafter\def\csname v@vint/gtcrn/held-lo\endcsname{5.1}
\expandafter\def\csname v@vint/gtcrn/kind/babble/fi\endcsname{8.76}
\expandafter\def\csname v@vint/gtcrn/kind/babble/fs\endcsname{8.44}
\expandafter\def\csname v@vint/gtcrn/kind/babble/missed\endcsname{0.4}
\expandafter\def\csname v@vint/gtcrn/kind/clean/fi\endcsname{0.00}
\expandafter\def\csname v@vint/gtcrn/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/gtcrn/kind/clean/missed\endcsname{0.0}
\expandafter\def\csname v@vint/gtcrn/kind/home/fi\endcsname{3.42}
\expandafter\def\csname v@vint/gtcrn/kind/home/fs\endcsname{3.62}
\expandafter\def\csname v@vint/gtcrn/kind/home/missed\endcsname{0.1}
\expandafter\def\csname v@vint/gtcrn/kind/music/fi\endcsname{3.09}
\expandafter\def\csname v@vint/gtcrn/kind/music/fs\endcsname{3.11}
\expandafter\def\csname v@vint/gtcrn/kind/music/missed\endcsname{0.1}
\expandafter\def\csname v@vint/gtcrn/kind/street/fi\endcsname{3.29}
\expandafter\def\csname v@vint/gtcrn/kind/street/fs\endcsname{3.28}
\expandafter\def\csname v@vint/gtcrn/kind/street/missed\endcsname{0.0}
\expandafter\def\csname v@vint/gtcrn/kind/talker/fi\endcsname{11.95}
\expandafter\def\csname v@vint/gtcrn/kind/talker/fs\endcsname{9.38}
\expandafter\def\csname v@vint/gtcrn/kind/talker/missed\endcsname{0.0}
\expandafter\def\csname v@vint/gtcrn/live/barge_p50\endcsname{0.67}
\expandafter\def\csname v@vint/gtcrn/live/caught\endcsname{94.9}
\expandafter\def\csname v@vint/gtcrn/live/eot_p50\endcsname{0.85}
\expandafter\def\csname v@vint/gtcrn/live/eot_p90\endcsname{2.00}
\expandafter\def\csname v@vint/gtcrn/live/fi_transcript\endcsname{5.05}
\expandafter\def\csname v@vint/gtcrn/live/fi_vad\endcsname{5.09}
\expandafter\def\csname v@vint/gtcrn/live/frame-p50\endcsname{3.2}
\expandafter\def\csname v@vint/gtcrn/live/frame-p99\endcsname{6.2}
\expandafter\def\csname v@vint/gtcrn/live/fs\endcsname{6.44}
\expandafter\def\csname v@vint/gtcrn/live/no_reply\endcsname{9.1}
\expandafter\def\csname v@vint/gtcrn/live/unfiltered_pct\endcsname{0.00}
\expandafter\def\csname v@vint/gtcrn/missed\endcsname{0.1}
\expandafter\def\csname v@vint/gtcrn/missed-d\endcsname{-0.6}
\expandafter\def\csname v@vint/gtcrn/missed-dabs\endcsname{0.6}
\expandafter\def\csname v@vint/gtcrn/missed-dhi\endcsname{-0.2}
\expandafter\def\csname v@vint/gtcrn/missed-dlo\endcsname{-1.0}
\expandafter\def\csname v@vint/gtcrn/missed-hi\endcsname{0.2}
\expandafter\def\csname v@vint/gtcrn/missed-lo\endcsname{0.0}
\expandafter\def\csname v@vint/gtcrn/recall\endcsname{95.4}
\expandafter\def\csname v@vint/gtcrn/snr/0.0/fi\endcsname{7.30}
\expandafter\def\csname v@vint/gtcrn/snr/10.0/fi\endcsname{6.23}
\expandafter\def\csname v@vint/gtcrn/snr/20.0/fi\endcsname{3.74}
\expandafter\def\csname v@vint/gtcrn/snr/None/fi\endcsname{0.00}
\expandafter\def\csname v@vint/gtcrn/wer\endcsname{11.0}
\expandafter\def\csname v@vint/gtcrn/wer/babble\endcsname{16.7}
\expandafter\def\csname v@vint/gtcrn/wer/clean\endcsname{1.6}
\expandafter\def\csname v@vint/gtcrn/wer/home\endcsname{12.6}
\expandafter\def\csname v@vint/gtcrn/wer/music\endcsname{7.9}
\expandafter\def\csname v@vint/gtcrn/wer/street\endcsname{8.1}
\expandafter\def\csname v@vint/gtcrn/wer/talker\endcsname{14.2}
\expandafter\def\csname v@vint/iw/agent/after\endcsname{0.20}
\expandafter\def\csname v@vint/iw/agent/after-hi\endcsname{0.35}
\expandafter\def\csname v@vint/iw/agent/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/iw/agent/all\endcsname{0.54}
\expandafter\def\csname v@vint/iw/agent/all-hi\endcsname{0.79}
\expandafter\def\csname v@vint/iw/agent/all-lo\endcsname{0.33}
\expandafter\def\csname v@vint/iw/agent/greet\endcsname{3.22}
\expandafter\def\csname v@vint/iw/agent/greet-hi\endcsname{4.58}
\expandafter\def\csname v@vint/iw/agent/greet-lo\endcsname{1.98}
\expandafter\def\csname v@vint/iw/cpu8/after\endcsname{0.80}
\expandafter\def\csname v@vint/iw/cpu8/after-hi\endcsname{1.24}
\expandafter\def\csname v@vint/iw/cpu8/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/iw/cpu8/all\endcsname{1.36}
\expandafter\def\csname v@vint/iw/cpu8/all-hi\endcsname{1.88}
\expandafter\def\csname v@vint/iw/cpu8/all-lo\endcsname{0.93}
\expandafter\def\csname v@vint/iw/cpu8/greet\endcsname{5.77}
\expandafter\def\csname v@vint/iw/cpu8/greet-hi\endcsname{7.41}
\expandafter\def\csname v@vint/iw/cpu8/greet-lo\endcsname{4.21}
\expandafter\def\csname v@vint/iw/cpuag8/after\endcsname{0.14}
\expandafter\def\csname v@vint/iw/cpuag8/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/iw/cpuag8/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/iw/cpuag8/all\endcsname{0.48}
\expandafter\def\csname v@vint/iw/cpuag8/all-hi\endcsname{0.71}
\expandafter\def\csname v@vint/iw/cpuag8/all-lo\endcsname{0.29}
\expandafter\def\csname v@vint/iw/cpuag8/greet\endcsname{3.14}
\expandafter\def\csname v@vint/iw/cpuag8/greet-hi\endcsname{4.45}
\expandafter\def\csname v@vint/iw/cpuag8/greet-lo\endcsname{1.94}
\expandafter\def\csname v@vint/iw/diff/inworld-agent/after\endcsname{+3.98}
\expandafter\def\csname v@vint/iw/diff/inworld-agent/after-hi\endcsname{+4.95}
\expandafter\def\csname v@vint/iw/diff/inworld-agent/after-lo\endcsname{+3.08}
\expandafter\def\csname v@vint/iw/diff/inworld-agent/all\endcsname{+3.98}
\expandafter\def\csname v@vint/iw/diff/inworld-agent/all-hi\endcsname{+4.93}
\expandafter\def\csname v@vint/iw/diff/inworld-agent/all-lo\endcsname{+3.11}
\expandafter\def\csname v@vint/iw/diff/inworld-cpuag8/after\endcsname{+4.04}
\expandafter\def\csname v@vint/iw/diff/inworld-cpuag8/after-hi\endcsname{+5.03}
\expandafter\def\csname v@vint/iw/diff/inworld-cpuag8/after-lo\endcsname{+3.13}
\expandafter\def\csname v@vint/iw/diff/inworld-cpuag8/all\endcsname{+4.04}
\expandafter\def\csname v@vint/iw/diff/inworld-cpuag8/all-hi\endcsname{+5.00}
\expandafter\def\csname v@vint/iw/diff/inworld-cpuag8/all-lo\endcsname{+3.17}
\expandafter\def\csname v@vint/iw/diff/inworld-none/after\endcsname{+1.76}
\expandafter\def\csname v@vint/iw/diff/inworld-none/after-hi\endcsname{+2.20}
\expandafter\def\csname v@vint/iw/diff/inworld-none/after-lo\endcsname{+1.33}
\expandafter\def\csname v@vint/iw/diff/inworld-none/all\endcsname{+1.75}
\expandafter\def\csname v@vint/iw/diff/inworld-none/all-hi\endcsname{+2.18}
\expandafter\def\csname v@vint/iw/diff/inworld-none/all-lo\endcsname{+1.34}
\expandafter\def\csname v@vint/iw/diff/inworld-reuse/after\endcsname{+3.94}
\expandafter\def\csname v@vint/iw/diff/inworld-reuse/after-hi\endcsname{+4.92}
\expandafter\def\csname v@vint/iw/diff/inworld-reuse/after-lo\endcsname{+3.05}
\expandafter\def\csname v@vint/iw/diff/inworld-reuse/all\endcsname{+3.58}
\expandafter\def\csname v@vint/iw/diff/inworld-reuse/all-hi\endcsname{+4.43}
\expandafter\def\csname v@vint/iw/diff/inworld-reuse/all-lo\endcsname{+2.79}
\expandafter\def\csname v@vint/iw/inworld/after\endcsname{4.18}
\expandafter\def\csname v@vint/iw/inworld/after-hi\endcsname{5.19}
\expandafter\def\csname v@vint/iw/inworld/after-lo\endcsname{3.24}
\expandafter\def\csname v@vint/iw/inworld/all\endcsname{4.52}
\expandafter\def\csname v@vint/iw/inworld/all-hi\endcsname{5.60}
\expandafter\def\csname v@vint/iw/inworld/all-lo\endcsname{3.54}
\expandafter\def\csname v@vint/iw/inworld/greet\endcsname{7.25}
\expandafter\def\csname v@vint/iw/inworld/greet-hi\endcsname{9.12}
\expandafter\def\csname v@vint/iw/inworld/greet-lo\endcsname{5.49}
\expandafter\def\csname v@vint/iw/none/after\endcsname{2.42}
\expandafter\def\csname v@vint/iw/none/after-hi\endcsname{3.29}
\expandafter\def\csname v@vint/iw/none/after-lo\endcsname{1.64}
\expandafter\def\csname v@vint/iw/none/all\endcsname{2.77}
\expandafter\def\csname v@vint/iw/none/all-hi\endcsname{3.73}
\expandafter\def\csname v@vint/iw/none/all-lo\endcsname{1.91}
\expandafter\def\csname v@vint/iw/none/greet\endcsname{5.52}
\expandafter\def\csname v@vint/iw/none/greet-hi\endcsname{7.39}
\expandafter\def\csname v@vint/iw/none/greet-lo\endcsname{3.80}
\expandafter\def\csname v@vint/iw/reuse/after\endcsname{0.24}
\expandafter\def\csname v@vint/iw/reuse/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/iw/reuse/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/iw/reuse/all\endcsname{0.95}
\expandafter\def\csname v@vint/iw/reuse/all-hi\endcsname{1.30}
\expandafter\def\csname v@vint/iw/reuse/all-lo\endcsname{0.63}
\expandafter\def\csname v@vint/iw/reuse/greet\endcsname{6.54}
\expandafter\def\csname v@vint/iw/reuse/greet-hi\endcsname{8.46}
\expandafter\def\csname v@vint/iw/reuse/greet-lo\endcsname{4.71}
\expandafter\def\csname v@vint/iw/silence/agent/after/down\endcsname{16.2}
\expandafter\def\csname v@vint/iw/silence/agent/after/silence\endcsname{98.6}
\expandafter\def\csname v@vint/iw/silence/agent/after/vad\endcsname{0.3}
\expandafter\def\csname v@vint/iw/silence/agent/kind/babble/after\endcsname{0.18}
\expandafter\def\csname v@vint/iw/silence/agent/kind/talker/after\endcsname{0.85}
\expandafter\def\csname v@vint/iw/silence/agent/missed\endcsname{2.7}
\expandafter\def\csname v@vint/iw/silence/agent/wer\endcsname{15.6}
\expandafter\def\csname v@vint/iw/silence/cpu8/after/down\endcsname{12.5}
\expandafter\def\csname v@vint/iw/silence/cpu8/after/silence\endcsname{74.9}
\expandafter\def\csname v@vint/iw/silence/cpu8/after/vad\endcsname{2.0}
\expandafter\def\csname v@vint/iw/silence/cpu8/kind/babble/after\endcsname{0.94}
\expandafter\def\csname v@vint/iw/silence/cpu8/kind/talker/after\endcsname{3.31}
\expandafter\def\csname v@vint/iw/silence/cpu8/missed\endcsname{0.3}
\expandafter\def\csname v@vint/iw/silence/cpu8/wer\endcsname{11.8}
\expandafter\def\csname v@vint/iw/silence/cpuag8/after/down\endcsname{18.4}
\expandafter\def\csname v@vint/iw/silence/cpuag8/after/silence\endcsname{99.3}
\expandafter\def\csname v@vint/iw/silence/cpuag8/after/vad\endcsname{0.4}
\expandafter\def\csname v@vint/iw/silence/cpuag8/kind/babble/after\endcsname{0.09}
\expandafter\def\csname v@vint/iw/silence/cpuag8/kind/talker/after\endcsname{0.73}
\expandafter\def\csname v@vint/iw/silence/cpuag8/missed\endcsname{2.4}
\expandafter\def\csname v@vint/iw/silence/cpuag8/wer\endcsname{16.2}
\expandafter\def\csname v@vint/iw/silence/inworld/after/down\endcsname{5.8}
\expandafter\def\csname v@vint/iw/silence/inworld/after/silence\endcsname{11.4}
\expandafter\def\csname v@vint/iw/silence/inworld/after/vad\endcsname{15.4}
\expandafter\def\csname v@vint/iw/silence/inworld/kind/babble/after\endcsname{8.02}
\expandafter\def\csname v@vint/iw/silence/inworld/kind/talker/after\endcsname{10.74}
\expandafter\def\csname v@vint/iw/silence/inworld/missed\endcsname{0.0}
\expandafter\def\csname v@vint/iw/silence/inworld/wer\endcsname{8.5}
\expandafter\def\csname v@vint/iw/silence/none/after/down\endcsname{0.0}
\expandafter\def\csname v@vint/iw/silence/none/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/iw/silence/none/after/vad\endcsname{11.8}
\expandafter\def\csname v@vint/iw/silence/none/kind/babble/after\endcsname{3.82}
\expandafter\def\csname v@vint/iw/silence/none/kind/talker/after\endcsname{9.35}
\expandafter\def\csname v@vint/iw/silence/none/missed\endcsname{0.4}
\expandafter\def\csname v@vint/iw/silence/none/wer\endcsname{7.4}
\expandafter\def\csname v@vint/iw/silence/reuse/after/down\endcsname{15.6}
\expandafter\def\csname v@vint/iw/silence/reuse/after/silence\endcsname{98.3}
\expandafter\def\csname v@vint/iw/silence/reuse/after/vad\endcsname{1.1}
\expandafter\def\csname v@vint/iw/silence/reuse/kind/babble/after\endcsname{0.06}
\expandafter\def\csname v@vint/iw/silence/reuse/kind/talker/after\endcsname{1.47}
\expandafter\def\csname v@vint/iw/silence/reuse/missed\endcsname{2.6}
\expandafter\def\csname v@vint/iw/silence/reuse/wer\endcsname{16.9}
\expandafter\def\csname v@vint/none/caught\endcsname{83.7}
\expandafter\def\csname v@vint/none/caught-d\endcsname{-6.2}
\expandafter\def\csname v@vint/none/caught-dabs\endcsname{6.2}
\expandafter\def\csname v@vint/none/caught-dhi\endcsname{-2.6}
\expandafter\def\csname v@vint/none/caught-dlo\endcsname{-10.3}
\expandafter\def\csname v@vint/none/caught-hi\endcsname{87.9}
\expandafter\def\csname v@vint/none/caught-lo\endcsname{79.0}
\expandafter\def\csname v@vint/none/fi\endcsname{2.77}
\expandafter\def\csname v@vint/none/fi-d\endcsname{+1.72}
\expandafter\def\csname v@vint/none/fi-dabs\endcsname{1.72}
\expandafter\def\csname v@vint/none/fi-dhi\endcsname{+2.39}
\expandafter\def\csname v@vint/none/fi-dlo\endcsname{+1.10}
\expandafter\def\csname v@vint/none/fi-hi\endcsname{3.73}
\expandafter\def\csname v@vint/none/fi-lo\endcsname{1.91}
\expandafter\def\csname v@vint/none/fs\endcsname{3.04}
\expandafter\def\csname v@vint/none/fs-d\endcsname{+1.81}
\expandafter\def\csname v@vint/none/fs-dabs\endcsname{1.81}
\expandafter\def\csname v@vint/none/fs-dhi\endcsname{+2.47}
\expandafter\def\csname v@vint/none/fs-dlo\endcsname{+1.19}
\expandafter\def\csname v@vint/none/fs-hi\endcsname{3.95}
\expandafter\def\csname v@vint/none/fs-lo\endcsname{2.14}
\expandafter\def\csname v@vint/none/held\endcsname{9.3}
\expandafter\def\csname v@vint/none/held-d\endcsname{+5.8}
\expandafter\def\csname v@vint/none/held-dabs\endcsname{5.8}
\expandafter\def\csname v@vint/none/held-dhi\endcsname{+9.0}
\expandafter\def\csname v@vint/none/held-dlo\endcsname{+2.9}
\expandafter\def\csname v@vint/none/held-hi\endcsname{13.5}
\expandafter\def\csname v@vint/none/held-lo\endcsname{5.6}
\expandafter\def\csname v@vint/none/kind/babble/fi\endcsname{4.03}
\expandafter\def\csname v@vint/none/kind/babble/fs\endcsname{4.44}
\expandafter\def\csname v@vint/none/kind/babble/missed\endcsname{0.3}
\expandafter\def\csname v@vint/none/kind/clean/fi\endcsname{0.00}
\expandafter\def\csname v@vint/none/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/none/kind/clean/missed\endcsname{0.0}
\expandafter\def\csname v@vint/none/kind/home/fi\endcsname{1.32}
\expandafter\def\csname v@vint/none/kind/home/fs\endcsname{1.45}
\expandafter\def\csname v@vint/none/kind/home/missed\endcsname{0.5}
\expandafter\def\csname v@vint/none/kind/music/fi\endcsname{0.15}
\expandafter\def\csname v@vint/none/kind/music/fs\endcsname{0.23}
\expandafter\def\csname v@vint/none/kind/music/missed\endcsname{1.3}
\expandafter\def\csname v@vint/none/kind/street/fi\endcsname{0.71}
\expandafter\def\csname v@vint/none/kind/street/fs\endcsname{0.79}
\expandafter\def\csname v@vint/none/kind/street/missed\endcsname{0.2}
\expandafter\def\csname v@vint/none/kind/talker/fi\endcsname{10.95}
\expandafter\def\csname v@vint/none/kind/talker/fs\endcsname{8.44}
\expandafter\def\csname v@vint/none/kind/talker/missed\endcsname{0.0}
\expandafter\def\csname v@vint/none/live/barge_p50\endcsname{0.65}
\expandafter\def\csname v@vint/none/live/caught\endcsname{93.3}
\expandafter\def\csname v@vint/none/live/eot_p50\endcsname{0.79}
\expandafter\def\csname v@vint/none/live/eot_p90\endcsname{2.07}
\expandafter\def\csname v@vint/none/live/fi_transcript\endcsname{5.30}
\expandafter\def\csname v@vint/none/live/fi_vad\endcsname{2.61}
\expandafter\def\csname v@vint/none/live/frame-p50\endcsname{0.0}
\expandafter\def\csname v@vint/none/live/frame-p99\endcsname{0.0}
\expandafter\def\csname v@vint/none/live/fs\endcsname{3.97}
\expandafter\def\csname v@vint/none/live/no_reply\endcsname{7.6}
\expandafter\def\csname v@vint/none/live/unfiltered_pct\endcsname{0.00}
\expandafter\def\csname v@vint/none/missed\endcsname{0.4}
\expandafter\def\csname v@vint/none/missed-d\endcsname{-0.2}
\expandafter\def\csname v@vint/none/missed-dabs\endcsname{0.2}
\expandafter\def\csname v@vint/none/missed-dhi\endcsname{+0.4}
\expandafter\def\csname v@vint/none/missed-dlo\endcsname{-0.8}
\expandafter\def\csname v@vint/none/missed-hi\endcsname{0.9}
\expandafter\def\csname v@vint/none/missed-lo\endcsname{0.1}
\expandafter\def\csname v@vint/none/recall\endcsname{94.4}
\expandafter\def\csname v@vint/none/snr/0.0/fi\endcsname{4.03}
\expandafter\def\csname v@vint/none/snr/10.0/fi\endcsname{2.72}
\expandafter\def\csname v@vint/none/snr/20.0/fi\endcsname{2.25}
\expandafter\def\csname v@vint/none/snr/None/fi\endcsname{0.00}
\expandafter\def\csname v@vint/none/wer\endcsname{7.4}
\expandafter\def\csname v@vint/none/wer/babble\endcsname{11.1}
\expandafter\def\csname v@vint/none/wer/clean\endcsname{1.2}
\expandafter\def\csname v@vint/none/wer/home\endcsname{7.5}
\expandafter\def\csname v@vint/none/wer/music\endcsname{4.9}
\expandafter\def\csname v@vint/none/wer/street\endcsname{5.1}
\expandafter\def\csname v@vint/none/wer/talker\endcsname{11.3}
\expandafter\def\csname v@vint/norule/bed-calls\endcsname{765}
\expandafter\def\csname v@vint/norule/calls\endcsname{816}
\expandafter\def\csname v@vint/norule/reuse/after\endcsname{0.24}
\expandafter\def\csname v@vint/norule/reuse/after/silence\endcsname{98.3}
\expandafter\def\csname v@vint/norule/reuse/after/vad\endcsname{1.1}
\expandafter\def\csname v@vint/norule/reuse/all\endcsname{0.95}
\expandafter\def\csname v@vint/norule/reuse/before/silence\endcsname{49.1}
\expandafter\def\csname v@vint/norule/reuse/before/vad\endcsname{17.7}
\expandafter\def\csname v@vint/norule/reuse/greet\endcsname{6.54}
\expandafter\def\csname v@vint/norule/reuse/kind/babble/after\endcsname{0.06}
\expandafter\def\csname v@vint/norule/reuse/kind/babble/after-hi\endcsname{0.14}
\expandafter\def\csname v@vint/norule/reuse/kind/babble/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/babble/after/silence\endcsname{99.9}
\expandafter\def\csname v@vint/norule/reuse/kind/babble/before/silence\endcsname{47.3}
\expandafter\def\csname v@vint/norule/reuse/kind/babble/greet\endcsname{8.45}
\expandafter\def\csname v@vint/norule/reuse/kind/babble/greet-hi\endcsname{11.99}
\expandafter\def\csname v@vint/norule/reuse/kind/babble/greet-lo\endcsname{5.13}
\expandafter\def\csname v@vint/norule/reuse/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/home/after\endcsname{0.04}
\expandafter\def\csname v@vint/norule/reuse/kind/home/after-hi\endcsname{0.10}
\expandafter\def\csname v@vint/norule/reuse/kind/home/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/home/after/silence\endcsname{99.9}
\expandafter\def\csname v@vint/norule/reuse/kind/home/before/silence\endcsname{51.3}
\expandafter\def\csname v@vint/norule/reuse/kind/home/greet\endcsname{4.37}
\expandafter\def\csname v@vint/norule/reuse/kind/home/greet-hi\endcsname{6.67}
\expandafter\def\csname v@vint/norule/reuse/kind/home/greet-lo\endcsname{2.16}
\expandafter\def\csname v@vint/norule/reuse/kind/music/after\endcsname{0.03}
\expandafter\def\csname v@vint/norule/reuse/kind/music/after-hi\endcsname{0.08}
\expandafter\def\csname v@vint/norule/reuse/kind/music/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/music/after/silence\endcsname{100.0}
\expandafter\def\csname v@vint/norule/reuse/kind/music/before/silence\endcsname{72.6}
\expandafter\def\csname v@vint/norule/reuse/kind/music/greet\endcsname{0.80}
\expandafter\def\csname v@vint/norule/reuse/kind/music/greet-hi\endcsname{1.66}
\expandafter\def\csname v@vint/norule/reuse/kind/music/greet-lo\endcsname{0.08}
\expandafter\def\csname v@vint/norule/reuse/kind/street/after\endcsname{0.02}
\expandafter\def\csname v@vint/norule/reuse/kind/street/after-hi\endcsname{0.05}
\expandafter\def\csname v@vint/norule/reuse/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse/kind/street/after/silence\endcsname{100.0}
\expandafter\def\csname v@vint/norule/reuse/kind/street/before/silence\endcsname{59.5}
\expandafter\def\csname v@vint/norule/reuse/kind/street/greet\endcsname{1.30}
\expandafter\def\csname v@vint/norule/reuse/kind/street/greet-hi\endcsname{2.00}
\expandafter\def\csname v@vint/norule/reuse/kind/street/greet-lo\endcsname{0.65}
\expandafter\def\csname v@vint/norule/reuse/kind/talker/after\endcsname{1.47}
\expandafter\def\csname v@vint/norule/reuse/kind/talker/after-hi\endcsname{2.89}
\expandafter\def\csname v@vint/norule/reuse/kind/talker/after-lo\endcsname{0.41}
\expandafter\def\csname v@vint/norule/reuse/kind/talker/after/silence\endcsname{89.0}
\expandafter\def\csname v@vint/norule/reuse/kind/talker/before/silence\endcsname{21.5}
\expandafter\def\csname v@vint/norule/reuse/kind/talker/greet\endcsname{21.70}
\expandafter\def\csname v@vint/norule/reuse/kind/talker/greet-hi\endcsname{23.80}
\expandafter\def\csname v@vint/norule/reuse/kind/talker/greet-lo\endcsname{19.67}
\expandafter\def\csname v@vint/norule/reuse/missed\endcsname{2.6}
\expandafter\def\csname v@vint/norule/reuse/recall\endcsname{87.2}
\expandafter\def\csname v@vint/norule/reuse/trig/down-p50\endcsname{5}
\expandafter\def\csname v@vint/norule/reuse/trig/n\endcsname{111}
\expandafter\def\csname v@vint/norule/reuse/trig/over20\endcsname{5}
\expandafter\def\csname v@vint/norule/reuse/wer\endcsname{16.9}
\expandafter\def\csname v@vint/norule/reuse_norule/after\endcsname{0.23}
\expandafter\def\csname v@vint/norule/reuse_norule/after/silence\endcsname{97.8}
\expandafter\def\csname v@vint/norule/reuse_norule/after/vad\endcsname{1.1}
\expandafter\def\csname v@vint/norule/reuse_norule/all\endcsname{0.92}
\expandafter\def\csname v@vint/norule/reuse_norule/before/silence\endcsname{40.7}
\expandafter\def\csname v@vint/norule/reuse_norule/before/vad\endcsname{18.1}
\expandafter\def\csname v@vint/norule/reuse_norule/greet\endcsname{6.34}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/babble/after\endcsname{0.07}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/babble/after-hi\endcsname{0.16}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/babble/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/babble/after/silence\endcsname{99.9}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/babble/before/silence\endcsname{38.2}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/babble/greet\endcsname{8.10}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/babble/greet-hi\endcsname{11.58}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/babble/greet-lo\endcsname{4.76}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/home/after\endcsname{0.04}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/home/after-hi\endcsname{0.10}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/home/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/home/after/silence\endcsname{99.8}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/home/before/silence\endcsname{43.9}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/home/greet\endcsname{3.76}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/home/greet-hi\endcsname{5.94}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/home/greet-lo\endcsname{1.67}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/music/after\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/music/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/music/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/music/after/silence\endcsname{100.0}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/music/before/silence\endcsname{65.6}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/music/greet\endcsname{0.80}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/music/greet-hi\endcsname{1.61}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/music/greet-lo\endcsname{0.15}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/street/after\endcsname{0.02}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/street/after-hi\endcsname{0.05}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/street/after/silence\endcsname{100.0}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/street/before/silence\endcsname{49.6}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/street/greet\endcsname{1.38}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/street/greet-hi\endcsname{2.06}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/street/greet-lo\endcsname{0.72}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/talker/after\endcsname{1.44}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/talker/after-hi\endcsname{2.78}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/talker/after-lo\endcsname{0.40}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/talker/after/silence\endcsname{86.5}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/talker/before/silence\endcsname{12.7}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/talker/greet\endcsname{21.51}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/talker/greet-hi\endcsname{23.49}
\expandafter\def\csname v@vint/norule/reuse_norule/kind/talker/greet-lo\endcsname{19.35}
\expandafter\def\csname v@vint/norule/reuse_norule/missed\endcsname{2.5}
\expandafter\def\csname v@vint/norule/reuse_norule/recall\endcsname{88.4}
\expandafter\def\csname v@vint/norule/reuse_norule/trig/down-p50\endcsname{5}
\expandafter\def\csname v@vint/norule/reuse_norule/trig/n\endcsname{107}
\expandafter\def\csname v@vint/norule/reuse_norule/trig/over20\endcsname{6}
\expandafter\def\csname v@vint/norule/reuse_norule/wer\endcsname{16.1}
\expandafter\def\csname v@vint/plans\endcsname{48}
\expandafter\def\csname v@vint/probe/lead/cpukd/music0/after-down\endcsname{45}
\expandafter\def\csname v@vint/probe/lead/cpukd/music0/db\endcsname{-29}
\expandafter\def\csname v@vint/probe/lead/cpukd/music0/down\endcsname{29}
\expandafter\def\csname v@vint/probe/lead/cpukd/music0/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/cpukd/music0/speech\endcsname{6}
\expandafter\def\csname v@vint/probe/lead/cpukd/music0/starts\endcsname{6.34}
\expandafter\def\csname v@vint/probe/lead/cpukd/music10/after-down\endcsname{33}
\expandafter\def\csname v@vint/probe/lead/cpukd/music10/db\endcsname{-15}
\expandafter\def\csname v@vint/probe/lead/cpukd/music10/down\endcsname{15}
\expandafter\def\csname v@vint/probe/lead/cpukd/music10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/cpukd/music10/speech\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/cpukd/music10/starts\endcsname{0.92}
\expandafter\def\csname v@vint/probe/lead/cpukd/music20/after-down\endcsname{29}
\expandafter\def\csname v@vint/probe/lead/cpukd/music20/db\endcsname{-7}
\expandafter\def\csname v@vint/probe/lead/cpukd/music20/down\endcsname{7}
\expandafter\def\csname v@vint/probe/lead/cpukd/music20/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/cpukd/music20/speech\endcsname{33}
\expandafter\def\csname v@vint/probe/lead/cpukd/music20/starts\endcsname{2.34}
\expandafter\def\csname v@vint/probe/lead/cpukd/talker10/after-down\endcsname{14}
\expandafter\def\csname v@vint/probe/lead/cpukd/talker10/db\endcsname{-2}
\expandafter\def\csname v@vint/probe/lead/cpukd/talker10/down\endcsname{2}
\expandafter\def\csname v@vint/probe/lead/cpukd/talker10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/cpukd/talker10/speech\endcsname{56}
\expandafter\def\csname v@vint/probe/lead/cpukd/talker10/starts\endcsname{8.39}
\expandafter\def\csname v@vint/probe/lead/none/music0/after-down\endcsname{-0}
\expandafter\def\csname v@vint/probe/lead/none/music0/db\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/none/music0/down\endcsname{-0}
\expandafter\def\csname v@vint/probe/lead/none/music0/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/none/music0/speech\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/none/music0/starts\endcsname{1.06}
\expandafter\def\csname v@vint/probe/lead/none/music10/after-down\endcsname{-0}
\expandafter\def\csname v@vint/probe/lead/none/music10/db\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/none/music10/down\endcsname{-0}
\expandafter\def\csname v@vint/probe/lead/none/music10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/none/music10/speech\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/none/music10/starts\endcsname{1.38}
\expandafter\def\csname v@vint/probe/lead/none/music20/after-down\endcsname{-0}
\expandafter\def\csname v@vint/probe/lead/none/music20/db\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/none/music20/down\endcsname{-0}
\expandafter\def\csname v@vint/probe/lead/none/music20/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/none/music20/speech\endcsname{23}
\expandafter\def\csname v@vint/probe/lead/none/music20/starts\endcsname{3.13}
\expandafter\def\csname v@vint/probe/lead/none/talker10/after-down\endcsname{-0}
\expandafter\def\csname v@vint/probe/lead/none/talker10/db\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/none/talker10/down\endcsname{-0}
\expandafter\def\csname v@vint/probe/lead/none/talker10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/none/talker10/speech\endcsname{72}
\expandafter\def\csname v@vint/probe/lead/none/talker10/starts\endcsname{9.87}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music0/after-down\endcsname{46}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music0/db\endcsname{-25}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music0/down\endcsname{25}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music0/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music0/speech\endcsname{2}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music0/starts\endcsname{3.17}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music10/after-down\endcsname{33}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music10/db\endcsname{-12}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music10/down\endcsname{12}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music10/speech\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music10/starts\endcsname{0.46}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music20/after-down\endcsname{32}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music20/db\endcsname{-6}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music20/down\endcsname{6}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music20/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music20/speech\endcsname{37}
\expandafter\def\csname v@vint/probe/lead/prodcpu/music20/starts\endcsname{2.34}
\expandafter\def\csname v@vint/probe/lead/prodcpu/talker10/after-down\endcsname{12}
\expandafter\def\csname v@vint/probe/lead/prodcpu/talker10/db\endcsname{-2}
\expandafter\def\csname v@vint/probe/lead/prodcpu/talker10/down\endcsname{2}
\expandafter\def\csname v@vint/probe/lead/prodcpu/talker10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/prodcpu/talker10/speech\endcsname{59}
\expandafter\def\csname v@vint/probe/lead/prodcpu/talker10/starts\endcsname{7.40}
\expandafter\def\csname v@vint/probe/lead/release/music0/after-down\endcsname{31}
\expandafter\def\csname v@vint/probe/lead/release/music0/db\endcsname{-26}
\expandafter\def\csname v@vint/probe/lead/release/music0/down\endcsname{26}
\expandafter\def\csname v@vint/probe/lead/release/music0/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/release/music0/speech\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/release/music0/starts\endcsname{1.06}
\expandafter\def\csname v@vint/probe/lead/release/music10/after-down\endcsname{38}
\expandafter\def\csname v@vint/probe/lead/release/music10/db\endcsname{-13}
\expandafter\def\csname v@vint/probe/lead/release/music10/down\endcsname{13}
\expandafter\def\csname v@vint/probe/lead/release/music10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/release/music10/speech\endcsname{3}
\expandafter\def\csname v@vint/probe/lead/release/music10/starts\endcsname{1.38}
\expandafter\def\csname v@vint/probe/lead/release/music20/after-down\endcsname{35}
\expandafter\def\csname v@vint/probe/lead/release/music20/db\endcsname{-6}
\expandafter\def\csname v@vint/probe/lead/release/music20/down\endcsname{6}
\expandafter\def\csname v@vint/probe/lead/release/music20/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/release/music20/speech\endcsname{39}
\expandafter\def\csname v@vint/probe/lead/release/music20/starts\endcsname{1.56}
\expandafter\def\csname v@vint/probe/lead/release/talker10/after-down\endcsname{10}
\expandafter\def\csname v@vint/probe/lead/release/talker10/db\endcsname{-2}
\expandafter\def\csname v@vint/probe/lead/release/talker10/down\endcsname{2}
\expandafter\def\csname v@vint/probe/lead/release/talker10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/release/talker10/speech\endcsname{53}
\expandafter\def\csname v@vint/probe/lead/release/talker10/starts\endcsname{6.91}
\expandafter\def\csname v@vint/probe/lead/reuse/music0/after-down\endcsname{74}
\expandafter\def\csname v@vint/probe/lead/reuse/music0/db\endcsname{-26}
\expandafter\def\csname v@vint/probe/lead/reuse/music0/down\endcsname{26}
\expandafter\def\csname v@vint/probe/lead/reuse/music0/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/reuse/music0/speech\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/reuse/music0/starts\endcsname{1.06}
\expandafter\def\csname v@vint/probe/lead/reuse/music10/after-down\endcsname{50}
\expandafter\def\csname v@vint/probe/lead/reuse/music10/db\endcsname{-33}
\expandafter\def\csname v@vint/probe/lead/reuse/music10/down\endcsname{33}
\expandafter\def\csname v@vint/probe/lead/reuse/music10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/reuse/music10/speech\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/reuse/music10/starts\endcsname{0.00}
\expandafter\def\csname v@vint/probe/lead/reuse/music20/after-down\endcsname{37}
\expandafter\def\csname v@vint/probe/lead/reuse/music20/db\endcsname{-42}
\expandafter\def\csname v@vint/probe/lead/reuse/music20/down\endcsname{42}
\expandafter\def\csname v@vint/probe/lead/reuse/music20/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/reuse/music20/speech\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/reuse/music20/starts\endcsname{0.00}
\expandafter\def\csname v@vint/probe/lead/reuse/talker10/after-down\endcsname{11}
\expandafter\def\csname v@vint/probe/lead/reuse/talker10/db\endcsname{-1}
\expandafter\def\csname v@vint/probe/lead/reuse/talker10/down\endcsname{1}
\expandafter\def\csname v@vint/probe/lead/reuse/talker10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/reuse/talker10/speech\endcsname{70}
\expandafter\def\csname v@vint/probe/lead/reuse/talker10/starts\endcsname{10.36}
\expandafter\def\csname v@vint/probe/lead/vb2/music0/after-down\endcsname{52}
\expandafter\def\csname v@vint/probe/lead/vb2/music0/db\endcsname{-26}
\expandafter\def\csname v@vint/probe/lead/vb2/music0/down\endcsname{26}
\expandafter\def\csname v@vint/probe/lead/vb2/music0/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/vb2/music0/speech\endcsname{0}
\expandafter\def\csname v@vint/probe/lead/vb2/music0/starts\endcsname{1.06}
\expandafter\def\csname v@vint/probe/lead/vb2/music10/after-down\endcsname{40}
\expandafter\def\csname v@vint/probe/lead/vb2/music10/db\endcsname{-16}
\expandafter\def\csname v@vint/probe/lead/vb2/music10/down\endcsname{16}
\expandafter\def\csname v@vint/probe/lead/vb2/music10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/vb2/music10/speech\endcsname{1}
\expandafter\def\csname v@vint/probe/lead/vb2/music10/starts\endcsname{0.46}
\expandafter\def\csname v@vint/probe/lead/vb2/music20/after-down\endcsname{37}
\expandafter\def\csname v@vint/probe/lead/vb2/music20/db\endcsname{-6}
\expandafter\def\csname v@vint/probe/lead/vb2/music20/down\endcsname{6}
\expandafter\def\csname v@vint/probe/lead/vb2/music20/n\endcsname{4}
\expandafter\def\csname v@vint/probe/lead/vb2/music20/speech\endcsname{37}
\expandafter\def\csname v@vint/probe/lead/vb2/music20/starts\endcsname{1.56}
\expandafter\def\csname v@vint/probe/lead/vb2/talker10/after-down\endcsname{16}
\expandafter\def\csname v@vint/probe/lead/vb2/talker10/db\endcsname{-2}
\expandafter\def\csname v@vint/probe/lead/vb2/talker10/down\endcsname{2}
\expandafter\def\csname v@vint/probe/lead/vb2/talker10/n\endcsname{8}
\expandafter\def\csname v@vint/probe/lead/vb2/talker10/speech\endcsname{53}
\expandafter\def\csname v@vint/probe/lead/vb2/talker10/starts\endcsname{6.42}
\expandafter\def\csname v@vint/probe/ret/cpukd/1.5/lost\endcsname{0.6}
\expandafter\def\csname v@vint/probe/ret/cpukd/11/lost\endcsname{2.2}
\expandafter\def\csname v@vint/probe/ret/cpukd/13/lost\endcsname{0.5}
\expandafter\def\csname v@vint/probe/ret/cpukd/15/lost\endcsname{0.2}
\expandafter\def\csname v@vint/probe/ret/cpukd/3/lost\endcsname{0.4}
\expandafter\def\csname v@vint/probe/ret/cpukd/5/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/cpukd/7/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/cpukd/9/lost\endcsname{0.2}
\expandafter\def\csname v@vint/probe/ret/cpukd/long/lost\endcsname{0.6}
\expandafter\def\csname v@vint/probe/ret/none/1.5/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/none/11/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/none/13/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/none/15/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/none/3/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/none/5/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/none/7/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/none/9/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/none/long/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/prodcpu/1.5/lost\endcsname{0.8}
\expandafter\def\csname v@vint/probe/ret/prodcpu/11/lost\endcsname{6.5}
\expandafter\def\csname v@vint/probe/ret/prodcpu/13/lost\endcsname{1.6}
\expandafter\def\csname v@vint/probe/ret/prodcpu/15/lost\endcsname{0.6}
\expandafter\def\csname v@vint/probe/ret/prodcpu/3/lost\endcsname{0.5}
\expandafter\def\csname v@vint/probe/ret/prodcpu/5/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/prodcpu/7/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/prodcpu/9/lost\endcsname{0.8}
\expandafter\def\csname v@vint/probe/ret/prodcpu/long/lost\endcsname{1.9}
\expandafter\def\csname v@vint/probe/ret/release/1.5/lost\endcsname{0.6}
\expandafter\def\csname v@vint/probe/ret/release/11/lost\endcsname{8.0}
\expandafter\def\csname v@vint/probe/ret/release/13/lost\endcsname{0.1}
\expandafter\def\csname v@vint/probe/ret/release/15/lost\endcsname{1.5}
\expandafter\def\csname v@vint/probe/ret/release/3/lost\endcsname{2.1}
\expandafter\def\csname v@vint/probe/ret/release/5/lost\endcsname{0.1}
\expandafter\def\csname v@vint/probe/ret/release/7/lost\endcsname{5.0}
\expandafter\def\csname v@vint/probe/ret/release/9/lost\endcsname{12.3}
\expandafter\def\csname v@vint/probe/ret/release/long/lost\endcsname{5.4}
\expandafter\def\csname v@vint/probe/ret/reuse/1.5/lost\endcsname{1.0}
\expandafter\def\csname v@vint/probe/ret/reuse/11/lost\endcsname{2.5}
\expandafter\def\csname v@vint/probe/ret/reuse/13/lost\endcsname{2.0}
\expandafter\def\csname v@vint/probe/ret/reuse/15/lost\endcsname{4.6}
\expandafter\def\csname v@vint/probe/ret/reuse/3/lost\endcsname{0.8}
\expandafter\def\csname v@vint/probe/ret/reuse/5/lost\endcsname{0.8}
\expandafter\def\csname v@vint/probe/ret/reuse/7/lost\endcsname{1.9}
\expandafter\def\csname v@vint/probe/ret/reuse/9/lost\endcsname{1.2}
\expandafter\def\csname v@vint/probe/ret/reuse/long/lost\endcsname{2.4}
\expandafter\def\csname v@vint/probe/ret/vb2/1.5/lost\endcsname{0.5}
\expandafter\def\csname v@vint/probe/ret/vb2/11/lost\endcsname{7.7}
\expandafter\def\csname v@vint/probe/ret/vb2/13/lost\endcsname{0.1}
\expandafter\def\csname v@vint/probe/ret/vb2/15/lost\endcsname{0.9}
\expandafter\def\csname v@vint/probe/ret/vb2/3/lost\endcsname{1.3}
\expandafter\def\csname v@vint/probe/ret/vb2/5/lost\endcsname{0.0}
\expandafter\def\csname v@vint/probe/ret/vb2/7/lost\endcsname{3.4}
\expandafter\def\csname v@vint/probe/ret/vb2/9/lost\endcsname{7.5}
\expandafter\def\csname v@vint/probe/ret/vb2/long/lost\endcsname{3.9}
\expandafter\def\csname v@vint/r4/check/engine/calls\endcsname{8}
\expandafter\def\csname v@vint/r4/check/engine/differ\endcsname{0}
\expandafter\def\csname v@vint/r4/check/engine/fp16-snr-min\endcsname{55}
\expandafter\def\csname v@vint/r4/check/engine/runs\endcsname{11}
\expandafter\def\csname v@vint/r4/check/engine/seconds\endcsname{60}
\expandafter\def\csname v@vint/r4/check/plugin/calls\endcsname{8}
\expandafter\def\csname v@vint/r4/check/plugin/differ\endcsname{0}
\expandafter\def\csname v@vint/r4/check/plugin/snr-min\endcsname{74}
\expandafter\def\csname v@vint/r4/check/server/calls\endcsname{8}
\expandafter\def\csname v@vint/r4/check/server/default-differ\endcsname{0}
\expandafter\def\csname v@vint/r4/check/server/default-snr-min\endcsname{50}
\expandafter\def\csname v@vint/r4/check/server/voicebot-differ\endcsname{3}
\expandafter\def\csname v@vint/r4/check/server/voicebot-snr-min\endcsname{35}
\expandafter\def\csname v@vint/r4/core/cpu\endcsname{17.0}
\expandafter\def\csname v@vint/r4/core/cpu8\endcsname{12.5}
\expandafter\def\csname v@vint/r4/core/cpuB\endcsname{17.2}
\expandafter\def\csname v@vint/r4/core/cpuB8\endcsname{12.5}
\expandafter\def\csname v@vint/r4/core/cpuBv\endcsname{17.2}
\expandafter\def\csname v@vint/r4/core/cpuBv8\endcsname{12.6}
\expandafter\def\csname v@vint/r4/core/cpuag\endcsname{17.3}
\expandafter\def\csname v@vint/r4/core/cpuag8\endcsname{12.7}
\expandafter\def\csname v@vint/r4/dev/calls\endcsname{608}
\expandafter\def\csname v@vint/r4/dev/cpu/decoy/after\endcsname{0.10}
\expandafter\def\csname v@vint/r4/dev/cpu/decoy/all\endcsname{0.28}
\expandafter\def\csname v@vint/r4/dev/cpu/decoy/cut\endcsname{67.5}
\expandafter\def\csname v@vint/r4/dev/cpu/decoy/greet\endcsname{1.67}
\expandafter\def\csname v@vint/r4/dev/cpu/decoy/missed\endcsname{23.22}
\expandafter\def\csname v@vint/r4/dev/cpu/decoy/recall\endcsname{68.6}
\expandafter\def\csname v@vint/r4/dev/cpu/decoy/talker\endcsname{0.48}
\expandafter\def\csname v@vint/r4/dev/cpu/longer/after\endcsname{0.10}
\expandafter\def\csname v@vint/r4/dev/cpu/longer/all\endcsname{0.52}
\expandafter\def\csname v@vint/r4/dev/cpu/longer/cut\endcsname{90.0}
\expandafter\def\csname v@vint/r4/dev/cpu/longer/greet\endcsname{3.67}
\expandafter\def\csname v@vint/r4/dev/cpu/longer/missed\endcsname{1.48}
\expandafter\def\csname v@vint/r4/dev/cpu/longer/missed-gain\endcsname{1.01}
\expandafter\def\csname v@vint/r4/dev/cpu/longer/recall\endcsname{90.7}
\expandafter\def\csname v@vint/r4/dev/cpu/longer/talker\endcsname{0.43}
\expandafter\def\csname v@vint/r4/dev/cpu/longer/wer\endcsname{18.96}
\expandafter\def\csname v@vint/r4/dev/cpu/none_old_gate/after\endcsname{0.14}
\expandafter\def\csname v@vint/r4/dev/cpu/none_old_gate/all\endcsname{0.54}
\expandafter\def\csname v@vint/r4/dev/cpu/none_old_gate/cut\endcsname{91.0}
\expandafter\def\csname v@vint/r4/dev/cpu/none_old_gate/greet\endcsname{3.49}
\expandafter\def\csname v@vint/r4/dev/cpu/none_old_gate/missed\endcsname{1.12}
\expandafter\def\csname v@vint/r4/dev/cpu/none_old_gate/recall\endcsname{91.5}
\expandafter\def\csname v@vint/r4/dev/cpu/none_old_gate/talker\endcsname{0.63}
\expandafter\def\csname v@vint/r4/dev/cpu/none_old_gate/wer\endcsname{18.07}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle/after\endcsname{0.12}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle/all\endcsname{0.26}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle/cut\endcsname{90.8}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle/greet\endcsname{1.33}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle/missed\endcsname{0.98}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle/recall\endcsname{91.6}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle/talker\endcsname{0.50}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle_old_gate/after\endcsname{0.11}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle_old_gate/all\endcsname{0.25}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle_old_gate/cut\endcsname{90.8}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle_old_gate/greet\endcsname{1.33}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle_old_gate/missed\endcsname{0.98}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle_old_gate/recall\endcsname{91.3}
\expandafter\def\csname v@vint/r4/dev/cpu/oracle_old_gate/talker\endcsname{0.48}
\expandafter\def\csname v@vint/r4/dev/cpu/pick/after\endcsname{0.14}
\expandafter\def\csname v@vint/r4/dev/cpu/pick/all\endcsname{0.53}
\expandafter\def\csname v@vint/r4/dev/cpu/pick/cut\endcsname{91.0}
\expandafter\def\csname v@vint/r4/dev/cpu/pick/greet\endcsname{3.45}
\expandafter\def\csname v@vint/r4/dev/cpu/pick/missed\endcsname{1.06}
\expandafter\def\csname v@vint/r4/dev/cpu/pick/recall\endcsname{91.7}
\expandafter\def\csname v@vint/r4/dev/cpu/pick/talker\endcsname{0.61}
\expandafter\def\csname v@vint/r4/dev/cpu/pick/wer\endcsname{18.04}
\expandafter\def\csname v@vint/r4/dev/cpu/shipped/after\endcsname{0.12}
\expandafter\def\csname v@vint/r4/dev/cpu/shipped/all\endcsname{0.54}
\expandafter\def\csname v@vint/r4/dev/cpu/shipped/cut\endcsname{89.7}
\expandafter\def\csname v@vint/r4/dev/cpu/shipped/greet\endcsname{3.67}
\expandafter\def\csname v@vint/r4/dev/cpu/shipped/missed\endcsname{2.49}
\expandafter\def\csname v@vint/r4/dev/cpu/shipped/recall\endcsname{89.1}
\expandafter\def\csname v@vint/r4/dev/cpu/shipped/talker\endcsname{0.56}
\expandafter\def\csname v@vint/r4/dev/cpu/shipped/wer\endcsname{20.90}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_longer/after\endcsname{0.11}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_longer/all\endcsname{0.32}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_longer/cut\endcsname{90.3}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_longer/greet\endcsname{1.89}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_longer/missed\endcsname{1.36}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_longer/recall\endcsname{90.3}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_longer/talker\endcsname{0.48}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_longer/wer\endcsname{19.00}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_none/after\endcsname{0.14}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_none/all\endcsname{0.27}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_none/cut\endcsname{91.1}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_none/greet\endcsname{1.22}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_none/missed\endcsname{0.98}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_none/recall\endcsname{91.2}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_none/talker\endcsname{0.61}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_none/wer\endcsname{18.40}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_pick/after\endcsname{0.12}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_pick/all\endcsname{0.26}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_pick/cut\endcsname{90.3}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_pick/greet\endcsname{1.26}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_pick/missed\endcsname{1.36}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_pick/recall\endcsname{90.6}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_pick/talker\endcsname{0.53}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_pick/wer\endcsname{18.76}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_shipped/after\endcsname{0.13}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_shipped/all\endcsname{0.34}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_shipped/cut\endcsname{89.8}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_shipped/greet\endcsname{1.89}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_shipped/missed\endcsname{2.36}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_shipped/recall\endcsname{88.8}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_shipped/talker\endcsname{0.61}
\expandafter\def\csname v@vint/r4/dev/cpu/vb_shipped/wer\endcsname{20.80}
\expandafter\def\csname v@vint/r4/dev/gpu/decoy/after\endcsname{0.10}
\expandafter\def\csname v@vint/r4/dev/gpu/decoy/all\endcsname{0.33}
\expandafter\def\csname v@vint/r4/dev/gpu/decoy/cut\endcsname{83.5}
\expandafter\def\csname v@vint/r4/dev/gpu/decoy/greet\endcsname{2.01}
\expandafter\def\csname v@vint/r4/dev/gpu/decoy/missed\endcsname{6.46}
\expandafter\def\csname v@vint/r4/dev/gpu/decoy/recall\endcsname{84.9}
\expandafter\def\csname v@vint/r4/dev/gpu/decoy/talker\endcsname{0.73}
\expandafter\def\csname v@vint/r4/dev/gpu/longer/after\endcsname{0.15}
\expandafter\def\csname v@vint/r4/dev/gpu/longer/all\endcsname{0.55}
\expandafter\def\csname v@vint/r4/dev/gpu/longer/cut\endcsname{89.6}
\expandafter\def\csname v@vint/r4/dev/gpu/longer/greet\endcsname{3.58}
\expandafter\def\csname v@vint/r4/dev/gpu/longer/missed\endcsname{1.75}
\expandafter\def\csname v@vint/r4/dev/gpu/longer/missed-gain\endcsname{0.24}
\expandafter\def\csname v@vint/r4/dev/gpu/longer/recall\endcsname{90.5}
\expandafter\def\csname v@vint/r4/dev/gpu/longer/talker\endcsname{1.09}
\expandafter\def\csname v@vint/r4/dev/gpu/longer/wer\endcsname{17.81}
\expandafter\def\csname v@vint/r4/dev/gpu/none/after\endcsname{0.19}
\expandafter\def\csname v@vint/r4/dev/gpu/none/all\endcsname{0.57}
\expandafter\def\csname v@vint/r4/dev/gpu/none/cut\endcsname{89.4}
\expandafter\def\csname v@vint/r4/dev/gpu/none/greet\endcsname{3.45}
\expandafter\def\csname v@vint/r4/dev/gpu/none/missed\endcsname{2.16}
\expandafter\def\csname v@vint/r4/dev/gpu/none/recall\endcsname{89.7}
\expandafter\def\csname v@vint/r4/dev/gpu/none/talker\endcsname{1.31}
\expandafter\def\csname v@vint/r4/dev/gpu/pick/after\endcsname{0.15}
\expandafter\def\csname v@vint/r4/dev/gpu/pick/all\endcsname{0.55}
\expandafter\def\csname v@vint/r4/dev/gpu/pick/cut\endcsname{89.6}
\expandafter\def\csname v@vint/r4/dev/gpu/pick/greet\endcsname{3.58}
\expandafter\def\csname v@vint/r4/dev/gpu/pick/missed\endcsname{1.99}
\expandafter\def\csname v@vint/r4/dev/gpu/pick/recall\endcsname{89.7}
\expandafter\def\csname v@vint/r4/dev/gpu/pick/talker\endcsname{1.06}
\expandafter\def\csname v@vint/r4/dev/gpu/pick/wer\endcsname{18.73}
\expandafter\def\csname v@vint/r4/dev/gpu/shipped/after\endcsname{0.15}
\expandafter\def\csname v@vint/r4/dev/gpu/shipped/all\endcsname{0.55}
\expandafter\def\csname v@vint/r4/dev/gpu/shipped/cut\endcsname{89.6}
\expandafter\def\csname v@vint/r4/dev/gpu/shipped/greet\endcsname{3.58}
\expandafter\def\csname v@vint/r4/dev/gpu/shipped/missed\endcsname{1.99}
\expandafter\def\csname v@vint/r4/dev/gpu/shipped/recall\endcsname{89.7}
\expandafter\def\csname v@vint/r4/dev/gpu/shipped/talker\endcsname{1.06}
\expandafter\def\csname v@vint/r4/dev/gpu/shipped/wer\endcsname{18.73}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_longer/after\endcsname{0.15}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_longer/all\endcsname{0.39}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_longer/cut\endcsname{89.8}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_longer/greet\endcsname{2.21}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_longer/missed\endcsname{1.70}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_longer/recall\endcsname{90.5}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_longer/talker\endcsname{1.09}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_longer/wer\endcsname{17.80}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_never/after\endcsname{0.15}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_never/all\endcsname{0.24}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_never/cut\endcsname{89.8}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_never/greet\endcsname{0.92}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_never/missed\endcsname{1.70}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_never/recall\endcsname{90.5}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_never/talker\endcsname{1.09}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_pick/after\endcsname{0.15}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_pick/all\endcsname{0.32}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_pick/cut\endcsname{89.8}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_pick/greet\endcsname{1.62}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_pick/missed\endcsname{1.70}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_pick/recall\endcsname{90.5}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_pick/talker\endcsname{1.09}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_pick/wer\endcsname{17.83}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_shipped/after\endcsname{0.15}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_shipped/all\endcsname{0.39}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_shipped/cut\endcsname{89.8}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_shipped/greet\endcsname{2.21}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_shipped/missed\endcsname{1.88}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_shipped/recall\endcsname{89.8}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_shipped/talker\endcsname{1.03}
\expandafter\def\csname v@vint/r4/dev/gpu/vb_shipped/wer\endcsname{18.70}
\expandafter\def\csname v@vint/r4/dev/none/after\endcsname{2.02}
\expandafter\def\csname v@vint/r4/dev/none/all\endcsname{2.38}
\expandafter\def\csname v@vint/r4/dev/none/cut\endcsname{88.1}
\expandafter\def\csname v@vint/r4/dev/none/greet\endcsname{5.10}
\expandafter\def\csname v@vint/r4/dev/none/missed\endcsname{0.30}
\expandafter\def\csname v@vint/r4/dev/none/recall\endcsname{94.5}
\expandafter\def\csname v@vint/r4/dev/none/talker\endcsname{9.94}
\expandafter\def\csname v@vint/r4/dev/reuse/after\endcsname{0.19}
\expandafter\def\csname v@vint/r4/dev/reuse/all\endcsname{0.89}
\expandafter\def\csname v@vint/r4/dev/reuse/cut\endcsname{89.2}
\expandafter\def\csname v@vint/r4/dev/reuse/greet\endcsname{6.04}
\expandafter\def\csname v@vint/r4/dev/reuse/missed\endcsname{3.19}
\expandafter\def\csname v@vint/r4/dev/reuse/recall\endcsname{87.6}
\expandafter\def\csname v@vint/r4/dev/reuse/talker\endcsname{1.39}
\expandafter\def\csname v@vint/r4/dev/reuse/wer\endcsname{20.52}
\expandafter\def\csname v@vint/r4/dev/sessions\endcsname{13}
\expandafter\def\csname v@vint/r4/pick/cpu/hold-s\endcsname{0.5}
\expandafter\def\csname v@vint/r4/pick/cpu/theta\endcsname{0.9}
\expandafter\def\csname v@vint/r4/pick/cpu/theta-off\endcsname{0.3}
\expandafter\def\csname v@vint/r4/pick/cpu/wait-keep\endcsname{1}
\expandafter\def\csname v@vint/r4/pick/gpu/hold-s\endcsname{1}
\expandafter\def\csname v@vint/r4/pick/gpu/theta\endcsname{0.9}
\expandafter\def\csname v@vint/r4/pick/gpu/theta-off\endcsname{0.2}
\expandafter\def\csname v@vint/r4/pick/gpu/wait-keep\endcsname{1}
\expandafter\def\csname v@vint/r4/probe/beds-n\endcsname{16}
\expandafter\def\csname v@vint/r4/probe/clean-n\endcsname{8}
\expandafter\def\csname v@vint/r4/probe/cpu/default/beds-all\endcsname{2.3}
\expandafter\def\csname v@vint/r4/probe/cpu/default/beds-first\endcsname{2.0}
\expandafter\def\csname v@vint/r4/probe/cpu/default/beds-runs\endcsname{0}
\expandafter\def\csname v@vint/r4/probe/cpu/default/clean-all\endcsname{3.9}
\expandafter\def\csname v@vint/r4/probe/cpu/default/clean-first\endcsname{0.5}
\expandafter\def\csname v@vint/r4/probe/cpu/default/clean-runs\endcsname{0}
\expandafter\def\csname v@vint/r4/probe/cpu/pick_default/beds-all\endcsname{2.0}
\expandafter\def\csname v@vint/r4/probe/cpu/pick_default/beds-first\endcsname{1.9}
\expandafter\def\csname v@vint/r4/probe/cpu/pick_default/beds-runs\endcsname{0}
\expandafter\def\csname v@vint/r4/probe/cpu/pick_default/clean-all\endcsname{1.2}
\expandafter\def\csname v@vint/r4/probe/cpu/pick_default/clean-first\endcsname{0.5}
\expandafter\def\csname v@vint/r4/probe/cpu/pick_default/clean-runs\endcsname{0}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot/beds-all\endcsname{16.0}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot/beds-first\endcsname{32.7}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot/beds-runs\endcsname{5}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot/clean-all\endcsname{12.8}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot/clean-first\endcsname{25.6}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot/clean-runs\endcsname{2}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot_before/beds-all\endcsname{16.0}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot_before/beds-first\endcsname{32.6}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot_before/beds-runs\endcsname{5}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot_before/clean-all\endcsname{14.1}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot_before/clean-first\endcsname{25.4}
\expandafter\def\csname v@vint/r4/probe/cpu/voicebot_before/clean-runs\endcsname{2}
\expandafter\def\csname v@vint/r4/probe/gpu/default/beds-all\endcsname{5.9}
\expandafter\def\csname v@vint/r4/probe/gpu/default/beds-first\endcsname{1.8}
\expandafter\def\csname v@vint/r4/probe/gpu/default/beds-runs\endcsname{0}
\expandafter\def\csname v@vint/r4/probe/gpu/default/clean-all\endcsname{2.0}
\expandafter\def\csname v@vint/r4/probe/gpu/default/clean-first\endcsname{0.3}
\expandafter\def\csname v@vint/r4/probe/gpu/default/clean-runs\endcsname{0}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot/beds-all\endcsname{9.3}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot/beds-first\endcsname{16.3}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot/beds-runs\endcsname{2}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot/clean-all\endcsname{8.1}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot/clean-first\endcsname{25.2}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot/clean-runs\endcsname{2}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot_before/beds-all\endcsname{9.1}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot_before/beds-first\endcsname{15.7}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot_before/beds-runs\endcsname{2}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot_before/clean-all\endcsname{8.1}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot_before/clean-first\endcsname{24.9}
\expandafter\def\csname v@vint/r4/probe/gpu/voicebot_before/clean-runs\endcsname{2}
\expandafter\def\csname v@vint/r4/replace-all\endcsname{0.05}
\expandafter\def\csname v@vint/r4/replace-missed\endcsname{0.3}
\expandafter\def\csname v@vint/r4/serve/cpu/hold-s\endcsname{0.3}
\expandafter\def\csname v@vint/r4/serve/cpu/theta\endcsname{0.9}
\expandafter\def\csname v@vint/r4/serve/cpu/theta-off\endcsname{0.2}
\expandafter\def\csname v@vint/r4/serve/cpu/vb/arrive-db\endcsname{6}
\expandafter\def\csname v@vint/r4/serve/cpu/vb/arrive-hold\endcsname{15}
\expandafter\def\csname v@vint/r4/serve/cpu/vb/hold-s\endcsname{0.5}
\expandafter\def\csname v@vint/r4/serve/cpu/vb/loud-within\endcsname{60}
\expandafter\def\csname v@vint/r4/serve/cpu/vb/theta\endcsname{0.9}
\expandafter\def\csname v@vint/r4/serve/cpu/vb/theta-off\endcsname{0.3}
\expandafter\def\csname v@vint/r4/serve/cpu/vb/wait-keep\endcsname{0}
\expandafter\def\csname v@vint/r4/serve/cpu/wait-keep\endcsname{1}
\expandafter\def\csname v@vint/r4/serve/gpu/hold-s\endcsname{1}
\expandafter\def\csname v@vint/r4/serve/gpu/theta\endcsname{0.9}
\expandafter\def\csname v@vint/r4/serve/gpu/theta-off\endcsname{0.2}
\expandafter\def\csname v@vint/r4/serve/gpu/vb/arrive-db\endcsname{6}
\expandafter\def\csname v@vint/r4/serve/gpu/vb/arrive-hold\endcsname{15}
\expandafter\def\csname v@vint/r4/serve/gpu/vb/hold-s\endcsname{1}
\expandafter\def\csname v@vint/r4/serve/gpu/vb/loud-within\endcsname{60}
\expandafter\def\csname v@vint/r4/serve/gpu/vb/theta\endcsname{0.9}
\expandafter\def\csname v@vint/r4/serve/gpu/vb/theta-off\endcsname{0.2}
\expandafter\def\csname v@vint/r4/serve/gpu/vb/wait-keep\endcsname{3}
\expandafter\def\csname v@vint/r4/serve/gpu/wait-keep\endcsname{1}
\expandafter\def\csname v@vint/r4/test/agent/after\endcsname{0.20}
\expandafter\def\csname v@vint/r4/test/agent/after-hi\endcsname{0.35}
\expandafter\def\csname v@vint/r4/test/agent/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/r4/test/agent/all\endcsname{0.54}
\expandafter\def\csname v@vint/r4/test/agent/all-hi\endcsname{0.79}
\expandafter\def\csname v@vint/r4/test/agent/all-lo\endcsname{0.33}
\expandafter\def\csname v@vint/r4/test/agent/cut\endcsname{84.8}
\expandafter\def\csname v@vint/r4/test/agent/greet\endcsname{3.22}
\expandafter\def\csname v@vint/r4/test/agent/greet-hi\endcsname{4.58}
\expandafter\def\csname v@vint/r4/test/agent/greet-lo\endcsname{1.98}
\expandafter\def\csname v@vint/r4/test/agent/missed\endcsname{2.7}
\expandafter\def\csname v@vint/r4/test/agent/recall\endcsname{88.4}
\expandafter\def\csname v@vint/r4/test/agent/silence-after\endcsname{98.6}
\expandafter\def\csname v@vint/r4/test/agent/talker\endcsname{0.85}
\expandafter\def\csname v@vint/r4/test/agent/wer\endcsname{15.6}
\expandafter\def\csname v@vint/r4/test/calls\endcsname{816}
\expandafter\def\csname v@vint/r4/test/cpu8/after\endcsname{0.80}
\expandafter\def\csname v@vint/r4/test/cpu8/after-hi\endcsname{1.24}
\expandafter\def\csname v@vint/r4/test/cpu8/after-lo\endcsname{0.44}
\expandafter\def\csname v@vint/r4/test/cpu8/all\endcsname{1.36}
\expandafter\def\csname v@vint/r4/test/cpu8/all-hi\endcsname{1.88}
\expandafter\def\csname v@vint/r4/test/cpu8/all-lo\endcsname{0.93}
\expandafter\def\csname v@vint/r4/test/cpu8/cut\endcsname{91.0}
\expandafter\def\csname v@vint/r4/test/cpu8/greet\endcsname{5.77}
\expandafter\def\csname v@vint/r4/test/cpu8/greet-hi\endcsname{7.41}
\expandafter\def\csname v@vint/r4/test/cpu8/greet-lo\endcsname{4.21}
\expandafter\def\csname v@vint/r4/test/cpu8/missed\endcsname{0.3}
\expandafter\def\csname v@vint/r4/test/cpu8/recall\endcsname{93.4}
\expandafter\def\csname v@vint/r4/test/cpu8/silence-after\endcsname{74.9}
\expandafter\def\csname v@vint/r4/test/cpu8/talker\endcsname{3.31}
\expandafter\def\csname v@vint/r4/test/cpu8/wer\endcsname{11.8}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/after\endcsname{0.82}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/after-hi\endcsname{1.25}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/after-lo\endcsname{0.45}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/all\endcsname{1.13}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/all-hi\endcsname{1.59}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/all-lo\endcsname{0.75}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/cut\endcsname{91.1}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/greet\endcsname{3.61}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/greet-hi\endcsname{4.66}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/greet-lo\endcsname{2.64}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/missed\endcsname{0.3}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/recall\endcsname{93.5}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/silence-after\endcsname{74.8}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/talker\endcsname{3.37}
\expandafter\def\csname v@vint/r4/test/cpu8_vb/wer\endcsname{11.7}
\expandafter\def\csname v@vint/r4/test/cpuB/after\endcsname{0.20}
\expandafter\def\csname v@vint/r4/test/cpuB/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/r4/test/cpuB/after-lo\endcsname{0.10}
\expandafter\def\csname v@vint/r4/test/cpuB/all\endcsname{0.53}
\expandafter\def\csname v@vint/r4/test/cpuB/all-hi\endcsname{0.77}
\expandafter\def\csname v@vint/r4/test/cpuB/all-lo\endcsname{0.32}
\expandafter\def\csname v@vint/r4/test/cpuB/cut\endcsname{88.8}
\expandafter\def\csname v@vint/r4/test/cpuB/greet\endcsname{3.10}
\expandafter\def\csname v@vint/r4/test/cpuB/greet-hi\endcsname{4.44}
\expandafter\def\csname v@vint/r4/test/cpuB/greet-lo\endcsname{1.88}
\expandafter\def\csname v@vint/r4/test/cpuB/missed\endcsname{1.3}
\expandafter\def\csname v@vint/r4/test/cpuB/recall\endcsname{90.9}
\expandafter\def\csname v@vint/r4/test/cpuB/silence-after\endcsname{99.0}
\expandafter\def\csname v@vint/r4/test/cpuB/talker\endcsname{0.89}
\expandafter\def\csname v@vint/r4/test/cpuB/wer\endcsname{14.7}
\expandafter\def\csname v@vint/r4/test/cpuB8/after\endcsname{0.20}
\expandafter\def\csname v@vint/r4/test/cpuB8/after-hi\endcsname{0.34}
\expandafter\def\csname v@vint/r4/test/cpuB8/after-lo\endcsname{0.10}
\expandafter\def\csname v@vint/r4/test/cpuB8/all\endcsname{0.53}
\expandafter\def\csname v@vint/r4/test/cpuB8/all-hi\endcsname{0.78}
\expandafter\def\csname v@vint/r4/test/cpuB8/all-lo\endcsname{0.33}
\expandafter\def\csname v@vint/r4/test/cpuB8/cut\endcsname{88.7}
\expandafter\def\csname v@vint/r4/test/cpuB8/greet\endcsname{3.14}
\expandafter\def\csname v@vint/r4/test/cpuB8/greet-hi\endcsname{4.49}
\expandafter\def\csname v@vint/r4/test/cpuB8/greet-lo\endcsname{1.91}
\expandafter\def\csname v@vint/r4/test/cpuB8/missed\endcsname{1.4}
\expandafter\def\csname v@vint/r4/test/cpuB8/recall\endcsname{90.8}
\expandafter\def\csname v@vint/r4/test/cpuB8/silence-after\endcsname{99.0}
\expandafter\def\csname v@vint/r4/test/cpuB8/talker\endcsname{0.89}
\expandafter\def\csname v@vint/r4/test/cpuB8/wer\endcsname{14.8}
\expandafter\def\csname v@vint/r4/test/cpuBv/after\endcsname{0.17}
\expandafter\def\csname v@vint/r4/test/cpuBv/after-hi\endcsname{0.32}
\expandafter\def\csname v@vint/r4/test/cpuBv/after-lo\endcsname{0.06}
\expandafter\def\csname v@vint/r4/test/cpuBv/all\endcsname{0.26}
\expandafter\def\csname v@vint/r4/test/cpuBv/all-hi\endcsname{0.44}
\expandafter\def\csname v@vint/r4/test/cpuBv/all-lo\endcsname{0.13}
\expandafter\def\csname v@vint/r4/test/cpuBv/cut\endcsname{88.4}
\expandafter\def\csname v@vint/r4/test/cpuBv/greet\endcsname{0.97}
\expandafter\def\csname v@vint/r4/test/cpuBv/greet-hi\endcsname{1.47}
\expandafter\def\csname v@vint/r4/test/cpuBv/greet-lo\endcsname{0.55}
\expandafter\def\csname v@vint/r4/test/cpuBv/missed\endcsname{1.6}
\expandafter\def\csname v@vint/r4/test/cpuBv/recall\endcsname{89.6}
\expandafter\def\csname v@vint/r4/test/cpuBv/silence-after\endcsname{99.2}
\expandafter\def\csname v@vint/r4/test/cpuBv/talker\endcsname{0.82}
\expandafter\def\csname v@vint/r4/test/cpuBv/wer\endcsname{16.8}
\expandafter\def\csname v@vint/r4/test/cpuBv8/after\endcsname{0.16}
\expandafter\def\csname v@vint/r4/test/cpuBv8/after-hi\endcsname{0.30}
\expandafter\def\csname v@vint/r4/test/cpuBv8/after-lo\endcsname{0.07}
\expandafter\def\csname v@vint/r4/test/cpuBv8/all\endcsname{0.26}
\expandafter\def\csname v@vint/r4/test/cpuBv8/all-hi\endcsname{0.42}
\expandafter\def\csname v@vint/r4/test/cpuBv8/all-lo\endcsname{0.13}
\expandafter\def\csname v@vint/r4/test/cpuBv8/cut\endcsname{88.3}
\expandafter\def\csname v@vint/r4/test/cpuBv8/greet\endcsname{0.97}
\expandafter\def\csname v@vint/r4/test/cpuBv8/greet-hi\endcsname{1.47}
\expandafter\def\csname v@vint/r4/test/cpuBv8/greet-lo\endcsname{0.55}
\expandafter\def\csname v@vint/r4/test/cpuBv8/missed\endcsname{1.7}
\expandafter\def\csname v@vint/r4/test/cpuBv8/recall\endcsname{89.5}
\expandafter\def\csname v@vint/r4/test/cpuBv8/silence-after\endcsname{99.2}
\expandafter\def\csname v@vint/r4/test/cpuBv8/talker\endcsname{0.79}
\expandafter\def\csname v@vint/r4/test/cpuBv8/wer\endcsname{16.8}
\expandafter\def\csname v@vint/r4/test/cpuag/after\endcsname{0.14}
\expandafter\def\csname v@vint/r4/test/cpuag/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/r4/test/cpuag/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/r4/test/cpuag/all\endcsname{0.48}
\expandafter\def\csname v@vint/r4/test/cpuag/all-hi\endcsname{0.71}
\expandafter\def\csname v@vint/r4/test/cpuag/all-lo\endcsname{0.29}
\expandafter\def\csname v@vint/r4/test/cpuag/cut\endcsname{87.9}
\expandafter\def\csname v@vint/r4/test/cpuag/greet\endcsname{3.14}
\expandafter\def\csname v@vint/r4/test/cpuag/greet-hi\endcsname{4.45}
\expandafter\def\csname v@vint/r4/test/cpuag/greet-lo\endcsname{1.94}
\expandafter\def\csname v@vint/r4/test/cpuag/missed\endcsname{2.4}
\expandafter\def\csname v@vint/r4/test/cpuag/recall\endcsname{88.7}
\expandafter\def\csname v@vint/r4/test/cpuag/silence-after\endcsname{99.3}
\expandafter\def\csname v@vint/r4/test/cpuag/talker\endcsname{0.73}
\expandafter\def\csname v@vint/r4/test/cpuag/wer\endcsname{16.0}
\expandafter\def\csname v@vint/r4/test/cpuag8/after\endcsname{0.14}
\expandafter\def\csname v@vint/r4/test/cpuag8/after-hi\endcsname{0.27}
\expandafter\def\csname v@vint/r4/test/cpuag8/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/r4/test/cpuag8/all\endcsname{0.48}
\expandafter\def\csname v@vint/r4/test/cpuag8/all-hi\endcsname{0.71}
\expandafter\def\csname v@vint/r4/test/cpuag8/all-lo\endcsname{0.29}
\expandafter\def\csname v@vint/r4/test/cpuag8/cut\endcsname{87.9}
\expandafter\def\csname v@vint/r4/test/cpuag8/greet\endcsname{3.14}
\expandafter\def\csname v@vint/r4/test/cpuag8/greet-hi\endcsname{4.45}
\expandafter\def\csname v@vint/r4/test/cpuag8/greet-lo\endcsname{1.94}
\expandafter\def\csname v@vint/r4/test/cpuag8/missed\endcsname{2.4}
\expandafter\def\csname v@vint/r4/test/cpuag8/recall\endcsname{88.7}
\expandafter\def\csname v@vint/r4/test/cpuag8/silence-after\endcsname{99.3}
\expandafter\def\csname v@vint/r4/test/cpuag8/talker\endcsname{0.73}
\expandafter\def\csname v@vint/r4/test/cpuag8/wer\endcsname{16.2}
\expandafter\def\csname v@vint/r4/test/diff/cpuB-cpuB8/after\endcsname{-0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuB-cpuB8/after-hi\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuB-cpuB8/after-lo\endcsname{-0.01}
\expandafter\def\csname v@vint/r4/test/diff/cpuB-cpuB8/all\endcsname{-0.01}
\expandafter\def\csname v@vint/r4/test/diff/cpuB-cpuB8/all-hi\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuB-cpuB8/all-lo\endcsname{-0.02}
\expandafter\def\csname v@vint/r4/test/diff/cpuB-cpuB8/greet\endcsname{-0.03}
\expandafter\def\csname v@vint/r4/test/diff/cpuB-cpuB8/greet-hi\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuB-cpuB8/greet-lo\endcsname{-0.07}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-cpuag8/after\endcsname{+0.06}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-cpuag8/after-hi\endcsname{+0.10}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-cpuag8/after-lo\endcsname{+0.03}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-cpuag8/all\endcsname{+0.06}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-cpuag8/all-hi\endcsname{+0.10}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-cpuag8/all-lo\endcsname{+0.02}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-cpuag8/greet\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-cpuag8/greet-hi\endcsname{+0.15}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-cpuag8/greet-lo\endcsname{-0.15}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-reuse/after\endcsname{-0.03}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-reuse/after-hi\endcsname{+0.07}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-reuse/after-lo\endcsname{-0.14}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-reuse/all\endcsname{-0.41}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-reuse/all-hi\endcsname{-0.26}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-reuse/all-lo\endcsname{-0.59}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-reuse/greet\endcsname{-3.41}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-reuse/greet-hi\endcsname{-2.36}
\expandafter\def\csname v@vint/r4/test/diff/cpuB8-reuse/greet-lo\endcsname{-4.52}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv-cpuBv8/after\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv-cpuBv8/after-hi\endcsname{+0.02}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv-cpuBv8/after-lo\endcsname{-0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv-cpuBv8/all\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv-cpuBv8/all-hi\endcsname{+0.02}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv-cpuBv8/all-lo\endcsname{-0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv-cpuBv8/greet\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv-cpuBv8/greet-hi\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv-cpuBv8/greet-lo\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpu8_vb/after\endcsname{-0.65}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpu8_vb/after-hi\endcsname{-0.37}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpu8_vb/after-lo\endcsname{-0.99}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpu8_vb/all\endcsname{-0.88}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpu8_vb/all-hi\endcsname{-0.59}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpu8_vb/all-lo\endcsname{-1.22}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpu8_vb/greet\endcsname{-2.63}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpu8_vb/greet-hi\endcsname{-1.98}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpu8_vb/greet-lo\endcsname{-3.33}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuB8/after\endcsname{-0.04}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuB8/after-hi\endcsname{-0.01}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuB8/after-lo\endcsname{-0.07}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuB8/all\endcsname{-0.28}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuB8/all-hi\endcsname{-0.17}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuB8/all-lo\endcsname{-0.41}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuB8/greet\endcsname{-2.16}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuB8/greet-hi\endcsname{-1.26}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuB8/greet-lo\endcsname{-3.17}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuag8/after\endcsname{+0.02}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuag8/after-hi\endcsname{+0.05}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuag8/after-lo\endcsname{+0.00}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuag8/all\endcsname{-0.22}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuag8/all-hi\endcsname{-0.12}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuag8/all-lo\endcsname{-0.34}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuag8/greet\endcsname{-2.16}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuag8/greet-hi\endcsname{-1.29}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-cpuag8/greet-lo\endcsname{-3.13}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-gpuv/after\endcsname{-0.02}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-gpuv/after-hi\endcsname{+0.02}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-gpuv/after-lo\endcsname{-0.06}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-gpuv/all\endcsname{-0.07}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-gpuv/all-hi\endcsname{-0.03}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-gpuv/all-lo\endcsname{-0.11}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-gpuv/greet\endcsname{-0.44}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-gpuv/greet-hi\endcsname{-0.22}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-gpuv/greet-lo\endcsname{-0.68}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-rel_vb/after\endcsname{-0.33}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-rel_vb/after-hi\endcsname{-0.16}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-rel_vb/after-lo\endcsname{-0.54}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-rel_vb/all\endcsname{-0.53}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-rel_vb/all-hi\endcsname{-0.35}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-rel_vb/all-lo\endcsname{-0.74}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-rel_vb/greet\endcsname{-2.05}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-rel_vb/greet-hi\endcsname{-1.47}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-rel_vb/greet-lo\endcsname{-2.66}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-reuse/after\endcsname{-0.07}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-reuse/after-hi\endcsname{+0.03}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-reuse/after-lo\endcsname{-0.19}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-reuse/all\endcsname{-0.69}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-reuse/all-hi\endcsname{-0.47}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-reuse/all-lo\endcsname{-0.95}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-reuse/greet\endcsname{-5.57}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-reuse/greet-hi\endcsname{-3.97}
\expandafter\def\csname v@vint/r4/test/diff/cpuBv8-reuse/greet-lo\endcsname{-7.24}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-agent/after\endcsname{-0.01}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-agent/after-hi\endcsname{+0.01}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-agent/after-lo\endcsname{-0.04}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-agent/all\endcsname{-0.22}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-agent/all-hi\endcsname{-0.12}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-agent/all-lo\endcsname{-0.33}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-agent/greet\endcsname{-1.81}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-agent/greet-hi\endcsname{-1.03}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-agent/greet-lo\endcsname{-2.71}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-rel_vb/after\endcsname{-0.31}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-rel_vb/after-hi\endcsname{-0.14}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-rel_vb/after-lo\endcsname{-0.53}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-rel_vb/all\endcsname{-0.46}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-rel_vb/all-hi\endcsname{-0.28}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-rel_vb/all-lo\endcsname{-0.67}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-rel_vb/greet\endcsname{-1.61}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-rel_vb/greet-hi\endcsname{-1.11}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-rel_vb/greet-lo\endcsname{-2.13}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-reuse/after\endcsname{-0.05}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-reuse/after-hi\endcsname{+0.05}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-reuse/after-lo\endcsname{-0.17}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-reuse/all\endcsname{-0.62}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-reuse/all-hi\endcsname{-0.41}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-reuse/all-lo\endcsname{-0.86}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-reuse/greet\endcsname{-5.13}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-reuse/greet-hi\endcsname{-3.63}
\expandafter\def\csname v@vint/r4/test/diff/gpuv-reuse/greet-lo\endcsname{-6.73}
\expandafter\def\csname v@vint/r4/test/gpuv/after\endcsname{0.19}
\expandafter\def\csname v@vint/r4/test/gpuv/after-hi\endcsname{0.33}
\expandafter\def\csname v@vint/r4/test/gpuv/after-lo\endcsname{0.09}
\expandafter\def\csname v@vint/r4/test/gpuv/all\endcsname{0.32}
\expandafter\def\csname v@vint/r4/test/gpuv/all-hi\endcsname{0.50}
\expandafter\def\csname v@vint/r4/test/gpuv/all-lo\endcsname{0.19}
\expandafter\def\csname v@vint/r4/test/gpuv/cut\endcsname{85.5}
\expandafter\def\csname v@vint/r4/test/gpuv/greet\endcsname{1.41}
\expandafter\def\csname v@vint/r4/test/gpuv/greet-hi\endcsname{2.02}
\expandafter\def\csname v@vint/r4/test/gpuv/greet-lo\endcsname{0.86}
\expandafter\def\csname v@vint/r4/test/gpuv/missed\endcsname{2.5}
\expandafter\def\csname v@vint/r4/test/gpuv/recall\endcsname{88.4}
\expandafter\def\csname v@vint/r4/test/gpuv/silence-after\endcsname{98.6}
\expandafter\def\csname v@vint/r4/test/gpuv/talker\endcsname{0.80}
\expandafter\def\csname v@vint/r4/test/gpuv/wer\endcsname{16.5}
\expandafter\def\csname v@vint/r4/test/none/after\endcsname{2.42}
\expandafter\def\csname v@vint/r4/test/none/after-hi\endcsname{3.29}
\expandafter\def\csname v@vint/r4/test/none/after-lo\endcsname{1.64}
\expandafter\def\csname v@vint/r4/test/none/all\endcsname{2.77}
\expandafter\def\csname v@vint/r4/test/none/all-hi\endcsname{3.73}
\expandafter\def\csname v@vint/r4/test/none/all-lo\endcsname{1.91}
\expandafter\def\csname v@vint/r4/test/none/cut\endcsname{84.8}
\expandafter\def\csname v@vint/r4/test/none/greet\endcsname{5.52}
\expandafter\def\csname v@vint/r4/test/none/greet-hi\endcsname{7.39}
\expandafter\def\csname v@vint/r4/test/none/greet-lo\endcsname{3.80}
\expandafter\def\csname v@vint/r4/test/none/missed\endcsname{0.4}
\expandafter\def\csname v@vint/r4/test/none/recall\endcsname{94.4}
\expandafter\def\csname v@vint/r4/test/none/silence-after\endcsname{0.0}
\expandafter\def\csname v@vint/r4/test/none/talker\endcsname{9.35}
\expandafter\def\csname v@vint/r4/test/none/wer\endcsname{7.4}
\expandafter\def\csname v@vint/r4/test/rel_vb/after\endcsname{0.50}
\expandafter\def\csname v@vint/r4/test/rel_vb/after-hi\endcsname{0.81}
\expandafter\def\csname v@vint/r4/test/rel_vb/after-lo\endcsname{0.25}
\expandafter\def\csname v@vint/r4/test/rel_vb/all\endcsname{0.78}
\expandafter\def\csname v@vint/r4/test/rel_vb/all-hi\endcsname{1.13}
\expandafter\def\csname v@vint/r4/test/rel_vb/all-lo\endcsname{0.49}
\expandafter\def\csname v@vint/r4/test/rel_vb/cut\endcsname{90.9}
\expandafter\def\csname v@vint/r4/test/rel_vb/greet\endcsname{3.02}
\expandafter\def\csname v@vint/r4/test/rel_vb/greet-hi\endcsname{3.97}
\expandafter\def\csname v@vint/r4/test/rel_vb/greet-lo\endcsname{2.12}
\expandafter\def\csname v@vint/r4/test/rel_vb/missed\endcsname{0.6}
\expandafter\def\csname v@vint/r4/test/rel_vb/recall\endcsname{92.1}
\expandafter\def\csname v@vint/r4/test/rel_vb/silence-after\endcsname{69.3}
\expandafter\def\csname v@vint/r4/test/rel_vb/talker\endcsname{2.48}
\expandafter\def\csname v@vint/r4/test/rel_vb/wer\endcsname{13.4}
\expandafter\def\csname v@vint/r4/test/reuse/after\endcsname{0.24}
\expandafter\def\csname v@vint/r4/test/reuse/after-hi\endcsname{0.45}
\expandafter\def\csname v@vint/r4/test/reuse/after-lo\endcsname{0.08}
\expandafter\def\csname v@vint/r4/test/reuse/all\endcsname{0.95}
\expandafter\def\csname v@vint/r4/test/reuse/all-hi\endcsname{1.30}
\expandafter\def\csname v@vint/r4/test/reuse/all-lo\endcsname{0.63}
\expandafter\def\csname v@vint/r4/test/reuse/cut\endcsname{87.4}
\expandafter\def\csname v@vint/r4/test/reuse/greet\endcsname{6.54}
\expandafter\def\csname v@vint/r4/test/reuse/greet-hi\endcsname{8.46}
\expandafter\def\csname v@vint/r4/test/reuse/greet-lo\endcsname{4.71}
\expandafter\def\csname v@vint/r4/test/reuse/missed\endcsname{2.6}
\expandafter\def\csname v@vint/r4/test/reuse/recall\endcsname{87.2}
\expandafter\def\csname v@vint/r4/test/reuse/silence-after\endcsname{98.3}
\expandafter\def\csname v@vint/r4/test/reuse/talker\endcsname{1.47}
\expandafter\def\csname v@vint/r4/test/reuse/wer\endcsname{16.9}
\expandafter\def\csname v@vint/r4/test/sessions\endcsname{17}
\expandafter\def\csname v@vint/r4/tie\endcsname{0.02}
\expandafter\def\csname v@vint/r4/tie/cpu/default/n\endcsname{12}
\expandafter\def\csname v@vint/r4/tie/cpu/default/settings\endcsname{18}
\expandafter\def\csname v@vint/r4/tie/cpu/default/wer-hi\endcsname{18.96}
\expandafter\def\csname v@vint/r4/tie/cpu/default/wer-lo\endcsname{18.04}
\expandafter\def\csname v@vint/r4/tie/cpu/voicebot/n\endcsname{2}
\expandafter\def\csname v@vint/r4/tie/cpu/voicebot/settings\endcsname{5}
\expandafter\def\csname v@vint/r4/tie/cpu/voicebot/wer-hi\endcsname{19.07}
\expandafter\def\csname v@vint/r4/tie/cpu/voicebot/wer-lo\endcsname{18.76}
\expandafter\def\csname v@vint/r4/tie/gpu/voicebot/n\endcsname{4}
\expandafter\def\csname v@vint/r4/tie/gpu/voicebot/settings\endcsname{8}
\expandafter\def\csname v@vint/r4/tie/gpu/voicebot/wer-hi\endcsname{18.73}
\expandafter\def\csname v@vint/r4/tie/gpu/voicebot/wer-lo\endcsname{17.83}
\expandafter\def\csname v@vint/r4/wait/cpu/0/all\endcsname{0.26}
\expandafter\def\csname v@vint/r4/wait/cpu/0/beds\endcsname{32.7}
\expandafter\def\csname v@vint/r4/wait/cpu/0/clean\endcsname{25.6}
\expandafter\def\csname v@vint/r4/wait/cpu/0/greet\endcsname{1.26}
\expandafter\def\csname v@vint/r4/wait/cpu/0/missed\endcsname{1.36}
\expandafter\def\csname v@vint/r4/wait/cpu/1/all\endcsname{0.34}
\expandafter\def\csname v@vint/r4/wait/cpu/1/beds\endcsname{32.6}
\expandafter\def\csname v@vint/r4/wait/cpu/1/clean\endcsname{25.4}
\expandafter\def\csname v@vint/r4/wait/cpu/1/greet\endcsname{1.94}
\expandafter\def\csname v@vint/r4/wait/cpu/1/missed\endcsname{1.35}
\expandafter\def\csname v@vint/r4/wait/cpu/12/all\endcsname{0.26}
\expandafter\def\csname v@vint/r4/wait/cpu/12/beds\endcsname{32.7}
\expandafter\def\csname v@vint/r4/wait/cpu/12/clean\endcsname{25.6}
\expandafter\def\csname v@vint/r4/wait/cpu/12/greet\endcsname{1.26}
\expandafter\def\csname v@vint/r4/wait/cpu/12/missed\endcsname{1.36}
\expandafter\def\csname v@vint/r4/wait/cpu/2/all\endcsname{0.31}
\expandafter\def\csname v@vint/r4/wait/cpu/2/beds\endcsname{32.6}
\expandafter\def\csname v@vint/r4/wait/cpu/2/clean\endcsname{25.6}
\expandafter\def\csname v@vint/r4/wait/cpu/2/greet\endcsname{1.74}
\expandafter\def\csname v@vint/r4/wait/cpu/2/missed\endcsname{1.35}
\expandafter\def\csname v@vint/r4/wait/cpu/3/all\endcsname{0.30}
\expandafter\def\csname v@vint/r4/wait/cpu/3/beds\endcsname{32.7}
\expandafter\def\csname v@vint/r4/wait/cpu/3/clean\endcsname{25.6}
\expandafter\def\csname v@vint/r4/wait/cpu/3/greet\endcsname{1.60}
\expandafter\def\csname v@vint/r4/wait/cpu/3/missed\endcsname{1.35}
\expandafter\def\csname v@vint/r4/wait/cpu/5/all\endcsname{0.28}
\expandafter\def\csname v@vint/r4/wait/cpu/5/beds\endcsname{32.7}
\expandafter\def\csname v@vint/r4/wait/cpu/5/clean\endcsname{25.6}
\expandafter\def\csname v@vint/r4/wait/cpu/5/greet\endcsname{1.47}
\expandafter\def\csname v@vint/r4/wait/cpu/5/missed\endcsname{1.35}
\expandafter\def\csname v@vint/r4/wait/cpu/closed/all\endcsname{0.16}
\expandafter\def\csname v@vint/r4/wait/cpu/closed/beds\endcsname{98.9}
\expandafter\def\csname v@vint/r4/wait/cpu/closed/clean\endcsname{100.0}
\expandafter\def\csname v@vint/r4/wait/cpu/closed/greet\endcsname{0.43}
\expandafter\def\csname v@vint/r4/wait/cpu/closed/missed\endcsname{1.60}
\expandafter\def\csname v@vint/r4/wait/cpu/pick\endcsname{never}
\expandafter\def\csname v@vint/r4/wait/gpu/0/all\endcsname{0.24}
\expandafter\def\csname v@vint/r4/wait/gpu/0/beds\endcsname{31.2}
\expandafter\def\csname v@vint/r4/wait/gpu/0/clean\endcsname{25.2}
\expandafter\def\csname v@vint/r4/wait/gpu/0/greet\endcsname{0.92}
\expandafter\def\csname v@vint/r4/wait/gpu/0/missed\endcsname{1.70}
\expandafter\def\csname v@vint/r4/wait/gpu/1/all\endcsname{0.39}
\expandafter\def\csname v@vint/r4/wait/gpu/1/beds\endcsname{15.7}
\expandafter\def\csname v@vint/r4/wait/gpu/1/clean\endcsname{24.9}
\expandafter\def\csname v@vint/r4/wait/gpu/1/greet\endcsname{2.21}
\expandafter\def\csname v@vint/r4/wait/gpu/1/missed\endcsname{1.70}
\expandafter\def\csname v@vint/r4/wait/gpu/12/all\endcsname{0.25}
\expandafter\def\csname v@vint/r4/wait/gpu/12/beds\endcsname{19.5}
\expandafter\def\csname v@vint/r4/wait/gpu/12/clean\endcsname{25.2}
\expandafter\def\csname v@vint/r4/wait/gpu/12/greet\endcsname{0.97}
\expandafter\def\csname v@vint/r4/wait/gpu/12/missed\endcsname{1.70}
\expandafter\def\csname v@vint/r4/wait/gpu/2/all\endcsname{0.35}
\expandafter\def\csname v@vint/r4/wait/gpu/2/beds\endcsname{16.1}
\expandafter\def\csname v@vint/r4/wait/gpu/2/clean\endcsname{25.0}
\expandafter\def\csname v@vint/r4/wait/gpu/2/greet\endcsname{1.87}
\expandafter\def\csname v@vint/r4/wait/gpu/2/missed\endcsname{1.70}
\expandafter\def\csname v@vint/r4/wait/gpu/3/all\endcsname{0.32}
\expandafter\def\csname v@vint/r4/wait/gpu/3/beds\endcsname{16.3}
\expandafter\def\csname v@vint/r4/wait/gpu/3/clean\endcsname{25.2}
\expandafter\def\csname v@vint/r4/wait/gpu/3/greet\endcsname{1.62}
\expandafter\def\csname v@vint/r4/wait/gpu/3/missed\endcsname{1.70}
\expandafter\def\csname v@vint/r4/wait/gpu/5/all\endcsname{0.27}
\expandafter\def\csname v@vint/r4/wait/gpu/5/beds\endcsname{18.4}
\expandafter\def\csname v@vint/r4/wait/gpu/5/clean\endcsname{25.2}
\expandafter\def\csname v@vint/r4/wait/gpu/5/greet\endcsname{1.22}
\expandafter\def\csname v@vint/r4/wait/gpu/5/missed\endcsname{1.70}
\expandafter\def\csname v@vint/r4/wait/gpu/closed/all\endcsname{0.17}
\expandafter\def\csname v@vint/r4/wait/gpu/closed/beds\endcsname{98.9}
\expandafter\def\csname v@vint/r4/wait/gpu/closed/clean\endcsname{100.0}
\expandafter\def\csname v@vint/r4/wait/gpu/closed/greet\endcsname{0.36}
\expandafter\def\csname v@vint/r4/wait/gpu/closed/missed\endcsname{1.97}
\expandafter\def\csname v@vint/r4/wait/gpu/pick\endcsname{3}
\expandafter\def\csname v@vint/r4/where/agent/after\endcsname{0.15}
\expandafter\def\csname v@vint/r4/where/agent/greet\endcsname{3.58}
\expandafter\def\csname v@vint/r4/where/agent/greet-minutes\endcsname{12}
\expandafter\def\csname v@vint/r4/where/agent/greet-share\endcsname{76}
\expandafter\def\csname v@vint/r4/where/agent/low-of-lost\endcsname{46}
\expandafter\def\csname v@vint/r4/where/agent/missed-high\endcsname{1.1}
\expandafter\def\csname v@vint/r4/where/agent/missed-low\endcsname{8.7}
\expandafter\def\csname v@vint/r4/where/agent/talker-greet\endcsname{15.3}
\expandafter\def\csname v@vint/r4/where/calls\endcsname{608}
\expandafter\def\csname v@vint/r4/where/cpuag/after\endcsname{0.12}
\expandafter\def\csname v@vint/r4/where/cpuag/greet\endcsname{3.67}
\expandafter\def\csname v@vint/r4/where/cpuag/greet-minutes\endcsname{12}
\expandafter\def\csname v@vint/r4/where/cpuag/greet-share\endcsname{80}
\expandafter\def\csname v@vint/r4/where/cpuag/low-of-lost\endcsname{61}
\expandafter\def\csname v@vint/r4/where/cpuag/missed-high\endcsname{1.2}
\expandafter\def\csname v@vint/r4/where/cpuag/missed-low\endcsname{14.3}
\expandafter\def\csname v@vint/r4/where/cpuag/talker-greet\endcsname{15.7}
\expandafter\def\csname v@vint/r4/where/first-p50\endcsname{5.9}
\expandafter\def\csname v@vint/r4/where/first-p90\endcsname{13.4}
\expandafter\def\csname v@vint/r4/where/low-calls\endcsname{67}
\expandafter\def\csname v@vint/r4/where/low-share\endcsname{11}
\expandafter\def\csname v@vint/r4/where/none/after\endcsname{2.02}
\expandafter\def\csname v@vint/r4/where/none/greet\endcsname{5.10}
\expandafter\def\csname v@vint/r4/where/none/greet-minutes\endcsname{12}
\expandafter\def\csname v@vint/r4/where/none/greet-share\endcsname{25}
\expandafter\def\csname v@vint/r4/where/none/low-of-lost\endcsname{21}
\expandafter\def\csname v@vint/r4/where/none/missed-high\endcsname{0.3}
\expandafter\def\csname v@vint/r4/where/none/missed-low\endcsname{0.6}
\expandafter\def\csname v@vint/r4/where/none/talker-greet\endcsname{17.8}
\expandafter\def\csname v@vint/r4/where/reuse/after\endcsname{0.19}
\expandafter\def\csname v@vint/r4/where/reuse/greet\endcsname{6.04}
\expandafter\def\csname v@vint/r4/where/reuse/greet-minutes\endcsname{12}
\expandafter\def\csname v@vint/r4/where/reuse/greet-share\endcsname{81}
\expandafter\def\csname v@vint/r4/where/reuse/low-of-lost\endcsname{28}
\expandafter\def\csname v@vint/r4/where/reuse/missed-high\endcsname{2.0}
\expandafter\def\csname v@vint/r4/where/reuse/missed-low\endcsname{8.5}
\expandafter\def\csname v@vint/r4/where/reuse/talker-greet\endcsname{18.8}
\expandafter\def\csname v@vint/rel/caught\endcsname{89.9}
\expandafter\def\csname v@vint/rel/caught-hi\endcsname{91.5}
\expandafter\def\csname v@vint/rel/caught-lo\endcsname{88.1}
\expandafter\def\csname v@vint/rel/fi\endcsname{1.05}
\expandafter\def\csname v@vint/rel/fi-hi\endcsname{1.48}
\expandafter\def\csname v@vint/rel/fi-lo\endcsname{0.69}
\expandafter\def\csname v@vint/rel/fs\endcsname{1.23}
\expandafter\def\csname v@vint/rel/fs-hi\endcsname{1.75}
\expandafter\def\csname v@vint/rel/fs-lo\endcsname{0.77}
\expandafter\def\csname v@vint/rel/held\endcsname{3.5}
\expandafter\def\csname v@vint/rel/held-hi\endcsname{5.4}
\expandafter\def\csname v@vint/rel/held-lo\endcsname{2.0}
\expandafter\def\csname v@vint/rel/kind/babble/fi\endcsname{0.84}
\expandafter\def\csname v@vint/rel/kind/babble/fs\endcsname{0.89}
\expandafter\def\csname v@vint/rel/kind/babble/missed\endcsname{0.0}
\expandafter\def\csname v@vint/rel/kind/clean/fi\endcsname{0.00}
\expandafter\def\csname v@vint/rel/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/rel/kind/clean/missed\endcsname{0.5}
\expandafter\def\csname v@vint/rel/kind/home/fi\endcsname{0.49}
\expandafter\def\csname v@vint/rel/kind/home/fs\endcsname{0.58}
\expandafter\def\csname v@vint/rel/kind/home/missed\endcsname{0.4}
\expandafter\def\csname v@vint/rel/kind/music/fi\endcsname{0.34}
\expandafter\def\csname v@vint/rel/kind/music/fs\endcsname{0.37}
\expandafter\def\csname v@vint/rel/kind/music/missed\endcsname{0.1}
\expandafter\def\csname v@vint/rel/kind/street/fi\endcsname{0.08}
\expandafter\def\csname v@vint/rel/kind/street/fs\endcsname{0.10}
\expandafter\def\csname v@vint/rel/kind/street/missed\endcsname{0.2}
\expandafter\def\csname v@vint/rel/kind/talker/fi\endcsname{4.92}
\expandafter\def\csname v@vint/rel/kind/talker/fs\endcsname{4.21}
\expandafter\def\csname v@vint/rel/kind/talker/missed\endcsname{2.7}
\expandafter\def\csname v@vint/rel/live/barge_p50\endcsname{0.77}
\expandafter\def\csname v@vint/rel/live/caught\endcsname{94.7}
\expandafter\def\csname v@vint/rel/live/eot_p50\endcsname{0.87}
\expandafter\def\csname v@vint/rel/live/eot_p90\endcsname{1.64}
\expandafter\def\csname v@vint/rel/live/fi_transcript\endcsname{3.44}
\expandafter\def\csname v@vint/rel/live/fi_vad\endcsname{0.91}
\expandafter\def\csname v@vint/rel/live/frame-p50\endcsname{0.2}
\expandafter\def\csname v@vint/rel/live/frame-p99\endcsname{25.7}
\expandafter\def\csname v@vint/rel/live/fs\endcsname{1.36}
\expandafter\def\csname v@vint/rel/live/no_reply\endcsname{6.2}
\expandafter\def\csname v@vint/rel/live/unfiltered_pct\endcsname{0.03}
\expandafter\def\csname v@vint/rel/missed\endcsname{0.7}
\expandafter\def\csname v@vint/rel/missed-hi\endcsname{1.1}
\expandafter\def\csname v@vint/rel/missed-lo\endcsname{0.3}
\expandafter\def\csname v@vint/rel/recall\endcsname{90.9}
\expandafter\def\csname v@vint/rel/server/calls\endcsname{16}
\expandafter\def\csname v@vint/rel/server/step-p50\endcsname{21}
\expandafter\def\csname v@vint/rel/server/step-p99\endcsname{22}
\expandafter\def\csname v@vint/rel/snr/0.0/fi\endcsname{1.90}
\expandafter\def\csname v@vint/rel/snr/10.0/fi\endcsname{0.90}
\expandafter\def\csname v@vint/rel/snr/20.0/fi\endcsname{0.64}
\expandafter\def\csname v@vint/rel/snr/None/fi\endcsname{0.00}
\expandafter\def\csname v@vint/rel/wer\endcsname{13.4}
\expandafter\def\csname v@vint/rel/wer/babble\endcsname{18.2}
\expandafter\def\csname v@vint/rel/wer/clean\endcsname{5.0}
\expandafter\def\csname v@vint/rel/wer/home\endcsname{12.6}
\expandafter\def\csname v@vint/rel/wer/music\endcsname{10.5}
\expandafter\def\csname v@vint/rel/wer/street\endcsname{10.2}
\expandafter\def\csname v@vint/rel/wer/talker\endcsname{19.7}
\expandafter\def\csname v@vint/rel_old/live/barge_p50\endcsname{0.79}
\expandafter\def\csname v@vint/rel_old/live/caught\endcsname{82.6}
\expandafter\def\csname v@vint/rel_old/live/eot_p50\endcsname{0.94}
\expandafter\def\csname v@vint/rel_old/live/eot_p90\endcsname{1.75}
\expandafter\def\csname v@vint/rel_old/live/fi_transcript\endcsname{3.57}
\expandafter\def\csname v@vint/rel_old/live/fi_vad\endcsname{1.23}
\expandafter\def\csname v@vint/rel_old/live/frame-p50\endcsname{12.8}
\expandafter\def\csname v@vint/rel_old/live/frame-p99\endcsname{30.4}
\expandafter\def\csname v@vint/rel_old/live/fs\endcsname{1.86}
\expandafter\def\csname v@vint/rel_old/live/no_reply\endcsname{8.1}
\expandafter\def\csname v@vint/rel_old/live/unfiltered_pct\endcsname{12.35}
\expandafter\def\csname v@vint/reuse/caught\endcsname{87.3}
\expandafter\def\csname v@vint/reuse/caught-d\endcsname{-2.6}
\expandafter\def\csname v@vint/reuse/caught-dabs\endcsname{2.6}
\expandafter\def\csname v@vint/reuse/caught-dhi\endcsname{-0.7}
\expandafter\def\csname v@vint/reuse/caught-dlo\endcsname{-5.1}
\expandafter\def\csname v@vint/reuse/caught-hi\endcsname{90.1}
\expandafter\def\csname v@vint/reuse/caught-lo\endcsname{84.0}
\expandafter\def\csname v@vint/reuse/fi\endcsname{0.95}
\expandafter\def\csname v@vint/reuse/fi-d\endcsname{-0.10}
\expandafter\def\csname v@vint/reuse/fi-dabs\endcsname{0.10}
\expandafter\def\csname v@vint/reuse/fi-dhi\endcsname{+0.02}
\expandafter\def\csname v@vint/reuse/fi-dlo\endcsname{-0.24}
\expandafter\def\csname v@vint/reuse/fi-hi\endcsname{1.30}
\expandafter\def\csname v@vint/reuse/fi-lo\endcsname{0.63}
\expandafter\def\csname v@vint/reuse/fs\endcsname{1.01}
\expandafter\def\csname v@vint/reuse/fs-d\endcsname{-0.22}
\expandafter\def\csname v@vint/reuse/fs-dabs\endcsname{0.22}
\expandafter\def\csname v@vint/reuse/fs-dhi\endcsname{-0.08}
\expandafter\def\csname v@vint/reuse/fs-dlo\endcsname{-0.37}
\expandafter\def\csname v@vint/reuse/fs-hi\endcsname{1.43}
\expandafter\def\csname v@vint/reuse/fs-lo\endcsname{0.64}
\expandafter\def\csname v@vint/reuse/held\endcsname{5.8}
\expandafter\def\csname v@vint/reuse/held-d\endcsname{+2.3}
\expandafter\def\csname v@vint/reuse/held-dabs\endcsname{2.3}
\expandafter\def\csname v@vint/reuse/held-dhi\endcsname{+5.2}
\expandafter\def\csname v@vint/reuse/held-dlo\endcsname{-0.1}
\expandafter\def\csname v@vint/reuse/held-hi\endcsname{10.1}
\expandafter\def\csname v@vint/reuse/held-lo\endcsname{2.2}
\expandafter\def\csname v@vint/reuse/kind/babble/fi\endcsname{1.02}
\expandafter\def\csname v@vint/reuse/kind/babble/fs\endcsname{0.87}
\expandafter\def\csname v@vint/reuse/kind/babble/missed\endcsname{0.4}
\expandafter\def\csname v@vint/reuse/kind/clean/fi\endcsname{0.00}
\expandafter\def\csname v@vint/reuse/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/reuse/kind/clean/missed\endcsname{0.0}
\expandafter\def\csname v@vint/reuse/kind/home/fi\endcsname{0.52}
\expandafter\def\csname v@vint/reuse/kind/home/fs\endcsname{0.52}
\expandafter\def\csname v@vint/reuse/kind/home/missed\endcsname{0.1}
\expandafter\def\csname v@vint/reuse/kind/music/fi\endcsname{0.11}
\expandafter\def\csname v@vint/reuse/kind/music/fs\endcsname{0.09}
\expandafter\def\csname v@vint/reuse/kind/music/missed\endcsname{0.0}
\expandafter\def\csname v@vint/reuse/kind/street/fi\endcsname{0.16}
\expandafter\def\csname v@vint/reuse/kind/street/fs\endcsname{0.14}
\expandafter\def\csname v@vint/reuse/kind/street/missed\endcsname{0.0}
\expandafter\def\csname v@vint/reuse/kind/talker/fi\endcsname{4.16}
\expandafter\def\csname v@vint/reuse/kind/talker/fs\endcsname{3.43}
\expandafter\def\csname v@vint/reuse/kind/talker/missed\endcsname{13.9}
\expandafter\def\csname v@vint/reuse/live/barge_p50\endcsname{0.84}
\expandafter\def\csname v@vint/reuse/live/caught\endcsname{88.7}
\expandafter\def\csname v@vint/reuse/live/eot_p50\endcsname{0.90}
\expandafter\def\csname v@vint/reuse/live/eot_p90\endcsname{1.67}
\expandafter\def\csname v@vint/reuse/live/fi_transcript\endcsname{4.05}
\expandafter\def\csname v@vint/reuse/live/fi_vad\endcsname{0.87}
\expandafter\def\csname v@vint/reuse/live/frame-p50\endcsname{0.1}
\expandafter\def\csname v@vint/reuse/live/frame-p99\endcsname{27.3}
\expandafter\def\csname v@vint/reuse/live/fs\endcsname{1.40}
\expandafter\def\csname v@vint/reuse/live/no_reply\endcsname{7.3}
\expandafter\def\csname v@vint/reuse/live/unfiltered_pct\endcsname{0.14}
\expandafter\def\csname v@vint/reuse/missed\endcsname{2.6}
\expandafter\def\csname v@vint/reuse/missed-d\endcsname{+1.9}
\expandafter\def\csname v@vint/reuse/missed-dabs\endcsname{1.9}
\expandafter\def\csname v@vint/reuse/missed-dhi\endcsname{+3.9}
\expandafter\def\csname v@vint/reuse/missed-dlo\endcsname{+0.3}
\expandafter\def\csname v@vint/reuse/missed-hi\endcsname{4.8}
\expandafter\def\csname v@vint/reuse/missed-lo\endcsname{0.7}
\expandafter\def\csname v@vint/reuse/recall\endcsname{87.2}
\expandafter\def\csname v@vint/reuse/server/calls\endcsname{11}
\expandafter\def\csname v@vint/reuse/server/step-p50\endcsname{34}
\expandafter\def\csname v@vint/reuse/server/step-p99\endcsname{48}
\expandafter\def\csname v@vint/reuse/snr/0.0/fi\endcsname{1.69}
\expandafter\def\csname v@vint/reuse/snr/10.0/fi\endcsname{0.86}
\expandafter\def\csname v@vint/reuse/snr/20.0/fi\endcsname{0.56}
\expandafter\def\csname v@vint/reuse/snr/None/fi\endcsname{0.00}
\expandafter\def\csname v@vint/reuse/wer\endcsname{16.9}
\expandafter\def\csname v@vint/reuse/wer/babble\endcsname{17.5}
\expandafter\def\csname v@vint/reuse/wer/clean\endcsname{1.2}
\expandafter\def\csname v@vint/reuse/wer/home\endcsname{12.3}
\expandafter\def\csname v@vint/reuse/wer/music\endcsname{7.7}
\expandafter\def\csname v@vint/reuse/wer/street\endcsname{9.4}
\expandafter\def\csname v@vint/reuse/wer/talker\endcsname{47.1}
\expandafter\def\csname v@vint/reuse_old/live/barge_p50\endcsname{0.83}
\expandafter\def\csname v@vint/reuse_old/live/caught\endcsname{79.0}
\expandafter\def\csname v@vint/reuse_old/live/eot_p50\endcsname{0.92}
\expandafter\def\csname v@vint/reuse_old/live/eot_p90\endcsname{1.69}
\expandafter\def\csname v@vint/reuse_old/live/fi_transcript\endcsname{3.85}
\expandafter\def\csname v@vint/reuse_old/live/fi_vad\endcsname{0.83}
\expandafter\def\csname v@vint/reuse_old/live/frame-p50\endcsname{1.8}
\expandafter\def\csname v@vint/reuse_old/live/frame-p99\endcsname{29.3}
\expandafter\def\csname v@vint/reuse_old/live/fs\endcsname{1.33}
\expandafter\def\csname v@vint/reuse_old/live/no_reply\endcsname{7.3}
\expandafter\def\csname v@vint/reuse_old/live/unfiltered_pct\endcsname{3.48}
\expandafter\def\csname v@vint/reuse_shared/server/calls\endcsname{16}
\expandafter\def\csname v@vint/reuse_shared/server/step-p50\endcsname{59}
\expandafter\def\csname v@vint/reuse_shared/server/step-p99\endcsname{66}
\expandafter\def\csname v@vint/reuse_void/live/barge_p50\endcsname{0.83}
\expandafter\def\csname v@vint/reuse_void/live/caught\endcsname{88.5}
\expandafter\def\csname v@vint/reuse_void/live/eot_p50\endcsname{1.03}
\expandafter\def\csname v@vint/reuse_void/live/eot_p90\endcsname{2.51}
\expandafter\def\csname v@vint/reuse_void/live/fi_transcript\endcsname{5.14}
\expandafter\def\csname v@vint/reuse_void/live/fi_vad\endcsname{2.26}
\expandafter\def\csname v@vint/reuse_void/live/frame-p50\endcsname{30.3}
\expandafter\def\csname v@vint/reuse_void/live/frame-p99\endcsname{31.0}
\expandafter\def\csname v@vint/reuse_void/live/fs\endcsname{3.44}
\expandafter\def\csname v@vint/reuse_void/live/no_reply\endcsname{6.5}
\expandafter\def\csname v@vint/reuse_void/live/unfiltered_pct\endcsname{79.46}
\expandafter\def\csname v@vint/sessions\endcsname{17}
\expandafter\def\csname v@vint/sessions/cpu/max\endcsname{1.78}
\expandafter\def\csname v@vint/sessions/cpu/min\endcsname{0.97}
\expandafter\def\csname v@vint/sessions/ft/max\endcsname{1.13}
\expandafter\def\csname v@vint/sessions/ft/min\endcsname{0.63}
\expandafter\def\csname v@vint/sessions/gtcrn/max\endcsname{6.32}
\expandafter\def\csname v@vint/sessions/gtcrn/min\endcsname{4.68}
\expandafter\def\csname v@vint/sessions/none/max\endcsname{3.28}
\expandafter\def\csname v@vint/sessions/none/min\endcsname{2.24}
\expandafter\def\csname v@vint/sessions/rel/max\endcsname{1.35}
\expandafter\def\csname v@vint/sessions/rel/min\endcsname{0.82}
\expandafter\def\csname v@vint/sessions/reuse/max\endcsname{1.16}
\expandafter\def\csname v@vint/sessions/reuse/min\endcsname{0.71}
\expandafter\def\csname v@vint/sessions/voxlock/max\endcsname{1.44}
\expandafter\def\csname v@vint/sessions/voxlock/min\endcsname{0.86}
\expandafter\def\csname v@vint/ship/cpu/caught\endcsname{91.0}
\expandafter\def\csname v@vint/ship/cpu/caught-hi\endcsname{92.6}
\expandafter\def\csname v@vint/ship/cpu/caught-lo\endcsname{89.3}
\expandafter\def\csname v@vint/ship/cpu/fi\endcsname{1.36}
\expandafter\def\csname v@vint/ship/cpu/fi-hi\endcsname{1.87}
\expandafter\def\csname v@vint/ship/cpu/fi-lo\endcsname{0.92}
\expandafter\def\csname v@vint/ship/cpu/fs\endcsname{1.57}
\expandafter\def\csname v@vint/ship/cpu/fs-hi\endcsname{2.16}
\expandafter\def\csname v@vint/ship/cpu/fs-lo\endcsname{1.04}
\expandafter\def\csname v@vint/ship/cpu/held\endcsname{3.4}
\expandafter\def\csname v@vint/ship/cpu/held-hi\endcsname{5.4}
\expandafter\def\csname v@vint/ship/cpu/held-lo\endcsname{1.7}
\expandafter\def\csname v@vint/ship/cpu/missed\endcsname{0.3}
\expandafter\def\csname v@vint/ship/cpu/missed-hi\endcsname{0.6}
\expandafter\def\csname v@vint/ship/cpu/missed-lo\endcsname{0.1}
\expandafter\def\csname v@vint/ship/cpu/wer\endcsname{11.9}
\expandafter\def\csname v@vint/ship/cpu8/caught\endcsname{90.9}
\expandafter\def\csname v@vint/ship/cpu8/caught-hi\endcsname{92.5}
\expandafter\def\csname v@vint/ship/cpu8/caught-lo\endcsname{89.1}
\expandafter\def\csname v@vint/ship/cpu8/fi\endcsname{1.36}
\expandafter\def\csname v@vint/ship/cpu8/fi-hi\endcsname{1.88}
\expandafter\def\csname v@vint/ship/cpu8/fi-lo\endcsname{0.93}
\expandafter\def\csname v@vint/ship/cpu8/fs\endcsname{1.58}
\expandafter\def\csname v@vint/ship/cpu8/fs-hi\endcsname{2.17}
\expandafter\def\csname v@vint/ship/cpu8/fs-lo\endcsname{1.05}
\expandafter\def\csname v@vint/ship/cpu8/held\endcsname{3.4}
\expandafter\def\csname v@vint/ship/cpu8/held-hi\endcsname{5.4}
\expandafter\def\csname v@vint/ship/cpu8/held-lo\endcsname{1.7}
\expandafter\def\csname v@vint/ship/cpu8/missed\endcsname{0.3}
\expandafter\def\csname v@vint/ship/cpu8/missed-hi\endcsname{0.6}
\expandafter\def\csname v@vint/ship/cpu8/missed-lo\endcsname{0.1}
\expandafter\def\csname v@vint/ship/cpu8/wer\endcsname{11.8}
\expandafter\def\csname v@vint/ship/cpu8_vb/caught\endcsname{90.9}
\expandafter\def\csname v@vint/ship/cpu8_vb/caught-hi\endcsname{92.6}
\expandafter\def\csname v@vint/ship/cpu8_vb/caught-lo\endcsname{89.2}
\expandafter\def\csname v@vint/ship/cpu8_vb/fi\endcsname{1.13}
\expandafter\def\csname v@vint/ship/cpu8_vb/fi-hi\endcsname{1.59}
\expandafter\def\csname v@vint/ship/cpu8_vb/fi-lo\endcsname{0.75}
\expandafter\def\csname v@vint/ship/cpu8_vb/fs\endcsname{1.40}
\expandafter\def\csname v@vint/ship/cpu8_vb/fs-hi\endcsname{1.98}
\expandafter\def\csname v@vint/ship/cpu8_vb/fs-lo\endcsname{0.89}
\expandafter\def\csname v@vint/ship/cpu8_vb/held\endcsname{3.3}
\expandafter\def\csname v@vint/ship/cpu8_vb/held-hi\endcsname{5.3}
\expandafter\def\csname v@vint/ship/cpu8_vb/held-lo\endcsname{1.7}
\expandafter\def\csname v@vint/ship/cpu8_vb/missed\endcsname{0.3}
\expandafter\def\csname v@vint/ship/cpu8_vb/missed-hi\endcsname{0.6}
\expandafter\def\csname v@vint/ship/cpu8_vb/missed-lo\endcsname{0.1}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/caught\endcsname{+0.1}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/caught-abs\endcsname{0.1}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/caught-abshi\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/caught-abslo\endcsname{0.2}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/caught-hi\endcsname{+0.2}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/caught-lo\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fi\endcsname{-0.23}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fi-abs\endcsname{0.23}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fi-abshi\endcsname{0.34}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fi-abslo\endcsname{0.14}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fi-hi\endcsname{-0.14}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fi-lo\endcsname{-0.34}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fs\endcsname{-0.17}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fs-abs\endcsname{0.17}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fs-abshi\endcsname{0.24}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fs-abslo\endcsname{0.11}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fs-hi\endcsname{-0.11}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/fs-lo\endcsname{-0.24}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/held\endcsname{-0.1}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/held-abs\endcsname{0.1}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/held-abshi\endcsname{0.2}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/held-abslo\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/held-hi\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/held-lo\endcsname{-0.2}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/missed\endcsname{-0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/missed-abs\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/missed-abshi\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/missed-abslo\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/missed-hi\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/vs-cpu8/missed-lo\endcsname{-0.0}
\expandafter\def\csname v@vint/ship/cpu8_vb/wer\endcsname{11.7}
\expandafter\def\csname v@vint/ship/cpu_vb/caught\endcsname{91.0}
\expandafter\def\csname v@vint/ship/cpu_vb/caught-hi\endcsname{92.6}
\expandafter\def\csname v@vint/ship/cpu_vb/caught-lo\endcsname{89.3}
\expandafter\def\csname v@vint/ship/cpu_vb/fi\endcsname{1.13}
\expandafter\def\csname v@vint/ship/cpu_vb/fi-hi\endcsname{1.58}
\expandafter\def\csname v@vint/ship/cpu_vb/fi-lo\endcsname{0.75}
\expandafter\def\csname v@vint/ship/cpu_vb/fs\endcsname{1.42}
\expandafter\def\csname v@vint/ship/cpu_vb/fs-hi\endcsname{2.00}
\expandafter\def\csname v@vint/ship/cpu_vb/fs-lo\endcsname{0.90}
\expandafter\def\csname v@vint/ship/cpu_vb/held\endcsname{3.3}
\expandafter\def\csname v@vint/ship/cpu_vb/held-hi\endcsname{5.3}
\expandafter\def\csname v@vint/ship/cpu_vb/held-lo\endcsname{1.6}
\expandafter\def\csname v@vint/ship/cpu_vb/missed\endcsname{0.3}
\expandafter\def\csname v@vint/ship/cpu_vb/missed-hi\endcsname{0.6}
\expandafter\def\csname v@vint/ship/cpu_vb/missed-lo\endcsname{0.1}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/caught\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/caught-abs\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/caught-abshi\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/caught-abslo\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/caught-hi\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/caught-lo\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fi\endcsname{-0.23}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fi-abs\endcsname{0.23}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fi-abshi\endcsname{0.34}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fi-abslo\endcsname{0.13}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fi-hi\endcsname{-0.13}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fi-lo\endcsname{-0.34}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fs\endcsname{-0.16}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fs-abs\endcsname{0.16}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fs-abshi\endcsname{0.22}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fs-abslo\endcsname{0.09}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fs-hi\endcsname{-0.09}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/fs-lo\endcsname{-0.22}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/held\endcsname{-0.1}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/held-abs\endcsname{0.1}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/held-abshi\endcsname{0.2}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/held-abslo\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/held-hi\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/held-lo\endcsname{-0.2}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/missed\endcsname{-0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/missed-abs\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/missed-abshi\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/missed-abslo\endcsname{0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/missed-hi\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/vs-cpu/missed-lo\endcsname{-0.0}
\expandafter\def\csname v@vint/ship/cpu_vb/wer\endcsname{11.8}
\expandafter\def\csname v@vint/ship/dev/cpu/fi\endcsname{0.95}
\expandafter\def\csname v@vint/ship/dev/cpu8/fi\endcsname{0.95}
\expandafter\def\csname v@vint/ship/dev/cpu8_vb/fi\endcsname{0.74}
\expandafter\def\csname v@vint/ship/dev/cpu_vb/fi\endcsname{0.74}
\expandafter\def\csname v@vint/ship/dev/none/fi\endcsname{2.47}
\expandafter\def\csname v@vint/ship/dev/rel/fi\endcsname{1.05}
\expandafter\def\csname v@vint/ship/dev/rel_vb/fi\endcsname{0.68}
\expandafter\def\csname v@vint/ship/dev/reuse/fi\endcsname{1.00}
\expandafter\def\csname v@vint/ship/none/caught\endcsname{83.7}
\expandafter\def\csname v@vint/ship/none/caught-hi\endcsname{87.9}
\expandafter\def\csname v@vint/ship/none/caught-lo\endcsname{79.0}
\expandafter\def\csname v@vint/ship/none/fi\endcsname{2.77}
\expandafter\def\csname v@vint/ship/none/fi-hi\endcsname{3.73}
\expandafter\def\csname v@vint/ship/none/fi-lo\endcsname{1.91}
\expandafter\def\csname v@vint/ship/none/fs\endcsname{3.04}
\expandafter\def\csname v@vint/ship/none/fs-hi\endcsname{3.95}
\expandafter\def\csname v@vint/ship/none/fs-lo\endcsname{2.14}
\expandafter\def\csname v@vint/ship/none/held\endcsname{9.3}
\expandafter\def\csname v@vint/ship/none/held-hi\endcsname{13.5}
\expandafter\def\csname v@vint/ship/none/held-lo\endcsname{5.6}
\expandafter\def\csname v@vint/ship/none/missed\endcsname{0.4}
\expandafter\def\csname v@vint/ship/none/missed-hi\endcsname{0.9}
\expandafter\def\csname v@vint/ship/none/missed-lo\endcsname{0.1}
\expandafter\def\csname v@vint/ship/none/wer\endcsname{7.4}
\expandafter\def\csname v@vint/ship/probe/beds/cpu/first\endcsname{1}
\expandafter\def\csname v@vint/ship/probe/beds/cpu/firstsec\endcsname{1}
\expandafter\def\csname v@vint/ship/probe/beds/cpu/later\endcsname{2}
\expandafter\def\csname v@vint/ship/probe/beds/cpu/runs\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/beds/cpu8/first\endcsname{1}
\expandafter\def\csname v@vint/ship/probe/beds/cpu8/firstsec\endcsname{1}
\expandafter\def\csname v@vint/ship/probe/beds/cpu8/later\endcsname{2}
\expandafter\def\csname v@vint/ship/probe/beds/cpu8/runs\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/beds/cpu8_vb/first\endcsname{31}
\expandafter\def\csname v@vint/ship/probe/beds/cpu8_vb/firstsec\endcsname{32}
\expandafter\def\csname v@vint/ship/probe/beds/cpu8_vb/later\endcsname{3}
\expandafter\def\csname v@vint/ship/probe/beds/cpu8_vb/runs\endcsname{5}
\expandafter\def\csname v@vint/ship/probe/beds/cpu_vb/first\endcsname{31}
\expandafter\def\csname v@vint/ship/probe/beds/cpu_vb/firstsec\endcsname{32}
\expandafter\def\csname v@vint/ship/probe/beds/cpu_vb/later\endcsname{3}
\expandafter\def\csname v@vint/ship/probe/beds/cpu_vb/runs\endcsname{5}
\expandafter\def\csname v@vint/ship/probe/beds/n\endcsname{16}
\expandafter\def\csname v@vint/ship/probe/beds/release/first\endcsname{1}
\expandafter\def\csname v@vint/ship/probe/beds/release/firstsec\endcsname{1}
\expandafter\def\csname v@vint/ship/probe/beds/release/later\endcsname{6}
\expandafter\def\csname v@vint/ship/probe/beds/release/runs\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/beds/release_vb/first\endcsname{31}
\expandafter\def\csname v@vint/ship/probe/beds/release_vb/firstsec\endcsname{30}
\expandafter\def\csname v@vint/ship/probe/beds/release_vb/later\endcsname{5}
\expandafter\def\csname v@vint/ship/probe/beds/release_vb/runs\endcsname{5}
\expandafter\def\csname v@vint/ship/probe/clean/cpu/first\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/clean/cpu/firstsec\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/clean/cpu/later\endcsname{3}
\expandafter\def\csname v@vint/ship/probe/clean/cpu/runs\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/clean/cpu8/first\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/clean/cpu8/firstsec\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/clean/cpu8/later\endcsname{3}
\expandafter\def\csname v@vint/ship/probe/clean/cpu8/runs\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/clean/cpu8_vb/first\endcsname{25}
\expandafter\def\csname v@vint/ship/probe/clean/cpu8_vb/firstsec\endcsname{26}
\expandafter\def\csname v@vint/ship/probe/clean/cpu8_vb/later\endcsname{4}
\expandafter\def\csname v@vint/ship/probe/clean/cpu8_vb/runs\endcsname{2}
\expandafter\def\csname v@vint/ship/probe/clean/cpu_vb/first\endcsname{25}
\expandafter\def\csname v@vint/ship/probe/clean/cpu_vb/firstsec\endcsname{26}
\expandafter\def\csname v@vint/ship/probe/clean/cpu_vb/later\endcsname{4}
\expandafter\def\csname v@vint/ship/probe/clean/cpu_vb/runs\endcsname{2}
\expandafter\def\csname v@vint/ship/probe/clean/n\endcsname{8}
\expandafter\def\csname v@vint/ship/probe/clean/release/first\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/clean/release/firstsec\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/clean/release/later\endcsname{2}
\expandafter\def\csname v@vint/ship/probe/clean/release/runs\endcsname{0}
\expandafter\def\csname v@vint/ship/probe/clean/release_vb/first\endcsname{25}
\expandafter\def\csname v@vint/ship/probe/clean/release_vb/firstsec\endcsname{26}
\expandafter\def\csname v@vint/ship/probe/clean/release_vb/later\endcsname{4}
\expandafter\def\csname v@vint/ship/probe/clean/release_vb/runs\endcsname{2}
\expandafter\def\csname v@vint/ship/rel/caught\endcsname{90.8}
\expandafter\def\csname v@vint/ship/rel/caught-hi\endcsname{92.4}
\expandafter\def\csname v@vint/ship/rel/caught-lo\endcsname{89.1}
\expandafter\def\csname v@vint/ship/rel/fi\endcsname{1.02}
\expandafter\def\csname v@vint/ship/rel/fi-hi\endcsname{1.45}
\expandafter\def\csname v@vint/ship/rel/fi-lo\endcsname{0.66}
\expandafter\def\csname v@vint/ship/rel/fs\endcsname{1.22}
\expandafter\def\csname v@vint/ship/rel/fs-hi\endcsname{1.74}
\expandafter\def\csname v@vint/ship/rel/fs-lo\endcsname{0.75}
\expandafter\def\csname v@vint/ship/rel/held\endcsname{3.7}
\expandafter\def\csname v@vint/ship/rel/held-hi\endcsname{5.6}
\expandafter\def\csname v@vint/ship/rel/held-lo\endcsname{2.2}
\expandafter\def\csname v@vint/ship/rel/missed\endcsname{0.6}
\expandafter\def\csname v@vint/ship/rel/missed-hi\endcsname{1.0}
\expandafter\def\csname v@vint/ship/rel/missed-lo\endcsname{0.3}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/caught\endcsname{+3.5}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/caught-abs\endcsname{3.5}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/caught-abshi\endcsname{1.5}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/caught-abslo\endcsname{6.1}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/caught-hi\endcsname{+6.1}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/caught-lo\endcsname{+1.5}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fi\endcsname{+0.08}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fi-abs\endcsname{0.08}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fi-abshi\endcsname{0.05}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fi-abslo\endcsname{0.21}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fi-hi\endcsname{+0.21}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fi-lo\endcsname{-0.05}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fs\endcsname{+0.21}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fs-abs\endcsname{0.21}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fs-abshi\endcsname{0.06}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fs-abslo\endcsname{0.36}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fs-hi\endcsname{+0.36}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/fs-lo\endcsname{+0.06}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/held\endcsname{-2.1}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/held-abs\endcsname{2.1}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/held-abshi\endcsname{4.9}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/held-abslo\endcsname{0.3}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/held-hi\endcsname{+0.3}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/held-lo\endcsname{-4.9}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/missed\endcsname{-1.9}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/missed-abs\endcsname{1.9}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/missed-abshi\endcsname{3.9}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/missed-abslo\endcsname{0.3}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/missed-hi\endcsname{-0.3}
\expandafter\def\csname v@vint/ship/rel/vs-reuse/missed-lo\endcsname{-3.9}
\expandafter\def\csname v@vint/ship/rel/wer\endcsname{13.4}
\expandafter\def\csname v@vint/ship/rel_vb/caught\endcsname{90.9}
\expandafter\def\csname v@vint/ship/rel_vb/caught-hi\endcsname{92.5}
\expandafter\def\csname v@vint/ship/rel_vb/caught-lo\endcsname{89.2}
\expandafter\def\csname v@vint/ship/rel_vb/fi\endcsname{0.78}
\expandafter\def\csname v@vint/ship/rel_vb/fi-hi\endcsname{1.13}
\expandafter\def\csname v@vint/ship/rel_vb/fi-lo\endcsname{0.49}
\expandafter\def\csname v@vint/ship/rel_vb/fs\endcsname{1.05}
\expandafter\def\csname v@vint/ship/rel_vb/fs-hi\endcsname{1.53}
\expandafter\def\csname v@vint/ship/rel_vb/fs-lo\endcsname{0.62}
\expandafter\def\csname v@vint/ship/rel_vb/held\endcsname{3.7}
\expandafter\def\csname v@vint/ship/rel_vb/held-hi\endcsname{5.6}
\expandafter\def\csname v@vint/ship/rel_vb/held-lo\endcsname{2.1}
\expandafter\def\csname v@vint/ship/rel_vb/missed\endcsname{0.6}
\expandafter\def\csname v@vint/ship/rel_vb/missed-hi\endcsname{1.0}
\expandafter\def\csname v@vint/ship/rel_vb/missed-lo\endcsname{0.3}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/caught\endcsname{+0.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/caught-abs\endcsname{0.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/caught-abshi\endcsname{0.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/caught-abslo\endcsname{0.3}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/caught-hi\endcsname{+0.3}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/caught-lo\endcsname{-0.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fi\endcsname{-0.24}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fi-abs\endcsname{0.24}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fi-abshi\endcsname{0.37}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fi-abslo\endcsname{0.13}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fi-hi\endcsname{-0.13}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fi-lo\endcsname{-0.37}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fs\endcsname{-0.17}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fs-abs\endcsname{0.17}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fs-abshi\endcsname{0.25}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fs-abslo\endcsname{0.09}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fs-hi\endcsname{-0.09}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/fs-lo\endcsname{-0.25}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/held\endcsname{-0.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/held-abs\endcsname{0.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/held-abshi\endcsname{0.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/held-abslo\endcsname{0.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/held-hi\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/held-lo\endcsname{-0.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/missed\endcsname{-0.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/missed-abs\endcsname{0.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/missed-abshi\endcsname{0.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/missed-abslo\endcsname{0.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/missed-hi\endcsname{+0.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-rel/missed-lo\endcsname{-0.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/caught\endcsname{+3.6}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/caught-abs\endcsname{3.6}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/caught-abshi\endcsname{1.5}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/caught-abslo\endcsname{6.2}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/caught-hi\endcsname{+6.2}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/caught-lo\endcsname{+1.5}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fi\endcsname{-0.17}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fi-abs\endcsname{0.17}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fi-abshi\endcsname{0.31}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fi-abslo\endcsname{0.03}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fi-hi\endcsname{-0.03}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fi-lo\endcsname{-0.31}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fs\endcsname{+0.04}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fs-abs\endcsname{0.04}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fs-abshi\endcsname{0.10}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fs-abslo\endcsname{0.18}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fs-hi\endcsname{+0.18}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/fs-lo\endcsname{-0.10}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/held\endcsname{-2.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/held-abs\endcsname{2.1}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/held-abshi\endcsname{5.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/held-abslo\endcsname{0.2}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/held-hi\endcsname{+0.2}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/held-lo\endcsname{-5.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/missed\endcsname{-2.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/missed-abs\endcsname{2.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/missed-abshi\endcsname{4.0}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/missed-abslo\endcsname{0.3}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/missed-hi\endcsname{-0.3}
\expandafter\def\csname v@vint/ship/rel_vb/vs-reuse/missed-lo\endcsname{-4.0}
\expandafter\def\csname v@vint/ship/rel_vb/wer\endcsname{13.4}
\expandafter\def\csname v@vint/ship/reuse/caught\endcsname{87.3}
\expandafter\def\csname v@vint/ship/reuse/caught-hi\endcsname{90.1}
\expandafter\def\csname v@vint/ship/reuse/caught-lo\endcsname{84.0}
\expandafter\def\csname v@vint/ship/reuse/fi\endcsname{0.95}
\expandafter\def\csname v@vint/ship/reuse/fi-hi\endcsname{1.30}
\expandafter\def\csname v@vint/ship/reuse/fi-lo\endcsname{0.63}
\expandafter\def\csname v@vint/ship/reuse/fs\endcsname{1.01}
\expandafter\def\csname v@vint/ship/reuse/fs-hi\endcsname{1.43}
\expandafter\def\csname v@vint/ship/reuse/fs-lo\endcsname{0.64}
\expandafter\def\csname v@vint/ship/reuse/held\endcsname{5.8}
\expandafter\def\csname v@vint/ship/reuse/held-hi\endcsname{10.1}
\expandafter\def\csname v@vint/ship/reuse/held-lo\endcsname{2.2}
\expandafter\def\csname v@vint/ship/reuse/missed\endcsname{2.6}
\expandafter\def\csname v@vint/ship/reuse/missed-hi\endcsname{4.8}
\expandafter\def\csname v@vint/ship/reuse/missed-lo\endcsname{0.7}
\expandafter\def\csname v@vint/ship/reuse/wer\endcsname{16.9}
\expandafter\def\csname v@vint/silence/bed-calls\endcsname{765}
\expandafter\def\csname v@vint/silence/calls\endcsname{816}
\expandafter\def\csname v@vint/silence/cpu/after\endcsname{0.80}
\expandafter\def\csname v@vint/silence/cpu/after/silence\endcsname{74.9}
\expandafter\def\csname v@vint/silence/cpu/after/vad\endcsname{2.0}
\expandafter\def\csname v@vint/silence/cpu/all\endcsname{1.36}
\expandafter\def\csname v@vint/silence/cpu/before/silence\endcsname{45.7}
\expandafter\def\csname v@vint/silence/cpu/before/vad\endcsname{15.8}
\expandafter\def\csname v@vint/silence/cpu/greet\endcsname{5.77}
\expandafter\def\csname v@vint/silence/cpu/kind/babble/after\endcsname{0.94}
\expandafter\def\csname v@vint/silence/cpu/kind/babble/after-hi\endcsname{1.84}
\expandafter\def\csname v@vint/silence/cpu/kind/babble/after-lo\endcsname{0.19}
\expandafter\def\csname v@vint/silence/cpu/kind/babble/after/silence\endcsname{67.2}
\expandafter\def\csname v@vint/silence/cpu/kind/babble/before/silence\endcsname{37.3}
\expandafter\def\csname v@vint/silence/cpu/kind/babble/greet\endcsname{5.99}
\expandafter\def\csname v@vint/silence/cpu/kind/babble/greet-hi\endcsname{7.23}
\expandafter\def\csname v@vint/silence/cpu/kind/babble/greet-lo\endcsname{4.73}
\expandafter\def\csname v@vint/silence/cpu/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/silence/cpu/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/cpu/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/cpu/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/silence/cpu/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/cpu/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/cpu/kind/home/after\endcsname{0.46}
\expandafter\def\csname v@vint/silence/cpu/kind/home/after-hi\endcsname{0.86}
\expandafter\def\csname v@vint/silence/cpu/kind/home/after-lo\endcsname{0.14}
\expandafter\def\csname v@vint/silence/cpu/kind/home/after/silence\endcsname{79.8}
\expandafter\def\csname v@vint/silence/cpu/kind/home/before/silence\endcsname{54.6}
\expandafter\def\csname v@vint/silence/cpu/kind/home/greet\endcsname{2.89}
\expandafter\def\csname v@vint/silence/cpu/kind/home/greet-hi\endcsname{4.47}
\expandafter\def\csname v@vint/silence/cpu/kind/home/greet-lo\endcsname{1.31}
\expandafter\def\csname v@vint/silence/cpu/kind/music/after\endcsname{0.23}
\expandafter\def\csname v@vint/silence/cpu/kind/music/after-hi\endcsname{0.49}
\expandafter\def\csname v@vint/silence/cpu/kind/music/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/silence/cpu/kind/music/after/silence\endcsname{82.5}
\expandafter\def\csname v@vint/silence/cpu/kind/music/before/silence\endcsname{51.3}
\expandafter\def\csname v@vint/silence/cpu/kind/music/greet\endcsname{2.74}
\expandafter\def\csname v@vint/silence/cpu/kind/music/greet-hi\endcsname{5.01}
\expandafter\def\csname v@vint/silence/cpu/kind/music/greet-lo\endcsname{0.65}
\expandafter\def\csname v@vint/silence/cpu/kind/street/after\endcsname{0.11}
\expandafter\def\csname v@vint/silence/cpu/kind/street/after-hi\endcsname{0.24}
\expandafter\def\csname v@vint/silence/cpu/kind/street/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/silence/cpu/kind/street/after/silence\endcsname{79.7}
\expandafter\def\csname v@vint/silence/cpu/kind/street/before/silence\endcsname{60.6}
\expandafter\def\csname v@vint/silence/cpu/kind/street/greet\endcsname{0.95}
\expandafter\def\csname v@vint/silence/cpu/kind/street/greet-hi\endcsname{1.40}
\expandafter\def\csname v@vint/silence/cpu/kind/street/greet-lo\endcsname{0.50}
\expandafter\def\csname v@vint/silence/cpu/kind/talker/after\endcsname{3.31}
\expandafter\def\csname v@vint/silence/cpu/kind/talker/after-hi\endcsname{5.60}
\expandafter\def\csname v@vint/silence/cpu/kind/talker/after-lo\endcsname{1.38}
\expandafter\def\csname v@vint/silence/cpu/kind/talker/after/silence\endcsname{61.6}
\expandafter\def\csname v@vint/silence/cpu/kind/talker/before/silence\endcsname{29.4}
\expandafter\def\csname v@vint/silence/cpu/kind/talker/greet\endcsname{19.83}
\expandafter\def\csname v@vint/silence/cpu/kind/talker/greet-hi\endcsname{21.21}
\expandafter\def\csname v@vint/silence/cpu/kind/talker/greet-lo\endcsname{18.40}
\expandafter\def\csname v@vint/silence/cpu/trig/down-p50\endcsname{12}
\expandafter\def\csname v@vint/silence/cpu/trig/n\endcsname{378}
\expandafter\def\csname v@vint/silence/cpu/trig/over20\endcsname{20}
\expandafter\def\csname v@vint/silence/ft/after\endcsname{0.39}
\expandafter\def\csname v@vint/silence/ft/after/silence\endcsname{65.5}
\expandafter\def\csname v@vint/silence/ft/after/vad\endcsname{0.7}
\expandafter\def\csname v@vint/silence/ft/all\endcsname{0.86}
\expandafter\def\csname v@vint/silence/ft/before/silence\endcsname{50.0}
\expandafter\def\csname v@vint/silence/ft/before/vad\endcsname{12.2}
\expandafter\def\csname v@vint/silence/ft/greet\endcsname{4.51}
\expandafter\def\csname v@vint/silence/ft/kind/babble/after\endcsname{0.34}
\expandafter\def\csname v@vint/silence/ft/kind/babble/after-hi\endcsname{0.69}
\expandafter\def\csname v@vint/silence/ft/kind/babble/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/silence/ft/kind/babble/after/silence\endcsname{56.9}
\expandafter\def\csname v@vint/silence/ft/kind/babble/before/silence\endcsname{40.6}
\expandafter\def\csname v@vint/silence/ft/kind/babble/greet\endcsname{3.96}
\expandafter\def\csname v@vint/silence/ft/kind/babble/greet-hi\endcsname{5.42}
\expandafter\def\csname v@vint/silence/ft/kind/babble/greet-lo\endcsname{2.46}
\expandafter\def\csname v@vint/silence/ft/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/silence/ft/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/ft/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/ft/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/silence/ft/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/ft/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/ft/kind/home/after\endcsname{0.25}
\expandafter\def\csname v@vint/silence/ft/kind/home/after-hi\endcsname{0.52}
\expandafter\def\csname v@vint/silence/ft/kind/home/after-lo\endcsname{0.03}
\expandafter\def\csname v@vint/silence/ft/kind/home/after/silence\endcsname{71.8}
\expandafter\def\csname v@vint/silence/ft/kind/home/before/silence\endcsname{59.6}
\expandafter\def\csname v@vint/silence/ft/kind/home/greet\endcsname{2.10}
\expandafter\def\csname v@vint/silence/ft/kind/home/greet-hi\endcsname{3.30}
\expandafter\def\csname v@vint/silence/ft/kind/home/greet-lo\endcsname{1.10}
\expandafter\def\csname v@vint/silence/ft/kind/music/after\endcsname{0.19}
\expandafter\def\csname v@vint/silence/ft/kind/music/after-hi\endcsname{0.39}
\expandafter\def\csname v@vint/silence/ft/kind/music/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/silence/ft/kind/music/after/silence\endcsname{70.7}
\expandafter\def\csname v@vint/silence/ft/kind/music/before/silence\endcsname{60.9}
\expandafter\def\csname v@vint/silence/ft/kind/music/greet\endcsname{0.88}
\expandafter\def\csname v@vint/silence/ft/kind/music/greet-hi\endcsname{1.83}
\expandafter\def\csname v@vint/silence/ft/kind/music/greet-lo\endcsname{0.08}
\expandafter\def\csname v@vint/silence/ft/kind/street/after\endcsname{0.03}
\expandafter\def\csname v@vint/silence/ft/kind/street/after-hi\endcsname{0.09}
\expandafter\def\csname v@vint/silence/ft/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/ft/kind/street/after/silence\endcsname{66.8}
\expandafter\def\csname v@vint/silence/ft/kind/street/before/silence\endcsname{63.2}
\expandafter\def\csname v@vint/silence/ft/kind/street/greet\endcsname{0.43}
\expandafter\def\csname v@vint/silence/ft/kind/street/greet-hi\endcsname{0.78}
\expandafter\def\csname v@vint/silence/ft/kind/street/greet-lo\endcsname{0.09}
\expandafter\def\csname v@vint/silence/ft/kind/talker/after\endcsname{1.68}
\expandafter\def\csname v@vint/silence/ft/kind/talker/after-hi\endcsname{3.17}
\expandafter\def\csname v@vint/silence/ft/kind/talker/after-lo\endcsname{0.58}
\expandafter\def\csname v@vint/silence/ft/kind/talker/after/silence\endcsname{59.9}
\expandafter\def\csname v@vint/silence/ft/kind/talker/before/silence\endcsname{30.9}
\expandafter\def\csname v@vint/silence/ft/kind/talker/greet\endcsname{18.25}
\expandafter\def\csname v@vint/silence/ft/kind/talker/greet-hi\endcsname{20.83}
\expandafter\def\csname v@vint/silence/ft/kind/talker/greet-lo\endcsname{15.83}
\expandafter\def\csname v@vint/silence/ft/trig/down-p50\endcsname{11}
\expandafter\def\csname v@vint/silence/ft/trig/n\endcsname{185}
\expandafter\def\csname v@vint/silence/ft/trig/over20\endcsname{18}
\expandafter\def\csname v@vint/silence/gtcrn/after\endcsname{5.07}
\expandafter\def\csname v@vint/silence/gtcrn/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/after/vad\endcsname{18.1}
\expandafter\def\csname v@vint/silence/gtcrn/all\endcsname{5.33}
\expandafter\def\csname v@vint/silence/gtcrn/before/silence\endcsname{0.1}
\expandafter\def\csname v@vint/silence/gtcrn/before/vad\endcsname{19.7}
\expandafter\def\csname v@vint/silence/gtcrn/greet\endcsname{7.33}
\expandafter\def\csname v@vint/silence/gtcrn/kind/babble/after\endcsname{8.64}
\expandafter\def\csname v@vint/silence/gtcrn/kind/babble/after-hi\endcsname{11.37}
\expandafter\def\csname v@vint/silence/gtcrn/kind/babble/after-lo\endcsname{5.94}
\expandafter\def\csname v@vint/silence/gtcrn/kind/babble/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/kind/babble/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/kind/babble/greet\endcsname{9.68}
\expandafter\def\csname v@vint/silence/gtcrn/kind/babble/greet-hi\endcsname{10.85}
\expandafter\def\csname v@vint/silence/gtcrn/kind/babble/greet-lo\endcsname{8.57}
\expandafter\def\csname v@vint/silence/gtcrn/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/silence/gtcrn/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/gtcrn/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/gtcrn/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/silence/gtcrn/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/gtcrn/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/gtcrn/kind/home/after\endcsname{3.49}
\expandafter\def\csname v@vint/silence/gtcrn/kind/home/after-hi\endcsname{5.38}
\expandafter\def\csname v@vint/silence/gtcrn/kind/home/after-lo\endcsname{1.80}
\expandafter\def\csname v@vint/silence/gtcrn/kind/home/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/kind/home/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/kind/home/greet\endcsname{2.80}
\expandafter\def\csname v@vint/silence/gtcrn/kind/home/greet-hi\endcsname{4.09}
\expandafter\def\csname v@vint/silence/gtcrn/kind/home/greet-lo\endcsname{1.57}
\expandafter\def\csname v@vint/silence/gtcrn/kind/music/after\endcsname{3.00}
\expandafter\def\csname v@vint/silence/gtcrn/kind/music/after-hi\endcsname{4.19}
\expandafter\def\csname v@vint/silence/gtcrn/kind/music/after-lo\endcsname{1.82}
\expandafter\def\csname v@vint/silence/gtcrn/kind/music/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/kind/music/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/kind/music/greet\endcsname{3.89}
\expandafter\def\csname v@vint/silence/gtcrn/kind/music/greet-hi\endcsname{5.99}
\expandafter\def\csname v@vint/silence/gtcrn/kind/music/greet-lo\endcsname{1.86}
\expandafter\def\csname v@vint/silence/gtcrn/kind/street/after\endcsname{3.52}
\expandafter\def\csname v@vint/silence/gtcrn/kind/street/after-hi\endcsname{4.94}
\expandafter\def\csname v@vint/silence/gtcrn/kind/street/after-lo\endcsname{2.03}
\expandafter\def\csname v@vint/silence/gtcrn/kind/street/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/kind/street/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/kind/street/greet\endcsname{1.38}
\expandafter\def\csname v@vint/silence/gtcrn/kind/street/greet-hi\endcsname{2.23}
\expandafter\def\csname v@vint/silence/gtcrn/kind/street/greet-lo\endcsname{0.56}
\expandafter\def\csname v@vint/silence/gtcrn/kind/talker/after\endcsname{10.22}
\expandafter\def\csname v@vint/silence/gtcrn/kind/talker/after-hi\endcsname{11.54}
\expandafter\def\csname v@vint/silence/gtcrn/kind/talker/after-lo\endcsname{8.89}
\expandafter\def\csname v@vint/silence/gtcrn/kind/talker/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/gtcrn/kind/talker/before/silence\endcsname{0.3}
\expandafter\def\csname v@vint/silence/gtcrn/kind/talker/greet\endcsname{23.18}
\expandafter\def\csname v@vint/silence/gtcrn/kind/talker/greet-hi\endcsname{24.76}
\expandafter\def\csname v@vint/silence/gtcrn/kind/talker/greet-lo\endcsname{21.70}
\expandafter\def\csname v@vint/silence/gtcrn/trig/down-p50\endcsname{5}
\expandafter\def\csname v@vint/silence/gtcrn/trig/n\endcsname{2382}
\expandafter\def\csname v@vint/silence/gtcrn/trig/over20\endcsname{1}
\expandafter\def\csname v@vint/silence/none/after\endcsname{2.42}
\expandafter\def\csname v@vint/silence/none/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/after/vad\endcsname{11.8}
\expandafter\def\csname v@vint/silence/none/all\endcsname{2.77}
\expandafter\def\csname v@vint/silence/none/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/before/vad\endcsname{18.3}
\expandafter\def\csname v@vint/silence/none/greet\endcsname{5.52}
\expandafter\def\csname v@vint/silence/none/kind/babble/after\endcsname{3.82}
\expandafter\def\csname v@vint/silence/none/kind/babble/after-hi\endcsname{6.33}
\expandafter\def\csname v@vint/silence/none/kind/babble/after-lo\endcsname{1.69}
\expandafter\def\csname v@vint/silence/none/kind/babble/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/babble/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/babble/greet\endcsname{5.63}
\expandafter\def\csname v@vint/silence/none/kind/babble/greet-hi\endcsname{7.27}
\expandafter\def\csname v@vint/silence/none/kind/babble/greet-lo\endcsname{4.02}
\expandafter\def\csname v@vint/silence/none/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/silence/none/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/none/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/none/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/silence/none/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/none/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/none/kind/home/after\endcsname{1.17}
\expandafter\def\csname v@vint/silence/none/kind/home/after-hi\endcsname{1.95}
\expandafter\def\csname v@vint/silence/none/kind/home/after-lo\endcsname{0.45}
\expandafter\def\csname v@vint/silence/none/kind/home/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/home/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/home/greet\endcsname{2.54}
\expandafter\def\csname v@vint/silence/none/kind/home/greet-hi\endcsname{4.14}
\expandafter\def\csname v@vint/silence/none/kind/home/greet-lo\endcsname{1.10}
\expandafter\def\csname v@vint/silence/none/kind/music/after\endcsname{0.07}
\expandafter\def\csname v@vint/silence/none/kind/music/after-hi\endcsname{0.13}
\expandafter\def\csname v@vint/silence/none/kind/music/after-lo\endcsname{0.02}
\expandafter\def\csname v@vint/silence/none/kind/music/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/music/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/music/greet\endcsname{0.80}
\expandafter\def\csname v@vint/silence/none/kind/music/greet-hi\endcsname{2.11}
\expandafter\def\csname v@vint/silence/none/kind/music/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/none/kind/street/after\endcsname{0.69}
\expandafter\def\csname v@vint/silence/none/kind/street/after-hi\endcsname{1.24}
\expandafter\def\csname v@vint/silence/none/kind/street/after-lo\endcsname{0.30}
\expandafter\def\csname v@vint/silence/none/kind/street/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/street/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/street/greet\endcsname{0.87}
\expandafter\def\csname v@vint/silence/none/kind/street/greet-hi\endcsname{1.53}
\expandafter\def\csname v@vint/silence/none/kind/street/greet-lo\endcsname{0.26}
\expandafter\def\csname v@vint/silence/none/kind/talker/after\endcsname{9.35}
\expandafter\def\csname v@vint/silence/none/kind/talker/after-hi\endcsname{10.38}
\expandafter\def\csname v@vint/silence/none/kind/talker/after-lo\endcsname{8.28}
\expandafter\def\csname v@vint/silence/none/kind/talker/after/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/talker/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/none/kind/talker/greet\endcsname{21.41}
\expandafter\def\csname v@vint/silence/none/kind/talker/greet-hi\endcsname{23.43}
\expandafter\def\csname v@vint/silence/none/kind/talker/greet-lo\endcsname{18.95}
\expandafter\def\csname v@vint/silence/none/trig/down-p50\endcsname{0}
\expandafter\def\csname v@vint/silence/none/trig/n\endcsname{1136}
\expandafter\def\csname v@vint/silence/none/trig/over20\endcsname{0}
\expandafter\def\csname v@vint/silence/rel/after\endcsname{0.50}
\expandafter\def\csname v@vint/silence/rel/after/silence\endcsname{69.4}
\expandafter\def\csname v@vint/silence/rel/after/vad\endcsname{1.2}
\expandafter\def\csname v@vint/silence/rel/all\endcsname{1.05}
\expandafter\def\csname v@vint/silence/rel/before/silence\endcsname{50.9}
\expandafter\def\csname v@vint/silence/rel/before/vad\endcsname{15.2}
\expandafter\def\csname v@vint/silence/rel/greet\endcsname{5.32}
\expandafter\def\csname v@vint/silence/rel/kind/babble/after\endcsname{0.31}
\expandafter\def\csname v@vint/silence/rel/kind/babble/after-hi\endcsname{0.64}
\expandafter\def\csname v@vint/silence/rel/kind/babble/after-lo\endcsname{0.04}
\expandafter\def\csname v@vint/silence/rel/kind/babble/after/silence\endcsname{61.4}
\expandafter\def\csname v@vint/silence/rel/kind/babble/before/silence\endcsname{42.5}
\expandafter\def\csname v@vint/silence/rel/kind/babble/greet\endcsname{4.93}
\expandafter\def\csname v@vint/silence/rel/kind/babble/greet-hi\endcsname{6.51}
\expandafter\def\csname v@vint/silence/rel/kind/babble/greet-lo\endcsname{3.25}
\expandafter\def\csname v@vint/silence/rel/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/silence/rel/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/rel/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/rel/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/silence/rel/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/rel/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/rel/kind/home/after\endcsname{0.24}
\expandafter\def\csname v@vint/silence/rel/kind/home/after-hi\endcsname{0.46}
\expandafter\def\csname v@vint/silence/rel/kind/home/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/silence/rel/kind/home/after/silence\endcsname{74.7}
\expandafter\def\csname v@vint/silence/rel/kind/home/before/silence\endcsname{59.3}
\expandafter\def\csname v@vint/silence/rel/kind/home/greet\endcsname{2.54}
\expandafter\def\csname v@vint/silence/rel/kind/home/greet-hi\endcsname{3.80}
\expandafter\def\csname v@vint/silence/rel/kind/home/greet-lo\endcsname{1.37}
\expandafter\def\csname v@vint/silence/rel/kind/music/after\endcsname{0.20}
\expandafter\def\csname v@vint/silence/rel/kind/music/after-hi\endcsname{0.41}
\expandafter\def\csname v@vint/silence/rel/kind/music/after-lo\endcsname{0.01}
\expandafter\def\csname v@vint/silence/rel/kind/music/after/silence\endcsname{74.9}
\expandafter\def\csname v@vint/silence/rel/kind/music/before/silence\endcsname{62.3}
\expandafter\def\csname v@vint/silence/rel/kind/music/greet\endcsname{1.50}
\expandafter\def\csname v@vint/silence/rel/kind/music/greet-hi\endcsname{2.59}
\expandafter\def\csname v@vint/silence/rel/kind/music/greet-lo\endcsname{0.55}
\expandafter\def\csname v@vint/silence/rel/kind/street/after\endcsname{0.02}
\expandafter\def\csname v@vint/silence/rel/kind/street/after-hi\endcsname{0.06}
\expandafter\def\csname v@vint/silence/rel/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/rel/kind/street/after/silence\endcsname{73.2}
\expandafter\def\csname v@vint/silence/rel/kind/street/before/silence\endcsname{66.5}
\expandafter\def\csname v@vint/silence/rel/kind/street/greet\endcsname{0.61}
\expandafter\def\csname v@vint/silence/rel/kind/street/greet-hi\endcsname{1.10}
\expandafter\def\csname v@vint/silence/rel/kind/street/greet-lo\endcsname{0.14}
\expandafter\def\csname v@vint/silence/rel/kind/talker/after\endcsname{2.53}
\expandafter\def\csname v@vint/silence/rel/kind/talker/after-hi\endcsname{4.33}
\expandafter\def\csname v@vint/silence/rel/kind/talker/after-lo\endcsname{1.05}
\expandafter\def\csname v@vint/silence/rel/kind/talker/after/silence\endcsname{60.1}
\expandafter\def\csname v@vint/silence/rel/kind/talker/before/silence\endcsname{29.6}
\expandafter\def\csname v@vint/silence/rel/kind/talker/greet\endcsname{20.52}
\expandafter\def\csname v@vint/silence/rel/kind/talker/greet-hi\endcsname{22.27}
\expandafter\def\csname v@vint/silence/rel/kind/talker/greet-lo\endcsname{18.74}
\expandafter\def\csname v@vint/silence/rel/trig/down-p50\endcsname{10}
\expandafter\def\csname v@vint/silence/rel/trig/n\endcsname{237}
\expandafter\def\csname v@vint/silence/rel/trig/over20\endcsname{16}
\expandafter\def\csname v@vint/silence/reuse/after\endcsname{0.24}
\expandafter\def\csname v@vint/silence/reuse/after/silence\endcsname{98.3}
\expandafter\def\csname v@vint/silence/reuse/after/vad\endcsname{1.1}
\expandafter\def\csname v@vint/silence/reuse/all\endcsname{0.95}
\expandafter\def\csname v@vint/silence/reuse/before/silence\endcsname{49.1}
\expandafter\def\csname v@vint/silence/reuse/before/vad\endcsname{17.7}
\expandafter\def\csname v@vint/silence/reuse/greet\endcsname{6.54}
\expandafter\def\csname v@vint/silence/reuse/kind/babble/after\endcsname{0.06}
\expandafter\def\csname v@vint/silence/reuse/kind/babble/after-hi\endcsname{0.14}
\expandafter\def\csname v@vint/silence/reuse/kind/babble/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/babble/after/silence\endcsname{99.9}
\expandafter\def\csname v@vint/silence/reuse/kind/babble/before/silence\endcsname{47.3}
\expandafter\def\csname v@vint/silence/reuse/kind/babble/greet\endcsname{8.45}
\expandafter\def\csname v@vint/silence/reuse/kind/babble/greet-hi\endcsname{11.99}
\expandafter\def\csname v@vint/silence/reuse/kind/babble/greet-lo\endcsname{5.13}
\expandafter\def\csname v@vint/silence/reuse/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/home/after\endcsname{0.04}
\expandafter\def\csname v@vint/silence/reuse/kind/home/after-hi\endcsname{0.10}
\expandafter\def\csname v@vint/silence/reuse/kind/home/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/home/after/silence\endcsname{99.9}
\expandafter\def\csname v@vint/silence/reuse/kind/home/before/silence\endcsname{51.3}
\expandafter\def\csname v@vint/silence/reuse/kind/home/greet\endcsname{4.37}
\expandafter\def\csname v@vint/silence/reuse/kind/home/greet-hi\endcsname{6.67}
\expandafter\def\csname v@vint/silence/reuse/kind/home/greet-lo\endcsname{2.16}
\expandafter\def\csname v@vint/silence/reuse/kind/music/after\endcsname{0.03}
\expandafter\def\csname v@vint/silence/reuse/kind/music/after-hi\endcsname{0.08}
\expandafter\def\csname v@vint/silence/reuse/kind/music/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/music/after/silence\endcsname{100.0}
\expandafter\def\csname v@vint/silence/reuse/kind/music/before/silence\endcsname{72.6}
\expandafter\def\csname v@vint/silence/reuse/kind/music/greet\endcsname{0.80}
\expandafter\def\csname v@vint/silence/reuse/kind/music/greet-hi\endcsname{1.66}
\expandafter\def\csname v@vint/silence/reuse/kind/music/greet-lo\endcsname{0.08}
\expandafter\def\csname v@vint/silence/reuse/kind/street/after\endcsname{0.02}
\expandafter\def\csname v@vint/silence/reuse/kind/street/after-hi\endcsname{0.05}
\expandafter\def\csname v@vint/silence/reuse/kind/street/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/reuse/kind/street/after/silence\endcsname{100.0}
\expandafter\def\csname v@vint/silence/reuse/kind/street/before/silence\endcsname{59.5}
\expandafter\def\csname v@vint/silence/reuse/kind/street/greet\endcsname{1.30}
\expandafter\def\csname v@vint/silence/reuse/kind/street/greet-hi\endcsname{2.00}
\expandafter\def\csname v@vint/silence/reuse/kind/street/greet-lo\endcsname{0.65}
\expandafter\def\csname v@vint/silence/reuse/kind/talker/after\endcsname{1.47}
\expandafter\def\csname v@vint/silence/reuse/kind/talker/after-hi\endcsname{2.89}
\expandafter\def\csname v@vint/silence/reuse/kind/talker/after-lo\endcsname{0.41}
\expandafter\def\csname v@vint/silence/reuse/kind/talker/after/silence\endcsname{89.0}
\expandafter\def\csname v@vint/silence/reuse/kind/talker/before/silence\endcsname{21.5}
\expandafter\def\csname v@vint/silence/reuse/kind/talker/greet\endcsname{21.70}
\expandafter\def\csname v@vint/silence/reuse/kind/talker/greet-hi\endcsname{23.80}
\expandafter\def\csname v@vint/silence/reuse/kind/talker/greet-lo\endcsname{19.67}
\expandafter\def\csname v@vint/silence/reuse/trig/down-p50\endcsname{5}
\expandafter\def\csname v@vint/silence/reuse/trig/n\endcsname{111}
\expandafter\def\csname v@vint/silence/reuse/trig/over20\endcsname{5}
\expandafter\def\csname v@vint/silence/voxlock/after\endcsname{0.65}
\expandafter\def\csname v@vint/silence/voxlock/after/silence\endcsname{2.6}
\expandafter\def\csname v@vint/silence/voxlock/after/vad\endcsname{1.8}
\expandafter\def\csname v@vint/silence/voxlock/all\endcsname{1.18}
\expandafter\def\csname v@vint/silence/voxlock/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/voxlock/before/vad\endcsname{16.4}
\expandafter\def\csname v@vint/silence/voxlock/greet\endcsname{5.35}
\expandafter\def\csname v@vint/silence/voxlock/kind/babble/after\endcsname{0.55}
\expandafter\def\csname v@vint/silence/voxlock/kind/babble/after-hi\endcsname{0.98}
\expandafter\def\csname v@vint/silence/voxlock/kind/babble/after-lo\endcsname{0.17}
\expandafter\def\csname v@vint/silence/voxlock/kind/babble/after/silence\endcsname{0.1}
\expandafter\def\csname v@vint/silence/voxlock/kind/babble/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/voxlock/kind/babble/greet\endcsname{5.63}
\expandafter\def\csname v@vint/silence/voxlock/kind/babble/greet-hi\endcsname{7.29}
\expandafter\def\csname v@vint/silence/voxlock/kind/babble/greet-lo\endcsname{3.95}
\expandafter\def\csname v@vint/silence/voxlock/kind/clean/after\endcsname{0.00}
\expandafter\def\csname v@vint/silence/voxlock/kind/clean/after-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/voxlock/kind/clean/after-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/voxlock/kind/clean/greet\endcsname{0.00}
\expandafter\def\csname v@vint/silence/voxlock/kind/clean/greet-hi\endcsname{0.00}
\expandafter\def\csname v@vint/silence/voxlock/kind/clean/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/voxlock/kind/home/after\endcsname{0.35}
\expandafter\def\csname v@vint/silence/voxlock/kind/home/after-hi\endcsname{0.54}
\expandafter\def\csname v@vint/silence/voxlock/kind/home/after-lo\endcsname{0.19}
\expandafter\def\csname v@vint/silence/voxlock/kind/home/after/silence\endcsname{2.1}
\expandafter\def\csname v@vint/silence/voxlock/kind/home/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/voxlock/kind/home/greet\endcsname{2.54}
\expandafter\def\csname v@vint/silence/voxlock/kind/home/greet-hi\endcsname{4.14}
\expandafter\def\csname v@vint/silence/voxlock/kind/home/greet-lo\endcsname{1.10}
\expandafter\def\csname v@vint/silence/voxlock/kind/music/after\endcsname{0.10}
\expandafter\def\csname v@vint/silence/voxlock/kind/music/after-hi\endcsname{0.18}
\expandafter\def\csname v@vint/silence/voxlock/kind/music/after-lo\endcsname{0.02}
\expandafter\def\csname v@vint/silence/voxlock/kind/music/after/silence\endcsname{3.2}
\expandafter\def\csname v@vint/silence/voxlock/kind/music/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/voxlock/kind/music/greet\endcsname{0.80}
\expandafter\def\csname v@vint/silence/voxlock/kind/music/greet-hi\endcsname{2.11}
\expandafter\def\csname v@vint/silence/voxlock/kind/music/greet-lo\endcsname{0.00}
\expandafter\def\csname v@vint/silence/voxlock/kind/street/after\endcsname{0.15}
\expandafter\def\csname v@vint/silence/voxlock/kind/street/after-hi\endcsname{0.25}
\expandafter\def\csname v@vint/silence/voxlock/kind/street/after-lo\endcsname{0.05}
\expandafter\def\csname v@vint/silence/voxlock/kind/street/after/silence\endcsname{0.7}
\expandafter\def\csname v@vint/silence/voxlock/kind/street/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/voxlock/kind/street/greet\endcsname{0.87}
\expandafter\def\csname v@vint/silence/voxlock/kind/street/greet-hi\endcsname{1.53}
\expandafter\def\csname v@vint/silence/voxlock/kind/street/greet-lo\endcsname{0.26}
\expandafter\def\csname v@vint/silence/voxlock/kind/talker/after\endcsname{3.04}
\expandafter\def\csname v@vint/silence/voxlock/kind/talker/after-hi\endcsname{4.97}
\expandafter\def\csname v@vint/silence/voxlock/kind/talker/after-lo\endcsname{1.42}
\expandafter\def\csname v@vint/silence/voxlock/kind/talker/after/silence\endcsname{8.6}
\expandafter\def\csname v@vint/silence/voxlock/kind/talker/before/silence\endcsname{0.0}
\expandafter\def\csname v@vint/silence/voxlock/kind/talker/greet\endcsname{20.42}
\expandafter\def\csname v@vint/silence/voxlock/kind/talker/greet-hi\endcsname{22.26}
\expandafter\def\csname v@vint/silence/voxlock/kind/talker/greet-lo\endcsname{18.15}
\expandafter\def\csname v@vint/silence/voxlock/trig/down-p50\endcsname{9}
\expandafter\def\csname v@vint/silence/voxlock/trig/n\endcsname{305}
\expandafter\def\csname v@vint/silence/voxlock/trig/over20\endcsname{13}
\expandafter\def\csname v@vint/trace/after/len\endcsname{20}
\expandafter\def\csname v@vint/trace/after/none/cutin-at\endcsname{51.5}
\expandafter\def\csname v@vint/trace/after/none/fi-at\endcsname{56.6}
\expandafter\def\csname v@vint/trace/after/snr\endcsname{0}
\expandafter\def\csname v@vint/trace/greet/first-on\endcsname{5.3}
\expandafter\def\csname v@vint/trace/greet/rel/fi-at\endcsname{3.3}
\expandafter\def\csname v@vint/trace/greet/rel/switched\endcsname{3}
\expandafter\def\csname v@vint/trace/greet/rel_vb/switched\endcsname{6}
\expandafter\def\csname v@vint/trace/greet/snr\endcsname{10}
\expandafter\def\csname v@vint/voxlock/caught\endcsname{82.5}
\expandafter\def\csname v@vint/voxlock/caught-d\endcsname{-7.4}
\expandafter\def\csname v@vint/voxlock/caught-dabs\endcsname{7.4}
\expandafter\def\csname v@vint/voxlock/caught-dhi\endcsname{-3.6}
\expandafter\def\csname v@vint/voxlock/caught-dlo\endcsname{-11.7}
\expandafter\def\csname v@vint/voxlock/caught-hi\endcsname{86.4}
\expandafter\def\csname v@vint/voxlock/caught-lo\endcsname{78.1}
\expandafter\def\csname v@vint/voxlock/core-pct\endcsname{220}
\expandafter\def\csname v@vint/voxlock/cores\endcsname{2.20}
\expandafter\def\csname v@vint/voxlock/fi\endcsname{1.18}
\expandafter\def\csname v@vint/voxlock/fi-d\endcsname{+0.13}
\expandafter\def\csname v@vint/voxlock/fi-dabs\endcsname{0.13}
\expandafter\def\csname v@vint/voxlock/fi-dhi\endcsname{+0.24}
\expandafter\def\csname v@vint/voxlock/fi-dlo\endcsname{+0.03}
\expandafter\def\csname v@vint/voxlock/fi-hi\endcsname{1.65}
\expandafter\def\csname v@vint/voxlock/fi-lo\endcsname{0.78}
\expandafter\def\csname v@vint/voxlock/frame-p50\endcsname{33.6}
\expandafter\def\csname v@vint/voxlock/frame-p99\endcsname{53.4}
\expandafter\def\csname v@vint/voxlock/fs\endcsname{1.34}
\expandafter\def\csname v@vint/voxlock/fs-d\endcsname{+0.11}
\expandafter\def\csname v@vint/voxlock/fs-dabs\endcsname{0.11}
\expandafter\def\csname v@vint/voxlock/fs-dhi\endcsname{+0.20}
\expandafter\def\csname v@vint/voxlock/fs-dlo\endcsname{+0.02}
\expandafter\def\csname v@vint/voxlock/fs-hi\endcsname{1.88}
\expandafter\def\csname v@vint/voxlock/fs-lo\endcsname{0.86}
\expandafter\def\csname v@vint/voxlock/held\endcsname{12.7}
\expandafter\def\csname v@vint/voxlock/held-d\endcsname{+9.2}
\expandafter\def\csname v@vint/voxlock/held-dabs\endcsname{9.2}
\expandafter\def\csname v@vint/voxlock/held-dhi\endcsname{+13.7}
\expandafter\def\csname v@vint/voxlock/held-dlo\endcsname{+5.3}
\expandafter\def\csname v@vint/voxlock/held-hi\endcsname{17.2}
\expandafter\def\csname v@vint/voxlock/held-lo\endcsname{8.6}
\expandafter\def\csname v@vint/voxlock/kind/babble/fi\endcsname{1.13}
\expandafter\def\csname v@vint/voxlock/kind/babble/fs\endcsname{1.18}
\expandafter\def\csname v@vint/voxlock/kind/babble/missed\endcsname{2.0}
\expandafter\def\csname v@vint/voxlock/kind/clean/fi\endcsname{0.00}
\expandafter\def\csname v@vint/voxlock/kind/clean/fs\endcsname{0.00}
\expandafter\def\csname v@vint/voxlock/kind/clean/missed\endcsname{0.0}
\expandafter\def\csname v@vint/voxlock/kind/home/fi\endcsname{0.59}
\expandafter\def\csname v@vint/voxlock/kind/home/fs\endcsname{0.65}
\expandafter\def\csname v@vint/voxlock/kind/home/missed\endcsname{10.2}
\expandafter\def\csname v@vint/voxlock/kind/music/fi\endcsname{0.17}
\expandafter\def\csname v@vint/voxlock/kind/music/fs\endcsname{0.24}
\expandafter\def\csname v@vint/voxlock/kind/music/missed\endcsname{17.6}
\expandafter\def\csname v@vint/voxlock/kind/street/fi\endcsname{0.22}
\expandafter\def\csname v@vint/voxlock/kind/street/fs\endcsname{0.19}
\expandafter\def\csname v@vint/voxlock/kind/street/missed\endcsname{5.5}
\expandafter\def\csname v@vint/voxlock/kind/talker/fi\endcsname{5.35}
\expandafter\def\csname v@vint/voxlock/kind/talker/fs\endcsname{4.45}
\expandafter\def\csname v@vint/voxlock/kind/talker/missed\endcsname{0.6}
\expandafter\def\csname v@vint/voxlock/live/barge_p50\endcsname{0.76}
\expandafter\def\csname v@vint/voxlock/live/caught\endcsname{77.7}
\expandafter\def\csname v@vint/voxlock/live/eot_p50\endcsname{0.97}
\expandafter\def\csname v@vint/voxlock/live/eot_p90\endcsname{1.97}
\expandafter\def\csname v@vint/voxlock/live/fi_transcript\endcsname{3.37}
\expandafter\def\csname v@vint/voxlock/live/fi_vad\endcsname{0.89}
\expandafter\def\csname v@vint/voxlock/live/frame-p50\endcsname{39.2}
\expandafter\def\csname v@vint/voxlock/live/frame-p99\endcsname{55.1}
\expandafter\def\csname v@vint/voxlock/live/fs\endcsname{1.48}
\expandafter\def\csname v@vint/voxlock/live/no_reply\endcsname{15.4}
\expandafter\def\csname v@vint/voxlock/live/unfiltered_pct\endcsname{0.00}
\expandafter\def\csname v@vint/voxlock/missed\endcsname{6.8}
\expandafter\def\csname v@vint/voxlock/missed-d\endcsname{+6.1}
\expandafter\def\csname v@vint/voxlock/missed-dabs\endcsname{6.1}
\expandafter\def\csname v@vint/voxlock/missed-dhi\endcsname{+9.4}
\expandafter\def\csname v@vint/voxlock/missed-dlo\endcsname{+3.3}
\expandafter\def\csname v@vint/voxlock/missed-hi\endcsname{10.0}
\expandafter\def\csname v@vint/voxlock/missed-lo\endcsname{4.0}
\expandafter\def\csname v@vint/voxlock/recall\endcsname{82.8}
\expandafter\def\csname v@vint/voxlock/snr/0.0/fi\endcsname{2.15}
\expandafter\def\csname v@vint/voxlock/snr/10.0/fi\endcsname{1.16}
\expandafter\def\csname v@vint/voxlock/snr/20.0/fi\endcsname{0.56}
\expandafter\def\csname v@vint/voxlock/snr/None/fi\endcsname{0.00}
\expandafter\def\csname v@vint/voxlock/wer\endcsname{17.0}
\expandafter\def\csname v@vint/voxlock/wer/babble\endcsname{20.2}
\expandafter\def\csname v@vint/voxlock/wer/clean\endcsname{1.1}
\expandafter\def\csname v@vint/voxlock/wer/home\endcsname{17.7}
\expandafter\def\csname v@vint/voxlock/wer/music\endcsname{21.4}
\expandafter\def\csname v@vint/voxlock/wer/street\endcsname{13.5}
\expandafter\def\csname v@vint/voxlock/wer/talker\endcsname{17.9}
\expandafter\def\csname v@vint/voxlock8/core-pct\endcsname{129}
\expandafter\def\csname v@vint/voxlock8/cores\endcsname{1.29}
\expandafter\def\csname v@vint/voxlock8/frame-p50\endcsname{21.7}
\expandafter\def\csname v@vint/voxlock8/frame-p99\endcsname{33.2}
\expandafter\def\csname v@vint/voxlock8/live/barge_p50\endcsname{0.71}
\expandafter\def\csname v@vint/voxlock8/live/caught\endcsname{86.3}
\expandafter\def\csname v@vint/voxlock8/live/eot_p50\endcsname{0.82}
\expandafter\def\csname v@vint/voxlock8/live/eot_p90\endcsname{1.59}
\expandafter\def\csname v@vint/voxlock8/live/fi_transcript\endcsname{4.52}
\expandafter\def\csname v@vint/voxlock8/live/fi_vad\endcsname{0.96}
\expandafter\def\csname v@vint/voxlock8/live/frame-p50\endcsname{26.6}
\expandafter\def\csname v@vint/voxlock8/live/frame-p99\endcsname{46.0}
\expandafter\def\csname v@vint/voxlock8/live/fs\endcsname{1.55}
\expandafter\def\csname v@vint/voxlock8/live/no_reply\endcsname{12.5}
\expandafter\def\csname v@vint/voxlock8/live/unfiltered_pct\endcsname{0.00}
\makeatother

